Achieving Starvation-Freedom with Greater Concurrency in Multi-Version Object-based Transactional Memory Systems

To utilize the multi-core processors properly concurrent programming is needed. Concurrency control is the main challenge while designing a correct and efficient concurrent program. Software Transactional Memory Systems (STMs) provides ease of multithreading to the programmer without worrying about concurrency issues such as deadlock, livelock, priority inversion, etc. Most of the STMs works on read-write operations known as RWSTMs. Some STMs work at high-level operations and ensure greater concurrency than RWSTMs. Such STMs are known as Object-Based STMs (OSTMs). The transactions of OSTMs can return commit or abort. Aborted OSTMs transactions retry. But in the current setting of OSTMs, transactions may starve. So, we proposed a Starvation-Free OSTM (SF-OSTM) which ensures starvation-freedom in object based STM systems while satisfying the correctness criteria as co-opacity. Databases, RWSTMs and OSTMs say that maintaining multiple versions corresponding to each key of transaction reduces the number of aborts and improves the throughput. So, to achieve greater concurrency, we proposed Starvation-Free Multi-Version OSTM (SF-MVOSTM) which ensures starvation-freedom while storing multiple versions corresponding to each key and satisfies the correctness criteria such as local opacity. To show the performance benefits, We implemented three variants of SF-MVOSTM (SF-MVOSTM, SF-MVOSTM-GC and SF-KOSTM) and compared it with state-of-the-art STMs.

==> Arxiv SFKOSTM SSS19/ap-correctness.tex <==
\section{Liveness Proof of SF-SVOSTM and SF-KOSTM}
\label{apn:ap-cc}
This section describes the liveness proof of SF-SVOSTM and SF-KOSTM. Both the algorithms ensures starvation-freedom as the progress guarantee.
\subsection{Liveness Proof of SF-SVOSTM}
\label{subsec:LP}

\paragraph{Proof Notations:} Following the notion derived for SF-SVOSTM algorithm, we assume that all the histories accepted by SF-SVOSTM algorithm as \emph{\gen{SF-SVOSTM}}. This subsection considers only histories that are generated by SF-SVOSTM unless explicitly stated otherwise. For simplicity, we consider the sequential histories for our discussion and we can get the sequential history using the linearization points (or LPs) as \emph{first unlocking point of each successful method}.

Let us consider a transaction $T_i$ from the history $H$ \emph{\gen{SF-SVOSTM}}. Each transaction $T_i$ maintains $\langle its_i, cts_i\rangle$. % If $T_i$ is the first incarnation then its \emph{Initial Timestamp (its)} and \emph{Current Timestamp (cts)} are same as $i$. We represent the $\langle its, cts\rangle$ as $\langle its_i, cts_i\rangle$ for transaction $T_i$. If $T_i$ is aborted then thread $Th_i$ executes it again with new incarnation of $T_i$ until $T_i$ commits. Let the new incarnation of $T_i$ say $T_j$ then thread $Th_i$ maintain its $\langle its, cts \rangle$ as $\langle its_i, cts_j \rangle$. $Th_i$ stores the first incarnation $its_i$ of $T_i$ to set the reincarnation $its_j$ of $T_j$ is same as $its_i$.
 The value of $cts$ is assigned atomically with the help of atomic global counter $gcounter$. So, we use $gcounter$ to approximate the system time.


Apart from these $cts_i$ and $its_i$ transaction $T_i$ maintains $lock$ and $status$. $T_i$ acquires the $lock$ on the keys before accessing it. $status$ can be $\langle live, false, commit \rangle$.  The value of $lock$ and $status$ field change as the execution proceeds. For the sake of understanding, we represent
 the timestamps of a transaction $T_i$ corresponding to history $H$ as $\htits{i}{H}$ and $\htcts{i}{H}$.
 
 To satisfy the \stfdm for SF-SVOSTM, We assumed bounded termination for the fair scheduler as described \asmref{bdtm} in \subsecref{prelim}. In the proposed algorithms, we have considered \emph{TB} as the maximum time-bound of a transaction $T_i$ within this either $T_i$ will return commit or abort in the absence of deadlock. We consider an assumption about the transactions of the system as described \asmref{self} in \subsecref{prelim} which will help to achieve and prove about the starvation-freedom of SF-SVOSTM.

\begin{theorem}
	SF-SVOSTM ensures starvation-freedom in presence of a fair scheduler that satisfies \asmref{bdtm}(bounded-termination) and in the absence of parasitic transactions that satisfies \asmref{self}.
\end{theorem}

\begin{proof}
	Consider any history $H$ generated by SF-SVOSTM algorithm with transaction $T_i$.  Initially, thread $Th_i$ calls \tbeg{()} for $T_i$ which maintains $\langle \emph{its, cts}\rangle$ and set the $status$ as $live$. If $T_i$ is the first incarnation then its \emph{Initial Timestamp (its)} and \emph{Current Timestamp (cts)} are same as $i$. We represent the $\langle its, cts\rangle$ as $\langle its_i, cts_i\rangle$ for transaction $T_i$. If $T_i$ is aborted then thread $Th_i$ executes it again with new incarnation of $T_i$ until $T_i$ commits. Let the new incarnation of $T_i$ say $T_j$ then thread $Th_i$ maintain its $\langle its, cts \rangle$ as $\langle its_i, cts_j \rangle$. $Th_i$ stores the first incarnation $its_i$ of $T_i$ to set the reincarnation $its_j$ of $T_j$ is same as $its_i$. The value of $cts$ is incremented atomically with the help of atomic global counter $gcounter$. So, we use $gcounter$ to approximate the system time. 
	
	Through  \asmref{bdtm}, we can say that $T_i$ will terminate ($\commit$ or $\abort$) in bounded time. If $T_i$ returns abort then $T_i$ will retry again with new incarnation of $T_i$, say $T_j$ while satisfying the \asmref{self}. The incarnation of $T_i$ transaction as $\langle its_i, cts_j \rangle$. So, it can be seen that, $T_i$ will get the lowest $its$ in the system and achieve the highest priority. Eventually, $T_i$ returns commit. Similarly, all the transactions of the $H$ generated by SF-SVOSTM will eventually commit. Hence, SF-SVOSTM ensures starvation-freedom.
\end{proof}

%Please find the detailed proof of liveness of SF-SVOSTM in accompanying technical report \cite{Juyal+:CORR:SF-MVOSTM:2019}.


\subsection{Liveness Proof of SF-KOSTM}
\label{subsec:LPK}

\paragraph{Proof Notations:}  It follows the notion derived for SF-KOSTM algorithm, we assume that all the histories accepted by SF-KOSTM algorithm as \emph{\gen{SF-KOSTM}}. This sub-section considers only histories that are generated by SF-KOSTM unless explicitly stated otherwise. For simplicity, we consider the sequential histories for our discussion and we can get the sequential history using the linearization points (or LPs) as \emph{first unlocking point of each successful method}.

The notions of SF-KOSTM is the extension of proof notion defined above for SF-SVOSTM. A transaction $T_i$ of a history $H$ generated by SF-KOSTM execute \tbeg{()} and obtained $wts$ along with $cts$, $its$ used in SF-SVOSTM. So, a transaction $T_i$ of SF-KOSTM maintains three timestamps as $its_i$, $cts_i$, and $wts_i$. The value of $cts_i$ is assigned atomically with the help of atomic global counter $gcounter$. So, we use $gcounter$ to approximate the system time. To achieve the highest $cts_i$, we use $wts_i$ which is significantly larger than $cts_i$ as defined in \subsecref{working}. Along with this SF-KOSTM maintains $tltl$ and $tutl$ corresponding to each transaction $T_i$ as $tltl_i$ and $tutl_i$ to maintain the real-time order.


Apart from these timestamps, transaction $T_i$ maintains $lock$, $vrt$ and $status$. $T_i$ acquires the $lock$ on the keys before accessing it. $vrt$ stands for \emph{version real time} order which helps to maintain the real-time order among the transactions. $status$ can be $\langle live, false, commit \rangle$ same as SF-SVOSTM.  The value of $lock$, $vrt$ and $status$ field change as the execution proceeds. So, we denote them as $\htlock{i}{H}, \htval{i}{H}, \htstat{i}{H}$. Sometimes, we also denote them based on the context of transaction $T_i$ while ignoring $H$ as $\tlock{i}, \tval{i}, \tstat{i}$. For the sake of understanding, we represent
the timestamps of a transaction $T_i$ corresponding to history $H$ as $\htits{i}{H}$, $\htcts{i}{H}$, and $\htwts{i}{H}$ along with  $\htltl{i}{H}, \htutl{i}{H}$.

We use $gcounter$ to approximate the system time. We denote the \syst of history $H$ as the value of $gcounter$ immediately after the last event of $H$. Here, we assume the value of $C$, used to derive the $wts$ as 0.1 in the arguments because on results $C$ as 0.1 performs best. But its not compulsory to keep it 0.1, it can be any value greater than 0 to prove the correctness of SF-KOSTM. 



%The other variables that a transaction maintains are: \ltl, \utl, \lock, \val, \stat. These values change as the execution proceeds. Hence, we denote them as: $\htltl{i}{H}, \htutl{i}{H},\\ \htlock{i}{H}, \htval{i}{H}, \htstat{i}{H}$. 
%These represent the values of \ltl, \utl, \lock, \val, \stat after the execution of last event in $H$. Depending on the context, we sometimes ignore $H$ and denote them only as: $\tlock{i}, \tval{i}, \tstat{i}, \ttltl{i}, \ttutl{i}$.

%We approximate the system time with the value of $gcounter$. We denote the \syst of history $H$ as the value of $gcounter$ immediately after the last event of $H$. Further, we also assume that the value of $C$ is 0.1 in our arguments. But, it can be seen that the proof will work for any value greater than 0 as well. 


The counter application invokes transactions in such a way that if the current $T_i$ transaction aborts, it invokes a new transaction $T_j$ with the same $its$. We say that $T_i$ is an \emph{\inc} of $T_j$ in a history $H$ if $\htits{i}{H} = \htits{j}{H}$. Thus the multiple \inc{s} of a transaction $T_i$ get invoked by the application until an \inc finally commits. 

To capture this notion of multiple transactions with the same $its$, we define \emph{\incset} (incarnation set) of $T_i$ in $H$ as the set of all the transactions in $H$ which have the same $its$ as $T_i$ and includes $T_i$ as well. Formally, 
\begin{equation*}
\incs{i}{H} = \{T_j|(T_i = T_j) \lor (\htits{i}{H} = \htits{j}{H})\}  
\end{equation*}

Note that from this definition of  \incset, we implicitly get that $T_i$ and all the transactions in its \incset of $H$ also belong to $H$. Formally, $\incs{i}{H} \in \txns{H}$. 

The application invokes different incarnations of a transaction $T_i$ in such a way that as long as an \inc is live, it does not invoke the next \inc. It invokes the next \inc after the current \inc has got aborted. Once an \inc of $T_i$ has committed, it can not have any future \inc{s}. Thus, the application views all the \inc{s} of a transaction as a single \emph{\aptr}. 

We assign \emph{\incn{s}} to all the transactions that have the same $its$. We say that a transaction $T_i$ starts \emph{afresh}, if $\inum{i}$ is 1. We say that $T_i$ is the \ninc of $T_i$ if $T_j$ and $T_i$ have the same $its$ and $T_i$'s \incn is $T_j$'s \incn + 1. Formally, $\langle (\nexti{i} = T_j) \equiv (\tits{i} = \tits{j}) \land (\inum{i} = \inum{j} + 1)\rangle$


As mentioned the objective of the application is to ensure that every \aptr eventually commits. Thus, the applications views the entire \incset as a single \aptr (with all the transactions in the \incset having the same $its$). We can say that an \aptr has committed if in the corresponding \incset a transaction in eventually commits. For $T_i$ in a history $H$, we denote this by a boolean value \incct (incarnation set committed) which implies that either $T_i$ or an \inc of $T_i$ has committed. Formally, we define it as $\inct{i}{H}$

\begin{equation*}
\inct{i}{H} = \begin{cases}
True  & (\exists T_j: (T_j \in \incs{i}{H}) \\ & \land (T_j \in \comm{H}))\\
False & \text{otherwise}
\end{cases}
\end{equation*}


\cmnt{
It can be seen that SF-KOSTM algorithm gives preference to transactions with lower $its$ to commit. To understand this notion of preference, we define a few notions of enablement of a transaction $T_i$ in a history $H$. We start with the definition of \emph{\itsen} as:

\begin{definition}
	\label{defn:itsen}
	We say $T_i$ is \emph{\itsen} in $H$ if for all transactions $T_j$ with $its$ lower than $its$ of $T_i$ in $H$ have \incct to be true. Formally, 
	\begin{equation*}
	\itsenb{i}{H} = \begin{cases}
	True    & (T_i \in \live{H}) \land (\forall T_j \in \txns{H} :\\ & (\htits{j}{H} < \htits{i}{H}) \implies (\inct{j}{H})) \\
	False	& \text{otherwise}
	\end{cases}
	\end{equation*}
\end{definition}

The interesting key insight of any transaction $T_i$ is such that a transaction $T_i$ with lowest $its_i$ and highest $wts_i$ will returns commit. If an \itsen transaction $T_i$ aborts then it is because of another transaction $T_j$ with $wts$ higher than $T_i$ has committed. To precisely capture this, we define two more notions of a transaction being enabled \emph{\cdsen} and \emph{\finen}. To define these notions of enabled, we in turn define a few other auxiliary notions. We start with \emph{\affset},
\begin{equation*}
\haffset{i}{H} = \{T_j|(T_j \in \txns{H}) \land (\htits{j}{H} < \htits{i}{H} + 2*TB)\}
\end{equation*}

From the description of SF-KOSTM algorithm, it can be seen that a transaction $T_i$'s commit can depend on committing of transactions (or their \inc{s}) which have their $its$ less than $its$ of $T_i$ + $2*TB$, which is $T_i$'s \affset. We capture this notion of dependency for a transaction $T_i$ in a history $H$ as \emph{commit dependent set} or \emph{\cdset} as: the set of all transactions $T_j$ in $T_i$'s \affset that do not any \inc that is committed yet, i.e., not yet have their \incct flag set as true. Formally, 

\begin{equation*}
\hcds{i}{H} = \{T_j| (T_j \in \haffset{i}{H}) \land (\neg\inct{j}{H}) \}
\end{equation*}

\noindent Based on this definition of \cdset, we next define the notion of \cdsen. Once the transaction $T_i$ is \cdsen, it will eventually commit.

\begin{definition}
	\label{defn:cdsen}
	We say that transaction $T_i$ is \emph{\cdsen} if the following conditions hold true (1) $T_i$ is live in $H$; (2) $cts$ of $T_i$ is greater than or equal to $its$ of $T_i$ + $2*TB$; (3) \cdset of $T_i$ is empty, i.e., for all transactions $T_j$ in $H$ with $its$ lower than $its$ of  $T_i$ + $2*TB$ in $H$ have their \incct to be true. Formally, 
	
	\begin{equation*}
	\hspace{-.3cm} \cdsenb{i}{H} = \begin{cases}
	True    & (T_i \in \live{H}) \land (\htcts{i}{H} \geq  \htits{i}{H} + 2*TB) \\ & \land (\hcds{i}{H} = \phi) \\
	%& (\forall T_j \in \txns{H} : (\htits{j}{H} < \htits{i}{H} + 2*TB) \implies (\inct{j}{H})) \\
	False	& \text{otherwise}
	\end{cases}
	\end{equation*}
\end{definition}

\begin{definition}
	\label{defn:finen}
	We say that transaction $T_i$ is \emph{\finen} if the following conditions hold true (1) $T_i$ is live in $H$; (2) $T_i$ is \cdsen is $H$; (3) $\htwts{j}{H}$ is greater than $\haffwts{i}{H}$. Formally, 
	
	\begin{equation*}
	\finenb{i}{H} = \begin{cases}
	True    & (T_i \in \live{H}) \land (\cdsenb{i}{H}) \\ & \land (\htwts{j}{H} > \haffwts{i}{H}) \\
	False	& \text{otherwise}
	\end{cases}
	\end{equation*}
\end{definition}


\begin{theorem}
	\label{thm:hwtm-com}
	Consider a history $H1$ with $T_i$ be a transaction in $\live{H1}$. Then there is an extension of $H1$, $H2$ in which an \inc of $T_i$, $T_j$ is committed. Formally, $\langle H1, T_i: (T_i\in \live{H}) \implies (\exists T_j, H2: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land (T_j \in \comm{H2})) \rangle$. 
\end{theorem}

\begin{proof}
	%Induction on \its. 
	Here we show the states that a transaction $T_i$ (or one of it its \inc{s}) undergoes before it commits. In all these transitions, it is possible that an \inc of $T_i$ can commit. But to show the worst case, we assume that no \inc of $T_i$ commits. Continuing with this argument, we show that finally an \inc of $T_i$ commits. 
	
	Consider a live transaction $T_i$ in $H1$. Then we get that there is a history $H2$, which is an extension of $H1$, in which $T_j$ an \inc of $T_i$ is either committed or \itsen. If $T_j$ is \itsen in $H2$, then we get that $T_k$, an \inc of $T_j$, will be \cdsen in a extension of $H2$, $H3$ (assuming that $T_k$ is not committed in $H3$). 
	
	We get that there is an extension of $H3$, $H4$ in which an \inc of $T_k$, $T_l$ will be \finen assuming that it is not committed in $H4$. Finally, we get that there is an extension of $H4$ in which $T_m$, an \inc of $T_l$, will be committed. This proves our theorem.
\end{proof}

\noindent From this theorem, we get the following corollary which states that any history generated by SF-KOSTM ensures $\stfdm$ while satisfying the \asmref{bdtm} and \asmref{self}.


\begin{corollary}
	SF-KOSTM ensures starvation-freedom in presence of a fair scheduler that satisfies \asmref{bdtm}(bounded-termination) and in the absence of parasitic transactions that satisfies \asmref{self}.
\end{corollary}

\noindent
Please find the detailed proof of liveness of SF-KOSTM in accompanying technical report \cite{Juyal+:CORR:SF-MVOSTM:2019}.
}

\noindent From the definition of \incct we get the following observations \& lemmas about a transaction $T_i$

\begin{observation}
	\label{obs:inct-term}
	Consider a transaction $T_i$ in a history $H$ with its \incct being true in $H$. Then $T_i$ is terminated (either committed or aborted) in $H$. Formally, $\langle H, T_i: (T_i \in \txns{H}) \land (\inct{i}{H}) \implies (T_i \in \termed{H}) \rangle$. 
\end{observation}

\begin{observation}
	\label{obs:inct-fut}
	Consider a transaction $T_i$ in a history $H$ with its \incct being true in $H1$. Let $H2$ be a extension of $H1$ with a transaction $T_j$ in it. Suppose $T_j$ is an \inc of $T_i$. Then $T_j$'s \incct is true in $H2$. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land (\inct{i}{H1}) \land (T_j \in \txns{H2}) \land (T_i \in \incs{j}{H2})\implies (\inct{j}{H2}) \rangle$. 
\end{observation}

\begin{lemma}
	\label{lem:inct-diff}
	Consider a history $H1$ with a strict extension $H2$. Let $T_i$ \& $T_j$ be two transactions in $H1$ \& $H2$ respectively. Let $T_j$ not be in $H1$. Suppose $T_i$'s \incct is true. Then \its of $T_i$ cannot be the same as \its of $T_j$. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubset H2) \land (\inct{i}{H1}) \land (T_j \in \txns{H2}) \land (T_j \notin \txns{H1}) \implies (\htits{i}{H1} \neq \htits{j}{H2}) \rangle$.
\end{lemma}


\begin{proof}
	Here, we have that $T_i$'s \incct is true in $H1$. Suppose $T_j$ is an \inc of $T_i$, i.e., their \its{s} are the same. We are given that $T_j$ is not in $H1$. This implies that $T_j$ must have started after the last event of $H1$. 
	
	We are also given that $T_i$'s \incct is true in $H1$. This implies that an \inc of $T_i$ or $T_i$ itself has committed in $H1$. After this commit, the application will not invoke another transaction with the same \its as $T_i$. Thus, there cannot be a transaction after the last event of $H1$ and in any extension of $H1$ with the same \its of $T_1$. Hence, $\htits{i}{H1}$ cannot be same as $\htits{j}{H2}$. 
\end{proof}

Now we show the liveness with the following observations, lemmas \& theorems. We start with two observations about that histories of which one is an extension of the other. The following states that for any history, there exists an extension. In other words, we assume that the STM system runs forever and does not terminate. This is required for showing that every transaction eventually commits. 

\begin{observation}
	\label{obs:hist-future}
	Consider a history $H1$ generated by \gen{\ksftm}. Then there is a history $H2$ in \gen{\ksftm} such that $H2$ is a strict extension of $H1$. Formally, $\langle \forall H1: (H1 \in \gen{\ksftm}) \implies (\exists H2: (H2 \in \gen{SF-KOSTM}) \land (H1 \sqsubset H2) \rangle$. 
\end{observation}

\noindent The follow observation is about the transaction in a history and any of its extensions. 

\begin{observation}
	\label{obs:hist-subset}
	Given two histories $H1$ \& $H2$ such that $H2$ is an extension of $H1$. Then, the set of transactions in $H1$ are a subset equal to  the set of transaction in $H2$. Formally, $\langle \forall H1, H2: (H1 \sqsubseteq H2) \implies (\txns{H1} \subseteq \txns{H2}) \rangle$. 
\end{observation}

In order for a transaction $T_i$ to commit in a history $H$, it has to compete with all the live transactions and all the aborted that can become live again as a different \inc. Once a transaction $T_j$ aborts, another \inc of $T_j$ can start and become live again. Thus $T_i$ will have to compete with this \inc of $T_j$ later. Thus, we have the following observation about aborted \& committed transactions. %Thus for a history $H$, we define $\relab{H}$ (relevant abort set) as the transactions whose incarnation can become live again follows \\
%$\relab{H} = \{T_i| (T_i \in \aborted{H}) \land (\neg \inct{i}{H})\}$. 

\begin{observation}
	\label{obs:abort-retry}
	Consider an aborted transaction $T_i$ in a history $H1$. Then there is an extension of $H1$, $H2$ in which an \inc of $T_i$, $T_j$ is live and has $\tcts{j}$ is greater than $\tcts{i}$. Formally, $\langle H1, T_i: (T_i \in \aborted{H1}) \implies(\exists T_j, H2: (H1 \sqsubseteq H2) \land (T_j \in \live{H2}) \land (\htits{i}{H2} = \htits{j}{H2}) \land (\htcts{i}{H2} < \htcts{j}{H2})) \rangle$. 
\end{observation}

\begin{observation}
	\label{obs:cmt-noinc}
	Consider an committed transaction $T_i$ in a history $H1$. Then there is no extension of $H1$, in which an \inc of $T_i$, $T_j$ is live. Formally, $\langle H1, T_i: (T_i \in \comm{H1}) \implies(\nexists T_j, H2: (H1 \sqsubseteq H2) \land (T_j \in \live{H2}) \land (\htits{i}{H2} = \htits{j}{H2})) \rangle$. 
\end{observation}

\begin{lemma}
	\label{lem:cts-wts}
	Consider a history $H1$ and its extension $H2$. Let $T_i, T_j$ be in $H1, H2$ respectively such that they are \inc{s} of each other. If \wts of $T_i$ is less than \wts of $T_j$ then \cts of $T_i$ is less than \cts $T_j$.
	Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubset H2) \land (T_i \in \txns{H1}) \land (T_j \in \txns{H2}) \land (T_i \in \incs{j}{H2}) \land (\htwts{i}{H1} < \htwts{j}{H2})\implies (\htcts{i}{H1} < \htcts{j}{H2}) \rangle$
\end{lemma}

\begin{proof}
	Here we are given that 
	\begin{equation}
	\label{eq:wts-ij}
	\htwts{i}{H1} < \htwts{j}{H2}
	\end{equation}
	
	The definition of \wts of $T_i$ is: $\htwts{i}{H1} = \htcts{i}{H1} + C * (\htcts{i}{H1} - \htits{i}{H1})$. Combining this \eqnref{wts-ij}, we get that 
	
	%Substituting for $c$ to be 1, we get that $\htwts{i}{H1} = 2 * \htcts{i}{H1} - \htits{i}{H1}$.
	%$2 * \htcts{i}{H1} - \htits{i}{H1} < 2 * \htcts{j}{H2} - \htits{j}{H2} \xrightarrow[\htits{i}{H1} = \htits{j}{H2}]{T_i \in \incs{j}{H2}} \htcts{i}{H1} < \htcts{j}{H2}$. 
	
	%Substituting for $C$ to be 1, we get that $\htwts{i}{H1} = 2 * \htcts{i}{H1} - \htits{i}{H1}$.
	$(C + 1) * \htcts{i}{H1} - C * \htits{i}{H1} < (C + 1) * \htcts{j}{H2} - C * \htits{j}{H2} \xrightarrow[\htits{i}{H1} = \htits{j}{H2}]{T_i \in \incs{j}{H2}} \htcts{i}{H1} < \htcts{j}{H2}$. 
\end{proof}

\begin{lemma}
	\label{lem:wts-great}
	Consider a live transaction $T_i$ in a history $H1$ with its $\twts{i}$ less than a constant $\alpha$. Then there is a strict extension of $H1$, $H2$ in which an \inc of $T_i$, $T_j$ is live with \wts greater than $\alpha$. Formally, $\langle H1, T_i: (T_i \in \live{H1}) \land (\htwts{i}{H1} < \alpha) \implies(\exists T_j, H2: (H1 \sqsubseteq H2) \land (T_i \in \incs{j}{H2}) \land ((T_j \in \comm{H2}) \lor ((T_j \in \live{H2}) \land (\htwts{j}{H2} > \alpha)))) \rangle$. 
\end{lemma}

\begin{proof}
	%If \wts of $T_i$ in $H1$ is already greater than $\alpha$ then we can consider $H1$ to be same as $H2$ and the proof directly follows. 
	The proof comes the behavior of an \aptr. The application keeps invoking a transaction with the same \its until it commits. Thus the transaction $T_i$ which is live in $H1$ will eventually terminate with an abort or commit. If it commits, $H2$ could be any history after the commit of $T_2$. 
	
	On the other hand if $T_i$ is aborted, as seen in \obsref{abort-retry} it will be invoked again or reincarnated with another \cts and \wts. It can be seen that \cts is always increasing. As a result, the \wts is also increasing. Thus eventually the \wts will become greater $\alpha$. Hence, we have that either an \inc of $T_i$ will get committed or will eventually have \wts greater than or equal to $\alpha$.
\end{proof}

\noindent Next we have a lemma about \cts of a transaction and the \syst of a history. 

\begin{lemma}
	\label{lem:cts-syst}
	Consider a transaction $T_i$ in a history $H$. Then, we have that \cts of $T_i$ will be less than or equal to \syst of $H$. Formally, $\langle T_i, H1: (T_i \in \txns{H}) \implies (\htcts{i}{H} \leq \hsyst{H}) \rangle$. 
\end{lemma}

\begin{proof}
	We get this lemma by observing the \mth{s} of the STM System that increment the \tcntr which are \begt and \tryc. It can be seen that \cts of $T_i$ gets assigned in the \begt \mth. So if the last \mth of $H$ is the \begt of $T_i$ then we get that \cts of $T_i$ is same as \syst of $H$. On the other hand if some other \mth got executed in $H$ after \begt of $T_i$ then we have that \cts of $T_i$ is less than \syst of $H$. Thus combining both the cases, we get that \cts of $T_i$ is less than or equal to as \syst of $H$, i.e., $(\htcts{i}{H} \leq \hsyst{H})$
\end{proof}

\noindent From this lemma, we get the following corollary which is the converse of the lemma statement

\begin{corollary}
	\label{cor:cts-syst}
	Consider a transaction $T_i$ which is not in a history $H1$ but in an strict extension of $H1$, $H2$. Then, we have that \cts of $T_i$ is greater than the \syst of $H$. Formally, $\langle T_i, H1, H2: (H1 \sqsubset H2) \land (T_i \notin \txns{H1}) \land (T_i \in \txns{H2}) \implies (\htcts{i}{H2} > \hsyst{H1}) \rangle$. 
\end{corollary}

\noindent Now, we have lemma about the \mth{s} of \ksftm completing in finite time. 

\begin{lemma}
	\label{lem:mth-fdm}
	If all the locks are fair and the underlying system scheduler is fair then all the \mth{s} of \ksftm will eventually complete.
\end{lemma}

\begin{proof}
	It can be seen that in any \mth, whenever a transaction $T_i$ obtains multiple locks, it obtains locks in the same order: first lock relevant \tobj{s} in a pre-defined order and then lock relevant \glock{s} again in a predefined order. Since all the locks are obtained in the same order, it can be seen that the \mth{s} of \ksftm will not deadlock. 
	
	It can also be seen that none of the \mth{s} have any unbounded while loops. All the loops in \tryc \mth iterate through all the \tobj{s} in the write-set of $T_i$. Moreover, since we assume that the underlying scheduler is fair, we can see that no thread gets swapped out infinitely. Finally, since we assume that all the locks are fair, it can be seen all the \mth{s} terminate in finite time.
\end{proof}

\begin{theorem}
	\label{thm:trans-com|abt}
	Every transaction either commits or aborts in finite time.
\end{theorem}

\begin{proof}
	This theorem comes directly from the \lemref{mth-fdm}. Since every \mth of \ksftm will eventually complete, all the transactions will either commit or abort in finite time.
\end{proof}

\noindent From this theorem, we get the following corollary which states that the maximum \emph{lifetime} of any transaction is $L$. 

\begin{corollary}
	\label{cor:cts-L}
	Any transaction $T_i$ in a history $H$ will either commit or abort before the \syst of $H$ crosses $\tcts{i} + L$. 
\end{corollary}

\noindent The following lemma connects \wts and \its of two transactions, $T_i, T_j$. 

\begin{lemma}
	\label{lem:wts-its}
	Consider a history $H1$ with two transactions $T_i, T_j$. Let $T_i$ be in $\live{H1}$. Suppose $T_j$'s \wts is greater or equal to $T_i$' s \wts. Then \its of $T_j$ is less than $\tits{i} + 2*L$. Formally, $\langle H, T_i, T_j : (\{ T_i, T_j\} \subseteq \txns{H}) \land ( T_i \in \live{H}) \land (\htwts{j}{H} \geq \htwts{i}{H}) \Longrightarrow (\htits{i}{H} + 2L \geq \htits{j}{H}) \rangle$.
	%Then for $T_j$, we have that $\langle H, T_i, T_j : (\{ T_i, T_j\} \subseteq \txns{H}) \land ( T_i \in \live{H}) \land (\htwts{j}{H} \geq \htwts{i}{H}) \Longrightarrow (\htits{i}{H} + 2L \geq \htits{j}{H}) \rangle$.
\end{lemma}

\begin{proof}
	Since $T_i$ is live in $H1$, from \corref{cts-L}, we get that it terminates before the system time, $\tcntr$ becomes $\tcts{i} + L$. Thus, \syst of history $H1$ did not progress beyond $\tcts{i} + L$. Hence, for any other transaction $T_j$ (which is either live or terminated) in $H1$, it must have started before \syst has crossed $\tcts{i} + L$. Formally $\langle \tcts{j} \leq \tcts{i} + L \rangle$.
	
	Note that we have defined \wts of a transaction $T_j$ as: $\twts{j} = (\tcts{j} + C * (\tcts{j} - \tits{j}))$. Now, let us consider the difference of the \wts{s} of both the transactions. 
	\noindent 
	\begin{math}
		\twts{j} - \twts{i}  = (\tcts{j} + C * (\tcts{j} - \tits{j})) - (\tcts{i} + C * (\tcts{i} - \tits{i})) \\ 
		= (C + 1)(\tcts{j} - \tcts{i}) - C(\tits{j} - \tits{i}) \\
		\leq (C + 1)L - C(\tits{j} - \tits{i}) \qquad [\because \tcts{j} \leq \tcts{i} + L] \\
		%= C(\tits{j} - \tits{i}) - (C + 1)L \\
		= 2*L + \tits{i} - \tits{j}  \qquad [\because C = 1] \\
	\end{math}
	
	\noindent Thus, we have that: $ \langle (\tits{i} + 2L - \tits{j}) \geq (\twts{j} - \twts{i}) \rangle$. This gives us that \\
	$((\twts{j} - \twts{i}) \geq 0) \Longrightarrow ((\tits{i} + 2L - \tits{j}) \geq 0)$. 
	
	\noindent From the above implication we get that, 
	$(\twts{j} \geq \twts{i}) \Longrightarrow (\tits{i} + 2L \geq \tits{j})$.
	
\end{proof}

It can be seen that \ksftm algorithm gives preference to transactions with lower \its to commit. To understand this notion of preference, we define a few notions of enablement of a transaction $T_i$ in a history $H$. We start with the definition of \emph{\itsen} as:

\begin{definition}
	\label{defn:itsen}
	We say $T_i$ is \emph{\itsen} in $H$ if for all transactions $T_j$ with \its lower than \its of $T_i$ in $H$ have \incct to be true. Formally, 
	\begin{equation*}
		\itsenb{i}{H} = \begin{cases}
			True    & (T_i \in \live{H}) \land (\forall T_j \in \txns{H} : (\htits{j}{H} < \htits{i}{H}) \\& \implies (\inct{j}{H})) \\
			False	& \text{otherwise}
		\end{cases}
	\end{equation*}
\end{definition}

\noindent The follow lemma states that once a transaction $T_i$ becomes \itsen it continues to remain so until it terminates. 

\begin{lemma}
	\label{lem:itsen-future}
	Consider two histories $H1$ and $H2$ with $H2$ being a extension of $H1$. Let a transaction $T_i$ being live in both of them. Suppose $T_i$ is \itsen in $H1$. Then $T_i$ is \itsen in $H2$ as well. Formally, $\langle H1, H2, T_i: (H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_i \in \live{H2}) \land (\itsenb{i}{H1}) \implies (\itsenb{i}{H2}) \rangle$. 
\end{lemma}

\begin{proof}
	When $T_i$ begins in a history $H3$ let the set of transactions with \its less than $\tits{i}$ be $smIts$. Then in any extension of $H3$, $H4$ the set of transactions with \its less than $\tits{i}$ remains as $smIts$. 
	
	Suppose $H1, H2$ are extensions of $H3$. Thus in $H1, H2$ the set of transactions with \its less than $\tits{i}$ will be $smIts$. Hence, if $T_i$ is \itsen in $H1$ then all the transactions $T_j$ in $smIts$ are $\inct{j}{H1}$. It can be seen that this continues to remain true in $H2$. Hence in $H2$, $T_i$ is also \itsen which proves the lemma.
\end{proof}

%\noindent The following lemma deals with a committed transaction $T_i$ and any transaction $T_j$ that terminates later. In the following lemma, $\incv$ is any constant greater than or equal to 2. 
The following lemma deals with a committed transaction $T_i$ and any transaction $T_j$ that terminates later. In the following lemma, $\incv$ is any constant greater than or equal to 1. %$(1 + C)$ which becomes 2 if we assume $C=1$. 

\begin{lemma}
	\label{lem:tryci-j}
	Consider a history $H$ with two transactions $T_i, T_j$ in it. Suppose transaction $T_i$ commits before $T_j$ terminates (either by commit or abort) in $H$. Then $\ct_i$ is less than $\ct_j$ by at least $\incv$. Formally, $\langle H, \{T_i, T_j\} \in \txns{H}: (\tryc_i <_H \term_j) \implies (\ct_i + \incv \leq \ct_j)\rangle$. 
\end{lemma}

\begin{proof}
	When $T_i$ commits, let the value of the global $\tcntr$ be $\alpha$. It can be seen that in \begt \mth, $\ct_j$ get initialized to $\infty$. The only place where $\ct_j$ gets modified is at \Lineref{tcv201} of \tryc. Thus if $T_j$ gets aborted before executing \tryc \mth or before this line of \tryc we have that $\ct_j$ remains at $\infty$. Hence in this case we have that $\langle \ct_i + \incv < \ct_j \rangle$.
	
	If $T_j$ terminates after executing \Lineref{tcv201} of \tryc \mth then $\ct_j$ is assigned a value, say $\beta$. It can be seen that $\beta$ will be greater than $\alpha$ by at least $\incv$ due to the execution of this line. Thus, we have that $\langle \alpha + \incv \leq \beta \rangle$
\end{proof}

\noindent The following lemma connects the \tltl and \ct of a transaction $T_i$. 

\begin{lemma}
	\label{lem:ti|tltl-comt}
	Consider a history $H$ with a transaction $T_i$ in it. Then in $H$, $\ttltl{i}$ will be less than or equal to $\ct_i$. Formally, $\langle H, \{T_i\} \in \txns{H}: (\htltl{i}{H} \leq H.\ct_i) \rangle$.
\end{lemma}

\begin{proof}
	Consider the transaction $T_i$. In \begt \mth, $\ct_i$ get initialized to $\infty$. The only place where $\ct_i$ gets modified is at \Lineref{tcv201} of \tryc. Thus if $T_i$ gets aborted before this line or if $T_i$ is live we have that $(\ttltl{i} \leq \ct_i)$. On executing \Lineref{tcv201}, $\ct_i$ gets assigned to some finite value and it does not change after that. 
	
	It can be seen that $\ttltl{i}$ gets initialized to $\tcts{i}$ in \Lineref{begin15} of \begt \mth. In that line, $\tcts{i}$ reads $\tcntr$ and increments it atomically. Then in \Lineref{tcv201}, $\ct_i$ gets assigned the value of $\tcntr$ after incrementing it. Thus, we clearly get that $\tcts{i} (= \ttltl{i}\text{ initially}) < \ct_i$. Then $\ttltl{i}$ gets updated on \Lineref{rvm25} of read, \Lineref{tcv20} and \Lineref{tcv34} of \tryc \mth{s}. Let us analyze them case by case assuming that $\ttltl{i}$ was last updated in each of these \mth{s} before the termination of $T_i$:
	
	\begin{enumerate}
		\item \label{case:read} \Lineref{rvm25} of read \mth: Suppose this is the last line where $\ttltl{i}$ updated. Here $\ttltl{i}$ gets assigned to 1 + \vt of the previously committed version which say was created by a transaction $T_j$. Thus, we have the following equation, 
		\begin{equation}
			\label{eq:tltl-vt}
			\ttltl{i} = 1 + x[j].\vt
		\end{equation}
		
		It can be seen that $x[j].\vt$ is same as $\ttltl{j}$ when $T_j$ executed \Lineref{tcv20} of \tryc. Further, $\ttltl{j}$ in turn is same as $\ttutl{j}$ due to \Lineref{tcv20} of \tryc. From \Lineref{tcv202}, it can be seen that $\ttutl{j}$ is less than or equal to $\ct_j$ when $T_j$ committed. Thus we have that 
		\begin{equation}
			\label{eq:tltl-ct}
			x[j].\vt = \ttltl{j} = \ttutl{j} \leq \ct_j
		\end{equation}
		
		It is clear that from the above discussion that  $T_j$ executed \tryc \mth before $T_i$ terminated (i.e. $\tryc_j <_{H1} \term_i$). From \eqnref{tltl-vt} and \eqnref{tltl-ct}, we get \\
		\begin{math}
			%\ttltl{i} \leq 1 + \ct_j < 1 + C + \ct_j \xrightarrow[]{\incv \geq 2} \ttltl{i} < \incv + \ct_j \xrightarrow[]{\lemref{tryci-j}} \ttltl{i} < \ct_i
			\ttltl{i} \leq 1 + \ct_j \xrightarrow[]{\incv \geq 1} \ttltl{i} \leq \incv + \ct_j \xrightarrow[]{\lemref{tryci-j}} \ttltl{i} \leq \ct_i
		\end{math}
		
		\item \label{case:tryc-short} \Lineref{tcv20} of \tryc \mth: The reasoning in this case is very similar to the above case. 
		
		\item \label{case:tryc-long} \Lineref{tcv34} of \tryc \mth: In this line, $\ttltl{i}$ is made equal to $\ttutl{i}$. Further, in \Lineref{tcv202}, $\ttutl{i}$ is made lesser than or equal to $\ct_{i}$. Thus combing these, we get that $\ttltl{i} \leq \ct_{i}$. It can be seen that the reasoning here is similar in part to \csref{read}.  
	\end{enumerate}
	
	Hence, in all the three cases we get that $\langle \ttltl{i} \leq \ct_i \rangle$. 
\end{proof}

\noindent The following lemma connects the \tutl,\ct of a transaction $T_i$ with \wts of a transaction $T_j$ that has already committed. 

\begin{lemma}
	\label{lem:ti|tutl-comt}
	Consider a history $H$ with a transaction $T_i$ in it. Suppose $\ttutl{i}$ is less than $\ct_i$. Then, there is a committed transaction $T_j$ in $H$ such that $\twts{j}$ is greater than $\twts{i}$. Formally, $\langle H \in \gen{\ksftm}, \{T_i\} \in \txns{H}: (\htutl{i}{H} < H.\ct_i) \implies (\exists T_j \in \comm{H}: \htwts{j}{H} > \htwts{i}{H}) \rangle$.
\end{lemma}

\begin{proof}
	It can be seen that $\tutl_i$ initialized in \begt \mth to $\infty$. $\ttutl{i}$ is updated in \Lineref{rvm22} of read \mth, \Lineref{tcv22} \& \Lineref{tcv202} of \tryc \mth. If $T_i$ executes \Lineref{rvm22} of read \mth and/or \Lineref{tcv22} of \tryc \mth then $\ttutl{i}$ gets decremented to some value less than $\infty$, say $\alpha$. Further, it can be seen that in both these lines the value of $\ttutl{i}$ is possibly decremented from $\infty$ because of $nextVer$ (or $ver$), a version of $x$ whose \ts is greater than $T_i$'s \wts. This implies that some transaction $T_j$, which is committed in $H$, must have created $nextVer$ (or $ver$) and $\twts{j} > \twts{i}$. 
	
	Next, let us analyze the value of $\alpha$. It can be seen that $\alpha = x[nextVer/ver].vrt - 1$ where $nextVer/ver$ was created by $T_j$. Further, we can see when $T_j$ executed \tryc, we have that $x[nextVer].vrt = \ttltl{j}$ (from \Lineref{tc19}). From \lemref{ti|tltl-comt}, we get that $\ttltl{j} \leq \ct_j$. This implies that $\alpha < \ct_j$. Now, we have that $T_j$ has already committed before the termination of $T_i$. Thus from \lemref{tryci-j}, we get that $\ct_j < \ct_i$. Hence, we have that, 
	
	\begin{equation}
		\label{eq:alph-ct}
		\alpha < \ct_i 
	\end{equation}
	
	Now let us consider \Lineref{tcv202} executed by $T_i$ which causes $\ttutl{i}$ to change. This line will get executed only after both \Lineref{rvm22} of read \mth, \Lineref{tcv22} of \tryc \mth. This is because every transaction executes \tryc \mth only after read \mth. Further within \tryc \mth, \Lineref{tcv202} follows \Lineref{tcv22}. 
	
	There are two sub-cases depending on the value of $\ttutl{i}$ before the execution of \Lineref{tcv202}: (i) If $\ttutl{i}$ was $\infty$  and then get decremented to $\ct_i$ upon executing this line, then we get $\ct_i =  \ttutl{i}$. From \eqnref{alph-ct},  we can ignore this case. (ii) Suppose the value of $\ttutl{i}$ before executing \Lineref{tcv202} was $\alpha$. Then from \eqnref{alph-ct} we get that $\ttutl{i}$ remains at $\alpha$ on execution of \Lineref{tcv202}. This implies that a transaction $T_j$ committed such that $\twts{j} > \twts{i}$.
\end{proof}

\noindent The following lemma connects the \tltl of a committed transaction $T_j$ and \ct of a transaction $T_i$ that commits later. 

\begin{lemma}
	\label{lem:tltlj-comti}
	Consider a history $H1$ with transactions $T_i, T_j$ in it. Suppose $T_j$ is committed and $T_i$ is live in $H1$. Then in any extension of $H1$, say $H2$, $\ttltl{j}$ is less than or equal to $\ct_i$. Formally, $\langle {H1, H2} \in \gen{\ksftm}, \{T_i, T_j\} \subseteq \txns{H1, H2}: (H1 \sqsubseteq H2) \land (T_j \in \comm{H1}) \land (T_i \in \live{H1}) \implies (\htltl{j}{H2} < H2.\ct_i) \rangle$.
\end{lemma}

\begin{proof}
	As observed in the previous proof of \lemref{ti|tltl-comt}, if $T_i$ is live  or aborted in $H2$, then its \ct is $\infty$. In both these cases, the result follows.
	
	If $T_i$ is committed in $H2$ then, one can see that \ct of $T_i$ is not $\infty$. In this case, it can be seen that $T_j$ committed before $T_i$. Hence, we have that $\ct_j < \ct_i$. From \lemref{ti|tltl-comt}, we get that $\ttltl{j} \leq \ct_j$. This implies that $\ttltl{j} < \ct_i$. 
\end{proof}

\noindent In the following sequence of lemmas, we identify the condition by when a transaction will commit. 

\begin{lemma}
	\label{lem:its-wts}
	Consider two histories $H1, H3$ such that $H3$ is a strict extension of $H1$. Let $T_i$ be a transaction in  $\live{H1}$ such that $T_i$ \itsen in $H1$ and $\gval_i$ flag is true in $H1$. Suppose $T_i$ is aborted in $H3$. Then there is a history $H2$ which is an extension of $H1$ (and could be same as $H1$) such that (1) Transaction $T_i$ is live in $H2$; (2) there is a transaction $T_j$ that is live in ${H2}$; (3) $\htwts{j}{H2}$ is greater than $\htwts{i}{H2}$; (4) $T_j$ is committed in $H3$. Formally, $ \langle H1, H3, T_i: (H1 \sqsubset H3) \land (T_i \in \live{H1}) \land (\htval{i}{H1} = True) \land (\itsenb{i}{H1}) \land (T_i \in \aborted{H3})) \implies (\exists H2, T_j: (H1 \sqsubseteq H2 \sqsubset H3) \land (T_i \in \live{H2}) \land (T_j \in \txns{H2}) \land (\htwts{i}{H2} < \htwts{j}{H2}) \land (T_j \in \comm{H3})) \rangle$. 
\end{lemma}

\begin{proof}
	To show this lemma, w.l.o.g we assume that $T_i$ on executing either read or \tryc in $H2$ (which could be same as $H1$) gets aborted resulting in $H3$. Thus, we have that $T_i$ is live in $H2$. Here $T_i$ is \itsen in $H1$. From \lemref{itsen-future}, we get that $T_i$ is \itsen in $H2$ as well.
	
	%Since it is live in $H2$, from \lemref{itsen-future}, we get that $T_i$ is \itsen in $H2$ as well. Note that $H2$ could be same as $H1$ as well. 
	
	Let us sequentially consider all the lines where a $T_i$ could abort. In $H2$, $T_i$ executes one of the following lines and is aborted in $H3$. We start with \tryc method. 
	
	\begin{enumerate}
		
		\item \tryc: 
		
		\begin{enumerate}
			\item \Lineref{tc3} \label{case:init-tc-chk}: This line invokes abort() method on $T_i$ which releases all the locks and returns $\mathcal{A}$ to the invoking thread. Here $T_i$ is aborted because its \val flag, is set to false by some other transaction, say $T_j$, in its \tryc algorithm. This can occur in Lines: \ref{lin:tcv14}, \ref{lin:tcv29} where $T_i$ is added to $T_j$'s \abl set. Later in \Lineref{tcv39}, $T_i$'s \val flag is set to false. Note that $T_i$'s \val is true (after the execution of the last event) in $H1$. Thus, $T_i$'s \val flag must have been set to false in an extension of $H1$, which we again denote as $H2$.
			
			This can happen only if in both the above cases, $T_j$ is live in $H2$ and its \its is less than $T_i$'s \its. But we have that $T_i$'s \itsen in $H2$. As a result, it has the smallest among all live and aborted transactions of $H2$. Hence, there cannot exist such a $T_j$ which is live and $\htits{j}{H2} < \htits{i}{H2}$. Thus, this case is not possible. 
			
			\item \Lineref{tcv111}: This line is executed in $H2$ if there exists no version of $x$ whose \ts is less than $T_i$'s \wts. This implies that all the versions of $x$ have \ts{s} greater than $\twts{i}$. Thus the transactions that created these versions have \wts greater than $\twts{i}$ and have already committed in $H2$. Let $T_j$ create one such version. Hence, we have that $\langle (T_j \in \comm{H2}) \implies (T_j \in \comm{H3}) \rangle$ since $H3$ is an extension of $H2$. 
			
			\item \Lineref{tcv10} \label{case:mid-tc-chk}: This case is similar to \csref{init-tc-chk}, i.e., \Lineref{tcv39}. %Here $T_i$ is aborted because its \gval flag, is set to false by some other live transaction, say $T_j$, in its \tryc algorithm. This can happen only if $T_j$'s \its is less than $T_i$'s \its. But from our assumption, we have that $T_i$'s \its is the smallest among all live transactions. Hence, there cannot exist such a $T_j$. Thus, this case is not possible.
			
			\item \Lineref{tcv15} \label{case:its-chk1}: In this line, $T_i$ is aborted as some other transaction $T_j$ in $T_i$'s \lrl has committed. Any transaction in $T_i$'s \lrl has \wts greater than $T_i$'s \wts. This implies that $T_j$ is already committed in $H2$ and hence committed in $H3$ as well. 
			
			\item \Lineref{tcv24} \label{case:tc-lts-cross}: In this line, $T_i$ is aborted because its lower limit has crossed its upper limit. First, let us consider $\ttutl{i}$. It is initialized in \begt \mth to $\infty$. As long as it is $\infty$, these limits cannot cross each other. Later, $\ttutl{i}$ is updated in \Lineref{rvm22} of read \mth, \Lineref{tcv22} \& \Lineref{tcv202} of \tryc \mth. Suppose $\ttutl{i}$ gets decremented to some value $\alpha$ by one of these lines. 
			
			Now there are two cases here: (1) Suppose $\ttutl{i}$ gets decremented to $\ct_i$ due to \Lineref{tcv202} of \tryc \mth. Then from \lemref{ti|tltl-comt}, we have $\ttltl{i} \leq \ct_i =  \ttutl{i}$. Thus in this case, $T_i$ will not abort. (2) $\ttutl{i}$ gets decremented to $\alpha$ which is less than $\ct_i$. Then from \lemref{ti|tutl-comt}, we get that there is a committed transaction $T_j$ in $\comm{H2}$ such that $\twts{j} > \twts{i}$. This implies that $T_j$ is in $\comm{H3}$.
			
			\ignore{
				It can be seen that if $T_i$ executes \Lineref{rd-ul-dec} of read \mth and/or \Lineref{tryc-ul-dec} of \tryc \mth then $\ttutl{i}$ gets decremented to some value less than $\infty$, say $\alpha$. Further, it can be seen that in both these lines the value of $\ttutl{i}$ is possibly decremented from $\infty$ because of $nextVer$ (or $ver$), a version of $x$ who \ts is greater than $T_i$. This implies that some transaction $T_j$ which is committed in $H$ must have created $nextVer$ ($ver$) and $\twts{j} > \twts{i}$. 
				
				Next, let us analyze the value of $\alpha$. It can be seen that $\alpha = x[nextVer/ver].vrt - 1$ where $nextVer/ver$ was created by $T_j$. Further, we can see when $T_j$ executed \tryc, we have that $x[nextVer].vrt = \ttltl{j}$ (from \Lineref{new-tup}). From \lemref{ti|tltl-comt}, we get that $\ttltl{j} \leq \ct_j$. This implies that $\alpha < \ct_j$. Now, we can see that $T_j$ has already committed before the termination of $T_i$. Thus from \lemref{tryci-j}, we get that $\ct_j < \ct_i$. Hence, we have that $\alpha < \ct_i$. 
				
				It is clear that before executing this line \Lineref{tc-lts-cross}, $T_i$ executed \Lineref{tryc-ul-cmt}. Now there are two sub-cases depending on the value of $\ttutl{i}$ before the execution of \Lineref{tryc-ul-cmt}: (i) If $\ttutl{i}$ was $\infty$ then it get decremented to $\ct_i$ upon executing this line. Then again from \lemref{ti|tltl-comt}, we have $\ttltl{i} \leq \ct_i =  \ttutl{i}$. Thus in this case, $T_i$ will not abort. (ii) Suppose the value of $\ttutl{i}$ before executing \Lineref{tryc-ul-cmt} was $\alpha$. Then from the above discussion we get that $\ttutl{i}$ remains at $\alpha$. This implies that a transaction $T_j$ committed such that $\twts{j} > \twts{i}$. Thus if $\ttltl{i}$ turned out to be greater than $\ttutl{i}$ causing $T_i$ to abort, we still have that the lemma is true.
			}
			
		%	\item \Lineref{tcv30}: This case is similar to \csref{init-tc-chk}, i.e., \Lineref{tc3}.
			%lin:its_lar-sml
			
			\item \Lineref{tcv30} \label{case:its-chk2}: In this case, $T_k$ is in $T_i$'s \srl and is committed in $H1$. And, from this case, we have that
			
			\begin{equation}
				\label{eq:tltl-k_i}
				\htutl{i}{H2} \leq \htltl{k}{H2}
			\end{equation}
			
			From the assumption of this case, we have that $T_k$ commits before $T_i$. Thus, from \lemref{tltlj-comti}, we get that $\ct_k < \ct_i$. From \lemref{ti|tltl-comt}, we have that $\ttltl{k} \leq \ct_k$. Thus, we get that $\ttltl{k} < \ct_i$. Combining this with the inequality of this case \eqnref{tltl-k_i}, we get that $\ttutl{i} < \ct_i$.
			
			Combining this inequality with \lemref{ti|tutl-comt}, we get that there is a transaction $T_j$ in $\comm{H2}$ and $\htwts{j}{H2} > \htwts{i}{H2}$. This implies that $T_j$ is in $\comm{H3}$ as well.
			
			%This case is similar to \stref{its-chk1}. In this line, $T_i$ is aborted as some other live transaction $T_j$ in $T_i$'s \lrl has lower \its. But from our assumption, we get that $T_i$ has the lowest \its among all the live transactions in $H1$. Hence, such a $T_j$ can not exist and as a result, this case is not possible. 
		\end{enumerate}
	\item STM read: 
	
	\begin{enumerate}
		\item \Lineref{rvm5}: This case is similar to \csref{init-tc-chk}, i.e., \Lineref{tc3}
		
		\item \Lineref{rvm27}: The reasoning here is similar to \csref{tc-lts-cross}, i.e., \Lineref{tcv24}.
	\end{enumerate}
	
\end{enumerate}

\end{proof}

The interesting aspect of the above lemma is that it gives us a insight as to when a $T_i$ will get commit. If an \itsen transaction $T_i$ aborts then it is because of another transaction $T_j$ with \wts higher than $T_i$ has committed. To precisely capture this, we define two more notions of a transaction being enabled \emph{\cdsen} and \emph{\finen}. To define these notions of enabled, we in turn define a few other auxiliary notions. We start with \emph{\affset},
\begin{equation*}
	\haffset{i}{H} = \{T_j|(T_j \in \txns{H}) \land (\htits{j}{H} < \htits{i}{H} + 2*L)\}
\end{equation*}

From the description of \ksftm algorithm and \lemref{wts-its}, it can be seen that a transaction $T_i$'s commit can depend on committing of transactions (or their \inc{s}) which have their \its less than \its of $T_i$ + $2*L$, which is $T_i$'s \affset. We capture this notion of dependency for a transaction $T_i$ in a history $H$ as \emph{commit dependent set} or \emph{\cdset} as: the set of all transactions $T_j$ in $T_i$'s \affset that do not any \inc that is committed yet, i.e., not yet have their \incct flag set as true. Formally, 

\begin{equation*}
	\hcds{i}{H} = \{T_j| (T_j \in \haffset{i}{H}) \land (\neg\inct{j}{H}) \}
\end{equation*}

\noindent Based on this definition of \cdset, we next define the notion of \cdsen. 

\begin{definition}
	\label{defn:cdsen}
	We say that transaction $T_i$ is \emph{\cdsen} if the following conditions hold true (1) $T_i$ is live in $H$; (2) \cts of $T_i$ is greater than or equal to \its of $T_i$ + $2*L$; (3) \cdset of $T_i$ is empty, i.e., for all transactions $T_j$ in $H$ with \its lower than \its of  $T_i$ + $2*L$ in $H$ have their \incct to be true. Formally, 
	
	\begin{equation*}
		\cdsenb{i}{H} = \begin{cases}
			True    & (T_i \in \live{H}) \land (\htcts{i}{H} \geq \htits{i}{H} + 2*L) \land 
			\\ &(\hcds{i}{H} = \phi) \\
			%& (\forall T_j \in \txns{H} : (\htits{j}{H} < \htits{i}{H} + 2*L) \implies (\inct{j}{H})) \\
			False	& \text{otherwise}
		\end{cases}
	\end{equation*}
\end{definition}

\noindent The meaning and usefulness of these definitions will become clear in the course of the proof. In fact, we later show that once the transaction $T_i$ is \cdsen, it will eventually commit. We will start with a few lemmas about these definitions. %The following observation comes from the definitions of \cdsen and \itsen. 


\begin{lemma}
	\label{lem:its-enb}	Consider a transaction $T_i$ in a history $H$. If $T_i$ is \cdsen then $T_i$ is also \itsen. Formally, $\langle H, T_i: (T_i \in \txns{H}) \land (\cdsenb{i}{H}) \implies (\itsenb{i}{H}) \rangle$. 
\end{lemma}

\begin{proof}
	If $T_i$ is \cdsen in $H$ then it implies that $T_i$ is live in $H$. From the definition of \cdsen, we get that $\hcds{i}{H}$ is $\phi$ implying that any transaction $T_j$ with $\tits{k}$ less than $\tits{i} + 2*L$ has its \incct flag as true in $H$. Hence, for any transaction $T_k$ having $\tits{k}$ less than $\tits{i}$, $\inct{k}{H}$ is also true. This shows that $T_i$ is \itsen in $H$.
\end{proof}

\begin{lemma}
	\label{lem:cds-tk-h1}
	Consider a transaction $T_i$ which is \cdsen in a history $H1$. Consider an extension of $H1$, $H2$ with a transaction $T_j$ in it such that $T_i$ is an \inc of $T_j$. Let $T_k$ be a transaction in the \affset of $T_j$ in $H2$ Then $T_k$ is also in the set of transaction of $H1$. Formally, $\langle H1, H2, T_i, T_j, T_k: (H1 \sqsubseteq H2) \land  (\cdsenb{i}{H1}) \land (T_i \in \incs{j}{H2}) \land (T_k \in \haffset{j}{H2}) \implies (T_k \in \txns{H1}) \rangle$
\end{lemma}

\begin{proof} 
	Since $T_i$ is \cdsen in $H1$, we get (from the definition of \cdsen) that 
	\begin{equation}
		\label{eq:ti-cts-its}
		\htcts{i}{H1} \geq \htits{i}{H1} + 2*L
	\end{equation}
	
	Here, we have that $T_k$ is in $\haffset{j}{H2}$. Thus from the definition of \affset, we get that 
	\begin{equation}
		\label{eq:tk-tj-aff}
		\htits{k}{H2} < \htits{j}{H2} + 2*L
	\end{equation}
	
	Since $T_i$ and $T_j$ are \inc{s} of each other, their \its are the same. Combining this with \eqnref{tk-tj-aff}, we get that %$\htits{k}{H2} < \htits{i}{H1} + 2*L$. 
	\begin{equation}
		\label{eq:tk-ti-h12}
		\htits{k}{H2} < \htits{i}{H1} + 2*L
	\end{equation}
	
	We now show this proof through contradiction. Suppose $T_k$ is not in $\txns{H1}$. Then there are two cases:
	
	\begin{itemize}
		\item No \inc of $T_k$ is in $H1$: This implies that $T_k$ starts afresh after $H1$. Since $T_k$ is not in $H1$, from \corref{cts-syst} we get that
		
		$\htcts{k}{H2} > \hsyst{H1} \xrightarrow [\htcts{k}{H2} = \htits{k}{H2}] {T_k \text{ starts afresh}}\htits{k}{H2} > \hsyst{H1} \xrightarrow [\hsyst{H1} \geq \htcts{i}{H1}]{(T_i \in H1) \land \lemref{cts-syst}} \htits{k}{H2} > \htcts{i}{H1} \xrightarrow {\eqnref{ti-cts-its}} \htits{k}{H2} > \htits{i}{H1} + 2*L \xrightarrow {\htits{i}{H1} = \htits{j}{H2}} \htits{k}{H2} > \htits{j}{H2} + 2*L$
		
		But this result contradicts with \eqnref{tk-tj-aff}. Hence, this case is not possible. 
		
		\item There is an \inc of $T_k$, $T_l$ in $H1$: In this case, we have that 
		
		\begin{equation}
			\label{eq:tl-h1}
			\htits{l}{H1} = \htits{k}{H2}
		\end{equation}
		
		%$\htits{l}{H1} = \htits{k}{H2}$
		
		Now combing this result with \eqnref{tk-ti-h12}, we get that $\htits{l}{H1} < \htits{i}{H1} + 2*L$. This implies that $T_l$ is in \affset of $T_i$ in $H1$. Since $T_i$ is \cdsen, we get that $T_l$'s \incct must be true. 
		
		We also have that $T_k$ is not in $H1$ but in $H2$ where $H2$ is an extension of $H1$. Since $H2$ has some events more than $H1$, we get that $H2$ is a strict extension of $H1$.
		
		Thus, we have that, $(H1 \sqsubset H2) \land (\inct{l}{H1}) \land (T_k \in \txns{H2}) \land (T_k \notin \txns{H1})$. Combining these with \lemref{inct-diff}, we get that $(\htits{l}{H1} \neq \htits{k}{H2})$. But this result contradicts \eqnref{tl-h1}. Hence, this case is also not possible.
	\end{itemize}
	Thus from both the cases we get that $T_k$ should be in $H1$. Hence proved.
\end{proof}

\begin{lemma}
	\label{lem:aff-tkinc-h1}
	Consider two histories $H1, H2$ where $H2$ is an extension of $H1$. Let $T_i, T_j, T_k$ be three transactions such that $T_i$ is in $\txns{H1}$ while $T_j, T_k$ are in $\txns{H2}$. Suppose we have that (1) $\tcts{i}$ is greater than $\tits{i} + 2*L$ in $H1$; (2) $T_i$ is an \inc of $T_j$; (3) $T_k$ is in \affset of $T_j$ in $H2$. Then an \inc of $T_k$, say $T_l$ (which could be same as $T_k$) is in $\txns{H1}$. Formally, $\langle H1, H2, T_i, T_j, T_k: (H1 \sqsubseteq H2) \land (T_i \in \txns{H1})  \land (\{T_j, T_k\} \in \txns{H2}) \land (\htcts{i}{H1} > \htits{i}{H1} + 2*L) \land (T_i \in \incs{j}{H2}) \land (T_k \in \haffset{j}{H2}) \implies (\exists T_l: (T_l \in \incs{k}{H2}) \land (T_l \in \txns{H1})) \rangle$
\end{lemma}

\begin{proof} 
	
	\noindent This proof is similar to the proof of \lemref{cds-tk-h1}. We are given that 
	\begin{equation}
		\label{eq:given-ti-ctsits}
		\htcts{i}{H1} \geq \htits{i}{H1} + 2*L
	\end{equation}
	
	We now show this proof through contradiction. Suppose no \inc of $T_k$ is in $\txns{H1}$. This implies that $T_k$ must have started afresh in some history $H3$ which is an extension of $H1$. Also note that $H3$ could be same as $H2$ or a prefix of it, i.e., $H3 \sqsubseteq H2$. Thus, we have that 
	
	\noindent
	\begin{math}
		\htits{k}{H3} > \hsyst{H1} \xrightarrow{\lemref{cts-syst}} \htits{k}{H3} > \htcts{i}{H1} \xrightarrow{\eqnref{given-ti-ctsits}} \htits{k}{H3} > \htits{i}{H1} + 2*L \xrightarrow{\htits{i}{H1} = \htits{j}{H2}} \htits{k}{H3} > \htits{j}{H2} + 2*L \xrightarrow[\obsref{hist-subset}]{H3 \sqsubseteq H2} \htits{k}{H2} > \htits{j}{H2} + 2*L \xrightarrow[definition]{\affset} T_k \notin \haffset{j}{H2}
	\end{math}
	
	But we are given that $T_k$ is in \affset of $T_j$ in $H2$. Hence, it is not possible that $T_k$ started afresh after $H1$. Thus, $T_k$ must have a \inc in $H1$.
\end{proof}

\begin{lemma}
	\label{lem:aff-same}
	Consider a transaction $T_i$ which is \cdsen in a history $H1$. Consider an extension of $H1$, $H2$ with a transaction $T_j$ in it such that $T_j$ is an \inc of $T_i$ in $H2$. Then \affset of $T_i$ in $H1$ is same as the \affset of $T_j$ in $H2$. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land  (\cdsenb{i}{H1}) \land (T_j \in \txns{H2}) \land (T_i \in \incs{j}{H2}) \implies ((\haffset{i}{H1} = \haffset{j}{H2})) \rangle$
\end{lemma}

\begin{proof}
	From the definition of \cdsen, we get that $T_i$ is in $\txns{H1}$. Now to prove that \affset{s} are the same, we have to show that $(\haffset{i}{H1} \subseteq \haffset{j}{H2})$ and $(\haffset{j}{H1} \subseteq \haffset{i}{H2})$. We show them one by one:
	
	\paragraph{$(\haffset{i}{H1} \subseteq \haffset{j}{H2})$:} Consider a transaction $T_k$ in $\haffset{i}{H1}$. We have to show that $T_k$ is also in $\haffset{j}{H2}$. From the definition of \affset, we get that 
	\begin{equation}
		\label{eq:tk-h1}
		T_k \in \txns{H1}
	\end{equation}
	
	\noindent Combining \eqnref{tk-h1} with \obsref{hist-subset}, we get that 
	\begin{equation}
		\label{eq:tk-h2}
		T_k \in \txns{H2}
	\end{equation}
	
	\noindent From the definition of \its, we get that 
	\begin{equation}
		\label{eq:its-h1-h2}
		\htits{k}{H1} = \htits{k}{H2}
	\end{equation}
	
	\noindent Since $T_i, T_j$ are \inc{s} we have that . 
	\begin{equation}
		\label{eq:its-ij}
		\htits{i}{H1} = \htits{j}{H2}
	\end{equation}
	
	\noindent From the definition of \affset, we get that, \\ 
	$\htits{k}{H1} < \htits{i}{H1} + 2*L \xrightarrow{\eqnref{its-h1-h2}} \htits{k}{H2} < \htits{i}{H1} + 2*L \xrightarrow{\eqnref{its-ij}} \htits{k}{H2} < \htits{j}{H2} + 2*L$
	
	\noindent Combining this result with \eqnref{tk-h2}, we get that $T_k \in \haffset{j}{H2}$. 
	\paragraph{$(\haffset{i}{H1} \subseteq \haffset{j}{H2})$:} Consider a transaction $T_k$ in $\haffset{j}{H2}$. We have to show that $T_k$ is also in $\haffset{i}{H1}$. From the definition of \affset, we get that $T_k \in \txns{H2}$.
	
	Here, we have that $(H1 \sqsubseteq H2) \land  (\cdsenb{i}{H1}) \land (T_i \in \incs{j}{H2}) \land (T_k \in \haffset{j}{H2})$. Thus from \lemref{cds-tk-h1}, we get that $T_k \in \txns{H1}$. Now, this case is similar to the above case. It can be seen that Equations \ref{eq:tk-h1}, \ref{eq:tk-h2}, \ref{eq:its-h1-h2}, \ref{eq:its-ij} hold good in this case as well. 
	
	Since $T_k$ is in $\haffset{j}{H2}$, we get that \\
	$\htits{k}{H2} < \htits{i}{H2} + 2*L \xrightarrow{\eqnref{its-h1-h2}} \htits{k}{H1} < \htits{j}{H2} + 2*L \xrightarrow{\eqnref{its-ij}} \htits{k}{H1} < \htits{i}{H1} + 2*L $
	
	\noindent Combining this result with \eqnref{tk-h1}, we get that $T_k \in \haffset{i}{H1}$.
\end{proof}

\noindent Next we explore how a \cdsen transaction remains \cdsen in the future histories once it becomes true.

\begin{lemma}
	\label{lem:cds-fut}
	Consider two histories $H1$ and $H2$ with $H2$ being an extension of $H1$. Let  $T_i$ and $T_j$ be two transactions which are live in $H1$ and $H2$ respectively. Let $T_i$ be an \inc of $T_j$ and $\tcts{i}$ is less than $\tcts{j}$. Suppose $T_i$ is \cdsen in $H1$. Then $T_j$ is \cdsen in $H2$ as well. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (T_i \in \incs{j}{H2}) \land (\htcts{i}{H1} < \htcts{j}{H2}) \land (\cdsenb{i}{H1}) \implies (\cdsenb{j}{H2}) \rangle$. 
\end{lemma}

\begin{proof}
	We have that $T_i$ is live in $H1$ and $T_j$ is live in $H2$. Since $T_i$ is \cdsen in $H1$, we get (from the definition of \cdsen) that 
	\begin{equation}
		\label{eq:cts-its}
		\htcts{i}{H1} \geq \htits{i}{H2} + 2*L
	\end{equation}
	
	We are given that $\tcts{i}$ is less than $\tcts{j}$ and $T_i, T_j$ are incarnations of each other. Hence, we have that
	
	\ignore{
		\begin{align*}
			\htcts{j}{H2} & > \htcts{i}{H1} \\
			\htcts{j}{H2} & > \htits{i}{H1} + 2*L & [\text{From \eqnref{cts-its}}] \\
			\htcts{j}{H2} & > \htits{j}{H2} + 2*L & [\tits{i} = \tits{j}] \\
			%\htcts{j}{H2} > & \htits{j}{H2} + 2*L
		\end{align*}
	}
	
	\begin{align*}
		\htcts{j}{H2} & > \htcts{i}{H1} \\
		& > \htits{i}{H1} + 2*L & [\text{From \eqnref{cts-its}}] \\
		& > \htits{j}{H2} + 2*L & [\tits{i} = \tits{j}] \\
	\end{align*}
	
	
	Thus we get that $\tcts{j} > \tits{j} + 2*L$. We have that $T_j$ is live in $H2$. In order to show that $T_j$ is \cdsen in $H2$, it only remains to show that \cdset of $T_j$ in $H2$ is empty, i.e., $\hcds{j}{H2} = \phi$. The \cdset becomes empty when all the transactions of $T_j$'s \affset in $H2$ have their \incct as true in $H2$.
	
	Since $T_j$ is live in $H2$, we get that $T_j$ is in $\txns{H2}$. Here, we have that $(H1 \sqsubseteq H2) \land (T_j \in \txns{H2}) \land (T_i \in \incs{j}{H2}) \land (\cdsenb{i}{H1})$. Combining this with \lemref{aff-same}, we get that $\haffset{i}{H1} = \haffset{j}{H2}$.
	
	Now, consider a transaction $T_k$ in $ \haffset{j}{H2}$. From the above result, we get that $T_k$ is also in $\haffset{i}{H1}$. Since $T_i$ is \cdsen in $H1$, i.e., $\cdsenb{i}{H1}$ is true, we get that $\inct{k}{H1}$ is true. Combining this with \obsref{inct-fut}, we get that $T_k$ must have its \incct as true in $H2$ as well, i.e. $\inct{k}{H2}$. This implies that all the transactions in $T_j$'s \affset have their \incct flags as true in $H2$. Hence the $\hcds{j}{H2}$ is empty. As a result, $T_j$ is \cdsen in $H2$, i.e., $\cdsenb{j}{H2}$. 
\end{proof}

Having defined the properties related to \cdsen, we start defining notions for \finen. Next, we define \emph{\maxwts} for a transaction $T_i$ in $H$ which is the transaction $T_j$ with the largest \wts in $T_i$'s \incset. Formally,
\begin{equation*}
	\hmaxwts{i}{H} = max\{\htwts{j}{H}|(T_j \in \incs{i}{H})\}
\end{equation*}

\noindent From this definition of \maxwts, we get the following simple observation. 

\begin{observation}
	\label{obs:max-wts} 
	For any transaction $T_i$ in $H$, we have that $\twts{i}$ is less than or equal to $\hmaxwts{i}{H}$. Formally, $\htwts{i}{H} \leq \hmaxwts{i}{H}$.
\end{observation}

Next, we combine the notions of \affset and \maxwts to define \emph{\affwts}. It is the maximum of \maxwts of all the transactions in its \affset. Formally, 
\begin{equation*}
	\haffwts{i}{H} = max\{\hmaxwts{j}{H}|(T_j \in \haffset{i}{H})\}
\end{equation*}

\noindent Having defined the notion of \affwts, we get the following lemma relating the \affset and \affwts of two transactions. 

\begin{lemma}
	\label{lem:affwts-same}
	Consider two histories $H1$ and $H2$ with $H2$ being an extension of $H1$. Let  $T_i$ and $T_j$ be two transactions which are live in $H1$ and $H2$ respectively. Suppose the \affset of $T_i$ in $H1$ is same as \affset of $T_j$ in $H2$. Then the \affwts of $T_i$ in $H1$ is same as \affwts of $T_j$ in $H2$. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land (T_i \in \txns{H1}) \land (T_j \in \txns{H2}) \land (\haffset{i}{H1} = \haffset{j}{H2}) \implies (\haffwts{i}{H1} = \haffwts{j}{H2}) \rangle$. 
\end{lemma}

\begin{proof}
	
	From the definition of \affwts, we get the following equations
	\begin{equation}
		\label{eq:h1-ti-affwts}
		\haffwts{i}{H} = max\{\hmaxwts{k}{H}|(T_k \in \haffset{i}{H1})\}
	\end{equation}
	
	\begin{equation}
		\label{eq:h2-tj-affwts}
		\haffwts{j}{H} = max\{\hmaxwts{l}{H}|(T_l \in \haffset{j}{H2})\}
	\end{equation}
	
	From these definitions, let us suppose that $\haffwts{i}{H1}$ is $\hmaxwts{p}{H1}$ for some transaction $T_p$ in $\haffset{i}{H1}$. Similarly, suppose that $\haffwts{j}{H2}$ is $\hmaxwts{q}{H2}$ for some transaction $T_q$ in $\haffset{j}{H2}$.
	
	Here, we are given that $\haffset{i}{H1} = \haffset{j}{H2})$. Hence, we get that $T_p$ is also in $\haffset{i}{H1}$. Similarly, $T_q$ is in $\haffset{j}{H2}$ as well. Thus from Equations \eqref{eq:h1-ti-affwts} \& \eqref{eq:h2-tj-affwts}, we get that 
	
	\begin{equation}
		\label{eq:ti-tp-max}
		\hmaxwts{p}{H1} \geq  \hmaxwts{q}{H2}
	\end{equation}
	
	\begin{equation}
		\label{eq:tj-tq-max}
		\hmaxwts{q}{H2} \geq \hmaxwts{p}{H1}
	\end{equation}
	
	Combining these both equations, we get that $\hmaxwts{p}{H1} = \hmaxwts{q}{H2}$ which in turn implies that $\haffwts{i}{H1} = \haffwts{j}{H2}$.
	
\end{proof}

\noindent Finally, using the notion of \affwts and \cdsen, we define the notion of \emph{\finen}

\begin{definition}
	\label{defn:finen}
	We say that transaction $T_i$ is \emph{\finen} if the following conditions hold true (1) $T_i$ is live in $H$; (2) $T_i$ is \cdsen is $H$; (3) $\htwts{j}{H}$ is greater than $\haffwts{i}{H}$. Formally, 
	
	\begin{equation*}
		\finenb{i}{H} = \begin{cases}
			True    & (T_i \in \live{H}) \land (\cdsenb{i}{H}) \land (\htwts{j}{H} \\& > \haffwts{i}{H}) \\
			False	& \text{otherwise}
		\end{cases}
	\end{equation*}
\end{definition}
It can be seen from this definition, a transaction that is \finen is also \cdsen. We now show that just like \itsen and \cdsen, once a transaction is \finen, it remains \finen until it terminates. The following lemma captures it. 
\begin{lemma}
	\label{lem:fin-fut}
	Consider two histories $H1$ and $H2$ with $H2$ being an extension of $H1$. Let  $T_i$ and $T_j$ be two transactions which are live in $H1$ and $H2$ respectively. Suppose $T_i$ is \finen in $H1$. Let $T_i$ be an \inc of $T_j$ and $\tcts{i}$ is less than $\tcts{j}$. Then $T_j$ is \finen in $H2$ as well. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (T_i \in \incs{j}{H2}) \land (\htcts{i}{H1} < \htcts{j}{H2}) \land (\finenb{i}{H1}) \implies (\finenb{j}{H2}) \rangle$. 
\end{lemma}

\begin{proof}
	Here we are given that $T_j$ is live in $H2$. Since $T_i$ is \finen in $H1$, we get that it is \cdsen in $H1$ as well. Combining this with the conditions given in the lemma statement, we have that, \\ 
	
	\begin{equation}
		\label{eq:fin-given}
		\begin{split}
			\langle (H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (T_i \in \incs{j}{H2}) \\\land (\htcts{i}{H1} < \htcts{j}{H2}) 
			\land (\cdsenb{i}{H1}) \rangle
		\end{split}
	\end{equation}
	%$(H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (T_i \in \incs{j}{H2}) \land (\htcts{i}{H1} < \htcts{j}{H2}) \land (\cdsenb{i}{H1})$.
	
	Combining \eqnref{fin-given} with \lemref{cds-fut}, we get that $T_j$ is \cdsen in $H2$, i.e., $\cdsenb{j}{H2}$. Now, in order to show that $T_j$ is \finen in $H2$ it remains for us to show that $\htwts{j}{H2} > \haffwts{j}{H2}$.
	
	We are given that $T_j$ is live in $H2$ which in turn implies that $T_j$ is in $\txns{H2}$. Thus changing this in \eqnref{fin-given}, we get the following 
	\begin{equation}
		\label{eq:mod-given}
		\begin{split}
			\langle (H1 \sqsubseteq H2) \land (T_j \in \txns{H2}) \land (T_i \in \incs{j}{H2}) \land (\htcts{i}{H1} < \htcts{j}{H2}) \\
			\land (\cdsenb{i}{H1}) \rangle
		\end{split}
	\end{equation}
	
	\noindent Combining \eqnref{mod-given} with \lemref{aff-same} we get that 
	\begin{equation}
		\label{eq:affs-eq}
		\haffwts{i}{H1} = \haffwts{j}{H2}
	\end{equation}
	
	\noindent We are given that $\htcts{i}{H1} < \htcts{j}{H2}$. Combining this with the definition of \wts, we get 
	\begin{equation}
		\label{eq:titj-wts}
		\htwts{i}{H1} < \htwts{j}{H2}
	\end{equation}
	
	\noindent Since $T_i$ is \finen in $H1$, we have that \\
	$\htwts{i}{H1} > \haffwts{i}{H1} \xrightarrow{\eqnref{titj-wts}} \htwts{j}{H2} > \haffwts{i}{H1} \xrightarrow{\eqnref{affs-eq}} \htwts{j}{H2} > \\
	\haffwts{j}{H2}$
	
	%\noindent Hence prove. 
\end{proof}

\noindent Now, we show that a transaction that is \finen will eventually commit. 

%Consider a transaction $T_i$ in a history $H1$. If $T_i$ is \finen in $H1$ then $T_i$ will be in committed in any extension of $H1$, $H3$ where $H3$'s \syst is greater than to $\tcts{i} + L$. Formally, $\langle H1, T_i: (T_i \in \live{H1}) \land (\htval{i}{H1}) \land (\finenb{i}{H1}) \implies (\forall H3: (H1 \sqsubset H3) \land (\hsyst{H3} > \htcts{i}{H3} + L) \land (T_i \in \comm{H3})) \rangle$. 

\begin{lemma}
	\label{lem:enbd-ct}
	Consider a live transaction $T_i$ in a history $H1$. Suppose $T_i$ is \finen in $H1$ and $\tval{i}$ is true in $H1$. Then there exists an extension of $H1$, $H3$ in which $T_i$ is committed. Formally, $\langle H1, T_i: (T_i \in \live{H1}) \land (\htval{i}{H1}) \land (\finenb{i}{H1}) \implies (\exists H3: (H1 \sqsubset H3) \land (T_i \in \comm{H3})) \rangle$. 
\end{lemma}

%\ignore{
\begin{proof}
	Consider a history $H3$ such that its \syst being greater than $\tcts{i} + L$. We will prove this lemma using contradiction. Suppose $T_i$ is aborted in $H3$. %From \corref{cts-L}, we get that $T_i$ must be terminated in $H3$. 
	
	Now consider $T_i$ in $H1$: $T_i$ is live; its \val flag is true; and is \enbd. From the definition of \finen, we get that it is also \cdsen. From \lemref{its-enb}, we get that $T_i$ is \itsen in $H1$. Thus from \lemref{its-wts}, we get that there exists an extension of $H1$, $H2$ such that (1) Transaction $T_i$ is live in $H2$; (2) there is a transaction $T_j$ in ${H2}$; (3) $\htwts{j}{H2}$ is greater than $\htwts{i}{H2}$; (4) $T_j$ is committed in $H3$. Formally, 
	
	\begin{equation}
		\label{eq:its-wts-ant}
		\begin{split}
			\langle (\exists H2, T_j: (H1 \sqsubseteq H2 \sqsubset H3) \land (T_i \in \live{H2}) \land (T_j \in \txns{H2}) \\\land (\htwts{i}{H2} < \htwts{j}{H2})
			\land (T_j \in \comm{H3})) \rangle
		\end{split}
	\end{equation}
	
	Here, we have that $H2$ is an extension of $H1$ with $T_i$ being live in both of them and $T_i$ is \finen in $H1$. Thus from \lemref{fin-fut}, we get that $T_i$ is \finen in $H2$ as well. Now, let us consider $T_j$ in $H2$. From \eqnref{its-wts-ant}, we get that $(\htwts{i}{H2} < \htwts{j}{H2})$. Combining this with the observation that $T_i$ being live in $H2$, \lemref{wts-its} we get that $(\htits{j}{H2} \leq \htits{i}{H2} + 2*L)$.
	
	%\begin{equation}
	%\label{eq:ji-aff}
	%(T_j \in \haffset{i}{H2}) 
	%\end{equation}
	
	This implies that $T_j$ is in \affset of $T_i$ in $H2$, i.e., $(T_j \in \haffset{i}{H2})$. From the definition of \affwts, we get that %\affwts of $T_i$ in $H2$ is greater than 
	
	\begin{equation}
		\label{eq:max-affwts}
		(\haffwts{i}{H2} \geq \hmaxwts{j}{H2}) 
	\end{equation}
	
	Since $T_i$ is \finen in $H2$, we get that $\twts{i}$ is greater than \affwts of $T_i$ in $H2$. 
	\begin{equation}
		\label{eq:wts-affwts}
		(\htwts{i}{H2} > \haffwts{i}{H2}) 
	\end{equation}
	
	Now combining Equations \ref{eq:max-affwts}, \ref{eq:wts-affwts} we get,
	\begin{align*}
		\htwts{i}{H2} & > \haffwts{i}{H2} \geq \hmaxwts{j}{H2} & \\
		& > \haffwts{i}{H2} \geq \hmaxwts{j}{H2} \geq \htwts{j}{H2}  & [\text{From \obsref{max-wts}}] \\
		& > \htwts{j}{H2}
	\end{align*}
	
	But this equation contradicts with \eqnref{its-wts-ant}. Hence our assumption that $T_i$ will get aborted in $H3$ after getting \finen is not possible. Thus $T_i$ has to commit in $H3$.
\end{proof}
\noindent Next we show that once a transaction $T_i$ becomes \itsen, it will eventually become \finen as well and then committed. We show this change happens in a sequence of steps. We first show that Transaction $T_i$ which is \itsen first becomes \cdsen (or gets committed). We next show that $T_i$ which is \cdsen becomes \finen or get committed. On becoming \finen, we have already shown that $T_i$ will eventually commit. 

Now, we show that a transaction that is \itsen will become \cdsen or committed. To show this, we introduce a few more notations and definitions. We start with the notion of \emph{\depits (dependent-its)} which is the set of \its{s} that a transaction $T_i$ depends on to commit. It is the set of \its of all the transactions in $T_i$'s \cdset in a history $H$. Formally, 

\begin{equation*}
	\hdep{i}{H} = \{\htits{j}{H}|T_j \in \hcds{i}{H}\}
\end{equation*}

\noindent We have the following lemma on the \depits of a transaction $T_i$ and its future \inc $T_j$ which states that \depits of a $T_i$ either reduces or remains the same. 

\begin{lemma}
	\label{lem:depits-fut}
	Consider two histories $H1$ and $H2$ with $H2$ being an extension of $H1$. Let  $T_i$ and $T_j$ be two transactions which are live in $H1$ and $H2$ respectively and $T_i$ is an \inc of $T_j$. In addition, we also have that $\tcts{i}$ is greater than $\tits{i} + 2*L$ in $H1$. Then, we get that $\hdep{j}{H2}$ is a subset of $\hdep{i}{H1}$. Formally, $\langle H1, H2, T_i, T_j: (H1 \sqsubseteq H2) \land (T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (T_i \in \incs{j}{H2}) \land (\htcts{i}{H1} \geq \htits{i}{H1} + 2*L) \implies (\hdep{j}{H2} \subseteq \hdep{i}{H1}) \rangle$. 
\end{lemma}

\begin{proof}
	Suppose $\hdep{j}{H2}$ is not a subset of $\hdep{i}{H1}$. This implies that there is a transaction $T_k$ such that $\htits{k}{H2} \in \hdep{j}{H2}$ but $\htits{k}{H1} \notin \hdep{j}{H1}$. This implies that $T_k$ starts afresh after $H1$ in some history say $H3$ such that $H1 \sqsubset H3 \sqsubseteq H2$. Hence, from \corref{cts-syst} we get the following
	
	\noindent
	\begin{math}
		\htits{k}{H3} > \hsyst{H1} \xrightarrow{\lemref{cts-syst}} \htits{k}{H3} > \htcts{i}{H1} \implies \htits{k}{H3} > \htits{i}{H1} + 2*L \xrightarrow{\htits{i}{H1} = \htits{j}{H2}} \htits{k}{H3} > \htits{j}{H2} + 2*L \xrightarrow[definitions]{\affset, \depits} \htits{k}{H2} \notin \hdep{j}{H2}
	\end{math}
	
	We started with $\tits{k}$ in $\hdep{j}{H2}$ and ended with $\tits{k}$ not in $\hdep{j}{H2}$. Thus, we have a contradiction. Hence, the lemma follows. 
	
	
	
\end{proof}

\noindent Next we denote the set of committed transactions in $T_i$'s \affset in $H$ as \emph{\cis (commit independent set)}. Formally, 

\begin{equation*}
	\hcis{i}{H} = \{T_j| (T_j \in \haffset{i}{H}) \land (\inct{j}{H}) \}
\end{equation*}

\noindent In other words, we have that $\hcis{i}{H} = \haffset{i}{H} - \hcds{i}{H}$. Finally, using the notion of \cis we denote the maximum of \maxwts of all the transactions in $T_i$'s \cis as \emph{\pawts} (partly affecting \wts). It turns out that the value of \pawts affects the commit of $T_i$ which we show in the course of the proof. Formally, \pawts is defined as 

\begin{equation*}
	\hpawts{i}{H} = max\{\hmaxwts{j}{H}|(T_j \in \hcis{i}{H})\}
\end{equation*}

\noindent Having defined the required notations, we are now ready to show that a \itsen transaction will eventually become \cdsen. 

\begin{lemma}
	\label{lem:its-cds}
	Consider a transaction $T_i$ which is live in a history $H1$ and $\tcts{i}$ is greater than or equal to $\tits{i} + 2*L$. If $T_i$ is \itsen in $H1$ then there is an extension of $H1$, $H2$ in which an \inc $T_i$, $T_j$ (which could be same as $T_i$), is either committed or \cdsen. Formally, $\langle H1, T_i: (T_i \in \live{H1}) \land (\htcts{i}{H1} \geq \htits{i}{H1} + 2*L) \land (\itsenb{i}{H1}) \implies (\exists H2, T_j: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land ((T_j \in \comm{H2}) \lor (\cdsenb{j}{H2}))) \rangle$. 
\end{lemma}

\begin{proof}
	We prove this by inducting on the size of $\hdep{i}{H1}$, $n$. For showing this, we define a boolean function $P(k)$ as follows:
	
	\begin{math}
		P(k) = \begin{cases}
			True & \langle H1, T_i: (T_i \in \live{H1}) \land (\htcts{i}{H1} \geq \htits{i}{H1} + 2*L) \land\\ & (\itsenb{i}{H1}) \land 
			 (k \geq |\hdep{i}{H1}|) \implies \\ & (\exists H2, T_j: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land \\
			& ((T_j \in \comm{H2}) \lor (\cdsenb{j}{H2}))) \rangle \\
			False & \text{otherwise}
		\end{cases}
	\end{math}
	
	As can be seen, here $P(k)$ means that if (1) $T_i$ is live in $H1$; (2) $\tcts{i}$ is greater than or equal to $\tits{i} + 2*L$; (3) $T_i$ is \itsen in $H1$ (4) the size of $\hdep{i}{H1}$ is less than or equal to $k$;  then there exists a history $H2$ with a transaction $T_j$ in it which is an \inc of $T_i$ such that $T_j$ is either committed or \cdsen in $H2$. We show $P(k)$ is true for all (integer) values of $k$ using induction. 
	
	\vspace{1mm}
	\noindent
	\textbf{Base Case - $P(0)$:} Here, from the definition of $P(0)$, we get that $|\hdep{i}{H1}| = 0$. This in turn implies that $\hcds{i}{H1}$ is null. Further, we are already given that $T_i$ is live in $H1$ and $\htcts{i}{H1} \geq \htits{i}{H1} + 2*L$. Hence, all these imply that $T_i$ is \cdsen in $H1$. 
	
	\vspace{1mm}
	\noindent
	\textbf{Induction case - To prove $P(k+1)$ given that $P(k)$ is true:} If $|\hdep{i}{H1}| \leq k$, from the induction hypothesis $P(k)$, we get that $T_j$ is either committed or \cdsen in $H2$. Hence, we consider the case when 
	
	\begin{equation}
		\label{eq:hdep-assn}
		|\hdep{i}{H1}| = k + 1
	\end{equation}
	
	Let $\alpha$ be $\hpawts{i}{H1}$. Suppose $\htwts{i}{H1} < \alpha$. Then from \lemref{wts-great}, we get that there is an extension of $H1$, say $H3$ in which an \inc of $T_i$, $T_l$ (which could be same as $T_i$) is committed or is live in $H3$ and has \wts greater than $\alpha$. If $T_l$ is committed then $P(k+1)$ is trivially true. So we consider the latter case in which $T_l$ is live in $H3$. In case $\htwts{i}{H1} \geq \alpha$, then in the analysis below follow where we can replace $T_l$ with $T_i$.
	
	Next, suppose $T_l$ is aborted in an extension of $H3$, $H5$. Then from \lemref{its-wts}, we get that there exists an extension of $H3$, $H4$ in which (1) $T_l$ is live; (2) there is a transaction $T_m$ in $\txns{H4}$; (3) $\htwts{m}{H4} > \htwts{l}{H4}$ (4) $T_m$ is committed in $H5$. 
	
	%Thus in $H4$, we have that $T_l, T_m$ in $\txns{H4}$ and $T_l$ is live in $H4$. 
	Combining the above derived conditions (1), (2), (3) with \lemref{ti|tltl-comt} we get that in $H4$, 
	
	\begin{equation}
		\label{eq:ml-tits}
		\htits{m}{H4} \leq \htits{l}{H4} + 2*L
	\end{equation}
	
	\eqnref{ml-tits} implies that $T_m$ is in $T_l$'s \affset. Here, we have that $T_l$ is an \inc of $T_i$ and we are given that $\htcts{i}{H1} \geq \htits{i}{H1} + 2*L$. Thus from \lemref{aff-tkinc-h1}, we get that there exists an \inc of $T_m$, $T_n$ in $H1$.
	
	Combining \eqnref{ml-tits} with the observations (a) $T_n, T_m$ are \inc{s}; (b) $T_l, T_i$ are \inc{s}; (c) $T_i, T_n$ are in $\txns{H1}$, we get that $\htits{n}{H1} \leq \htits{i}{H1} + 2*L$. This implies that $T_n$ is in $\haffset{i}{H1}$. Since $T_n$ is not committed in $H1$ (otherwise, it is not possible for $T_m$ to be an \inc of $T_n$), we get that $T_n$ is in $\hcds{i}{H1}$. Hence, we get that $\htits{m}{H4} = \htits{n}{H1}$ is in $\hdep{i}{H1}$.  
	
	From \eqnref{hdep-assn}, we have that $\hdep{i}{H1}$ is $k+1$. From \lemref{depits-fut}, we get that $\hdep{i}{H4}$ is a subset of $\hdep{i}{H1}$. Further, we have that transaction $T_m$ has committed. Thus $\htits{m}{H4}$ which was in $\hdep{i}{H1}$ is no longer in $\hdep{i}{H4}$. This implies that $\hdep{i}{H4}$ is a strict subset of $\hdep{i}{H1}$ and hence\\ $|\hdep{i}{H4}| \leq k$. 
	
	\noindent Since $T_i$ and $T_l$ are \inc{s}, we get that $\hdep{i}{H4} = \hdep{l}{H1}$. Thus, we get that 
	
	\begin{equation}
		\label{eqn:hdep-ilh4}
		|\hdep{i}{H4}| \leq k \implies |\hdep{l}{H4}| \leq k
	\end{equation}
	
	\noindent Further, we have that $T_l$ is a later \inc of $T_i$. So, we get that
	
	\begin{equation}
		\label{eqn:cts-its}
		\htcts{l}{H4} > \htcts{i}{H4} \xrightarrow{given} \htcts{l}{H4} > \htits{i}{H4} + 2*L \xrightarrow{\htits{i}{H4} = \htits{l}{H4}} \htcts{l}{H4} > \htits{l}{H4} + 2*L
	\end{equation}
	
	We also have that $T_l$ is live in $H4$. Combining this with Equations \ref{eqn:hdep-ilh4}, \ref{eqn:cts-its} and given the induction hypothesis that $P(k)$ is true, we get that there exists a history extension of $H4$, $H6$ in which an \inc of $T_l$ (also $T_i$), $T_p$ is either committed or \cdsen. This proves the lemma.
\end{proof}

\begin{lemma}
	\label{lem:cds-fin}
	Consider a transaction $T_i$ in a history $H1$. If $T_i$ is \cdsen in $H1$ then there is an extension of $H1$, $H2$ in which an \inc $T_i$, $T_j$ (which could be same as $T_i$), is either committed or \finen. Formally, $\langle H1, T_i: (T_i \in \live{H}) \land (\cdsenb{i}{H1}) \implies (\exists H2, T_j: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land ((T_j \in \comm{H2}) \lor (\finenb{j}{H2})) \rangle$. 
\end{lemma}

\begin{proof}
	In $H1$, suppose $\haffwts{i}{H1}$ is $\alpha$. From \lemref{wts-great}, we get that there is a extension of $H1$, $H2$ with a transaction $T_j$ which is an \inc of $T_i$. Here there are two cases: (1) Either $T_j$ is committed in $H2$. This trivially proves the lemma; (2) Otherwise, $\twts{j}$ is greater than $\alpha$. 
	
	\noindent In the second case, we get that %$\htwts{i}{H1} < \htwts{j}{H2}$. 
	
	\begin{equation}
		\label{eq:ext}
		\begin{split}
			(T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (\cdsenb{i}{H}) \land (T_j \in \incs{i}{H2}) \land \\
			(\htwts{i}{H1} < \htwts{j}{H2})
		\end{split}
	\end{equation}
	
	\noindent Combining the above result with \lemref{cts-wts}, we get that $\htcts{i}{H1} < \htcts{j}{H2}$. Thus the modified equation is 
	
	\begin{equation}
		\label{eq:new-ext}
		\begin{split}
			(T_i \in \live{H1}) \land (T_j \in \live{H2}) \land (\cdsenb{i}{H1}) \land (T_j \in \incs{i}{H2}) \land \\
			(\htcts{i}{H1} < \htcts{j}{H2})
		\end{split}
	\end{equation}
	
	\noindent Next combining \eqnref{new-ext} with \lemref{aff-same}, we get that 
	\begin{equation}
		\label{eq:affs-ij}
		\haffset{i}{H1} = \haffset{j}{H2}
	\end{equation}
	
	\noindent Similarly, combining \eqnref{new-ext} with \lemref{cds-fut} we get that $T_j$ is \cdsen in $H2$ as well. Formally, 
	\begin{equation}
		\label{eq:th-cdsen}
		\cdsenb{j}{H2}
	\end{equation}
	
	Now combining \eqnref{affs-ij} with \lemref{affwts-same}, we get that 
	\begin{equation}
		\label{eq:affwts-same}
		\haffwts{i}{H1} = \haffwts{j}{H2}
	\end{equation}
	
	From our initial assumption we have that $\haffwts{i}{H1}$ is $\alpha$. From \eqnref{affwts-same}, we get that $\haffwts{j}{H2} = \alpha$. Further, we had earlier also seen that $\htwts{j}{H2}$ is greater than $\alpha$. Hence, we have that $\htwts{j}{H2} > \haffwts{j}{H2}$. 
	
	\noindent Combining the above result with \eqnref{th-cdsen}, $\cdsenb{j}{H2}$, we get that $T_j$ is \finen, i.e., $\finenb{j}{H2}$. 
\end{proof}

\noindent Next, we show that every live transaction eventually become \itsen. 

\begin{lemma}
	\label{lem:live-its}
	Consider a history $H1$ with $T_i$ be a transaction in $\live{H1}$. Then there is an extension of $H1$, $H2$ in which an \inc of $T_i$, $T_j$ (which could be same as $T_i$) is either committed or is \itsen. Formally, $\langle H1, T_i: (T_i\in \live{H}) \implies (\exists T_j, H2: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land (T_j \in \comm{H2}) \lor (\itsenb{i}{H})) \rangle$. 
\end{lemma}

\begin{proof}
	\noindent We prove this lemma by inducting on \its. 
	
	\vspace{1mm}
	\noindent
	\textbf{Base Case - $\tits{i} = 1$:} In this case, $T_i$ is the first transaction to be created. There are no transactions with smaller \its. Thus $T_i$ is trivially \itsen. 
	
	\vspace{1mm}
	\noindent
	\textbf{Induction Case:} Here we assume that for any transaction $\tits{i} \leq k$ the lemma is true. 
\end{proof}

Combining these lemmas gives us the result that for every live transaction $T_i$ there is an incarnation $T_j$ (which could be the same as $T_i$) that will commit. This implies that every \aptr eventually commits. The follow lemma captures this notion.

\begin{theorem}
	\label{thm:hwtm-com}
	Consider a history $H1$ with $T_i$ be a transaction in $\live{H1}$. Then there is an extension of $H1$, $H2$ in which an \inc of $T_i$, $T_j$ is committed. Formally, $\langle H1, T_i: (T_i\in \live{H}) \implies (\exists T_j, H2: (H1 \sqsubset H2) \land (T_j \in \incs{i}{H2}) \land (T_j \in \comm{H2})) \rangle$. 
\end{theorem}

\begin{proof}
	%Induction on \its. 
	Here we show the states that a transaction $T_i$ (or one of it its \inc{s}) undergoes before it commits. In all these transitions, it is possible that an \inc of $T_i$ can commit. But to show the worst case, we assume that no \inc of $T_i$ commits. Continuing with this argument, we show that finally an \inc of $T_i$ commits. 
	
	Consider a live transaction $T_i$ in $H1$. Then from \lemref{live-its}, we get that there is a history $H2$, which is an extension of $H1$, in which $T_j$ an \inc of $T_i$ is either committed or \itsen. If $T_j$ is \itsen in $H2$, then from \lemref{its-cds}, we get that $T_k$, an \inc of $T_j$, will be \cdsen in a extension of $H2$, $H3$ (assuming that $T_k$ is not committed in $H3$). 
	
	From \lemref{cds-fin}, we get that there is an extension of $H3$, $H4$ in which an \inc of $T_k$, $T_l$ will be \finen assuming that it is not committed in $H4$. Finally, from \lemref{enbd-ct}, we get that there is an extension of $H4$ in which $T_m$, an \inc of $T_l$, will be committed. This proves our theorem.
\end{proof}

\noindent From this theorem, we get the following corollary which states that any history generated by \ksftm is $\stfdm$.

\begin{corollary}
	\ksftm algorithm ensures \stfdm. 
\end{corollary}





==> Arxiv SFKOSTM SSS19/ap-counters.tex <==
%\clearpage
\subsection{Pseudo code of Counter Application}
\label{apn:countercode}
To analyze the absolute benefit of starvation-freedom, we use a \emph{Counter Application} which provides us the flexibility to create a high contention environment where the probability of transactions undergoing starvation on an average is very high. In this subsection we describe the detailed functionality of \emph{Counter Application} though pseudo code as follows:    
%OP\_LT\_SEED is defined as number of operations per transaction, T\_OBJ\_SEED is defined as number of transaction objects in the system, TRANS\_LT defines the total number of transactions to be executed in the system, and READ\_PER is the percentage of read operation which is used to define various workloads.
\label{apn:conters}
\begin{algorithm}  
	\caption{\emph{main()}: The main function invoked by \emph{Counter Application}.} \label{algo:main} 
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{143}\makeatother		
	\State /*Each thread $th_i$ log \emph{abort counts, average time taken by each transaction to commit and worst case time} (maximum time to commit the transaction) in $abortCount_{th_i}$, $timeTaken_{th_i}$ and $worstTime_{th_i}$ respectively;*/
	%	\State abortCount[threads] 
	%	\State \Comment{To log average time taken by each transaction to commit}
	%	\State $time\_taken[$NUMTHREADS$]$ 
	%	\State \Comment{To log the time of longest running transaction by each thread, worst case time}
	%	\State $worst\_time[$NUMTHREADS$]$
		\ForAll{(numOfThreads)} /*Multiple threads call the helper function*/
		\State \emph{helperFun()};
		\EndFor 
		\ForAll{(numOfThreads)} 
		\State /*Join all the threads*/ 
		\EndFor 
%		\State Initialize the \emph{maxWorstTime}, \emph{totalAbortCount} and \emph{avgTimeTaken} as 0.
		\ForAll{(numOfThreads)}
		\If{($maxWorstTime$ $<$ $worstTime_{th_i}$)}
		\State /*Calculate the \emph{Maximum Worst Case Time}*/
		\State $maxWorstTime$ = $worstTime_{th_i}$; 
		\EndIf
		\State /*Calculate the \emph{Total Abort Count}*/
		\State $totalAbortCount$ += $abortCount_{th_i}$;
		\State /*Calculate the \emph{Average Time Taken}*/
		\State $AvgTimeTaken$ /= $TimeTaken_{th_i}$;
		\EndFor
	\end{algorithmic}
\end{algorithm}

\vspace{1mm}
\begin{algorithm} [H] 
	\caption{\emph{helperFun()}:Multiple threads invoke this function.} \label{algo:testFunc} 
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{160}\makeatother		
	    \State Initialize the Transaction Count $txCount_i$ of $T_i$ as 0;
		\While{(\emph{numOfTransac\texttt{}tions})} /*Execute until number of  transactions are non zero*/
%		    \State \Comment{Log the time at the start of every transaction}
		    \State $startTime_{th_i}$ = timeRequest(); /*get the start time of thread $th_i$*/%$begin\_time = time\_request()$
		    \State\Comment{Execute the transactions $T_i$ by invoking \emph{testSTM} functions;}
		    \State $abortCount_{th_i}$ = $testSTM_i()$;
		    \State Increment the $txCount_i$ of $T_i$ by one.
		    \State $endTime_{th_i}$ = timeRequest(); /*get the end time of thread $th_i$*/
		    \State /*Calculate the \emph{Total Time Taken} by each thread $th_i$*/
		    \State $timeTaken_{th_i}$ += ($endTime_{th_i}$ - $startTime_{th_i}$);
		    \State /*Calculate the \emph{Worst Case Time} taken by each thread $th_i$*/
		    \If{($worstTime_{th_i}$ $<$ ($endTime_{th_i}$ - $startTime_{th_i}$))}
		    \State $worstTime_{th_i}$ = ($endTime_{th_i}$ - $startTime_{th_i}$); %/*Update the worst case time*/
		    \EndIf
		    \State Atomically, decrement the \emph{numOfTransactions};
%		    \State $abort\_count[thread\_id] = test\_function()$
%		    \State $transaction\_count++$
\cmnt{
		    			\algstore{myalg}
		\end{algorithmic}
	\end{algorithm}
	\begin{algorithm}
		\begin{algorithmic}
			\algrestore{myalg}
}			
%		    \State\Comment{Log the time at the end of every transaction}
%		    \State $end\_time = time\_request()$
%		    \State $time\_taken[thread\_id] += (end\_time - begin\_time)$
%		    \If{($worst\_time[thread_id] < (end\_time - begin\_time)$)}
%		    \State $worst\_time[thread_id] = (end\_time - begin\_time)$
%		    \EndIf
%		    \State TRANS\_LT -= 1
		\EndWhile
		\State /*Calculate the \emph{Average Time} taken by each thread $th_i$*/
		\State $TimeTaken_{th_i}$ /= $txCount_i$;
	\end{algorithmic}
\end{algorithm}

\vspace{1mm}
\begin{algorithm} [H] 
	\caption{$testSTM_i()$: Main function which executes the methods of the transaction $T_i$ (or $i$) by thread $th_i$.} \label{algo:testFunx} 
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{177}\makeatother			
%    \State Transaction $\ast$T = new Transaction;
%    \State $T\rightarrow g\_its$ = NIL
%    \State $local\_abort\_count$ = 0
 %   \State label:
    \While{(\emph{true})}
    \If{(\emph{i.its} != \emph{nil})}\label{lin:begin}
%    \State \emph{its} = \emph{i.its};%$its = T\rightarrow g\_its$
    \State \emph{STM\_begin(i.its)};  /*If $T_i$ is an incarnation*/
	\Else
	\State \emph{STM\_begin(nil)}; /*If $T_i$ is first invocation*/
    \EndIf
    \ForAll{(\emph{numOfMethods})}
    \State $k_i$ = rand()\%totalKeys;/*Select the key randomly*/%$t\_obj = rand()\%T\_OBJ\_SEED$
    \State $m_i$ = rand()\%100;/*Select the method randomly*/%$randVal = rand()\%OP\_SEED$
    		\Switch{($m_i$)}\label{lin:cminer8}
    \Case{($m_i$ $\leq$ \emph{STM\_lookup}()):}\label{lin:cminer9}
    \State $v$ $\gets$ \emph{STM\_lookup{($k_i$)}}; /*Lookup key $k$ from a shared memory*/\label{lin:cminer10}
    \If{($v$ == $abort$)}\label{lin:cminer11}
    \State $txAbortCount_i++$; /*Increment the transaction abort count*/
    \State goto \Lineref{begin};\label{lin:cminer12}
    \EndIf\label{lin:cminer13}
    \EndCase
    \Case{(\emph{STM\_lookup()} $<$ $m_i$ $\leq$ \emph{STM\_insert}()):} \label{lin:cminer14}
    \State /*Insert key $k_i$ into $T_i$ local memory with value $v$*/\label{lin:cminer15}
    \State \emph{STM\_insert($k_i, v$)}; \label{lin:cminer16}
    \EndCase
    \Case{(\emph{STM\_insert()} $<$ $m_i$ $\leq$ \emph{STM\_delete}()}):
    \State /*Actual deletion happens after successful \emph{STM\_tryC()}*/
    \State \emph{STM\_delete($k_i$)};
    \EndCase
    \Case{default:}\label{lin:cminer17}
    \State /*Neither lookup nor insert/delete on shared memory*/\label{lin:cminer18}
    %\State execute curStep;\label{lin:cminer19}
    \EndCase
    \State $v$ = \emph{STM\_tryC()}; /*Validate all the methods of $T_i$ in tryC*/
    \If{($v$ == \emph{abort})}
     \State $txAbortCount_i++$;
        \State goto \Lineref{begin};
  %      \EndIf
   % \Else
    %\State $stm$-$write(t\_obj, value)$
    \EndIf
        \EndSwitch
    \EndFor
    \State return $\langle txAbortCount_i \rangle$;
    \EndWhile
	\end{algorithmic}
\end{algorithm}

==> Arxiv SFKOSTM SSS19/ap-gop.tex <==
\section{Graph Characterization of Co-opacity and SF-SVOSTM Correctness}
\label{sec:gcofo}

This section describes the graph characterization of the history $H$ which helps to prove the correctness of STMs. We follow the  graph characterization by Guerraoui and Kapalka \cite{tm-book} and modified it for sequential histories with high-level methods to prove the correctness of SF-SVOSTM. 

As discussed in \secref{sm}, SF-SVOSTM executes high-level methods through transactions on history $H$ which internally invoke multiple read-write (or lower-level) operations including invocation and response known as \emph{events} (or $evts$). So, high-level methods are interval instead of dots (atomic). Methods of same transaction $T_i$ are always real-time ordered, i.e., none of the methods of $T_i$ overlaps each other. But due to the concurrent execution of history $H$ with methods are interval, two methods from different transactions may overlap. Thus, we order the overlapping methods of transactions based on their \emph{linearization point (LP)}. We consider \emph{first unlocking point} of each successful method as the \emph{LP} of the respective method.

In the concurrent execution of a history $H$, we make high-level methods of a transaction as atomic based on their \emph{linearization points (LPs)} as defined above. But, as we know from \secref{sm}, a transaction internally invokes multiple high-level methods and transactions are overlapping to each other in concurrent history $H$. So, with the help of \emph{graph characterization of co-opacity}, SF-SVOSTM ensures the atomicity of the transaction. 
%\textbf{\textit{M\_Order$_H$:}}% It stands for method order of history H in which methods of transactions are interval (consists of invocation and response of a method) instead of dot (atomic). Because of having method as an interval, methods of different transactions can overlap. To prove the correctness as \textit{(co-opacity)} for SF-OSTM and \textit{(local-opacity)} for SF-KOSTM, we need to order the overlapping methods. First unlocking point of each successful method is the linearization point (or LP).




A graph for the conflict-opacity (co-opacity) is represented as $\copg{H}{\ll} = (V, E)$ which consists of $V$ vertices and $E$ edges. Here, each committed transaction is consider as a vertex and edges are as follows:
\begin{itemize}
	\item \textit{Conflict (or \confc{}) edge}: The conflict edges between two transactions depends on the conflicts between them. Two transactions $T_i$ and $T_j$ of the sequential history are said to be in conflict, if one of the following holds:
	\begin{itemize}
		\item \textbf{tryC-tryC} conflict: Two transactions $T_i$ \& $T_j$ are in tryC-tryC conflict (1) If $T_i$ and $T_j$ are committed; (2) Both $T_i$ \& $T_j$ update the same key $k$ of the \tab{}, $ht$, i.e., $(\langle ht,k \rangle \in \udset{T_i}) \land (\langle ht,k \rangle \in \udset{T_j})$, here $\udset{T_i}$ is set of keys in which $T_i$ performs update methods (or $\upmt{s}$); (3) and \tryc{()} of $T_i$ has completed before \tryc{()} of $T_j$, i.e., $\tryc_i() \prec_{H}^{\mr} \tryc_j()$. 
		
		\item \textbf{tryC-rv} conflict: Two transactions $T_i$ \& $T_j$ are in tryC-rv conflict (1) If $T_i$ has updated the key $k$ of \tab{}, $ht$ and committed; (2) After that $T_j$ invokes a \rvmt{} $rvm_{j}$ on the key same $k$ of \tab{} $ht$ and returns the value updated by $T_i$, i.e., $\tryc_i \prec_{H}^{\mr} \rvm_{j}$.% Same conflict is preserved by the subsequent \mth{s} of $T_j$, we call it \emph{conflict inheritance}. 
		
		\item \textbf{rv-tryC} conflict: Two transactions $T_i$ \& $T_j$ are in rv-tryC conflict (1) $T_i$ invokes a \rvmt{} $rvm_{i}$ on the key $k$ of \tab{} $ht$ and returns the value updated by $T_k$, i.e., $\tryc_k \prec_{H}^{\mr} \rvm_{i}$; (2) After that $T_j$ update the same key $k$ of the \tab{}, $ht$, i.e., $(\langle ht,k \rangle \in \udset{T_j})$ and $T_j$ returns commit, i.e., $\rvm_{i} \prec_{H}^{\mr} \tryc_j$.
	\end{itemize}
	If any of the above defined conflicts occur then conflict edge goes from $T_i$ to $T_j$. As described in \secref{sm}, \emph{STM\_lookup()}, and \emph{STM\_delete()} return the value from underlying data structure so, we called these methods as \emph{return value methods (or $\rvmt{s}$)}. Whereas, \emph{STM\_insert()}, and \emph{STM\_delete()} are updating the underlying data structure after successful \emph{STM\_tryC()} so, we called these as \emph{update} \mth{s} (or $\upmt{s}$). So, the conflicts are defined between the \mth{s} that accesses the shared memory.  \emph{(STM\_tryC$_i$(), STM\_tryC$_j$()), (STM\_tryC$_i$(), STM\_lookup$_j$()), (STM\_lookup$_i$(), STM\_tryC$_j$()), (STM\_tryC$_i$(), STM\_delete$_j$()) and (STM\_delete$_i$(), STM\_tryC$_j$())} are the possible conflicting \mth{s}.  
	
	\item \textit{real-time (or \rt) edge}: If transaction $T_i$ returns commit before the beginning of other transaction $T_j$ then real-time edge goes from $T_i$ to $T_j$. Formally, ($\tryc_i() \prec_{H}$ \emph{STM\_begin$_j$()}) $\implies$  $T_i$ $\rightarrow$ $T_j$.
	
\end{itemize}

For better understanding, we consider a history $H$: $l_1(ht, k_5, nil), l_2(ht, k_7, nil),\\ d_1(ht, k_6, nil), C_1, i_2(ht, k_5, v_2), C_2, l_3(ht, k_5, v_2), i_3(ht, k_7, v_3), C_3$ and show the time line view of it in \figref{gco}.(a). We construct $\copg{H}{\ll} = (V, E)$ shown in \figref{gco}.(b). There exist a (rv-tryC) edge between $T_1$ to $T_2$ because $T_2$ updates the key $k_5$ with value $v_2$ after $T_1$ lookups it. $T_3$ begins after the commit of $T_1$ and $T_2$ so, \rt{} edges are going from $T_1$ to $T_3$ and $T_2$ to $T_3$. Here, $T_3$ lookups key $k_5$ after updated by $T_2$ and returns the value $v_2$. So, (tryC-rv) edge  is going from $T_2$ to $T_3$. Hence, $H$ constructs an acyclic graph (CG) with equivalent serial schedule $T_1 T_2 T_3$.

\begin{figure}
	\centerline{
		\scalebox{0.4}{\input{figs/co.pdf_t}}}
	\captionsetup{justification=centering}
	\caption{Illustration of Graph Characterization of Co-opacity}
	\label{fig:gco}
\end{figure}


\begin{lemma}
	\label{lem:concycle}
For any \legal{} \tseq{} history $S$ the conflict graph $\copg{S, \ll_S}$ is acyclic.
\end{lemma}

\begin{proof}
	\tseq{} history $S$ consists of multiple transactions, we order all the them into real-time order on the basis of their increasing order of timestamp (TS). For example, consider two transaction $T_i$ and $T_j$ with $TS(T_i)$ is less than $TS(T_j)$ then $T_i$ will occur before $T_j$ in $S$. Formally, $TS(T_i) < TS(T_j)$ $\Leftrightarrow T_i <_S T_j$.	 To proof the order between transactions, we analyze all the edges of $\copg{S, \ll_S}$ one by one: 
	\begin{itemize}
		\item \rt{} edges: It follow that any transaction begin after commit of previous transaction only. Hence, all the \rt{} edges go from a lower TS transaction $T_i$ to higher TS transaction $T_j$ and follow timestamp order. 
		
		\item \confc{} edges: If any transaction $T_j$ lookups key $k$ from $T_i$ in $S$ then $T_i$ has to be committed before invoking of lookup of $T_j$. Similarly, other conflicting edges are following TS order as $TS(T_i) < TS(T_j)$ $\Leftrightarrow T_i <_S T_j$. Thus, all the \confc{} edges go from a lower TS transaction to higher TS transaction.
		
	%	\item \mv{} edges: Consider a successful \rvmt{} $\rvm_j(k_x, u)$ and a committed transaction $T_k$ writing $v$ to $k_x$ where $u \neq v$. Let $c_i$ be $\rvm_j(k_x, u)$'s \lastw. Thus, $\up_i(k_{x,i}, u) \in \evts{T_i}$. Thus, we have that $\ord{T_i} < \ord{T_j}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_k} < \ord{T_i}$. We now have that $T_k \ll T_i$. In this case, the mv edge is from $T_k$ to $T_i$. (2) Suppose $\ord{T_i} < \ord{T_k}$ which implies that $T_i \ll T_k$. Since $S$ is legal, we get that $\ord{T_j} < \ord{T_k}$. This case also implies that there is an edge from $\ord{T_j}$ to $\ord{T_k}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 
		
		%\item \mv{} edges: Consider a successful \rvmt{} $\rvm_k(k_x, v)$ and a committed transaction $T_i$ writing $u$ to $k_x$ where $u \neq v$. Let $c_j$ be $\rvm_k(k_x, v)$'s \lastw. Thus, $\up_j(k_{x,j}, v) \in \evts{T_j}$. Thus, we have that $\ord{T_j} < \ord{T_k}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_i} < \ord{T_j}$. We now have that $T_i \ll T_j$. In this case, the mv edge is from $T_i$ to $T_j$. (2) Suppose $\ord{T_j} < \ord{T_i}$ which implies that $T_j \ll T_i$. Since $S$ is legal, we get that $\ord{T_k} < \ord{T_i}$. This case also implies that there is an edge from $\ord{T_k}$ to $\ord{T_i}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 
	\end{itemize}
	Hence, all the edges of $\copg{S, \ll_S}$ are following increasing of the TS of the transactions, i.e. all the edges goes from lower TS transaction to higher TS transaction in $S$. Conflict graph $\copg{S, \ll_S}$ is acyclic.
\end{proof}



\begin{theorem}
	\label{thm:cocg}
	A history H is co-opaque iff $\copg{H}{\ll_H}$ is acyclic.
\end{theorem}

\begin{proof}
	\textbf{(if part):} First, we consider $\copg{H}{\ll_H}$ is acyclic and we need to prove that history $H$ is co-opaque. Since $\copg{H}{\ll_H}$ is acyclic, we apply topological sort on $\copg{H}{\ll_H}$ and generate a \tseq{} history $S$ such that $S$ is equivalent to $\overline{H}$.
	$\copg{H}{\ll_H}$ maintains real-time edges as well and $S$ has been generated from it. So, $S$ also respect real-time order \rt{} as $H$. Formally, $\prec_H^{RT} \subseteq \prec_S^{RT}$.
	
	Since $\copg{H}{\ll_H}$ maintains all the conflicting (or \confc{}) edges as well defined above. $S$ has been generated by applying topological sort on $\copg{H}{\ll_H}$. So, $S$ respects all the conflicting edges present in $H$. Formally, $\prec_H^{Conf} \subseteq \prec_S^{Conf}$. 
	
	It can be seen in $\copg{H}{\ll_H}$ that \rvmt{s()} on any key $k$ by transaction $T_i$ returns the value written on $k$ by previous closest committed transaction $T_j$. $H$ maintains all the \rvmt{s()} in conflicting (or \confc{}) edges of $\copg{H}{\ll_H}$. Since $S$ has been generated by applying topological sort on $\copg{H}{\ll_H}$. So, $S$ returns all the value of the \rvmt{s()} from previous closest committed transactions. Hence, $S$ is $legal$.
	
	$S$ satisfies all the properties of \emph{co-opacity} and equivalent to $H$ because $S$ has been generated from the topological sort on $\copg{H}{\ll_H}$. Hence, history H is co-opaque.
	
%	Here we have a version order $\ll_H$ such that $G_H=\opg{H}{\ll}$ is acyclic. Now we have to show that $H$ is opaque. Since the $G_H$ is acyclic, a topological sort can be obtained on all the vertices of $G_H$. Using the topological sort, we can generate a \tseq{} history $S$. It can be seen that $S$ is equivalent to $\overline{H}$. Since $S$ is obtained by a topological sort on $G_H$ which maintains the real-time edges of $H$, it can be seen that $S$ respects the \rt{} order of $H$, i.e $\prec_H^{RT} \subseteq \prec_S^{RT}$. 
	
	%Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_j(k_x, u)$ such that its \lastw{} in $S$ is $c_k$ and $T_k$ updates value $v (\neq u)$ to $k_x$, i.e $\up_k(k_{x,k}, v) \in \evts{T_k}$. Further, we also have that there is a transaction $T_i$ that insert $u$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Since $S$ is \valid, as shown above, we have that $T_i \prec_{S}^{RT} T_k \prec_{S}^{RT} T_j$.
	
	%Now in $\ll_H$, if $k_{x,k} \ll_H k_{x,i}$ then there is an edge from $T_k$ to $T_i$ in $G_H$. Otherwise ($k_{x,i} \ll_H k_{x,k}$), there is an edge from $T_j$ to $T_k$. Thus in either case $T_k$ can not be in between $T_i$ and $T_j$ in $S$ contradicting our assumption. This shows that $S$ is legal. 
	
	
	%Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_k(k_x, v)$ such that its \lastw{} in $S$ is $c_i$ and $T_i$ updates value $u (\neq v)$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Further, we also have that there is a transaction $T_j$ that insert $v$ to $k_x$, i.e $\up_j(k_{x,j}, v) \in \evts{T_j}$. Since $S$ is \valid, as shown above, we have that $T_j \prec_{S}^{RT} T_i \prec_{S}^{RT} T_k$.
	
	%Now in $\ll_H$, if $k_{x,i} \ll_H k_{x,j}$ then there is an edge from $T_i$ to $T_j$ in $G_H$. Otherwise ($k_{x,j} \ll_H k_{x,i}$), there is an edge from $T_k$ to $T_i$. Thus in either case $T_i$ can not be in between $T_j$ and $T_k$ in $S$ contradicting our assumption. This shows that $S$ is legal. 
	
	\textbf{(Only if part):} Now, we consider $H$ is co-opaque and we have to prove that $\copg{H}{\ll_H}$ is acyclic.
	Since $H$ is co-opaque there exists an equivalent  \legal{} \tseq{} history $S$ to $\overline{H}$ which maintains real-time (\rt{}) and conflict ($Conf$) order of $H$. From the \lemref{concycle}, we can say that conflict graph $\copg{S, \ll_S}$ is acyclic. As we know, $\copg{H}{\ll_H}$ is the subgraph of $\copg{S, \ll_S}$.
	Hence, $\copg{H}{\ll_H}$ is acyclic.
	
	
	
	
	% Since $H$ is opaque there exists a \legal{} \tseq{} history $S$ equivalent to $\overline{H}$ such that it respects real-time order of $H$. Now, we define a version order for $S$, $\ll_S$ as in \defref{seqver}. Since the $S$ is equivalent to $\overline{H}$, $\ll_S$ is applicable to $\overline{H}$ as well. From \lemref{seracycle}, we get that $G_S=\opg{S}{\ll_S}$ is acyclic. Now consider $G_H = \opg{\overline{H}}{\ll_S}$. The vertices of $G_H$ are the same as $G_S$. Coming to the edges, 
	
	\cmnt{
	\begin{itemize}
		\item \rt{} edges: We have that $S$ respects real-time order of $H$, i.e $\prec_{H}^{RT} \subseteq \prec_{S}^{RT}$. Hence, all the \rt{} edges of $H$ are a subset of $S$. 
		
		\item \rvf{} edges: Since $\overline{H}$ and $S$ are equivalent, the return value-from relation of $\overline{H}$ and $S$ are the same. Hence, the \rvf{} edges are the same in $G_H$ and $G_S$. 
		
		\item \mv{} edges: Since the version-order and the \op{s} of the $H$ and $S$ are the same, from \lemref{eqv_hist_mvorder} it can be seen that $\overline{H}$ and $S$ have the same \mv{} edges as well.
	\end{itemize}
	
	Thus, the graph $G_H$ is a subgraph of $G_S$. Since we already know that $G_S$ is acyclic from \lemref{seracycle}, we get that $G_H$ is also acyclic. 

}
\end{proof}
\cmnt{
To prove that a STM system satisfies opacity, it is useful to consider graph characterization of histories. In this section, we describe the graph characterization of Guerraoui and Kapalka \cite{tm-book} modified for sequential histories.

Consider a history $H$ which consists of multiple version for each \tobj. The graph characterization uses the notion of \textit{version order}. Given $H$ and a \tobj{} $k$, we define a version order for $k$ as any (non-reflexive) total order on all the versions of $k$ ever created by committed transactions in $H$. It must be noted that the version order may or may not be the same as the actual order in which the version of $k$ are generated in $H$. A version order of $H$, denoted as $\ll_H$ is the union of the version orders of all the \tobj{s} in $H$. 

Consider the history $H3$ as shown in \figref{mvostm3} $: lu_1(ht, k_{x, 0}, null), lu_2(ht, k_{x, 0}, null),\\ lu_1(ht, k_{y, 0}, null), lu_3(ht, k_{z, 0}, null), ins_1(ht, k_{x, 1}, v_{11}), ins_3(ht,
k_{y, 3}, v_{31}), ins_2(ht, \\k_{y, 2}, v_{21}), ins_1(ht, k_{z, 1}, v_{12}), c_1, c_2, lu_4(ht, k_{x, 1}, v_{11}), lu_4(ht, k_{y, 2}, v_{21}), ins_3(ht, k_{z, 3},\\ v_{32}), c_3, lu_4(ht, k_{z, 1}, v_{12}), lu_5(ht, k_{x, 1}, v_{11}), lu_6(ht, k_{y, 2}, v_{21}), c_4, c_5, c_6$. Using the notation that a committed transaction $T_i$ writing to $k_x$ creates a version $k_{x, i}$, a possible version order for $H3$ $\ll_{H3}$ is: $\langle k_{x, 0} \ll k_{x, 1} \rangle, \langle k_{y, 0} \ll k_{y, 2} \ll k_{y, 3} \rangle, \langle k_{z, 0} \ll k_{z, 1} \ll k_{z, 3} \rangle $.}
\cmnt{
Consider the history $H4: l_1(ht, k_{x, 0}, NULL) l_2(ht, k_{x, 0}, NULL) l_1(ht, k_{y, 0}, NULL) l_3(ht, k_{z, 0},\\ NULL) i_1(ht, k_{x, 1}, v_{11}) i_3(ht, k_{y, 3}, v_{31}) i_2(ht, k_{y, 2}, v_{21}) i_1(ht, k_{z, 1}, v_{12}) c_1 c_2 l_4(ht, k_{x, 1}, v_{11}) l_4(ht,\\ k_{y, 2}, v_{21}) i_3(ht, k_{z, 3}, v_{32}) c_3 l_4(ht, k_{z, 1}, v_{12}) l_5(ht, k_{x, 1}, v_{11}), l_6(ht, k_{y, 2}, v_{21}) c_4, c_5, c_6$. In our representation, we abbreviate \tins{} as $i$, \tdel{} as $d$ and \tlook{} as $l$. Using the notation that a committed transaction $T_i$ writing to $k_x$ creates a version $k_{x, i}$, a possible version order for $H4$ $\ll_{H4}$ is: $\langle k_{x, 0} \ll k_{x, 1} \rangle, \langle k_{y, 0} \ll k_{y, 2} \ll k_{y, 3} \rangle, \langle k_{z, 0} \ll k_{z, 1} \ll k_{z, 3} \rangle $. 
}
%\vspace{-.3cm}
\cmnt{
\begin{figure}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.45}{\input{figs/ppopp2.pdf_t}}}
	\caption{History $H3$ in time line view}
	\label{fig:mvostm3}
\end{figure}
}
%\vspace{-.3cm}
\cmnt{
\begin{figure}[tbph]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.45}{\input{figs/mvostm3.pdf_t}}}
	\caption{History $H4$ in time line view}
	\label{fig:mvostm3}
\end{figure}
}


\begin{theorem}
	\label{thm:coopqhprev}
	A legal SF-SVOSTM history $H$ is co-opaque iff $\copg{H}{\ll_H}$ is acyclic.
\end{theorem}
\begin{proof}
	\textbf{(if part):} First, we consider $H$ is \emph{legal} and $\copg{H}{\ll_H}$ is acyclic then we need to prove that history $H$ is co-opaque. Since $\copg{H}{\ll_H}$ is acyclic, we apply topological sort on $\copg{H}{\ll_H}$ and obtained a \tseq{} history $S$ which is equivalent to $\overline{H}$.
	%Since $\copg{H}{\ll_H}$ maintains real-time as well as conflict edges and $S$ has been generated from it. So, 
	$S$ also respect real-time edges (or \rt{}) and \confc{} edges as $\overline{H}$. Formally, $S$ respects $\prec$$^{RT}_H$ = $\prec$$^{RT}_{\overline{H}}$ and $\prec$$^{Conf}_H$ = $\prec$$^{Conf}_{\overline{H}}$. %Formally, $\prec_H^{RT} \subseteq \prec_S^{RT}$.
	
	Since Conflict relation between two methods of SF-SVOSTM in $S$ are also present in $\overline{H}$. Formally, $\prec_{\overline{H}}^{Conf} \subseteq \prec_S^{Conf}$. Given that $H$ is \emph{legal} which implies that  $\overline{H}$ is also \emph{legal}. So, we can say that $S$ is \emph{legal}. Collectively, $H$ satisfies all the necessary conditions of \emph{co-opacity}. Hence, history $H$ is co-opaque.
	
	\textbf{(Only if part):} Now, we consider $H$ is co-opaque and legal then we have to prove that $\copg{H}{\ll_H}$ is acyclic.
	Since $H$ is co-opaque there exists an equivalent  \legal{} \tseq{} history $S$ to $\overline{H}$ which maintains real-time (\rt{}) and conflict ($Conf$) order of $H$, i.e, S respects $\prec$$^{RT}_H$ and $\prec$$^{Conf}_H$ ((from the definition of co-opacity\cite{KuznetsovPeri:Non-interference:TCS:2017})). So, we can observe from the conflict graph construction that $\copg{H}{\ll_H}$ = $\copg{H}{\ll_{\overline{H}}}$ and both are the subgraph of $\copg{S}{\ll_S}$. Since $S$ is a  \tseq{} history, so $\copg{S}{\ll_S}$ is acyclic. As we know, any subgraph of any acyclic graph is also acyclic and $\copg{H}{\ll_H}$ is the subgraph of $\copg{S}{\ll_S}$. %($\copg$($\bar{H}$)=$\copg$(H)) is a sub graph of CG(S). Since S is sequential, it can be inferred that CG(S) is acyclic. Any sub graph of an acyclic graph is also acyclic. Hence CG(H) is also acyclic. We can say that conflict graph $\copg{S, \ll_S}$ is acyclic. As we know, $\copg{H}{\ll_H}$ is the subgraph of $\copg{S, \ll_S}$.
	Hence, $\copg{H}{\ll_H}$ is acyclic.

	
	
	
	
	
	
	%A history H is co-opaque iff CG(H) is acyclic.(Only if) If H is co-opaque and legal, then CG(H) is acyclic: Since H is co-opaque, there exists a legal t-sequential history S equivalent to $\bar{H}$ and S respects $\prec$$^{RT}_H$ and $\prec$$^{CO}_H$ (from co-opacity\cite{KuzPer:NI:TCS:2017}). Thus from the conflict graph construction we have that (CG($\bar{H}$)=CG(H)) is a sub graph of CG(S). Since S is sequential, it can be inferred that CG(S) is acyclic. Any sub graph of an acyclic graph is also acyclic. Hence CG(H) is also acyclic.(if) If H is legal and CG(H) is acyclic then H is co-opaque:	Suppose that CG(H) = CG($\bar{H}$) is acyclic. Thus we can
%perform a topological sort on the vertices of the graph and
%%sequential schedule S that is equivalent to $\bar{H}$. Moreover, by construction,. 
	
	%Since every two operations related by the conflict relation in S are also related by $\prec$$^{CO}_{\bar{H}}$, we obtain $\prec$$^{CO}_{\bar{H}}$ $\subseteq$ $\prec$$^{CO}_S$. Since H is legal, $\bar{H}$ is also legal. We get that S is also legal. This satisfies all the conditions necessary for H to be co-opaque. Hence, Any history $H$ generated by SF-OSTM satisfies co-opacity.
\end{proof}

\begin{theorem}
	\label{thm:coopq}
	Any legal history $H$ generated by SF-SVOSTM satisfies co-opacity.
\end{theorem}

\begin{proof}
In order to prove this, we construct the co-opacity graph $\copg{H}{\ll}$ generated by SF-SVOSTM algorithm and prove that $\copg{H}{\ll}$ graph is acyclic. After that with the help of \thmref{coopqhprev}, we can say that generated $\copg{H}{\ll}$ graph is acyclic so any legal history $H$ generated by SF-SVOSTM is co-opaque.

To prove the $\copg{H}{\ll}$ generated by SF-SVOSTM algorithm is acyclic. We construct $\copg{H}{\ll} = (V, E)$ which consists of $V$ vertices and $E$ edges. Here, each committed transaction is consider as a vertex and edges are as follows:
\begin{itemize}
	\item \textit{real-time (or \rt) edge}: If transaction $T_i$ returns commit before the beginning of other transaction $T_j$ then real-time edge goes from $T_i$ to $T_j$ in SF-SVOSTM. Formally, ($\tryc_i() \prec_{H}$ \emph{STM\_begin$_j$}()) $\implies$ $TS(T_i) < TS(T_j)$ $\implies$ $T_i$ $\rightarrow$ $T_j$.
	
	\item \textit{conflict (or \confc{}) edge}: The conflict edges between two transactions depends on the conflicts between them. Two transactions $T_i$ and $T_j$ of the sequential history are said to be in conflict, if both of them  access same key $k$ and at least one transaction performs \emph{update} method. As described in \secref{sm}, \emph{STM\_lookup()}, and \emph{STM\_delete()} return the value from underlying data structure so, we called these methods as \emph{return value methods (or $\rvmt{s}$)}. Whereas, \emph{STM\_insert()}, and \emph{STM\_delete()} are updating the underlying data structure after successful \emph{STM\_tryC()} so, we called these as \emph{update} \mth{s} (or $\upmt{s}$). So, the conflicts are defined between the \mth{s} that accesses the shared memory.  \emph{(STM\_tryC$_i$(), STM\_tryC$_j$()), (STM\_tryC$_i$(), STM\_lookup$_j$()), (STM\_lookup$_i$(), STM\_tryC$_j$()), (STM\_tryC$_i$(), STM\_delete$_j$()) and (STM\_delete$_i$(), STM\_tryC$_j$())} are the possible conflicting \mth{s} in SF-SVOSTM. On conflict between two transaction $T_i$ and $T_j$ where $TS(T_i) < TS(T_j)$, the conflict edge going from $T_i$ to $T_j$. In SF-SVOSTM, if higher timestamp (TS) transaction $T_j$ has already been committed then lower TS transaction $T_i$ returns abort and retry with higher TS in the incarnation of $T_i$ and returns commit. So, conflicts edges in SF-SVOSTM follows increasing of their TS. Formally, $TS(T_i) < TS(T_j)$ $\implies$ $T_i$ $\rightarrow$ $T_j$.
	
\end{itemize}
So, all the edges of $\copg{H}{\ll}$ generated by SF-SVOSTM algorithm follows the increasing order of  TS of the transactions. Thus, $\copg{H}{\ll}$ graph is acyclic. Hence, with the help of \thmref{coopqhprev}, any legal history $H$ generated by SF-SVOSTM satisfies co-opacity.  

\end{proof}


==> Arxiv SFKOSTM SSS19/ap-goplo.tex <==
\section{Graph Characterization of Local Opacity and SF-KOSTM Correctness}
\label{sec:gcoflo}


This section describes the graph characterization of local opacity for the history $H$ which maintains multiple versions corresponding to each key. Graph Characterization helps to prove the correctness of STMs for a given version order. Lets assume a history $H$ with given version order $\ll$. Following the  graph characterization by Chaudhary et al. \cite{Chaudhary+:KSFTM:Corr:2017} and modified it for sequential histories with high-level methods while maintaining multiple versions corresponding to each key and extend it for local opacity which helps to prove the correctness of SF-KOSTM. 


Similar to \secref{gcofo}, SF-KOSTM executes a concurrent history $H$ which consists of multiple transactions. Each transaction calls high-level methods which internally invokes multiple read-write (or lower-level) operations including method invocation and response known as \emph{events} (or $evts$) as discussed in \secref{sm}. So, we need to ensure the atomicity on both the levels. First, we ensure method level atomicity using the \emph{linearization point (LP)} of respective method. After that we ensure the atomicity of transaction on the basis of graph characterization of local-opacity. 

High-level methods are interval instead of dots (atomic). In order to make it atomic, we order the high-level method on the basis of their \emph{linearization point (LP)}. We consider \emph{first unlocking point} of each successful method as the \emph{LP} of the respective method.
Now, we need to ensure the atomicity at transactional level, a transaction internally invokes multiple high-level methods and transactions are overlapping to each other in concurrent history $H$. So, with the help of \emph{graph characterization} of \emph{local-opacity}, SF-KOSTM ensures the atomicity of the transaction defined below.


We construct a opacity graph represented as $\lopg{H}{\ll} = (V, E)$ which consists of $V$ vertices and $E$ edges. Here, each committed transaction $T_i$ is consider as a vertex and edges are as follows:
\begin{itemize}
	\item \textit{real-time (or \rt) edge}: This is same as \rt{} edge defined in $\copg{H}{\ll_H}$. If transaction $T_i$ returns commit before the beginning of other transaction $T_j$ then real-time edge goes from $T_i$ to $T_j$. Formally, ($\tryc_i() \prec_{H}$ \emph{STM\_begin$_j$}()) $\implies$  $T_i$ $\rightarrow$ $T_j$.
	\item \textit{return value from (or \rvf) edge}: There exist a \emph{\rvf} edge between two transaction $T_i$ and $T_j$ such that (1) If $T_i$ is the latest transaction that has updated ($\upmt{()}$) the key $k$ of \tab{}, $ht$ and committed; (2) After that $T_j$ invokes a \rvmt{} $rvm_{j}$ on the same key $k$ of \tab{} $ht$ and returns the value updated by $T_i$, i.e., $\upmt{_i()} \prec_{H}^{\mr} \rvm_{j}$. As defined in \secref{sm}, \upmt{()} can either be \emph{STM\_insert()} or \emph{STM\_delete()}. If the $\upmt{_i()}$ is \emph{STM\_insert()} method on key $k$ then \rvmt{()} returns the value updated by $T_i$, i.e.,  $i_i(k, v) <_H c_i <_H \rvm_j(k, v)$. If the $\upmt{_i()}$ is \emph{STM\_delete()} method on key $k$ then \rvmt returns $null$, i.e.,  $d_i(k, null) <_H c_i <_H \rvm_j(k, null)$.
	\item \textit{multi-version (or \mv) edge}: It depends on the version order between two transactions $T_i$ and $T_j$. For the sake of understanding, consider a triplet of three transactions $T_i$, $T_j$ and $T_k$ with successful methods on key $k$ as  $\up_i(k,u)$, $\rvm_j(k,u)$, $\up_k(k,v)$ , where $u \neq v$ and $up_i$ stands for \upmt{$_i$()} of $T_i$. It can observe that a \emph{return value from edge} is going from $T_i$ to $T_j$ because of $\rvm_j(k,u)$. If the version order is $k_i \ll k_k$ then the multi-version edge is going from $T_j$ to $T_k$. Otherwise, multi-version edge is from $T_k$ to $T_i$ because of version order ($k_k \ll k_i$). 
\end{itemize}
\cmnt{
%We define the graph characterization based on a given version order. Consider a history $H$ and a version order $\ll$. We then define a graph (called opacity graph) on $H$ using $\ll$, denoted as $\opg{H}{\ll} = (V, E)$. The vertex set $V$ consists of a vertex for each transaction $T_i$ in $\overline{H}$. The edges of the graph are of three kinds and are defined as follows:
\begin{enumerate}
	\setlength\itemsep{0em}
	\item \textit{\rt}(real-time) edges: If commit of $T_i$ happens before beginning of  $T_j$ in $H$, then there exist a real-time edge from $v_i$ to $v_j$. We denote set of such edges as $\rt(H)$.
	%\vspace{-.2cm}
	\item \textit{\rvf}(return value-from) edges: If $T_j$ invokes \rvmt on key $k_1$ from $T_i$ which has already been committed in $H$, then there exist a return value-from edge from $v_i$ to $v_j$. If $T_i$ is having \upmt{} as insert on the same key $k_1$ then $ins_i(k_{1, i}, v_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, v_{i1})$. If $T_i$ is having \upmt{} as delete on the same key $k_1$ then $del_i(k_{1, i}, null) <_H c_i <_H \rvm_j(k_{1, i}, null)$. We denote set of such edges as $\rvf(H)$.
	%\vspace{-.2cm}
	\item \textit{\mv}(multi-version) edges: This is based on version order. Consider a triplet with successful methods as  $\up_i(k_{1, i},u)$, $\rvm_j(k_{1, i},u)$, $\up_k(k_{1, k},v)$ , where $u \neq v$. As we can observe it from $\rvm_j(k_{1,i},u)$, $c_i <_H\rvm_j(k_{1,i},u)$. if $k_{1,i} \ll k_{1,k}$ then there exist a multi-version edge from $v_j$ to $v_k$. Otherwise ($k_{1,k} \ll k_{1,i}$), there exist a multi-version edge from $v_k$ to $v_i$. We denote set of such edges as $\mv(H, \ll)$.
\end{enumerate}
}
\cmnt{
	\begin{enumerate}
		
		\item \textit{\rt}(real-time) edges: If commit of $T_i$ happens before beginning of  $T_j$ in $H$, then there exist a real-time edge from $v_i$ to $v_j$. We denote set of such edges as $\rt(H)$.
		
		\item \textit{\rvf}(return value-from) edges: If $T_j$ invokes \rvmt on key $k_1$ from $T_i$ which has already been committed in $H$, then there exist a return value-from edge from $v_i$ to $v_j$. If $T_i$ is having \upmt{} as insert on the same key $k_1$ then $i_i(k_{1, i}, v_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, v_{i1})$. If $T_i$ is having \upmt{} as delete on the same key $k_1$ then $d_i(k_{1, i}, nil_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, nil_{i1})$. We denote set of such edges as $\rvf(H)$.
		
		\item \textit{\mv}(multi-version) edges: This is based on version order. Consider a triplet with successful methods as  $\up_i(k_{1,i},u)$ $\rvm_j(k_1,u)$ $\up_k(k_{1,k},v)$ , where $u \neq v$. As we can observe it from $\rvm_j(k_1,u)$, $c_i <_H\rvm_j(k_1,u)$. if $k_{1,i} \ll k_{1,k}$ then there exist a multi-version edge from $v_j$ to $v_k$. Otherwise ($k_{1,k} \ll k_{1,i}$), there exist a multi-version edge from $v_k$ to $v_i$. We denote set of such edges as $\mv(H, \ll)$.
		\vspace{-.3cm}
	\end{enumerate}
}


\noindent
For better understanding, we consider a history $H$: $l_1(ht, k_5, nil), l_2(ht, k_7, nil),\\ d_1(ht, k_6, nil), C_1, i_2(ht, k_5, v_2), C_2, l_3(ht, k_5, v_2), i_3(ht, k_7, v_3), C_3$ and show the time line view of it in \figref{glo}.(a). We construct $\lopg{H}{\ll} = (V, E)$ shown in \figref{glo}.(b). There exist a \mv{} edge between $T_1$ and $T_2$ because $T_1$ lookups the value of key $k_5$ from $T_0$ and after that $T_2$ creates a version on $k_5$ with value $v_2$. $T_3$ begins after the commit of $T_1$ and $T_2$ so, \rt{} edges are going from $T_1$ to $T_3$ and $T_2$ to $T_3$. Here, $T_3$ lookups key $k_5$ from the version created by $T_2$ and returns the value $v_2$. So, \rvf{} edge  is going from $T_2$ to $T_3$. Hence, $H$ constructs an acyclic graph (OG) with equivalent serial schedule $T_1 T_2 T_3$.

%For better understanding, consider a \figref{glo} with history $H$:
%\noindent We now show that if a version order $\ll$ exists for a history $H$ such that it is acyclic, then $H$ is \opq. 

%Using this construction, the $\opg{H3}{\ll_{H3}}$ for history $H3$ and $\ll_{H3}$ is given above is shown in \figref{mvostm1}. The edges are annotated. The only \mv{} edge from $T4$ to $T3$ is because of \tobj{s} $k_y, k_z$. $T4$ lookups value $v_{12}$ for $k_z$ from $T1$ whereas $T3$ also inserts $v_{32}$ to $k_z$ and commits before $lu_4(ht, k_{z,1}, v_{12})$. 

\cmnt{\begin{figure}[H]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.7}{\input{figs/mvostm2.pdf_t}}}
	\caption{$\opg{H3}{\ll_{H3}}$}
	\label{fig:mvostm1}
\end{figure}}

\begin{figure}
	\centerline{
		\scalebox{0.4}{\input{figs/lo.pdf_t}}}
	\captionsetup{justification=centering}
	\caption{Illustration of Graph Characterization of Opacity}
	\label{fig:glo}
\end{figure}


For a given history $H$ and version order $\ll$, we consider a complete graph $\overline{H}$ instead of $H$ and construct the graph $\lopg{\overline{H}}{\ll}$. It can be seen that $\overline{H}$ has more $\rt{}$ edges than $H$, i.e., $\prec_H^{RT} \subseteq \prec_{\overline{H}}^{RT}$. But, for the graph construction, we consider only $\rt{}$ edges of $H$ with the assumption $\rt(H) = \rt(\overline{H})$ that satisfies the following property:
%Given a history $H$ and a version order $\ll$, consider the graph $\opg{\overline{H}}{\ll}$. While considering the $\rt{}$ edges in this graph, we only consider the real-time relation of $H$ and not $\overline{H}$. It can be seen that $\prec_H^{RT} \subseteq \prec_{\overline{H}}^{RT}$ but with this assumption, $\rt(H) = \rt(\overline{H})$. Hence,  we get the following property, 

\begin{property}
	\label{prop:hoverh}
	For a given history $H$ and version order $\ll$, the opacity graphs $\lopg{H}{\ll}$ and $\lopg{\overline{H}}{\ll}$ are same.
\end{property}
%~
\begin{definition}
	\label{def:seqver}
	We define a version order $\ll_S$ for \tseq{} history $S$ such that if two committed transactions $T_i$ and $T_j$ has created versions on key $k$ as $k_i$ and $k_j$ respectively with version order $k_i \ll_S k_j$ then $T_i$ committed before $T_j$ in $S$. Formally, $\langle k_i \ll_S k_j \Leftrightarrow T_i <_S T_j \rangle $.
	
	
%	For a \tseq{} history $S$, we define a version order $\ll_S$ as follows: For two version $k_{x,i}, k_{x,j}$ created by committed transactions $T_i, T_j$ in $S$, $\langle k_{x,i} \ll_S k_{x,j} \Leftrightarrow T_i <_S T_j \rangle $. 
\end{definition}
%~
%Now, consider the following lemmas,
\noindent
This definition along with below defined lemmas and theorems will help us to prove the correctness of our graph characterization.  

\begin{lemma}
	\label{lem:seracycle1}
	The opacity graph for \legal{} \tseq{} history $S$ as $\lopg{S, \ll_S}$ is acyclic.
	%Consider a \legal{} \tseq{} history $S$. Then the graph $\opg{S, \ll_S}$ is acyclic.
\end{lemma}

\begin{proof}
	The proof of this lemma is similar as \lemref{concycle} of \secref{gcofo}. We order all the transactions of $S$ into real-time order on the basis of their increasing order of timestamp (TS). For example, consider two transaction $T_i$ and $T_j$ with $TS(T_i)$ is less than $TS(T_j)$ then $T_i$ will occur before $T_j$ in $S$. Formally, $TS(T_i) < TS(T_j)$ $\Leftrightarrow T_i <_S T_j$. We consider all the types edges of $\lopg{S, \ll_S}$ and analyze it one by one as follows to show the acyclicity of it:
	%We numerically order all the transactions in $S$ by their real-time order by using a function \textit{\ordfn}. For two transactions $T_i, T_j$, we define $\ord{T_i} < \ord{T_j} \Leftrightarrow T_i <_S T_j$. Let us analyze the edges of $\opg{S, \ll_S}$ one by one: 
	\begin{itemize}
		\item \rt{} edge: It follow that any transaction begin after commit of previous transaction only. Hence, all the \rt{} edges go from a lower TS transaction $T_i$ to higher TS transaction $T_j$ and follow timestamp order. 
		
		\item \rvf{} edge: Any transaction $T_j$ lookups key $k$ from $T_i$ in $S$ then $T_i$ has to be committed before invoking of lookup of $T_j$. So, $TS{(T_i)} < TS{(T_j)}$. Hence, all the \rvf{} edges goes from a lower TS transaction to a higher TS transaction.
		
		\item \mv{} edge: Consider a triplet of three transactions $T_i$, $T_j$ and $T_k$ with successful methods on key $k$ as  $\up_i(k,u)$, $\rvm_j(k,u)$, $\up_k(k,v)$ , where $u \neq v$. Here, $\rvm_j(k,u)$ method is returning the latest value written by $T_i$ on key $k$ with value $u$ using $\up_i(k,u)$. So, there exist a \rvf{} edge with $TS(T_i) < TS(T_j)$. There are two cases for the version order of $k$ as follows: (1) If the version order is $T_k \ll_S T_i$ which implies that $TS(T_k) < TS(T_i)$ then multi-version edge goes from $T_k$ to $T_i$ which also follows the increasing order of $TS$. (2) If the version order is $T_i \ll_S T_k$ which implies that $TS(T_i) < TS(T_k)$. Since $S$ is a \legal{} \tseq{} history, so, $TS(T_j) < TS(T_k)$ and then multi-version edge goes from $T_j$ to $T_k$ which again follows the increasing order of $TS$. So, \mv{} edges also follow the increasing order of $TS$ order.	
		
		
	%	Consider a successful \rvmt{} $\rvm_j(k_x, u)$ and a committed transaction $T_k$ writing $v$ to $k_x$ where $u \neq v$. Let $c_i$ be $\rvm_j(k_x, u)$'s \lastw. Thus, $\up_i(k_{x,i}, u) \in \evts{T_i}$. Thus, we have that $\ord{T_i} < \ord{T_j}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_k} < \ord{T_i}$. We now have that $T_k \ll T_i$. In this case, the mv edge is from $T_k$ to $T_i$. (2) Suppose $\ord{T_i} < \ord{T_k}$ which implies that $T_i \ll T_k$. Since $S$ is legal, we get that $\ord{T_j} < \ord{T_k}$. This case also implies that there is an edge from $\ord{T_j}$ to $\ord{T_k}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 
		
		%\item \mv{} edges: Consider a successful \rvmt{} $\rvm_k(k_x, v)$ and a committed transaction $T_i$ writing $u$ to $k_x$ where $u \neq v$. Let $c_j$ be $\rvm_k(k_x, v)$'s \lastw. Thus, $\up_j(k_{x,j}, v) \in \evts{T_j}$. Thus, we have that $\ord{T_j} < \ord{T_k}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_i} < \ord{T_j}$. We now have that $T_i \ll T_j$. In this case, the mv edge is from $T_i$ to $T_j$. (2) Suppose $\ord{T_j} < \ord{T_i}$ which implies that $T_j \ll T_i$. Since $S$ is legal, we get that $\ord{T_k} < \ord{T_i}$. This case also implies that there is an edge from $\ord{T_k}$ to $\ord{T_i}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 
	\end{itemize}
	
	Therefore, all the types of edges follow the increasing order of transaction's $TS$ as defined above. All the edges of $S$ goes from lower $TS$ transaction to higher $TS$ transactions. This implies that the opacity graph generated by \legal{} \tseq{} history $S$ as $\lopg{S, \ll_S}$ is acyclic. 
\end{proof}

\begin{lemma}
	\label{lem:eqv_hist_mvorder}
	Consider a history $H$ with given version order $\ll_H$. Another history $H'$ is equivalent to $H$ then the mv edges $\mv(H, \ll_H)$ induced by $\ll_H$ in $H$ and $H'$ will be same.	
%	Consider two histories $H, H'$ that are equivalent to each other. Consider a version order $\ll_H$ on the \tobj{s} created by $H$. The mv edges $\mv(H, \ll_H)$ induced by $\ll_H$ are the same in $H$ and $H'$.
\end{lemma}

\begin{proof}
	Since history $H$ and $H'$ are equivalent, so, version order of  $\ll_H$ will be same as version order of  $\ll_{H'}$. We can observe that \mv{} edges depend on version order $\ll$ and the methods of the history. It is independent from the order of the methods in $H$. So, being equivalence $H'$ also contains the same version order $\ll_H$ and the methods as in $H$. Thus, multi-version \mv{} edges are same in $H$ and $H'$. 
	%Since the histories are equivalent to each other, the version order $\ll_H$ is applicable to both of them. It can be seen that the \mv{} edges depend only on events of the history and version order $\ll$. It does not depend on the ordering of the events in $H$. Hence, the \mv{} edges of $H$ and $H'$ are equivalent to each other. 
\end{proof}

%\noindent Using these lemmas, we prove the following theorem. 


\begin{theorem}
	\label{thm:opg}
	A \valid{} history $H$ is opaque with a version order $\ll_H$ iff $\lopg{H}{\ll_H}$ is acyclic.
\end{theorem}

\begin{proof}
	\textbf{(if part):} First, we consider $\lopg{H}{\ll_H}$ is acyclic and we need to prove that history $H$ is opaque. Since $\lopg{H}{\ll_H}$ is acyclic, we apply topological sort on $\lopg{H}{\ll_H}$ and generate a \tseq{} history $S$ such that $S$ is equivalent to $\overline{H}$.
	$\lopg{H}{\ll_H}$ maintains real-time edges as well and $S$ has been generated from it. So, $S$ also respect real-time order (or \rt{}) as $H$. Formally, $\prec_H^{RT} \subseteq \prec_S^{RT}$.
	
	$\lopg{H}{\ll_H}$ maintains the return value from (or \rvf{}) edges for \rvmt{()} on any key $k$ by transaction $T_i$ returns the value written on $k$ by previously committed transaction $T_j$. So, $S$ is \emph{valid}. Now, we need to prove that $S$ is \emph{legal}. We prove it by contradiction, so we assume that $S$ is not \emph{legal}. That means, a \rvmt{()} $\rvm_j(k, u)$ lookups on key $k$ from a committed transaction $T_i$ which wrote the value of $k$ as $u$. But between these two transaction $T_i$ and $T_j$, an another committed transaction $T_k$ exist in $S$ which wrote to $k$ with value $v$ and ($u \neq v$). Formally, $T_i \prec_{S}^{RT} T_k \prec_{S}^{RT} T_j$. Consider a given version order in $H$ as $\ll_H$, if the version order is $T_k \ll_S T_i$ then the multi-version edge goes from $T_k$ to $T_i$. Consider the other version order is $T_i \ll_S T_k$ then the multi-version edge goes from $T_j$ to $T_k$. So, in both the cases $T_k$ is not coming between $T_i$ and $T_j$. So, our assumption is wrong. Hence,  $S$ is \emph{legal}. 
	

%Thus, there is a successful \rvmt{} $\rvm_j(k_x, u)$ such that its \lastw{} in $S$ is $c_k$ and $T_k$ updates value $v (\neq u)$ to $k_x$, i.e $\up_k(k_{x,k}, v) \in \evts{T_k}$. Further, we also have that there is a transaction $T_i$ that insert $u$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Since $S$ is \valid, as shown above, we have that $T_i \prec_{S}^{RT} T_k \prec_{S}^{RT} T_j$.

%Now in $\ll_H$, if $k_{x,k} \ll_H k_{x,i}$ then there is an edge from $T_k$ to $T_i$ in $G_H$. Otherwise ($k_{x,i} \ll_H k_{x,k}$), there is an edge from $T_j$ to $T_k$. Thus in either case $T_k$ can not be in between $T_i$ and $T_j$ in $S$ contradicting our assumption. This shows that $S$ is legal. 


%H$ maintains all the (\rvf{}) methods in conflicting \confc{} edges of $\lopg{H}{\ll_H}$. Since $S$ has been generated by applying topological sort on $\lopg{H}{\ll_H}$. So, $S$ returns all the return value methods from previous closest committed transactions. Hence, $S$ is $legal$.
	
	$S$ satisfies all the properties of \emph{opacity} and equivalent to $H$ because $S$ has been generated from the topological sort on $\lopg{H}{\ll_H}$. Hence, history H is opaque.
	
	
	\textbf{(Only if part):} Now, we consider $H$ is opaque and have to prove that $\lopg{H}{\ll_H}$ is acyclic.
	Since $H$ is opaque there exists an equivalent  \legal{} \tseq{} history $S$ to $\overline{H}$ which maintains real-time (\rt{}) and conflict ($Conf$) order of $H$. From the \lemref{seracycle1}, we can say that opacity graph $\lopg{S, \ll_S}$ is acyclic. As we know, $\lopg{H}{\ll_H}$ is the subgraph of $\lopg{S, \ll_S}$.
	Hence, $\lopg{H}{\ll_H}$ is acyclic.
	
\end{proof}
	
	%Here we have a version order $\ll_H$ such that $G_H=\opg{H}{\ll}$ is acyclic. Now we have to show that $H$ is opaque. Since the $G_H$ is acyclic, a topological sort can be obtained on all the vertices of $G_H$. Using the topological sort, we can generate a \tseq{} history $S$. It can be seen that $S$ is equivalent to $\overline{H}$. Since $S$ is obtained by a topological sort on $G_H$ which maintains the real-time edges of $H$, it can be seen that $S$ respects the \rt{} order of $H$, i.e $\prec_H^{RT} \subseteq \prec_S^{RT}$. 
	
	%Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_j(k_x, u)$ such that its \lastw{} in $S$ is $c_k$ and $T_k$ updates value $v (\neq u)$ to $k_x$, i.e $\up_k(k_{x,k}, v) \in \evts{T_k}$. Further, we also have that there is a transaction $T_i$ that insert $u$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Since $S$ is \valid, as shown above, we have that $T_i \prec_{S}^{RT} T_k \prec_{S}^{RT} T_j$.
	
%	Now in $\ll_H$, if $k_{x,k} \ll_H k_{x,i}$ then there is an edge from $T_k$ to $T_i$ in $G_H$. Otherwise ($k_{x,i} \ll_H k_{x,k}$), there is an edge from $T_j$ to $T_k$. Thus in either case $T_k$ can not be in between $T_i$ and $T_j$ in $S$ contradicting our assumption. This shows that $S$ is legal. 
	
	
	%Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_k(k_x, v)$ such that its \lastw{} in $S$ is $c_i$ and $T_i$ updates value $u (\neq v)$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Further, we also have that there is a transaction $T_j$ that insert $v$ to $k_x$, i.e $\up_j(k_{x,j}, v) \in \evts{T_j}$. Since $S$ is \valid, as shown above, we have that $T_j \prec_{S}^{RT} T_i \prec_{S}^{RT} T_k$.
	
	%Now in $\ll_H$, if $k_{x,i} \ll_H k_{x,j}$ then there is an edge from $T_i$ to $T_j$ in $G_H$. Otherwise ($k_{x,j} \ll_H k_{x,i}$), there is an edge from $T_k$ to $T_i$. Thus in either case $T_i$ can not be in between $T_j$ and $T_k$ in $S$ contradicting our assumption. This shows that $S$ is legal. 
	
%	\textbf{(Only if part):} Here we are given that $H$ is opaque and we have to show that there exists a version order $\ll$ such that $G_H=\opg{H}{\ll} (=\opg{\overline{H}}{\ll}$, \propref{hoverh}) is acyclic. Since $H$ is opaque there exists a \legal{} \tseq{} history $S$ equivalent to $\overline{H}$ such that it respects real-time order of $H$. Now, we define a version order for $S$, $\ll_S$ as in \defref{seqver}. Since the $S$ is equivalent to $\overline{H}$, $\ll_S$ is applicable to $\overline{H}$ as well. From \lemref{seracycle1}, we get that $G_S=\lopg{S}{\ll_S}$ is acyclic. Now consider $G_H = \lopg{\overline{H}}{\ll_S}$. The vertices of $G_H$ are the same as $G_S$. Coming to the edges, 
	







\noindent The above defined lemmas and theorems of \emph{opacity} can be extended the proof of \emph{local-opacity}.
\begin{theorem}
	\label{thm:log}
	A \valid{} history $H$ is \lopq iff all the sub-histories $\shset{H}$ (defined in \secref{sm}) for a history $H$ are opaque, i.e., A \valid{} history $H$ is \lopq iff the opacity graph $\lopg{sh}{\ll_{sh}}$ generated for each sub-history $sh$ of $\shset{H}$ with given version order $\ll_{sh}$ is acyclic. Formally,$\langle (H \text{ is \lopq}) \Leftrightarrow (\forall sh \in \shset{H}, \exists \ll_{sh}: \lopg{sh}{\ll_{sh}} \text{ is acyclic}) \rangle$.
	
	
	%A \valid{} history $H$ is \lopq iff for each sub-history $sh$ in $\shset{H}$ there exists a version order $\ll_{sh}$ such that $\opg{sh}{\ll_{sh}}$ is acyclic. Formally,\\ $\langle (H \text{ is \lopq}) \Leftrightarrow (\forall sh \in \shset{H}, \exists \ll_{sh}: \opg{sh}{\ll_{sh}} \text{ is acyclic}) \rangle$. 
\end{theorem}

\begin{proof}
	
	In order to prove it, we need to show that each sub-history $sh$ from the sub-histories of $H$, $\shset{H}$ is \emph{valid}. After that the remaining proof follows \thmref{opg}.
	
	To prove sub-history $sh$ is \emph{valid}, consider a $sh$ with any \rvmt{()} $\rvm_j(k,u)$ of a transaction $T_j$. We can easily observe that \rvm method returns the value of key $k$ that has been written by a committed transaction $T_i$ on $k$ with value $u$. So, it can be seen that $sh$ has all the transactions that has committed before $\rvm_j(k,u)$. Similarly, all the \rvm methods of $sh$ return the value from previously committed transactions. Thus, sub-history $sh$ is \emph{valid}.
	
	Now, we need to show each sub-history $sh$ is opaque with a version order $\ll_{sh}$ iff $\lopg{sh}{\ll_{sh}}$ is acyclic. The proof of this is directly coming \thmref{opg} while replacing $H$ with $sh$.
	Similarly, all the sub-histories of $\shset{H}$ are \emph{valid} and satisfying  \thmref{opg}. So, all the sub-histories of history $H$ are \emph{opaque}. Hence, a \valid{} history $H$ is \lopq.
	
		%To prove this theorem, we have to show that each sub-history $sh$ in $\shset{H}$ is \valid. Then the rest follows from . Now consider a sub-history $sh$. Consider any read \op $r_i(x, v)$ of a transaction $T_i$. It is clear that $T_i$ must have read a version of $x$ created by a previously committed transaction. From the construction of $sh$, we get that all the transaction that committed before $r_i$ are also in $sh$. Hence $sh$ is also \valid. 
	
	%Now, proving $sh$ to be \opq iff there exists a version order $\ll_{sh}$ such that $\opg{sh}{\ll_{sh}}$ is acyclic follows from \thmref{opg}. 
\end{proof}

\noindent
Now, we consider the algorithms defined for each method of \emph{SF-KOSTM} in \secref{pm} and prove the correctness of SF-KOSTM. Consider a history $H$ generated by SF-KOSTM with two transaction $T_i$ and $T_j$ with status either \emph{live or committed} using $status$ flags as true. Then the edges between $T_i$ and $T_j$ follow the $\tltl$ order. SF-KOSTM algorithm ensures that $\tltl$ are keep on increasing order of the transaction timestamp (TS) order using atomic counter $\gtcnt$ in \emph{STM\_begin()}. Though the value of $\tltl$ is increasing in the other methods of SF-KOSTM still its maintaining the increasing order of transactions TS. We assume all the histories generate (or gen) by SF-KOSTM algorithm as $\gen{\emph{SF-KOSTM}}.$

\begin{lemma}
	\label{lem:tltl-edge}
	Any history $H$ generated by SF-KOSTM as $\gen{\emph{SF-KOSTM}}$ with two transactions $T_i$ and 
	$T_j$ such that status flags of both the transactions are true.  If there is an edge from $T_i$ to $T_j$ then $\tltl_i$ is less than $\tltl_j$. Formally, $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$.		
\end{lemma}

\begin{proof}
	We consider all types of edges in $\lopg{H}{\ll_H}$ and analyze it as follows:
	
	\begin{itemize}
		\item \textit{real-time (or \rt) edge}: Here, the transaction $T_i$ returns commit before the begin of other transaction $T_j$ then real-time edge goes from $T_i$ to $T_j$. Hence, $\tltl_i$ gets the value from $\gtcnt$ earlier than begin of $T_j$. So, $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$.
		
		\item \textit{return value from (or \rvf) edge}: The transaction $T_i$ has updated ($\upmt{()}$) the key $k$ of \tab{}, $ht$ and committed. After that transaction $T_j$ invokes a $rvm_{j}$ on the same key $k$ and returns the value updated by $T_i$. SF-KOSTM ensures that $T_j$ returns the value of $k$ from the transaction which has lesser TS than $T_j$ i.e., $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$. %$\upmt{_i} \prec_{H}^{\mr} \rvm_{j}$. As defined in \secref{sm}, \upmt{} can either be $insert$ or $delete$. If the $\upmt{_i}$ is $insert$ method on key $k$ then \rvmt returns the value updated by $T_i$, i.e.,  $ins_i(k, v) <_H c_i <_H \rvm_j(k, v)$. If the $\upmt{_i}$ is $delete$ method on key $k$ then \rvmt returns $null$, i.e.,  $del_i(k, null) <_H c_i <_H \rvm_j(k, null)$.
		\item \textit{multi-version (or \mv) edge}: SF-KOSTM ensures that version order between two transactions $T_i$ and $T_j$ are also following TS order using their $\tltl$. Consider a triplet generated by SF-KOSTM with three transactions $T_i$, $T_j$ and $T_k$ with successful methods on key $k$ as  $\up_i(k,u)$, $\rvm_j(k,u)$, $\up_k(k,v)$ , where $u \neq v$. It can observe that a return value from edge is going from $T_i$ to $T_j$ because of $\rvm_j(k,u)$, so,  $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$. If the version order is $k_i \ll k_k$ then the multi-version edge is going from $T_j$ to $T_k$. Hence, the order among the transactions are  ($T_i$ $\rightarrow$ $T_j$ $\rightarrow$ $T_k$) $\implies$ ($\tltl_i$ $<$ $\tltl_j$ $<$ $\tltl_k$). Otherwise, multi-version edge is from $T_k$ to $T_i$ because of version order ($k_k \ll k_i$). Then the relation is ($T_k$ $\rightarrow$ $T_i$ $\rightarrow$ $T_j$) $\implies$ ($\tltl_k$ $<$ $\tltl_i$ $<$ $\tltl_j$). 
	\end{itemize}
	So, all the edges of $\lopg{H}{\ll_H}$  are following increasing order of transactions $\tltl$. Hence, $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$.
		
\end{proof}

\begin{theorem}
	\label{thm:coopqh}
	A valid SF-KOSTM history $H$ is locally-opaque iff $\lopg{H}{\ll_H}$ is acyclic.
\end{theorem}
\begin{proof}
	\textbf{(if part):} First, we consider $H$ is \emph{valid} and $\lopg{H}{\ll_H}$ generated by SF-KOSTM is acyclic then we need to prove that history $H$ is locally-opaque. Since $\lopg{H}{\ll_H}$ is acyclic, we apply topological sort on $\lopg{H}{\ll_H}$ and obtained a \tseq{} history $S$ which is equivalent to $\overline{H}$.
	%Since $\copg{H}{\ll_H}$ maintains real-time as well as conflict edges and $S$ has been generated from it. So, 
	$S$ also respect real-time (or $RT$), return value from (or $RVF$) and multi-version (or $MV$)  edges as $\overline{H}$. Formally, $S$ respects $\prec$$^{RT}_S$ = $\prec$$^{RT}_{\overline{H}}$, $\prec$$^{RVF}_S$ = $\prec$$^{RVF}_{\overline{H}}$ and $\prec$$^{MV}_S$ = $\prec$$^{MV}_{\overline{H}}$. %Formally, $\prec_H^{RT} \subseteq \prec_S^{RT}$.
	
	Since \rvf{} and \rt{} relation between the methods of SF-KOSTM for a given version in $S$ are also present in $\overline{H}$. Formally, $\prec_{\overline{H}}^{RT} \subseteq \prec_S^{RT}$ and $\prec_{\overline{H}}^{RVF} \subseteq \prec_S^{RVF}$. Given that $H$ is \emph{valid} which implies that  $\overline{H}$ is also \emph{valid}. So, we can say that $S$ is \emph{legal} for a given version order. Similarly, we can prove that all the sub-histories $\shset{H}$ for a history $H$ are opaque. Hence with the help of \thmref{log}, collectively, $H$ satisfies all the necessary conditions of \emph{local-opacity}. Hence, history $H$ is locally-opaque.
	
	\textbf{(Only if part):} Now, we consider $H$ is locally-opaque and valid then we have to prove that $\lopg{H}{\ll_H}$ is acyclic. We prove it through contradiction, so we assume there exist a cycle in $\lopg{H}{\ll_H}$. From \lemref{tltl-edge}, any two transactions $T_i$ and 
	$T_j$ generated by SF-KOSTM such that both their status flags are true and $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$. Consider the transitive case with $k$ transactions
 $T_1, T_2, T_3...T_k$ such	that status flags of all the $k$ transactions are true. If edges exist like ($T_1$ $\rightarrow$ $T_2$ $\rightarrow$ $T_3$ 
	$\rightarrow$....$\rightarrow$ $T_k$) $\implies$ ($\tltl_1 $ $<$ $\tltl_2$ $<$ 
	$\tltl_3$ $<$ ....$<$ $\tltl_k$).\\
	Now, we consider our assumption, there exist a cycle in $\lopg{H}{\ll_H}$. So, $T_1$ 
	$\rightarrow$ $T_2$ $\rightarrow$ $T_3$ $\rightarrow$....$\rightarrow$ 
	$T_k$ $\rightarrow$ $T_1$ that implies $\tltl_1 $ $<$ $\tltl_2$ $<$ 
	$\tltl_3$ $<$ ....$<$ $\tltl_k$ $<$ $\tltl_1$.\\
	Hence, above assumption says that, $\tltl_1$ $<$ $\tltl_1$ but this is not possible. So, our assumption there exist a cycle in $\lopg{H}{\ll_H}$ is wrong.\\
	Therefore, $\lopg{H}{\ll_H}$ produced by SF-KOSTM is acyclic.
\end{proof}


\begin{theorem}
	Any valid history $H$ generated by SF-KOSTM satisfies local-opacity.
\end{theorem}

\begin{proof}
	With the help of \lemref{tltl-edge}, we can say that any history $H$  $\gen{\emph{SF-KOSTM}}$ with two transactions $T_i$ and 
	$T_j$ such that status flags of both the transactions are true.  If there is an edge from $T_i$ to $T_j$ then $\tltl_i$ is less than $\tltl_j$. Formally, $T_i$ $\rightarrow$ $T_j$ $\implies$ $\tltl_i$ $<$ $\tltl_j$. So, we can infer that any valid history $H$ generated by SF-KOSTM following the edges $T_i$ $\rightarrow$ $T_j$ in increasing order of $\tltl_i$ $<$ $\tltl_j$ with the help of atomic \gtcnt. Hence, we can conclude that SF-KOSTM always produce an acyclic $\lopg{H}{\ll_H}$ graph.
	
	Now, using \thmref{coopqh}, we can infer that if a valid history $H$ generated by SF-KOSTM always produces an acyclic $\lopg{H}{\ll_H}$  graph then $H$ is locally-opaque. Hence, any valid history $H$ generated by SF-KOSTM satisfies local-opacity.
	
\end{proof}


==> Arxiv SFKOSTM SSS19/ap-model.tex <==
\section{Remaining System Model}
\label{apn:ap-model}
In this section we define other useful notions and definitions used in main
paper such as sequential histories, real-time order and serial history, valid and
legal history, sub-histories, opacity, conflict-opacity, local opacity and 
strict-serializability as follows:

\noindent
\textbf{Sequential Histories:} Following \cite{KuznetsovPeri:Non-interference:TCS:2017, KuznetsovRavi:ConcurrencyTM:OPODIS:2011},  if all the methods of the history are complete and isolated from each other, i.e. all the methods of history are atomic and following the total order in $H$. So, with this assumption, the only relevant methods of a transaction $T_i$ are $l_i(k,v)$, 
$l_i(k,\abort)$, $i_i(k, v)$, $d_i(k, v)$, $\tryc_i(\commit)$ (or $c_i$ for short), 
$\tryc_i(\abort)$, and $\trya_i(\abort)$ (or $a_k$ for short). We form the complete history $\overline{H}$, by immediately inserting the abort to all the live transactions of $H$. But, if the first operation of \emph{STM\_tryC$_i$()} has returned successfully then $T_i$ returns commit.

\noindent
\textbf{Real-Time Order and Serial History:} Two complete method $m_{ij}$ and $m_{xy}$ are said to be in method real-time order (or MR), if the response of $m_{ij}$ happens before the invocation of $m_{xy}$. Formally, if ($rsp(m_{ij}) <_H inv(m_{xy})$)$\implies$($m_{ij} \prec_H^{\mr} m_{xy}$). Following \cite{Papad:1979:JACM}, if transaction $T_i$ terminates (either commits or aborts) before beginning of $T_j$ then $T_i$ and $T_j$  follows transaction real-time order (or TR). Formally, if ($Term(T_i) <_H \tbeg_j()$)$\implies$($T_i \prec_H^{\tr} T_j$).  If all the transactions of a history $H$ follow the real-time order, i.e. transactions are atomic then such history is known as \emph{serial} \cite{Papad:1979:JACM} or \emph{t-sequential} \cite{KuznetsovRavi:ConcurrencyTM:OPODIS:2011} history. % Since, transactions are atomic then implicitly methods will also be atomic so, any serial history will also be a sequential history.
Formally, $\langle (H \text{ is serial}) \implies (\forall T_{i} \in \txns{H}: (T_i \in Term{(H)}) \land (\forall T_{i}, T_{j} \in \txns{H}: (T_{i} \prec_H^{\tr} T_{j}) \lor (T_{j} \prec_H^{\tr} T_{i}))\rangle$. In the serial history all the methods within a transaction are also ordered, it is also sequential.
%\noindent
%\textbf{Valid and Legal History:} If all the \emph{rv} methods of $H$ returns the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}. Whereas, If all the \emph{rv} methods of $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.


%has been considered corresponding to each aborted transactions while keeping all the committed transaction including the aborted transaction till its successful method.

\noindent
\textbf{Valid and Legal History:}  If \emph{$rv\_method()$}  on key $k$ returns the value from any of the previously committed transactions then such \emph{$rv\_method()$} is known as \emph{valid method}. If all the \emph{$rv\_methods()$} of history $H$ return the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}.

 Whereas, If \emph{$rv\_method()$}  on key $k$ returns the value from previous closest committed transaction then such \emph{$rv\_method()$} is known as \emph{legal method}. If all the \emph{$rv\_methods()$} of history $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.
 
 \cmnt{
 %\section{Valid and Legal Histories}
 %\label{apn:legal}
 %\vspace{-2mm}
 %In this section, we start with defining legal histories. 
 To simplify our analysis, we assume that there exists an initial transaction $T_0$ that invokes $\tdel$ \mth on all the keys of the \tab{} used by any transaction. 
 
 A \rvmt{} (\tdel{} and \tlook{}) $m_{ij}$ on key $k$ is valid if it returns the value updated by any of the previous committed transaction that updated key $k$. A history $H$ is said to valid if all the \rvmt{s} of H are valid. 
 
 We define \emph{\legality{}} of \rvmt{s} on sequential histories which we use to define correctness criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}. Consider a sequential history $H$ having a \rvmt{} $\rvm_{ij}(ht, k, v)$ (with $v \neq null$) as $j^{th}$ method belonging to transaction $T_i$. We define this \rvm \mth{} to be \emph{\legal} if: 
 \vspace{-1mm}
 \begin{enumerate}
 	%\setlength\itemsep{-1em}
 	%\vspace{-.2cm}
 	\item[LR1] \label{step:leg-same} If the $\rvm_{ij}$ is not first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $m_{ix}$ is the previous \mth of $T_i$ on $\langle ht, k \rangle$. Formally, $\rvm_{ij} \neq \fkmth{\langle ht, k \rangle}{T_i}{H}$ $\land (m_{ix}\\(ht, k, v') = \pkmth{\langle ht, k \rangle}{T_i}{H})$ (where $v'$ could be null). Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		%		\item if $m_{ix}(ht, k, v')$ is a \tins{} \mth i.e. $\tins_{ix}(ht, k, v')$ then $v = v'$. 
 		%		\item if $m_{ix}(ht, k, v')$ is a \tlook{} \mth i.e. $\tlook_{ix}(ht, k, v')$ then $v = v'$. 
 		%		\item if $m_{ix}(ht, k, v')$ is a \tdel{} \mth i.e. $\tdel_{ix}(ht, k, v'/NULL)$ then $v = NULL$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tins{} \mth then $v = v'$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tlook{} \mth then $v = v'$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tdel{} \mth then $v = null$.
 	\end{enumerate}
 	
 	In this case, we denote $m_{ix}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $m_{ix}(ht, k, v') = \\\lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 	
 	\item[LR2] \label{step:leg-ins} If $\rvm_{ij}$ is the first \mth{} of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is not null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v \neq null)$. Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		\item There is a \tins{} \mth{} $\tins_{pq}(ht, k, v)$ in $\met{H}$ such that $T_p$ committed before $\rvm_{ij}$. Formally, $\langle \exists \tins_{pq}(ht, k, v) \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. 
 		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 	\end{enumerate}
 	
 	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $\tryc_{p}(ht, k, v)$= $\lupdt{\rvm_{ij}(ht, k, v)}{H}$.
 	
 	\item[LR3] \label{step:leg-del} If $\rvm_{ij}$ is the first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v = null)$. Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		\item There is \tdel{} \mth{} $\tdel_{pq}(ht, k, v')$ in $\met{H}$ such that $T_p$ (which could be $T_0$ as well) committed before $\rvm_{ij}$. Formally, $\langle \exists \tdel_{pq}\\(ht, k,$ $ v') \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. Here $v'$ could be null. 
 		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 	\end{enumerate}
 	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e., $\tryc_{p}(ht, k, v)$ $= \lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 \end{enumerate}
 %\vspace{-.3cm}
 We assume that when a transaction $T_i$ operates on key $k$ of a \tab{} $ht$, the result of this \mth is stored in \emph{local logs} of $T_i$, $\llog_i$ for later \mth{s} to reuse. Thus, only the first \rvmt{} operating on $\langle ht, k \rangle$ of $T_i$ accesses the shared-memory. The other \rvmt{s} of $T_i$ operating on $\langle ht, k \rangle$ do not access the shared-memory and they see the effect of the previous \mth{} from the \emph{local logs}, $\llog_i$. This idea is utilized in LR1. With reference to LR2 and LR3, it is possible that $T_x$ could have aborted before $\rvm_{ij}$. For LR3, since we are assuming that transaction $T_0$ has invoked a \tdel{} \mth{} on all the keys used of the \tab{} objects, there exists at least one \tdel{} \mth{} for every \rvmt on $k$ of $ht$. We formally prove legality in \apnref{cmvostm} and then we finally show that history generated by \hmvotm{} is \opq{} \cite{GuerKap:Opacity:PPoPP:2008}.
 
 %This we also call \emph{conflict inheritance} as the conflict of the later \mth{} of $T_i$ operating on $\langle ht, k \rangle$ can be found using the conflicts of the first \mth{} of $T_i$.
 
 Coming to \tins{} \mth{s}, since a \tins{} \mth{} always returns $ok$ as they overwrite the node if already present therefore they always take effect on the $ht$. Thus, we denote all \tins{} \mth{s} as \legal{} and only give legality definition for \rvmt{}. We denote a sequential history $H$ as \emph{\legal} or \emph{linearized} if all its \rvm \mth{s} are \legal.%A sequential history \emph{linearized} \cite{HerlWing:1990:TPLS}

}



\noindent
\textbf{Sub-history:} Following \cite{Chaudhary+:KSFTM:Corr:2017}, A \textit{sub-history} ($SH$) of a history ($H$) is a collection of events represented as $\evts{SH}$. We denote a $SH$ as the tuple $\langle \evts{SH},$ $<_{SH}\rangle$, here $<_{SH}$ represents the
total order of among all the events of $SH$. Formally, $SH$ is defined as: (1) $<_{SH} \subseteq <_{H}$; (2) $\evts{SH} \subseteq \evts{H}$; (3) If an event of a transaction $T_k\in\txns{H}$ is in $SH$ then all the events of $T_k$ in $H$ should also be in $SH$. 

Let $P$ is a subset of $H$ which consists of a set transactions $\txns{H}$. Then the sub-history of $H$ is represented as $\shist{P}{H}$ which comprises of $\evts{}$ of $P$. 

\noindent
\textbf{Conflict-opacity (or Co-opacity):} It is a well known correctness criteria of STMs that is polynomial time verifiable. Co-opacity \cite{Peri+:OSTM:Netys:2018} is a subclass of opacity. A history $H$ is co-opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time as $H$ $\prec_S^{\tr} \subseteq \prec_H^{\tr}$. (4) $S$ preserves conflict-order of $H$, i.e. $\prec_S^{Conf} \subseteq \prec_H^{Conf}$.

\noindent
\textbf{Opacity and Strict Serializability:} A popular correctness criteria for STMs is opacity \cite{GuerKap:Opacity:PPoPP:2008}. A valid history $H$ is opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time order as $H$, i.e. $\prec_S^{\tr} \subseteq \prec_H^{\tr}$.

 A valid history $H$ is strict serializable \cite{Papad:1979:JACM}, if sub-history  of $H$ as $\subhist(H)$ (consists of all the committed transactions of $H$) is opaque, i.e., $H.subhist(H.committed)$ is \emph{opaque}. So, if a history is \emph{strict serializable} then it will be \opq as well but  the vice-versa is not true. Unlike opacity, \emph{strict serializability} does not consider aborted transactions.

A commonly used correctness criteria in databases is \emph{serializability} \cite{Papad:1979:JACM} which considers committed transactions only. Guerraoui \& Kapalka \cite{GuerKap:Opacity:PPoPP:2008} show that STMs considers the correctness of \emph{aborted} transactions along with \emph{committed} transactions as well. So,  \emph{serializability} is not suitable for STMs. On the other hand, \emph{opacity} \cite{GuerKap:Opacity:PPoPP:2008} is a popular correctness criteria for STMs which considers \emph{aborted} as well as \emph{committed} transactions. Similar to \emph{opacity} but less restrictive, an another popular correctness criteria is \emph{local opacity} defined below.



\noindent
\textbf{Local Opacity (or LO):} It is an another popular correctness criteria for STMs which is less restrictive than opacity. Local-opacity \cite{KuznetsovPeri:Non-interference:TCS:2017} is a superclass of opacity. It considers a set of sub-histories for history $H$, denoted as $\shset{H}$ as follows: (1) We construct a $\subhist$ corresponding to each aborted transaction $T_i$ while including all the events $\evts{}$ of previously \emph{committed} transactions along with all successful $\evts{}$ of $T_i$ (i.e., $\evts{}$ which has not returned $\mathcal{A}$ yet) and put \emph{committed} $\mathcal{C}$ immediately after last successful operation of $T_i$; (2) We construct one more sub-history corresponding to last \emph{committed} transaction $T_l$ which considers all the previously \emph{committed} transactions only including  $T_l$.

If all the above defined sub-histories $\shset{H}$ for a history $H$ are opaque then $H$ is said to be \emph{\lopq} \cite{KuznetsovPeri:Non-interference:TCS:2017}. We can observe that a sub-history corresponding to an aborted transaction $T_i$ contains $\evts{}$ from only one aborted transaction which is $T_i$ itself and does not consider any other live/aborted transactions. Similarly, sub-history corresponding to last \emph{committed} transaction $T_l$ does not consider any $\evts{}$ of aborted and live transactions. Thus in \lopty, neither aborted nor live transaction cause any other transaction to abort. Researchers have been proved that \lopty 
\cite{KuznetsovPeri:Non-interference:TCS:2017} ensures greater concurrency than \opty \cite{GuerKap:Opacity:PPoPP:2008}. If a history is \opq then it will be \lopq as well but  the vice-versa is not true. On the other hand, if a history is \lopq then it will be \stsble as well, but the vice-versa need not be true. Please find  illustrations of local opacity in \apnref{gcoflo}.




\cmnt{
\todo{Copy conflict-notion from OSTM}



Opacity is a popular \cc{} for STMs. But, as observed in \secref{intro}, it can be proved that verifying the membership of \opty similar to view-serializability (VSR) in databases is NP-Complete \cite{Papad:1979:JACM}. To circumvent this issue, researchers in databases have identified an efficient sub-class of VSR, called conflict-serializability or \csr, based on the notion of conflicts. The membership of \csr can be verified in polynomial time using conflict graph characterization. Along the same lines, we develop the notion of conflicts for \otm and identify a sub-class of \opty, \coopty. The proposed \cc{} is extension of the notion of conflict-opacity developed for \emph{\rwtm} by Kuznetsov \& Peri \cite{KuzPer:NI:TCS:2017}.

We say two transactions $T_i, T_j$ of a sequential history $H$ for \otm{} are in \emph{conflict} if atleast one of the following conflicts holds:
\vspace{-.2cm}
\begin{itemize}
	\setlength\itemsep{0em}
	\item \textbf{tryC-tryC} conflict:(1) $T_i$ \& $T_j$ are committed and (2) $T_i$ \& $T_j$ update the same key $k$ of the \tab{}, $ht$, i.e., $(\langle ht,k \rangle \in \udset{T_i}) \land (\langle ht,k \rangle \in \udset{T_j})$, where $\udset{T_i}$ is update set of $T_i$. (3) $T_i$'s \tryc{} completed before $T_j$'s \tryc, i.e., $\tryc_i \prec_{H}^{\mr} \tryc_j$. 
	
	\item \textbf{tryC-rv} conflict:(1) $T_i$ is committed (2) $T_i$ updates the key $k$ of \tab{}, $ht$. $T_j$ invokes a \rvmt{} $rvm_{jy}$ on the key same $k$ of \tab{} $ht$ which is the first \mth{} on $\langle ht, k \rangle$. Thus, $(\langle ht,k \rangle \in \udset{T_i}) \land (\rvm_{jy}(ht, k, v) \in \rvset{T_j}) \land (\rvm_{jy}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_j}{H})$, where $\rvset{T_j}$ is return value set of $T_j$. (3) $T_i$'s \tryc{} completed before $T_j$'s \rvm, i.e., $\tryc_i \prec_{H}^{\mr} \rvm_{jy}$.% Same conflict is preserved by the subsequent \mth{s} of $T_j$, we call it \emph{conflict inheritance}. 
	
	\item \textbf{rv-tryC} conflict:(1) $T_j$ is committed (2) $T_i$ invokes a \rvmt on the key same $k$ of \tab{} $ht$ which is the first \mth{} on $\langle ht, k \rangle$. $T_j$ updates the key $k$ of the \tab{}, $ht$. Thus, $(\rvm_{ix}(ht, k, v) \in \rvset{T_i}) \land (\rvm_{ix}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H}) \land (\langle ht,k \rangle \in \udset{T_j})$ (3) $T_i$'s \rvm completed before $T_j$'s \tryc, i.e., $\rvm_{ix} \prec_{H}^{\mr} \tryc_j$. %Similarly, all subsequent \mth{s} of $T_i$ which happen before $\tryc_j$ preserve the same conflict we term it as \emph{conflict inheritance}. 
\end{itemize}

A \rvmt{} $\rvm_{ij}$ conflicts with a \tryc{} \mth{} only if $\rvm_{ij}$ is the first \mth{} of $T_i$ that operates on \tab{} with a given key. Thus the conflict notion is defined only by the \mth{s} that access the shared memory. $(\tryc_i{}, \tryc_j{})$, $(\tryc_i{}, \tlook_j)$, $(\tlook_i, \tryc_j{})$, $(\tryc_i{}, \tdel_j)$ and $(\tdel_i, \tryc_j{})$ can be the possible conflicting \mth{s}. For example, consider the history $H5: l_1(ht, k_1, NULL) l_2(ht, k_2$ $, NULL) i_2(ht, k_1, v_1) i_1(ht, k_4,$ $v_1) c_1 i_3(ht, k_3\\, v_3) c_3 d_2(ht, k_4, v_1) c_2 l_4(ht, k_4, NULL)$ $i_4(ht, k_2, v_4) c_4$ in \figref{netys}. $(l_1(ht, k_1, NULL), i_3(ht, k_1, v_1))$ and $(l_2(ht, k_2, NULL), i_4$ $(ht, k_2, v_4))$ are a conflict of type \emph{rv-tryC}. Conflict type of $(i_1(ht, k_4, v_1), \\d_2(ht, k_4, v_1))$ and $(i_1(ht, k_4, v_1),$ $l_4(ht, k_4, NULL))$ are \emph{tryC-tryC} and \emph{tryC-rv} respectively. 
%\vspace{-.3cm}
\begin{figure}[H]
	\centering
	%		\captionsetup{justification=centering}
	\scalebox{.5}{\input{figs/netys.pdf_t}}
	% \vspace{-16cm}
	\caption{Graph Characterization of history $H5$}
	\label{fig:netys}
\end{figure}

\vspace{1mm}
\noindent
\textbf{Conflict Opacity:} Using this conflict notion, we can now define \coopty. A sequential history $H$ is conflict-opaque (or co-opaque) if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e. , $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$ and (4) S preserves conflicts (i.e. $\prec^{CO}_{H}\subseteq\prec^{CO}_{S}$). 

\noindent Thus from the above definition, it can be seen that any history that is \coop is also \opq. 
\ignore{
	\vspace{-.4cm}
	\begin{definition}
		\label{def:co-opacity}
		\texttt{Co-opacity :} 	A sequential history $H$ is conflict-opaque (or co-opaque) if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e. , $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$ and (4) S preserves conflicts (i.e. $\prec$$^{CO}_{H}$ $\subseteq$ $\prec$$^{CO}_{S}$) \cite{KuzPer:NI:TCS:2017}. 
	\end{definition}
	\vspace{-.5cm}
}

\vspace{1mm}
\noindent
\textbf{Graph Characterization:} We now develop a graph characterization of \coopty. For a sequential history $H$, we define \emph{conflict-graph} of $H$, $\cg{H}$ as the pair $(V, E)$ where $V$ is the set of $\txns{H}$ and \emph{E} can be of following types: (a) \emph{conflict edges:} \{($T_i$, $T_j$) : ($T_i$, $T_j$) $\in$ \conf{H}\} where, \conf{H} is an ordered pair of transactions such that the transactions have one of the above pair of conflicts. (b) \emph{real-time edge(or rt edge):} \{($T_i$, $T_j$): Transaction $T_i$ precedes $T_j$ in real-time, i.e., $T_i \prec_{H}^{\tr} T_j $\}.

\ignore{
	\vspace{-.2cm}
	\begin{itemize}%[noitemsep,nolistsep]
		\item \emph{conflict edges:} \{($T_i$, $T_j$) : ($T_i$, $T_j$) $\in$ \conf{H}\} where, \conf{H} is an ordered pair of transactions such that the transactions have one of the above pair of conflicts. 
		
		\item \emph{real-time edge(or rt edge):} \{($T_i$, $T_j$) : $T_i \prec_{H}^{\tr} T_j $\}
	\end{itemize}
}

Now, we have the following theorem which explains how graph characterization is useful.

\ignore{
	\begin{lemma}
		\otm{} histories are sequential and legal.
		\vspace{-0.4cm}
	\end{lemma}
	
	In the accompanying report\cite{DBLP:journals/corr/abs-1709-00681} we show that at operational level \otm{} histories are linearizable and the conflicts \mth{} can be ordered in such a way that the generated sequential histories are legal.
}
%\vspace{-.3cm}
\begin{theorem}
	\label{thm:coop-graph}
	A legal \otm{} history $H$ is \coop{} iff CG(H) is acyclic.
	%\vspace{-0.4cm}
\end{theorem}
\noindent Using this framework, we next develop \otm using the notion of \bto. We show the correctness of the proposed algorithm by showing that all conflict graph of the histories generated by it are acyclic. %The legality and conflict notion established here are used to prove that histories generated by the \otm{} are correct or \coop{}\cite{KuzPer:NI:TCS:2017} in \secref{POC}.





\noindent
\textbf{Local-Opacity:} Following \cite{KuznetsovPeri:Non-interference:TCS:2017}, it is also a correctness criteria of a history $H$ which says if all the sub histories $SH$ corresponding to each aborted transactions and $SH$ corresponding to last committed transactions while considering only committed transactions are opaque then $H$ is locally opaque. Here, a sub history $SH$ consists of committed transaction till the successful methods of aborted transactions in it.

%Due to lack of space, please refer  \apnref{ap-corr} for the definition of valid history, legal history, opacity, co-opacity and local-opacity.

}

==> Arxiv SFKOSTM SSS19/ap-rcode.tex <==
\section{Working of SF-SVOSTM and Remaining Pseudo code of SF-KOSTM Algorithms}
\label{apn:ap-rcode}
In this section, we cover the working of \emph{Starvation-Free Single-Version OSTM (SF-SVOSTM)} algorithm and remaining pseudo code of \emph{Starvation-Free Multi-Version OSTM (SF-MVOSTM)}.
\subsection{Working of SF-SVOSTM Algorithm and Importance of Timestamp ranges}
\label{apn:ap-sfostm}

This subsection describes the working of \emph{Starvation-Free Single-Version OSTM (SF-SVOSTM)} algorithm which includes the detail description of SF-SVOSTM methods and challenges to make it starvation-free.  

SF-SVOSTM invokes \tbeg{()}, \tlook{()}, \tdel{()}, \tins{()}, and \tryc{()} methods. \tlook{()} and \tdel{()} works as \rvmt{()} which lookup the value of key $k$ from shared memory and returns it. Whereas \tins{()} and \tdel{()} work as \upmt{()} that modifies the value of $k$ in shared memory. We propose optimistic SF-SVOSTM, so, \upmt{()} first update the value of $k$ in its local log $txLog$ and the actual effect of \upmt{()} will be visible after successful \tryc{()}. This subsection explains the functionality of each method as follows:

\noindent
\textbf{\tbeg{():}} %STM transactions are called by the thread $Th_i$. 
We show the high-level view of \tbeg{()} in \algoref{obegin1}. When a thread $Th_i$ invokes transaction $T_i$ for the first time (or first incarnation) then \tbeg{()} assigns a unique timestamp known as \emph{current timestamp} $(cts)$ as shown in \Lineref{obeg6}. It is incremented atomically with the help of atomic global counter ($gcounter$). If $T_i$ gets aborted then thread $Th_i$ executes it again with new incarnation of $T_i$, say $T_j$ with the new $cts$ until $T_i$ commits but retains its initial $cts$ as \emph{initial timestamp} $(its)$ at \Lineref{obeg8}. $Th_i$ uses $its$ to inform the STM system that whether $T_i$ is a new invocation or an incarnation. %So, $Th_i$ maintains $\langle \emph{its, cts}\rangle$ for transaction $T_i$.
If $T_i$ is the first incarnation then $its$ and $cts$ are same as $cts_i$ so, $Th_i$ maintains $\langle \emph{$its_i$, $cts_i$}\rangle$. If $T_i$ gets aborted and retries with $T_j$ then $Th_i$ maintains $\langle \emph{$its_i$, $cts_j$}\rangle$. We use timestamp (\emph{ts}) $i$ of $T_i$ as $cts_i$, i.e., $\langle cts_i$ = $i\rangle$ for SF-SVOSTM. 
% Initially, thread $Th_i$ calls \tbeg{()} which maintains $\langle \emph{its, cts}\rangle$ for transaction $T_i$. If $T_i$ is the first incarnation then its \emph{Initial Timestamp (its)} and \emph{Current Timestamp (cts)} are same as $i$. We represent the $\langle its, cts\rangle$ as $\langle its_i, cts_i\rangle$ for transaction $T_i$. If $T_i$ is aborted then thread $Th_i$ executes it again with new incarnation of $T_i$ until $T_i$ commits. Let the new incarnation of $T_i$ say $T_j$ then thread $Th_i$ maintain its $\langle its, cts \rangle$ as $\langle its_i, cts_j \rangle$. $Th_i$ stores the first incarnation $its_i$ of $T_i$ to set the reincarnation $its_j$ of $T_j$ is same as $its_i$. $cts$ is incremented atomically with the help of atomic global counter. %SF-KOSTM is unable to achieve the starvation-freedom with the help of $cts$ as shown in \tabref{sfillus1}.  


%\vspace{-.1cm}

%\vspace{.05mm}

By assigning priority to the lowest $its$ (i.e. transaction have been in the system for longer time) \emph{Starvation-Freedom} can achieve in \emph{Single-Version OSTM}. %But achieving \emph{Starvation-Freedom} in finite \emph{K-Versions OSTM (SF-KOSTM)} is challenging. Though the transaction $T_i$ has lowest $its$ but $T_i$ may return abort because due to finite versions $T_i$ did not find a correct version to lookup from or overwrite a version. \tabref{sfillus1} shows the key insight to achieve the \stfdm in finite K-versions OSTM. Here, we considered two transaction $T_{10}$ and $T_{20}$ with $cts$ 10 and 20 that performs $lookup$ $($or $l)$ and $insert$ $($or $i)$ on same key $k$. We assume, there exist a version of $k$ with $cts$ 5. We can observed it from the \tabref{sfillus1}, in some cases $T_{10}$ has to return abort. But if $T_{20}$ gets the lowest $its$ then $T_{20}$ never returns abort. This ensures that a transaction with lowest $its$ and highest $cts$ will never return abort. But achieving highest $cts$ along with lowest $its$ is bit difficult because new transactions are keep on coming with higher $cts$ using $gcounter$. So, to achieve the highest $cts$, we used a new timestamp as \emph{working timestamp (wts)} which is significantly larger than $cts$. 

\begin{algorithm}[H] 
%	\scriptsize
	\caption{\emph{STM\_begin($its$)}: This method is invoke by a thread $Th_i$ to start a new transaction $T_i$. It pass a parameter $its$ which is the initial timestamp of the first incarnation of $T_i$. If $T_i$ is the first incarnation then $its$ is $nil$.}
	\label{algo:obegin1} 
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{209}\makeatother
			\Procedure{\emph{STM\_begin($its$)}}{}  \label{lin:obeg1}
			\State Create a local log $txLog_i$ for each transaction $T_i$. \label{lin:obeg2}
			\If {($its == nil$)} \label{lin:obeg3}
			\State /* Atomically get the value from the global counter and set it to its, and, \blank{1cm} cts.*/ \label{lin:obeg4}
			\State $its_i$ = $cts_i$ = \emph{gcounter.get\&Inc()}; \label{lin:obeg5}
			\Else  \label{lin:obeg6}
			\State /*Set the $its_i$ to first incarnation of $T_i$ $its$*/ \label{lin:obeg7}
			\State $its_i$ = $its$; \label{lin:obeg8}
			\State /*Atomically get the value from the global counter for $cts_i$*/ \label{lin:obeg9}
			\State $cts_i$ = \emph{gcounter.get\&Inc()}. \label{lin:obeg10}
			%		\State \txll.$L\_t\_id$ $\gets$ $\gcts_i \gets \gtcnt.get\&Inc()$; 
			%		\State /*Set the $wts$ value with the help of $cts_i$ and $its_i$*/
			%		\State $wts_i$ = $cts_i$+C*($cts_i$-$its_i$).
			\EndIf \label{lin:obeg11}
			%		\State /*Set the $tltl_i$ as $cts_i$*/
			%		\State $tltl$ = $cts_i$.  
			%		\State /*Set the $tutl_i$ as possible large value*/
			%		\State $tutl_i$ = $\infty$.
			\State /*Initially, set the $status_i$ of $T_i$ as $live$*/ \label{lin:obeg12}
			\State $status_i$ = $live$;  \label{lin:obeg13}
			\State return $\langle cts_i, its_i\rangle$ \label{lin:obeg14}
			
			\EndProcedure
		\end{algorithmic}
%	\end{multicols}
\end{algorithm}

\cmnt{

\begin{algorithm} 
	\scriptsize
	\caption{\emph{STM\_begin($its$)}: This method is invoke by a thread to start a new transaction $T_i$. It pass a parameter $its$ which is the initial timestamp of the first incarnation of $T_i$. If this is the first incarnation then $its$ is $nil$.}
		\label{algo:obegin1} 
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{68}\makeatother
		\Procedure{\emph{STM\_begin($its$)}}{}  \label{lin:obeg1}
		\State Creating a local log $txLog_i$ for each transaction. \label{lin:obeg2}
		\If {($its == nil$)} \label{lin:obeg3}
		\State /* Atomically get the value from the global \blank{.7cm} counter and set it to its, and, cts.*/ \label{lin:obeg4}
		\State $its_i$ = $cts_i$ = \emph{gcounter.get\&Inc()}; \label{lin:obeg5}
		\Else  \label{lin:obeg6}
		\State /*Set the $its_i$ to first incarnation of $T_i$ $its$*/ \label{lin:obeg7}
		\State $its_i$ = $its$; \label{lin:obeg8}
		\State /*Atomically get the value from the global \blank{.7cm} counter for $cts_i$*/ \label{lin:obeg9}
		\State $cts_i$ = \emph{gcounter.get\&Inc()}. \label{lin:obeg10}
		%		\State \txll.$L\_t\_id$ $\gets$ $\gcts_i \gets \gtcnt.get\&Inc()$; 
%		\State /*Set the $wts$ value with the help of $cts_i$ and $its_i$*/
%		\State $wts_i$ = $cts_i$+C*($cts_i$-$its_i$).
		\EndIf \label{lin:obeg11}
%		\State /*Set the $tltl_i$ as $cts_i$*/
%		\State $tltl$ = $cts_i$.  
%		\State /*Set the $tutl_i$ as possible large value*/
%		\State $tutl_i$ = $\infty$.
		\State /*Initially, set the $status_i$ of $T_i$ as $live$*/ \label{lin:obeg12}
		\State $state_i$ = $live$;  \label{lin:obeg13}
		\State return $\langle cts_i, its_i\rangle$ \label{lin:obeg14}
		
		\EndProcedure
	\end{algorithmic}
	\end{multicols}
\end{algorithm}

\noindent
\tbeg{()} maintains the $wts$ for transaction $T_i$ as $wts_i$, which is potentially higher timestamp as compare to $cts_i$. So, we derived,
\setlength\abovedisplayskip{0pt}
\begin{equation}
	\label{eq:wtsf}
	\twts{i} = \tcts{i} + C * (\tcts{i} - \tits{i});
	\vspace{-.2cm}
\end{equation}
%$wts_i$ = $cts_i$ + C*($cts_i$-$its_i$)
Where C is any constant value greater than 0. When $T_i$ is issued for the first time then $wts_i$, $cts_i$, and $its_i$ are same. If $T_i$ gets aborted again and again then drift between the $cts_i$ and $wts_i$ will increases. The advantage for maintaining $wts_i$ is if any transaction keeps getting aborted then its $wts_i$ will be high and $its_i$ will be low. So, eventually $T_i$ will get chance to commit in finite number of steps to achieve starvation-freedom. 
\vspace{-.2cm}
\begin{observation}
	Any transaction $T_i$ with lowest $its_i$ and highest $wts_i$ will never abort.
\end{observation}

%\vspace{.2mm}
\vspace{-.1cm}
Sometimes, the value of $wts$ is significantly larger than $cts$. So, $wts$ is unable to maintain \emph{real-time order} between the transactions as shown in \figref{} in \apnref{ap-rcode}. To address this issue SF-KOSTM uses the idea of timestamp ranges \cite{Riegel+:LSA:DISC:2006,Guer+:disc1:2008, Crain+:RI_VWC:ICA3PP:2011} along with the $\langle its_i, cts_i, wts_i \rangle$ for transaction $T_i$ in \tbeg{()}. It maintains the \emph{transaction lower timestamp limit ($tltl_i$)} and \emph{transaction upper timestamp limit ($tutl_i$)} for transaction $T_i$. It helps to maintain the \emph{real-time order} among the transactions. Initially, $\langle its_i, cts_i, wts_i, tltl_i \rangle$ are the same for $T_i$. $tutl_i$ would be set as a largest possible value denoted as $+\infty$ for $T_i$. After successful execution of \tryc{()} of transaction $T_i$, $tltl_i$ gets incremented and $tutl_i$ gets decremented\footnote{Practically $\infty$ can't be decremented for $tutl_i$ so we assign the highest possible value to $tutl_i$ which gets decremented.}.
}
 \tbeg{()} initializes the \emph{transaction local log $(txLog_i)$} for each transaction $T_i$ to store the information in it. Whenever a transaction starts it atomically sets its \emph{status} to be \emph{live} as a global variable at \Lineref{obeg13}. Transaction \emph{status} can be $\langle live, commit, false\rangle$. After successful execution of \tryc{()}, $T_i$ sets its \emph{status} to be \emph{commit}. If the \emph{status} of the transaction $T_i$ is \emph{false} then it returns \emph{abort} which says that $T_i$ is not having the lowest $its$ among other concurrent conflicting transactions. So to propose starvation-free SVOSTM other conflicting transactions sets its \emph{status} field as \emph{false} and force transaction $T_i$ to \emph{abort}.
  %For more details please refer the algorithm of \tbeg{()} in \apnref{ap-rcode}.  


%Initially, each threads $Th_x$ call this method and gets the unique time stamp (\emph{ts}) $i$ for each transaction $T_i$. If $Th_x$ calls $T_i$ for first time then its \emph{Current Timestamp (cts)} would be $i$. If $T_i$ gets aborted and executed again by the $Th_x$ as a reincarnation of $T_i$ to $T_j$ then its cts would be $j$. cts is incremented atomically with the help of global counter. If $T_i$ is not the first incarnation then $Th_x$ pass its first incarnation cts to STM system to notify that this is not the first incarnation. STM system maintains the first incarnation of $T_i$ as \emph{Initial Timestamp (its)} for all its incarnation such as $T_j$. Each incarnation of $T_i$ as $T_j$ maintains two timestamp such as $\langle its, cts\rangle$. For the first incarnation of $T_i$ $\langle its, cts \rangle$ are same.


%\tryc{()} maintains the $wts_j$ of current version $ver_j$ of each key $k$ in currVL. It maintains the 

\noindent
\textbf{\tlook{()} and \tdel{()} as \rvmt{s()}:} \emph{\rvmt{(ht, k, val)}} returns the value (\emph{val}) corresponding to the key \emph{k} from the shared memory as hash table (\emph{ht}). We show the high-level overview of the \rvmt{()} in \algoref{orvmt}. First, it identifies the key $k$ in the transaction local log as \emph{$txLog_i$} for transaction $T_i$. If $k$ exists then it updates the $txLog_i$ and returns the $val$ at \Lineref{orvm2}.


If key $k$ does not exist in the $txLog_i$ then before identifying the location in share memory \rvmt{()} checks the \emph{status} of $T_i$ at \Lineref{orvm5}. If the \emph{status} of $T_i$ (or $i$) is \emph{false} then $T_i$ has to \emph{abort} which says that $T_i$ is not having the lowest $its$ among other concurrent conflicting transactions. So to propose starvation-free SVOSTM other conflicting transactions sets its \emph{status} field as \emph{false} and force transaction $T_i$ to \emph{abort}.

\begin{algorithm}
	%	\scriptsize
	\caption{\emph{\rvmt{(ht, k, val)}:} It can either be $\tdel_i(ht, k, val)$ or $\tlook_i(ht, k, val)$ on key $k$ of transaction $T_i$.} \label{algo:orvmt} 	
	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{224}\makeatother
		\Procedure{$\rvmt_i$}{$ht, k, val$}	\label{lin:orvm1}	
		\If{($k \in \llog_i$)}
		\State Update the local log and return $val$.  \label{lin:orvm2}
		\Else \label{lin:orvm3}
		\State /*Atomically check the \emph{status} of its own transaction $T_i$ (or $i$)*/ \label{lin:orvm4} %after acquiring \emph{atomic lock} on it*/
		\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:orvm5}
		\EndIf\label{lin:orvm6}
		\State Identify the \emph{preds[]} and \emph{currs[]} for $k$ in bucket $M_k$ of \lsl using \bn \blank{1cm} and \rn . \label{lin:orvm7}
		\State Acquire locks on \emph{preds[]} \& \emph{currs[]} in increasing order. \label{lin:orvm8}
		\If{(\emph{!rv\_Validation(preds[], currs[])})} \label{lin:orvm9}
		\State Release the locks and goto \linref{orvm7}. \label{lin:orvm10}
		\EndIf \label{lin:orvm11}
		%			\State Release the locks; update the $\llog_i$ with $k$ \blank{.7cm} and value. \label{lin:orvm30}
		%	\EndIf \label{lin:orvm31}
		%		\State return $\langle$$ver_j.val$$\rangle$. \label{lin:orvm32}
		\If{($k  ~ \notin ~ M_k.\lsl$)} \label{lin:orvm12} 
		\State Create a new node $n$ with key $k$ as:  $\langle$\emph{key=k, lock=false, mark=true, \blank{1.5cm} rvl=i, nNext=}$\phi\rangle$./*$n$ is marked*/  \label{lin:orvm13}
		%\State \Comment{The $vl$ consists of a single element $v$ with $ts$ as $i$}
		%			\State Create version $ver$ as:$\langle$\emph{ts=0, val=null, rvl=i, \blank{1.1cm} vrt=0, vNext=$\phi$}$\rangle$. \label{lin:orvm14}
		\State Insert $n$ into $M_k.$\emph{\lsl} s.t. it is accessible only via \rn{s}. /*\emph{lock} sets \blank{1.6cm}\emph{true}*/  \label{lin:orvm15}  	
		\State Release locks; update the $\llog_i$ with $k$.\label{lin:orvm16}
		\State return $\langle$\emph{val}$\rangle$. /*\emph{val} as $null$*/\label{lin:orvm17}
		\Else
		\State Add $i$ into the $rvl$ of \emph{currs[]}. \label{lin:orvm29} 
		%		\State $retVal = ver_j.val$.
		\State Release the locks; update the $\llog_i$ with $k$ and value. \label{lin:orvm30}
		\State return $\langle$$val$$\rangle$. \label{lin:orvm32}
		\EndIf \label{lin:orvm18}
		%			\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the largest timestamp smaller (lts) than $i$.\label{lin:orvm19}
		%			\If{($ver_j$ == $null$)} /*Finite Versions*/
		%			\State return $\langle abort_i\rangle$ \label{lin:orvm111}
		%		\EndIf
		%			\ElsIf{($ver_j.vNext$ != $null$)}\label{lin:orvm20}
		%\State /*$tutl_i$ should be less then \emph{vrt} of next ver- \blank{1.1cm}sion $ver_j$*/\label{lin:orvm21}
		%\State 	Calculate $tutl_i$ = min($tutl_i$, $ver_j.vNext$ $\blank{1.1cm}.vrt-1$).\label{lin:orvm22}
		%\EndIf\label{lin:orvm23}
		%			\State /*$tltl_i$ should be greater then $vrt$ of $ver_j$*/\label{lin:orvm24}
		%			\State 	Calculate $tltl_i$ = max($tltl_i$, $ver_j.vrt+1$).\label{lin:orvm25}
		%		\State /*If limit has crossed each other then abort $T_i$*/\label{lin:orvm26}
		%		\If{($tltl_i$ $>$ $tutl_i$)} return $\langle abort_i \rangle$. \label{lin:orvm27}
		%		\EndIf\label{lin:orvm28}
		%\State $ver_j = find\_lts(k)$.\label{lin:corr-ver} 
		\EndIf \label{lin:orvm31}
		\EndProcedure \label{lin:orvm33}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
\vspace{.2mm}



If the \emph{status} of $T_i$ is not \emph{false} and $k$ is not exist in the $txLog_i$ then it identifies the location optimistically (without acquiring the locks similar to the \emph{lazy-list}\cite{Heller+:LazyList:PPL:2007}) in the shared memory at \Lineref{orvm7}. SF-SVOSTM maintains the shared memory in the form of a hash table with $M$ buckets as shown in \subsecref{dsde}, where each bucket stores the keys in the form of \emph{\lsl}. Each node contains two pointer $\langle \rn, \bn \rangle$. So, it identifies the two \emph{predecessors (pred)} and two \emph{current (curr)} with respect to each node. First, it identifies the pred and curr for key $k$ in \bn{} as $\langle \bp, \bc \rangle$. After that it identifies the pred and curr for key $k$ in \rn{} as $\langle \rp, \rc \rangle$. If $\langle \rp, \rc \rangle$ are not marked then $\langle \bp=\rp, \bc=\rc\rangle$. SF-SVOSTM maintains the keys are in increasing order. So the order among the nodes are $\langle \bp.key \leq \rp.key < k \leq \rc.key \leq \bc.key\rangle$.



\rvmt{()} acquires the lock in predefined order on all the identified preds and currs for key $k$ to avoid the deadlock at \Lineref{orvm8} and do the \emph{rv\_Validation()} at \Lineref{orvm9}. If $\langle \bp \vee \bc\rangle$ is marked or preds are not pointing to identified currs as $\langle (\bp.\bn \neq \bc) \vee (\rp.\rn \neq \rc)\rangle$ shown in \algoref{llsearch} then it releases the locks on all the preds and currs and identify the new preds and currs for key $k$ in shared memory. 



\cmnt{

\begin{algorithm}
	\scriptsize
	\caption{\emph{\rvmt{()}:} Could be either $\tdel_i(ht, k, val)$ or $\tlook_i(ht, k, val)$ on key $k$.} \label{algo:orvmt} 	
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{83}\makeatother
			\Procedure{$\rvmt_i$}{$ht, k, val$}	\label{lin:orvm1}	
			\If{($k \in \llog_i$)} \label{lin:orvm2}
			\State Update the local log and return $val$. 
			\Else \label{lin:orvm3}
			\State /*Atomically check the \emph{status} of its own transac- \blank{.7cm}tion $T_i$ (or $i$)*/ \label{lin:orvm4} %after acquiring \emph{atomic lock} on it*/
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:orvm5}
			\EndIf\label{lin:orvm6}
			\State Identify the \emph{preds[]} and \emph{currs[]} for $k$ in bucket \blank{.7cm} $M_k$ of \lsl using \bn and \rn . \label{lin:orvm7}
			\State Acquire locks on \emph{preds[]} \& \emph{currs[]} in increasing \blank{.7cm} order. \label{lin:orvm8}
			\If{(\emph{!rv\_Validation(preds[], currs[])})} \label{lin:orvm9}
			\State Release the locks and goto \linref{orvm7}. \label{lin:orvm10}
			\EndIf \label{lin:orvm11}
	%			\State Release the locks; update the $\llog_i$ with $k$ \blank{.7cm} and value. \label{lin:orvm30}
		%	\EndIf \label{lin:orvm31}
	%		\State return $\langle$$ver_j.val$$\rangle$. \label{lin:orvm32}
			\If{($k  ~ \notin ~ M_k.\lsl$)} \label{lin:orvm12} 
			\State Create a new node $n$ with key $k$ as: \blank{.8cm} $\langle$\emph{key=k, lock=false, mark=true, rvl=i, \blank{1.1cm} nNext=}$\phi\rangle$./*$n$ is marked*/  \label{lin:orvm13}
			%\State \Comment{The $vl$ consists of a single element $v$ with $ts$ as $i$}
%			\State Create version $ver$ as:$\langle$\emph{ts=0, val=null, rvl=i, \blank{1.1cm} vrt=0, vNext=$\phi$}$\rangle$. \label{lin:orvm14}
			\State Insert $n$ into $M_k.$\emph{\lsl} s.t. it is accessi- \blank{1.1cm}ble only via \rn{s}.  \label{lin:orvm15}  	
			\State Release locks; update the $\llog_i$ with $k$.\label{lin:orvm16}
			\State return $\langle$\emph{val}$\rangle$. /*\emph{val} as $null$*/\label{lin:orvm17}
			\Else
			\State Add $i$ into the $rvl$ of \emph{currs[]}. \label{lin:orvm29} 
			%		\State $retVal = ver_j.val$.
			\State Release the locks; update the $\llog_i$ with \blank{1.1cm} $k$ and value. \label{lin:orvm30}
			\State return $\langle$$val$$\rangle$. \label{lin:orvm32}
			\EndIf \label{lin:orvm18}
%			\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the largest timestamp smaller (lts) than $i$.\label{lin:orvm19}
%			\If{($ver_j$ == $null$)} /*Finite Versions*/
%			\State return $\langle abort_i\rangle$ \label{lin:orvm111}
			%		\EndIf
%			\ElsIf{($ver_j.vNext$ != $null$)}\label{lin:orvm20}
			%\State /*$tutl_i$ should be less then \emph{vrt} of next ver- \blank{1.1cm}sion $ver_j$*/\label{lin:orvm21}
			%\State 	Calculate $tutl_i$ = min($tutl_i$, $ver_j.vNext$ $\blank{1.1cm}.vrt-1$).\label{lin:orvm22}
			%\EndIf\label{lin:orvm23}
%			\State /*$tltl_i$ should be greater then $vrt$ of $ver_j$*/\label{lin:orvm24}
%			\State 	Calculate $tltl_i$ = max($tltl_i$, $ver_j.vrt+1$).\label{lin:orvm25}
	%		\State /*If limit has crossed each other then abort $T_i$*/\label{lin:orvm26}
	%		\If{($tltl_i$ $>$ $tutl_i$)} return $\langle abort_i \rangle$. \label{lin:orvm27}
	%		\EndIf\label{lin:orvm28}
			%\State $ver_j = find\_lts(k)$.\label{lin:corr-ver} 
			\EndIf \label{lin:orvm31}
			\EndProcedure \label{lin:orvm33}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}
\vspace{.2mm}
}



If key $k$ does not exist in the \emph{\lsl{}} of the corresponding bucket $M_k$ at \Lineref{orvm12} then it creates a new node $n$ with key $k$ as $\langle \emph{key=k, lock=false, mark=true, rvl=i, nNext=}\phi \rangle$ at \Lineref{orvm13}. $T_i$ adds its \emph{$cts_i$} in the \emph{rvl}. Finally, it inserts the node $n$ into $M_k.\lsl$ such that it is accessible via \rn{} only at \Lineref{orvm15}. \rvmt{()} releases the locks and update the $txLog_i$ with key $k$ and value as $null$ (\Lineref{orvm16}). Eventually, it returns the \emph{val} as $null$ at \Lineref{orvm17}.  

  

\begin{algorithm}[H]
	%\label{alg:llsearch} 
	%	\scriptsize
	\caption{\emph{rv\_Validation(preds[], currs[])}: It is mainly used for \emph{rv\_method()} validation.}
	\label{algo:llsearch} 
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{248}\makeatother
		\Procedure{$rv\_Validation{(\emph{preds[], currs[]})}$}{} \label{lin:orvv1}
		\If{$((\bp.mark) || (\bc.mark) || ((\bp.\bn)\neq \blank{1.8cm} \bc) || ((\rp.\rn) \neq {\rc})$)}\label{lin:orvv2}
		return $\langle false \rangle$. 
		\Else{} return $\langle true \rangle$. \label{lin:orvv3}
		\EndIf \label{lin:orvv4}
		\EndProcedure \label{lin:orvv5}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}

%\vspace{.2mm}  

\vspace{-.5mm}

If key $k$ exists in the $M_k.\lsl$ then %it identifies the current version $ver_j$ with $ts$ = $j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$ at \Lineref{rvm19}. If $ver_j$ is $null$ at \Lineref{rvm111} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise it identifies the next version with the help of $ver_j.vNext$. If next version ($ver_j.vNext$ as $ver_k$) exist then $T_i$ maintains the $tutl_i$ which should be minimum between $\langle tutl_i$ $\vee$ $ver_k.vrt-1\rangle$ to maintains the \emph{real-time order} among the transactions at \Lineref{rvm22}. Same as it maintains the $tltl_i$ which should be maximum of $\langle tltl_i \vee $ $ver_j.vrt+1$$\rangle$ at \Lineref{rvm25}. If $tltl_i$ is greater than $tutl_i$ at \Lineref{rvm27} then transaction $T_i$ have to returns \emph{abort} (fail to maintain the timestamp order) otherwise 
it adds the $cts_i$ of $T_i$ as $i$ in the $rvl$ of \emph{currs[]} at \Lineref{orvm29}. Finally, it releases the lock and updates the $txLog_i$ with key $k$ and value as val at \Lineref{orvm30}. Eventually, it returns the \emph{val} at \Lineref{orvm32}.  


\noindent
\textbf{\tins{()} and \tdel{()} as \upmt{s()}:} Actual effect of \tins{()} and \tdel{()} comes after successful \tryc{()}. %They creates the version corresponding to the key in shared memory. 
We shows the high level view of \tryc{()} in \algoref{otryc}. First, \tryc{()} checks the \emph{status} of the transaction $T_i$ at \Lineref{otc3}. If \emph{status} of $T_i$ is \emph{false} then $T_i$ has to \emph{abort} same as explained above in \rvmt{()}. 



If the \emph{status} is not false then \tryc{()} sort the keys (exist in $txLog_i$ of $T_i$) of \upmt{s()} in increasing order. % which belongs to  only. % such as \tins{()} and \tdel{()}. 
It takes one by one method ($m_{ij}$) from the $txLog_i$ and identifies the location of the key $k$ in \emph{$M_k$.\lsl} as explained above in \rvmt{()}. After identifying the preds and currs for $k$ it acquires the locks in predefined order to avoid the deadlock at \Lineref{otc10} and calls \emph{tryC\_Validation()} to validate the methods of $T_i$.

\emph{tryC\_Validation()} identifies whether the methods of invoking transaction $T_i$ are inserting/updating a node corresponding to the keys while ensuring the \emph{starvation-freedom}. %First, it do the \emph{rv\_Validation()} as explained in \rvmt{()} above. If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise maintains the information of $ver_j$ and its next version ($ver_j.vNext$) which helps transaction $T_i$ to sets its $tltl_i$ and $tutl_i$. If $wts_i$ of $T_i$ is less then other $live$ transactions $wts$ exist in $ver_j.rvl$ then $T_i$ sets the $status$ to be $false$ to all other transactions otherwise $T_i$ returns to $abort$. The detailed descriptions are in \apnref{ap-rcode}.
%It maintains the Current Version List (currVL), Next Version List (nextVL), All Return Value List (allRVL), Large Return Value List (largeRVL), Small Return Value List (smallRVL) from $ver_j$ of key $k$. currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. These terms helps to decide, whether  $T_i$ will create the version and commit while aborting the conflicting transactions or $T_i$ returns abort. 
First, it do the \emph{rv\_Validation()} at \Lineref{otcv2} as explained in \rvmt{()}. If \emph{rv\_Validation()} is successful and key $k$ exists in the $M_k.\lsl$ then %it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$ at \Lineref{tcv5}. If $ver_j$ is $null$ at \Lineref{tcv111} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise after identifying the current version $ver_j$ 
it maintains the All Return Value List (allRVL) from \emph{currs[]} of key $k$ at \Lineref{otcv6}. %currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. 
Acquire the locks on \emph{status} of all the transactions present in allRVL list including $T_i$ it self in predefined order to avoid the deadlock at \Lineref{otcv8}. First, it checks the \emph{status} of its own transaction $T_i$ at \Lineref{otcv10}. If the \emph{status} of $T_i$ is \emph{false} then $T_i$ has to \emph{abort} the same reason as explained in \rvmt{()}. 



If \emph{status} of $T_i$ is not \emph{false} then it compares the $its_i$ of its own transaction $T_i$ with the $its_p$ of other transactions $T_p$ ($p$) present in the allRVL at \Lineref{otcv13}. Along with this it checks the \emph{status} of $p$. If above conditions $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ succeed then it includes $T_p$ in the Abort Return Value List (abortRVL) at \Lineref{otcv14} to abort $T_p$ later otherwise abort $T_i$ itself at \Lineref{otcv15}.  

\begin{algorithm}
	
	%	\scriptsize
	\caption{\tryc{($T_i$)}: Validate the \upmt{s()} of the transaction $T_i$ and returns \emph{commit}.}
	%	\setlength{\multicolsep}{0pt}
	\label{algo:otryc}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{253}\makeatother
		\Procedure{$\tryc{(T_i)}$}{} \label{lin:otc1}
		%\State Get the local log list for corresponding transaction;
		\State /*Atomically check the \emph{status} of its own transaction $T_i$ (or $i$)*/ \label{lin:otc2}
		\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:otc3}
		\EndIf \label{lin:otc4}
		\State /*Sort the $keys$ of $\llog_i$ in increasing order.*/ \label{lin:otc5}
		\State /*Method ($m$) will be either \tins or \emph{STM\_delete}*/\label{lin:otc6}
		\ForAll{($m_{ij}$ $\in$ $\llog_i$)} \label{lin:otc7}
		\If{($m_{ij}$==\tins$||$$m_{ij}$==\tdel)}\label{lin:otc8}
		\State Identify the \emph{preds[]} \& \emph{currs[]} for \emph{k} in bucket $M_k$ of \emph{\lsl} using \blank{1.5cm} \bn \& \rn. \label{lin:otc9}
		\State Acquire the locks on \emph{preds[]} \& \emph{currs[]} in increasing order. \label{lin:otc10}
		\If{($!tryC\_Validation()$)}
		\State return $\langle abort_i \rangle$.\label{lin:otc11}
		\EndIf\label{lin:otc12}
		\EndIf\label{lin:otc13}
		\EndFor\label{lin:otc14}
		\ForAll{($m_{ij}$ $\in$ $\llog_i$)}\label{lin:otc15}
		\State \emph{poValidation()}  modifies the \emph{preds[]} \& \emph{currs[]} of current method which \blank{1cm} would have been updated by previous method of the same transaction.\label{lin:otc16}
		\If{(($m_{ij}$==\tins)\&\&(k$\notin$$M_k$.\lsl))}\label{lin:otc17}
		\State Create new node $n$ with $k$ as: $\langle$\emph{key=k, lock=false, mark=false, rvl=$\phi$, \blank{1.5cm} nNext=$\phi$}$\rangle$. \label{lin:otc18}
		%			\State Create first version $ver$ for $T_0$ and next for \blank{1.1cm} $i$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, vNext=$\phi$}$\rangle$.\label{lin:otc19}
		\State Insert node $n$ into $M_k$.\emph{\lsl} such that it is accessible via \rn{} as \blank{1.5cm} well as \bn{}. /*\emph{lock} sets \emph{true}*/ \label{lin:otc20}
		%		\State /*\emph{lock} sets \emph{true}*/  \label{lin:otc20}
		\ElsIf{($m_{ij}$ == \tins{})}\label{lin:otc21}
		\State /*Sets \emph{rvl} as $\phi$ and update the value*/.
		\State Node (\emph{currs[]}) is accessible via \rn and \bn. /*\emph{mark} sets \emph{false}*/
		%\State Add $ver$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, \blank{1.1cm} vNext=$\phi$}$\rangle$ into $M_k$.\emph{\lsl} \& accessible \blank{1.1cm} via \rn{}, \bn. /*\emph{mark=false}*/\label{lin:otc22}
		\EndIf\label{lin:otc23}
		\If{($m_{ij}$ == \tdel{})}\label{lin:otc24}
		\State /*Sets \emph{rvl} as $\phi$ and 			\emph{mark} as \emph{true}*/.
		\State Node (\emph{currs[]}) is accessible via \rn only.
		\label{lin:otc25}
		\EndIf\label{lin:otc26}
		\State Update the \emph{preds[]} \& \emph{currs[]} of $m_{ij}$ in $\llog_i$.\label{lin:otc27}
		
		\EndFor \label{lin:otc28}
		%\EndFor
		\State Release the locks.
		\State return $\langle commit_i \rangle$.\label{lin:otc29}
		\EndProcedure \label{lin:otc30}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}




%After that \tryc{()} maintains the $tltl_i$ and $tutl_i$ of transaction $T_i$ at \Lineref{tcv19} and \Lineref{tcv22}. The requirement of $tltl_i$ and $tutl_i$ is explained above in the \rvmt{()}. If limit of $tltl_i$ crossed with $tutl_i$ then $T_i$ have to abort at \Lineref{tcv24}. If $tltl_p$ greater than $tutl_i$ at \Lineref{tcv27} then it checks the $its_i$ and $its_p$. If $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ then add the transaction $T_p$ in the abortRVL for all the smallRVL transactions at \Lineref{tcv29} otherwise \emph{abort} $T_i$ itself at \Lineref{tcv30}.

%At \Lineref{tcv34}, $tltl_i$ would be equal to $tutl_i$ and after this step transaction $T_i$ will never \emph{abort}. $T_i$ helps the other transaction $T_p$ to update the $tutl_p$ which exists in the smallRVL and still $live$ then it sets the $tutl_p$ to minimum of $\langle tutl_p \vee tltl_i-1\rangle$ to maintain the real-time order among the transaction at \Lineref{tcv36}. 
At \Lineref{otcv39}, \tryc{()} aborts all other conflicting transactions which are present in the abortRVL while modifying the \emph{status} field to be \emph{false} to achieve \emph{starvation-freedom}. 


%\emph{tryC\_Validation()} identifies whether the methods of invoking transaction $T_i$ are able to insert or delete a version corresponding to the keys while ensuring the \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions. It does four steps for validation. Step 1: First, it does the \emph{rv\_Validation()} as explained in \rvmt{()} above. Step 2: If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts$ = $j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because it does not found the version to replace. Step 3: If $ver_j$ \emph{exist} then it compare the $its_i$ of $T_i$ with $its$ of other $live$ transactions present in $ver_j.rvl$. If $its_i$ of $T_i$ is less than the $its$ of such transactions then $T_i$ sets the $status$ of all those transactions to be $false$, otherwise, $T_i$ returns $abort$. Step 4: To maintain the \emph{real-time order}, $T_i$ update the $tltl_i$ and $tutl_i$ of it with the help of $ver_j$ and its next version ($ver_j.vNext$) respectively (explained in \rvmt{} above). Please find the detailed descriptions in \apnref{ap-rcode}.

\cmnt{
	\emph{tryC\_Validation()} identifies whether the methods of invoking transaction $T_i$ are able to insert or delete a version corresponding to the keys while ensuring the \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions. It follow the following steps for validation. Step 1: First, it do the \emph{rv\_Validation()} as explained in \rvmt{()} above. Step 2: If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise maintains the information of $ver_j$ and its next version ($ver_j.vNext$) which helps transaction $T_i$ to sets its $tltl_i$ and $tutl_i$. Step 3: If $wts_i$ of $T_i$ is less then other $live$ transactions $wts$ exist in $ver_j.rvl$ then $T_i$ sets the $status$ to be $false$ to all conflicting \emph{live} transactions otherwise $T_i$ returns $abort$. The detailed descriptions are in \apnref{ap-rcode}.
}


All the steps of the \emph{tryC\_Validation()} are successful than the actual effect of the \tins{()} and \tdel{()} will be visible to the shared memory. At \Lineref{otc16}, \tryc{()} checks for \emph{poValidation()}. When two subsequent methods $\langle m_{ij}, m_{ik}\rangle$ of the same transaction $T_i$ identify the overlapping location of preds and currs in \emph{\lsl}. Then \emph{poValidation()} updates the current method $m_{ik}$ preds and currs with the help of previous method $m_{ij}$ preds and currs. 



If $m_{ij}$ is \tins{()} and key $k$ does not exist in the $M_k.\lsl{}$ then it creates the new node $n$ with key $k$ as $\langle \emph{key=k, lock=false, mark=false, rvl=$\phi$, nNext=}\phi \rangle$ at \Lineref{otc18}. %Later, it creates a version ($ver$) for transaction $T_0$ and $T_i$ as $\langle$ \emph{ts=0, val=null, rvl=i, vrt=0, vNext=i} $\rangle$ and $\langle \emph{ts=i, val=v, rvl=}\phi, \emph{vrt=i, vNext=}\phi \rangle$ at \Lineref{tc19}. Transaction $T_i$ creates the version of transaction $T_0$ so that other concurrent conflicting transaction with lower timestamp than $T_i$ can find the version to lookup. It sets the \emph{rvl} as $\phi$ and \emph{vrt} as $i$. 
Finally, it inserts the node $n$ into $M_k.\lsl$ such that it is accessible via \rn{} as well as \bn{} at \Lineref{otc20}. If $m_{ij}$ is \tins{()} and key $k$ exists in the $M_k.\lsl{}$ then it updates the value and \emph{rvl} to $\phi$ for node corresponding to the key $k$. %If the limit of the version reach to $K$ then SF-KOSTM replace the oldest version with new version which is accessible via \rn{} as well as \bn{} at \Lineref{tc22}. 


\cmnt{
\begin{algorithm}
	
	\scriptsize
	\caption{\emph{\tryc($T_i$)}: Validate the \upmt{s} of the transaction and return \emph{commit}.}
	\setlength{\multicolsep}{0pt}
	\label{algo:otryc}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{112}\makeatother
			\Procedure{$\tryc{(T_i)}$}{} \label{lin:otc1}
			%\State Get the local log list for corresponding transaction;
			\State /*Atomically check the \emph{status} of its own transaction \blank{.3cm} $T_i$ (or $i$)*/ \label{lin:otc2}
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:otc3}
			\EndIf \label{lin:otc4}
			\State /*Sort the $keys$ of $\llog_i$ in increasing order.*/ \label{lin:otc5}
			\State /*Method ($m$) will be either \tins or \emph{STM\_ \blank{.3cm} delete}*/\label{lin:otc6}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)} \label{lin:otc7}
			\If{($m_{ij}$==\tins$||$$m_{ij}$==\tdel)}\label{lin:otc8}
			\State Identify the \emph{preds[]} \& \emph{currs[]} for \emph{k} in bucket \blank{1cm} $M_k$ of \emph{\lsl} using \bn\& \rn. \label{lin:otc9}
			\State Acquire the locks on \emph{preds[]} \& \emph{currs[]} in \blank{1cm} increasing order. \label{lin:otc10}
			\If{($!tryC\_Validation()$)}
			\State return $\langle abort_i \rangle$.\label{lin:otc11}
			\EndIf\label{lin:otc12}
			\EndIf\label{lin:otc13}
			\EndFor\label{lin:otc14}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)}\label{lin:otc15}
			\State \emph{poValidation()}  modifies the \emph{preds[]} \& \emph{currs[]} of \blank{.6cm} current method which would have been updated \blank{.6cm} by previous method of the same transaction.\label{lin:otc16}
			\If{(($m_{ij}$==\tins)\&\&(k$\notin$$M_k$.\lsl))}\label{lin:otc17}
			\State Create new node $n$ with $k$ as: $\langle$\emph{key=k, \blank{1.1cm} lock=false, mark=false, rvl=$\phi$, nNext=$\phi$}$\rangle$. \label{lin:otc18}
%			\State Create first version $ver$ for $T_0$ and next for \blank{1.1cm} $i$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, vNext=$\phi$}$\rangle$.\label{lin:otc19}
			\State Insert node $n$ into $M_k$.\emph{\lsl} such that \blank{1.1cm} it is accessible via \rn{} as well as \bn{}.
			\State /*\emph{lock} sets \emph{true}*/  \label{lin:otc20}
			\ElsIf{($m_{ij}$ == \tins{})}\label{lin:otc21}
			\State /*Sets \emph{rvl} as $\phi$ and update the value*/.
			\State Node (\emph{currs[]}) is accessible via \rn and \bn.
			%\State Add $ver$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, \blank{1.1cm} vNext=$\phi$}$\rangle$ into $M_k$.\emph{\lsl} \& accessible \blank{1.1cm} via \rn{}, \bn. /*\emph{mark=false}*/\label{lin:otc22}
			\EndIf\label{lin:otc23}
			\If{($m_{ij}$ == \tdel{})}\label{lin:otc24}
			\State /*Sets \emph{rvl} as $\phi$ and 			\emph{mark} as \emph{true}*/.
			\State Node (\emph{currs[]}) is accessible via \rn only.
			\label{lin:otc25}
			\EndIf\label{lin:otc26}
			\State Update the \emph{preds[]} \& \emph{currs[]} of $m_{ij}$ in $\llog_i$.\label{lin:otc27}
			
			\EndFor \label{lin:otc28}
			%\EndFor
			\State Release the locks; return $\langle commit_i \rangle$.\label{lin:otc29}
			\EndProcedure \label{lin:otc30}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}


\vspace{.2mm}
\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{tryC\_Validation():} It is only use from \tryc{()} validation.}
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{145}\makeatother
			\Procedure{\emph{tryC\_Validation{()}}}{} \label{lin:otcv1}
			\If{(\emph{!rv\_Validation()})}
			Release the locks and \emph{retry}.\label{lin:otcv2}
			\EndIf\label{lin:otcv3}
			\If{(k $\in$ $M_k.\lsl$)}\label{lin:otcv4}
	%		\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the largest timestamp smaller (lts)  than $i$.\label{lin:otcv5}
	%		\If{($ver_j$ == $null$)} /*Finite Versions*/
	%		\State return $\langle abort_i\rangle$ \label{lin:otcv111}
	%		\EndIf
			\State Maintain the list of \emph{currs[].rvl} as allRVL for \blank{.7cm} all \emph{k} of $T_i$.\label{lin:otcv6}
			\State /*p is the \emph{tsimestamp} of transaction $T_p$*/
			\If{($p$ $\in$ allRVL)} /*Includes $i$ in allRVL*/\label{lin:otcv7}
			\State Lock \emph{status} of each $p$ in pre-defined order. \label{lin:otcv8}
			\EndIf\label{lin:otcv9}
			\If{(\emph{i.status == false})} return $\langle false \rangle$. \label{lin:otcv10}
			\EndIf\label{lin:otcv11}
			\ForAll{($T_p$ $\in$ allRVL)}\label{lin:otcv12}
			\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:otcv13}
			\State Maintain \emph{abort list} as abortRVL \& in- \blank{1.5cm}cludes \emph{p} in it.\label{lin:otcv14}
			\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:otcv15}
			\EndIf\label{lin:otcv16}
			
			\EndFor\label{lin:otcv17}
\cmnt{			\ForAll{($ver$ $\in$ currVL)}\label{lin:otcv18}
			\State Calculate $tltl_i$ = min($tltl_i$, $ver.vrt+1$).\label{lin:otcv19}
			\EndFor\label{lin:otcv20}
			\ForAll{($ver$ $\in$ nextVL)}\label{lin:otcv21}
			\State Calculate $tutl_i$ = min($tutl_i$, $ver.vNext$ \blank{1.1cm}$.vrt-1$).\label{lin:otcv22}
			\EndFor\label{lin:otcv23}
			\If{($tltl_i$ $>$ $tutl_i$)} /*abort $i$ itself*/
			\State return $\langle false \rangle$. \label{lin:otcv24}
			\EndIf\label{lin:otcv25}
			\ForAll{($p$ $\in$ smallRVL)}\label{lin:otcv26}
			\If{($tltl_p$ $>$ $tutl_i$)}\label{lin:otcv27}%/*Ensure limit don't cross for both $i$ and $k$*/
			\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:otcv28}
			\State Includes $p$ in abortRVL list.\label{lin:otcv29}
			\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:otcv30}
			\EndIf\label{lin:otcv31}
			\EndIf	\label{lin:otcv32}	
			\EndFor \label{lin:otcv33}
			\State $tltl_i$ = $tutl_i$. /*After this point $i$ can't abort*/\label{lin:otcv34}
			\ForAll{($p$ $\in$ smallRVL)}
			\State /*Only for \emph{live} transactions*/ \label{lin:otcv35}
			\State Calculate the $tutl_p$ = min($tutl_p$, $tltl_i-1$).\label{lin:otcv36}
			\EndFor \label{lin:otcv37}
}			
			\ForAll{($p$ $\in$ abortRVL)} \label{lin:otcv38}
			\State Set the \emph{status} of $p$ to be $false$. \label{lin:otcv39}
			\EndFor \label{lin:otcv40}
			%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
			%		\If{($j.max_{rvl}$ > $i$)}\label{lin:trycv7}
			%		\State return $false$.\label{lin:trycv8}
			%		\EndIf \label{lin:trycv9}
			%		\EndFor\label{lin:trycv10}
			\EndIf\label{lin:otcv41}
			\State return $\langle true \rangle$.\label{lin:otcv42}
			\EndProcedure \label{lin:otcv43}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}
\vspace{.2mm}

}

\vspace{.2mm}
\begin{algorithm}
	%\label{alg:llsearch} 
%	\scriptsize
	\caption{\emph{tryC\_Validation():} It is only use for \tryc{()} validation.}
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{286}\makeatother
			\Procedure{\emph{tryC\_Validation{()}}}{} \label{lin:otcv1}
			\If{(\emph{!rv\_Validation()})}
			Release the locks and \emph{retry}.\label{lin:otcv2}
			\EndIf\label{lin:otcv3}
			\If{(k $\in$ $M_k.\lsl$)}\label{lin:otcv4}
			%		\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the largest timestamp smaller (lts)  than $i$.\label{lin:otcv5}
			%		\If{($ver_j$ == $null$)} /*Finite Versions*/
			%		\State return $\langle abort_i\rangle$ \label{lin:otcv111}
			%		\EndIf
			\State Maintain the list of \emph{currs[].rvl} as allRVL for all key \emph{k} of $T_i$.\label{lin:otcv6}
			\State /*p is the \emph{timestamp} of transaction $T_p$*/
			\If{($p$ $\in$ allRVL)} /*Includes $i$ as well in allRVL*/\label{lin:otcv7}
			\State Lock \emph{status} of each $p$ in pre-defined order. \label{lin:otcv8}
			\EndIf\label{lin:otcv9}
			\If{(\emph{i.status == false})} return $\langle false \rangle$. \label{lin:otcv10}
			\EndIf\label{lin:otcv11}
			\ForAll{($p$ $\in$ allRVL)}\label{lin:otcv12}
			\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:otcv13}
			\State Maintain \emph{abort list} as abortRVL \& includes \emph{p} in it.\label{lin:otcv14}
			\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:otcv15}
			\EndIf\label{lin:otcv16}
			
			\EndFor\label{lin:otcv17}
			\cmnt{			\ForAll{($ver$ $\in$ currVL)}\label{lin:otcv18}
				\State Calculate $tltl_i$ = min($tltl_i$, $ver.vrt+1$).\label{lin:otcv19}
				\EndFor\label{lin:otcv20}
				\ForAll{($ver$ $\in$ nextVL)}\label{lin:otcv21}
				\State Calculate $tutl_i$ = min($tutl_i$, $ver.vNext$ \blank{1.1cm}$.vrt-1$).\label{lin:otcv22}
				\EndFor\label{lin:otcv23}
				\If{($tltl_i$ $>$ $tutl_i$)} /*abort $i$ itself*/
				\State return $\langle false \rangle$. \label{lin:otcv24}
				\EndIf\label{lin:otcv25}
				\ForAll{($p$ $\in$ smallRVL)}\label{lin:otcv26}
				\If{($tltl_p$ $>$ $tutl_i$)}\label{lin:otcv27}%/*Ensure limit don't cross for both $i$ and $k$*/
				\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:otcv28}
				\State Includes $p$ in abortRVL list.\label{lin:otcv29}
				\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:otcv30}
				\EndIf\label{lin:otcv31}
				\EndIf	\label{lin:otcv32}	
				\EndFor \label{lin:otcv33}
				\State $tltl_i$ = $tutl_i$. /*After this point $i$ can't abort*/\label{lin:otcv34}
				\ForAll{($p$ $\in$ smallRVL)}
				\State /*Only for \emph{live} transactions*/ \label{lin:otcv35}
				\State Calculate the $tutl_p$ = min($tutl_p$, $tltl_i-1$).\label{lin:otcv36}
				\EndFor \label{lin:otcv37}
			}			
			\ForAll{($p$ $\in$ abortRVL)} \label{lin:otcv38}
			\State Set the \emph{status} of $p$ to be $false$. \label{lin:otcv39}
			\EndFor \label{lin:otcv40}
			%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
			%		\If{($j.max_{rvl}$ > $i$)}\label{lin:trycv7}
			%		\State return $false$.\label{lin:trycv8}
			%		\EndIf \label{lin:trycv9}
			%		\EndFor\label{lin:trycv10}
			\EndIf\label{lin:otcv41}
			\State return $\langle true \rangle$.\label{lin:otcv42}
			\EndProcedure \label{lin:otcv43}
		\end{algorithmic}
%	\end{multicols}
\end{algorithm}
\vspace{.2mm}


If $m_{ij}$ is \tdel{()} and key $k$ exists in the $M_k.\lsl{}$ then it sets the \emph{rvl} as $\phi$ and \emph{mark} field as $true$ for node corresponding to the key $k$ at \Lineref{otc25}. At last, it updates the preds and currs of each $m_{ij}$ into its $txLog_i$ to help the upcoming methods of the same transactions in \emph{poValidation()} at \Lineref{otc27}. Finally, it releases the locks on all the keys in a predefined order and returns \emph{commit} at \Lineref{otc29}.
\cmnt{
\vspace{-.2cm}

\begin{theorem}
	Any history $H$ generated by SF-SVOSTM satisfies co-opacity.
\end{theorem}
\vspace{-.3cm}
\begin{theorem}
	Any history $H$ generated by SF-KOSTM satisfies  local-opacity.
\end{theorem}
\vspace{-.3cm}
\begin{theorem}
	SF-KOSTM ensures starvation-freedom in presence of a fair scheduler that satisfies \asmref{bdtm}(bounded-termination) and in the absence of parasitic transactions that satisfies \asmref{self}.
\end{theorem}
\vspace{-.2cm}
Due to lack of space, please refer the proof of above stated theorems in \apnref{ap-cc}.
}

\cmnt{
\subsection{Remaining Pseudo code of SF-KOSTM Algorithm}
\label{apn:ap-kostm}
This subsection describes the remaining pseudo code of SF-KOSTM algorithm which includes \emph{STM\_begin()}, \emph{rv\_Validation()} and \emph{tryC\_Validation()} as follows: 

\noindent
\textbf{\emph{tryC\_Validation()}:} It identifies whether the methods of invoking transaction $T_i$ are able to create or delete a version corresponding to the keys while ensuring the \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions.% First, it do the \emph{rv\_Validation()} as explained in \rvmt{()} above. If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise maintains the information of $ver_j$ and its next version ($ver_j.vNext$) which helps transaction $T_i$ to sets its $tltl_i$ and $tutl_i$. If $wts_i$ of $T_i$ is less then other $live$ transactions $wts$ exist in $ver_j.rvl$ then $T_i$ sets the $status$ to be $false$ to all other transactions otherwise $T_i$ returns to $abort$. The detailed descriptions are in \apnref{ap-rcode}.

%It maintains the Current Version List (currVL), Next Version List (nextVL), All Return Value List (allRVL), Large Return Value List (largeRVL), Small Return Value List (smallRVL) from $ver_j$ of key $k$. currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. These terms helps to decide, whether  $T_i$ will create the version and commit while aborting the conflicting transactions or $T_i$ returns abort. 





First, it do the \emph{rv\_Validation()} at \Lineref{tcv2} as explained in \rvmt{()}. If \emph{rv\_Validation()} is successful and key $k$ exists in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$ at \Lineref{tcv5}. If $ver_j$ is $null$ at \Lineref{tcv111} then SF-KOSTM returns $abort$ for transaction $T_i$ because it does not find the version to replace otherwise after identifying the current version $ver_j$ it maintains the Current Version List (currVL), Next Version List (nextVL), All Return Value List (allRVL), Large Return Value List (largeRVL), Small Return Value List (smallRVL) from $ver_j$ of key $k$ at \Lineref{tcv6}. currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. Acquire the locks on \emph{status} of all the transactions present in allRVL list including $T_i$ it self in predefined order to avoid the deadlock at \Lineref{tcv8}. First, it checks the \emph{status} of its own transaction $T_i$ at \Lineref{tcv10}. If \emph{status} of $T_i$ is \emph{false} then $T_i$ has to \emph{abort} the same reason as explained in \rvmt{()}. 


\begin{algorithm}[H] 
%	\scriptsize
	\caption{\emph{STM\_begin($its$)}: This method is invoke by a thread $Th_i$ to start a new transaction $T_i$. It pass a parameter $its$ which is the initial timestamp of the first incarnation of $T_i$. If $T_i$ is the first incarnation then $its$ is $nil$.}
		\label{algo:begin1} 
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{168}\makeatother
			\Procedure{\emph{STM\_begin($its$)}}{} 
			\State Create a local log $txLog_i$ for each transaction.
			\If {($its == nil$)}
			\State /* Atomically get the value from the global counter and set it to its, cts, and \blank{1cm} wts.*/
			\State $its_i$ = $cts_i$ = $wts_i$ = \emph{gcounter.get\&Inc()};
			\Else 
			\State /*Set the $its_i$ to first incarnation of $T_i$ $its$*/
			\State $its_i$ = $its$;
			\State /*Atomically get the value from the global counter for $cts_i$*/
			\State $cts_i$ = \emph{gcounter.get\&Inc()}.
			%		\State \txll.$L\_t\_id$ $\gets$ $\gcts_i \gets \gtcnt.get\&Inc()$; 
			\State /*Set the $wts$ value with the help of $cts_i$ and $its_i$*/
			\State $wts_i$ = $cts_i$+C*($cts_i$-$its_i$).
			\EndIf
			\State /*Set the $tltl_i$ as $cts_i$*/
			\State $tltl$ = $cts_i$.  
			\State /*Set the $tutl_i$ as possible large value*/
			\State $tutl_i$ = $\infty$.
			\State /*Initially, set the $status_i$ of $T_i$ as $live$*/
			\State $status_i$ = $live$; 
			\State return $\langle cts_i, wts_i\rangle$
			
			\EndProcedure
		\end{algorithmic}
%	\end{multicols}
\end{algorithm}

\cmnt{

\begin{algorithm} 
	\label{alg:begin1} 
	\scriptsize
	\caption{STM\_begin($its$): This method is invoke by a thread to start a new transaction $T_i$. It pass a parameter $its$ which is the initial timestamp of the first incarnation of $T_i$. If this is the first incarnation then $its$ is $nil$.}
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{168}\makeatother
		\Procedure{STM begin($its$)}{} 
		\State Creating a local log $txLog_i$ for each transaction.
		\If {($its == nil$)}
		\State /* Atomically get the value from the global \blank{.7cm} counter and set it to its, cts, and wts.*/
		\State $its_i$ = $cts_i$ = $wts_i$ = \emph{gcounter.get\&Inc()};
		\Else 
		\State /*Set the $its_i$ to first incarnation of $T_i$ $its$*/
		\State $its_i$ = its;
		\State /*Atomically get the value from the global \blank{.7cm} counter for $cts_i$*/
		\State $cts_i$ = \emph{gcounter.get\&Inc()}.
		%		\State \txll.$L\_t\_id$ $\gets$ $\gcts_i \gets \gtcnt.get\&Inc()$; 
		\State /*Set the $wts$ value with the help of $cts_i$ and \blank{.7cm} $its_i$*/
		\State $wts_i$ = $cts_i$+C*($cts_i$-$its_i$).
		\EndIf
		\State /*Set the $tltl_i$ as $cts_i$*/
		\State $tltl$ = $cts_i$.  
		\State /*Set the $tutl_i$ as possible large value*/
		\State $tutl_i$ = $\infty$.
		\State /*Initially, set the $status_i$ of $T_i$ as $live$*/
		\State $state_i$ = $live$; 
		\State return $\langle cts_i, wts_i\rangle$
		
		\EndProcedure
	\end{algorithmic}
	\end{multicols}
\end{algorithm}


\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{rv\_Validation(preds[], currs[])}: It is mainly used for \emph{rv\_method()} validation.}
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{189}\makeatother
		\Procedure{$rv\_Validation{(preds[], currs[])}$}{} \label{lin:rvv1}
		\If{$((\bp.mark) || (\bc.mark) || (\bp.\bn)\neq \blank{.15cm} \bc || (\rp.\rn) \neq {\rc})$}\label{lin:rvv2}
		return $\langle false \rangle$. 
		\Else{} return $\langle true \rangle$. \label{lin:rvv3}
		\EndIf \label{lin:rvv4}
		\EndProcedure \label{lin:rvv5}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
}

\begin{algorithm}[H]
	%\label{alg:llsearch} 
%	\scriptsize
	\caption{\emph{rv\_Validation(preds[], currs[])}: It is mainly used for \emph{rv\_method()} validation.}
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{189}\makeatother
		\Procedure{$rv\_Validation{(preds[], currs[])}$}{} \label{lin:rvv1}
		\If{$((\bp.mark) || (\bc.mark) || ((\bp.\bn)\neq \blank{1.7cm} \bc) || ((\rp.\rn) \neq {\rc})$)}\label{lin:rvv2}
		return $\langle false \rangle$. 
		\Else{} return $\langle true \rangle$. \label{lin:rvv3}
		\EndIf \label{lin:rvv4}
		\EndProcedure \label{lin:rvv5}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}

\vspace{.2mm}




If the \emph{status} of $T_i$ is not \emph{false} then it compares the $its_i$ of its own transaction $T_i$ with the $its_p$ of other transactions $T_p$ present in the largeRVL at \Lineref{tcv13}. Along with this it checks the \emph{status} of $p$. If above conditions $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ succeed then it includes $T_p$ in the Abort Return Value List (abortRVL) at \Lineref{tcv14} to abort it later otherwise abort $T_i$ itself at \Lineref{tcv15}.  

\vspace{.2mm}
\begin{algorithm}
	%\label{alg:llsearch} 
	%	\scriptsize
	\caption{\emph{tryC\_Validation():} It is use for \tryc{()} validation.}
		\label{algo:trycVal} 
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{194}\makeatother
		\Procedure{\emph{tryC\_Validation{()}}}{} \label{lin:tcv1}
		\If{(\emph{!rv\_Validation()})}
		Release the locks and \emph{retry}.\label{lin:tcv2}
		\EndIf\label{lin:tcv3}
		\If{(k $\in$ $M_k.\lsl$)}\label{lin:tcv4}
		\State Identify the version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp \blank{1cm} smaller (lts)} than $i$ and there exists no other version with timestamp $p$ by $T_p$ \blank{1cm} on key $k$ such that $\langle \emph{j $<$ p $<$ i}\rangle$.\label{lin:tcv5}
		\If{($ver_j$ == $null$)} /*Finite Versions*/
		\State return $\langle abort_i\rangle$ \label{lin:tcv111}
		\EndIf
		\State Maintain the list of $ver_j$, $ver_j.vNext$, $ver_j.rvl$, $(ver_j.rvl>i)$, and \blank{1cm} $(ver_j.rvl<i)$ as prevVL, nextVL, allRVL, largeRVL and smallRVL \blank{1cm} respectively for all key \emph{k} of $T_i$.\label{lin:tcv6}
		\State /*$p$ is the timestamp of transaction $T_p$*/
		\If{($p$ $\in$ allRVL)} /*Includes $i$ as well in allRVL*/\label{lin:tcv7}
		\State Lock \emph{status} of each $p$ in pre-defined order. \label{lin:tcv8}
		\EndIf\label{lin:tcv9}
		\If{(\emph{i.status == false})} return $\langle false \rangle$. \label{lin:tcv10}
		\EndIf\label{lin:tcv11}
		\ForAll{($p$ $\in$ largeRVL)}\label{lin:tcv12}
		\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv13}
		\State Maintain \emph{abort list} as abortRVL \& includes \emph{p} in it.\label{lin:tcv14}
		\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv15}
		\EndIf\label{lin:tcv16}
		
		\EndFor\label{lin:tcv17}
		\ForAll{($ver$ $\in$ nextVL)}\label{lin:tcv21}
		\State Calculate $tutl_i$ = min($tutl_i$, $ver.vNext$$.vrt-1$).\label{lin:tcv22}
		\EndFor\label{lin:tcv23}
		\ForAll{($ver$ $\in$ currVL)}\label{lin:tcv18}
		\State Calculate $tltl_i$ = max($tltl_i$, $ver.vrt+1$).\label{lin:tcv19}
		\EndFor\label{lin:tcv20}
		\If{($tltl_i$ $>$ $tutl_i$)} /*abort $i$ itself*/
		\State return $\langle false \rangle$. \label{lin:tcv24}
		\EndIf\label{lin:tcv25}
		\ForAll{($p$ $\in$ smallRVL)}\label{lin:tcv26}
		\If{($tltl_p$ $>$ $tutl_i$)}\label{lin:tcv27}%/*Ensure limit don't cross for both $i$ and $k$*/
		\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv28}
		\State Includes $p$ in abortRVL list.\label{lin:tcv29}
		\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv30}
		\EndIf\label{lin:tcv31}
		\EndIf	\label{lin:tcv32}	
		\EndFor \label{lin:tcv33}
		\State $tltl_i$ = $tutl_i$. /*After this point $i$ can't abort*/\label{lin:tcv34}
		\ForAll{($p$ $\in$ smallRVL)}
		\State /*Only for \emph{live} transactions*/ \label{lin:tcv35}
		\State Calculate the $tutl_p$ = min($tutl_p$, $tltl_i-1$).\label{lin:tcv36}
		\EndFor \label{lin:tcv37}
		\ForAll{($p$ $\in$ abortRVL)} \label{lin:tcv38}
		\State Set the \emph{status} of $p$ to be $false$. \label{lin:tcv39}
		\EndFor \label{lin:tcv40}
		%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
		%		\If{($j.max_{rvl}$ > $i$)}\label{lin:trycv7}
		%		\State return $false$.\label{lin:trycv8}
		%		\EndIf \label{lin:trycv9}
		%		\EndFor\label{lin:trycv10}
		\EndIf\label{lin:tcv41}
		\State return $\langle true \rangle$.\label{lin:tcv42}
		\EndProcedure \label{lin:tcv43}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
\vspace{.2mm}

After that \tryc{()} maintains the $tltl_i$ and $tutl_i$ of transaction $T_i$ at \Lineref{tcv19} and \Lineref{tcv22}. The requirement of $tltl_i$ and $tutl_i$ is explained above in the \rvmt{()}. If limit of $tltl_i$ crossed with $tutl_i$ then $T_i$ have to abort at \Lineref{tcv24}. If $tltl_p$ greater than $tutl_i$ at \Lineref{tcv27} then it checks the $its_i$ and $its_p$. If $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ then add the transaction $T_p$ in the abortRVL for all the smallRVL transactions at \Lineref{tcv29} otherwise, \emph{abort} $T_i$ itself at \Lineref{tcv30}.

At \Lineref{tcv34}, $tltl_i$ would be equal to $tutl_i$ and after this step transaction $T_i$ will never \emph{abort}. $T_i$ helps the other transaction $T_p$ to update the $tutl_p$ which exists in the smallRVL and still $live$ then it sets the $tutl_p$ to minimum of $\langle tutl_p \vee tltl_i-1\rangle$ to maintain the real-time order among the transaction at \Lineref{tcv36}. At \Lineref{tcv39}, \tryc{()} aborts all other conflicting transactions which are present in the abortRVL while modifying the \emph{status} field to be \emph{false} to achieve \emph{starvation-freedom}.

}
\subsection{Importance of Timestamp Ranges in SF-KOSTM}
\label{apn:wtsdis}

\textbf{Violation of Real-Time Order by wts:} As described in \subsecref{working}, $cts$ respects the real-time order among the transactions but SF-KOSTM uses $wts$ which may not respect real-time order. Sometimes, the value of $wts$ is significantly larger than $cts$ which leads to violate the real-time order among the transactions. \figref{sfmv-correct} illustrates it with history $H$: $l_1(ht,k_1,v_0) l_2(ht,k_2,v_0) i_1(ht,k_1,v_{10}) C_1 i_2(ht,k_1, v_{20}) C_2 l_3(ht,k_1,v_{10}) i_3(ht,k_3,v_{25})\\ C_3$ consists of three transactions $T_1, T_2, T_3$ with $cts$ as 100, 110, 130 and $wts$ as 100, 150, 130 respectively. $T_1$ and $T_2$ has been committed before the beginning of $T_3$, so $T_1$ and $T_2$ are in real-time order with $T_3$. Formally, $T_1 \prec_{H}^{RT} T_3$ and $T_2 \prec_{H}^{RT} T_3$. But, $T_2$ has higher $wts$ than $T_3$. Now, $T_3$ lookups key $k_1$ from $T_1$ and returns the value as $v_{10}$  because $T_1$ is the available largest $wts$ (100) smaller than $T_3$ $wts$ (130). The only possible equivalent serial order $S$ to history $H$ is $T_1 T_3 T_2$ which is \legal as well. But $S$ violates real-time order because $T_3$ is serialized before $T_2$ in $S$ but $T_2$ has been committed before the beginning of $T_3$ in $H$. It can  easily be seen that, such history $H$ can be accepted by the algorithm when it uses only $wts$ instead of $cts$. But this should not happen because its violating the real-time order which says it does not satisfy the correctness criteria as \emph{local opacity}. 

A simple solution to this issue is by delaying the committing transaction say $T_i$ with $wts_i$ until the real-time catches up to the $wts_i$. Delaying such $T_i$ will ensure the correctness criteria as \emph{local opacity} while making the $wts$ of the transaction same as real-time. But, this is highly unacceptable. It seems like transaction $T_i$ acquires the locks on all the keys it wants to update and wait. It will show the adverse effect and reduces the performance of SF-KOSTM system.

\noindent
\textbf{Regaining the Real-Time Order using Timestamp Ranges along with wts:} We require that all the transactions of history $H$ generated by SF-KOSTM are serialized based on their $wts$ while respecting the real-time order among them. Another efficient solution is to allow the transaction $T_i$ with $wts_i$ to catch up with the actual time if $T_i$ does not violates the real-time order. So, to respect the real-time order among the transactions SF-KOSTM uses the time constraints. SF-KOSTM uses the idea of timestamp ranges \cite{Riegel+:LSA:DISC:2006,Guer+:disc1:2008, Crain+:RI_VWC:ICA3PP:2011} along with $\langle its_i, cts_i, wts_i \rangle$ for transaction $T_i$ in \tbeg{()}. It maintains the \emph{transaction lower timestamp limit ($tltl_i$)} and \emph{transaction upper timestamp limit ($tutl_i$)} for $T_i$. Initially, $\langle its_i, cts_i, wts_i, tltl_i \rangle$ are the same for $T_i$. $tutl_i$ would be set as a largest possible value denoted as $+\infty$ for $T_i$. After successful execution of \emph{\rvmt{s()}} or \tryc{()} of $T_i$, $tltl_i$ gets incremented and $tutl_i$ gets decremented to respect the real-time order among the transactions as explained in \subsecref{working}. 

\begin{figure}
	\centerline{
		\scalebox{0.48}{\input{figs/wtsDis.pdf_t}}}
	\captionsetup{justification=centering}
	\caption{Violating the \emph{real-time order} by \emph{wts}}
	\label{fig:sfmv-correct}
\end{figure}


For better understanding consider \figref{tltltutl}, which shows the regaining the \emph{real-time order} using timestamp ranges ($tltl$ and $tutl$) along with \emph{wts} on history $H$. Initially, $T_1$ begins with $cts_1$ = $wts_1$ = $tltl_1$ = 100, $tutl_1$ = $\infty$ and $T_1$ returns commit. We assume at the time of commit of $T_1$, $gcounter$ is 120. So, $tutl_1$ reduces to 120. After that $T_2$ commits and with suppose $tutl_2$ reduces to 121 (so, the current value $gcounter$ is 121). $T_1$ and $T_2$ both access the key $k_1$ and $T_2$ is updating $k_1$. So, $T_1$ and $T_2$ are conflicting. Hence, $tltl_2$ is incremented to a value greater than $tutl_1$, say 121. Now, when $T_3$ begins , it assigns 
$cts_3$ = $wts_3$ = $tltl_3$ = 130, and $tutl_3$ = $\infty$. At the time of $l_3(ht,k_1,v_{10})$, as $T_3$ lookups the version of $k_1$ from $T_1$, so, $T_3$ reduces its $tutl_3$ less than $tltl_2$ (currently, $tltl_2$ is 121). Hence, $tutl_3$ becomes say 120. But, $tltl_3$ is already 130. So, $tltl_3$ has crossed the limit of $tutl_3$ which is causing $T_3$ to abort. Intuitively, this implies that $wts_3$ and real-time order are out of synchrony and can not be reconciled. Hence, by using the timestamp ranges $H$ executes correctly by SF-KOSTM algorithm with equivalent serial schedule $T_1 T_2$. 


%We illustrate this technique with the history $H1$ shown in \figref{sfmv-correct}. When $T_1$ starts its $\tcts{1} = 50, \ttltl{1} = 50, \ttutl{1}=\infty$. Now when $T_1$ commits, suppose $\gtcnt$ is 70. Hence, $\ttutl{1}$ reduces to 70. Next, when $T_2$ commits, suppose $\ttutl{2}$ reduces to 75 (the current value of $\gtcnt$). As $T_1, T_2$ have accessed a common \tobj $x$ in a conflicting manner, $\ttltl{2}$ is incremented to a value greater than $\ttutl{1}$, say 71. Next, when $T_3$ begins, $\ttltl{3}$ is assigned $\tcts{3}$ which is 80 and $\ttutl{3}$ is initialized to $\infty$. When $T_3$ reads 10 from $T_1$, which is $r_3(x, 10)$, $\ttutl{3}$ is reduced to a value less than $\ttltl{2} (= 71)$, say 70. But $\ttltl{3}$ is already at 80. Hence, the limits of $T_3$ have crossed and thus causing $T_3$ to abort. The resulting history consisting of only committed transactions $T_1 T_2$ is \stsble. 

\cmnt{
\begin{figure}
	\centerline{
		\scalebox{0.5}{\input{figs/WTSdraw.pdf_t}}}
	\captionsetup{justification=centering}
	\caption{\emph{wts} violating \emph{real-time order}}
	\label{fig:sfmv-correct}
\end{figure}
}


\begin{figure}
	\centerline{
		\scalebox{0.43}{\input{figs/tltltutl.pdf_t}}}
	\captionsetup{justification=centering}
	\caption{Regaining the \emph{real-time order} using Timestamp Ranges along with \emph{wts}}
	\label{fig:tltltutl}
\end{figure}





\cmnt{


\vspace{.2mm}
\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{tryC\_Validation():} It is only use from \tryc{()} validation.}
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{194}\makeatother
			\Procedure{\emph{tryC\_Validation{()}}}{} \label{lin:tcv1}
			\If{(\emph{!rv\_Validation()})}
			Release the locks and \emph{retry}.\label{lin:tcv2}
			\EndIf\label{lin:tcv3}
			\If{(k $\in$ $M_k.\lsl$)}\label{lin:tcv4}
			\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the \emph{largest timestamp smaller (lts)} than $i$.\label{lin:tcv5}
			\If{($ver_j$ == $null$)} /*Finite Versions*/
			\State return $\langle abort_i\rangle$ \label{lin:tcv111}
			\EndIf
			\State Maintain the list of $ver_j$, $ver_j.vNext$, \blank{.7cm} $ver_j.rvl$, $(ver_j.rvl>i)$, and $(ver_j.rvl<\blank{.7cm}i)$ as prevVL, nextVL, allRVL, largeRVL, small- \blank{.7cm}RVL respectively for all key \emph{k} of $T_i$.\label{lin:tcv6}
			\If{($p$ $\in$ allRVL)} /*Includes $i$ in allRVL*/\label{lin:tcv7}
			\State Lock \emph{status} of each $p$ in pre-defined order. \label{lin:tcv8}
			\EndIf\label{lin:tcv9}
			\If{(\emph{i.status == false})} return $\langle false \rangle$. \label{lin:tcv10}
			\EndIf\label{lin:tcv11}
			\ForAll{($p$ $\in$ largeRVL)}\label{lin:tcv12}
			\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv13}
			\State Maintain \emph{abort list} as abortRVL \& in- \blank{1.5cm}cludes \emph{p} in it.\label{lin:tcv14}
			\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv15}
			\EndIf\label{lin:tcv16}
			
			\EndFor\label{lin:tcv17}
			\ForAll{($ver$ $\in$ currVL)}\label{lin:tcv18}
			\State Calculate $tltl_i$ = max($tltl_i$, $ver.vrt+1$).\label{lin:tcv19}
			\EndFor\label{lin:tcv20}
			\ForAll{($ver$ $\in$ nextVL)}\label{lin:tcv21}
			\State Calculate $tutl_i$ = min($tutl_i$, $ver.vNext$ \blank{1.1cm}$.vrt-1$).\label{lin:tcv22}
			\EndFor\label{lin:tcv23}
			\If{($tltl_i$ $>$ $tutl_i$)} /*abort $i$ itself*/
			\State return $\langle false \rangle$. \label{lin:tcv24}
			\EndIf\label{lin:tcv25}
			\ForAll{($p$ $\in$ smallRVL)}\label{lin:tcv26}
			\If{($tltl_p$ $>$ $tutl_i$)}\label{lin:tcv27}%/*Ensure limit don't cross for both $i$ and $k$*/
			\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv28}
			\State Includes $p$ in abortRVL list.\label{lin:tcv29}
			\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv30}
			\EndIf\label{lin:tcv31}
			\EndIf	\label{lin:tcv32}	
			\EndFor \label{lin:tcv33}
			\State $tltl_i$ = $tutl_i$. /*After this point $i$ can't abort*/\label{lin:tcv34}
			\ForAll{($p$ $\in$ smallRVL)}
			\State /*Only for \emph{live} transactions*/ \label{lin:tcv35}
			\State Calculate the $tutl_p$ = min($tutl_p$, $tltl_i-1$).\label{lin:tcv36}
			\EndFor \label{lin:tcv37}
			\ForAll{($p$ $\in$ abortRVL)} \label{lin:tcv38}
			\State Set the \emph{status} of $p$ to be $false$. \label{lin:tcv39}
			\EndFor \label{lin:tcv40}
			%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
			%		\If{($j.max_{rvl}$ > $i$)}\label{lin:trycv7}
			%		\State return $false$.\label{lin:trycv8}
			%		\EndIf \label{lin:trycv9}
			%		\EndFor\label{lin:trycv10}
			\EndIf\label{lin:tcv41}
			\State return $\langle true \rangle$.\label{lin:tcv42}
			\EndProcedure \label{lin:tcv43}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}
\vspace{.2mm}


}



==> Arxiv SFKOSTM SSS19/ap-result.tex <==
\section{Remaining Experimental Evaluation}
\label{apn:ap-result}
This section explains the additional results and analysis that boost the potential of our work experimentally. %Along with this, it describes a few low-level implementation details of proposed algorithms and our flexible counter application.

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/htli-us.pdf}
	\caption{ Performance analysis among SF-SVOSTM and variants of SF-KOSTM on hash table}
	\label{fig:htus}
\end{figure}

\noindent
We started our experiments with hash table data structure of bucket size 5 as shown in \figref{htus}. First, we compared \emph{max-time} taken by all our proposed HT-SF-SVOSTM and variations of HT-SF-KOSTM (HT-SF-MVOSTM, HT-SF-MVOSTM-GC, and HT-SF-KOSTM) while varying the number of threads from 50 to 250. We did these experiments on \emph{high contention environment} which includes only 30 keys, number of threads ranging from 50 to 250, each thread spawns upon a transaction, where each transaction performs 10 operations (insert, delete and lookup) depending upon the workload chosen. We analyze through \figref{htus} that the finite version HT-SF-KOSTM performs best among all the proposed algorithms on all the three types of workloads (W1, W2, and W3 defined in \secref{exp}) with value of $K$ and C as 5 and 0.1 respectively. Here, $K$ is the number of versions in the version list and C is the variable used to derive the $wts$. Similarly, we consider another data structure as linked-list on \emph{high contention environment} and compared \emph{max-time} taken by all our proposed list-SF-SVOSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC, and list-SF-KOSTM algorithms. \figref{listus} represents that list-SF-KOSTM performs best for all the workloads (W1, W2, and W3) with value of $K$ and C as 5 and 0.1 respectively. 

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-us.pdf}
	\caption{ Performance analysis among SF-SVOSTM and variants of SF-KOSTM on list}
	\label{fig:listus}
\end{figure}
\cmnt{

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/htCK.pdf}
	\caption{ Optimal value of K and C along with Stability for hash table}
	\label{fig:htck}
\end{figure}

\noindent
\textbf{Best value of $K$, $C$, and Stability in SF-KOSTM:} We identified the  best value of $K$ for both HT-SF-KOSTM and list-SF-KOSTM algorithms. \figref{htck}.(a). demonstrates the best value of $K$ as 5 for HT-SF-KOSTM on counter application. We achieve this while varying value of $K$ on \emph{high contention environment} with 64 threads on all the workloads $W1, W2, W3$. \figref{htck}.(b). illustrates the best value of $C$ as 0.1 for HT-SF-KOSTM on all the workloads $W1, W2, W3$. \figref{htck}.(c). represents the $stability$ of HT-SF-KOSTM algorithm overtime for the counter application. For this experiment, we fixed 32 threads, 1000 shared data-items (or keys), the value of $K$ as 5, and $C$ as 0.1. Along with this, we consider, 5 seconds warm-up period on all the workloads $W1, W2, W3$. Each thread invokes transactions until its time-bound of 60 seconds expires.
We calculate the number of transactions committed in the incremental interval of 5 seconds. \figref{htck}.(c). shows that over time HT-SF-KOSTM is stable which helps to hold the claim that the performance of HT-SF-KOSTM will continue in the same manner if time is increased to higher orders. Similarly, we perform the same experiments for the linked-list data structure as well. \figref{listck}.(a). and \figref{listck}.(b). demonstrate the best value of $K$ as 5 and $C$ as 0.1 for list-SF-KOSTM on all the workloads $W1, W2, W3$. Similarly, \figref{listck}.(c). illustrates the $stability$ of list-SF-KOSTM and shows that it is stable over time on all the workloads $W1, W2, W3$.

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/listCK.pdf}
	\caption{ Optimal value of K and C along with Stability for list}
	\label{fig:listck}
\end{figure}
%Similarly, we calculate the best value of $K$ as 5 for \pkto on the same parameters. $C$, is a constant that is used to calculate $WTS$ of a transaction. i.e., $\twts{i} = \tcts{i} + C * (\tcts{i} - \tits{i});$ where, $C$ is any constant greater than 0. We run or experiments across load $W1$, for 64 threads and other parameters are same as defined in the methodology of \secref{exp}, we achieve the best value of $C$ as 0.1 for counter application. Experimental results are shown in \figref{optimalC} (b).
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-time-us.pdf}
	\caption{Time comparison among SF-SVOSTM and variants of SF-KOSTM on hash table}
	\label{fig:httimeus}
\end{figure}


We have done some experiments on \textit{low contention environment} which involves 1000 keys, threads varying from 2 to 64 in power of 2, each thread spawns one transaction and each transaction executes 10 operations (insert, delete and lookup) depending upon the workload chosen. We observed that HT-SF-KOSTM performs best out of all the proposed algorithms on $W1$ and $W2$ workload as shown in \figref{httimeus}. For a lesser number of threads on $W3$, HT-SF-KOSTM was taking a bit more time than other proposed algorithms as shown in \figref{httimeus}.(c). This may be because of the finite version, finding and replacing the oldest version is taking time. After that, we consider  HT-SF-KOSTM and compared against state-of-the-art STMs.  \figref{httimecomp} shows that our proposed algorithm performs better than all other state-of-art-STMs algorithms but slightly lesser than the non starvation-free HT-KOSTM. But to provide the guarantee of starvation-freedom this slight slag of time is worth paying. For the better clarification of speedups, please refer to \tabref{htspeed}.  Similarly, \figref{listtimeus} represents the analysis of \emph{low contention environment} for list data structure where list-SF-KOSTM performs best out of all the proposed algorithms. \figref{listtimecomp} demonstrates the comparison of proposed list-SF-KOSTM with list based state-of-the-art STMs and shows the significant performance gain in terms of a speedup as presented in \tabref{listspeed}. For low contention environment, starvation-freedom is appearing as an overhead so, both HT-SF-KOSTM and list-SF-KOSTM  achieve a bit less speedup than HT-KOSTM and list-KOSTM. But for high contention environment, starvation-free algorithms are always better so, both HT-SF-KOSTM and list-SF-KOSTM achieve better speedup than HT-KOSTM and list-KOSTM as explained in \secref{exp}.

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-time-comp.pdf}
	\caption{Time comparison of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:httimecomp}
\end{figure}


\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-time-us.pdf}
	\caption{Time comparison among SF-SVOSTM and variants of SF-KOSTM on list}
	\label{fig:listtimeus}
\end{figure}
%\vspace{1cm}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-time-comp.pdf}
	\caption{Time comparison of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listtimecomp}
\end{figure}

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-abort-us.pdf}
	\caption{Abort Count of SF-SVOSTM and variants of SF-KOSTM on hash table}
	\label{fig:htabortus}
\end{figure}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-abort-us.pdf}
	\caption{Abort Count of SF-SVOSTM and variants of SF-KOSTM on list}
	\label{fig:listabortus}
\end{figure}


\noindent
\textbf{Abort Count:} We analyzed the number of aborts on low contention environment as defined above. \figref{htabortus} and \figref{listabortus} show the number of aborts comparison among all the proposed variants in all three workloads W1, W2 and W3 for both data structures hash table and linked-list. The results show that HT-SF-KOSTM and list-SF-KOSTM have relatively less  number of aborts than other proposed algorithms. Similarly, \figref{htabortcomp} and \figref{listabortcomp} shows the number of aborts comparison among proposed HT-SF-KOSTM with hash table based state-of-the-art STMs and proposed list-SF-KOSTM with list based state-of-the-art STMs in all three workloads W1, W2, and W3. The result shows that the least number of aborts are happening with HT-SF-KOSTM and list-SF-KOSTM.
\noindent



%\vspace{1cm}

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-abort-comp.pdf}
	\caption{Abort Count of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:htabortcomp}
\end{figure}

%\vspace{1cm}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-abort-comp.pdf}
	 \caption{Abort Count of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listabortcomp}
\end{figure}


\noindent
\textbf{Garbage Collection:} To delete the unwanted versions, we use garbage collection mechanism in SF-MVOSTM and proposed SF-MVOSTM-GC. The results show that SF-MVOSTM-GC performs better than SF-MVOSTM. Garbage collection method deletes the unwanted version corresponding to the key. In garbage collection we use a \textit{livelist}, this livelist contains all the transaction that are live, which means every transaction on the start of its first incarnation logs its time in livelist and when commit/abort remove its entry from livelist in sorted order of transactions on the basis of $wts$. Garbage collection is achieved by deleting the version which is not latest, whose timestamp is smaller than the $wts$ of smallest live transaction. \figref{mc} represents the \textbf{\emph{Memory Consumption}} by SF-MVOSTM-GC and SF-KOSTM algorithms for \emph{high contention (or HC)} and \emph{low contention (or LC)} environment on workload $W_3$ for the linked-list data structure. Here, each algorithm creates a version corresponding to the key after successful \emph{STM\_tryC()}. We calculate the memory consumption based on the \emph{Version Count (or VC)}. If version is created then VC is incremented by 1 and after garbage collection, VC is decremented by 1. \figref{mc}. (a). demonstrates that memory consumption is kept on increasing in SF-MVOSTM-GC but memory consumption by SF-KOSTM is constant because of maintaining finite versions corresponding to the less number of keys (high contention). \figref{mc}. (b). shows for \emph{low contention} environment where memory consumption are keeps on increasing in SF-MVOSTM-GC as well as SF-KOSTM. But once limit of $K$-version reach corresponding to all the keys in SF-KOSTM, memory consumption will be stable. Similar observation can be found for other workloads $W_1, W_2$ and other data structure hash table as well.

\begin{figure}[H]
	\centering
	\includegraphics[width=10cm, height=5cm]{figs/mc.pdf}
\vspace{-.4cm}	\caption{Comparison of Memory Consumption in SF-KOSTM and SF-MVOSTM-GC}
	\label{fig:mc}
\end{figure}


\begin{table}[H]
	\small
	\begin{tabular}{ | m{4.5cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} | } 
		\hline
		Algorithm & W1 & W2 & W3 \\ 
		\hline
		HT-SF-SVOSTM & 1.49 & 1.13 & 1.09 \\
		\hline
		HT-SF-MVOSTM & 1.22 & 1.08 & 1.04 \\
		\hline
		HT-SF-MVOSTM-GC	& 1.13 & 1.03 & 1.02 \\
		\hline
		HT-SVOSTM & 3.3 & 0.77 & 1.57 \\
		\hline
		ESTM & 2.92 & 1.4 & 3.03 \\
		\hline
		RWSTM & 3.13 & 2.65 & 13.36  \\
		\hline
		HT-MVTO & 2.37 & 4.74 & 49.39  \\
		\hline
		HT-KOSTM & 0.91 & 0.7 & 0.8 \\
		\hline
		
		\hline
	
	\end{tabular}
	\captionsetup{justification=centering}
	\caption{Speedup by HT-SF-KOSTM  }
	\label{tab:htspeed}
\end{table}


\begin{table}[H]
	\small
	\begin{tabular}{ | m{4.5cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} | } 
		\hline
		Algorithm & W1 & W2 & W3 \\ 
		\hline
		list-SF-SVOSTM & 1.29 & 1.26 & 1.22 \\
		\hline
		list-SF-MVOSTM & 1.25 & 1.29 & 1.12 \\
		\hline
		list-SF-MVOSTM-GC	& 1.14 & 1.5 & 1.13 \\
		\hline
		list-SVOSTM & 2.4 & 1.5 & 1.4 \\
		\hline
		Trans-list & 24.15 & 19.06 & 23.26 \\
		\hline
		Boosting-list & 22.43 & 22.52 & 27.2  \\
		\hline
		NOrec-list & 26.12 & 27.33 & 31.05  \\
		\hline
		list-MVTO & 10.8 & 23.1 & 19.57  \\
		\hline
		list-KSFTM & 5.7 & 18.4 &  74.20 \\
		\hline
		list-KOSTM	 & 0.96 & 0.98 & 0.8 \\
		\hline
		
		\hline
	
	\end{tabular}
	\captionsetup{justification=centering}
	\caption{Speedup by list-SF-KOSTM  }
	\label{tab:listspeed}
\end{table}
%\vspace{-1cm}

}

==> Arxiv SFKOSTM SSS19/citations <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Sathya Peri",
%%%     date            = "17 Spet 2009",
%%%     filename        = "citations.bib",
%%%     url             = ""
%%%     www-home        = "http://www.cs.mun.ca/~sathya/",
%%%     address         = "Department of Computer Science,
%%%                        MUN,
%%%                        St John's, CA A1B 3X5,
%%%                        Canada",
%%%     email           = "sathya at mun.ca",
%%%     dates           = {1950--},
%%%     keywords        = "",
%%%     supported       = "yes",
%%%     supported-by    = "Sathya Peri",
%%%     abstract        = "Bibliography for Sathya Peri"
%%%  }
%%% ====================================================================


@String{PROC = {Proceedings of the}}
@String{AMS = {American Mathematical Society}}
@String{AW = {Addison-Wesley}}
@String{TCS = {Theoretical Computer Science}}
@String{JPDC = {Journal of Parallel and Distributed Computing (JPDC)}}
@String{WDAG = {Workshop on Distributed Algorithms (WDAG)}}
@String{WPDD = {ACM/ONR Workshop on Parallel and Distributed Debugging}}
@String{DC = {Distributed Computing (DC)}}
@String{TrCS = {ACM Transactions on Computer Systems}}
@String{SPDP = {IEEE Symposium on Parallel and Distributed Processing (SPDP)}}
@String{ICPP = {International Conference on Parallel Processing}}
@String{Com = {IEEE Computer}}
@String{KAP = {Kluwer Academic Publishers}}
@String{WAD = {International Workshop on Automated Debugging (AADEBUG)}}
@String{CSS = {International Conference on System Sciences}}
@String{Fre = {W. H. Freeman and Company, New York}}
@String{TPDS = {IEEE Transactions on Parallel and Distributed Systems (TPDS)}}
@String{FTCS = {IEEE Fault-Tolerant Computing Symposium (FTCS)}}
@String{JCC = {Journal of Computer Communications}}
@String{WSCT = {International Workshop on Structures in Concurrency Theory (STRICT)}}
@String{MH = {McGraw-Hill}}
@String{CACM = {Communications of the ACM (CACM)}}
@String{ICDCS = {IEEE International Conference on Distributed Computing Systems (ICDCS)}}
@String{PODC = {ACM Symposium on Principles of Distributed Computing (PODC)}}
@String{JS = {Journal of Supercomputing}}
@String{CAV = {International Conference on Computer-Aided Verification (CAV)}}
@String{LNCS = {Lecture Notes in Computer Science (LNCS)}}
@String{WPDS = {Workshop on Parallel and Distributed Simulation}}
@String{DISC = {Symposium on Distributed Computing (DISC)}}
@String{CSE = {Computer Science and Education}}
@String{TMH = {Tata McGraw-Hill Publishing Company Limited}}
@String{ES = {Elsevier Science Publishers B. V. (North-Holland)}}
@String{PDS = {The Parallel and Distributed Systems Laboratory}}
@String{DECE = {Department of Electrical and Computer Engineering}}
@String{DCS = {Department of Computer Science}}
@String{PPL = {Parallel Programming Laboratory}}
@String{UIUC = {University of Illinois at Urbana-Champaign}}
@String{UTA = {The University of Texas at Austin}}
@String{OSU = {The Ohio State University}}
@String{UTD = {The University of Texas at Dallas}}
@String{TC = {IEEE Transactions on Computers}}
@String{IPL = {Information Processing Letters (IPL)}}
@String{AMCSJ = {Applied Mathematics and Computer Science Journal}}
@String{WLCPC = {Workshop on Language and Compilers for Parallel Computing}}
@String{IBMARC = {IBM Almaden Research Center}}
@String{IBMZ = {IBM Research Laboratory, Zurich}}
@String{ICDE = {International Conference on Data Engineering (ICDE)}}
@String{CUP = {Cambridge University Press}}
@String{MVPP = {International Meeting on Vector and Parallel Processing}}
@String{TOPLAS = {ACM Transactions on Programming Languages and Systems (TOPLAS)}}
@String{SPDT = {Symposium on Parallel and Distributed Tools}}
@String{CJ = {The Computer Journal}}
@String{PH = {Prentice Hall}}
@String{MK = {Morgan Kaufmann}}
@String{SIGMOD = {ACM SIGMOD International Conference on Managament of Data}}
@String{SIGACT = {ACM Special Interest Group on Algorithms and Computation Theory (SIGACT)}}
@String{USPATENT = {United States Patent Number}}
@String{INFORMIX = {Informix Software Incorporated}}
@String{SV = {Springer-Verlag}}
@String{PDCS = {ISCA International Conference on Parallel and Distributed Computing Systems (PDCS)}}
@String{MIT = {The MIT Press}}
@String{JHUP = {The Johns Hopkins University Press}}
@String{DAM = {Discrete Applied Mathematics}}
@String{DM = {Discrete Mathematics}}
@String{DS = {Distributed Systems}}
@String{ICSKE = {IEEE International Conference on Software and Knowledge Engineering}}
@String{FSTTCS = {Conference on the Foundations of Software Technology and Theoretical
                  Computer Science (FSTTCS)}}
@String{TSE = {IEEE Transactions on Software Engineering}}
@String{JSS = {The Journal of Systems and Software}}
@String{WGCS = {International Workshop on Graph-Theoretic Concepts in Computer Science (WG)}}
@String{JWS = {John Wiley and Sons Limited}}
@String{JWSUS = {John Wiley and Sons, Incorporated}}
@String{ORDAL = {International Conference on Orders, Algorithms and Applications (ORDAL)}}
@String{AJM = {American Journal of Mathematics}}
@String{SRKU = {Sci. Reports Kanazawa Univ.}}
@String{SIAMJDM = {SIAM Journal on Discrete Mathematics}}
@String{KRUSE = {International KRUSE Symposium: Knowledge Use, Retrieval and Storage for Efficiency}}
@String{SIAMJADM = {SIAM Journal on Algebraic and Discrete Methods}}
@String{SIAMJC = {SIAM Journal on Computing}}
@String{MCT = {Mathematical Center Tracts}}
@String{STOC = {Annual ACM Symposium on Theory of Computing (STOC)}}
@String{OOPSLA = {Conference on Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}}
@String{JLMS = {Journal London Mathematics Society}}
@String{AM = {Annals of Mathematics}}
@String{TIT = {IEEE Transactions on Information Theory}}
@String{TR = {IEEE Transactions on Reliability}}
@String{WLP = {Workshop on Logics of Programs}}
@String{ISP = {International Symposium in Programming}}
@String{WSS = {Workshop on Self-Stabilizing Systems (WSS)}}
@String{ICALP = {International Colloquium on Automata, Languages and Systems (ICALP)}}
@String{JA = {Journal of Algorithms}}
@String{KDE = {IEEE Transactions on Knowledge and Data Engineering}}
@String{CS = {ACM Computing Surveys (CSUR)}}
@String{IPDPS = {International Parallel and Distributed Processing Symposium (IPDPS)}}
@String{PDC = {Parallel and Distributed Conference}}
@String{SP = {IEEE Symposium on Security and Privacy}}
@String{USS = {USENIX Security Symposium}}
@String{WNTS = {USENIX Windows NT Symposium}}
@String{UCS = {Computing Systems}}
@String{NCSC = {National Computer Security Conference}}
@String{RV = {Workshop on Runtime Verification (RV)}}
@String{ICPDCS = {IASTED International Conference on Parallel and Distributed Computing and Systems}}
@String{MCDS = {SCS MultiConference on Distributed Simulation}}
@String{SCS = {Society for Computer Simulation}}
@String{BCPC = {The Benjamin Cummings Publishing Company, Incorporated}}
@String{OPODIS = {International Conference on Principles of Distributed Systems (OPODIS)}}
@String{TWSIS = {Texas Workshop on Security of Information Systems (TWSIS)}}
@String{SCISS = {South Central Information Security Symposium (SCISS)}}
@String{CSS = {Computing Systems}}
@String{UCD = {University of California, Davis}}
@String{CSAC = {Annual Computer Security Applications Conference}}
@String{WETICE = {IEEE Workshop on Enabling Technologies: Infrastructure for Collaborative
                  Enterprises (WETICE)}}
@String{TOG = {ACM Transactions on Graphics}}
@String{SCCS = {School of Computer and Communication Sciences}}
@String{EPFL = {{\'E}cole Polytechnique F{\'e}d{\'e}rale de Laussane (EPFL)}}
@String{CORNELL = {Cornell University}}
@String{COMPSAC = {Annual Internation Computer Software and Applications Conference (COMPSAC)}}
@String{JPL = {Journal of Programming Languages}}
@String{PC = {Parallel Computing}}
@String{UWM = {University of Wisconsin, Madison}}
@String{UWTC = {USENIX Winter Technical Conference}}
@String{ICSSE = {Israeli Conference on Computer Systems and Software Engineering}}
@String{IPPS = {International Parallel and Processing Symposium (IPPS)}}
@String{HIS = {Journal of High Integrity Systems}}
@String{HPL = {Hewlett Packard Laboratories}}
@String{ACTA = {Acta Informatica}}
@String{FOCS = {Annual Symposium on Foundations of Computer Science (FOCS)}}
@String{CDS = {IEEE Proceedings---Computers and Digital Techniques}}
@String{JISE = {Journal of Information Science and Engineering}}
@String{ICPADS = {International Conference on Parallel and Distributed Systems (ICPADS)}}
@String{WPPS = {International Workshop on Peer-to-Peer Systems}}
@String{SAC = {IEEE Journal on Selected Areas in Communications}}
@String{TN = {IEEE/ACM Transactions on Networking}}
@String{SNA = {ACM-SIAM Symposium on Discrete Algorithms}}
@String{SIU = {Studia Informatica Universalis}}


@Unpublished{8LGM:1992,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk} (January 1992)}
}

@Article{AchBad:1992:IPL,
  author =   {A. Acharya and B. R. Badrinath},
  title =    {{Recording Distributed Snapshots Based on Causal
                   Order of Message Delivery}},
  journal =  IPL,
  volume =   {44},
  number =   {6},
  pages =    {317-321},
  year =     {1992},
  OPTurl =   {http://citeseer.nj.nec.com/acharya92recording.html}
}

@Misc{Adv:1990:SM,
  title =    {{Sendmail Vulnerability}},
  howpublished = {CERT Advisory CA-90:01 available from \textsf{cert.org} via anonymous ftp},
  month =    JAN,
  year =     {1990}
}

@Article{Adv:1992:Mail,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    JAN,
  year =     1992
}

@Article{Adv:1994:Pwd,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-7.UNIX.passwd.11-May-1994}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    MAY,
  year =     1994
}

@Article{AfeBre:1998:TCS,
  author =   {Y. Afek and A. Bremler},
  title =    {{Self-Stabilizing Unidirectional Network Algorithms by Power Supply}},
  journal =      TCS,
  year =     1998,
  volume =   1998,
  number =   3,
  month =    DEC
}

@InProceedings{AfeKut+:1991:WDAG,
  author =       {Y. Afek and S. Kutten and M. Yung},
  title =        {{Memory-Efficient Self-Stabilizing Protocols for General Networks}},
  booktitle =    PROC # " 4th " # WDAG,
  year =         {1991},
  pages =        {15-28},
  address =      {Bari, Italy},
  publisher =    SV,
}

@Manual{AgaGoe+:1996:IBM,
  author =   {A. Agarwal and A. Goel and A. Sood},
  title =    {{Software Design Description for DLFS on Solaris,
                  HP-UX, and AIX}},
  year =     {1996}
}

@InProceedings{AgrBor+:1989:MD,
  author =   {R. Agrawal and A. Borgida and H. V. Jagadish},
  title =    {{Efficient Management of Transitive Relationships in
                  Large Data and Knowledge Bases}},
  booktitle =    PROC # " " # SIGMOD,
  pages =    {253-262},
  year =     1989,
  address =  {Portland, Oregon}
}

@Book{AhoHop:1974:AW,
  author =   {A. V. Aho and J. E. Hopcroft and J. D. Ullman},
  OPTeditor =    {~},
  title =    {{The Design and Analysis of Computer Algorithms}},
  publisher =    AW,
  year =     1974,
  OPTnote =  {pages 384-386}
}

@InProceedings{AlaVen:1993:WAD,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Hierarchy in Testing Distributed Programs}},
  booktitle =    PROC # " " # WAD,
  pages =    {101-116},
  year =     {1993}
}

@Article{AlaVen:1994:IPL,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{An Optimal Algorithm for Recording Snapshots using Casual
                   Message Delivery}},
  journal =  IPL,
  year =     {1994},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  pages =    {311-316},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@InProceedings{AlaVen:1994:PDS,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  booktitle =    PROC # " " # PDS,
  pages =    {412-417},
  month =    DEC,
  year =     {1994}
}

@Article{AlaVen:2001:TSE,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  journal =  TSE,
  year =     2001,
  volume =   27,
  number =   8,
  pages =    {704-714},
  month =    AUG
}

@TechReport{AlaVid:1999:TR,
  author =   {K. Alagarsamy and K.Vidyasankar},
  title =    {{Elegant Solutions for Group Mutual Exclusion Problem}},
  institution =  {Department of Computer Science, Memorial University of Newfoundland,
                  St.John's, Newfoundland, Canada},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlmBaq+:2002:ICDCS,
  author =   {P. S. Almeida and C. Baquero and V. Fonte},
  title =    {{Version Stamps---Decentralized Version Vectors}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 22nd " # ICDCS,
  pages =    {544-551},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlvEln+:1999:FTCS,
  author =   {L. Alvisi and E. N. Elnozahy and S. Rao and
                  S. A. Hussain and A. D. Mel},
  title =    {{An Analysis of Communication-Induced Checkpointing}},
  booktitle =    PROC # " 29th " # FTCS,
  pages =    {242-249},
  year =     1999,
  address =  {Madison, Wisconsin},
  month =    JUN
}

@InProceedings{AlvMar:1995:ICDCS,
  author =   {L. Alvisi and K. Marzullo},
  title =    {{Message Logging: Pessimistic, Optimistic, and Causal}},
  booktitle =    PROC # " 15th " # ICDCS,
  pages =    {229-236},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@MastersThesis{Ang:2001:Thesis,
  author =   {R. Anguiano},
  title =    {{A Static Analysis Technique for the Detection of
                   TOCTTOU Vulnerabilities}},
  school =   {University of California, Davis},
  year =     {2001},
  OPTkey =   {},
  OPTtype =  {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{AroGou:1994:TC,
  author =   {A. Arora and M. G. Gouda},
  title =    {{Distributed Reset}},
  journal =      TC,
  year =     1994,
  volume =   43,
  number =   9,
  pages =    {1026-1038}
}

@Article{AroSin:1995:HIS,
  author =   {A. Arora and A. Singhai},
  title =    {{Fault-Tolerant Reconfiguration of Trees and Rings in Distributed Systems}},
  journal =      HIS,
  year =     1995,
  volume =   1,
  number =   4,
  pages =    {375-384}
}

@InProceedings{AtrMit+:2003:OPODIS,
  author =   {R. Atreya and N. Mittal and V. K. Garg},
  title =    {{Detecting Locally Stable Predicates without
                   Modifying Application Messages}},
  booktitle =    PROC # " 7th " # OPODIS,
  year =     2003,
  pages =        {20-33},
  address =  {La Martinique, France},
  month =    DEC
}

@Article{BabFro+:1996:JSS,
  author =   {{\"O}. Babao{\v{g}}lu and E. Fromentin and
                  M. Raynal},
  title =    {{A Unified Framework for the Specification and Run-time Detection
                   of Dynamic Properties in Distributed Computations}},
  journal =  JSS,
  volume =   {33},
  number =   {3},
  month =    JUN,
  pages =    {287-298},
  year =     {1996},
  url =      {http://citeseer.nj.nec.com/10396.html}
}

@incollection{BabMar:1993:DS,
  author =   {{\"{O}}. Babao{\v g}lu and K. Marzullo},
  title =    {{Consistent Global States of Distributed Systems: Fundamental Concepts and
                   Mechanisms}},
  booktitle =    DS,
  publisher =    AW,
  editor =   {S. Mullender},
  pages =    {55-96},
  year =     {1993},
  url =
                  {http://citeseer.nj.nec.com/babaoglu93consistent.html}
}

@Article{BabRay:1995:JPDC,
  author =   {{\"{O}}. Babao{\v g}lu and M. Raynal},
  title =    {{Specification and Verification of Dynamic Properties in Distributed Computations}},
  journal =  JPDC,
  year =     1995,
  volume =   28,
  number =   2,
  pages =    {173-185}
}

@Book{Bac:1987:Book,
  author =   {M. J Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987,
  isbn =     0132017997
}

@Book{Bac:1987:PH,
  author =   {M. J. Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987
}

@Manual{BalKan:1999:INFORMIX,
  author =   {I. Balabine and R. Kandasamy},
  title =    {{File System Interface to a Database}},
  note =     USPATENT # " 5937406 granted to " # INFORMIX,
  year =     {1999},
  month =    AUG
}

@InProceedings{BarBra+:1996:ICSSE,
  author =   {A. Barak and A. Braverman and A. Gilderman and O. La'adan},
  title =    {{Performance of PVM with MOSIX Preemptive Process Migration}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 7th " # ICSSE,
  pages =    {38-45},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Herzliya},
  month =    JUN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BeaCan+:2003:JISE,
  author =   {J. Beauquier and S. Cantarell and A. K. Datta and F. Petit},
  title =    {{Group Mutual Exclusion in Tree Networks}},
  journal =      JISE,
  year =     {2003},
  OPTkey =   {},
  volume =   {19},
  number =   {3},
  pages =    {415-432},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{BegDon+:PVM2.0,
  title =    {{H}ence: {A} users' guide - version 2.0. {PVM}
                  {D}esign and {V}isualization},
  author =   {A. Beguelin and J. Dongarra and G. A. Geist and
                  R. Manchek and K. Moore and P. Newton and
                  V. Sunderam}
}

@InProceedings{Bel:1990:MCDS,
  author =   {S. Bellenot},
  title =    {{Global Virtual Time Algorithms}},
  booktitle =    PROC # " " # MCDS,
  pages =    {122-127},
  year =     1990,
  volume =   22,
  number =   1,
  month =    JAN,
  organization = SCS
}

@TechReport{Bis:1995:TR:8,
  author =   {M. Bishop},
  title =    {{Race Conditions, Files, and Security Flaws: or, The
                   Tortoise and the Hare \emph{Redux}}},
  institution =  DCS # ", " # UCD,
  year =     {1995},
  OPTkey =   {},
  OPTtype =  {},
  number =   {95-8},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{BisDil:1996:CSS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File Accesses}},
  journal =  CSS,
  year =     2003,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Article{BisDil:1996:UCS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File
                  Accesses}},
  journal =  UCS,
  year =     1996,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Unpublished{BisHol:1978:PR:13,
  author =   {R. Bisbey and D. Hollingsworth},
  title =    {{Protection Analysis Project Final Report}},
  note =     {ISI/RR-78-13, DTIC AD A056816, USC/Information
                  Sciences Institute},
  OPTkey =   {},
  month =    MAY,
  year =     {1978},
  OPTannote =    {}
}

@Article{Bou:1987:TCS,
  author =   {L. Bouge},
  title =    {{Repeated Snapshots in Distributed Systems
                  with Synchronous Communication and their
                  Implementation in CSP}},
  journal =  TCS,
  year =     1987,
  volume =   49,
  pages =    {145-169}
}

@Article{Bre:1966:TIT,
  author =   {M. Breuer},
  title =    {{Coding Vertexes of a Graph}},
  journal =  TIT,
  year =     1966,
  volume =   12,
  pages =    {148-153}
}

@TechReport{BriLit+:1992:CONDOR,
  author =   {A. Bricker and M. Litzkow and M. Livny},
  title =    {{Condor Technical Summary, Version 4.1b}},
  institution =  "Computer Science Department, " # UWM,
  year =     {1992},
  OPTkey =   {},
  OPTtype =      {},
  number =   {CS-TR-92-1069},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BrzHel+:1993:ICDCS,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal},
  title =    {{Termination Detection in a Very General Distributed
                   Computing Model}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {374-381},
  year =     1993
}

@article{BrzHel+:1995:JPDC,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal and
                  M. Singhal},
  title =    {{Deadlock Models and a General Algorithm for
                   Distributed Deadlock Detection}},
  journal =  JPDC,
  volume =   {31},
  number =   {2},
  pages =    {112-125},
  year =     "1995"
}

@Misc{Bug:2002:RDR,
  title =    {{Recursive Directory Removal Race Condition}},
  howpublished = {http://mail.gnu.org/pipermail/bug-fileutils/2002-March/002433.html},
  month =    MAR,
  year =     2002
}

@Manual{CORBA:1997,
  author =   {Object Management Group},
  title =    {{The Common Object Request Broker: Architecture and Specification}}
}

@InProceedings{CanDat+:2001:ICDCS,
  author =   {S. Cantarell and A. K. Datta and F. Petit and V. Villain},
  title =    {{Token Based Group Mutual Exclusion for Asynchronous Rings}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {691-694},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Cap:1994:ORDAL,
  author =   {C. Capelle},
  title =    {{Representation of an Order as Union of Interval Orders}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {143-161},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =  {Lyon, France},
  month =    JUL,
  publisher =    SV
}

@InProceedings{Cas:1993:OOPSLA,
  author =   {Y. Caseau},
  title =    {{Efficient Handling of Multiple Inheritance Hierarchies}},
  booktitle =    PROC # " " # OOPSLA,
  pages =    {271-287},
  year =     1993
}

@Article{Cas:1995:CSS,
  author =   {J. Casas and R. Konuru and S. W. Otto and R. M. Prouty and J. Walpole},
  title =    {{MPVM---A Migration Transparent Version of PVM}},
  journal =      CSS,
  year =     {1995},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {171-216},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaDel+:1995:TOPLAS,
  author =   {B. Charron-Bost and C. Delporte-Gallet and
                  H. Fauconnier},
  title =    {{Local and Temporal Predicates in Distributed Systems}},
  journal =  TOPLAS,
  year =     1995,
  volume =   17,
  number =   1,
  pages =    {157-179}
}

@InProceedings{ChaGar:1995:WDAG,
  author =   {C. Chase and V. K. Garg},
  title =    {{On Techniques and their Limitations for the Global Predicate
                   Detection Problem}},
  booktitle =    PROC # " " # WDAG,
  year =     1995,
  address =  {France},
  month =    SEP,
  pages =    {303-317}
}

@Article{ChaGar:1998:DC,
  author =   {C. Chase and V. K. Garg},
  title =    {{Detection of Global Predicates: Techniques and their Limitations}},
  journal =  DC,
  year =     1998,
  volume =   11,
  number =   4,
  pages =    {191-201}
}

@Article{ChaLam:1985:TrCS,
  author =   {K. M. Chandy and L. Lamport},
  title =    {{Distributed Snapshots: Determining Global States of Distributed Systems}},
  journal =  TrCS,
  year =     1985,
  volume =   3,
  number =   1,
  pages =    {63-75},
  month =    FEB
}

@Article{ChaMis+:1983:TrCS,
  author =   {K. M. Chandy and J. Misra and L. M. Haas},
  title =    {{Distributed Deadlock Detection}},
  journal =      TrCS,
  year =     1983,
  volume =   1,
  number =   2,
  pages =    {144-156},
  month =    MAY
}

@Article{ChaMis:1984:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{The Drinking Philosophers Problem}},
  journal =      TOPLAS,
  year =     {1984},
  OPTkey =   {},
  volume =   {6},
  number =   {4},
  pages =    {632-646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:DC,
  author =   {K. M. Chandy and J. Misra},
  title =    {{How Processes Learn}},
  journal =  DC,
  year =     {1986},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {40-52},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Book{ChaMis:1988:Book,
  author =   {K. M. Chandy and J. Misra},
  title =    {{Parallel Program Design: A Foundation}},
  publisher =    AW,
  year =     1988
}

@Article{ChaTou:1996:JACM,
  author =   {T. D. Chandra and S. Toueg},
  title =    {{Unreliable Failure Detectors for Reliable Distributed Systems}},
  journal =  JACM,
  year =     {1996},
  volume =   {43},
  number =   {2},
  pages =    {225-267}
}

@Article{ChaVen:1990:JPDC,
  author =   {S. Chandrasekaran and S. Venkatesan},
  title =    {{A Message-Optimal Algorithm for Distributed
                  Termination Detection}},
  journal =  JPDC,
  year =     {1990},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {245-252},
  month =    MAR,
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Charron-Bost:size,
  author =   {B. Charron-Bost},
  title =    {{Concerning the Size of Logical Clocks in Distributed Systems}},
  journal =  IPL,
  year =     1991,
  month =    JUL,
  volume =   {39},
  pages =    {11-16},
}

@InProceedings{Che:1993:WAD,
  author =   {J. Cheng},
  title =    {{Slicing Concurrent Programs---A Graph-Theoretical Approach}},
  booktitle =    PROC # " " # WAD,
  pages =    {223-240},
  year =     1993
}

@Article{ChoMil+:1991:TOPLAS,
  author =   {J. Choi and B. P. Miller and R. Netzer},
  title =    {{Techniques for Debugging Parallel Programs with Flowback Analysis}},
  journal =  TOPLAS,
  year =     1991,
  volume =   13,
  number =   4,
  pages =    {491-530},
  month =    OCT
}

@InProceedings{ClaEme:1981:WLP,
  author =   {E. M. Clarke and E. A. Emerson},
  title =    {{Design and Synthesis of Synchronization Skeletons using
                   Branching Time Temporal Logic}},
  booktitle =    PROC # " " # WLP,
  address =  {Yorktown Heights, New York},
  month =    MAY,
  series =   LNCS,
  volume =   131,
  year =     1981
}

@InProceedings{CohLeh:1982:PODC,
  author =   {S. Cohen and D. Lehmann},
  title =    {{Dynamic Systems and their Distributed Termination}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # PODC,
  pages =    {29-33},
  year =     {1982},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Ottawa},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ColDol:1994:IPL,
  author =   {Z. Collin and S. Dolev},
  title =    {{Self-Stabilizing Depth-First Search}},
  journal =      IPL,
  year =     1994,
  volume =   49,
  number =   6,
  pages =    {297-301}
}

@InProceedings{CooMar:1991:WPDD,
  author =   {R. Cooper and K. Marzullo},
  title =    {{Consistent Detection of Global Predicates}},
  booktitle =    PROC # " " # WPDD,
  pages =    {163-173},
  year =     1991,
  address =  {Santa Cruz, California}
}

@Book{CorLei+:1991:MIT,
  author =   {T. H. Cormen and C. E. Leiserson and R. L. Rivest},
  title =    {{Introduction to Algorithms}},
  publisher =    MIT,
  address =  {Cambridge, Massachusetts},
  year =     {1991},
}

@InProceedings{CowBea+:2001:USS,
  author =   {C. Cowan and S. Beattie and C. Wright and
                  G. Korah-Hartman},
  title =    {{RaceGuard: Kernel Protection from Temporary File
                   Race Vulnerabilities}},
  booktitle =    PROC # " 10th " # USS,
  pages =    {165-172},
  year =     2001,
  month =    AUG
}

@Book{CoxGoo:1994:PH,
  author =   {J. Cox and B. Goodheart},
  title =    {{The Magic Garden Explained: The Internals of Unix
                   System V Release 4: An Open Systems Design}},
  publisher =    PH,
  year =     1994
}

@InProceedings{CypLeu:1995:SPDP,
  author =   {R. Cypher and E. Leu},
  title =    {{Efficient Race Detection for Message-Passing
                   Programs with Nonblocking Sends and Receives}},
  booktitle =    PROC # " " # SPDP,
  pages =    {534-541},
  year =     1995
}

@Manual{DB2SQL:1999:IBM,
  title =    {DB2 UDB SQL Reference},
  organization = {IBM},
  edition =  {V6.1},
  year =     1999
}

@Article{DarMay:2003:JPDC,
  author =   {D. Darling and J. Mayo},
  title =    {{Stable Predicate Detection in Dynamic Systems}},
  journal =      "Submitted to the " # JPDC,
  OPTpages =     {},
  year =     {2003},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{Dav:1999:IBM,
  title =    {{DataLinks: Managing External Data with DB2
                   Universal Database}},
  organization = {IBM Corporation},
  month =    FEB,
  year =     {1999},
  note =     {White paper prepared by J. R. Davis}
}

@Book{DavPri:1990:CUP,
  author =   {B. A. Davey and H. A. Priestley},
  title =    {{Introduction to Lattices and Order}},
  publisher =    CUP,
  address =  {Cambridge, UK},
  year =     {1990},
}

@TechReport{DemAro:2000:TR:05,
  author =   {M. Demirbas and A. Arora},
  title =    {{An Optimal Termination Detection Algorithm for
                   Rings}},
  institution =  OSU,
  year =     2000,
  number =   {OSU-CISRC-2/00-TR05},
  month =    FEB
}

@Article{Den:1987:TSE,
  author =   {D. Denning},
  title =    {{An Intrusion Detection Model}},
  journal =  TSE,
  volume =   {13},
  number =   {2},
  month =    FEB,
  year =     {1987},
  pages =    {222-232}
}

@Article{DhaIye+:1997:PC,
  author =   {D. M. Dhamdhere and S. R. Iyer and E. K. K. Reddy},
  title =    {{Distributed Termination Detection for Dynamic Systems}},
  journal =      PC,
  year =     {1997},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {2025-2045},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dij:1965:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Solution of a Problem in Concurrent Programming
                   Control}},
  journal =  CACM,
  pages =    569,
  year =     1965,
  volume =   8,
  number =   9,
  organization = {ACM}
}

@Article{Dij:1971:ACTA,
  author =   {E. W. Dijkstra},
  title =    {{Hierarchical Ordering of Sequential Processes}},
  journal =      ACTA,
  year =     1971,
  volume =   1,
  number =   2,
  pages =    {115-138},
  month =    OCT
}

@Article{Dij:1974:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Self-Stabilizing Systems in spite of Distributed Control}},
  journal =  CACM,
  year =     {1974},
  volume =   {17},
  number =   {11},
  pages =    {643-644}
}

@InCollection{Dij:1985:SV,
  author =   {E. W. Dijsktra},
  title =    {{The Distributed Snapshot of K. M. Chandy and L. Lamport}},
  booktitle =    {Control Flow and Data Flow: Concepts of Distributed
                  Programming},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    SV,
  year =     {1985},
  editor =   {M. Broy},
  volume =   {F14},
  OPTnumber =    {},
  series =   {NATO ASI},
  OPTtype =  {},
  OPTchapter =   {},
  address =  {New York, NY},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Dij:1986:DC,
  author =   {E. W. Dijkstra},
  title =    {{A Belated Proof of Self-Stabilization}},
  journal =  DC,
  year =     {1986},
  volume =   {1},
  pages =    {5-6}
}

@Article{DijFei+:1983:IPL,
  author =   {E. W. Dijkstra and W. H. J. Feijen and A. J. M. van
                  Gasteren},
  title =    {{Derivation of a Termination Detection Algorithm for
                   Distributed Computations}},
  journal =  IPL,
  volume =   {16},
  pages =    {217-219},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1983},
  OPTannote =    {}
}

@Article{DijSch:1980:IPL,
  author =   {E. W. Dijkstra and C. S. Scholten},
  title =    {{Termination Detection for Diffusing Computations}},
  journal =  IPL,
  year =     1980,
  volume =   11,
  number =   1,
  pages =    {1-4}
}

@Article{Dil:1950:AM,
  author =   {R. P. Dilworth},
  title =    {{A Decomposition Theorem for Partially Ordered Sets}},
  journal =  AM,
  year =     1950,
  volume =   51,
  pages =    {161-166}
}

@Article{DolIsr+:1993:DC,
  author =   {S. Dolev and A. Israeli and S. Moran},
  title =    {{Self-Stabilization of Dynamic Systems Assuming Only Read/Write Atomicity}},
  journal =      DC,
  year =     1993,
  volume =   7,
  number =   1,
  pages =    {3-16}
}

@InProceedings{DueGup+:1992:WLCPC,
  author =   {E. Duesterwald and R. Gupta and M. L. Soffa},
  title =    {{Distributed Slicing and Partial Re-execution for Distributed Programs}},
  booktitle =    PROC # " 5th " # WLCPC,
  pages =    {329-337},
  year =     1992
}

@Article{DusMil:1941:AJM,
  author =   {B. Dushnik and E. W. Miller},
  title =    {{Partially Ordered Sets}},
  journal =  AJM,
  year =     1941,
  volume =   63,
  pages =    {600-610}
}

@PhdThesis{Ell:1995:PhD,
  author =   {G. Ellis},
  title =    {{Managing Complex Objects}},
  school =   {University of Queensland},
  year =     1995
}

@Article{ElnAlv+:2002:CS,
  author =   {E. N. Elnozahy and L. Alvisi and Y.-M. Wang and
                  D. B. Johnson},
  title =    {{A Survey of Rollback-Recovery Protocols in
                   Message-Passing Systems}},
  journal =  CS,
  volume =   {34},
  number =   {3},
  year =     {2002},
  pages =    {373-408},
}

@Article{FelHab+:1994:SIAMJDM,
  author =   {S. Felsner and M. Habib and R. H. M{\"o}hring},
  title =    {{On the Interplay of Interval Dimension and Dimension}},
  journal =  SIAMJDM,
  volume =   7,
  pages =    {32-40},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/Idim-dim.ps.gz},
}

@Article{FelTro:1994:DM,
  author =   {S. Felsner and W. T. Trotter},
  title =    {{On the Fractional Dimension of Partially Ordered Sets}},
  journal =  DM,
  volume =   136,
  pages =    {101-117},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/fdim.ps.gz},
}

@Article{Fid:1991:Com,
  author =   {C. Fidge},
  title =    {{Logical Time in Distributed Computing Systems}},
  journal =  Com,
  year =     1991,
  volume =   24,
  number =   8,
  pages =    {28-33},
  month =    AUG
}

@InProceedings{FisLyn+:1979:FCS,
  author =   {M. J. Fischer and N. A. Lynch and  J. E. Burns and A. Borodin},
  title =    {{Resource Allocation with Immunity to Limited Process Failure
                   (preliminary report)}},
  booktitle =    PROC # " 20th " # FOCS,
  pages =    {234-254},
  year =     1979,
  month =    OCT
}

@Article{Fra:1980:TOPLAS,
  author =   {N. Francez},
  title =    {{Distributed Termination}},
  journal =  TOPLAS,
  year =     1980,
  volume =   2,
  number =   1,
  pages =    {42-55},
  month =    JAN
}

@InProceedings{FroRay+:1994:ICPP,
  author =   {E. Fromentin and M. Raynal and V. K. Garg and
                  A. I. Tomlinson},
  title =    {{On the Fly Testing of Regular Patterns in Distributed Computations}},
  booktitle =    PROC # " 23rd " # ICPP,
  pages =    {73-76},
  year =     1994,
  number =   2,
  address =  {Chicago, Illinois},
  month =    AUG
}

@InProceedings{FroRay:1994:SPDP,
  author =   {E. Fromentin and M. Raynal},
  title =    {{Inevitable Global States: A Concept to Detect
                   Unstable Properties of Distributed Computations in
                   an Observer Independent Way}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {242-248},
  year =     {1994},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}

@Misc{GDB,
  OPTkey =   {},
  OPTauthor =    {},
  title =    {{GDB: The GNU Project Debugger}},
  OPThowpublished = {},
  OPTmonth =     {},
  OPTyear =      {},
  note =     {Available at
                  \texttt{http://www.gnu.org/software/gdb/gdb.html}},
  OPTannote =    {}
}

@TechReport{Gae:2003:TR:38,
  author =   {F. C. G{\"a}rtner},
  title =    {{A Survey of Self-Stabilizing Spanning-Tree Construction Algorithms}},
  institution =  SCCS # ", " # EPFL,
  address =      {Lausanne, Switzerland},
  year =     2003,
  number =   {IC 2003/38}
}

@InProceedings{GaeKlo:2000:SRDS,
  author =   {F. C. G{\"a}rtner and S. Kloppenburg},
  title =    {{Consistent Detection of Global Predicates under a Weak Fault Assumption}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # ", " # SRDS,
  pages =    {94-103},
  year =     {2000},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {N{\"u}rnberg, Germany},
  month =    OCT,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{GaePle:2001:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in
                  Crash-Affected Systems using
                  Interrupt-Style Failure Detectors (Brief Announcement)}},
  booktitle =    PROC # " " # DISC,
  year =     2001,
  address =  {Lisbon, Portugal},
  month =    {October}
}
@TechReport{GaePle:2001:TR,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  institution =  IBMZ,
  year =     2001,
  number =   {RZ 3361 (\# 93407)},
  month =    AUG
}
@InProceedings{GaePle:2001:WSS,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  booktitle =    PROC # " 5th " # WSS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {98-113},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS # " 2194",
  address =  {Lisbon, Portugal},
  month =    {October},
  OPTorganization ={},
  publisher =    SV,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GaePle:2002:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{Failure Detection Sequencers: Necessary and Sufficient
                  Information about Failures to Solve Predicate Detection}},
  booktitle =    PROC # " 16th " #  DISC,
  pages =    {280-294},
  year =     2002,
  number =   2508,
  series =   LNCS,
  publisher =    SV
}
@InProceedings{GamNes+:1987:ICALP,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{Posets, Boolean Representations and Quick
                   Path Searching}},
  booktitle =    PROC # " 14th " # ICALP,
  year =     1987,
  pages =    {404-424},
  number =   267,
  series =   LNCS
}
@Article{GamNes+:1990:TCS,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{On Locally Presented Posets}},
  journal =  TCS,
  year =     {1990},
  OPTkey =   {},
  volume =   {70},
  number =   {2},
  pages =    {251-260},
  month =    JAN,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{Gar:1996:ICSKE,
  author =   {V. K. Garg},
  title =    {{Observation of Global Properties in Distributed Systems}},
  booktitle =    ICSKE,
  pages =    {418-425},
  year =     1996,
  address =  {Lake Tahoe, Nevada},
  month =    JUN
}
@Book{Gar:1996:KAP,
  author =   {V. K. Garg},
  OPTeditor =    {~},
  title =    {{Principle of Distributed Systems}},
  publisher =    KAP,
  year =     1996
}
@InProceedings{Gar:1997:WAD,
  author =   {V. K. Garg},
  title =    {{Observation and Control for Debugging
                   Distributed Computations}},
  booktitle =    PROC # " " # WAD,
  pages =    {1-12},
  year =     1997,
  address =  {Link{\"o}ping, Sweden},
  note =     {Keynote Presentation}
}
@Book{Gar:2002:Book,
  author =   {V. K. Garg},
  title =    {{Elements of Distributed Computing}},
  publisher =    JWSUS,
  address =  {New York, NY},
  year =     {2002},
}
@InProceedings{Gar:2002:FSTTCS,
  author =   {V. K. Garg},
  title =    {{Algorithmic Combinatorics based on Slicing Posets}},
  booktitle =    PROC # " 22nd " # FSTTCS,
  year =     2002,
  address =  {Kanpur, India},
  month =    {December}
}
@Article{GarBar:1985:ACM,
  author =   {H. Garcia-Molina and D. Barbar},
  title =    {{How to Assign Votes in a Distributed System}},
  journal =  JACM,
  year =     {1985},
  volume =   {32},
  number =   {4},
  pages =    {841-860},
  month =    OCT
}
@InProceedings{GarCha+:1995:CSS,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Detecting Conjunctive Channel Predicates in
                   a Distributed Programming Environment}},
  booktitle =    PROC # " " # CSS,
  pages =    {232-241},
  year =     1995,
  volume =   2,
  address =  {Maui, Hawaii},
  month =    JAN
}
@Article{GarCha+:1997:JPDC,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Efficient Detection of Channel Predicates in
                   Distributed Systems}},
  journal =  JPDC,
  year =     {1997},
  volume =   {45},
  number =   {2},
  pages =    {134-147},
  month =    SEP
}
@InProceedings{GarCha:1995:ICDCS,
  author =   {V. K. Garg and C. Chase},
  title =    {{Distributed Algorithms for Detecting
                   Conjunctive Predicates}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {423-430},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@Book{GarJoh:1991:Fre,
  author =   {M. R. Garey and D. S. Johnson},
  OPTeditor =    {Victor Klee},
  title =    {{Computer and Intractability: A Guide to the
                   Theory of \mbox{NP-Completeness}}},
  publisher =    Fre,
  year =     1991
}
@InProceedings{GarLun:1991:NCSC,
  author =   {T. D. Garvey and T. F. Lunt},
  title =    {{Model-Based Intrusion Detection}},
  booktitle =    PROC # " 14th " # NCSC,
  pages =    {372-385},
  year =     1991
}
@Article{GarMit+:2003:SIGACT,
  author =   {V. K. Garg and N. Mittal and A. Sen},
  title =    {{Applications of Lattice Theory to Distributed
                  Computing}},
  journal =  SIGACT # " News Distributed Computing Column",
  year =     2003,
  OPTpublisher = {ACM Press},
  editor =   {Sergio Rajsbaum},
  volume =   34,
  number =   3,
  pages =    {40-61},
  month =    SEP
}
@InProceedings{GarMit:1998:FSTTCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Implementable Failure Detectors in
                   Asynchronous Systems}},
  booktitle =    PROC # " " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {158-169},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =  {Chennai, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GarMit:1998:ICDCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Distributed Predicate Detection in a Faulty
                   Environment}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {416-423},
  year =     {1998},
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}
@InProceedings{GarMit:2001:ICDCS,
  author =   {V. K. Garg and N. Mittal},
  title =    {{On Slicing a Distributed Computation}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {322-329},
  year =     2001,
  address =  {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@InProceedings{GarSka:2001:PODC,
  author =   {V. K. Garg and C. Skawratananond},
  title =    {{String Realizers of Posets with Applications
                   to Distributed Computing}},
  booktitle =    PROC # " 20th " # PODC,
  year =     2001,
  address =  {Newport, Rhode Island},
  month =    AUG,
  pages =    {72-80}
}
@InProceedings{GarTom+:1995:SPDP,
  author =   {V. K. Garg and A. I. Tomlinson and E. Fromentin and
                  Michel Raynal},
  title =    {{E}xpressing and {D}etecting {G}eneral {C}ontrol
                  {F}low {P}roperties of {D}istributed {C}omputations},
  booktitle =    PROC # " 7th " # SPDP,
  pages =    {432-438},
  year =     1995,
  address =  {San Antonio, Texas},
  month =    OCT
}
@InProceedings{GarWal:1991:WPDD,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  month =    MAY,
  year =     {1991},
  OPTorganization ={ACM/ONR},
}
@InProceedings{GarWal:1992:FSTTCS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates in
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 12th " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {253-264},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS,
  address =  {New Delhi, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@Article{GarWal:1994:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Weak Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1994,
  volume =   5,
  number =   3,
  pages =    {299-307},
  month =    MAR
}
@Article{GarWal:1996:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Strong Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1996,
  volume =   7,
  number =   12,
  pages =    {1323-1333},
  month =    DEC
}
@Article{GhoGup+:1996:JCI,
  author =   {S. Ghosh and A. Gupta and S. V. Pemmaraju},
  title =    {{A Fault-containing Self-stabilizing Spanning Tree Algorithm}},
  journal =      JCI,
  year =     1996,
  volume =   2,
  number =   1,
  pages =    {322-328}
}
@Book{God:1996:SV,
  author =   {P. Godefroid},
  ALTeditor =    {},
  title =    {{P}artial-{O}rder {M}ethods for the {V}erification of
                  {C}oncurrent {S}ystems},
  publisher =    SV,
  year =     {1996},
  volume =   {1032},
  series =   {Lecture Notes in Computer Science}
}
@Book{GodCox:1993:PH,
  author =   {B. Goodheart and J. Cox},
  title =    {The Magic Garden Explained: The Internals of Unix
                  System V Release 4},
  publisher =    PH,
  year =     {1993}
}
@Misc{GoySit+:2003:SCISS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{A Partial Order Approach to Detect Race Condition Attacks}},
  howpublished = "Abstract published in " # SCISS ,
  month =    APR,
  year =     2003
}
@TechReport{GoySit+:2003:TR:03,
  author =       {B. Goyal and S. Sitaraman and S. Venkatesan},
  title =        {{A Unified Approach to Detect Binding Based Race Condition Attacks}},
  number =       {UTDCS-02-03},
  year =         2003,
  institution =  DCS # ", " # UTD # ", " # "\textsf{http://www.utdallas.edu/{\textasciitilde}venky/publications/race.pdf}"
}
@InProceedings{GoySri+:2003:TWSIS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{Methods To Tackle Vulnerabilities Caused by Lack of Mutual Exclusion}},
  booktitle =    PROC # " " # TWSIS,
  year =     2003,
  pages =        {17-21},
  address =      {College Station, Texas},
  month =    APR
}
@Book{GraReu:1993:MK,
  author =   {J. Gray and A. Reuter},
  title =    {Transaction Processing: Concepts and Techniques},
  publisher =    MK,
  year =     {1993}
}
@InProceedings{GraVol:1993:MVPP,
  author =   {S. Grabner and J. Volkert},
  title =    {{Debugging Parallel Programs Using Event Graph Manipulation}},
  booktitle =    PROC # " " # MVPP,
  pages =    {443-450},
  year =     1993,
  month =    OCT
}
@Book{Gratzer,
  author =       {G. Gratzer},
  title =        {{General Lattice Theory}},
  publisher =    {Academic Press},
  address =      {New York, NY},
  year =         1978
}
@InProceedings{HabHuc+:1995:KRUSE,
  author =   {M. Habib and M. Huchard and L. Nourine},
  title =    {{Embedding Partially Ordered Sets into Chain-Products}},
  booktitle =    PROC # " " # KRUSE,
  pages =    {147-161},
  year =     1995,
  address =      {University of California, Santa Cruz},
  month =    AUG
}
@InProceedings{HabNou:1994:ORDAL,
  author =   {M. Habib and L. Nourine},
  title =    {{Bit-Vector Encoding for Partially Ordered Sets}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {1-12},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =      {Lyon, France},
  month =    JUL,
  publisher = SV
}

@inproceedings{KuznetsovRavi:ConcurrencyTM:OPODIS:2011,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  booktitle = {OPODIS},
  year      = {2011},
  pages     = {112-127},
  ee        = {http://dx.doi.org/10.1007/978-3-642-25873-2_9}
}


@InProceedings{Had:2001:PODC,
  author =   {V. Hadzilacos},
  title =    {{A Note on Group Mutual Exclusion}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 20th " # PODC,
  OPTpages =     {},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    AUG,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Hadzilacos:1988:JACM,
 author = {Hadzilacos, Vassos},
 title = {A theory of reliability in database systems},
 journal = {J. ACM},
 issue_date = {Jan. 1988},
 volume = {35},
 number = {1},
 month = jan,
 year = {1988},
 issn = {0004-5411},
 pages = {121--145},
 numpages = {25}
} 


@InProceedings{HelJar+:1987:PODC,
  author =       {J.-M. H{\'e}lary and C. Jard and N. Plouzeau and M. Raynal},
  title =        {{Detection of Stable Properties in Distributed Applications}},
  booktitle =    PROC # " " # PODC,
  pages =        {125-136},
  year =         {1987}
}
@article{HelRay:1994:DC,

  author =       {J.-M. H{\'e}lary and M. Raynal},
  title =        {{Towards the Construction of Distributed Detection Programs, with
                   an Application to Distributed Termination}},
  journal =      DC,
  volume =       {7},
  number =       {3},
  pages =        {137-147},
  year =         "1994"
}
@Article{Hir:1951:SRKU,
  author =   {T. Hiraguchi},
  title =    {{On the Dimension of Partially Ordered Sets}},
  journal =      SRKU,
  year =     1951,
  volume =   1,
  pages =    {77-94}
}
@Article{Hir:1955:SRKU,
  author =   {T. Hiraguchi},
  title =    {{O}n the {D}imension of {O}rders},
  journal =      SRKU,
  year =     1955,
  volume =   4,
  pages =    {1-20}
}
@Article{HoRam:1982:TSE,
  author =   {G. S. Ho and C. V. Ramamoorthy},
  title =    {{Protocols for Deadlock Detection in Distributed Database Systems}},
  journal =      TSE,
  year =     {1982},
  OPTkey =   {},
  volume =   {8},
  number =   {6},
  pages =    {554-557},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hol:1997:TSE,
  author =   {G. Holzmann},
  title =    {{The Model Checker SPIN}},
  journal =      TSE,
  year =     1997,
  OPTkey =   {},
  volume =   23,
  number =   5,
  pages =    {279-295},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{HsiMit:2000:TC,
  author =   {H. Hsiao and N. Mittal},
  title =    {{Database Managed External File Update}},
  institution =  IBMARC,
  year =     2000,
  number =   {RJ10183},
  address =  {San Jose, California, 95120}
}
@Manual{HsiNar:1999:IBMARC,
  author =   {H. Hsiao and I. Narang},
  title =    {{Update In-Place Support with DataLinks}},
  organization = IBMARC,
  year =     {1999},
  note =     {Internal Document}
}
@InProceedings{HsiNar:2000:SIGMOD,
  author =   {H. Hsiao and I. Narang},
  title =    {{DLFM: A Transactional Resource Manager}},
  booktitle =    PROC # " 19th " # SIGMOD,
  pages =    {518-528},
  year =     2000,
  address =  {Dallas, Texas},
  month =    MAY
}
@InProceedings{Hua:1989:ICDCS,
  author =   {S.-T. Huang},
  title =    {{Detecting Termination of Distributed Computations by External Agents}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {79-84},
  year =     {1989},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hua:1989:IPL,
  author =   {S.-T. Huang},
  title =    {{Termination Detection by using Distributed Snapshots}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {32},
  OPTnumber =    {},
  pages =    {113-119},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{HuaChe:1992:IPL,
  author =   {S.-T. Huang and N.-S. Chen},
  title =    {{A Self-Stabilizing Algorithm for Constructing Breadth-First Trees}},
  journal =      IPL,
  year =     1992,
  volume =   41,
  number =   2,
  pages =    {109-117},
  month =    FEB
}
@InProceedings{HuaKin:1993:FTCS,
  author =   {Y. Huang and C. Kintala},
  title =    {{S}oftware {I}mplemented {F}ault {T}olerance:
                  {T}echnologies and {E}xperience},
  booktitle =    PROC # " " # FTCS,
  pages =    {138-144},
  year =     1993,
  month =    JUN
}
@InProceedings{HurMiz+:1996:SPDP,
  author =   {M. Hurfin and M. Mizuno and M. Raynal and
                  M. Singhal},
  title =    {{Efficient Distributed Detection of Conjunctions of Local Predicates in
                   Asynchronous Computations}},
  booktitle =    PROC # " 8th " # SPDP,
  pages =    {588-594},
  year =     1996,
  address =  {New Orleans},
  month =    OCT
}
@Article{HurPlo+:1993:JCC,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{A Debugging Tool for Distributed Estelle Programs}},
  journal =  JCC,
  year =     1993,
  volume =   16,
  number =   5,
  pages =    {328-333},
  month =    MAY
}
@InProceedings{HurPlo+:1993:WPDD,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{D}etecting {A}tomic {S}equences of {P}redicates in
                  {D}istributed {C}omputations},
  booktitle =    PROC # " " # WPDD,
  pages =    {32-42},
  year =     1993
}
@InProceedings{HurRay:1996:WGCS,
  author =   {M. Hurfin and M. Raynal},
  title =    {{D}etecting {D}iamond {N}ecklaces in {L}abeled {D}ags
                  ({A} {P}roblem from {D}istributed  {D}ebugging},
  booktitle =    PROC # " " # WGCS,
  pages =    {211-223},
  year =     1996,
  series =   LNCS,
  publisher =    SV
}
@Manual{ISO:1993,
  author =       {ISO},
  title =        {{S}pecification of the {A}synchronous {T}ransfer {M}ode
                  {R}ing {(ATMR)} {P}rotocol},
  month =        JAN,
  year =         1993,
}
@InProceedings{JarJer+:1994:ICDCS,
  author =       {C. Jard and T. J{\'e}ron and G.-V. Jourdan and J.-X. Rampon},
  title =        {{A} {G}eneral {A}pproach to {T}race-{C}hecking in
                  {D}istributed {C}omputing {S}ystems},
  booktitle =    PROC # " " # ICDCS,
  pages =        {396-403},
  year =         {1994},
  url =          {http://citeseer.nj.nec.com/jard94general.html}
}
@InProceedings{JegMed+:1995:WSCT,
  author =   {R. Jegou and R. Medina and L. Nourine},
  title =    {{L}inear {S}pace {A}lgorithm for {O}n-line
                  {D}etection of {G}lobal {P}redicates},
  booktitle =    PROC # " " # WSCT,
  pages =        {175-189},
  year =     1995,
  editor =   {J. Desel},
  publisher =    SV
}
@InProceedings{JohZwa:1988:PODC,
  author =   {D. B. Johnson and W. Zwaenepoel},
  title =    {{R}ecovery in {D}istributed {S}ystems {U}sing
                  {O}ptimistic {M}essage {L}ogging and
                  {C}heckpointing},
  booktitle =    PROC # " 6th " # PODC,
  pages =    {171-181},
  year =     1988,
  month =    AUG
}
@Article{JohZwa:1990:JA,
  author =       {D. B. Johnson and W. Zwaenepoel},
  title =        {{R}ecovery in {D}istributed {S}ystems using {O}ptimistic {M}essage {L}ogging
                 and {C}heckpointing},
  journal =      JA,
  volume =       {11},
  number =       {3},
  month =        SEP,
  year =         {1990},
  pages =        {462-491},
}
@Article{Jou:2000:DC,
  author =       {Y.-J. Joung},
  title =        {{A}synchronous {G}roup {M}utual {E}xclusion},
  journal =      DC,
  volume =       {13},
  number =       {4},
  pages =        {189-206},
  year =         {2000},
}
@Article{Jou:2002:DC,
  author =       {Y.-J. Joung},
  title =        {{T}he {C}ongenial {T}alking {P}hilosophers {P}roblem in {C}omputer
                  {N}etworks},
  journal =       DC,
  pages =        {155-175},
  year =         {2002},
}
@Article{Jou:2003:TPDS,
  author =       {Y.-J. Joung},
  title =        {{Q}uorum-{B}ased {A}lgorithms for {G}roup {M}utual {E}xclusion},
  journal =      TPDS,
  pages =        {463-475},
  year =         {2003},
  volume =       {14},
  number =       {5},
  month =        MAY
}
@Article{KaeMoh:1978:SIAM,
  author =   {R. Kaerkes and R. H. M{\"o}hring},
  title =    {{V}orlesungen u{\"b}er {O}rdnungen und {N}etzplantheorie},
  journal =      {Schriften zur Informatik und Angewandten Mathematik 45, RWTH Aachen},
  year =     1978
}
@InProceedings{KanNao+:1988:STOC,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  booktitle =    PROC # " 20th " # STOC,
  pages =    {334-343},
  year =     1988,
  address =      {Chicago},
  month =    MAY
}
@Article{KanNao+:1992:SIAMJDM,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  journal =      SIAMJDM,
  year =     1992,
  volume =   5,
  number =   4,
  pages =    {596-603},
  month =    NOV
}
@InProceedings{KanWil+:2003:ICDCS,
  author =   {B. B. H. Kang and R. Wilensky and J, Kubiatowicz},
  title =    {{The Hash History Approach for Reconciling Mutual Inconsistency}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {670-677},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Providence, Rhode Island},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KeaMoi:1999:PODC,
  author =   {P. Keane and M. Moir},
  title =    {{A} {S}imple {L}ocal-{S}pin {G}roup {M}utual {E}xclusion {A}lgorithm},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PODC,
  pages =    {23-32},
  year =     {1999},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{KhoHam+:2003:JPDC,
  author =   {A. A. Khokhar and S. E. Hambrusch and E. Kocalar},
  title =    {{Termination Detection in Data-Driven Parallel Computations/Applications}},
  journal =      JPDC,
  year =     2003,
  volume =   63,
  number =   3,
  pages =    {312-326},
  month =    MAR
}
@Article{KilCha:1997:CJ,
  author =   {R. Kilgore and C. Chase},
  title =    {{T}esting {D}istributed {P}rograms {C}ontaining
                  {R}acing {M}essages},
  journal =  CJ,
  year =     1997,
  volume =   40,
  number =   8,
  pages =    {489-498},
  month =    NOV
}
@InProceedings{KilCha:1997:CSS,
  author =   {R. Kilgore and C. Chase},
  title =    {{R}e-execution of {D}istributed {P}rograms to
                  {D}etect {B}ugs {H}idden by {R}acing {M}essages},
  booktitle =    PROC # " " # CSS,
  pages =        {423-432},
  year =     1997,
  address =  {Hawaii},
  month =    JAN
}
@PhdThesis{KoChe:1996:Thesis,
  author =       {C. Ko and W. Cheuk},
  title =        {{Execution Monitoring Of Security Critical Programs in a Distributed
                   System: A Specification Based Approach}},
  year =         1996,
  school =       UCD
},
  month =        {August},
  year =         1997
}
@InProceedings{KoRed:2002:SP,
  author =   {C. Ko and T. Redmond},
  title =    {{Noninterference and Intrusion Detection}},
  year =     2002,
  booktitle =    PROC # " " # SP,
  pages =        {177-187},
  address =      {Berkeley, California},
  month =    MAY
}
@InProceedings{KocKho+:1999:PDC,
  author =   {E. Kocalar and A. A. Khokhar and S. E. Hambrusch},
  title =    {{T}ermination {D}etection: {M}odels and {A}lgorithms for {SPMD}
                  {C}omputing {P}aradigms},
  booktitle =    PROC # " " # PDC,
  year =     1999
}
@Book{Koh:1978:MH,
  author =   {Z. Kohavi},
  OPTeditor =    {~},
  title =    {{S}witching and {F}inite {A}utomata {T}heory},
  publisher =    MH,
  year =     1978,
  edition =  {2nd}
}
@Misc{KohGei:1995,
  OPTkey =   {},
  author =   {J. A. Kohl and G. A. Geist},
  title =    {{T}he {PVM 3.4} {T}racing {F}acility and {XPVM 1.1}},
  howpublished = {Computer Science and Mathematics Divison, Oak Ridge National Laboratory, TN, USA},
  OPTmonth =     {},
  year =     {1995},
  note =     {},
  OPTannote =    {}
}
@Article{KorFer:1992:AMCSJ,
  author =   {B. Korel and R. Ferguson},
  title =    {{Dynamic Slicing of Distributed Programs}},
  journal =  AMCSJ,
  year =     1992,
  volume =   2,
  number =   2,
  pages =    {199-215}
}
@Article{KorLas:1988:IPL,
  author =   {B. Korel and J. Laski},
  title =    {{Dynamic Program Slicing}},
  journal =  IPL,
  year =     1988,
  volume =   29,
  number =   3,
  pages =    {155-163}
}
@InProceedings{KorRil:1997:WAD,
  author =   {B. Korel and J. Rilling},
  title =    {{Application of Dynamic Slicing in Program Debugging}},
  booktitle =    PROC # " 3rd " # WAD,
  pages =    {43-57},
  year =     1997,
  editor =   {Mariam Kamkar},
  address =  {Link{\" o}ping, Sweden},
  month =    MAY
}
@Article{Ksh:1998:TCS,
  author =   {A. D. Kshemkalyani},
  title =    {{A Framework for Viewing Atomic Events in Distributed Computations}},
  journal =      TCS,
  year =     {1998},
  OPTkey =   {},
  volume =   {196},
  number =   {1-2},
  pages =    {45-70},
  month =    APR,
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KshSin:1990:SPDP,
  author =       {A. D. Kshemkalyani and M. Singhal},
  title =        {{Correct Two-phase and One-phase Deadlock Detection
                   Algorithms for Distributed Systems}},
  booktitle =    PROC # " " # SPDP,
  pages =        {126-129},
  month =        DEC,
  year =         {1990}
}
@Article{KunBla+:1997:CJ,
  author =   {T. Kunz and J. P. Black and D. J. Taylor and T. Basten},
  title =    {{POET}: {T}arget-{S}ystem {I}ndependent {V}isualizations of {C}omplex
                  {D}istributed-{A}pplications {E}xecutions},
  journal =      CJ,
  year =     {1997},
  OPTkey =   {},
  volume =   {40},
  number =   {8},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lai:1986:JPDC,
  author =   {T. H. Lai},
  title =    {{Termination Detection for Dynamic Distributed Systems with
                  Non-First-In-First-Out Communication}},
  journal =      JPDC,
  year =     {1986},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {577-599},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{LaiTse+:1992:IPPS,
  author =       {T.-H. Lai and Y.-C. Tseng and X. Dong},
  title =        {{A More Efficient Message-Optimal Algorithm for
                  Distributed Termination Detection}},
  booktitle =    PROC # " 6th " # IPPS,
  year =         {1992},
  pages =        {646--649},
  publisher = {IEEE Computer Society},
}
@Article{LaiWu:1995:TPDS,
  author =   {T.-H. Lai and L.-F. Wu},
  title =    {{An $(N -1)$-Resilient Algorithm for Distributed Termination Detection}},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   1,
  pages =    {63-78}
}
@Article{LaiYan:1987:IPL,
  author =   {T.-H. Lai and T. H. Yang},
  title =    {{On Distributed Snapshots}},
  journal =      IPL,
  year =     {1987},
  OPTkey =   {},
  volume =   {25},
  number =   {3},
  pages =    {153-158},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1974:CACM,
  author =   {L. Lamport},
  title =    {{A New Solution of Dijkstra's Concurrent Programming Problem}},
  journal =      CACM,
  year =     {1974},
  OPTkey =   {},
  volume =   {18},
  number =   {8},
  pages =    {453-455},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1978:CACM,
  author =   {L. Lamport},
  title =    {{T}ime, {C}locks, and the {O}rdering of {E}vents in
                  a {D}istributed {S}ystem},
  journal =  CACM,
  year =     1978,
  volume =   21,
  number =   7,
  pages =    {558-565},
  month =    JUL
}
@Article{LanBul+:1994:CS,
  author =   {C. E. Landwehr and A. R. Bull and J. P. McDermott and W. S. Choi},
  title =    {{A} {T}axonomy of {C}omputer {P}rogram {S}ecurity {F}laws},
  journal =      CS,
  year =     1994,
  volume =   26,
  number =   3,
  pages =    {211-254},
  issn =         {0360-0300}
}
@Article{Law:1976:MCT,
  author =   {E. L. Lawler},
  title =    {{G}raphical {A}lgorithms and their {C}omplexity},
  journal =      MCT,
  year =     1976,
  volume =   81,
  pages =    {3-32}
}
@Article{LebMel:1987:TC,
  author =   {T. J. LeBlanc and J. M. Mellor-Crummey},
  title =    {{D}ebugging {P}rograms with {I}nstant {R}eplay},
  journal =  TC,
  year =     1987,
  volume =   {C-36},
  number =   4,
  pages =    {471-482},
  month =    APR
}
@Article{MadWes:1991:DM,
  author =   {T. Madej and D. B. West},
  title =    {{T}he {I}nterval {I}nclusion {N}umber of a {P}artially {O}rdered {S}et},
  journal =      DM,
  year =     1991,
  volume =   88,
  pages =    {259-277},
  note =     ES
}
@Article{Mae:1985:TrCS,
  author =       {M. Maekawa},
  title =        {{A}lgorithm for {M}utual {E}xclusion in {D}ecentralized {S}ystem},
  journal =      TrCS,
  pages =        {145-159},
  year =         {1985},
  volume =       {3},
  number =       {2},
  month =        MAY,
  OPTorganization = {ACM}
}
@Book{Mae:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  OPTeditor =    {},
  title =    {{Operating Systems Advanced Concepts}},
  publisher =    BCPC,
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Menlo Park, California},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{MaeOld+:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  title =    {{O}perating {S}ystems {A}dvanced {C}oncepts},
  publisher =    BCPC,
  year =     1987,
  address =      {Menlo Park, California}
}
@Article{MagWel+:1981:TCS,
  author =   {A. Maggiolo-Schettini and H. Welde and J. Winkowski},
  title =    {{M}odeling a {S}olution for a {C}ontrol {P}roblem in
                  {D}istributed {S}ystems by {R}estrictions},
  journal =  TCS,
  year =     1981,
  volume =   13,
  number =   1,
  pages =    {61-83},
  month =    JAN
}
@Unpublished{MahDut:2004:JPDC,
  author =   {N. R. Mahapatra and S. Dutt},
  title =    {{An Efficient Delay-Optimal Distributed Termination Detection Algorithm}},
  note =     "To Appear in " # JPDC,
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2004},
  OPTannote =    {}
}
@Misc{Man:Rdist,
   title =      {{Man pages: Rdist - Remote File Distribution Program}},
   organization = {Sun Microsystems}
}
@article{ManIma:1992:JPDC,
  author =       {Y. Manabe and M. Imase},
  title =        {{G}lobal {C}onditions in {D}ebugging {D}istributed {P}rograms},
  journal =      JPDC,
  volume =       {15},
  number =       {1},
  pages =        {62-69},
  year =         {1992}
}
@InProceedings{MarNei:1991:WDAG,
  author =       {K. Marzullo and G. Neiger},
  title =        {{D}etection of {G}lobal {S}tate {P}redicates},
  booktitle =    PROC # " " # WDAG,
  pages =        {254-272},
  year =         {1991}
}
@Article{MarSab:1994:DC,
  author = {K. Marzullo and L. Sabel},
  title = {{E}fficient {D}etection of a {C}lass of {S}table {P}roperties},
  journal = DC,
  volume = {8},
  number = {2},
  pages = {81-91},
  year = {1994},
  url = "citeseer.nj.nec.com/marzullo94efficient.html"
}
@Article{Mat:1987:DC,
  author =   {F. Mattern},
  title =    {{Algorithms for Distributed Termination Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {161-175},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Mat:1989:IPL,
  author =   {F. Mattern},
  title =    {{Global Quiescence Detection based on Credit Distribution
                   and Recovery}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {195-200},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Mat:1989:WDAG,
  author =   {F. Mattern},
  title =    {{Virtual Time and Global States of Distributed Systems}},
  booktitle =    "Parallel and Distributed Algorithms: " # PROC # " "
                  # WDAG,
  pages =    {215-226},
  year =     1989,
  publisher =    ES
}
@Article{Mat:1993:JPDC,
  author =       {F. Mattern},
  title =        {{E}fficient {A}lgorithms for {D}istributed {S}napshots and {G}lobal
                  {V}irtual {T}ime {A}pproximation},
  journal =      JPDC,
  volume =       {18},
  number =       {4},
  pages =        {423-434},
  year =         {1993},
  url =          {http://citeseer.nj.nec.com/mattern93efficient.html}
}
@Article{MatCap:1999:JSS,
  author =   {J. Matocha and T. Camp},
  title =    {{A Taxonomy of Distributed Termination Detection Algorithms}},
  journal =      JSS,
  year =     1999,
  volume =   43,
  number =   3,
  pages =    {207-221},
  month =    NOV
}
@Techreport{MatMeh+:1991:TR:32,
  author =       {F. Mattern and H. Mehl and A. Schoone and G. Tel},
  title =        {{Global Virtual Time Approximation with Distributed
                  Termination Detection Algorithms}},
  institution =  {University of Utrecht, The Netherlands},
  number =       {RUU-CS-91-32},
  year =         {1991},
  url =          {http://citeseer.nj.nec.com/mattern91global.html}
}
@Manual{MatMel+:1997:ISO,
  author =   {N. Mattos and J. Melton and J. Richey},
  title =    {Database Language SQL - Part 9: Management of
                  External Data (SQL/MED)},
  organization = {ISO working draft},
  month =    JUN,
  year =     1997
}
@InProceedings{McMLi:1993:COMPSAC,
  author =   {P. Li and B. McMillin},
  title =    {{Fault-Tolerant Distributed Deadlock Detection/Resolution}},
  booktitle =    PROC # " 17th " # COMPSAC,
  pages =    {224-230},
  year =     1993,
  month =    NOV
}
@InProceedings{MilCho:1988:ICDCS,
  author =   {B. P. Miller and J. Choi},
  title =    {{B}reakpoints and {H}alting in {D}istributed
                  {P}rograms},
  booktitle =    PROC # " 8th " # ICDCS,
  pages =    {316-323},
  year =     1988
}
@InProceedings{Mis:1983:PODC,
  author =   {J. Misra},
  title =    {{Detecting Termination of Distributed Computations using Markers}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  pages =    {290-294},
  year =     {1983},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@PhdThesis{Mit:2002:Thesis,
  author =       {N. Mittal},
  title =        {{T}echniques for {A}nalyzing {D}istributed {C}omputations},
  school =       UTA,
  year =         2002,
  month =        MAY,
  note =         {Available at \texttt{http://www.utdallas.edu/{\symbol{126}}neerajm}}
}
@InProceedings{MitGar:1998:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  booktitle =    PROC # " 18th " # ICDCS,
  pages =    {582-589},
  year =     {1998},
  address =      {Amsterdam, The Netherlands},
  month =    MAY
}
@TechReport{MitGar:1998:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     1998,
  number =   {TR-PDS-1998-005},
  address =      {Austin, TX 78712}
}
@InProceedings{MitGar:2000:PODC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  booktitle =    PROC # " 19th " # PODC,
  pages =    {239-248},
  year =     2000,
  address =  {Portland, Oregon},
  month =    JUL
}
@TechReport{MitGar:2000:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2000,
  number =   {TR-PDS-2000-002},
  address =  {Austin, TX 78712},
  month =    MAY
}
@InProceedings{MitGar:2001:DISC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  booktitle =    PROC # " " # DISC,
  pages =    {78-92},
  year =     2001,
  address =      {Lisbon, Portugal},
  month =    OCT
}
@InProceedings{MitGar:2001:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{On Detecting Global Predicates in Distributed Computations}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {3-10},
  year =     2001,
  address =      {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at
                  \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@TechReport{MitGar:2001:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2001,
  number =   {TR-PDS-2001-002},
  OPTaddress =   {Austin, TX 78712},
  month =    APR,
  note =         {Available at \texttt{http://www.cs.utexas.edu/users/neerajm}}
}
@TechReport{MitGar:2001:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{A Rigorous Proof of $O(n^2)$ Bound on the Number of Moves
                  for Stabilization of Dijkstra's 3-State Algorithm}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2001-005},
  address =      {Austin, TX 78712},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitGar:2003:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Software Fault Tolerance of Distributed Programs using Computation Slicing}},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {105-113},
  year =     2003,
  address =  {Providence, Rhode Island},
  month =    MAY
}
@TechReport{MitGar:2003:TR:15,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Techniques and Applications of Computation Slicing}},
  institution =  DCS # ", " # UTD,
  year =     2003,
  number =   {UTDCS-15-03},
  OPTaddress =   {Richardson, TX 75083},
  month =    APR
}
@Article{MitGar:2004:DC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Finding Missing Synchronization in a Distributed Computation using
                  Controlled Re-execution}},
  journal =      DC,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  month =    MAR,
  note =     {Online First},
  OPTannote =    {}
}
@InProceedings{MitHsi:2000:ICDE,
  author =   {N. Mittal and H. Hsiao},
  title =    {{D}atabase {M}anaged {E}xternal {F}ile {U}pdate},
  booktitle =    PROC # " 17th " # ICDE,
  pages =    {557-564},
  year =     2001,
  address =  {Heidelberg, Germany},
  month =    APR
}
@InProceedings{MitSen+:2004:IPDPS,
  author =   {N. Mittal and A. Sen and V. K. Garg and R. Atreya},
  title =    {{Finding Satisfying Global States: All for One and One for All}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # IPDPS,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    APR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitVen+:2004:DISC,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  booktitle =    PROC # " " # DISC,
  pages =        {290-304},
  year =     2004,
  address =      {Amsterdam, The Netherlands},
  month =    OCT
}
@TechReport{MitVen+:2004:TR,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  institution =  UTD,
  number =       {UTDCS-08-04},
  month =        FEB,
  year =     2004,
  note =     {Available at
                  \texttt{http://www.utdallas.edu/{\textasciitilde}neerajm/}}
}
@InProceedings{MurGar:1997:ICDCS,
  author =   {V. V. Murty and V. K. Garg},
  title =    {{C}haracterization of {M}essage {O}rdering
                  {S}pecifications and {P}rotocols},
  booktitle =    PROC # " 17th " # ICDCS,
  year =     1997,
  month =    MAY
}
@Article{Nas:1961:JLMS,
  author =   {C. Nash-Williams},
  title =    {{E}dge-{D}isjoint {S}panning {T}rees of {F}inite {G}raphs},
  journal =      JLMS,
  year =     1961,
  volume =   36,
  pages =    {445-450}
}
@InProceedings{NetBre+:1996:SPDT,
  author =   {R. Netzer and T. Brennan and S. Damodaran-Kamal},
  title =    {{D}ebugging {R}ace {C}onditions in
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " " # SPDT,
  pages =    {31-40},
  year =     1996,
  month =    MAY
}
@Article{NetMil:1995:JS,
  author =   {R. H. B. Netzer and B. P. Miller},
  title =    {{O}ptimal {T}racing and {R}eplay for {D}ebugging
                  {M}essage-{P}assing {P}rograms},
  journal =  JS,
  year =     1995,
  volume =   8,
  number =   4,
  pages =    {371-388}
}
@Article{NetXu:1995:TPDS,
  author =   {R. H. B. Netzer and J. Xu},
  title =    {{N}ecessary and {S}ufficient {C}onditions for {C}onsistent
                  {G}lobal {S}napshots},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   2,
  pages =    {165-169},
  month =    FEB
}
@Unpublished{POTAwebsite,
  author =   {A. Sen and V. K. Garg},
  title =    {{P}artial {O}rder {T}race {A}nalyzer {(POTA)}},
  note =     {http://maple.ece.utexas.edu/{\textasciitilde}sen/POTA.html},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}
@Article{PapWas+:1999:SIGMOD,
  author =   {M. Papiani and J. Wason and A. Dunlop and D. Nicole},
  title =    {{A} {D}istributed {S}cientific {A}rchive {U}sing the
                  {W}eb, {XML} and {SQL}/{MED}},
  journal =  {SIGMOD Record},
  volume =   {28},
  number =   {3},
  pages =    {56-62},
  month =    SEP,
  year =     {1999}
}
@Article{ParPop+:1983:TSE,
  author =   {D. S. Parker and G. J. Popek and G. Rudisin and A. Stoughton
                  and B. J. Walker and E. Walton and J. M. Chow and D. A. Edwards
                  and S. Kiser and C. S. Kline},
  title =    {{Detection of Mutual Inconsistency in Distributed Systems}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {240-247},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PerMit:2004:PDCS,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  booktitle =    PROC # " " # PDCS,
  pages =        {209-215},
  year =     2004,
  address =      {San Francisco, California},
  month =    SEP
}
@TechReport{PerMit:2004:TR,
  author =   {S. Peri and N. Mittal},
  title =    {{An Efficient Snapshot Protocol for a Dynamic System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{PerMit:2004:TR:15,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-15-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PlaBec+:1995:UWTC,
  author =   {J. S. Plank and M. Beck and G. Kingsley},
  title =    {{Libckpt: Transparent Checkpointing under UNIX}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # UWTC,
  pages =    {213-223},
  year =     {1995},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New Orleans, Louisiana},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Misc{Pom:2000:TUT,
  OPTkey =   {},
  author =   {W. Torres-Pomales},
  title =    {{S}oftware {F}ault {T}olerance: {A} {T}utorial},
  OPThowpublished = {},
  OPTmonth =     {},
  year =     {2000},
  note =     {NASA Langley Research Center},
  OPTannote =    {}
}
@InProceedings{PraSin:1994:SPDP,
  author =   {R. Prakash and M. Singhal},
  title =    {{Maximal Global Snapshot with Concurrent Initiators}},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {344-351},
  year =     1994,
  address =      {Dallas, Texas},
  month =    OCT
}
@InProceedings{QueSif:1982:ISP,
  author =       {J. P. Queille and J. Sifakis},
  title =        {{S}pecification and {V}erification of {C}oncurrent {S}ystems in {CESAR}},
  address =      {New York},
  booktitle =    PROC # " 5th " # ISP,
  pages =        {337-351},
  publisher =    SV,
  series =       LNCS,
  volume =       137,
  year =         1982
}
@Article{Ran:1983:IPL,
  author =   {S. P. Rana},
  title =    {{A Distributed Solution of the Distributed Termination
                   Problem}},
  journal =      IPL,
  year =     {1983},
  OPTkey =   {},
  volume =   {17},
  number =   {1},
  pages =    {43-46},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{RaoAlv+:2000:KDE,
  author =       {S. Rao and L. Alvisi and H. Vin},
  title =        {{T}he {C}ost of {R}ecovery in {M}essage {L}ogging {P}rotocols},
  journal =      KDE,
  volume =       {12},
  number =       {2},
  year =         {2000},
  pages =        {160-173},
}
@Book{Ray:1988:JWS,
  author =       {M. Raynal},
  title =        {{D}istributed {A}lgorithms and {P}rotocols},
  publisher =    JWS,
  year =         {1988}
}
@Article{Ray:1989:TrCS,
  author =   {K. Raymond},
  title =    {{A} {T}ree based {A}lgorithm for {D}istributed {M}utual {E}xclusion},
  journal =      TrCS,
  year =     1989,
  volume =   7,
  number =   1,
  pages =    {61-77}
}
@Article{RicAgr:1981:CACM,
  author =       {G. Ricart and A. K. Agrawala},
  title =        {{An Optimal Algorithm for Mutual Exclusion in Computer Networks}},
  journal =      CACM,
  volume =       {24},
  number =       {1},
  year =         {1981},
  pages =        {9-17},
  publisher =    {ACM Press},
  month =        JAN,
}
@Article{Riv:1974:AMS,
  author =   {I. Rival},
  title =    {{M}aximal {S}ublattices of {F}inite {D}istributive {L}attices {II}},
  journal =      PROC # " " # AMS,
  year =     1974,
  volume =   44,
  number =   2,
  pages =    {263-268}
}
@Book{STA,
  author =       {R. Stanley},
  title =        {{E}numerative {C}ombinatorics {V}olume 1},
  publisher =    {Wadsworth and Brookes/Cole},
  address =      {Monterey, California},
  year =         1986
}
@Unpublished{SafDij:1987:998,
  author =   {E. W. Dijkstra},
  title =    {{Shmuel Safra's Version of Termination Detection}},
  note =     {EWD Manuscript 998. Available at \texttt{http://www.cs.utexas.edu/users/EWD}},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1987},
  OPTannote =    {}
}
@TechReport{Sai:2002:TR:51,
  author =   {Y. Saito},
  title =    {{Unilateral Version Vector Pruning using Loosely Synchronized Clocks}},
  institution =  HPL,
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {HPL-2002-51},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{SchGet:1987:TOG,
  author =       {R.W. Scheifler and J. Gettys},
  title =        {{The X Window System}},
  journal =      TOG,
  month =        APR,
  year =         1987,
  volume =       5,
  number =       2,
  pages =        {79-109}
}
@Article{SchMat:1994:DC,
  author =   {R. Schwartz and F. Mattern},
  title =    {{D}etecting {C}ausal {R}elationships in {D}istributed  {C}omputations:
                  {I}n {S}earch of the {H}oly {G}rail},
  journal =      DC,
  year =     1994,
  volume =   7,
  number =   3,
  pages =    {149-174}
}
@InProceedings{SchWyl:1991:SOSP,
  author =   {F. Schmuck and J. Wyllie},
  title =    {{Experience with Transactions in QuickSilver}},
  booktitle =    PROC # " 13th " # SOSP,
  pages =    {239-253},
  year =     1991,
  month =    OCT
}
@InProceedings{SenGar:2002:IPDPS,
  author =   {A. Sen and V. K. Garg},
  title =    {{D}etecting {T}emporal {L}ogic {P}redicates in the {H}appened-{B}efore {M}odel},
  booktitle =    PROC # " " # IPDPS,
  year =     2002,
  address =      {Florida},
  month =    APR
}
@TechReport{SenGar:2002:TR:001,
  author =   {A. Sen and V. K. Garg},
  title =    {{A}utomatic {G}eneration of {C}omputation {S}lices for
                  {D}etecting {T}emporal {L}ogic {P}redicates},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2003-001},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{SenGar:2003:OPODIS,
  author =       {A. Sen and V. K. Garg},
  title =        {{Detecting Temporal Logic Predicates in Distributed
                   Programs using Computation Slicing}},
  booktitle =    PROC # " " # OPODIS,
  OPTpages =     {},
  month =        DEC,
  year =         {2003}
}
@InProceedings{SenGar:2003:RV,
  author =       {A. Sen and V. K. Garg},
  title =        {{P}artial {O}rder {T}race {A}nalyzer ({POTA}) for
                  {D}istributed {P}rograms},
  booktitle =    PROC # " Third " # RV,
  OPTseries =    {Electronic Notes in Theoretical Computer Science},
  volume =       {89},
  issue =        {2},
  publisher =    {Elsevier},
  year =         {2003}
}


@InProceedings{ShaFra:1986:ICALP,
  author =   {N. Shavit and N. Francez},
  title =    {{A New Approach to Detection of Locally Indicative Stability}},
  booktitle =    PROC # " " # ICALP,
  pages =    {344-358},
  year =     1986,
  address =      {Rennes, France}
}


@TechReport{ShaTou:1984:TR:624,
  author =   {A. Shah and S. Toueg},
  title =    {{Distributed Snapshots in spite of Failures}},
  institution =  DCS # ", " # CORNELL,
  year =     1984,
  number =   {TR84-624},
  address =      {Ithaca, NY},
  month =    JUL,
  note =     {(Revised February 1985)}
}


@InProceedings{SheDea:2002:WETICE,
  author =       {J. S. Sherif and T. G. Dearmond},
  title =        {{Intrusion Detection: Systems and Models}},
  booktitle =    PROC # " " # WETICE,
  pages =        {115-136},
  month =        JUN,
  year =         {2002},
  address =      {Pittsburgh, Pennsylvania}
}


@Book{SinShi:1994:Book,
  author =       {M. Singhal and N. G. Shivaratri},
  title =        {{Advanced Concepts in Operating Systems}},
  publisher =    MH # " and " # MIT,
  year =         {1994},
  ISBN =         {0-07-057572-X}
}

@InProceedings{SkaMit+:1999:PDCS,
  author =   {C. Skawratananond and N. Mittal and V. K. Garg},
  title =    {{A} {L}ightweight {A}lgorithm for {C}ausal {M}essage
                  {O}rdering in {M}obile {C}omputing {S}ystems},
  booktitle =    PROC # " 12th " # PDCS,
  pages =    {245-250},
  year =     {1999},
  address =      {Florida}
}


@Unpublished{SolDes,
  author =   {Solar Designer},
  title =    {{Root Programs and Links}},
  note =     {Available at \texttt{http://www.openwall.com/linux/}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@Unpublished{SolDes:OP,
  author =   {Openwall Project},
  title =    {{Linux Kernel Patch}},
  note =     {\textsf{http://www.openwall.com/linux}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@InProceedings{SpeKea:1986:ICDCS,
  author =   {M. Spezialetti and P. Kearns},
  title =    {{Efficient Distributed Snapshots}},
  booktitle =    PROC # " 6th " # ICDCS,
  pages =    {382-388},
  year =     1986
}


@Article{SpiBra:1987:DAM,
  author =   {J. Spinrad and A. Brandstadt and L. Stewart},
  title =    {{Bipartite Permutation Graphs}},
  journal =      DAM,
  year =     1987,
  volume =   18,
  pages =    {279-292}
}



@InProceedings{SriSiv:2002:ICPDCS,
  author =   {N. Sridhar and P. A. G. Sivilotti},
  title =    {{L}azy {S}napshots},
  booktitle =    PROC # " 14th " # ICPDCS,
  pages =    {96-101},
  year =     {2002},
  OPTeditor =    {S.G. Akl and T.Gonzalez},
  address =      {Cambridge, MA},
  month =    NOV,
  OPTorganization = {IASTED},
  OPTpublisher =    {ACTA Press},
  OPTurl =          {http://citeseer.nj.nec.com/sridhar02lazy.html}
}



@InProceedings{SroSch+:1998:WNTS,
  author =   {J. Srouji and P. Schuster and M. Bach and Y. Kuzmin},
  title =    {{A Transparent Checkpoint Facility on NT}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 2nd " # WNTS,
  OPTpages =     {},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Seattle, Washington},
  month =    {August},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Sta:2001:PH,
  author =   {W. Stallings},
  title =    {{O}perating {S}ystems: {I}nternals and {D}esign {P}rinciples},
  publisher =    PH,
  year =     2001
}




@InCollection{StoLiu:1998:CAV,
  author =   {S. D. Stoller and Y. A. Liu},
  title =    {{E}fficient {S}ymbolic {D}etection of {G}lobal
                  {P}roperties in {D}istributed {S}ystems},
  booktitle =    PROC # " 10th " # CAV,
  pages =    {357-368},
  publisher =    {Springer-Verlag},
  year =     1998,
  editor =   {Alan J. Hu and Moshe Y. Vardi},
  volume =   1427,
  series =   LNCS
}



@InProceedings{StoSch:1995:WDAG,
  author =   {S. D. Stoller and F. Schneider},
  title =    {{F}aster {P}ossibility {D}etection by {C}ombining
                  {T}wo {A}pproaches},
  booktitle =    PROC # " " # WDAG,
  pages =        {318-332},
  year =     1995,
  volume =       {972},
  series =       LNCS,
  address =  {France},
  month =    SEP
}


@InProceedings{StoUnn+:2000:CAV,
  author =   {S. D. Stoller and L. Unnikrishnan and Y. A. Liu},
  title =    {{Efficient Detection of Global Properties in
                  Distributed Systems Using Partial-Order Methods}},
  booktitle =    PROC # " 12th " # CAV,
  pages =    {264-279},
  year =     2000,
  volume =   1855,
  series =   LNCS,
  month =    JUL,
  publisher =    {Springer-Verlag}
}



@InProceedings{Stu:2002:DISC,
  author =   {G. Stupp},
  title =    {{Stateless Termination Detection}},
  booktitle =    PROC # " 16th " # DISC,
  pages =    {163-172},
  year =     2002,
  address =      {Toulouse, France}
}


@InProceedings{Tai:1997:ICDCS,
  author =   {K. Tai},
  title =    {{R}ace {A}nalysis of {T}races of {A}synchronous
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " 17th " # ICDCS,
  pages =    {261-268},
  year =     1997
}



@PhdThesis{Tar:2000:Thesis,
  author =   {A. Tarafdar},
  title =    {{S}oftware {F}ault {T}olerance in {D}istributed {S}ystems
                  {U}sing {C}ontrolled {R}e-execution},
  school =   {The University of Texas at Austin},
  year =     2000,
  month =    AUG
}


@InProceedings{TarGar:1998:ICDCS,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{A}ddressing {F}alse {C}ausality while {D}etecting
                  {P}redicates in {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # ICDCS,
  pages =    {94-101},
  year =     1998,
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}

@InProceedings{TarGar:1998:SPDP,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{P}redicate {C}ontrol for {A}ctive {D}ebugging of
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # SPDP,
  pages =        {763-769},
  year =     1998,
  address =  {Orlando}
}

@InProceedings{TarGar:1999:DISC,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{S}oftware {F}ault {T}olerance of {C}oncurrent
                  {P}rograms {U}sing {C}ontrolled {R}e-execution},
  booktitle =    PROC # " 13th " # DISC,
  pages =    {210-224},
  year =     1999,
  address =  {Bratislava, Slovak Republic},
  month =    SEP
}


@Book{Tel:2000:CUP,
  author =   {G. Tel},
  title =    {{Introduction to Distributed Algorithms}},
  publisher =    CUP # "~(US Server)",
  year =     2000,
  edition =      {Second},
  month =    SEP
}

@Article{TelMat:1993:TOPLAS,
  author =   {G. Tel and F. Mattern},
  title =    {{The Derivation of Distributed Termination Detection Algorithms from Garbage Collection Schemes}},
  journal =      TOPLAS,
  year =     1993,
  volume =   15,
  number =   1,
  pages =    {1-35},
  month =    JAN
}



@Article{Tip:1995:JPL,
  author =   {F. Tip},
  title =    {{A Survey of Program Slicing Techniques}},
  journal =      JPL,
  year =     1995,
  volume =   3,
  number =   3,
  pages =    {121-189}
}

@InProceedings{TomGar:1993:WPDS,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{An Algorithm for Minimally Latent Global Virtual Time}},
  booktitle =    PROC # " 7th " # WPDS,
  pages =        {35-42},
  year =     1993,
  address =  {San Diego, California},
  month =    MAY
}


@InProceedings{TomGar:1994:CSE,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{Maintaining Global Assertions in Distributed Systems}},
  booktitle =    CSE,
  pages =    {257-272},
  year =     1994,
  publisher =    TMH
}


@Article{TomGar:1994:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@InProceedings{TomGar:1995:FSTTCS,
  author =       {A. I. Tomlinson and V. K. Garg},
  title =        {{Observation of Software for Distributed Systems with RCL}},
  booktitle =    PROC # " 15th " # FSTTCS,
  pages =        {195-209},
  year =         {1995},
  url =          {http://citeseer.nj.nec.com/tomlinson95observation.html}
}

@Article{TomGar:1997:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {2},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@Book{Tro:1992:JHUP,
  author =   {W. T. Trotter},
  title =    {{C}ombinatorics and {P}artially {O}rdered {S}ets: {D}imension {T}heory},
  publisher =    JHUP,
  year =     1992,
  address =      {Baltimore, MD}
}

@article{Tse:1995:JPDC,
  author =       {Y.-C. Tseng},
  title =        {{Detecting Termination by Weight-Throwing in a Faulty Distributed System}},
  journal =      JPDC,
  volume =       {25},
  number =       {1},
  pages =        {7-15},
  year =         "1995",
  OPTnote =      "previous label was Tse:1992:JPDC"
}

@Article{TseTan:2001:TPDS,
  author =       {Y.-C. Tseng and C.-C. Tan},
  title =        {{On Termination Detection Protocols in a Mobile Distributed
                   Computing Environment}},
  journal =      TPDS,
  year =         2001,
  volume =       12,
  number =       6,
  pages =        {558-566}
}


@InProceedings{TsyYee:2003:USS,
  author =   {E. Tsyrklevich and B. Yee},
  title =    {{Dynamic Detection and Prevention of Race Conditions in File Accesses}},
  booktitle =    PROC # " 12th " # USS,
  pages =    {243-255},
  year =     2003,
  month =    AUG
}

@Article{Tur:1984:DAM,
  author =   {G. Turan},
  title =    {{Succinct Representations of Graphs}},
  journal =      DAM,
  year =     1984,
  volume =   8,
  pages =    {289-294}
}

@Book{Vah:1996:PH,
  author =   {U. Vahalia},
  title =    {Unix Internals: The New Frontiers},
  publisher =    PH,
  year =     1996,
  month =    JAN
}

@Article{ValTar+:1982:SIAMJC,
  author =   {J. Valdes and R. E. Tarjan and E. L. Lawler},
  title =    {{T}he {R}ecognition of {S}eries-{P}arallel {D}igraphs},
  journal =      SIAMJC,
  year =     1982,
  volume =   11,
  pages =    {298-314}
}

@Article{Ven:1989:TR,
  author =   {S. Venkatesan},
  title =    {{Reliable Protocols for Distributed Termination Detection}},
  journal =      TR,
  year =     1989,
  volume =   38,
  number =   1,
  pages =    {103-110},
  month =    APR
}




@Article{Ven:1995:TOPLAS,
  author =   {G. Venkatesh},
  title =    {{Experimental Results from Dynamic Slicing of C Programs}},
  journal =      TOPLAS,
  year =     1995,
  volume =   17,
  number =   2,
  pages =    {197-216}
}







@Article{SuzKas:1985:TrCS,
  author =   {I. Suzuki and T. Kasami},
  title =    {{A Distributed Mutual Exclusion Algorithm}},
  journal =      TrCS,
  year =     1985,
  volume =   3,
  number =   4,
  pages =    {344-349}
}



@Article{VenDat:1995:TSE,
  author =   {S. Venkatesan and B. Dathan},
  title =    {{T}esting and {D}ebugging {D}istributed {P}rograms {U}sing
                  {G}lobal {P}redicates},
  journal =      TSE,
  year =     1995,
  volume =   21,
  number =   2,
  pages =    {163-177},
  month =    FEB
}


@InProceedings{VieBlo+:2000:CSAC,
  author =   {J. Viega, J. Bloch, T. Kohno and G. McGraw},
  title =    {{ITS4: A Static Vulnerability Scanner for C and C++ Code}},
  booktitle =    PROC # " " # CSAC,
  year =     2000,
  month =    DEC
}


@InProceedings{WalGar:1991:WPDD,
  author =       {B. Waldecker and V. K. Garg },
  title =        {{U}nstable {P}redicate {D}etection in {D}istributed
                  {P}rogram {D}ebugging},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  pages =        {276-278},
  month =    MAY,
  year =     1991
}

@Article{Wan:1997:TC,
  author =   {Y.-M. Wang},
  title =    {{C}onsistent {G}lobal {C}heckpoints that {C}ontain a
                  {G}iven {S}et of {L}ocal {C}heckpoints},
  journal =      TC,
  year =     1997,
  volume =   46,
  number =   4,
  pages =    {456-468},
  month =    APR
}


@InProceedings{WanDam+:1997:ICDCS,
  author =       {Y. M. Wang and O. P. Damani and V. K. Garg},
  title =        {{D}istributed {R}ecovery with {K}-{O}ptimistic Logging},
  pages =        {60-67},
  booktitle =    PROC # " 17th " # ICDCS,
  address =      {Baltimore, Maryland},
  month =        JUN,
  publisher =    {IEEE},
  address =  {Washington - Brussels - Tokyo},
  year =         1997,
}



@Article{WanHua+:1997:TC,
  author =   {Y.-M. Wang and Y. Huang and W. K. Fuchs and
                  C. Kintala and G. Suri},
  title =    {{P}rogressive {R}etry for {S}oftware {F}ailure
                  {R}ecovery in {M}essage-{P}assing {A}pplications},
  journal =  TC,
  year =     1997,
  volume =   46,
  number =   10,
  pages =    {1137-1141},
  month =    OCT
}



@InProceedings{WanMay:2004:IPDPS,
  author =   {X. Wang and J. Mayo},
  title =    {{A General Model for Detecting Termination in Dynamic Systems}},
  booktitle =    PROC # " 18th " # IPDPS,
  year =     2004,
  address =      {Santa Fe, New Mexico},
  month =    APR
}


@Article{Wei:1982:CACM,
  author =   {M. Weiser},
  title =    {{P}rogrammers {U}se {S}lices when {D}ebugging},
  journal =  CACM,
  year =     1982,
  volume =   25,
  number =   7,
  pages =    {446-452}
}

@Article{WuJou:2000:CDS,
  author =   {K.-P. Wu and Y.-J. Joung},
  title =    {{Asynchronous Group Mutual Exclusion in Ring Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  journal =      CDS,
  pages =    {1-8},
  year =     {2000},
  OPTeditor =    {},
  volume =   {147},
  number =   {1}
}



@Article{Yan:1982:SIAMHADM,
  author =   {M. Yannakakis},
  title =    {{T}he {C}omplexity of the {P}artial {O}rder {D}imension {P}roblem},
  journal =      SIAMJADM,
  year =     1982,
  volume =   3,
  pages =    {351-358}
}




@InProceedings{ZibGil:1997:OOPSLA,
  author =   {Y. Zibin and Y. Gil},
  title =    {{E}fficient {S}ubtyping {T}ests with {PQ}-{E}ncoding},
  booktitle =    PROC # " 16th Annual " # OOPSLA,
  pages =    {96-107},
  year =     1997,
  address =      {Tampa Bay, Florida},
  month =    OCT
}

@Manual{iFS:1999,
  author =   {Oracle},
  title =    {iFS: Oracle Internet File System},
  note =     {\\ {\sf
                  http://www.oracle.com/database/options/ifs.html}},
  year =     1999
}

@InProceedings{WuLai+:1992:ICPADS,
  author =   {L.-F. Wu and T.-H. Lai and Y.-C. Tseng},
  title =    {{Consensus and Termination Detection in the Presence of Faulty Processes}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPADS,
  pages =    {267-274},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Hsinchu, Taiwan},
  month =    DEC,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{DwoLyn+:1988:JACM,
  author =       {C. Dwork and N. Lynch and L. Stockmeyer},
  title =        {{Consensus in the presence of partial synchrony}},
  OPTcrossref =  "",
  OPTkey =       "",
  journal =      JACM,
  year =         "1988",
  volume =       "35",
  number =       "2",
  pages =        {288-323},
  month =        APR,
  OPTnote =      "",
  annote =       "The authors study practically motivated models of
                  synchrony that lie between fully asynchronous and
                  fully synchronous systems in which consensus shall
                  be achieved. The models of partial synchrony studied
                  include: (1) upper bounds on processor speeds and
                  message latency exist but are unknown, and (2) upper
                  bounds exists and are known, but only hold after
                  some unknown time (eventually). In both cases
                  consensus with different resiliency can be achieved."
}


@InProceedings{DelFau+:2004:PODC,
  author =   {C. Delporte-Gallet and H. Fauconnier and R. Guerraoui and
                  V. Hadzilacos and P. Kouznetsov and S. Toueg},
  title =    {{The Weakest Failure Detector to Solve Certain Fundamental Problems
                   in Distributed Computing}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {St. Johns, Newfoundland, Canada},
  month =    JUL,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{MitGae+:2004:TR:37,
  author =   {N. Mittal and F. G{\"a}rtner and S. Venkatesan and L. D. Penso},
  title =    {{ Detecting Termination in a Crash-Prone Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-37-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{HurMiz+:1998:TSE,
  author =       {M. Hurfin and M. Mizuno and M. Singhal and M. Raynal},
  title =        {Efficient Distributed Detection of Conjunctions of Local Predicates},
  journal =      TSE,
  volume =       {24},
  number =       {8},
  year =         {1998},
  issn =         {0098-5589},
  pages =        {664--677},
  doi =          {http://dx.doi.org/10.1109/32.707701},
  publisher =    {IEEE Press},
}

@Book{Lyn:1996:MK,
  author =   {N. Lynch},
  OPTeditor =    {},
  title =    {{Distributed Algorithms}},
  publisher =    MK,
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Awe:1987:STOC,
  author =       {B. Awerbuch},
  title =        {{Optimal Distributed Algorithms for Minimum Weight Spanning Tree, Counting,
                   Leader Election, and Related Problems}},
  booktitle =    PROC # " 19th " # STOC,
  year =         {1987},
  pages =        {230-240},
  address =      {New York, New York, United States},
  publisher =    {ACM Press},
}

@Article{SchSan:1994:DC,
  author =   {A. Schiper and A. Sandoz},
  title =    {{Strong Stable Properties in Distributed Systems}},
  journal =      DC,
  year =     {1994},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {93-103},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{SinKal+:1993:TR:93-11,
  author =   {A. Sinha and L. Kal{\'e} and B. Ramkumar},
  title =    {{A Dynamic and Adaptive Quiescence Detection Algorithm}},
  institution =  PPL # ", " #  DCS # ", "  # UIUC,
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {93-11},
  OPTaddress =   {Urbana-Champaign, IL 61801},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{An Example of Stepwise Refinement of Distributed Programs: Quiescence Detection}},
  journal =      TOPLAS,
  year =     {1986},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {326-343},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{KshSin:1994:TSE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{Efficient Detection and Resolution of Generalized Distributed Deadlocks}},
  journal =      TSE,
  year =     {1994},
  OPTkey =   {},
  volume =   {20},
  number =   {1},
  pages =    {43-54},
  month =    JAN,
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BraTou:1987:DC,
  author =   {G. Bracha and S. Toueg},
  title =    {{Distributed Deadlock Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {127-138},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Kna:1987:CS,
  author =   {E. Knapp},
  title =    {{Deadlock Detection in Distributed Databases}},
  journal =      CS,
  year =     {1987},
  OPTkey =   {},
  volume =   {19},
  number =   {4},
  pages =    {303-328},
  month =    DEC,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LynMal+:2002:WPPS,
  author =   {N. Lynch and D. Malkhi and D. Ratajczak},
  title =    {{Atomic Data Access in Content Addressable Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # WPPS,
  pages =    {295-305},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LiMis+:2004:DISC,
  author =   {X. Li and J. Misra and C. G. Plaxton},
  title =    {{Active and Concurrent Topology Maintenance}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # DISC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{ZhaHua+:2003:SAC,
  author =   {B. Y. Zhao and L. Huang and J. Stribling and S. C. Rhea and A. D. Joseph and J. Kubiatowicz},
  title =    {{Tapestry: A Resilient Global-Scale Overlay for Service Deployment}},
  journal =      SAC,
  year =     {2003},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {41-53},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoMor+:2003:TN,
  author =   {I. Stoica and R. Morris and D. Liben-Nowell and D. R. Karger and M. F. Kaashoek
                  and F. Dabek and H. Balakrishnan},
  title =    {{Chord: A Scalable Peer-to-Peer Lookup Service for Internet Applications}},
  journal =      TN,
  year =     {2003},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {17-32},
  month =    FEB,
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AspSha:2003:SDA,
  author =   {J. Aspnes and G. Shah},
  title =    {{Skip Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 14th Annual " # SDA,
  pages =    {384-393},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BanMay:2004:SIU,
  author =   {S. Bansod and J. Mayo},
  title =    {{A Distributed Algorithm for Unstable Global Predicate Evaluation with Approximately Synchronized Clocks}},
  journal =      SIU,
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {2},
  pages =    {151-168},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{AgaGar:2004:TR,
  author =   {A. Agarwal and V. K. Garg},
  title =    {{Chain Clock: Efficient Causality Tracking for Shared Memory Systems}},
  note =     "Submitted to the " # ICDCS,
  OPTkey =   {},
  month =    JUN,
  year =     {2005},
  OPTannote =    {}
}



@Article{Lee:2004:TSE,
  author =   {S. Lee},
  title =    {{Fast, Centralized Detection and Resolution of Distributed Deadlocks in the
                   Generalized Model}},
  journal =      TSE,
  year =     {2004},
  OPTkey =   {},
  volume =   {30},
  number =   {9},
  pages =    {561-573},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BouTro:1998:TPDS,
  author =   {A. Boukerche and C. Tropper},
  title =    {{A Distributed Graph Algorithm for the Detection of Local Cycles and Knots}},
  journal =      TPDS,
  year =     {1998},
  OPTkey =   {},
  volume =   {9},
  number =   {8},
  pages =    {748-757},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{CheDen+:1996:ICDCS,
  author =   {S. Chen and Y. Deng and P. C. Attie and W. Sun},
  title =    {{Optimal Deadlock Detection in Distributed Systems based on
                   Locally Constructed Wait-For Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {613-619},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAY,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hol:1972:CS,
  author =   {R. C. Holt},
  title =    {{Some Deadlock Properties of Computer Systems}},
  journal =      CS,
  year =     {1972},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  pages =    {179-195},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1999:KDE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{A One-Phase Algorithm to Detect Distributed Deadlocks in
                   Replicated Databases}},
  journal =      KDE,
  year =     {1999},
  OPTkey =   {},
  volume =   {11},
  number =   {6},
  pages =    {880-895},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{ManSin:2002:ICPP,
  author =   {D. Manivannan and M. Singhal},
  title =    {{A Distributed Algorithm for Knot Detection in a Distributed Graph}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPP,
  OPTpages =     {},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ManSin:2003:TPDS,
  author =   {D. Manivannan and M. Singhal},
  title =    {{An Efficient Distributed Algorithm for Detecting Knots and
                   Cycles in a Distributed Graph}},
  journal =      TPDS,
  year =     {2003},
  OPTkey =   {},
  volume =   {14},
  OPTnumber =    {10},
  pages =    {961-972},
  month =    OCT,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Sin:1989:Com,
  author =   {M. Singhal},
  title =    {{Deadlock Detection in Distributed Systems}},
  journal =      Com,
  year =     {1989},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {37-48},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1994:JPDC,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{On Characterization and Correctness of Distributed Deadlock Detection}},
  journal =      JPDC,
  year =     {1994},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {44-59},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{JagVas:1983:TSE,
  author =   {J. R. Jagannathan and R. Vasudevan},
  title =    {{Comments on ``Protocols for Deadlock Detection in
                  Distributed Database Systems''}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {371},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Awe:1985:JACM,
  author =   {B. Awerbuch},
  title =    {{Complexity of Network Synchronization}},
  journal =      JACM,
  year =     {1985},
  OPTkey =   {},
  volume =   {32},
  number =   {4},
  pages =    {804-823},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@inproceedings{XiaPlax:2002:POMC,
 author = {Xiaozhou Li and C. Greg Plaxton},
 title = {On name resolution in peer-to-peer networks},
 booktitle = {POMC '02: Proceedings of the second ACM international workshop on Principles of mobile computing},
 year = {2002},
 isbn = {1-58113-511-4},
 pages = {82--89},
 location = {Toulouse, France},
 doi = {http://doi.acm.org/10.1145/584490.584507},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@URL{dist,
  author =       {},
  title =        "www.distributed.net/rc5",
  howpublished = {},
  year =         "2002",
  month =        "Dec",
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
  file = F
}

@CONFERENCE{SatNeer:2005:FSTTCS,
  author =       {Sathya Peri and Neeraj Mittal},
  title =        {Monitoring Stable Properties in Dynamic Peer-to-Peer Distributed Systems},
  booktitle =    PROC # " 25th " # FSTTCS,
  year =         {2005},
  pages  =       {420-431},
  address =      {Hyderabad, India},
  month =        {December},
  note =         {},
  key =          {},
  crossref =     {},
  annote =       {},
}

@TECHREPORT{BalHelPier:2004:TR,
  AUTHOR =       {R. Baldoni and J. Helary and S. Tucci Piergiovanni},
  TITLE =        {Maintaining group connectivity in dynamic asynchronous distributed systems},
  INSTITUTION =  {``Dipartimento di Informatica e Sistemistica, A.Ruberti, Universit?? di Roma la Sapienza"},
  YEAR =         {2004},
  doi=           {"http://www.dis.uniroma1.it/~midlab"},
}

@article{PageJacChen:1993:TPDS,
 author = {I. Page and T. Jacob and E. Chern},
 title = {Fast Algorithms for Distributed Resource Allocation},
 journal = {IEEE Trans. Parallel Distrib. Syst.},
 volume = {4},
 number = {2},
 year = {1993},
 issn = {1045-9219},
 pages = {188--197},
 doi = {http://dx.doi.org/10.1109/71.207594},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
}

@article{ChoiSing:1995:TOPLAS,
 author = {Manhoi Choy and Ambuj K. Singh},
 title = {Efficient fault-tolerant algorithms for distributed resource allocation},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {17},
 number = {3},
 year = {1995},
 issn = {0164-0925},
 pages = {535--559},
 doi = {http://doi.acm.org/10.1145/203095.203101},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@TECHREPORT{SatNeer:2006:TR,
  AUTHOR =       {Sathya Peri and Neeraj Mittal},
  TITLE =        {Lower bounds on Departures for Dynamic Asynchronous Peer-to-Peer systems},
  INSTITUTION =  {University of Texas at Dallas},
  YEAR =         {2006},
}

@INPROCEEDINGS{WeidPagPerv:1991:SPDP,
  AUTHOR =       {Weidman.E.B and Page.I.P and Pervin.W.J},
  TITLE =        {{Explicit dynamic exclusion algorithm}},
  BOOKTITLE =    {Proceedings of the Third IEEE Symposium on Parallel and Distributed Processing},
  YEAR =         {1991},
  pages =        {142-149},
  month =        {DEC},
  organization = {IEEE},
}

@INPROCEEDINGS{LynMalRata:2002:IPTPS,
  AUTHOR =       {N. Lynch and D. Malkhi and D. Ratajczak},
  TITLE =        {{Atomic Data Access in Content Addressable Networks}},
  BOOKTITLE =    {Proceedings for the 1st International Workshop on Peer-to-Peer Systems (IPTPS '02)},
  YEAR =         {2002},
  month =        {Mar},
  publisher =    {Springer-Verlag},
}
%% Citations included by Sat in the area of STMs

@article{HerlMoss:1993:SigArch,
 author = {Maurice Herlihy and J. Eliot B.Moss },
 title = {{Transactional memory: {A}rchitectural {S}upport for {L}ock-{F}ree {D}ata {S}tructures}},
 journal = {SIGARCH Comput. Archit. News},
 volume = {21},
 number = {2},
 year = {1993},
 issn = {0163-5964},
 pages = {289--300},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ShavTou:1995:PODC,
 author = {Shavit, Nir and Touitou, Dan},
 title = {{{S}oftware {T}ransactional {M}emory}},
 booktitle = {PODC},
 year = {1995},
 isbn = {0-89791-710-3},
 pages = {204--213},
 location = {Ottowa, Ontario, Canada},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{Harretal:2005:PPoPP,
 author = {Tim Harris and Simon Marlow and Simon Peyton-Jones and Maurice Herlihy},
 title = {{Composable memory transactions}},
 booktitle = {PPoPP},
 year = {2005},
 isbn = {1-59593-080-9},
 pages = {48--60},
 location = {Chicago, IL, USA},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Yangetal:2007:PPoPP,
 author = {Ni, Yang and Menon, Vijay S. and Adl-Tabatabai, Ali-Reza and Hosking, Antony L. and Hudson, Richard L. and Moss, J. Eliot B. and Saha, Bratin and Shpeisman, Tatiana},
 title = {{Open nesting in software transactional memory}},
 booktitle = {PPoPP},
 year = {2007},
 isbn = {978-1-59593-602-8},
 pages = {68--78},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1229428.1229442},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{AgarLeiSukh:2006:MSPC,
 author = {Agrawal, Kunal and Leiserson, Charles E. and Sukha, Jim},
 title = {{Memory models for open-nested transactions}},
 booktitle = {MSPC '06: Proceedings of the 2006 workshop on Memory system performance and correctness},
 year = {2006},
 isbn = {1-59593-578-9},
 pages = {70--81},
 location = {San Jose, California},
 doi = {http://doi.acm.org/10.1145/1178597.1178610},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{MossAnt:2006:SCP,
 author = {Moss, J. Eliot B. and Hosking, Antony L.},
 title = {{Nested transactional memory: model and architecture sketches}},
 journal = {Sci. Comput. Program.},
 volume = {63},
 number = {2},
 year = {2006},
 issn = {0167-6423},
 pages = {186--201},
 doi = {http://dx.doi.org/10.1016/j.scico.2006.05.010},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@inproceedings{AgarFinSukh:2008:PPoPP,
 author = {Agrawal, Kunal and Fineman, Jeremy T. and Sukha, Jim},
 title = {{Nested parallelism in transactional memory}},
 booktitle = {PPoPP '08: Proceedings of the 13th ACM SIGPLAN Symposium on Principles and practice of parallel programming},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {163--174},
 location = {Salt Lake City, UT, USA},
 doi = {http://doi.acm.org/10.1145/1345206.1345232},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Moretal:2006:ASPLOS,
 author = {Moravan, Michelle J. and Bobba, Jayaram and Moore, Kevin E. and Yen, Luke and Hill, Mark D. and Liblit, Ben and Swift, Michael M. and Wood, David A.},
 title = {{Supporting nested transactional memory in logTM}},
 booktitle = {ASPLOS-XII: Proceedings of the 12th international conference on Architectural support for programming languages and operating systems},
 year = {2006},
 isbn = {1-59593-451-0},
 pages = {359--370},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1168857.1168902},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@Article{Moss:2006:MPI,
	author = {J.E.B.Moss},
	journal = {In Workshop on Memory Performance Issues},
	year = {2006},
	title = {{Open Nested Transactions: Semantics and Support}}
}

@inproceedings{GuerKap:Opacity:PPoPP:2008,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {{On the {C}orrectness of {T}ransactional {M}emory}},
 booktitle = {PPoPP},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {},
 location = {},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{ImbsRay:LockSTM:OPODIS:2008,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A Lock-Based STM Protocol That Satisfies Opacity and Progressiveness}},
 booktitle = {OPODIS '08: Proceedings of the 12th International Conference on Principles of Distributed Systems},
 year = {2008},
 isbn = {978-3-540-92220-9},
 pages = {226--245},
 location = {Luxor, Egypt},
 doi = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 }

@article{Herlihy+:Linearizability:TPLS:1990,
 author = {Herlihy, Maurice P. and Wing, Jeannette M.},
 title = {{Linearizability: a correctness condition for concurrent objects}},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {12},
 number = {3},
 year = {1990},
 issn = {0164-0925},
 pages = {463--492},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{Papad:1979:JACM,
 author = {Papadimitriou, Christos H.},
 title = {{The serializability of concurrent database updates}},
 journal = {J. ACM},
 volume = {26},
 number = {4},
 year = {1979},
 issn = {0004-5411},
 pages = {},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@BOOK{tm-book,
	AUTHOR		= {Guerraoui, Rachid and  Kapalka, Michal},
	TITLE		= {{Principles of Transactional Memory, Synthesis Lectures on Distributed Computing Theory}},
	PUBLISHER	= {Morgan and Claypool},
	YEAR		= {2010},
}

@article{Vidya:1987:AINF,
 author = {Vidyasankar, K.},
 title = {{Generalized theory of serializability}},
 journal = {Acta Inf.},
 volume = {24},
 number = {1},
 year = {1987},
 issn = {0001-5903},
 pages = {105--109},
 doi = {http://dx.doi.org/10.1007/BF00290709},
 publisher = {Springer-Verlag New York, Inc.},
 address = {Secaucus, NJ, USA},
 }

@article{RenAbba:1994:IPL,
 author = {Resende, R. F. and El Abbadi, A.},
 title = {{On the serializability theorem for nested transactions}},
 journal = {Inf. Process. Lett.},
 volume = {50},
 number = {4},
 year = {1994},
 issn = {0020-0190},
 pages = {177--183},
 doi = {http://dx.doi.org/10.1016/0020-0190(94)00033-6},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@book{WeiVoss:TIS:2002:Morg,
  author    = {Gerhard Weikum and
               Gottfried Vossen},
  title     = {{Transactional Information Systems: Theory, Algorithms, and
               the Practice of Concurrency Control and Recovery}},
  publisher = {Morgan Kaufmann},
  year      = {2002},
  isbn      = {1-55860-508-8},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Imbs+:2009:PODC,
 author = {Imbs, Damien and de Mendivil, Jos\'{e} Ramon and Raynal, Michel},
 title = {{Brief announcement: virtual world consistency: a new condition for STM systems}},
 booktitle = {PODC '09: Proceedings of the 28th ACM symposium on Principles of distributed computing},
 year = {2009},
 isbn = {978-1-60558-396-9},
 pages = {280--281},
 location = {Calgary, AB, Canada},
 doi = {http://doi.acm.org/10.1145/1582716.1582764},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ImbsRay:2009:SIROCCO,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A versatile {STM} protocol with invisible read operations that satisfies the virtual world consistency condition}},
 booktitle = {Proceedings of the 16th international conference on Structural Information and Communication Complexity},
 series = {SIROCCO'09},
 year = {2010},
 isbn = {3-642-11475-X, 978-3-642-11475-5},
 location = {Piran, Slovenia},
 pages = {266--280},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-11476-2_21},
 doi = {10.1007/978-3-642-11476-2_21},
 acmid = {2174448},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {atomic object, causal past, commit/abort, concurrency control, consistency condition, consistent global state, lock, read-from relation, regular read/write object, serializability, shared memory, software transactional memory, transaction, vector clock},
} 

@inproceedings{CIR11,
  author    = {Tyler Crain and
               Damien Imbs and
               Michel Raynal},
  title     = {{Read Invisibility, Virtual World Consistency and Probabilistic
               Permissiveness are Compatible}},
  booktitle = {ICA3PP (1)},
  year      = {2011},
  pages     = {244-257}
}

@inproceedings{israeli-disjoint,
 author = {Israeli, Amos and Rappoport, Lihu},
 title = {{Disjoint-access-parallel implementations of strong shared memory primitives}},
 booktitle = {Proceedings of the thirteenth annual ACM symposium on Principles of distributed computing},
 series = {PODC '94},
 year = {1994},
 isbn = {0-89791-654-9},
 location = {Los Angeles, California, United States},
 pages = {151--160},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/197917.198079},
 doi = {http://doi.acm.org/10.1145/197917.198079},
 acmid = {198079},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{AHM09,
 author = {Attiya, Hagit and Hillel, Eshcar and Milani, Alessia},
 title = {{Inherent limitations on disjoint-access parallel implementations of transactional memory}},
 booktitle = {Proceedings of the twenty-first annual symposium on Parallelism in algorithms and architectures},
 series = {SPAA '09},
 year = {2009},
 isbn = {978-1-60558-606-9},
 location = {Calgary, AB, Canada},
 pages = {69--78},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1583991.1584015},
 doi = {http://doi.acm.org/10.1145/1583991.1584015},
 acmid = {1584015},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {disjoint-access parallelism, impossibility result, lower bound, partial snapshots, transactional memory},
} 

@InProceedings{Doherty+:2009:REFINE,
	booktitle = {REFINE},
	year = {2009},
	author = {Simon Doherty and Lindsay Groves and Victor Luchangco and Mark Moir},
	title = {{Towards Formally Specifying and Verifying Transactional Memory}}
}

@TechReport{SatVid:2010:TR,
	author = {Sathya Peri and K.Vidyasankar},
	institution = {Memorial University of Newfoundland},
	title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
	year = {July, 2011}
}

@inproceedings{SatVid:2011:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
 booktitle = {12th International Conference on Distributed Computing and Networking},
 pages = {95--106},
 year = {2011},
 location = {Bangalore, Canada},
 }

@inproceedings{SatVid:2012:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{An efficient scheduler for closed nested transactions that satisfies all-read-consistency and non-interference}},
 booktitle = {13th International Conference on Distributed Computing and Networking},
 year = {2012},
 location = {Bangalore, Canada},
 }



@inproceedings{Guer+:disc1:2008, author = {Rachid Guerraoui and Thomas A. Henzinger and Vasu Singh}, title = {Permissiveness in Transactional Memories}, booktitle = {DISC}, pages = {305--319}, year = {2008}, crossref = {DBLP:conf/wdag/2008}, url = {https://doi.org/10.1007/978-3-540-87779-0\_21}, doi = {10.1007/978-3-540-87779-0\_21}, timestamp = {Tue, 13 Jun 2017 10:37:55 +0200}, biburl = {https://dblp.org/rec/bib/conf/wdag/GuerraouiHS08}, bibsource = {dblp computer science bibliography, https://dblp.org} }

@inproceedings{Crain+:RI_VWC:ICA3PP:2011, author = {Tyler Crain and Damien Imbs and Michel Raynal}, title = {Read Invisibility, Virtual World Consistency and Probabilistic Permissiveness are Compatible}, booktitle = {ICA3PP}, pages = {244--257}, year = {2011}, crossref = {DBLP:conf/ica3pp/2011-1}, url = {https://doi.org/10.1007/978-3-642-24650-0\_21}, doi = {10.1007/978-3-642-24650-0\_21}, timestamp = {Sun, 11 Mar 2018 01:37:22 +0100}, biburl = {https://dblp.org/rec/bib/conf/ica3pp/CrainIR11}, bibsource = {dblp computer science bibliography, https://dblp.org} }

@InProceedings{Baretto+:PPoPP:2010,
   address     = { },
   affiliation = {EPFL},
   author      = {Baretto, Joao and Dragojevic, Aleksandar and Ferreira,
                 Paulo and Guerraoui, Rachid and Kapalka, Michal},
   booktitle   = {Proceedings of the 15th {ACM} {SIGPLAN} symposium on
                 {P}rinciples and {P}ractice of {P}arallel {C}omputing},
   details     = {http://infoscience.epfl.ch/record/144050},
   documenturl = {http://infoscience.epfl.ch/getfile.py?recid=144050&mode=best},
   doi         = {10.1145/1693453.1693466},
   keywords    = {Nested parallel programs; Fork-join; Work-stealing; Transactional memory},
   location    = {Bangalore, India},
   pages       = {91--100},
   publisher   = {ACM},
   review      = {REVIEWED},
   series      = { },
   status      = {PUBLISHED},
   title       = {{Leveraging {P}arallel {N}esting in {T}ransactional {M}emory}},
   unit        = {LPD},
   url         = { },
   year        = 2010
}

@InProceedings{RanVid:Tran:2011,
	author = {Ranjeet Kumar and Krishnamurthy Vidyasankar},
	booktitle = {TRANSACT 2011},
	title = {{HParSTM: A Hierarchy-based STM Protocol for Supporting Nested Parallelism}},
	month = {June},
	year = {2011}
}

@Article{RaviSat:IJCCT:2012,
	title = {{A Correctness Criterion for Eager Approach Validation for Transactional Memory System}},
	year = {2012},
	pages = {43-49},
	author = {Ravi Kumar and Sathya Peri},
	volume = {3},
	journal = {International Journal of Computer and Communication Technology (IJCCT)},
	number = {2}
}

@article{KuzSat:Corr:2012,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{On Non-Interference of Transactions}},
  journal   = {CoRR},
  volume    = {abs/1211.6315},
  year      = {2012},
  ee        = {http://arxiv.org/abs/1211.6315},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Bernstein+:MCC:TDS:1983,
 author = {Bernstein, Philip A. and Goodman, Nathan},
 title = {{{M}ultiversion {C}oncurrency {C}ontrol: {T}heory and {A}lgorithms}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {Dec. 1983},
 volume = {8},
 number = {4},
 month = dec,
 year = {1983},
 issn = {0362-5915},
 pages = {465--483},
 numpages = {19},
 url = {http://doi.acm.org/10.1145/319996.319998},
 doi = {10.1145/319996.319998},
 acmid = {319998},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transaction processing},
}
 
@Article{CachRito:2006:CP,
	title = {{{V}ersioned {B}oxes as the basis for {M}emory {T}ransactions}},
	year = {2006},
	number = {2},
	author = {J. Cachopo and A. Rito-Silva},
	pages = {172--185},
	journal = {Science of Computer Programming},
	volume = {63}
}

@inproceedings{AydAbd:2008:Serial:transact,
  author	= {Aydonat, Utku and Abdelrahman, Tarek},
  title		= {{Serializability of {T}ransactions in {S}oftware {T}ransactional {M}emory}},
  booktitle	= {TRANSACT~'08: 3rd Workshop on Transactional Computing},
  pdf		= {http://www.unine.ch/transact08/papers/Aydonat-Serializability.pdf},
  year		= {2008},
  month		= {feb},
}

@article{PapadKanel:1984:MultVer:TDS,
 author = {Papadimitriou, Christos H. and Kanellakis, Paris C.},
 title = {{On Concurrency Control by Multiple Versions}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {March 1984},
 volume = {9},
 number = {1},
 month = mar,
 year = {1984},
 issn = {0362-5915},
 pages = {89--99},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/348.318588},
 doi = {10.1145/348.318588},
 acmid = {318588},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Perel+:2011:SMV:DISC,
  author    = {Dmitri Perelman and
               Anton Byshevsky and
               Oleg Litmanovich and
               Idit Keidar},
  title     = {{SMV}: {S}elective {M}ulti-{V}ersioning {STM}},
  booktitle = {DISC},
  year      = {2011},
  pages     = {125-140},
  ee        = {http://dx.doi.org/10.1007/978-3-642-24100-0_9},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{herlihy+:2003:stm-dynamic:podc,
  author	= {Herlihy, Maurice and Luchangco, Victor and Moir, Mark and {William N. Scherer}, III},
  title		= {{Software Transactional Memory for Dynamic-Sized Data Structures}},
  booktitle	= {PODC~'03: Proc. 22nd ACM Symposium on Principles of Distributed Computing},
  pages		= {92--101},
  month		= {Jul},
  urlpage	= {http://doi.acm.org/10.1145/872035.872048},
  year		= {2003},
}

@inproceedings{dice:2006:tl2:disc,
  author	= {Dice, Dave and Shalev, Ori and Shavit, Nir},
  title		= {{Transactional Locking II}},
  booktitle	= {DISC~'06: Proc. 20th International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 4167},
  pages		= {194--208},
  year		= {2006},
  month		= {sep},
}

@inproceedings{perel+:2010:MultVer:PODC,
  author    = {Dmitri Perelman and Rui Fan and Idit Keidar},
  title     = {{{O}n {M}aintaining {M}ultiple {V}ersions in {STM}}},
  booktitle = {PODC},
  year      = {2010},
  pages     = {16-25},
  ee        = {http://doi.acm.org/10.1145/1835698.1835704},
}

@incollection{riegel+:2006:LSA:DISC,
  author	= {Riegel, Torvald and Felber, Pascal and Fetzer, Christof},
  editor	= {},
  title		= {{A {L}azy {S}napshot {A}lgorithm with {E}ager {V}alidation}},
  booktitle	= {Proceedings of the 20th International Symposium on Distributed Computing, {DISC} 2006},
  publisher	= {Springer},
  month		= {Sep},
  year		= {},
  volume	= {4167},
  isbn		= {3-540-44624-9},
  pages		= {284--298},
  series	= {Lecture Notes in Computer Science},
  urlpage	= {http://dx.doi.org/10.1007/11864219_20}
}

@inproceedings{riegel+:sistm:transact:2006,
  author	= {Riegel, Torvald and Fetzer, Christof and Felber, Pascal},
  booktitle	= {Proceedings of the First ACM SIGPLAN Workshop on Languages, Compilers, and Hardware Support for Transactional Computing},
  month		= {Jun},
  title		= {{Snapshot Isolation for Software Transactional Memory }},
  year		= {2006}
}

@article{attiyaHill:sinmvperm:tcs:2012,
  author    = {Hagit Attiya and
               Eshcar Hillel},
  title     = {{A {S}ingle-{V}ersion {STM} that is {M}ulti-{V}ersioned {P}ermissive}},
  journal   = {Theory Comput. Syst.},
  volume    = {51},
  number    = {4},
  year      = {2012},
  pages     = {425-446},
  ee        = {http://dx.doi.org/10.1007/s00224-012-9406-3},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{prisat:mvto:corr:2013,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{A TimeStamp based Multi-version STM Protocol that satisfies
               Opacity}},
  journal   = {CoRR},
  volume    = {abs/1305.6624},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1305.6624},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Fern+:LSMVSTM:PPoPP:2011,
 author = {Fernandes, S{\'e}rgio Miguel and Cachopo, Joao},
 title = {{Lock-free and {S}calable {M}ulti-version {S}oftware {T}ransactional {M}emory}},
 booktitle = {},
 series = {PPoPP '11},
 year = {2011},
 isbn = {978-1-4503-0119-0},
 location = {San Antonio, TX, USA},
 pages = {},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1941553.1941579},
 doi = {10.1145/1941553.1941579},
 acmid = {1941579},
 publisher = {},
 address = {New York, NY, USA},
 keywords = {garbage collection, lock-free synchronization, multi-version concurrency control, transactional memory},
} 

@Article{LuScott:UMV:Transact:2012,
	journal = {Transact},
	title = {{Unmanaged Multiversion STM}},
	year = {2012},
	author = {Li Lu and Michael L. Scott}
}

@inproceedings{SinhaMalik:RuntimeSee:IPDPS:2010,
  author    = {Arnab Sinha and
               Sharad Malik},
  title     = {{Runtime checking of serializability in software transactional
               memory}},
  booktitle = {IPDPS},
  year      = {2010},
  pages     = {1-12},
  ee        = {http://dx.doi.org/10.1109/IPDPS.2010.5470389},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{HadzPapad:AAMVCC:PODS:1985,
 author = {Hadzilacos, Thanasis and Papadimitriou, Christos H.},
 title = {{Algorithmic aspects of multiversion concurrency control}},
 booktitle = {Proceedings of the fourth ACM SIGACT-SIGMOD symposium on Principles of database systems},
 series = {PODS '85},
 year = {1985},
 isbn = {0-89791-153-9},
 location = {Portland, Oregon, USA},
 pages = {96--104},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/325405.325417},
 doi = {10.1145/325405.325417},
 acmid = {325417},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{KuznetsovPeri:Non-interference:TCS:2017,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{Non-interference and local correctness in transactional memory}},
  journal   = {Theor. Comput. Sci. 2017},
  volume    = {},
  pages     = {},
  year      = {},
  url       = {},
  doi       = {},
  timestamp = {Tue, 04 Jul 2017 17:27:30 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/tcs/KuznetsovP17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Kumar+:MVTO:ICDCN:2014,
  author    = {Priyanka Kumar and
               Sathya Peri and
               K. Vidyasankar},
  title     = {{A TimeStamp Based Multi-version STM Algorithm}},
  booktitle = {ICDCN},
  year      = {2014},
  pages     = {},
  ee        = {http://dx.doi.org/10.1007/978-3-642-45249-9_14},
  crossref  = {DBLP:conf/icdcn/2014},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@book{Har+:TMBook:2010,
  author    = {Tim Harris and
               James R. Larus and
               Ravi Rajwar},
  title     = {{Transactional Memory, 2nd edition}},
  booktitle = {Transactional Memory (2.ed.)},
  publisher = {Morgan {\&} Claypool Publishers},
  series    = {Synthesis Lectures on Computer Architecture},
  year      = {2010},
  ee        = {http://dx.doi.org/10.2200/S00272ED1V01Y201006CAC011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{OluHamm:MicroBook:Queue:2005,
 author = {Olukotun, Kunle and Hammond, Lance},
 title = {{The Future of Microprocessors}},
 journal = {Queue},
 issue_date = {September 2005},
 volume = {3},
 number = {7},
 month = sep,
 year = {2005},
 issn = {1542-7730},
 pages = {26--29},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1095408.1095418},
 doi = {10.1145/1095408.1095418},
 acmid = {1095418},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@book{HerlihyShavit:AMP:Book:2012,
	author = {Herlihy, Maurice and Shavit, Nir},
	title = {The Art of Multiprocessor Programming, Revised Reprint},
	year = {2012},
	isbn = {9780123973375, 9780123977953},
	edition = {1st},
	publisher = {Morgan Kaufmann Publishers Inc.},
	address = {San Francisco, CA, USA},
} 

@inproceedings{HerlihyShavit:Progress:Opodis:2011,
	author = {Herlihy, Maurice and Shavit, Nir},
	title = {On the Nature of Progress},
	booktitle = {},
	series = {OPODIS 2011},
	year = {},
	isbn = {978-3-642-25872-5},
	location = {Toulouse, France},
	pages = {},
	numpages = {16},
	url = {},
	doi = {},
	acmid = {2183558},
	publisher = {},
	address = {},
} 

@inproceedings{Harris:NBList:DISC:2001,
	author    = {Timothy L. Harris},
	title     = {A Pragmatic Implementation of Non-blocking Linked-Lists},
	booktitle = {DISC},
	pages     = {},
	year      = {2001},
	
	timestamp = {Fri, 26 May 2017 14:09:14 +0200},
	biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/wdag/Harris01},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Herlihy:WaitFree:1991,
  title={{Wait-free synchronization}},
  author={Herlihy, Maurice},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={13},
  number={1},
  pages={124--149},
  year={1991},
  publisher={ACM}
}

@INPROCEEDINGS{Attiya+:DUOp:ICDCS:2013,
author={Attiya, H. and Hans, S. and Kuznetsov, P. and Ravi, S.},
booktitle={Distributed Computing Systems (ICDCS), 2013 IEEE 33rd International Conference on},
title={{Safety of Deferred Update in Transactional Memory}},
year={2013},
month={July},
pages={601-610},
keywords={concurrency control;transaction processing;committed transactions;deferred update safety;deferred-update semantics;opacityc riterion;prefix serializations;sequential execution;sequential order;speculative transactions;transactional memory;unique-write assumption;History;Law;Real-time systems;Safety;Semantics;Silicon;Limit-closure;Safety;Transactional Memory},
doi={10.1109/ICDCS.2013.57},
ISSN={1063-6927},}

@article{PriSat:MVC:Corr:2015,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{Multi-Version Conflict Notion}},
  journal   = {CoRR},
  volume    = {abs/1307.8256},
  year      = {2013},
  url       = {http://arxiv.org/abs/1307.8256},
  timestamp = {Thu, 15 Aug 2013 15:30:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KumarP13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Attiya+:TMS:DISC:2014,
  author    = {Hagit Attiya and
               Alexey Gotsman and
               Sandeep Hans and
               Noam Rinetzky},
  title     = {{Safety of Live Transactions in Transactional Memory: {TMS} is Necessary
               and Sufficient}},
  booktitle = {Distributed Computing - 28th International Symposium, {DISC} 2014,
               Austin, TX, USA, October 12-15, 2014. Proceedings},
  pages     = {376--390},
  year      = {2014},
  crossref  = {DBLP:conf/wdag/2014},
  url       = {http://dx.doi.org/10.1007/978-3-662-45174-8_26},
  doi       = {10.1007/978-3-662-45174-8_26},
  timestamp = {Tue, 30 Sep 2014 10:44:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/AttiyaGHR14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Herlihy:WFS:TPLS:1991,
 author = {Herlihy, Maurice},
 title = {{Wait-free Synchronization}},
 journal = {ACM Trans. Program. Lang. Syst.},
 issue_date = {Jan. 1991},
 volume = {13},
 number = {1},
 month = jan,
 year = {1991},
 issn = {0164-0925},
 pages = {124--149},
 numpages = {26},
 url = {http://doi.acm.org/10.1145/114005.102808},
 doi = {10.1145/114005.102808},
 acmid = {102808},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {linearization, wait-free synchronization},
} 



@inproceedings{LuScott:GMV:DISC:2013,
  author    = {Li Lu and
               Michael L. Scott},
  title     = {{Generic Multiversion {STM}}},
  booktitle = {DISC},
  pages     = {134--148},
  year      = {2013},
  crossref  = {DBLP:conf/wdag/2013},
  url       = {http://dx.doi.org/10.1007/978-3-642-41527-2_10},
  doi       = {10.1007/978-3-642-41527-2_10},
  timestamp = {Mon, 28 Oct 2013 18:03:50 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/LuS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{CachAnt:VBoxes:SCOOL:2005,
  author	= {Cachopo, Joao and Rito-Silva, Antonio},
  title		= {{Versioned Boxes as the Basis for Memory Transactions}},
  booktitle	= {OOPSLA 2005 Workshop on Synchronization and Concurrency in Object-Oriented Languages (SCOOL)},
  urlpage	= {http://hdl.handle.net/1802/2101},
  year		= {2005},
  month		= {oct},
}

@article{Thomas:TWR:TDS:1979,
 author = {Thomas, Robert H.},
 title = {{A Majority Consensus Approach to Concurrency Control for Multiple Copy Databases}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {June 1979},
 volume = {4},
 number = {2},
 month = jun,
 year = {1979},
 issn = {0362-5915},
 pages = {180--209},
 numpages = {30},
 url = {http://doi.acm.org/10.1145/320071.320076},
 doi = {10.1145/320071.320076},
 acmid = {320076},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {clock synchronization, computer networks, concurrency control, distributed computation, distributed control, distributed databases, multiprocess systems, update synchronization},
} 

@inproceedings{Gramoli+:OptListSet:DISC-BA:2015,
  TITLE = {{Brief Announcement: A Concurrency-Optimal List-Based Set}},
  AUTHOR = {Gramoli, Vincent and Kuznetsov, Petr and Ravi, Srivatsan and Shang, Di},
  URL = {https://hal.archives-ouvertes.fr/hal-01207872},
  BOOKTITLE = {{DISC 2015}},
  ADDRESS = {Tokyo, Japan},
  ORGANIZATION = {{Toshimitsu Masuzawa and Koichi Wada}},
  EDITOR = {Yoram Moses and Matthieu Roy},
  PUBLISHER = {{Springer-Verlag Berlin Heidelberg}},
  SERIES = {29th International Symposium on Distributed Computing},
  VOLUME = {LNCS 9363},
  YEAR = {2015},
  MONTH = Oct,
  PDF = {https://hal.archives-ouvertes.fr/hal-01207872/file/37-BA.pdf},
  HAL_ID = {hal-01207872},
  HAL_VERSION = {v1},
}

@article{Gramoli+:OptListSet:CoRR:2015,
  author    = {Vincent Gramoli and
               Petr Kuznetsov and
               Srivatsan Ravi and
               Di Shang},
  title     = {{A Concurrency-Optimal List-Based Set}},
  journal   = {CoRR},
  volume    = {abs/1502.01633},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.01633},
  timestamp = {Mon, 02 Mar 2015 14:17:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GramoliKRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Heller+:LazyList:PPL:2007,
  author    = {Steve Heller and
               Maurice Herlihy and
               Victor Luchangco and
               Mark Moir and
               William N. Scherer III and
               Nir Shavit},
  title     = {{A Lazy Concurrent List-Based Set Algorithm}},
  journal   = {Parallel Processing Letters},
  volume    = {17},
  number    = {4},
  pages     = {411-424},
  year      = {2007},
  url       = {},
  doi       = {},
  timestamp = {Mon, 23 Jun 2008 13:43:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ppl/HellerHLMSS07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Ziv+:Composing:POPL:2015,
  title={{Composing Concurrency Control}},
  author={Ziv, Ofri and Aiken, Alex and Golan-Gueta, Guy and Ramalingam, G and Sagiv, Mooly},
  booktitle={Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
  pages={240--249},
  year={2015},
  organization={ACM}
}

@article{marathe2004qualitative,
  title={{A qualitative survey of modern software transactional memory systems}},
  author={Marathe, Virendra J and Scott, Michael L},
  journal={University of Rochester Computer Science Dept., Tech. Rep},
  year={2004}
}

@inproceedings{Vafeiadis:2006:PCH:1122971.1122992,
 author = {Vafeiadis, Viktor and Herlihy, Maurice and Hoare, Tony and Shapiro, Marc},
 title = {{Proving Correctness of Highly-concurrent Linearisable Objects}},
 booktitle = {PPoPP},
 series = {},
 year = {2006},
 isbn = {1-59593-189-9},
 location = {},
 pages = {129--136},
 numpages = {8},
 url = {},
 doi = {},
 acmid = {1122992},
 publisher = {},
 address = {},
 keywords = {concurrent programming, formal verification, linearisability, rely-guarantee reasoning, shared-memory concurrency},
}


@techreport{marathe:stm-survey:urcs-tr:2004,
  author	= {Marathe, Virendra J. and Scott, Michael L.},
  title		= {{A Qualitative Survey of Modern Software Transactional Memory Systems}},
  number	= {TR 839},
  institution	= {University of Rochester Computer Science Dept.},
  month		= {Jun},
  year		= {2004},
  pdf		= {http://www.cs.rochester.edu/u/scott/papers/2004_TR839.pdf}
}

@phdthesis{Fraser:PracticalLF:2004,
  title={{Practical lock-freedom}},
  author={Fraser, Keir},
  year={2004},
  school={University of Cambridge}
}

@inproceedings{Herlihy+:STM-DynamicSize:PODC:2003,
  title={{Software transactional memory for dynamic-sized data structures}},
  author={Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer III, William N},
  booktitle={Proceedings of the twenty-second annual symposium on Principles of distributed computing},
  pages={92--101},
  year={2003},
  organization={ACM}
}
@inproceedings{Marathe+:STM-Tradeoff:LCRS:2004,
  title={{Design tradeoffs in modern software transactional memory systems}},
  author={Marathe, Virendra J and Scherer, William N and Scott, Michael L},
  booktitle={Proceedings of the 7th workshop on Workshop on languages, compilers, and run-time support for scalable systems},
  pages={1--7},
  year={2004},
  organization={ACM}
}

@article{Barghouti:1991:CCA:116873.116875,
 author = {Barghouti, Naser S. and Kaiser, Gail E.},
 title = {{Concurrency Control in Advanced Database Applications}},
 journal = {ACM Comput. Surv.},
 issue_date = {Sept. 1991},
 volume = {23},
 number = {3},
 month = sep,
 year = {1991},
 issn = {0360-0300},
 pages = {269--317},
 numpages = {49},
 url = {http://doi.acm.org/10.1145/116873.116875},
 doi = {10.1145/116873.116875},
 acmid = {116875},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {advanced database applications, concurrency control, cooperative transactions, design environments, extended transaction models, long transactions, object-oriented databases, relaxing serializability},
}

@article{Beeri+:Nested:JACM:1989,
 author = {Beeri, Catriel and Bernstein, Philip A. and Goodman, Nathan},
 title = {{A Model for Concurrency in Nested Transactions Systems}},
 journal = {J. ACM},
 issue_date = {April 1989},
 volume = {36},
 number = {2},
 month = apr,
 year = {1989},
 issn = {0004-5411},
 pages = {230--269},
 numpages = {40},
 url = {http://doi.acm.org/10.1145/62044.62046},
 doi = {10.1145/62044.62046},
 acmid = {62046},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{HerlihyKosk:Boosting:PPoPP:2008,
	author    = {Maurice Herlihy and
	Eric Koskinen},
	title     = {Transactional boosting: a methodology for highly-concurrent transactional
	objects},
	booktitle = {{PPOPP}},
	pages     = {},
	year      = {2008},
	crossref  = {DBLP:conf/ppopp/2008},
	url       = {http://doi.acm.org/10.1145/1345206.1345237},
	doi       = {10.1145/1345206.1345237},
	timestamp = {Tue, 22 May 2012 15:24:56 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/ppopp/HerlihyK08},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Hassan+:OptBoost:PPoPP:2014,
	author    = {Ahmed Hassan and
	Roberto Palmieri and
	Binoy Ravindran},
	title     = {{Optimistic transactional boosting}},
	booktitle = {PPoPP},
	pages     = {},
	year      = {2014},
	crossref  = {DBLP:conf/ppopp/2014},
	url       = {},
	doi       = {},
	timestamp = {Sun, 03 Jul 2016 16:10:52 +0200},
	biburl    = {http://dblp.dagstuhl.de/rec/bib/conf/ppopp/HassanPR14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Hassan:OptTransLazy:Opodis:2014,
	title={{On developing optimistic transactional lazy set}},
	author={Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
	booktitle={OPODIS},
	pages={437--452},
	year={2014},
	organization={Springer}
}

@inproceedings{Spiegelman+:TransDS:PLDI:2016,
	title={{Transactional data structure libraries}},
	author={Spiegelman, Alexander and Golan-Gueta, Guy and Keidar, Idit},
	booktitle={PLDI},
	pages={682--696},
	year={2016},
	organization={ACM}
}

@article{Anand+:CaPRa:Corr:2015,
  author    = {Anshu S. Anand and
               R. K. Shyamasundar and
               Sathya Peri},
  title     = {{Opacity Proof for CaPR+ Algorithm}},
  journal   = {CoRR},
  volume    = {abs/1510.06967},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.06967},
  timestamp = {Sun, 01 Nov 2015 17:30:45 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AnandSP15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Lev-Ari+:OnCorrectness:DISC:2014,
	author    = {Kfir Lev{-}Ari and
	Gregory V. Chockler and
	Idit Keidar},
	title     = {{On Correctness of Data Structures under Reads-Write Concurrency}},
	booktitle = {DISC},
	pages     = {273--287},
	year      = {2014},
	crossref  = {DBLP:conf/wdag/2014},
	url       = {},
	doi       = {},
	timestamp = {Fri, 19 May 2017 01:25:17 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/Lev-AriCK14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Lev-Ari+:ConsApproachLinz:DISC:2015,
	author = {Lev-Ari, Kfir and Chockler, Gregory V and Keidar, Idit},
	booktitle = {DISC},
	doi = {},
	editor = {Moses, Yoram},
	isbn = {978-3-662-48652-8},
	pages = {356--370},
	publisher = {Springer},
	series = {},
	title = {{A Constructive Approach for Proving Data Structures' Linearizability}},
	url = {},
	volume = {},
	year = {2015}
}

@article{zhang2016high,
  title={{High-Performance Composable Transactional Data Structures}},
  author={Zhang, Deli},
  year={2016}
}

@techreport{zhang2010composability,
  author={Zhang, Rui and Budimli{\'c}, Zoran and Scherer III, William N},
  title={{Composability for application-specific transactional optimizations}},
  institution={Department of Computer Science, Rice University},
  year={2010}
}

@article{DBLP:journals/corr/abs-0910-0366,
  author    = {Daniel Cederman and
               Philippas Tsigas},
  title     = {{Supporting Lock-Free Composition of Concurrent Data Objects}},
  journal   = {CoRR},
  volume    = {abs/0910.0366},
  year      = {2009},
  url       = {},
  timestamp = {Wed, 07 Jun 2017 14:40:49 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/corr/abs-0910-0366},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Hassan2015,
author = {Hassan, Ahmed and Wang, Chao and Broadwater, Robert P},
mendeley-groups = {PhD Thesis},
title = {{Designing , Modeling , and Optimizing Transactional Data Structures}},
year = {2015}
}

@article{harris2007abstract,
	title={{Abstract nested transactions}},
	author={Harris, Tim and others},
	year={2007},
	publisher={Citeseer}
}


@inproceedings{Peri+:OSTM:Netys:2018,
	author = {Sathya Peri and
	Ajay Singh and
	Archit Somani},
	title = {{Efficient means of Achieving Composability using Transactional Memory}},
	booktitle = {},
	series = {NETYS '18},
	year = {2018},
	isbn = {978-1-4503-4210-0},
	keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@article{Felber+:ElasticTrans:2017:jpdc,
 author = {Felber, Pascal and Gramoli, Vincent and Guerraoui, Rachid},
 title = {{Elastic Transactions}},
 journal = {J. Parallel Distrib. Comput.},
 issue_date = {February 2017},
 volume = {100},
 number = {C},
 month = feb,
 year = {2017},
 issn = {0743-7315},
 pages = {},
 numpages = {25},
 url = {https://doi.org/10.1016/j.jpdc.2016.10.010},
 doi = {10.1016/j.jpdc.2016.10.010},
 acmid = {3066828},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Concurrent data structures, Transactional memory},
} 


@inproceedings{ZhangDech:LockFreeTW:SPAA:2016,
 author = {Zhang, Deli and Dechev, Damian},
 title = {{Lock-free Transactions Without Rollbacks for Linked Data Structures}},
 booktitle = {},
 series = {SPAA '16},
 year = {2016},
 isbn = {978-1-4503-4210-0},
 location = {Pacific Grove, California, USA},
 pages = {},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2935764.2935780},
 doi = {10.1145/2935764.2935780},
 acmid = {2935780},
 publisher = {},
 address = {New York, NY, USA},
 keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@inproceedings{Dalessandro+:NoRec:PPoPP:2010,
  added-at = {2010-01-19T00:00:00.000+0100},
  author = {Dalessandro, Luke and Spear, Michael F. and Scott, Michael L.},
  biburl = {https://www.bibsonomy.org/bibtex/2bb4ff560750c574e33fceb87457d3cce/dblp},
  booktitle = {PPOPP},
  crossref = {conf/ppopp/2010},
  editor = {Govindarajan, R. and Padua, David A. and Hall, Mary W.},
  ee = {http://doi.acm.org/10.1145/1693453.1693464},
  interhash = {65ad98c6f111ce3b454219b4fd45ebb8},
  intrahash = {bb4ff560750c574e33fceb87457d3cce},
  isbn = {978-1-60558-877-3},
  keywords = {dblp},
  pages = {},
  publisher = {ACM},
  timestamp = {2012-05-23T11:41:17.000+0200},
  title = {{NOrec: Streamlining STM by Abolishing Ownership Records}},
  url = {http://dblp.uni-trier.de/db/conf/ppopp/ppopp2010.html#DalessandroSS10},
  year = 2010
}



@online{ethereum,
	author    = {Ethereum},
	url       = {http://github.com/ethereum}
}

@misc{Nakamoto:Bitcoin:2009,
	added-at = {2014-04-17T08:33:06.000+0200},
	author = {Nakamoto, Satoshi},
	biburl = {https://www.bibsonomy.org/bibtex/23db66df0fc9fa2b5033f096a901f1c36/ngnn},
	interhash = {423c2cdff70ba0cd0bca55ebb164d770},
	intrahash = {3db66df0fc9fa2b5033f096a901f1c36},
	keywords = {imported},
	timestamp = {2014-04-17T08:33:06.000+0200},
	title = {Bitcoin: A peer-to-peer electronic cash system},
	url = {http://www.bitcoin.org/bitcoin.pdf},
	year = 2009
}

@inproceedings{Dickerson+:ACSC:PODC:2017,
	author = {Dickerson, Thomas and Gazzillo, Paul and Herlihy, Maurice and Koskinen, Eric},
	title = {Adding Concurrency to Smart Contracts},
	booktitle = {},
	series = {PODC '17},
	year = {},
	isbn = {978-1-4503-4992-5},
	location = {Washington, DC, USA},
	pages = {},
	numpages = {10},
	url = {},
	doi = {},
	acmid = {3087835},
	publisher = {},
	address = {},
	keywords = {blockchain, concurrency, ethereum, fork-join, miners, smart contracts, validators},
} 


@inproceedings{SergeyandHobor:ACP:2017,
	title={A Concurrent Perspective on Smart Contracts},
	author={Ilya Sergey and Aquinas Hobor},
	booktitle={Financial Cryptography Workshops},
	year={2017}
}

@InProceedings{ZangandZang:ECSC:WBD:2018,
	author="Zhang, An
	and Zhang, Kunlong",
	editor="Cai, Yi
	and Ishikawa, Yoshiharu
	and Xu, Jianliang",
	title="Enabling Concurrency on Smart Contracts Using Multiversion Ordering",
	booktitle="Web and Big Data",
	year="2018",
	publisher="",
	address="Cham",
	pages="425--439",
	abstract="Blockchain-based platforms, such as Ethereum, allow transactions in blocks to call user-defined scripts named smart contracts. In the blockchain network, after being generated by a miner, a block will be validated many times by the peers who accept it. Hence by enabling concurrency on smart contracts, especially validation, we can improve the efficiency and the throughput of those platforms.",
	isbn="978-3-319-96893-3"
}


@article{Nick:PublicN:journals:1997, 
	author = {Nick Szabo}, 
	title = {Formalizing and Securing Relationships on Public Networks}, 
	journal = {First Monday}, 
	volume = {2}, number = {9}, year = {1997} } 

@inproceedings{Luu+:DIC:CCS:2015, 
	author = {Luu, Loi and Teutsch, Jason and Kulkarni, Raghav and Saxena, Prateek}, title = {Demystifying Incentives in the Consensus Computer}, booktitle = {Proceedings of the 22Nd ACM SIGSAC Conference on Computer and Communications Security}, series = {CCS '15}, year = {2015}, isbn = {978-1-4503-3832-5}, location = {Denver, Colorado, USA}, pages = {706--719}, numpages = {14}, url = {}, doi = {}, acmid = {2813659}, publisher = {ACM}, address = {New York, NY, USA}, keywords = {bitcoin, consensus computer, cryptocurrency, ethereum, incentive compatibility, verifiable computation}, }

@online{Solidity,
	author    = {Solidity documentation},
	url       = {http://solidity.readthedocs.io/en/latest/index.html}
}


@inproceedings{Luu+:MSC:CCS:2016,
	author = {Luu, Loi and Chu, Duc-Hiep and Olickel, Hrishi and Saxena, Prateek and Hobor, Aquinas},
	title = {Making Smart Contracts Smarter},
	booktitle = {CCS '16},
	series = {},
	year = {},
	isbn = {978-1-4503-4139-4},
	location = {Vienna, Austria},
	pages = {},
	numpages = {16},
	url = {},
	doi = {},
	acmid = {2978309},
	publisher = {},
	address = {},
	keywords = {blockchain, cryptocurrencies, ethereum, smart contract, symbolic execution},
} 

@inproceedings{Delmolino+:SSTCSC:FC:2016,
	author    = {Kevin Delmolino and
	Mitchell Arnett and
	Ahmed E. Kosba and
	Andrew Miller and
	Elaine Shi},
	title     = {Step by Step Towards Creating a Safe Smart Contract: Lessons and Insights
	from a Cryptocurrency Lab},
	booktitle = {Financial Cryptography and Data Security - {FC} 2016 International
	Workshops, BITCOIN, VOTING, and WAHC, Christ Church, Barbados, February
	26, 2016.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/fc/2016w},
	url       = {},
	doi       = {},
	timestamp = {Wed, 30 May 2018 16:11:58 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/fc/DelmolinoAKMS16},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{HerlihyandWing:1990:LCC:ACM,
	author = {Herlihy, Maurice P. and Wing, Jeannette M.},
	title = {Linearizability: A Correctness Condition for Concurrent Objects},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {July 1990},
	volume = {12},
	number = {3},
	month = jul,
	year = {1990},
	issn = {0164-0925},
	pages = {463--492},
	numpages = {30},
	url = {},
	doi = {},
	acmid = {78972},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{DBLP:journals/corr/abs-1809-01326,
  author    = {Parwat Singh Anjana and
               Sweta Kumari and
               Sathya Peri and
               Sachin Rathor and
               Archit Somani},
  title     = {An Efficient Framework for Concurrent Execution of Smart Contracts},
  journal   = {CoRR},
  volume    = {abs/1809.01326},
  year      = {2018},
  url       = {http://arxiv.org/abs/1809.01326},
  archivePrefix = {arXiv},
  eprint    = {1809.01326},
  timestamp = {Fri, 05 Oct 2018 11:34:52 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1809-01326},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{Bushkov+:Live-TM:PODC:2012,
	author    = {Victor Bushkov and Rachid Guerraoui and Michal Kapalka},
	title     = {On the liveness of transactional memory},
	booktitle = {PODC'12.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/podc/2012},
	url       = {http://doi.acm.org/10.1145/2332432.2332435},
	doi       = {10.1145/2332432.2332435},
	timestamp = {Sun, 15 Jul 2012 18:49:17 +0200},
	biburl    = {http://dblp.org/rec/bib/conf/podc/BushkovGK12},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Gramoli+:TM2C:Eurosys:2012,
	author = {Gramoli, Vincent and Guerraoui, Rachid and Trigonakis, Vasileios},
	title = {{TM2C: A Software Transactional Memory for Many-cores}},
	booktitle = {},
	series = {EuroSys 2012},
	year = {2012},
	isbn = {978-1-4503-1223-3},
	location = {Bern, Switzerland},
	pages = {},
	numpages = {14},
	url = {},
	doi = {},
	acmid = {2168872},
	publisher = {},
	address = {},
	keywords = {concurrent programming, contention management, many-cores, transactional memory},
} 


@article{WaliSten:Starve:CC:2009,
	author    = {M. M. Waliullah and
	Per Stenstr{\"{o}}m},
	title     = {{Schemes for Avoiding Starvation in Transactional Memory Systems}},
	journal   = {Concurrency and Computation: Practice and Experience},
	volume    = {},
	number    = {},
	pages     = {},
	year      = {2009},
	url       = {},
	doi       = {},
	timestamp = {Sat, 20 May 2017 00:25:18 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/concurrency/WaliullahS09},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@unknown{Spear+:CCM:PPoPP:2009,
author = {Spear, Michael F. and Dalessandro, Luke and Marathe, Virendra J. and Scott, Michael L.},
 title = {A Comprehensive Strategy for Contention Management in Software Transactional Memory},
 booktitle = {Proceedings of the 14th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '09},
 year = {2009},
 isbn = {978-1-60558-397-6},
 location = {Raleigh, NC, USA},
 pages = {141--150},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1504176.1504199},
 doi = {10.1145/1504176.1504199},
 acmid = {1504199},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {condition synchronization, contention management, inevitability, priority, software transactional memory},
} 


@inproceedings{Juyal+:SSS:2018,
	author    = {Chirag Juyal and
	Sandeep S. Kulkarni and
	Sweta Kumari and
	Sathya Peri and
	Archit Somani},
	title     = {An Innovative Approach to Achieve Compositionality Efficiently Using
	Multi-version Object Based Transactional Systems},
	booktitle = {{SSS'18}.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/sss/2018},
	url       = {https://doi.org/10.1007/978-3-030-03232-6\_19},
	doi       = {10.1007/978-3-030-03232-6\_19},
	timestamp = {Thu, 06 Dec 2018 00:00:00 +0100},
	biburl    = {https://dblp.org/rec/bib/conf/sss/JuyalKKPS18},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Chaudhary+:KSFTM:Corr:2017a,
	author    = {Ved Prakash Chaudhary and Chirag Juyal and Sandeep S. Kulkarni and Sweta Kumari and Sathya Peri},
	title     = {Achieving Starvation Freedom in Multi-Version Transactional Memory Systems},
	journal   = {CoRR},
	volume    = {abs/1709.01033},
	year      = {2017},
	url       = {http://arxiv.org/abs/1709.01033},
	archivePrefix = {arXiv},
	eprint    = {1709.01033},
	timestamp = {Thu, 06 Dec 2018 17:39:41 +0100},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1709-01033},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Chaudhary+:KSFTM:Corr:2017,
	author    = {Ved Prakash Chaudhary and Chirag Juyal and Sandeep S. Kulkarni and Sweta Kumari and Sathya Peri},
	title     = {Achieving Starvation Freedom in Multi-Version Transactional Memory Systems},
	journal   = {NETYS 2019},
	volume    = {},
	year      = {},
	url       = {},
	archivePrefix = {},
	eprint    = {},
	timestamp = {},
	biburl    = {},
	bibsource = {}
}

@inproceedings{Bobba:2007:PPH:1250662.1250674,
	author = {Bobba, Jayaram and Moore, Kevin E. and Volos, Haris and Yen, Luke and Hill, Mark D. and Swift, Michael M. and Wood, David A.},
	title = {Performance Pathologies in Hardware Transactional Memory},
	booktitle = {Proceedings of the 34th Annual International Symposium on Computer Architecture},
	series = {ISCA '07},
	year = {2007},
	isbn = {978-1-59593-706-3},
	location = {San Diego, California, USA},
	pages = {81--91},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1250662.1250674},
	doi = {10.1145/1250662.1250674},
	acmid = {1250674},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {contention management, hardware, pathology, performance, transactional memory},
} 

@MASTERSTHESIS{Erb2012, author = {Benjamin Erb}, title = {Concurrent Programming for Scalable Web Architectures}, school = {Institute of Distributed Systems, Ulm University}, year = {2012}, type = {Diploma Thesis}, keywords = {web, scalability, architecture, concurrency}, month = {April}, number = {VS-D01-2012}, url = {http://www.benjamin-erb.de/thesis} } 

@inproceedings{Riegel+:LSA:DISC:2006,
	author    = {Torvald Riegel and
	Pascal Felber and
	Christof Fetzer},
	title     = {A Lazy Snapshot Algorithm with Eager Validation},
	booktitle = {DISC 2006.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/wdag/2006},
	url       = {},
	doi       = {},
	timestamp = {Fri, 02 Jun 2017 13:01:06 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/RiegelFF06},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Juyal+:CORR:SF-MVOSTM:2019,
	author    = {Chirag Juyal and
	Sandeep S. Kulkarni and
	Sweta Kumari and
	Sathya Peri and
	Archit Somani},
	title     = {Obtaining Progress Guarantee and GreaterConcurrency in Multi-Version
	Object Semantics},
	journal   = {CoRR},
	volume    = {abs/1904.03700},
	year      = {2019},
	url       = {http://arxiv.org/abs/1904.03700},
	archivePrefix = {arXiv},
	eprint    = {1904.03700},
	timestamp = {Thu, 25 Apr 2019 13:55:01 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1904-03700},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

==> Arxiv SFKOSTM SSS19/conc.tex <==
\vspace{-.5cm}
\section{Conclusion}
\label{sec:conc}
\vspace{-0.3cm}
\noindent
We proposed a novel \emph{Starvation-Free K-Version Object-based STM (SF-KOSTM)} which ensure the \emph{\stfdm} while maintaining the latest $K$-versions corresponding to each key and satisfies the correctness criteria as \emph{local-opacity}. The value of $K$ can vary from 1 to $\infty$. When $K$ is equal to 1 then SF-KOSTM boils down to \emph{Single-Version Starvation-Free OSTM (SF-SVOSTM)}. When $K$ is $\infty$ then SF-KOSTM algorithm maintains unbounded versions corresponding to each key known as \emph{Multi-Version Starvation-Free OSTM (SF-MVOSTM)}. To delete the unused version from the version list,  SF-MVOSTM calls a separate Garbage Collection (GC) method and proposed SF-MVOSTM-GC. SF-KOSTM provides greater concurrency and higher throughput using higher-level methods. We implemented all the proposed algorithms for \emph{hash table} and \emph{linked-list} data structure but it is generic for other data structures as well. %SF-KOSTM performs best among SF-OSTM and all the proposed three variants of SF-MVOSTM. 
Results of SF-KOSTM shows significant performance gain over state-of-the-art STMs. 

%We introduced a novel SF-OSTM which ensures the \stfdm at object-level and satisfies the correctness criteria as co-opacity. Here, We observed that while ensuring the \stfdm, long-running transaction with high priority cause multiple transactions to abort. So, we proposed an efficient and novel SF-MVOSTM which ensures \stfdm while maintaining the multiple versions corresponding to each key. It gives the privilege to lookup method to read from any of previously committed versions and insert, delete method to create a version and commit successfully. So, proposed SF-MVOSTM reduces the number of aborts and improves the throughput. SF-MVOSTM satisfies the correctness criteria as local-opacity. 

%We proposed three variants of SF-MVOSTM: (1) SF-MVOSTM without garbage collection (or GC) which has unlimited versions of each key in the absence of gc(). (2) SF-MVOSTM with garbage collection which deletes the unwanted version corresponding to the keys and improves the performance. (3) Finite version SF-MVOSTM (or SF-KOSTM) which maintains finite versions (maximum $K$ versions) corresponding to each key. We proposed and implemented all the above defined STMs for hash table and linked-list data structure but it is generic for other data structure as well. SF-KOSTM performs best among SF-OSTM and all the proposed three variants of SF-MVOSTM. Results of SF-KOSTM shows significant performance gain over state-of-the-art STMs.    

==> Arxiv SFKOSTM SSS19/dsDesign.tex <==
\subsection{Data Structure and Design of SF-OSTM and SF-MVOSTM}
\label{subsec:dsde}



==> Arxiv SFKOSTM SSS19/figs/dsDesign.tex <==
\subsection{Data Structure and Design of SF-OSTM and SF-MVOSTM}
\label{subsec:dsde}



==> Arxiv SFKOSTM SSS19/figs/figures.tex <==
\section{Designated Figures}
\label{sec:figs}

\begin{figure}
	\centerline{\scalebox{0.5}{\input{figs/adv.pdf_t}}}
	\caption{Advantage of OSTMs over RWTSMs}
	\label{fig:adv}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/sostm.pdf_t}}}
	\caption{Advantage of SF-OSTM over OSTMs}
	\label{fig:sostm}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/advmvostm.pdf_t}}}
	\caption{Benefits of MVOSTM over Single version SF-OSTM}
	\label{fig:advmvostm}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/design.pdf_t}}}
	\caption{Data Structure and Design of SF-MVOSTM}
	\label{fig:advmvostm}
\end{figure} 


\begin{figure}
	\centering
	\begin{minipage}[b]{0.49\textwidth}
		\centering
		\captionsetup{justification=centering}
		\scalebox{.45}{\input{figs/stmore.pdf_t}}
		% \vspace{-16cm}
		\caption{Searching $k_9$ over \emph{lazy-list}}
		\label{fig:nostm2}
	\end{minipage}   
	\hfill
	\begin{minipage}[b]{0.49\textwidth}
		\scalebox{.45}{\input{figs/stless.pdf_t}}
		\centering
		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{Searching $k_9$ over $\lsl{}$}
		\label{fig:nostm}
	\end{minipage}
\end{figure}

==> Arxiv SFKOSTM SSS19/figs/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

%\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}

%\newtheorem{definition}{Definition}

\newcounter{history}
\newcommand{\hist}[1]{\refstepcounter{history} {#1}}

%\newcommand{\proof}[1][]{\noindent{\bf\boldmath
 %                         P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------Theorem Notations Defined by Petr --------------------------------------------------------------------------------------------------------
%% Defined by Petr

%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{observation}[theorem]{Observation}


%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\insref}[1]{line~\ref{ins:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

\newcommand{\linref}[1]{Line~\ref{lin:#1}}
%\newcommand{\algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}
\newcommand{\algoref}[1]{{Algo~\ref{algo:#1}}}
\newcommand{\subsecref}[1]{SubSection{\ref{subsec:#1}}}

\newcommand{\histref}[1]{\ref{hist:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{eq(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}
\newcommand{\Confref}[1]{Conflict~\ref{conf:#1}}




\newcommand{\theqed}{$\Box$}


\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}


%------------------------------------------------------------------------------------------------------------------
% Definitions for Object STM paper
%------------------------------------------------------------------------------------------------------------------
%

\newcommand{\tobj} {t-object\xspace}
\newcommand{\txns}[1] {txns(#1)}
\newcommand {\comm}[1] {committed(#1)}
\newcommand {\aborted}[1] {aborted(#1)}
\newcommand {\incomp}[1] {incomp(#1)}
\newcommand {\live}[1] {live(#1)}
\newcommand {\term}[1] {term(#1)}
\newcommand {\key}[1] {key(#1)}
\newcommand {\confevt}[1] {conf-event(#1)}
\newcommand {\confmth}[1] {conf-method(#1)}
\newcommand {\conf}[1] {conflict(#1)}
\newcommand {\termn}[1] {terminate(#1)}

\newcommand {\tcomp} {t-complete\xspace}
\newcommand {\tinc} {t-incomplete\xspace}

\newcommand{\ssch} {sub-history}
\newcommand{\sschs} {sub-histories}

\newcommand{\nseq} {non-sequential}
\newcommand{\tseq} {t-sequential\xspace}
%\newcommand{\seq} {sequential}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}

\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\vwrite} {valWrite}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastup} {lastUpdt}
\newcommand{\lupdt}[2] {#2.lastUpdt(#1)}
\newcommand{\lseen}[2] {#2.lastSeen(#1)}

\newcommand{\mr} {MR}
\newcommand{\tr} {TR}

%\newcommand{\valid} {valid}
\newcommand{\validity} {validity\xspace}
\newcommand{\legal} {legal\xspace}
\newcommand{\legality} {legality\xspace}

\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}
%\newcommand{\rvmt} {rv\_method\xspace}
%\newcommand{\upmt} {upd\_method\xspace}
\newcommand{\rvp} {\emph{\rvmt execution} phase}
\newcommand{\cp} {\emph{\upmt execution} phase}

\newcommand{\termop} {terminal operation\xspace}
\newcommand{\cc} {correctness-criterion\xspace}
\newcommand{\ccs} {correctness-criteria\xspace}
\newcommand{\gen}[1] {gen(#1)}

\newcommand{\inv} {$inv$}
\newcommand{\rsp} {$rsp$}
\newcommand{\rmw} {rmw}
\newcommand{\first}[1] {first(#1)}
\newcommand{\last}[1] {last(#1)}

\newcommand{\evts}[1] {evts(#1)}
\newcommand{\met}[1] {methods(#1)}

\newcommand{\sgt} {SGT\xspace}
\newcommand{\memop} {memory operation\xspace}
\newcommand{\pref}[2] {#2.prefix(#1)}

\newcommand{\init} {\emph{init}\xspace}
\newcommand{\tbeg} {\emph{t\_begin}\xspace}
\newcommand{\tread} {\emph{t\_read}\xspace}
\newcommand{\twrite} {\emph{t\_write}\xspace}
\newcommand{\tins} {\emph{STM\_insert}\xspace}
\newcommand{\tdel} {\emph{STM\_delete}\xspace}
\newcommand{\tlook} {\emph{STM\_lookup}\xspace}
\newcommand{\tryc} {\emph{tryC}\xspace}%{\emph{tryC}}
\newcommand{\trya} {\emph{tryA}\xspace}%{\emph{tryA}}


\newcommand{\failed} {failed\xspace}
\newcommand{\unaborted} {unaborted\xspace}

%\newcommand{\ins} {\emph{list\_insert}}
%\newcommand{\del} {\emph{list\_del}}
%\newcommand{\look} {\emph{list\_lookup}}

\newcommand{\inss} {\emph{list\_insert}}
\newcommand{\dell} {\emph{list\_del}}
\newcommand{\lookk} {\emph{list\_lookup}}

\newcommand{\ins} {\emph{lsl\_ins}\xspace}
\newcommand{\del} {\emph{lsl\_del}\xspace}
\newcommand{\look} {\emph{lsl\_Search}\xspace}

\newcommand{\rv} {\emph{rv}}
\newcommand{\up} {\emph{up}}

\newcommand{\rset}[1] {rset(#1)}
\newcommand{\wset}[1] {wset(#1)}
\newcommand{\rvar} {readVar}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co\text{-}opacity\xspace}

\newcommand{\vwc} {VWC\xspace}
\newcommand{\lo} {LO\xspace}
\newcommand{\lopty} {LO\xspace}
\newcommand{\lopq} {locally-opaque\xspace}

\newcommand{\tab} {hash-table\xspace}
\newcommand{\set}{table\xspace}
\newcommand{\llist} {list\xspace}
\newcommand{\otm} {\textit{OSTM}\xspace}%{ObjSTM}
\newcommand{\sotm} {\textit{SV-OSTM}\xspace}%{ObjSTM}

\newcommand{\rwtm} {\textit{RWSTM}\xspace}
%\newcommand{\lotm} {Table-OSTM}
\newcommand{\lotm} {OSTMs\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\bst} {BST\xspace}
\newcommand{\lsl} {rblazy\text{-}list\xspace}
\newcommand{\lazy} {lazy-list\xspace}

\newcommand{\csr} {CSR\xspace}

\newcommand{\perm} {permissive\xspace}
\newcommand{\pness} {permissiveness\xspace}
\newcommand{\permfn}[1] {perm(#1)}

\newcommand{\sspec} {sequential-specification\xspace}
\newcommand{\samp} {sample-stm\xspace}

\newcommand{\cg}[1] {CG(#1)}

\newcommand{\uset} {updtSet\xspace}
\newcommand{\lset} {lookupSet\xspace}
\newcommand{\rvm} {\emph{rvm}\xspace}
%\newcommand{\ht} {\emph{hash table}}

\newcommand{\firste} {firstEvt\xspace}
\newcommand{\laste} {lastEvt\xspace}
\newcommand{\fevt}[1] {#1.firstEvt}
\newcommand{\levt}[1] {#1.lastEvt}

\newcommand{\fkmth}[3] {#3.firstKeyMth(#1, #2)}
\newcommand{\pkmth}[3] {#3.prevKeyMth(#1, #2)}

\newcommand{\bstu} {\emph{bst-update}}
\newcommand{\lllist} {locallog\_list}

\newcommand{\udset}[1] {updtSet(#1)}
\newcommand{\rvset}[1] {rvSet(#1)}
%\newcommand{\bst}{BST}

\newcommand{\refr}[1]{refNode(#1)}
\newcommand{\lin}[1]{#1.LP\xspace}

%\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\newcommand\tabspace[1][1cm]{\hspace*{#1}}

%%%%%%% DS macros
%\newcommand{\glslhead}{getLslHead($obj\_id \downarrow, key \downarrow$)}


%\newcommand{\txlfind} {\textup{translog.find\_in\_loclog}$(obj\_id \downarrow, key \downarrow)$}
\newcommand{\txgid} {txlog.getTid()}
%\newcommand{\txgllist} {txlog.getLlList($t_{i} \downarrow$)}
\newcommand{\txsetst}[1] {L\_txlog.setStatus($L\_txstatus \downarrow$, $ OK \downarrow$)}
\newcommand{\txbegin}[1] {begin(#1)}

%\newcommand{\lsls}[1] {list\_lookup($obj\_id \downarrow,  key \downarrow, knext \uparrow, value \uparrow$, #1)}

\newcommand{\rvvalidate} {rvValidate($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

%\newcommand{\lslins}[1] {lslIns($preds[] \downarrow$, $currs[] \downarrow$, #1)}
\newcommand{\lsldel} {lslDel($preds[] \downarrow$, $currs[] \downarrow$)}


%\newcommand{\rlsol} {releaseOrderedLocks($ordered\_ll\_list \downarrow$)}

\newcommand{\ctov} {commitTOValidation($ll\_entry_i \downarrow$)}
\newcommand{\rvtov} {rvTOValidation($ key \downarrow$, $curr \downarrow$)}
\newcommand{\toval} {toValidation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}
\newcommand{\validation} {validation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}


\newcommand{\ifvalidation} {$$\textup{interferenceValidation}$(preds[] \downarrow, currs[] \downarrow)$$}
%\newcommand{\handlea}{tryAbort($obj\_id \downarrow$)}

%\newcommand{\llsort}{ll.sort ($ll\_list \downarrow$)}

%%---------------------macro w/o parameter

\newcommand{\npctov} {\emph{commitTOValidation()}}
\newcommand{\nptov} {\emph{toValidation()}}
\newcommand{\npintv} {\emph{intraTransValidation()}}
\newcommand{\nptc} {\emph{STM tryC()}}
\newcommand{\npins} {\emph{STM insert()}}
\newcommand{\npdel} {\emph{STM delete()}}
\newcommand{\npluk} {\emph{STM lookup()}}
\newcommand{\nplsls} {\emph{list\_lookup()}}
\newcommand{\nplsldel} {\emph{lslDel()}}
\newcommand{\nplslins} {\emph{list\_Ins()}}
\newcommand{\npbegin} {\emph{STM begin}}
\newcommand{\nppoval} {\emph{lostUpdateValidation()}}
\newcommand{\tcins} {\emph{tryC_{ins}}}
\newcommand{\npcld}{\emph{commonLu\&Del()}}


\newcommand{\rn} {\textcolor{red}{RL}\xspace}
\newcommand{\bn} {\textcolor{blue}{BL}\xspace}

\newcommand{\rc} {\textcolor{red}{currs[0]}}
\newcommand{\bc} {\textcolor{blue}{currs[1]}}
\newcommand{\bp} {\textcolor{blue}{preds[0]}}
\newcommand{\rp} {\textcolor{red}{preds[1]}}


\newcommand{\eevts}[1] {#1.evts}
\newcommand{\hst}[1] {#1.hist\xspace}
\newcommand{\exec}[1] {#1.exec\xspace}
%\newcommand{\state}[1] {#1.state\xspace}
\newcommand{\alls}[1] {#1.allStates\xspace}
\newcommand{\pres}[1] {#1.pre\text{-}state\xspace}
\newcommand{\posts}[1] {#1.post\text{-}state\xspace}

\newcommand{\shist}[2] {#2.subhist(#1)}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subh}  {sub\text{-}history\xspace}

\newcommand{\preds} {G\_preds[]}
\newcommand{\currs} {G\_currs[]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mvotm} {\textit{MVOSTM}\xspace}
\newcommand{\mvotms} {\textit{MV-OSTM}\xspace}
\newcommand{\hmvotm} {\textit{HT-MVOSTM}\xspace}
\newcommand{\lmvotm} {\textit{list-MVOSTM}\xspace}
\newcommand{\hotm} {\textit{HT-OSTM}\xspace}
\newcommand{\kotm} {\textit{KOSTM}\xspace}
\newcommand{\hkotm} {\textit{HT-KOSTM}\xspace}
\newcommand{\lkotm} {\textit{list-KOSTM}\xspace}
\newcommand{\mvotmgc} {\textit{MVOSTM-GC}\xspace}
\newcommand{\hmvotmgc} {\textit{HT-MVOSTM-GC}\xspace}
\newcommand{\lmvotmgc} {\textit{list-MVOSTM-GC}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% Local %%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\llog} {txLog\xspace}

\newcommand{\txlfind} {$L\_txlog.find(L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow)$}
\newcommand{\txll} {$L\_txlog$}
\newcommand{\txllf} {$L\_txlog()$}
\newcommand{\llsopn}[1] {$L\_rec.setOpn(L\_obj\_id \downarrow$, $L\_key \downarrow$, #1)}
\newcommand{\llsval}[1] {$L\_rec.setVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}
\newcommand{\llsopst}[1] {$L\_rec.setOpStatus(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}

\newcommand{\llgopn}[1] {$L\_rec.getOpn(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsopn}[1] {$L\_getOpn((obj\_id \downarrow$, $key \downarrow$, #1)}

\newcommand{\llgval}[1] {$L\_rec.getVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsval}[1] {loclog.getVal($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llspc} {$L\_rec.setPred\&Curr(L\_obj\_id \downarrow$, $ L\_key \downarrow$, $G\_pred \downarrow$, $G\_curr \downarrow$)}

\newcommand{\llgaptc}[1] {$L\_rec.getAptCurr$(#1)}
\newcommand{\llgkeyobj} {$L\_rec.getKey\&Objid(L\_rec_{i} \downarrow$)}

\newcommand{\llgopst} {$L\_rec.getOpStatus(L\_obj\_id \downarrow$, $L\_key \downarrow$)}
%\newcommand{\llsopst}[1] {loclog.getOpStatus($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llgallpc}{$L\_rec.getAllPreds\&Currs(L\_rec_{i} \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}

\newcommand{\poval}{lostUpdateValidation($L\_rec_{i}\downarrow$, $preds[]\uparrow$, $currs[]\uparrow$ )}

\newcommand{\llsort}{$L\_txlog.sort$($L\_list \downarrow$)}

\newcommand{\txgllist} {$L\_txlog.getList(L\_t\_id \downarrow$)}

\newcommand{\cld}{$commonLu\&Del$($L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$)}
%%%%%%%%%%%%%%%%%%%% Global %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cnt} {G\_cnt}
\newcommand{\livetx} {live\_trans}
\newcommand{\gi} {$get\&inc(G\_cnt \downarrow)$}
\newcommand{\glslhead}{getListHead($L\_obj\_id \downarrow, L\_key \downarrow$)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%From MVTO%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}

\newcommand{\mv} {mv}
\newcommand{\rvf} {rvf}
\newcommand{\rt} {rt}
\newcommand{\rvmt} {rv\_method\xspace}
\newcommand{\upmt} {upd\_method\xspace}

%\newcommand{\op} {operation}
\newcommand{\checkv} {check\_versions}
\newcommand{\remid} {removeId}
\newcommand{\instup} {ins\_tuple}
\newcommand{\gc} {gc}
\newcommand{\liveset} {liveSet}
\newcommand{\livel} {liveList}
\newcommand{\locko} {lockOrder}
\newcommand{\mvto} {MV-OSTM}
\newcommand{\valid} {valid}
\newcommand{\seq}[2] {linearize(#2, #1)}
\newcommand{\stl}[3] {#3.stl(#1, #2)}
%\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\aco} {accessOrder}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% methods%%%%%%%%%%%%%%%%%%

\newcommand{\lsls}[1] {list\_lookup($L\_obj\_id \downarrow,  L\_key \downarrow, G\_pred \uparrow, G\_curr \uparrow$)}
\newcommand{\find} {find\_lts}
\newcommand{\handlea}{return ABORT}
\newcommand{\lslins}[1] {list\_Ins($G\_pred \downarrow$, $G\_curr \downarrow$, $node \uparrow$)}
\newcommand{\rlsol} {releaseOrderedLocks($L\_list \downarrow$)}

\newcommand{\mvperm} {mv-permissive\xspace}
\newcommand{\mvpness} {mv-permissiveness\xspace}

\newcommand {\cmnts}[1] {\State{\textcolor{gray}{/* #1 */} }}
\renewcommand{\thefootnote}{\arabic{footnote}}	

%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
\algrenewcommand{\algorithmiccomment}[1]{/* #1 */}

\newcommand{\stfdm} {starvation\text{-}freedom\xspace}
\newcommand{\stf} {starvation\text{-}free\xspace}
\newcommand{\wtfdm} {wait\text{-}freedom\xspace}
\newcommand{\wtf} {wait\text{-}free\xspace}
\newtheorem{assumption}{Assumption}

==> Arxiv SFKOSTM SSS19/figs/pm.tex <==
\section{Proposed Mechanism}
\label{sec:pm}

\input{stardef}

\input{dsDesign}

\input{working}

==> Arxiv SFKOSTM SSS19/figures.tex <==
\section{Designated Figures}
\label{sec:figs}


%\vspace{1cm}

\begin{figure*}
	\centerline{\scalebox{0.45}{\input{figs/sostm.pdf_t}}}
	\caption{Advantage of SF-OSTM over OSTMs}
	\label{fig:sostm}
\end{figure*} 

%\vspace{1cm}


%\vspace{5cm}



%\vspace{3cm}%


%\clearpage
\cmnt{
\begin{figure}[H]
	\centerline{\scalebox{0.6}{\input{figs/sfmv-correct.pdf_t}}}
	\caption{$wts$ violating the real-time order}
	\label{fig:wtsf}
\end{figure} 
}

%\clearpage
%\vspace{1.5cm}


==> Arxiv SFKOSTM SSS19/intro.tex <==
%\newpage
\vspace{-10mm}
\section{Introduction}
\label{sec:intro}

\noindent
In the era of multi-core processors, we can exploit the cores by concurrent programming. But developing an efficient concurrent program while ensuring the correctness is difficult. Software Transactional Memory Systems (STMs) are a convenient programming interface to access the shared memory concurrently while removing the concurrency responsibilities from the programmer. STMs ensure that consistency issues such as deadlock, livelock, priority inversion, etc will not occur. It provides a high-level abstraction to the programmer with the popular correctness criteria opacity \cite{GuerKap:Opacity:PPoPP:2008}, local opacity \cite{KuznetsovPeri:Non-interference:TCS:2017} which consider all the transactions (a piece of code) including aborted one as well in the equivalent serial history. This property makes it different from correctness criteria of database serializability,  strict-serializability \cite{Papad:1979:JACM} and ensures even aborted transactions read correct value in STMs which prevent from divide-by-zero, infinite loop, crashes, etc. Another advantage of STMs is composability which ensures the effect of multiple operations of the transaction will be atomic. This paper considers the optimistic execution of STMs in which transactions are writing into its local log until the successful validation.

%There are two types of STMs available in the literature. (1) Pessimistic STMs which shows the effect of the operation of a transaction immediately and on inconsistency it rollback and transaction returns abort. (2) Optimistic STMs in which transactions are writing into its local log until the successful validation so, rollback is not required. 

A traditional STM system invokes following methods:(1) \tbeg{()}: begins a transaction $T_i$ with unique timestamp $i$. (2) $\tread_i${($k$)} (or $r_i(k)$): $T_i$ reads the value of key $k$ from shared memory. (3) $\twrite_i{(k,v)}$ (or $w_i(k,v)$): $T_i$ writes the value of $k$ as $v$ locally. (4) \emph{STM\_tryC$_i$()}: on successful validation, the effect of $T_i$ will be visible to the shared memory and $T_i$ returns commit otherwise (5) \emph{STM\_tryA$_i$()}: $T_i$ returns abort. These STMs are known as \emph{read-write STMs (RWSTMs)} because it is working at lower-level operations such as read and write. 

Herlihy et al.\cite{HerlihyKosk:Boosting:PPoPP:2008}, Hassan et al. \cite{ Hassan+:OptBoost:PPoPP:2014}, and Peri et al. \cite{Peri+:OSTM:Netys:2018} have shown that working at higher-level operations such as insert, delete and lookup on the linked-list and hash table gives better concurrency than RWSTMs. STMs which work on higher-level operations are known as \emph{Single-Version Object-based STMs (SVOSTMs)} \cite{Peri+:OSTM:Netys:2018}. It exports the following methods: (1) \emph{STM\_begin()}: begins a transaction $T_i$ with unique timestamp $i$ same as RWSTMs. (2) \emph{STM\_lookup$_i(k)$} (or $l_i(k)$): $T_i$ lookups key $k$ from shared memory and returns the value. (3) \emph{STM\_insert$_i(k,v)$} (or $i_i(k,v)$): $T_i$ inserts a key $k$ with value $v$ into its local memory. (4) \emph{STM\_delete$_i(k)$}(or $d_i(k)$): $T_i$ deletes key $k$. (5) \emph{STM\_tryC$_i$()}: the actual effect of \emph{STM\_insert()} and \emph{STM\_delete()} will be visible to the shared memory after successful validation and $T_i$ returns commit otherwise (6) \emph{STM\_tryA$_i$()}: $T_i$ returns abort. 

\setlength{\intextsep}{0pt}

\begin{figure*}
	\centerline{\scalebox{0.41}{\input{figs/adv.pdf_t}}}
\vspace{-.2cm}	\caption{Advantage of SVOSTMs over RWTSMs}
	\label{fig:adv}
\end{figure*} 

\noindent
\textbf{Motivation to work on SVOSTMs}: \figref{adv} represents the advantage of SVOSTMs over RWSTMs while achieving greater concurrency and reducing the number of aborts. \figref{adv}.(a) depicts the underlying data structure as a hash table (or $ht$) with $M$ buckets and bucket $1$ stores three keys $k_1, k_4$ and $k_9$ in the form of the list. Thus, to access $k_4$, a thread has to access $k_1$ before it. \figref{adv}.(b) shows the tree structure of concurrent execution of two transactions $T_1$ and $T_2$ with RWSTMs at layer-0 and SVOSTMs at layer-1 respectively. Consider the execution at layer-0, $T_1$ and $T_2$ are in conflict because write operation of $T_2$ on key $k_1$ as $w_2(k_1)$ is occurring between two read operations of $T_1$ on $k_1$ as $r_1(k_1)$. Two transactions are in conflict if both are accessing the same key $k$ and at least one transaction performs write operation on $k$. So, this concurrent execution cannot be atomic as shown in \figref{adv}.(c). To make it atomic either $T_1$ or $T_2$ has to return abort. Whereas execution at layer-1 shows the higher-level operations $l_1(k_1)$, $d_2(k_4)$ and $l_1(k_9)$ on different keys $k_1, k_4$ and $k_9$ respectively. All the higher-level operations are isolated to each other so tree can be pruned \cite[Chap 6]{WeiVoss:TIS:2002:Morg} from layer-0 to layer-1 and both the transactions return commit with equivalent serial schedule $T_1T_2$ or $T_2T_1$ as shown in \figref{adv}.(d). Hence, some conflicts of RWSTMs does not matter at SVOSTMs which reduce the number of aborts and improve the concurrency using SVOSTMs.    


%Short running transactions with fewer conflicts in optimistic OSTMs performs better than pessimistic OSTMs \cite{Erb2012}. 
\noindent
\textbf{Starvation-Freedom}: For long-running transactions along with high conflicts, starvation can occur in SVOSTMs. So, SVOSTMs should ensure the progress guarantee as \emph{starvation-freedom} \cite[chap 2]{HerlihyShavit:AMP:Book:2012}. SVOSTMs is said to be \emph{\stf}, if a thread invoking a transaction $T_i$ gets the opportunity to retry $T_i$ on every abort (due to the presence of a fair underlying scheduler with bounded termination) and $T_i$ is not \emph{parasitic}, i.e., if scheduler will give a fair chance to $T_i$ to commit then $T_i$ will eventually return commit. If a transaction gets a chance to commit, still it is not committing because of the infinite loop or some other error such transactions are known as Parasitic transactions \cite{Bushkov+:Live-TM:PODC:2012}. 

We explored another well known non-blocking progress guarantee \emph{wait-freedom} for STM  which ensures every transaction commits regardless of the nature of concurrent transactions and the underlying scheduler \cite{HerlihyShavit:Progress:Opodis:2011}. However, Guerraoui and  Kapalka  \cite{Bushkov+:Live-TM:PODC:2012, tm-book} showed that achieving wait-freedom is impossible in dynamic STMs in which data-items (or keys) of transactions are not known in advance. So in this paper, we explore the weaker progress condition of \emph{\stfdm} for SVOSTM while assuming that the keys of the transactions are not known in advance.  

\noindent
\textbf{Related work on Starvation-free STMs:} Some researchers Gramoli et al. \cite{Gramoli+:TM2C:Eurosys:2012}, Waliullah and Stenstrom \cite{WaliSten:Starve:CC:2009}, Spear et al. \cite{Spear+:CCM:PPoPP:2009}, Chaudhary et al. \cite{Chaudhary+:KSFTM:Corr:2017} have explored starvation-freedom in RWSTMs. Most of them assigned priority to the transactions. On conflict, higher priority transaction returns commit whereas lower priority transaction returns abort. On every abort, a transaction retries a sufficient number of times, will eventually get the highest priority and returns commit.
We inspired with these researchers and propose a novel \emph{Starvation-Free SVOSTM (SF-SVOSTM)} which assigns the priority to the transaction on conflict. In SF-SVOSTM whenever a conflicting transaction $T_i$ aborts, it retries with $T_j$ which has higher priority than $T_i$. To ensure the \stfdm, this procedure will repeat until $T_i$ gets the highest priority and eventually returns commit.%

% Here, each transaction maintains two timestamps, \emph{Initial Timestamp} ($its$) and \emph{Current Timestamp} ($cts$). Whenever  a transaction $T_i$ starts for the first time, it gets a unique timestamp $i$ using \emph{STM\_begin()} as $its$ which is equal to $cts$ as well. On abort $T_i$ gets new timestamp as $cts$ but it retains same $its$. Consider the \figref{sostm}.(b) in which $T_{1,1}$ as $T_{\langle cts, its \rangle }$ represents the first incarnation of $T_1$ so, $cts$ equals to $its$ as 1. $T_{1,1}$ conflicts with $T_{2,2}$ and $T_{3,3}$. As $T_{1,1}$ have the lowest $its$ so $T_1$  gets the priority to execute whereas $T_{2,2}$ and $T_{3,3}$ return aborts. On abort, $T_{2,2}$ and $T_{3,3}$ retries with new $cts$ 4 and 5 but with same $its$ 2 and 3 respectively. So, due to lowest $its$ $T_{4,2}$ returns commit but $T_{5,3}$ returns abort and so on. Hence, none of the transaction starves. So, when conflicts occur assigning priority to the lowest $its$ transaction ensures the \stfdm in OSTMs.  

\vspace{.2mm}
\begin{figure}
	\centerline{\scalebox{0.36}{\input{figs/advmvostmNEW.pdf_t}}}
	\vspace{-.2cm}	\caption{Benefits of Starvation-Free Multi-Version OSTM over SF-SVOSTM}
	\label{fig:advmvostm}
\end{figure} 



\noindent
\textbf{Motivation to Propose Starvation-Freedom in Multi-Version OSTM}: In SF-SVOSTM, if the highest priority transaction becomes slow (for some reason) then it may cause several other transactions to abort and bring down the progress of the system. \figref{advmvostm}.(a). demonstrates this in which the highest priority transaction $T_1$ became slow so, it is forcing the conflicting transactions $T_2$ and $T_3$ to abort again and again until $T_1$ commits. Database, RWSTMs \cite{Kumar+:MVTO:ICDCN:2014,LuScott:GMV:DISC:2013,Fern+:LSMVSTM:PPoPP:2011,Perel+:2011:SMV:DISC} and SVOSTMs \cite{Juyal+:SSS:2018} say that maintaining multiple versions corresponding to each key reduces the number of aborts and improves throughput.% OSTMs maintains single version corresponding to each key whereas \emph{Multi-Version OSTM} (or MVOSTM) \cite{Juyal+:SSS:2018} maintains multiple versions corresponding to each key which improves the concurrency further. 

So, this paper proposes the first \emph{Starvation-Free Multi-Version OSTM (SF-MVOSTM)} which maintains multiple versions corresponding to each key. \figref{advmvostm}.(b). shows the benefits of using SF-MVOSTM in which $T_1$ lookups from the older version with value $v_0$ created by transaction $T_0$ (assuming as initial transaction) for key $k_1$ and $k_4$. Concurrently, $T_2$ and $T_3$ create the new versions for key $k_4$. So, all the three transactions commit with equivalent serial schedule $T_1T_2T_3$. So, SF-MVOSTM improves the concurrency than SF-SVOSTM while reducing the number of aborts and ensures the \stfdm.



%Proposed SF-MVOSTM, SF-MVOSTM-GC, SF-KOSTM ensure the progress guarantee as \stfdm and correctness criteria as local opacity \cite{KuznetsovPeri:Non-interference:TCS:2017}. 

%We develop the SF-OSTM and SF-MVOSTM for the \emph{hash table (or ht)} as HT-SF-OSTM and HT-SF-MVOSTM and for \emph{linked-list (or list)} as list-SF-OSTM and list-SF-MVOSTM. SF-OSTM and SF-MVOSTM are generic for other data structures as well. 
%We implement two variants of SF-MVOSTM and compare its performance: (1) SF-MVOSTM without \emph{garbage collection} (or gc) (2) SF-MVOSTM with gc (or SF-MVOSTM-GC): It deletes the unwanted versions from version list of keys. (3) Finite version of SF-MVOSTM as SF-KOSTM which stores finite say $K$ number of versions corresponding to each key $k$. After creation of $K$ version, $K+1$ version replaces the oldest version. 

\noindent
\textbf{Contributions of the paper:}  We propose two Starvation-Free OSTMs as follows:
\vspace{-.1cm}
\begin{itemize}
\item Initially, we propose Starvation-Freedom for Single-Version OSTM as SF-SVOSTM which satisfies correctness criteria as \emph{conflict-opacity (or co-opacity)}\cite{Peri+:OSTM:Netys:2018}.
\item To achieve the greater concurrency further, we propose Starvation-Freedom for Multi-Version OSTM as SF-MVOSTM in \secref{pm} which maintains multiple versions corresponding to each key and satisfies the correctness as \emph{local opacity} \cite{KuznetsovPeri:Non-interference:TCS:2017}.
\item We propose SF-SVOSTM and SF-MVOSTM for \emph{hash table} and \emph{linked-list} data structure describe in \subsecref{dsde} but its generic for other data structures as well.
\item SF-MVOSTM works for unbounded versions with \emph{Garbage Collection (GC)} as SF-MVOSTM-GC which deletes the unwanted versions from version list of keys and for bounded/finite versions as SF-KOSTM which stores finite say latest $K$ number of versions corresponding to each key $k$. So, whenever any thread creates $(K+1)^{th}$ version of key, it replaces the oldest version of it. The most challenging task is achieving \stfdm in bounded version OSTM because say, a highest priority transaction rely on the oldest version that has been replaced. So, in this case highest priority transaction has to return abort and hence make it harder to achieve starvation-freedom unlike the approach follow in SF-SVOSTM. Thus, in this paper we propose a novel approach SF-KOSTM which bridges the gap by developing \stf OSTM while maintaining bounded number of versions. 
%\item \subsecref{dsde} describes design and data structure of 
\item \secref{exp} shows that SF-KOSTM is best among all propose Starvation-Free OSTMs (SF-SVOSTM, SF-MVOSTM, and SF-MVOSTM-GC) for both hash table and linked-list data structure. Proposed hash table based SF-KOSTM (HT-SF-KOSTM) performs 3.9x, 32.18x, 22.67x, 10.8x and 17.1x average speedup on \emph{max-time} for a transaction to commit than state-of-the-art STMs HT-KOSTM \cite{Juyal+:SSS:2018}, HT-SVOSTM \cite{Peri+:OSTM:Netys:2018}, 
ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, RWSTM \cite [Chap. 4]{ WeiVoss:TIS:2002:Morg}, and HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014} respectively. Proposed list based SF-KOSTM (list-SF-KOSTM)  performs 2.4x, 10.6x, 7.37x, 36.7x, 9.05x, 14.47x, and 1.43x average speedup on \emph{max-time} for a transaction to commit than state-of-the-art STMs list-KOSTM \cite{Juyal+:SSS:2018}, list-SVOSTM \cite{Peri+:OSTM:Netys:2018}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, and list-KSFTM \cite{Chaudhary+:KSFTM:Corr:2017} respectively.

%list-KOSTM \cite{Juyal+:SSS:2018}, list-SVOSTM \cite{Peri+:OSTM:Netys:2018}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, and list-KSFTM \cite{Chaudhary+:KSFTM:Corr:2017}, 

\end{itemize}
%\noindent



==> Arxiv SFKOSTM SSS19/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

%\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}

%\newtheorem{definition}{Definition}

\newcounter{history}
\newcommand{\hist}[1]{\refstepcounter{history} {#1}}

%\newcommand{\proof}[1][]{\noindent{\bf\boldmath
 %                         P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------Theorem Notations Defined by Petr --------------------------------------------------------------------------------------------------------
%% Defined by Petr

%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{observation}{Observation}


%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Fig~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{Step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\insref}[1]{line~\ref{ins:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

\newcommand{\linref}[1]{Line~\ref{lin:#1}}
%\newcommand{\algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}
\newcommand{\algoref}[1]{{Algo~\ref{algo:#1}}}
\newcommand{\subsecref}[1]{SubSection{\ref{subsec:#1}}}

\newcommand{\histref}[1]{\ref{hist:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{eq(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}
\newcommand{\Confref}[1]{Conflict~\ref{conf:#1}}




\newcommand{\theqed}{$\Box$}


\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}


%------------------------------------------------------------------------------------------------------------------
% Definitions for Object STM paper
%------------------------------------------------------------------------------------------------------------------
%

\newcommand{\tobj} {t-object\xspace}
\newcommand{\txns}[1] {txns(#1)}
\newcommand {\comm}[1] {committed(#1)}
\newcommand {\aborted}[1] {aborted(#1)}
\newcommand {\incomp}[1] {incomp(#1)}
\newcommand {\live}[1] {live(#1)}
\newcommand {\term}[1] {term(#1)}
\newcommand {\key}[1] {key(#1)}
\newcommand {\confevt}[1] {conf-event(#1)}
\newcommand {\confmth}[1] {conf-method(#1)}
\newcommand {\conf}[1] {conflict(#1)}
\newcommand {\confc}[1] {Conf}
\newcommand {\termn}[1] {terminate(#1)}

\newcommand {\tcomp} {t-complete\xspace}
\newcommand {\tinc} {t-incomplete\xspace}

\newcommand{\ssch} {sub-history}
\newcommand{\sschs} {sub-histories}

\newcommand{\nseq} {non-sequential}
\newcommand{\tseq} {t-sequential\xspace}
%\newcommand{\seq} {sequential}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}

\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\vwrite} {valWrite}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastup} {lastUpdt}
\newcommand{\lupdt}[2] {#2.lastUpdt(#1)}
\newcommand{\lseen}[2] {#2.lastSeen(#1)}

\newcommand{\mr} {MR}
\newcommand{\tr} {TR}

%\newcommand{\valid} {valid}
\newcommand{\validity} {validity\xspace}
\newcommand{\legal} {legal\xspace}
\newcommand{\legality} {legality\xspace}

\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}
%\newcommand{\rvmt} {rv\_method\xspace}
%\newcommand{\upmt} {upd\_method\xspace}
\newcommand{\rvp} {\emph{\rvmt execution} phase}
\newcommand{\cp} {\emph{\upmt execution} phase}

\newcommand{\termop} {terminal operation\xspace}
\newcommand{\cc} {correctness-criterion\xspace}
\newcommand{\ccs} {correctness-criteria\xspace}
\newcommand{\gen}[1] {gen(#1)}

\newcommand{\inv} {$inv$}
\newcommand{\rsp} {$rsp$}
\newcommand{\rmw} {rmw}
\newcommand{\first}[1] {first(#1)}
\newcommand{\last}[1] {last(#1)}

\newcommand{\evts}[1] {evts(#1)}
\newcommand{\met}[1] {methods(#1)}

\newcommand{\sgt} {SGT\xspace}
\newcommand{\memop} {memory operation\xspace}
\newcommand{\pref}[2] {#2.prefix(#1)}

\newcommand{\init} {\emph{init}\xspace}
\newcommand{\tbeg} {\emph{STM\_begin}\xspace}
\newcommand{\tread} {\emph{STM\_read}\xspace}
\newcommand{\twrite} {\emph{STM\_write}\xspace}
\newcommand{\tins} {\emph{STM\_insert}\xspace}
\newcommand{\tdel} {\emph{STM\_delete}\xspace}
\newcommand{\tlook} {\emph{STM\_lookup}\xspace}
\newcommand{\tryc} {\emph{STM\_tryC}\xspace}%{\emph{tryC}}
\newcommand{\trya} {\emph{STM\_tryA}\xspace}%{\emph{tryA}}


\newcommand{\failed} {failed\xspace}
\newcommand{\unaborted} {unaborted\xspace}

%\newcommand{\ins} {\emph{list\_insert}}
%\newcommand{\del} {\emph{list\_del}}
%\newcommand{\look} {\emph{list\_lookup}}

\newcommand{\inss} {\emph{list\_insert}}
\newcommand{\dell} {\emph{list\_del}}
\newcommand{\lookk} {\emph{list\_lookup}}

\newcommand{\ins} {\emph{lsl\_ins}\xspace}
\newcommand{\del} {\emph{lsl\_del}\xspace}
\newcommand{\look} {\emph{lsl\_Search}\xspace}

\newcommand{\rv} {\emph{rv}}
\newcommand{\up} {\emph{up}}

\newcommand{\rset}[1] {rset(#1)}
\newcommand{\wset}[1] {wset(#1)}
\newcommand{\rvar} {readVar}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co\text{-}opacity\xspace}

\newcommand{\vwc} {VWC\xspace}
\newcommand{\lo} {LO\xspace}
\newcommand{\lopty} {LO\xspace}
\newcommand{\lopq} {locally-opaque\xspace}

\newcommand{\tab} {hash-table\xspace}
\newcommand{\set}{table\xspace}
\newcommand{\llist} {list\xspace}
\newcommand{\otm} {\textit{OSTM}\xspace}%{ObjSTM}
\newcommand{\sotm} {\textit{SV-OSTM}\xspace}%{ObjSTM}

\newcommand{\rwtm} {\textit{RWSTM}\xspace}
%\newcommand{\lotm} {Table-OSTM}
\newcommand{\lotm} {OSTMs\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\bst} {BST\xspace}
\newcommand{\lsl} {rblazy\text{-}list\xspace}
\newcommand{\lazy} {lazy-list\xspace}

\newcommand{\csr} {CSR\xspace}

\newcommand{\perm} {permissive\xspace}
\newcommand{\pness} {permissiveness\xspace}
\newcommand{\permfn}[1] {perm(#1)}

\newcommand{\sspec} {sequential-specification\xspace}
\newcommand{\samp} {sample-stm\xspace}

\newcommand{\cg}[1] {CG(#1)}

\newcommand{\uset} {updtSet\xspace}
\newcommand{\lset} {lookupSet\xspace}
\newcommand{\rvm} {\emph{rvm}\xspace}
%\newcommand{\ht} {\emph{hash table}}

\newcommand{\firste} {firstEvt\xspace}
\newcommand{\laste} {lastEvt\xspace}
\newcommand{\fevt}[1] {#1.firstEvt}
\newcommand{\levt}[1] {#1.lastEvt}

\newcommand{\fkmth}[3] {#3.firstKeyMth(#1, #2)}
\newcommand{\pkmth}[3] {#3.prevKeyMth(#1, #2)}

\newcommand{\bstu} {\emph{bst-update}}
\newcommand{\lllist} {locallog\_list}

\newcommand{\udset}[1] {updtSet(#1)}
\newcommand{\rvset}[1] {rvSet(#1)}
%\newcommand{\bst}{BST}

\newcommand{\refr}[1]{refNode(#1)}
\newcommand{\lin}[1]{#1.LP\xspace}

%\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\newcommand\tabspace[1][1cm]{\hspace*{#1}}

%%%%%%% DS macros
%\newcommand{\glslhead}{getLslHead($obj\_id \downarrow, key \downarrow$)}


%\newcommand{\txlfind} {\textup{translog.find\_in\_loclog}$(obj\_id \downarrow, key \downarrow)$}
\newcommand{\txgid} {txlog.getTid()}
%\newcommand{\txgllist} {txlog.getLlList($t_{i} \downarrow$)}
\newcommand{\txsetst}[1] {L\_txlog.setStatus($L\_txstatus \downarrow$, $ OK \downarrow$)}
\newcommand{\txbegin}[1] {begin(#1)}

%\newcommand{\lsls}[1] {list\_lookup($obj\_id \downarrow,  key \downarrow, knext \uparrow, value \uparrow$, #1)}

\newcommand{\rvvalidate} {rvValidate($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

%\newcommand{\lslins}[1] {lslIns($preds[] \downarrow$, $currs[] \downarrow$, #1)}
\newcommand{\lsldel} {lslDel($preds[] \downarrow$, $currs[] \downarrow$)}


%\newcommand{\rlsol} {releaseOrderedLocks($ordered\_ll\_list \downarrow$)}

\newcommand{\ctov} {commitTOValidation($ll\_entry_i \downarrow$)}
\newcommand{\rvtov} {rvTOValidation($ key \downarrow$, $curr \downarrow$)}
\newcommand{\toval} {toValidation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}
\newcommand{\validation} {validation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}


\newcommand{\ifvalidation} {$$\textup{interferenceValidation}$(preds[] \downarrow, currs[] \downarrow)$$}
%\newcommand{\handlea}{tryAbort($obj\_id \downarrow$)}

%\newcommand{\llsort}{ll.sort ($ll\_list \downarrow$)}

%%---------------------macro w/o parameter

\newcommand{\npctov} {\emph{commitTOValidation()}}
\newcommand{\nptov} {\emph{toValidation()}}
\newcommand{\npintv} {\emph{intraTransValidation()}}
\newcommand{\nptc} {\emph{STM tryC()}}
\newcommand{\npins} {\emph{STM insert()}}
\newcommand{\npdel} {\emph{STM delete()}}
\newcommand{\npluk} {\emph{STM lookup()}}
\newcommand{\nplsls} {\emph{list\_lookup()}}
\newcommand{\nplsldel} {\emph{lslDel()}}
\newcommand{\nplslins} {\emph{list\_Ins()}}
\newcommand{\npbegin} {\emph{STM begin}}
\newcommand{\nppoval} {\emph{lostUpdateValidation()}}
\newcommand{\tcins} {\emph{tryC_{ins}}}
\newcommand{\npcld}{\emph{commonLu\&Del()}}


\newcommand{\rn} {\textcolor{red}{RL}\xspace}
\newcommand{\bn} {\textcolor{blue}{BL}\xspace}

\newcommand{\rc} {\textcolor{red}{currs[0]}}
\newcommand{\bc} {\textcolor{blue}{currs[1]}}
\newcommand{\bp} {\textcolor{blue}{preds[0]}}
\newcommand{\rp} {\textcolor{red}{preds[1]}}


\newcommand{\eevts}[1] {#1.evts}
\newcommand{\hst}[1] {#1.hist\xspace}
\newcommand{\exec}[1] {#1.exec\xspace}
%\newcommand{\state}[1] {#1.state\xspace}
\newcommand{\alls}[1] {#1.allStates\xspace}
\newcommand{\pres}[1] {#1.pre\text{-}state\xspace}
\newcommand{\posts}[1] {#1.post\text{-}state\xspace}

\newcommand{\shist}[2] {#2.subhist(#1)}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subh}  {sub\text{-}history\xspace}

\newcommand{\preds} {preds[]}
\newcommand{\currs} {currs[]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mvotm} {\textit{MVOSTM}\xspace}
\newcommand{\mvotms} {\textit{MV-OSTM}\xspace}
\newcommand{\hmvotm} {\textit{HT-MVOSTM}\xspace}
\newcommand{\lmvotm} {\textit{list-MVOSTM}\xspace}
\newcommand{\hotm} {\textit{HT-OSTM}\xspace}
\newcommand{\kotm} {\textit{KOSTM}\xspace}
\newcommand{\hkotm} {\textit{HT-KOSTM}\xspace}
\newcommand{\lkotm} {\textit{list-KOSTM}\xspace}
\newcommand{\mvotmgc} {\textit{MVOSTM-GC}\xspace}
\newcommand{\hmvotmgc} {\textit{HT-MVOSTM-GC}\xspace}
\newcommand{\lmvotmgc} {\textit{list-MVOSTM-GC}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% Local %%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\llog} {txLog\xspace}

\newcommand{\txlfind} {$L\_txlog.find(L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow)$}
\newcommand{\txll} {$L\_txlog$}
\newcommand{\txllf} {$L\_txlog()$}
\newcommand{\llsopn}[1] {$L\_rec.setOpn(L\_obj\_id \downarrow$, $L\_key \downarrow$, #1)}
\newcommand{\llsval}[1] {$L\_rec.setVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}
\newcommand{\llsopst}[1] {$L\_rec.setOpStatus(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}

\newcommand{\llgopn}[1] {$L\_rec.getOpn(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsopn}[1] {$L\_getOpn((obj\_id \downarrow$, $key \downarrow$, #1)}

\newcommand{\llgval}[1] {$L\_rec.getVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsval}[1] {loclog.getVal($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llspc} {$L\_rec.setPred\&Curr(L\_obj\_id \downarrow$, $ L\_key \downarrow$, $G\_pred \downarrow$, $G\_curr \downarrow$)}

\newcommand{\llgaptc}[1] {$L\_rec.getAptCurr$(#1)}
\newcommand{\llgkeyobj} {$L\_rec.getKey\&Objid(L\_rec_{i} \downarrow$)}

\newcommand{\llgopst} {$L\_rec.getOpStatus(L\_obj\_id \downarrow$, $L\_key \downarrow$)}
%\newcommand{\llsopst}[1] {loclog.getOpStatus($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llgallpc}{$L\_rec.getAllPreds\&Currs(L\_rec_{i} \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}

\newcommand{\poval}{lostUpdateValidation($L\_rec_{i}\downarrow$, $preds[]\uparrow$, $currs[]\uparrow$ )}

\newcommand{\llsort}{$L\_txlog.sort$($L\_list \downarrow$)}

\newcommand{\txgllist} {$L\_txlog.getList(L\_t\_id \downarrow$)}

\newcommand{\cld}{$commonLu\&Del$($L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$)}
%%%%%%%%%%%%%%%%%%%% Global %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cnt} {cnt}
\newcommand{\livetx} {live\_trans}
\newcommand{\gi} {$get\&inc(cnt \downarrow)$}
\newcommand{\glslhead}{getListHead($L\_obj\_id \downarrow, L\_key \downarrow$)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%From MVTO%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\copg}[2] {CG(#1, #2)}
\newcommand{\lopg}[2] {OG(#1, #2)}

\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}

\newcommand{\mv} {mv}
\newcommand{\rvf} {rvf}
\newcommand{\rt} {rt}
\newcommand{\rvmt} {rv\_method\xspace}
\newcommand{\upmt} {upd\_method\xspace}

%\newcommand{\op} {operation}
\newcommand{\checkv} {check\_versions}
\newcommand{\remid} {removeId}
\newcommand{\instup} {ins\_tuple}
\newcommand{\gc} {gc}
\newcommand{\liveset} {liveSet}
\newcommand{\livel} {liveList}
\newcommand{\locko} {lockOrder}
\newcommand{\mvto} {MV-OSTM}
\newcommand{\valid} {valid}
\newcommand{\seq}[2] {linearize(#2, #1)}
\newcommand{\stl}[3] {#3.stl(#1, #2)}
%\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\aco} {accessOrder}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% methods%%%%%%%%%%%%%%%%%%

\newcommand{\lsls}[1] {list\_lookup($L\_obj\_id \downarrow,  L\_key \downarrow, pred \uparrow, curr \uparrow$)}
\newcommand{\find} {find\_lts}
\newcommand{\handlea}{return ABORT}
\newcommand{\lslins}[1] {list\_Ins($pred \downarrow$, $curr \downarrow$, $node \uparrow$)}
\newcommand{\rlsol} {releaseOrderedLocks($L\_list \downarrow$)}

\newcommand{\mvperm} {mv-permissive\xspace}
\newcommand{\mvpness} {mv-permissiveness\xspace}

\newcommand {\cmnts}[1] {\State{\textcolor{gray}{/* #1 */} }}
\renewcommand{\thefootnote}{\arabic{footnote}}	

%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
\algrenewcommand{\algorithmiccomment}[1]{/* #1 */}

\newcommand{\stfdm} {starvation\text{-}freedom\xspace}
\newcommand{\stf} {starvation\text{-}free\xspace}
\newcommand{\wtfdm} {wait\text{-}freedom\xspace}
\newcommand{\wtf} {wait\text{-}free\xspace}
\newtheorem{assumption}{Assumption}

\newcommand{\commit}{\mathcal{C}}
\newcommand{\abort}{\mathcal{A}}

\newenvironment{proofsketch}[1][Proof Sketch]{\noindent#1: }{\hfill $\qed$\\[0.4mm]} 
%\newcommand {\live}[1] {#1.live}
\newcommand {\inc} {incarnation\xspace}
\newcommand {\incs}[2] {#2.incarSet(T_#1)\xspace}
\newcommand {\itsen} {itsEnabled\xspace}
\newcommand {\itsenb}[2] {#2.itsEnabled(T_#1)\xspace}
\newcommand {\cdsen} {cdsEnabled\xspace}
\newcommand {\cdsenb}[2] {#2.cdsEnabled(T_#1)\xspace}
\newcommand {\finen} {finEnabled\xspace}
\newcommand {\finenb}[2] {#2.finEnabled(T_#1)\xspace}
\newcommand {\enbd} {finEnabled\xspace}
\newcommand {\enb}[2] {#2.finEnabled(T_#1)\xspace}
\newcommand{\tcts}[1] {cts_#1\xspace}
\newcommand{\tits}[1] {its_#1\xspace}
\newcommand{\twts}[1] {wts_#1\xspace}
\newcommand{\htlock}[2] {#2.lock_#1\xspace}
\newcommand{\htval}[2] {#2.vrt_#1\xspace}
\newcommand{\htstat}[2] {#2.state_#1\xspace}
\newcommand{\htits}[2] {#2.its_#1\xspace}
\newcommand{\htcts}[2] {#2.cts_#1\xspace}
\newcommand{\htwts}[2] {#2.wts_#1\xspace}
\newcommand{\htltl}[2] {#2.tltl_#1\xspace}
\newcommand{\htutl}[2] {#2.tutl_#1\xspace}
\newcommand{\ltl} {tltl\xspace}
\newcommand{\utl} {tutl\xspace}
\newcommand{\lock} {lock\xspace}
\newcommand{\val} {valid\xspace}
\newcommand{\stat} {state\xspace}

% Global counters for PCode
\newcommand{\gtcnt} {gcounter\xspace}
\newcommand{\gicnt} {idCntr\xspace}

% Global counters for References
\newcommand{\tcntr} {tCntr\xspace}

\newcommand{\incv} {incrVal\xspace}

%Per transaction shared variables
\newcommand{\glock} {lock\xspace}
\newcommand{\gval} {valid\xspace}
\newcommand{\gstat} {state\xspace}
\newcommand{\gits} {its\xspace}
\newcommand{\gcts} {cts\xspace}
\newcommand{\gwts} {wts\xspace}
\newcommand{\tltl} {tltl\xspace}
\newcommand{\tutl} {tutl\xspace}
%\newcommand{\tcts}[1] {cts_#1\xspace}
%\newcommand{\tits}[1] {its_#1\xspace}
%\newcommand{\twts}[1] {wts_#1\xspace}
\newcommand{\ttltl}[1] {tltl_#1\xspace}
\newcommand{\ttutl}[1] {tutl_#1\xspace}
\newcommand{\tlock}[1] {lock_#1\xspace}
\newcommand{\tval}[1] {vrt_#1\xspace}
\newcommand{\tstat}[1] {state_#1\xspace}
%\newcommand{\tcntr} {tCntr\xspace}
\newcommand{\syst} {sys\text{-}time\xspace}
\newcommand {\incset} {incarSet\xspace}
\newcommand {\incn} {incNum\xspace}
\newcommand {\inum}[1] {T_#1.incNum\xspace}
\newcommand {\ninc} {nextInc\xspace}
\newcommand {\aptr} {application-transaction\xspace}
\newcommand {\nexti}[1] {T_#1.nextInc\xspace}
%\newcommand {\incs}[2] {#2.incarSet(T_#1)\xspace}
%\newcommand {\incset} {incarSet\xspace}
\newcommand {\inct}[2] {#2.incarCt(T_#1)\xspace}
\newcommand {\incct} {incarCt\xspace}
\newcommand {\affset} {affectSet\xspace}
\newcommand {\haffset}[2] {#2.affectSet(T_#1)\xspace}
%\newcommand {\affset} {affectSet\xspace}
\newcommand {\hmaxwts}[2] {#2.maxWTS(T_#1)\xspace}
\newcommand {\maxwts} {maxWTS\xspace}
\newcommand {\haffwts}[2] {#2.affwts(T_#1)\xspace}
\newcommand {\affwts} {affWTS\xspace}
\newcommand {\cdset} {cds\xspace}
\newcommand {\tcds}[1] {T_#1.cds\xspace}
\newcommand {\hcds}[2] {#2.cds(T_#1)\xspace}
\newcommand{\shset}[1] {#1.subhistSet\xspace}
\newcommand{\stsble} {strict\text{-}serializable\xspace}



%\newcommand{\shist}[2] {#2.subhist(#1)\xspace}
%\newcommand{\subhist} {subhist\xspace}
\newcommand{\subhs} {subhistSet\xspace}
%\newcommand{\shset}[1] {#1.subhistSet\xspace}

\newcommand{\termed}[1] {#1.terminated\xspace}
%\newcommand {\incct} {incarCt\xspace}
%\newcommand{\its} {its\xspace}
\newcommand{\ksftm} {\textit{SF-KOSTM}\xspace}
\newcommand{\cts} {cts\xspace}
\newcommand{\its} {its\xspace}
\newcommand{\wts} {wts\xspace}
%\newcommand{\syst} {sys\text{-}time\xspace}
\newcommand{\hsyst}[1] {#1.sys\text{-}time\xspace}
\newcommand{\begt} {stm\text{-}begin\xspace}
\newcommand{\ct} {comTime\xspace}
\newcommand{\vt} {\texttt{vrt}\xspace}
\newcommand{\csref}[1]{Case~\ref{case:#1}}
\newcommand{\lrl} {largeRL\xspace}
\newcommand{\abl} {abortRL\xspace}
\newcommand{\srl} {smallRL\xspace}
\newcommand {\cis} {cis\xspace}
\newcommand {\hcis}[2] {#2.cis(T_#1)\xspace}
\newcommand {\depits} {depits\xspace}
\newcommand {\hdep}[2] {#2.depits(T_#1)\xspace}
\newcommand {\pawts} {partAffwts\xspace}
\newcommand {\hpawts}[2] {#2.partAffwts(T_#1)\xspace}

==> Arxiv SFKOSTM SSS19/pm.tex <==
\vspace{-.1cm}
\section{The Proposed SF-KOSTM Algorithm}
\label{sec:pm}
\vspace{-.1cm}

In this section, we propose \emph{Starvation-Free K-version OSTM (SF-KOSTM)} algorithm which maintains $K$ number of versions corresponding to each key. The value of $K$ can vary from 1 to $\infty$. When $K$ is equal to 1 then SF-KOSTM boils down to \emph{Starvation-Free Single-Version OSTM (SF-SVOSTM)}. When $K$ is $\infty$ then SF-KOSTM maintains unbounded versions corresponding to each key known as \emph{Starvation-Free Multi-Version OSTM (SF-MVOSTM)} algorithm. To delete the unused version from the version list of SF-MVOSTM, it calls a separate Garbage Collection (GC) method \cite{Kumar+:MVTO:ICDCN:2014} and proposes SF-MVOSTM-GC.  In this paper, we propose SF-SVOSTM and all the variants of SF-KOSTM \emph{(SF-MVOSTM, SF-MVOSTM-GC, SF-KOSTM)} for two data structures \emph{hash table} and \emph{linked-list} but it is generic for other data structures as well.


\subsecref{prelim} describes the definition of \emph{starvation-freedom} followed by our assumption about the scheduler that helps us to achieve \stfdm in SF-KOSTM. \subsecref{dsde} explains the design and data structure of SF-KOSTM. \subsecref{working} shows the working of SF-KOSTM algorithm. 

%SF-MVOSTM maintains unlimited versions corresponding to each key which is taking more space to keep the versions and also increases the searching time to access the correct version corresponding to the key. This motivates us to apply the garbage collection (or GC) to delete the unwanted verions of the keys and we propose SF-MVOSTM-GC. We analyzed that SF-MVOSTM-GC is also taking enough space. So, 



\input{stardef}

\vspace{-.1cm}
\subsection{Design and Data Structure of SF-KOSTM Algorithm}
\label{subsec:dsde}
\vspace{-.1cm}
In this subsection, we show the design and underlying data structure of SF-KOSTM algorithm to maintain the shared data-items (or keys).% internally.   

To achieve the \emph{Starvation-Freedom} in \emph{K-version Object-based STM (SF-KOSTM)}, we use chaining hash table (or $ht$) as an underlying data structure where the size of the hash table is \emph{M} buckets as shown in \figref{dsdesign}.(a) and we propose HT-SF-KOSTM. Hash table with bucket size $one$ becomes the linked-list data structure for SF-KOSTM represented as list-SF-KOSTM.  The representation of SF-KOSTM is similar to MVOSTM \cite{Juyal+:SSS:2018}. Each bucket stores multiple nodes in the form of linked-list between the two sentinel nodes \emph{Head}(-$\infty$) and \emph{Tail}(+$\infty$). \figref{dsdesign}.(b) illustrates the structure of each node as $\langle$\emph{key, lock, mark, vl, nNext}$\rangle$. Where, \emph{key} is the unique value from the range of [1 to $\mathcal{K}$] stored in the increasing order between the two sentinel nodes similar to linked-list based concurrent set implementation \cite{Heller+:LazyList:PPL:2007, Harris:NBList:DISC:2001}. The \emph{lock} field is acquired by the transaction before updating (inserting or deleting) on the node. \emph{mark} is the boolean field which says anode is deleted or not. If \emph{mark} sets to true then node is logically deleted else present in the hash table. Here, the deletion is in a lazy manner similar to concurrent linked-list structure \cite{Heller+:LazyList:PPL:2007}. The field \emph{vl} stands for version list. SF-KOSTM maintains the finite say latest $K$-versions corresponding to each key to achieving the greater concurrency as explained in \secref{intro}. Whenever $(K+1)^{th}$ version created for the key then it overwrites the oldest version corresponding to that key. %So, SF-KOSTM maintains only $K$ versions corresponding to each key which make it space and time efficient to identify a correct version. 
 If $K$ is equal to 1, i.e., version list contains only one version corresponding to each key which boils down to \emph{Starvation-Free Single-Version OSTM (SF-SVOSTM)}. So, the data structure of SF-SVOSTM is same as SF-KOSTM with one version. The field \emph{nNext} points to next available node in the linked-list. From now onwards, we will use the term key and node interchangeably.
% \vspace{1mm}
 \begin{figure}
 	\centerline{\scalebox{0.35}{\input{figs/design.pdf_t}}}
\vspace{-.3cm} 	\caption{Design and Data Structure of SF-KOSTM}
 	\label{fig:dsdesign}
 \end{figure} 
% \vspace{1mm} 
\begin{figure}
	\centering
	\begin{minipage}[b]{0.48\textwidth}
		\centering
		\captionsetup{justification=centering}
		\scalebox{.36}{\input{figs/stmore.pdf_t}}
		 \vspace{-.5cm}
		\caption{Searching $k_9$ over \emph{lazy-list}}
		\label{fig:stmore}
	\end{minipage}   
	\hfill
	\begin{minipage}[b]{0.48\textwidth}
		\scalebox{.36}{\input{figs/stless.pdf_t}}
		\centering
		\captionsetup{justification=centering}
		 \vspace{-.5cm}
		\caption{Searching $k_9$ over $\lsl{}$}
		\label{fig:stless}
	\end{minipage}
\end{figure}
%\vspace{-.2cm}

\noindent
The structure of the \emph{vl} is $\langle$\emph{ts, val, rvl, vrt, vNext}$\rangle$ as shown in \figref{dsdesign}.(b). \emph{ts} is the unique timestamp assigned by the \tbeg{()}. If value (\emph{val}) is \emph{nil} then version is created by the \tdel{()} otherwise \tins{()} creates a version with not \emph{nil} value. To satisfy the correctness criteria as \emph{local opacity}, \tdel{()} also maintains the version corresponding to each key with \emph{mark} field as $true$. It allows the concurrent transactions to lookup from the older version of the marked node and returns the value as not \emph{nil}. \emph{rvl} stands for \emph{return value list} which maintains the information about lookup transaction that has lookups from a particular version. It maintains the timestamp (\emph{ts}) of \rvmt{s} (\tlook{()} or \tdel{()}) transaction in it. \emph{vrt} stands for \emph{version real time} which helps to maintain the \emph{real-time order} among the transactions. \emph{vNext} points to next available version in the version list. 

Maintaining the deleted node along with the live (not deleted) node will increase the traversal time to search a particular node in thelist. Consider \figref{stmore}, where red color depicts the deleted node $\langle k_1, k_2, k_4 \rangle$ and blue color depicts the live node $\langle k_9\rangle$. When any method of SF-KOSTM searches the key $k_9$ then it has to traverse the deleted nodes $\langle k_1, k_2, k_4 \rangle$ as well before reach to $k_9$ that increases the traversal time.  

This motivated us to modify the lazy-list structure of a node to form a skip list based on red and blue links. We called it as a \emph{red-blue lazy-list} or \emph{\lsl{}}. This idea has been explored by Peri et al. in SVOSTMs\cite{Peri+:OSTM:Netys:2018}. \emph{\lsl{}} maintains two-pointer corresponding to each node such as red link (\rn{}) and blue link (\bn{}). Where \bn{} points to the live node and \rn{} points to live node as well as deleted node. Let us consider the same example as discussed above with this modification, key $k_9$ is directly searched from the head of the list with the help of \bn{} as shown in \figref{stless}. In this case, traversal time is efficient because any method of SF-KOSTM need not traverse the deleted nodes. To maintain the \rn{} and \bn{} in each node we modify the structure of \emph{lazy-list} as $\langle \emph{key, lock, mark, vl, \rn, \bn, nNext} \rangle$ and called it as \emph{\lsl}.





\input{working}

==> Arxiv SFKOSTM SSS19/results.tex <==
\vspace{-.3cm}
\section{Experimental Evaluation}
%\section{Conclusion}
\label{sec:exp}
\vspace{-.2cm}
This section represents the experimental analysis of variants of the proposed Starvation-Free Object-based STMs (SF-SVOSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM)\footnote{Code is available here: https://github.com/PDCRL/SF-MVOSTM.} for two data structure \emph{hash table} (HT-SF-SVOSTM, HT-SF-MVOSTM, HT-SF-MVOSTM-GC and HT-SF-KOSTM)  and \emph{linked-list} (list-SF-SVOSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM) implemented in C++. We analyzed that HT-SF-KOSTM and  list-SF-KOSTM perform best among all the proposed algorithms. So, we compared our HT-SF-KOSTM with hash table based state-of-the-art STMs HT-KOSTM \cite{Juyal+:SSS:2018}, HT-SVOSTM \cite{Peri+:OSTM:Netys:2018}, 
ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, RWSTM \cite [Chap. 4]{ WeiVoss:TIS:2002:Morg}, HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014} %ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, RWSTM \cite [Chap. 4]{ WeiVoss:TIS:2002:Morg}, HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, HT-SVOSTM \cite{Peri+:OSTM:Netys:2018}, HT-KOSTM \cite{Juyal+:SSS:2018} 
and our list-SF-KOSTM with list based state-of-the-art STMs list-KOSTM \cite{Juyal+:SSS:2018}, list-SVOSTM \cite{Peri+:OSTM:Netys:2018}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, list-KSFTM \cite{Chaudhary+:KSFTM:Corr:2017}.  
%For a fair experimental evaluation we have implemented all our proposed variations of starvation free object based STMs in C++, and we have compared the performance against all the existing state-of-the-art algorithms depending on whether their data-structure is hash-table or list. Our Hash-Table implementation of SF-OSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM is compared with ESTM[1], RWSTM[2], MVTO[3], OSTM[4], KOSTM[5] and our list implementation is compared with NoRec[6], Translist[7], Boosting[8], OSTM[9], MVTO[3], OSTM[4], KOSTM[5].

\noindent
\textbf{Experimental Setup:} The system configuration for experiments is 2 socket Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 14 cores per socket and 2 hyper-threads per core, a total of 56 threads. A private 32KB L1 cache and 256 KB L2 cache is with each core. It has 32 GB RAM with Ubuntu 16.04.2 LTS running Operating System. Default scheduling algorithm of Linux with all threads have the same base priority is used in our experiments. This satisfies \asmref{bdtm}(bounded-termination) of the scheduler and we ensure the absence of parasitic transactions for our setup to satisfy \asmref{self}. %(bounded-termination) to hold. We completely ensure that no parasitic transactions[10] exists in our setup.

\begin{figure}
	\includegraphics[width=12cm, height=5cm]{figs/htli-comp.pdf}
\vspace{-.3cm}	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:htcomp}
\end{figure}

\noindent	
\textbf{Methodology:} %Irrespective of underlying data structures (hash table and linked-list) the methodology for our experiments remain same.
 We have considered three different types of workloads namely, W1 (Lookup Intensive - 5\% insert, 5\% delete, and 90\% lookup), W2 (Mid Intensive - 25\% insert, 25\% delete, and 50\% lookup), and W3 (Update Intensive - 45\% insert, 45\% delete, and 10\% lookup). To analyze the absolute benefit of starvation-freedom, we used a customized application called as the \emph{Counter Application} (refer the pseudo-code in \apnref{countercode}) which provides us the flexibility to create a high contention environment where the probability of transactions undergoing starvation on an average is very high. Our \emph{high contention} environment includes only 30 shared data-items (or keys), number of threads ranging from 50 to 250, each thread spawns upon a transaction, where each transaction performs 10 operations depending upon the workload chosen. To study starvation-freedom of various algorithms, we have used \emph{max-time} which is the maximum time required by a transaction to finally commit from its first incarnation, which also involves time taken by all its aborted incarnations. We perform each of our experiments 10 times and consider the average of it to avoid the effect of outliers. 
%\vspace{1.5cm}

%\vspace{1.5cm}

%\vspace{1.5cm}

\vspace{-.05cm}
\noindent
\textbf{Results Analysis:} All our results reflect the same ideology as proposed showcasing the benefits of Starvation-Freedom in Multi-Version OSTMs. We started our experiments with \emph{hash table} data structure of bucket size 5 and %observed that HT-SF-KOSTM performs best among all the proposed algorithms (HT-SF-SVOSTM, HT-SF-MVOSTM, HT-SF-MVOSTM-GC) on all the workloads (W1, W2, and W3) as shown in \figref{htus} of \apnref{ap-result}. So, we 
compared \emph{max-time} for a transaction to commit by proposed HT-SF-KOSTM (best among all the proposed algorithms shown in \figref{htus} of \apnref{ap-result}) with hash table based state-of-the-art STMs. HT-SF-KOSTM achieved an average speedup of 3.9x, 32.18x, 22.67x, 10.8x and 17.1x over HT-KOSTM, HT-SVOSTM, ESTM, RWSTM and HT-MVTO respectively as shown in \figref{htcomp}.

%So, we chose the HT-SF-KOSTM to compare against rest state-of-the-arts STMs with hash table data structure. \figref{htcomp} shows that HT-SF-KOSTM takes minimum \emph{max-time} for a transaction to commit, 

We further considered another data structure \emph{linked-list} and %analysed that list-SF-KOSTM performs best among all the proposed algorithms (list-SF-SVOSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC) on all the workloads (W1, W2, and W3) as shown in \figref{listus} of \apnref{ap-result}. So, in a next genuine step, we 
compared \emph{max-time} for a transaction to commit by proposed list-SF-KOSTM (best among all the proposed algorithms shown in \figref{listus} of \apnref{ap-result}) with list based state-of-the-arts STMs. %observed that list-SF-KOSTM beats all other algorithm by taking the minimum $max-time$ on an average for a transaction to commit under high contention, high starving environment as shown in \figref{listcomp}. list-SF-KOSTM 
list-SF-KOSTM achieved an average  speedup of 2.4x, 10.6x, 7.37x, 36.7x, 9.05x, 14.47x, and 1.43x over list-KOSTM, list-SVOSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO and list-KSFTM respectively as shown in \figref{listcomp}. We consider number of versions in the version list $K$ as 5 and value of C as 0.1. % which we found are the optimal values by experimenting and tuning these hyper-parameters across different workloads for hash table and linked-list as shown in \figref{htck} (a), (b) and \figref{listck} (a), (b) respectively of \apnref{ap-result}. %Additionally, we perform experiments to analyze the stability of our algorithm and observe that HT-SF-KOSTM and list-SF-KOSTM are indeed stable over the time as shown in \figref{htck} (c) and \figref{listck} (c) of \apnref{ap-result}. We have done lot more experiments to show the claim that achieving \stfdm reduces the max-time.

%\noindent
%For additional experiments please refer the \apnref{ap-result} which shows the performance of HT-SF-KOSTM and list-SF-KOSTM under \emph{low contention} is slightly lesser than non starvation-free HT-KOSTM and list-KOSTM. It also has plots of number of aborts while varying number of threads, best value of $K$ and $C$, $stability$ and \emph{memory consumption}.
 
 \begin{figure}
 	\includegraphics[width=12cm, height=5cm]{figs/List-comp.pdf}
\vspace{-.3cm} 	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on list}
 	\label{fig:listcomp}
 \end{figure}

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/htCK.pdf}
	\caption{ Optimal value of K and C along with Stability for hash table}
	\label{fig:htck}
\end{figure}

\noindent
\textbf{Best value of $K$, $C$, and Stability in SF-KOSTM:} We identified the  best value of $K$ for both HT-SF-KOSTM and list-SF-KOSTM algorithms. \figref{htck}.(a). demonstrates the best value of $K$ as 5 for HT-SF-KOSTM on counter application. We achieve this while varying value of $K$ on \emph{high contention environment} with 64 threads on all the workloads $W1, W2, W3$. \figref{htck}.(b). illustrates the best value of $C$ as 0.1 for HT-SF-KOSTM on all the workloads $W1, W2, W3$. \figref{htck}.(c). represents the $stability$ of HT-SF-KOSTM algorithm overtime for the counter application. For this experiment, we fixed 32 threads, 1000 shared data-items (or keys), the value of $K$ as 5, and $C$ as 0.1. Along with this, we consider, 5 seconds warm-up period on all the workloads $W1, W2, W3$. Each thread invokes transactions until its time-bound of 60 seconds expires.
We calculate the number of transactions committed in the incremental interval of 5 seconds. \figref{htck}.(c). shows that over time HT-SF-KOSTM is stable which helps to hold the claim that the performance of HT-SF-KOSTM will continue in the same manner if time is increased to higher orders. Similarly, we perform the same experiments for the linked-list data structure as well. \figref{listck}.(a). and \figref{listck}.(b). demonstrate the best value of $K$ as 5 and $C$ as 0.1 for list-SF-KOSTM on all the workloads $W1, W2, W3$. Similarly, \figref{listck}.(c). illustrates the $stability$ of list-SF-KOSTM and shows that it is stable over time on all the workloads $W1, W2, W3$.

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/listCK.pdf}
	\caption{ Optimal value of K and C along with Stability for list}
	\label{fig:listck}
\end{figure}
%Similarly, we calculate the best value of $K$ as 5 for \pkto on the same parameters. $C$, is a constant that is used to calculate $WTS$ of a transaction. i.e., $\twts{i} = \tcts{i} + C * (\tcts{i} - \tits{i});$ where, $C$ is any constant greater than 0. We run or experiments across load $W1$, for 64 threads and other parameters are same as defined in the methodology of \secref{exp}, we achieve the best value of $C$ as 0.1 for counter application. Experimental results are shown in \figref{optimalC} (b).
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-time-us.pdf}
	\caption{Time comparison among SF-SVOSTM and variants of SF-KOSTM on hash table}
	\label{fig:httimeus}
\end{figure}


We have done some experiments on \textit{low contention environment} which involves 1000 keys, threads varying from 2 to 64 in power of 2, each thread spawns one transaction and each transaction executes 10 operations (insert, delete and lookup) depending upon the workload chosen. We observed that HT-SF-KOSTM performs best out of all the proposed algorithms on $W1$ and $W2$ workload as shown in \figref{httimeus}. For a lesser number of threads on $W3$, HT-SF-KOSTM was taking a bit more time than other proposed algorithms as shown in \figref{httimeus}.(c). This may be because of the finite version, finding and replacing the oldest version is taking time. After that, we consider  HT-SF-KOSTM and compared against state-of-the-art STMs.  \figref{httimecomp} shows that our proposed algorithm performs better than all other state-of-art-STMs algorithms but slightly lesser than the non starvation-free HT-KOSTM. But to provide the guarantee of starvation-freedom this slight slag of time is worth paying. For the better clarification of speedups, please refer to \tabref{htspeed}.  Similarly, \figref{listtimeus} represents the analysis of \emph{low contention environment} for list data structure where list-SF-KOSTM performs best out of all the proposed algorithms. \figref{listtimecomp} demonstrates the comparison of proposed list-SF-KOSTM with list based state-of-the-art STMs and shows the significant performance gain in terms of a speedup as presented in \tabref{listspeed}. For low contention environment, starvation-freedom is appearing as an overhead so, both HT-SF-KOSTM and list-SF-KOSTM  achieve a bit less speedup than HT-KOSTM and list-KOSTM. But for high contention environment, starvation-free algorithms are always better so, both HT-SF-KOSTM and list-SF-KOSTM achieve better speedup than HT-KOSTM and list-KOSTM as explained in \secref{exp}.

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-time-comp.pdf}
	\caption{Time comparison of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:httimecomp}
\end{figure}


\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-time-us.pdf}
	\caption{Time comparison among SF-SVOSTM and variants of SF-KOSTM on list}
	\label{fig:listtimeus}
\end{figure}
%\vspace{1cm}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-time-comp.pdf}
	\caption{Time comparison of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listtimecomp}
\end{figure}

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-abort-us.pdf}
	\caption{Abort Count of SF-SVOSTM and variants of SF-KOSTM on hash table}
	\label{fig:htabortus}
\end{figure}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-abort-us.pdf}
	\caption{Abort Count of SF-SVOSTM and variants of SF-KOSTM on list}
	\label{fig:listabortus}
\end{figure}


\noindent
\textbf{Abort Count:} We analyzed the number of aborts on low contention environment as defined above. \figref{htabortus} and \figref{listabortus} show the number of aborts comparison among all the proposed variants in all three workloads W1, W2 and W3 for both data structures hash table and linked-list. The results show that HT-SF-KOSTM and list-SF-KOSTM have relatively less  number of aborts than other proposed algorithms. Similarly, \figref{htabortcomp} and \figref{listabortcomp} shows the number of aborts comparison among proposed HT-SF-KOSTM with hash table based state-of-the-art STMs and proposed list-SF-KOSTM with list based state-of-the-art STMs in all three workloads W1, W2, and W3. The result shows that the least number of aborts are happening with HT-SF-KOSTM and list-SF-KOSTM.
\noindent



%\vspace{1cm}

\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/ht-abort-comp.pdf}
	\caption{Abort Count of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:htabortcomp}
\end{figure}

%\vspace{1cm}
\begin{figure}[H]
	\includegraphics[width=12cm, height=5cm]{figs/list-abort-comp.pdf}
	\caption{Abort Count of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listabortcomp}
\end{figure}


\noindent
\textbf{Garbage Collection:} To delete the unwanted versions, we use garbage collection mechanism in SF-MVOSTM and proposed SF-MVOSTM-GC. The results show that SF-MVOSTM-GC performs better than SF-MVOSTM. Garbage collection method deletes the unwanted version corresponding to the key. In garbage collection we use a \textit{livelist}, this livelist contains all the transaction that are live, which means every transaction on the start of its first incarnation logs its time in livelist and when commit/abort remove its entry from livelist in sorted order of transactions on the basis of $wts$. Garbage collection is achieved by deleting the version which is not latest, whose timestamp is smaller than the $wts$ of smallest live transaction. \figref{mc} represents the \textbf{\emph{Memory Consumption}} by SF-MVOSTM-GC and SF-KOSTM algorithms for \emph{high contention (or HC)} and \emph{low contention (or LC)} environment on workload $W_3$ for the linked-list data structure. Here, each algorithm creates a version corresponding to the key after successful \emph{STM\_tryC()}. We calculate the memory consumption based on the \emph{Version Count (or VC)}. If version is created then VC is incremented by 1 and after garbage collection, VC is decremented by 1. \figref{mc}. (a). demonstrates that memory consumption is kept on increasing in SF-MVOSTM-GC but memory consumption by SF-KOSTM is constant because of maintaining finite versions corresponding to the less number of keys (high contention). \figref{mc}. (b). shows for \emph{low contention} environment where memory consumption are keeps on increasing in SF-MVOSTM-GC as well as SF-KOSTM. But once limit of $K$-version reach corresponding to all the keys in SF-KOSTM, memory consumption will be stable. Similar observation can be found for other workloads $W_1, W_2$ and other data structure hash table as well.

\begin{figure}[H]
	\centering
	\includegraphics[width=10cm, height=5cm]{figs/mc.pdf}
	\vspace{-.4cm}	\caption{Comparison of Memory Consumption in SF-KOSTM and SF-MVOSTM-GC}
	\label{fig:mc}
\end{figure}


\begin{table}[H]
	\small
	\begin{tabular}{ | m{4.5cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} | } 
		\hline
		Algorithm & W1 & W2 & W3 \\ 
		\hline
		HT-SF-SVOSTM & 1.49 & 1.13 & 1.09 \\
		\hline
		HT-SF-MVOSTM & 1.22 & 1.08 & 1.04 \\
		\hline
		HT-SF-MVOSTM-GC	& 1.13 & 1.03 & 1.02 \\
		\hline
		HT-SVOSTM & 3.3 & 0.77 & 1.57 \\
		\hline
		ESTM & 2.92 & 1.4 & 3.03 \\
		\hline
		RWSTM & 3.13 & 2.65 & 13.36  \\
		\hline
		HT-MVTO & 2.37 & 4.74 & 49.39  \\
		\hline
		HT-KOSTM & 0.91 & 0.7 & 0.8 \\
		\hline
		
		\hline
		
	\end{tabular}
	\captionsetup{justification=centering}
	\caption{Speedup by HT-SF-KOSTM  }
	\label{tab:htspeed}
\end{table}


\begin{table}[H]
	\small
	\begin{tabular}{ | m{4.5cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} | } 
		\hline
		Algorithm & W1 & W2 & W3 \\ 
		\hline
		list-SF-SVOSTM & 1.29 & 1.26 & 1.22 \\
		\hline
		list-SF-MVOSTM & 1.25 & 1.29 & 1.12 \\
		\hline
		list-SF-MVOSTM-GC	& 1.14 & 1.5 & 1.13 \\
		\hline
		list-SVOSTM & 2.4 & 1.5 & 1.4 \\
		\hline
		Trans-list & 24.15 & 19.06 & 23.26 \\
		\hline
		Boosting-list & 22.43 & 22.52 & 27.2  \\
		\hline
		NOrec-list & 26.12 & 27.33 & 31.05  \\
		\hline
		list-MVTO & 10.8 & 23.1 & 19.57  \\
		\hline
		list-KSFTM & 5.7 & 18.4 &  74.20 \\
		\hline
		list-KOSTM	 & 0.96 & 0.98 & 0.8 \\
		\hline
		
		\hline
		
	\end{tabular}
	\captionsetup{justification=centering}
	\caption{Speedup by list-SF-KOSTM  }
	\label{tab:listspeed}
\end{table}
%\vspace{-1cm}


%\vspace{-.02cm}
%First, we compared all our proposed HT-SF-OSTM and variations of HT-SF-MVOSTM which are HT-SF-MVOSTM, HT-SF-MVOSTM-GC (due to lack of space please find the implementation details in the \apnref{ap-result}), and HT-SF-KOSTM to find the best out of the all. \figref{htus} depicts that the finite version HT-SF-KOSTM performs best among all the proposed algorithms on all the three types of workloads (W1, W2, and W3) with value of $K$ and C as 5 and 0.1 respectively. Where $K$ is the number of versions in the version list and C is the variable used to define the $wts$. So, we chose the HT-SF-KOSTM to compare against rest state-of-the-arts STMs with hash table data structure. \figref{htcomp} shows that HT-SF-KOSTM takes minimum \emph{max-time} for a transaction to commit, and achieved an average speedup of 3.9x, 32.18x, 22.67x, 10.8x and 17.1x over HT-KOSTM, HT-OSTM, ESTM, RWSTM and HT-MVTO respectively.





 %All our results reflect the same ideology as proposed showcasing the benefits of starvation-free multi-version object based STMs. We started our experiments with hash table data structure of bucket size 5 as shown in \figref{htus}. First, we compared all our proposed HT-SF-OSTM and variations of HT-SF-MVOSTM which are HT-SF-MVOSTM, HT-SF-MVOSTM-GC (due to lack of space please find the implementation details in the \apnref{ap-result}), and HT-SF-KOSTM to find the best out of the all. \figref{htus} depicts that the finite version HT-SF-KOSTM performs best among all the proposed algorithms on all the three types of workloads (W1, W2, and W3) with value of $K$ and C as 5 and 0.1 respectively. Where $K$ is the number of versions in the version list and C is the variable used to define the $wts$. So, we chose the HT-SF-KOSTM to compare against rest state-of-the-arts STMs with hash table data structure. \figref{htcomp} shows that HT-SF-KOSTM takes minimum \emph{max-time} for a transaction to commit, and achieved an average speedup of 3.9x, 32.18x, 22.67x, 10.8x and 17.1x over HT-KOSTM, HT-OSTM, ESTM, RWSTM and HT-MVTO respectively.

%We further considered another data structure the linked-list and compared among all our proposed variants list-SF-OSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM. \figref{listus} represents that list-SF-KOSTM performs best for all the workloads. So, in a next genuine step, we compared list-SF-KOSTM with rest state-of-the-arts STMs  and observed that list-SF-KOSTM beats all other algorithm by taking the minimum $max-time$ on an average for a transaction to commit under high contention, high starving environment as shown in \figref{listcomp}. list-SF-KOSTM achieved an average  speedup of 2.4x, 10.6x, 7.37x, 36.7x, 9.05x, 14.47x, and 1.43x over list-KOSTM, list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO and list-KSFTM respectively.



%In all our experiments, we have taken value of K as 5 and value of C as 0.1 which we found are the optimal values by experimenting and tuning these hyper-parameters across different workloads for hash table and linked-list as shown in \figref{htck} (a), (b) and \figref{listck} (a), (b) respectively. Additionally, we perform experiments to analyze the stability of our algorithm. By \textit{stability} we refer to the number of transactions committed should be approximately same in increasing time intervals where each thread performs relatively large number of transactions. \figref{htck} (c) and \figref{listck} (c) displays that number of committed transactions are almost consistent in HT-SF-KOSTM and list-SF-KOSTM for all the workloads while varying time interval and considered 5 seconds as warm-up period. This shows indeed that algorithm proposed here is stable.  Please refer the \apnref{ap-result} for further experiments which involve performance of HT-SF-KOSTM and list-SF-KOSTM under low contention and number of aborts with varying number of threads.

==> Arxiv SFKOSTM SSS19/resultsold.tex <==
%\vspace{-0.3cm}
\section{Experimental Evaluation}
%\section{Conclusion}
\label{sec:exp}

This section represents the experimental analysis of variants of the proposed starvation free object-based STMs (SF-OSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM)\footnote{Code is available here: https://github.com/PDCRL/SF-MVOSTM.} for two data structure hash table (HT-SF-OSTM, HT-SF-MVOSTM, HT-SF-MVOSTM-GC and HT-SF-KOSTM)  and linked-list (list-SF-OSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM) implemented in C++. We analyzed that HT-SF-KOSTM and  list-SF-KOSTM perform best among all the proposed variants of STMs. So, we compared our HT-SF-KOSTM with hash table based state-of-the-art STMs ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, RWSTM \cite [Chap. 4]{ WeiVoss:TIS:2002:Morg}, HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, HT-OSTM \cite{Peri+:OSTM:Netys:2018}, HT-KOSTM \cite{Juyal+:SSS:2018} and our list-SF-KOSTM with list based state-of-the-art STMs NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, list-OSTM \cite{Peri+:OSTM:Netys:2018}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, list-KSFTM \cite{Chaudhary+:KSFTM:Corr:2017}, list-KOSTM \cite{Juyal+:SSS:2018}.  
%For a fair experimental evaluation we have implemented all our proposed variations of starvation free object based STMs in C++, and we have compared the performance against all the existing state-of-the-art algorithms depending on whether their data-structure is hash-table or list. Our Hash-Table implementation of SF-OSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM is compared with ESTM[1], RWSTM[2], MVTO[3], OSTM[4], KOSTM[5] and our list implementation is compared with NoRec[6], Translist[7], Boosting[8], OSTM[9], MVTO[3], OSTM[4], KOSTM[5].

\noindent
\textbf{Experimental Setup:} The system configuration for experiments is 2 socket Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 14 cores per socket and 2 hyper-threads per core, for a total of 56 threads. A private 32KB L1 cache and 256 KB L2 cache is with each core. It has 32 GB RAM with Ubuntu 16.04.2 LTS running Operating System. Default scheduling algorithms of Linux are used in our experiments, where all threads have the same base priority. This allows \asmref{bdtm}(bounded-termination) to hold and we ensure the absence of parasitic transactions for our setup that satisfies \asmref{self}. %(bounded-termination) to hold. We completely ensure that no parasitic transactions[10] exists in our setup.

\noindent	
\textbf{Methodology:} Irrespective of underlying data structures (hash table and linked-list) the methodology for our experiments remain same. We have considered three different types of workloads namely, W1 (Lookup Intensive (Li)- 8\% Insert, 2\% Delete, and 90\% Lookup), W2 (Mid Intensive (Mi) - 25\% Insert, 25\% Delete, and 50\% Lookup), and W3 (Update Intensive (Ui) - 45\% Insert, 45\% Delete, and 10\% Lookup) respectively. To analyze the absolute benefit of starvation-freedom we used a customized application called as the Counter application which provides us flexibility to create a high contention environment where the probability of transactions undergoing starvation on an average is very high. Our high contention environment includes only 30 keys, number of threads ranging from 50 to 250, each thread spawns upon a transaction, where each transaction performs 10 operations (Insert, Delete and Lookup) depending upon the workload chosen. To study starvation-freedom of various algorithms, we have used \emph{max-time} which is the maximum time required by a transaction to finally commit from its first incarnation, which also involves time taken by all its aborted incarnations. We perform each of our experiments 10 times and considered the average of these runs in order to avoid the effect of outliers. 


%\vspace{1.5cm}
\begin{figure}
	\includegraphics[width=12cm, height=5cm]{figs/htli-comp.pdf}
	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:htcomp}
\end{figure}


%\vspace{1.5cm}
\begin{figure}
	\includegraphics[width=12cm, height=5cm]{figs/List-comp.pdf}
	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listcomp}
\end{figure}
%\vspace{1.5cm}

%\vspace{1.5cm}


\noindent
\textbf{Results Analysis:} All our results reflect the same ideology as proposed showcasing the benefits of starvation-free multi-version object based STMs. We started our experiments with hash table data structure of bucket size 5 as shown in \figref{htus}. First, we compared all our proposed HT-SF-OSTM and variations of HT-SF-MVOSTM which are HT-SF-MVOSTM, HT-SF-MVOSTM-GC (due to lack of space please find the implementation details in the \apnref{ap-result}), and HT-SF-KOSTM to find the best out of the all. \figref{htus} depicts that the finite version HT-SF-KOSTM performs best among all the proposed algorithms on all the three types of workloads (W1, W2, and W3) with value of $K$ and C as 5 and 0.1 respectively. Where $K$ is the number of versions in the version list and C is the variable used to define the $wts$. So, we chose the HT-SF-KOSTM to compare against rest state-of-the-arts STMs with hash table data structure. \figref{htcomp} shows that HT-SF-KOSTM takes minimum \emph{max-time} for a transaction to commit, and achieved an average speedup of 3.9x, 32.18x, 22.67x, 10.8x and 17.1x over HT-KOSTM, HT-OSTM, ESTM, RWSTM and HT-MVTO respectively.

We further considered another data structure the linked-list and compared among all our proposed variants list-SF-OSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM. \figref{listus} represents that list-SF-KOSTM performs best for all the workloads. So, in a next genuine step, we compared list-SF-KOSTM with rest state-of-the-arts STMs  and observed that list-SF-KOSTM beats all other algorithm by taking the minimum $max-time$ on an average for a transaction to commit under high contention, high starving environment as shown in \figref{listcomp}. list-SF-KOSTM achieved an average  speedup of 2.4x, 10.6x, 7.37x, 36.7x, 9.05x, 14.47x, and 1.43x over list-KOSTM, list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO and list-KSFTM respectively.



In all our experiments, we have taken value of K as 5 and value of C as 0.1 which we found are the optimal values by experimenting and tuning these hyper-parameters across different workloads for hash table and linked-list as shown in \figref{htck} (a), (b) and \figref{listck} (a), (b) respectively. Additionally, we perform experiments to analyze the stability of our algorithm. By \textit{stability} we refer to the number of transactions committed should be approximately same in increasing time intervals where each thread performs relatively large number of transactions. \figref{htck} (c) and \figref{listck} (c) displays that number of committed transactions are almost consistent in HT-SF-KOSTM and list-SF-KOSTM for all the workloads while varying time interval and considered 5 seconds as warm-up period. This shows indeed that algorithm proposed here is stable.  Please refer the \apnref{ap-result} for further experiments which involve performance of HT-SF-KOSTM and list-SF-KOSTM under low contention and number of aborts with varying number of threads.

==> Arxiv SFKOSTM SSS19/stardef.tex <==
\vspace{-.2cm}
\subsection{Description of Starvation-Freedom}
\label{subsec:prelim}
\vspace{-.1cm}
%This subsection describes the definition of \stfdm followed by our assumption about the scheduler that helps us to achieve \stfdm in SF-KOSTM.
%\subsection{Transaction Inovcation \& Starvation Freedom}
%\subsection{Transaction Inovcation}
%\label{subsec:trans-inv} \todo{in-line this}
\vspace{-.1cm}
\begin{definition}
\label{defn:stf}
\textbf{Starvation-Freedom:} An STM system is said to be \stf if a thread invoking a non-parasitic transaction $T_i$ gets the opportunity to retry $T_i$ on every abort, due to the presence of a fair scheduler, then $T_i$ will eventually commit.
\end{definition}
\vspace{-.1cm}
Herlihy \& Shavit \cite{HerlihyShavit:Progress:Opodis:2011} defined the fair scheduler which ensures that none of the thread will crash or delayed forever. Hence, any thread $Th_i$ acquires the lock on the shared data-items while executing transaction $T_i$ will eventually release the locks. So, a thread will never block other threads to progress. To satisfy the \stfdm for SF-KOSTM, we assumed bounded termination for the fair scheduler.
\vspace{-.1cm}
\begin{assumption}
	\label{asm:bdtm}
	\textbf{Bounded-Termination:} For any transaction $T_i$, invoked by a thread $Th_i$, the fair system scheduler ensures, in the absence of deadlocks, $Th_i$ is given sufficient time on a CPU (and memory, etc) such that $T_i$ terminates ($\commit$ or $\abort$) in bounded time. 
\end{assumption}
\vspace{-.1cm}
In the proposed algorithms, we have considered \emph{TB} as the maximum time-bound of a transaction $T_i$ within this either $T_i$ will return commit or abort in the absence of deadlock. Approach for achieving the \emph{deadlock-freedom} is motivated from the literature in which threads executing transactions acquire the locks in increasing order of the keys and releases the locks in bounded time either by committing or aborting the transaction. We consider an assumption about the transactions of the system as follows.
\vspace{-.1cm}
\begin{assumption}
	\label{asm:self}
	We assume, if other concurrent conflicting transactions do not exist in the system then every transaction will commit. i.e. (a) If a transaction $T_i$ is executing in the system with the absence of other conflicting transactions then $T_i$ will not self-abort. (b) Transactions of the system are non-parasitic as explained in \secref{intro}.
\end{assumption}
\vspace{-.1cm}
\noindent If transactions self-abort or parasitic then ensuring \stfdm is impossible.


==> Arxiv SFKOSTM SSS19/sysmodel.tex <==
\vspace{-.6cm}
\section{System Model and Preliminaries}
\label{sec:sm}
This section follows the notion and definition described in \cite{Juyal+:SSS:2018,tm-book}, 
we assume a system of $n$ processes/threads, $th_1,\ldots,th_n$  that run in a completely asynchronous manner and communicate through a set of \emph{keys} $\mathcal{K}$ (or \emph{{transaction-object}s}). We also assume that none of the threads crash or fail abruptly. In this paper, a thread executes higher-level methods on $\mathcal{K}$ via atomic \emph{transactions} $T_1,\ldots,T_n$ and receives the corresponding response. 

\noindent
\textbf{Events and Methods:}
Threads execute the transactions with higher-level methods (or operations) which internally invoke multiple read-write (or lower-level) operations known as \emph{events} (or $evts$). 
%Each transaction has been identified by a unique identifier. 
Transaction $T_i$ of the system at read-write level invokes \emph{STM\_begin()}, \emph{STM\_read$_i$(k)},  \emph{STM\_write$_i$(k,v)}, \emph{STM\_tryC$_i$()} and \emph{STM\_tryA$_i$()} as defined in \secref{intro}. We denote a method $m_{ij}$ as the $j^{th}$ method of $T_i$. Method \emph{invocation} (or $inv$) and \emph{response} (or $rsp$) on higher-level methods are also considered as an event.

A thread executes higher-level operations on $\mathcal{K}$ via transaction $T_i$ are known as \emph{methods} (or $mths$). $T_i$ at object level (or higher-level) invokes \emph{STM\_begin()}, \emph{STM\_lookup$_i$($k$) (or $l_i(k)$)},  \emph{STM\_insert$_i$($k,v$) (or $i_i(k,v)$)}, \emph{STM\_delete$_i$($k$) (or $d_i(k)$)}, \emph{STM\_tryC$_i$()}, and  \emph{STM\_tryA$_i$()} methods described in \secref{intro}. %A transaction $T_i$ begins with unique timestamp $i$ using \emph{STM\_begin()} and completes with any of its operation which returns either commit as $\commit$ or abort as $\abort$. 
Here, \emph{STM\_lookup()}, and \emph{STM\_delete()} return the value from underlying data structure so, we called these methods as \emph{return value methods (or $\rvmt{s}$)}. Whereas, \emph{STM\_insert()}, and \emph{STM\_delete()} are updating the underlying data structure after successful \emph{STM\_tryC()} so, we called these methods as \emph{update} \mth{s} (or $\upmt{s}$).

% Object level methods internally calls multiple read/write operations known as \emph{events}. Method invocation and response are also considered as events.

\noindent
\textbf{Transactions:} We follow multi-level transactions\cite{WeiVoss:TIS:2002:Morg} model which consists of two layers. Layer 0 (or lower-level) composed of read-write operations whereas layer 1 (or higher-level) comprises of object-level methods which internally calls multiple read-write events. Formally, we define a transaction $T_i$ at higher-level as the tuple $\langle \evts{T_i}, <_{T_i}\rangle$, here $<_{T_i}$ represents the total order among all the events of $T_i$. 
%There are two terminal operations (commit or abort) for a transaction after that it won't execute any other operations. 
Transaction $T_i$ cannot invoke any more operation after returning commit ($\commit$) or abort ($\abort$). Any operation that returns $\commit$ or $\abort$ are known as \emph{\termop{s}} represented as $Term(T_i)$. The transaction which neither committed nor aborted is known as \emph{live transactions} (or $trans.live$).

\noindent
\textbf{Histories:} %A \emph{history} $H$ is a collection of multiple read/write events from different transactions. Hence, 
A history $H$ consists of multiple transactions, a transaction calls multiple methods and each method internally invokes multiple read-write events. So, a history is a collection of events belonging to the different transactions is represented as $\evts{H}$. Formally, we define a history $H$ as the tuple $\langle \evts{H}, <_H\rangle$, here $<_H$ represents the total order among all the events of $H$. If all the method invocation of $H$  match with the corresponding response then such history is known as \emph{complete history} denoted as $\overline{H}$. Suppose total transactions in $H$ is $H.trans$, in which number of committed and aborted transactions are $H.committed$ and $H.aborted$ then the \emph{incomplete history} or \emph{live history} is defined as: $H.incomp$ = $H.live$ = \emph{($H.trans$ - $H.committed$ - $H.aborted$)}. This paper considers only \emph{well-form history} which ensures (1) the response of the previous method has received then only the transaction $T_i$ can invoke another method. (2) transaction can not invoke any other method after receiving the response as $\commit$ or $\abort$. 
  
 \noindent
 \textbf{Sequential Histories:} Following \cite{KuznetsovPeri:Non-interference:TCS:2017, KuznetsovRavi:ConcurrencyTM:OPODIS:2011},  if all the methods of the history are complete and isolated from each other, i.e. all the methods of history are atomic and following the total order in $H$. So, with this assumption, the only relevant methods of a transaction $T_i$ are $l_i(k,v)$, 
 $l_i(k,\abort)$, $i_i(k, v)$, $d_i(k, v)$, $\tryc_i(\commit)$ (or $c_i$ for short), 
 $\tryc_i(\abort)$, and $\trya_i(\abort)$ (or $a_k$ for short). We form the complete history $\overline{H}$, by immediately inserting the abort to all the live transactions of $H$. But, if the first operation of \emph{STM\_tryC$_i$()} has returned successfully then $T_i$ returns commit.
 
 \noindent
 \textbf{Real-Time Order and Serial History:} Two complete method $m_{ij}$ and $m_{xy}$ are said to be in method real-time order (or MR), if the response of $m_{ij}$ happens before the invocation of $m_{xy}$. Formally, if ($rsp(m_{ij}) <_H inv(m_{xy})$)$\implies$($m_{ij} \prec_H^{\mr} m_{xy}$). Following \cite{Papad:1979:JACM}, if transaction $T_i$ terminates (either commits or aborts) before beginning of $T_j$ then $T_i$ and $T_j$  follows transaction real-time order (or TR). Formally, if ($Term(T_i) <_H \tbeg_j()$)$\implies$($T_i \prec_H^{\tr} T_j$).  If all the transactions of a history $H$ follow the real-time order, i.e. transactions are atomic then such history is known as \emph{serial} \cite{Papad:1979:JACM} or \emph{t-sequential} \cite{KuznetsovRavi:ConcurrencyTM:OPODIS:2011} history. % Since, transactions are atomic then implicitly methods will also be atomic so, any serial history will also be a sequential history.
 Formally, $\langle (H \text{ is serial}) \implies (\forall T_{i} \in \txns{H}: (T_i \in Term{(H)}) \land (\forall T_{i}, T_{j} \in \txns{H}: (T_{i} \prec_H^{\tr} T_{j}) \lor (T_{j} \prec_H^{\tr} T_{i}))\rangle$. In the serial history all the methods within a transaction are also ordered, it is also sequential.
 %\noindent
 %\textbf{Valid and Legal History:} If all the \emph{rv} methods of $H$ returns the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}. Whereas, If all the \emph{rv} methods of $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.
 
 
 %has been considered corresponding to each aborted transactions while keeping all the committed transaction including the aborted transaction till its successful method.
 
 \noindent
 \textbf{Valid and Legal History:}  If \emph{$rv\_method()$}  on key $k$ returns the value from any of the previously committed transactions then such \emph{$rv\_method()$} is known as \emph{valid method}. If all the \emph{$rv\_methods()$} of history $H$ return the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}.
 
 Whereas, If \emph{$rv\_method()$}  on key $k$ returns the value from previous closest committed transaction then such \emph{$rv\_method()$} is known as \emph{legal method}. If all the \emph{$rv\_methods()$} of history $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.
 
 \cmnt{
 	%\section{Valid and Legal Histories}
 	%\label{apn:legal}
 	%\vspace{-2mm}
 	%In this section, we start with defining legal histories. 
 	To simplify our analysis, we assume that there exists an initial transaction $T_0$ that invokes $\tdel$ \mth on all the keys of the \tab{} used by any transaction. 
 	
 	A \rvmt{} (\tdel{} and \tlook{}) $m_{ij}$ on key $k$ is valid if it returns the value updated by any of the previous committed transaction that updated key $k$. A history $H$ is said to valid if all the \rvmt{s} of H are valid. 
 	
 	We define \emph{\legality{}} of \rvmt{s} on sequential histories which we use to define correctness criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}. Consider a sequential history $H$ having a \rvmt{} $\rvm_{ij}(ht, k, v)$ (with $v \neq null$) as $j^{th}$ method belonging to transaction $T_i$. We define this \rvm \mth{} to be \emph{\legal} if: 
 	\vspace{-1mm}
 	\begin{enumerate}
 		%\setlength\itemsep{-1em}
 		%\vspace{-.2cm}
 		\item[LR1] \label{step:leg-same} If the $\rvm_{ij}$ is not first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $m_{ix}$ is the previous \mth of $T_i$ on $\langle ht, k \rangle$. Formally, $\rvm_{ij} \neq \fkmth{\langle ht, k \rangle}{T_i}{H}$ $\land (m_{ix}\\(ht, k, v') = \pkmth{\langle ht, k \rangle}{T_i}{H})$ (where $v'$ could be null). Then,
 		\begin{enumerate}
 			\setlength\itemsep{0em}
 			%		\item if $m_{ix}(ht, k, v')$ is a \tins{} \mth i.e. $\tins_{ix}(ht, k, v')$ then $v = v'$. 
 			%		\item if $m_{ix}(ht, k, v')$ is a \tlook{} \mth i.e. $\tlook_{ix}(ht, k, v')$ then $v = v'$. 
 			%		\item if $m_{ix}(ht, k, v')$ is a \tdel{} \mth i.e. $\tdel_{ix}(ht, k, v'/NULL)$ then $v = NULL$. 
 			\item If $m_{ix}(ht, k, v')$ is a \tins{} \mth then $v = v'$. 
 			\item If $m_{ix}(ht, k, v')$ is a \tlook{} \mth then $v = v'$. 
 			\item If $m_{ix}(ht, k, v')$ is a \tdel{} \mth then $v = null$.
 		\end{enumerate}
 		
 		In this case, we denote $m_{ix}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $m_{ix}(ht, k, v') = \\\lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 		
 		\item[LR2] \label{step:leg-ins} If $\rvm_{ij}$ is the first \mth{} of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is not null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v \neq null)$. Then,
 		\begin{enumerate}
 			\setlength\itemsep{0em}
 			\item There is a \tins{} \mth{} $\tins_{pq}(ht, k, v)$ in $\met{H}$ such that $T_p$ committed before $\rvm_{ij}$. Formally, $\langle \exists \tins_{pq}(ht, k, v) \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. 
 			\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 		\end{enumerate}
 		
 		In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $\tryc_{p}(ht, k, v)$= $\lupdt{\rvm_{ij}(ht, k, v)}{H}$.
 		
 		\item[LR3] \label{step:leg-del} If $\rvm_{ij}$ is the first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v = null)$. Then,
 		\begin{enumerate}
 			\setlength\itemsep{0em}
 			\item There is \tdel{} \mth{} $\tdel_{pq}(ht, k, v')$ in $\met{H}$ such that $T_p$ (which could be $T_0$ as well) committed before $\rvm_{ij}$. Formally, $\langle \exists \tdel_{pq}\\(ht, k,$ $ v') \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. Here $v'$ could be null. 
 			\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 		\end{enumerate}
 		In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e., $\tryc_{p}(ht, k, v)$ $= \lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 	\end{enumerate}
 	%\vspace{-.3cm}
 	We assume that when a transaction $T_i$ operates on key $k$ of a \tab{} $ht$, the result of this \mth is stored in \emph{local logs} of $T_i$, $\llog_i$ for later \mth{s} to reuse. Thus, only the first \rvmt{} operating on $\langle ht, k \rangle$ of $T_i$ accesses the shared-memory. The other \rvmt{s} of $T_i$ operating on $\langle ht, k \rangle$ do not access the shared-memory and they see the effect of the previous \mth{} from the \emph{local logs}, $\llog_i$. This idea is utilized in LR1. With reference to LR2 and LR3, it is possible that $T_x$ could have aborted before $\rvm_{ij}$. For LR3, since we are assuming that transaction $T_0$ has invoked a \tdel{} \mth{} on all the keys used of the \tab{} objects, there exists at least one \tdel{} \mth{} for every \rvmt on $k$ of $ht$. We formally prove legality in \apnref{cmvostm} and then we finally show that history generated by \hmvotm{} is \opq{} \cite{GuerKap:Opacity:PPoPP:2008}.
 	
 	%This we also call \emph{conflict inheritance} as the conflict of the later \mth{} of $T_i$ operating on $\langle ht, k \rangle$ can be found using the conflicts of the first \mth{} of $T_i$.
 	
 	Coming to \tins{} \mth{s}, since a \tins{} \mth{} always returns $ok$ as they overwrite the node if already present therefore they always take effect on the $ht$. Thus, we denote all \tins{} \mth{s} as \legal{} and only give legality definition for \rvmt{}. We denote a sequential history $H$ as \emph{\legal} or \emph{linearized} if all its \rvm \mth{s} are \legal.%A sequential history \emph{linearized} \cite{HerlWing:1990:TPLS}
 	
 }
 
 
 
 \noindent
 \textbf{Sub-history:} Following \cite{Chaudhary+:KSFTM:Corr:2017}, A \textit{sub-history} ($SH$) of a history ($H$) is a collection of events represented as $\evts{SH}$. We denote a $SH$ as the tuple $\langle \evts{SH},$ $<_{SH}\rangle$, here $<_{SH}$ represents the
 total order of among all the events of $SH$. Formally, $SH$ is defined as: (1) $<_{SH} \subseteq <_{H}$; (2) $\evts{SH} \subseteq \evts{H}$; (3) If an event of a transaction $T_k\in\txns{H}$ is in $SH$ then all the events of $T_k$ in $H$ should also be in $SH$. 
 
 Let $P$ is a subset of $H$ which consists of a set transactions $\txns{H}$. Then the sub-history of $H$ is represented as $\shist{P}{H}$ which comprises of $\evts{}$ of $P$. 
 
 \noindent
 \textbf{Conflict-opacity (or Co-opacity):} It is a well known correctness criteria of STMs that is polynomial time verifiable. Co-opacity \cite{Peri+:OSTM:Netys:2018} is a subclass of opacity. A history $H$ is co-opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time as $H$ $\prec_S^{\tr} \subseteq \prec_H^{\tr}$. (4) $S$ preserves conflict-order of $H$, i.e. $\prec_S^{Conf} \subseteq \prec_H^{Conf}$.
 
 \noindent
 \textbf{Opacity and Strict Serializability:} A popular correctness criteria for STMs is opacity \cite{GuerKap:Opacity:PPoPP:2008}. A valid history $H$ is opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time order as $H$, i.e. $\prec_S^{\tr} \subseteq \prec_H^{\tr}$.
 
 A valid history $H$ is strict serializable \cite{Papad:1979:JACM}, if sub-history  of $H$ as $\subhist(H)$ (consists of all the committed transactions of $H$) is opaque, i.e., $H.subhist(H.committed)$ is \emph{opaque}. So, if a history is \emph{strict serializable} then it will be \opq as well but  the vice-versa is not true. Unlike opacity, \emph{strict serializability} does not consider aborted transactions.
 
 A commonly used correctness criteria in databases is \emph{serializability} \cite{Papad:1979:JACM} which considers committed transactions only. Guerraoui \& Kapalka \cite{GuerKap:Opacity:PPoPP:2008} show that STMs considers the correctness of \emph{aborted} transactions along with \emph{committed} transactions as well. So,  \emph{serializability} is not suitable for STMs. On the other hand, \emph{opacity} \cite{GuerKap:Opacity:PPoPP:2008} is a popular correctness criteria for STMs which considers \emph{aborted} as well as \emph{committed} transactions. Similar to \emph{opacity} but less restrictive, an another popular correctness criteria is \emph{local opacity} defined below.
 
 
 
 \noindent
 \textbf{Local Opacity (or LO):} It is an another popular correctness criteria for STMs which is less restrictive than opacity. Local-opacity \cite{KuznetsovPeri:Non-interference:TCS:2017} is a superclass of opacity. It considers a set of sub-histories for history $H$, denoted as $\shset{H}$ as follows: (1) We construct a $\subhist$ corresponding to each aborted transaction $T_i$ while including all the events $\evts{}$ of previously \emph{committed} transactions along with all successful $\evts{}$ of $T_i$ (i.e., $\evts{}$ which has not returned $\mathcal{A}$ yet) and put \emph{committed} $\mathcal{C}$ immediately after last successful operation of $T_i$; (2) We construct one more sub-history corresponding to last \emph{committed} transaction $T_l$ which considers all the previously \emph{committed} transactions only including  $T_l$.
 
 If all the above defined sub-histories $\shset{H}$ for a history $H$ are opaque then $H$ is said to be \emph{\lopq} \cite{KuznetsovPeri:Non-interference:TCS:2017}. We can observe that a sub-history corresponding to an aborted transaction $T_i$ contains $\evts{}$ from only one aborted transaction which is $T_i$ itself and does not consider any other live/aborted transactions. Similarly, sub-history corresponding to last \emph{committed} transaction $T_l$ does not consider any $\evts{}$ of aborted and live transactions. Thus in \lopty, neither aborted nor live transaction cause any other transaction to abort. Researchers have been proved that \lopty 
 \cite{KuznetsovPeri:Non-interference:TCS:2017} ensures greater concurrency than \opty \cite{GuerKap:Opacity:PPoPP:2008}. If a history is \opq then it will be \lopq as well but  the vice-versa is not true. On the other hand, if a history is \lopq then it will be \stsble as well, but the vice-versa need not be true. Please find  illustrations of local opacity in \secref{gcoflo}. 
%Due to lack of space, we define other useful notions and definitions used in this paper such assequential histories \cite{KuznetsovPeri:Non-interference:TCS:2017}, real-time order and serial history \cite{Papad:1979:JACM}, valid and legal history \cite{Juyal+:SSS:2018}, sub-histories \cite{Chaudhary+:KSFTM:Corr:2017}, conflict-opacity \cite{Peri+:OSTM:Netys:2018}, opacity \cite{GuerKap:Opacity:PPoPP:2008}, strict-serializability \cite{Papad:1979:JACM}, local opacity \cite{KuznetsovPeri:Non-interference:TCS:2017} formally in \apnref{ap-model} and accompanying technical report \cite{Juyal+:CORR:SF-MVOSTM:2019}.
%\todo{
%An alternate way to achieve SF-SVOSTM while maintaining the number of version $K$ is 1 in SF-KOSTM. So, In the entire paper, we will discuss about  SF-KOSTM. }




 
 
 
 
 
 
 
 

==> Arxiv SFKOSTM SSS19/working.tex <==
%\\\clearpage
\vspace{-.4cm}
\subsection{Working of SF-KOSTM Algorithm}
\label{subsec:working}
In this subsection, we describe the working of SF-KOSTM algorithm which includes the detail description of SF-KOSTM methods and challenges to make it starvation-free. This description can easily be extended to SF-MVOSTM and SF-MVOSTM-GC as well. 

SF-KOSTM invokes \tbeg{()}, \tlook{()}, \tdel{()}, \tins{()}, and \tryc{()} methods. \tlook{()} and \tdel{()} work as \rvmt{s()} which lookup the value of key $k$ from shared memory and return it. Whereas \tins{()} and \tdel{()} work as \upmt{s()} that modify the value of $k$ in shared memory. We propose optimistic SF-KOSTM, so, \upmt{s()} first update the value of $k$ in transaction local log $txLog$ and the actual effect of \upmt{s()} will be visible after successful \tryc{()}. Now, we explain the functionality of each method as follows:

\noindent
\textbf{\tbeg{():}} %STM transactions are called by the thread $Th_i$. 
When a thread $Th_i$ invokes transaction $T_i$ for the first time (or first incarnation), \tbeg{()} assigns a unique timestamp known as \emph{current timestamp} $(cts)$ using atomic global counter ($gcounter$). If $T_i$ gets aborted then thread $Th_i$ executes it again with new incarnation of $T_i$, say $T_j$ with the new $cts$ until $T_i$ commits but retains its initial $cts$ as \emph{initial timestamp} $(its)$. $Th_i$ uses $its$ to inform the SF-KOSTM system that whether $T_i$ is a new invocation or an incarnation. %So, $Th_i$ maintains $\langle \emph{its, cts}\rangle$ for transaction $T_i$.
 If $T_i$ is the first incarnation then $its$ and $cts$ are same as $cts_i$ so, $Th_i$ maintains $\langle \emph{$its_i$, $cts_i$}\rangle$. If $T_i$ gets aborted and retries with $T_j$ then $Th_i$ maintains $\langle \emph{$its_i$, $cts_j$}\rangle$.
% Initially, thread $Th_i$ calls \tbeg{()} which maintains $\langle \emph{its, cts}\rangle$ for transaction $T_i$. If $T_i$ is the first incarnation then its \emph{Initial Timestamp (its)} and \emph{Current Timestamp (cts)} are same as $i$. We represent the $\langle its, cts\rangle$ as $\langle its_i, cts_i\rangle$ for transaction $T_i$. If $T_i$ is aborted then thread $Th_i$ executes it again with new incarnation of $T_i$ until $T_i$ commits. Let the new incarnation of $T_i$ say $T_j$ then thread $Th_i$ maintain its $\langle its, cts \rangle$ as $\langle its_i, cts_j \rangle$. $Th_i$ stores the first incarnation $its_i$ of $T_i$ to set the reincarnation $its_j$ of $T_j$ is same as $its_i$. $cts$ is incremented atomically with the help of atomic global counter. %SF-KOSTM is unable to achieve the starvation-freedom with the help of $cts$ as shown in \tabref{sfillus1}.  


%\vspace{-.1cm}

%\vspace{.05mm}

By assigning priority to the lowest $its$ transaction (i.e. transaction have been in the system for longer time) in \emph{Single-Version OSTM}, \emph{Starvation-Freedom} can easily achieved as explained in \secref{intro}. The detailed working of \emph{Starvation-Free Single-Version OSTM (SF-SVOSTM)} is in \apnref{ap-sfostm}. But achieving \emph{Starvation-Freedom} in finite \emph{K-versions OSTM (SF-KOSTM)} is challenging. Though the transaction $T_i$ has lowest $its$ but $T_i$ may return abort because of finite versions $T_i$ did not find a correct version to lookup from or overwrite a version. \tabref{sfillus1} shows the key insight to achieve the \stfdm in finite K-versions OSTM. Here, we considered two transaction $T_{10}$ and $T_{20}$ with $cts$ 10 and 20 that performs \emph{STM\_lookup()} $($or $l)$ and \emph{STM\_insert()} $($or $i)$ on same key $k$. We assume that a version of $k$ exists with $cts$ 5, so, \emph{STM\_lookup()} of $T_{10}$ and $T_{20}$ find a previous version to lookup and never return abort. Due to the optimistic execution in SF-KOSTM, effect of \emph{STM\_insert()} comes after successful \emph{STM\_tryC()}, so \emph{STM\_lookup()} of a transaction comes before effect of its \emph{STM\_insert()}. Hence, total six permutations are possible as defined in \tabref{sfillus1}. We can observe from the \tabref{sfillus1} that in some cases $T_{10}$ returns abort. But if $T_{20}$ gets the lowest $its$ then $T_{20}$ never returns abort. This ensures that a transaction with lowest $its$ and highest $cts$ will never return abort. But achieving highest $cts$ along with lowest $its$ is bit difficult because new transactions are keep on coming with higher $cts$ using $gcounter$. So, to achieve the highest $cts$, we introduce a new timestamp as \emph{working timestamp (wts)} which is significantly larger than $cts$. 

\begin{table}[H]
	\small
	\begin{tabular}{ | m{1cm} | m{4cm}| m{7cm} | } 
		\hline
		S. No.& Execution Sequence & Possible actions by Transactions  \\ 
		\hline
		1. & $l_{10}(k), i_{10}(k), l_{20}(k), i_{20}(k)$ & $T_{20}(k)$ lookups the version inserted by $T_{10}$. No conflict. \\
		\hline
		2. & $l_{10}(k), l_{20}(k), i_{10}(k), i_{20}(k)$ & Conflict detected at $i_{10}(k)$. Either abort $T_{10}$ or $T_{20}$. \\
		\hline
		3. & $l_{10}(k), l_{20}(k), i_{20}(k), i_{10}(k)$ & Conflict detected at $i_{10}(k)$. Hence, abort $T_{10}$. \\
		\hline
		4. & $l_{20}(k), l_{10}(k), i_{20}(k), i_{10}(k)$ & Conflict detected at $i_{10}(k)$. Hence, abort $T_{10}$. \\
		\hline
		5. & $l_{20}(k), l_{10}(k), i_{10}(k), i_{20}(k)$ & Conflict detected at $i_{10}(k)$. Either abort $T_{10}$ or $T_{20}$. \\
		\hline
		6. & $l_{20}(k), i_{20}(k), l_{10}(k), i_{10}(k)$ & Conflict detected at $i_{10}(k)$. Hence, abort $T_{10}$.\\
		\hline
	\end{tabular}
	\captionsetup{justification=centering}
	\caption{Possible Permutations of Methods}
	\label{tab:sfillus1}
\end{table}

\vspace{-.4cm}
\noindent
\tbeg{()} maintains the $wts$ for transaction $T_i$ as $wts_i$, which is potentially higher timestamp as compare to $cts_i$. So, we derived,
\setlength\abovedisplayskip{0pt}
\begin{equation}
\label{eq:wtsf}
\twts{i} = \tcts{i} + C * (\tcts{i} - \tits{i});
\vspace{-.2cm}
\end{equation}
%$wts_i$ = $cts_i$ + C*($cts_i$-$its_i$)
where C is any constant value greater than 0. When $T_i$ is issued for the first time then $wts_i$, $cts_i$, and $its_i$ are same. If $T_i$ gets aborted again and again then drift between the $cts_i$ and $wts_i$ will increases. The advantage for maintaining $wts_i$ is if any transaction keeps getting aborted then its $wts_i$ will be high and $its_i$ will be low. Eventually, $T_i$ will get chance to commit in finite number of steps to achieve starvation-freedom. For simplicity, we use timestamp (\emph{ts}) $i$ of $T_i$ as $wts_i$, i.e., $\langle wts_i$ = $i\rangle$ for SF-KOSTM. 
\vspace{-.2cm}
\begin{observation}
Any transaction $T_i$ with lowest $its_i$ and highest $wts_i$ will never abort.
\end{observation}
%\vspace{.2mm}
\vspace{-.1cm}
Sometimes, the value of $wts$ is significantly larger than $cts$. So, $wts$ is unable to maintain \emph{real-time order} between the transactions which violates the correctness of SF-KOSTM (shown in \figref{sfmv-correct} in \apnref{wtsdis}). To address this issue SF-KOSTM uses the idea of timestamp ranges \cite{Riegel+:LSA:DISC:2006,Guer+:disc1:2008, Crain+:RI_VWC:ICA3PP:2011} along with $\langle its_i, cts_i, wts_i \rangle$ for transaction $T_i$ in \tbeg{()}. It maintains the \emph{transaction lower timestamp limit ($tltl_i$)} and \emph{transaction upper timestamp limit ($tutl_i$)} for $T_i$. Initially, $\langle its_i, cts_i, wts_i, tltl_i \rangle$ are the same for $T_i$. $tutl_i$ would be set as a largest possible value denoted as $+\infty$ for $T_i$. After successful execution of \emph{\rvmt{s()}} or \tryc{()} of $T_i$, $tltl_i$ gets incremented and $tutl_i$ gets decremented\footnote{Practically $\infty$ can't be decremented for $tutl_i$ so we assign the highest possible value to $tutl_i$ which gets decremented.} to respect the real-time order among the transactions. \tbeg{()} initializes the \emph{transaction local log $(txLog_i)$} for each transaction $T_i$ to store the information in it. Whenever a transaction starts it atomically sets its \emph{status} to be \emph{live} as a global variable. Transaction \emph{status} can be $\langle \emph{live, commit, false}\rangle$. After successful execution of \tryc{()}, $T_i$ sets its \emph{status} to be \emph{commit}. If \emph{status} of the transaction is \emph{false} then it returns \emph{abort}. For more details please refer the high level view of \tbeg{()} in \algoref{begin1}.% in \apnref{ap-kostm}.  

\begin{algorithm}[H] 
	%	\scriptsize
	\caption{\emph{STM\_begin($its$)}: This method is invoke by a thread $Th_i$ to start a new transaction $T_i$. It pass a parameter $its$ which is the initial timestamp of the first incarnation of $T_i$. If $T_i$ is the first incarnation then $its$ is $nil$.}
	\label{algo:begin1} 
	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{0}\makeatother
		\Procedure{\emph{STM\_begin($its$)}}{}  \label{lin:begin1}
		\State Create a local log $txLog_i$ for each transaction. \label{lin:begin2}
		\If {($its == nil$)} \label{lin:begin3}
		\State /* Atomically get the value from the global counter and set it to its, cts, and \blank{1cm} wts.*/ \label{lin:begin4}
		\State $its_i$ = $cts_i$ = $wts_i$ = \emph{gcounter.get\&Inc()}; \label{lin:begin5}
		\Else  \label{lin:begin6}
		\State /*Set the $its_i$ to first incarnation of $T_i$ $its$*/ \label{lin:begin7}
		\State $its_i$ = $its$; \label{lin:begin8}
		\State /*Atomically get the value from the global counter for $cts_i$*/ \label{lin:begin9}
		\State $cts_i$ = \emph{gcounter.get\&Inc()}. \label{lin:begin10}
		%		\State \txll.$L\_t\_id$ $\gets$ $\gcts_i \gets \gtcnt.get\&Inc()$; 
		\State /*Set the $wts$ value with the help of $cts_i$ and $its_i$*/ \label{lin:begin11}
		\State $wts_i$ = $cts_i$+C*($cts_i$-$its_i$). \label{lin:begin12}
		\EndIf \label{lin:begin13}
		\State /*Set the $tltl_i$ as $cts_i$*/ \label{lin:begin14}
		\State $tltl$ = $cts_i$.   \label{lin:begin15}
		\State /*Set the $tutl_i$ as possible large value*/ \label{lin:begin16}
		\State $tutl_i$ = $\infty$. \label{lin:begin17}
		\State /*Initially, set the $status_i$ of $T_i$ as $live$*/ \label{lin:begin18}
		\State $status_i$ = $live$;  \label{lin:begin19}
		\State return $\langle cts_i, wts_i\rangle$ \label{lin:begin20}
		
		\EndProcedure
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}


%Initially, each threads $Th_x$ call this method and gets the unique time stamp (\emph{ts}) $i$ for each transaction $T_i$. If $Th_x$ calls $T_i$ for first time then its \emph{Current Timestamp (cts)} would be $i$. If $T_i$ gets aborted and executed again by the $Th_x$ as a reincarnation of $T_i$ to $T_j$ then its cts would be $j$. cts is incremented atomically with the help of global counter. If $T_i$ is not the first incarnation then $Th_x$ pass its first incarnation cts to STM system to notify that this is not the first incarnation. STM system maintains the first incarnation of $T_i$ as \emph{Initial Timestamp (its)} for all its incarnation such as $T_j$. Each incarnation of $T_i$ as $T_j$ maintains two timestamp such as $\langle its, cts\rangle$. For the first incarnation of $T_i$ $\langle its, cts \rangle$ are same.


%\tryc{()} maintains the $wts_j$ of current version $ver_j$ of each key $k$ in currVL. It maintains the 

\noindent
\textbf{\tlook{()} and \tdel{()} as \rvmt{s()}:} \emph{\rvmt{s(ht, k, val)}} return the value (\emph{val}) corresponding to the key \emph{k} from the shared memory as hash table (\emph{ht}). We show the high level overview of the \rvmt{s()} in \algoref{rvmt}. First, it identifies the key $k$ in the transaction local log as \emph{$txLog_i$} for transaction $T_i$. If $k$ exists then it updates the $txLog_i$ and returns the $val$ at \Lineref{rvm2}.


If key $k$ does not exist in the $txLog_i$ then before identify the location in share memory \rvmt{s()} check the \emph{status} of $T_i$ at \Lineref{rvm5}. If \emph{status} of $T_i$ (or $i$) is \emph{false} then $T_i$ has to \emph{abort} which says that $T_i$ is not having the lowest $its$ and highest $wts$ among other concurrent conflicting transactions. So, to propose starvation-freedom in SF-KOSTM other conflicting transactions set the \emph{status} of $T_i$ as \emph{false} and force it to \emph{abort}.

%\vspace{-.2cm}
If \emph{status} of $T_i$ is not \emph{false} and key $k$ does not exist in the $txLog_i$ then it identifies the location of key $k$ optimistically (without acquiring the locks similar to the \emph{lazy-list}\cite{Heller+:LazyList:PPL:2007}) in the shared memory at \Lineref{rvm7}. SF-KOSTM maintains the shared memory in the form of hash table with $M$ buckets as shown in \subsecref{dsde}, where each bucket stores the keys in \emph{\lsl}. Each node contains two pointer $\langle \rn, \bn \rangle$. So, it identifies the two \emph{predecessors (pred)} and two \emph{current (curr)} with respect to each node. First, it identifies the pred and curr for key $k$ in \bn{} as $\langle \bp, \bc \rangle$. After that it identifies the pred and curr for key $k$ in \rn{} as $\langle \rp, \rc \rangle$. If $\langle \rp, \rc \rangle$ are not marked then $\langle \bp=\rp, \bc=\rc\rangle$. SF-KOSTM maintains the keys are in increasing order. So, the order among the nodes are $\langle \bp.key \leq \rp.key < k \leq \rc.key \leq \bc.key\rangle$.



\rvmt{s()} acquire the lock in predefined order on all the identified preds and currs for key $k$ to avoid the deadlock at \Lineref{rvm8} and do the \emph{rv\_Validation()} as shown in \algoref{rvm}. If $\langle \bp \vee \bc\rangle$ is marked or preds are not pointing to identified currs as $\langle (\bp.\bn \neq \bc) \vee (\rp.\rn \neq \rc)\rangle$ then it releases the locks from all the preds and currs and identify the new preds and currs for $k$ in shared memory. 

\begin{algorithm}[H]
	
	%	\scriptsize
	\caption{\emph{rv\_Validation(preds[], currs[])}: It is mainly used for \emph{rv\_method()} validation.}
	\label{algo:rvm} 
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{21}\makeatother
		\Procedure{$rv\_Validation{(preds[], currs[])}$}{} \label{lin:rvv1}
		\If{$((\bp.mark) || (\bc.mark) || ((\bp.\bn)\neq \blank{1.7cm} \bc) || ((\rp.\rn) \neq {\rc})$)}\label{lin:rvv2}
		return $\langle false \rangle$. 
		\Else{} return $\langle true \rangle$. \label{lin:rvv3}
		\EndIf \label{lin:rvv4}
		\EndProcedure \label{lin:rvv5}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}

\vspace{.4mm}
\setlength{\intextsep}{0pt}
\begin{algorithm}
%	\scriptsize
	\caption{\emph{\rvmt{s(ht, k, val)}:} It can either be $\tdel_i(ht, k, val)$ or $\tlook_i(ht, k, val)$ on key $k$ by transaction $T_i$.} \label{algo:rvmt} 	
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{26}\makeatother
			\Procedure{$\rvmt{s}_i$}{$ht, k, val$}	\label{lin:rvm1}	
			\If{($k \in \llog_i$)} 
			\State Update the local log of $T_i$ and return $val$. \label{lin:rvm2}
			\Else \label{lin:rvm3}
			\State /*Atomically check the \emph{status} of its own transaction $T_i$ (or $i$).*/ \label{lin:rvm4} %after acquiring \emph{atomic lock} on it*/
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:rvm5}
			\EndIf\label{lin:rvm6}
			\State Identify the \emph{preds[]} and \emph{currs[]} for key $k$ in bucket $M_k$ of \emph{\lsl} using \blank{1cm} \bn and \rn . \label{lin:rvm7}
			\State Acquire locks on \emph{preds[]} \& \emph{currs[]} in increasing order of keys to avoid the \blank{1cm} deadlock. \label{lin:rvm8}
			\If{(\emph{!rv\_Validation(preds[], currs[])})} \label{lin:rvm9}
			\State Release the locks and goto \linref{rvm7}. \label{lin:rvm10}
			\EndIf \label{lin:rvm11}
			\If{($k  ~ \notin ~ M_k.\lsl$)} \label{lin:rvm12} 
			\State Create a new node $n$ with key $k$ as: $\langle$\emph{key=k, lock=false, mark=true, \blank{1.5cm} vl=ver, nNext=}$\phi\rangle$./*$n$ is marked*/  \label{lin:rvm13}
			%\State \Comment{The $vl$ consists of a single element $v$ with $ts$ as $i$}
			\State Create version $ver$ as:$\langle$\emph{ts=0, val=nil, rvl=i, vrt=0, vNext=$\phi$}$\rangle$. \label{lin:rvm14}
			\State Insert $n$ into $M_k.$\emph{\lsl} s.t. it is accessible only via \rn{s}. /*\emph{lock} sets \blank{1.5cm} \emph{true}*/  \label{lin:rvm15}  	
			\State Release locks; update the $\llog_i$ with $k$.\label{lin:rvm16}
			\State return $\langle$\emph{val}$\rangle$. /*\emph{val} as $nil$*/\label{lin:rvm17}
			\EndIf \label{lin:rvm18}
			\State Identify the version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp \blank{1cm} smaller (lts)} than $i$.\label{lin:rvm19}
			\If{($ver_j$ == $nil$)} /*Finite Versions*/\label{lin:rvm111}
			\State return $\langle abort_i\rangle$ 
			%		\EndIf
			\ElsIf{($ver_j.vNext$ != $nil$)}\label{lin:rvm20}
			\State /*$tutl_i$ should be less then \emph{vrt} of next version $ver_j$*/\label{lin:rvm21}
			\State 	Calculate $tutl_i$ = min($tutl_i$, $ver_j.vNext$ $.vrt-1$).\label{lin:rvm22}
			\EndIf\label{lin:rvm23}
			\State /*$tltl_i$ should be greater then $vrt$ of $ver_j$*/\label{lin:rvm24}
			\State 	Calculate $tltl_i$ = max($tltl_i$, $ver_j.vrt+1$).\label{lin:rvm25}
			\State /*If limit has crossed each other then abort $T_i$*/\label{lin:rvm26}
			\If{($tltl_i$ $>$ $tutl_i$)} return $\langle abort_i \rangle$. \label{lin:rvm27}
			\EndIf\label{lin:rvm28}
			%\State $ver_j = find\_lts(k)$.\label{lin:corr-ver} 
			\State Add $i$ into the $rvl$ of $ver_j$. \label{lin:rvm29} 
			%		\State $retVal = ver_j.val$.
			\State Release the locks; update the $\llog_i$ with $k$ and value. \label{lin:rvm30}
			\EndIf \label{lin:rvm31}
			\State return $\langle$$ver_j.val$$\rangle$. \label{lin:rvm32}
			\EndProcedure \label{lin:rvm33}
		\end{algorithmic}
%	\end{multicols}
\end{algorithm}
\vspace{.2mm}


\cmnt{
\vspace{.4mm}
\setlength{\intextsep}{0pt}
\begin{algorithm}
	\scriptsize
	\caption{\emph{\rvmt{s(ht, k, val)}:} It can either be $\tdel_i(ht, k, val)$ or $\tlook_i(ht, k, val)$ on key $k$ by transaction $T_i$.} \label{algo:rvmt} 	
	\setlength{\multicolsep}{0pt}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			%\makeatletter\setcounter{ALG@line}{0}\makeatother
			\Procedure{$\rvmt{s}_i$}{$ht, k, val$}	\label{lin:rvm1}	
			\If{($k \in \llog_i$)} 
			\State Update the local log of $T_i$ and return $val$. \label{lin:rvm2}
			\Else \label{lin:rvm3}
			\State /*Atomically check the \emph{status} of its own transac- \blank{.7cm}tion $T_i$ (or $i$).*/ \label{lin:rvm4} %after acquiring \emph{atomic lock} on it*/
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:rvm5}
			\EndIf\label{lin:rvm6}
			\State Identify the \emph{preds[]} and \emph{currs[]} for key $k$ in \blank{.7cm} bucket $M_k$ of \emph{\lsl} using \bn and \rn . \label{lin:rvm7}
			\State Acquire locks on \emph{preds[]} \& \emph{currs[]} in increasing \blank{.7cm} order of keys to avoid the deadlock. \label{lin:rvm8}
			\If{(\emph{!rv\_Validation(preds[], currs[])})} \label{lin:rvm9}
			\State Release the locks and goto \linref{rvm7}. \label{lin:rvm10}
			\EndIf \label{lin:rvm11}
			\If{($k  ~ \notin ~ M_k.\lsl$)} \label{lin:rvm12} 
			\State Create a new node $n$ with key $k$ as: \blank{.8cm} $\langle$\emph{key=k, lock=false, mark=true, vl=ver, \blank{1.1cm} nNext=}$\phi\rangle$./*$n$ is marked*/  \label{lin:rvm13}
			%\State \Comment{The $vl$ consists of a single element $v$ with $ts$ as $i$}
			\State Create version $ver$ as:$\langle$\emph{ts=0, val=nil, rvl=i, \blank{1.1cm} vrt=0, vNext=$\phi$}$\rangle$. \label{lin:rvm14}
			\State Insert $n$ into $M_k.$\emph{\lsl} s.t. it is accessi- \blank{1.1cm}ble only via \rn{s}. /*\emph{lock} sets \emph{true}*/  \label{lin:rvm15}  	
			\State Release locks; update the $\llog_i$ with $k$.\label{lin:rvm16}
			\State return $\langle$\emph{val}$\rangle$. /*\emph{val} as $nil$*/\label{lin:rvm17}
			\EndIf \label{lin:rvm18}
			\State Identify the version $ver_j$ with $ts=j$ such that \blank{.7cm} $j$ is the \emph{largest timestamp smaller (lts)} than $i$.\label{lin:rvm19}
			\If{($ver_j$ == $nil$)} /*Finite Versions*/\label{lin:rvm111}
			\State return $\langle abort_i\rangle$ 
			%		\EndIf
			\ElsIf{($ver_j.vNext$ != $nil$)}\label{lin:rvm20}
			\State /*$tutl_i$ should be less then \emph{vrt} of next ver- \blank{1.1cm}sion $ver_j$*/\label{lin:rvm21}
			\State 	Calculate $tutl_i$ = min($tutl_i$, $ver_j.vNext$ $\blank{1.1cm}.vrt-1$).\label{lin:rvm22}
			\EndIf\label{lin:rvm23}
			\State /*$tltl_i$ should be greater then $vrt$ of $ver_j$*/\label{lin:rvm24}
			\State 	Calculate $tltl_i$ = max($tltl_i$, $ver_j.vrt+1$).\label{lin:rvm25}
			\State /*If limit has crossed each other then abort $T_i$*/\label{lin:rvm26}
			\If{($tltl_i$ $>$ $tutl_i$)} return $\langle abort_i \rangle$. \label{lin:rvm27}
			\EndIf\label{lin:rvm28}
			%\State $ver_j = find\_lts(k)$.\label{lin:corr-ver} 
			\State Add $i$ into the $rvl$ of $ver_j$. \label{lin:rvm29} 
			%		\State $retVal = ver_j.val$.
			\State Release the locks; update the $\llog_i$ with $k$ \blank{.7cm} and value. \label{lin:rvm30}
			\EndIf \label{lin:rvm31}
			\State return $\langle$$ver_j.val$$\rangle$. \label{lin:rvm32}
			\EndProcedure \label{lin:rvm33}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}
\vspace{.2mm}
}

If key $k$ does not exist in the \emph{\lsl{}} of corresponding bucket $M_k$ at \Lineref{rvm12} then it creates a new node $n$ with key $k$ as $\langle \emph{key=k, lock=false, mark=true, vl=ver, nNext=}\phi \rangle$ at \Lineref{rvm13} and creates a version (\emph{ver}) for transaction $T_0$ as $\langle$\emph{ts=0, val=nil, rvl=i, vrt=0, vNext=}$\phi\rangle$ at \Lineref{rvm14}. Transaction $T_i$ creates the version of $T_0$, so, other concurrent conflicting transaction (say $T_p$) with lower timestamp than $T_i$, i.e., $\langle p < i\rangle$ can lookup from $T_0$ version. Thus, $T_i$ save $T_p$ to abort while creating a $T_0$ version and ensures greater concurrency. After that $T_i$ adds its \emph{$wts_i$} in the \emph{rvl} of $T_0$ and sets the \emph{vrt} 0 as timestamp of $T_0$ version. Finally, it insert the node $n$ into $M_k.\lsl$ such that it is accessible via \rn{} only at \Lineref{rvm15}. \rvmt{()} releases the locks and update the $txLog_i$ with key $k$ and value as $nil$ (\Lineref{rvm16}). Eventually, it returns the \emph{val} as $nil$ at \Lineref{rvm17}.      

\vspace{-.5mm}

If key $k$ exists in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts$ = $j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$ at \Lineref{rvm19} and there exists no other version with timestamp $p$ by $T_p$ on same key $k$ such that $\langle \emph{j $<$ p $<$ i}\rangle$. If $ver_j$ is $nil$ at \Lineref{rvm111} then SF-KOSTM returns $abort$ for transaction $T_i$ because it does not found version to lookup otherwise it identifies the next version with the help of $ver_j.vNext$. If next version ($ver_j.vNext$ as $ver_k$) exist then $T_i$ maintains the $tutl_i$ with minimum of $\langle tutl_i$ $\vee$ $ver_k.vrt-1\rangle$ at \Lineref{rvm22} and $tltl_i$ with maximum of $\langle tltl_i \vee $ $ver_j.vrt+1$$\rangle$ at \Lineref{rvm25} to respect the \emph{real-time order} among the transactions. If $tltl_i$ is greater than $tutl_i$ at \Lineref{rvm27} then transaction $T_i$ returns \emph{abort} (fail to maintains real-time order) otherwise it adds the $ts$ of $T_i$ ($wts_i$) in the $rvl$ of $ver_j$ at \Lineref{rvm29}. Finally, it releases the lock and update the $txLog_i$ with key $k$ and value as current version value ($ver_j.val$) at \Lineref{rvm30}. Eventually, it returns the value as $ver_j.val$ at \Lineref{rvm32}.  


\noindent
\textbf{\tins{()} and \tdel{()} as \upmt{s()}:} Actual effect of \tins{()} and \tdel{()} come after successful \tryc{()}. They create the version corresponding to the key in shared memory. We show the high level view of \tryc{()} in \algoref{tryc}. First, \tryc{()} checks the \emph{status} of the transaction $T_i$ at \Lineref{tc3}. If \emph{status} of $T_i$ is \emph{false} then $T_i$ returns \emph{abort} with similar reasoning explained above in \rvmt{()}. 



If \emph{status} is not false then \tryc{()} sort the keys (exist in $txLog_i$ of $T_i$) of \upmt{s()} in increasing order. % which belongs to  only. % such as \tins{()} and \tdel{()}. 
It takes the method ($m_{ij}$) from $txLog_i$ one by one and identifies the location of the key $k$ in \emph{$M_k$.\lsl} as explained above in \rvmt{()}. After identifying the preds and currs for $k$ it acquire the locks in predefined order to avoid the deadlock at \Lineref{tc10} and calls \emph{tryC\_Validation()} to validate the methods of $T_i$.


%\emph{tryC\_Validation()} identifies whether the methods of invoking transaction $T_i$ are able to insert or delete a version corresponding to the keys while ensuring the progress guarantee as \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions. It does four steps for validation. Step 1: First, it does the \emph{rv\_Validation()} as explained in \rvmt{()} above. Step 2: If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts$ = $j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because it does not found the version to replace. Step 3: If $ver_j$ \emph{exist} then $T_i$ compares $its_i$ with $its$ of other $live$ transactions present in $ver_j.rvl$. If $its_i$ of $T_i$ is less than the $its$ of such transactions then $T_i$ sets the $status$ of all those transactions to be $false$, otherwise, $T_i$ returns $abort$. Step 4: To maintain the \emph{real-time order}, $T_i$ update the $tltl_i$ and $tutl_i$ of it with the help of $ver_j$ and its next version ($ver_j.vNext$) respectively (explained in \rvmt{()} above). Please find the detailed descriptions of \emph{tryC\_Validation()} \algoref{trycVal} in \apnref{ap-kostm}.

\noindent
\textbf{\emph{tryC\_Validation()}:} It identifies whether the methods of invoking transaction $T_i$ are able to create or delete a version corresponding to the keys while ensuring the \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions.% First, it do the \emph{rv\_Validation()} as explained in \rvmt{()} above. If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise maintains the information of $ver_j$ and its next version ($ver_j.vNext$) which helps transaction $T_i$ to sets its $tltl_i$ and $tutl_i$. If $wts_i$ of $T_i$ is less then other $live$ transactions $wts$ exist in $ver_j.rvl$ then $T_i$ sets the $status$ to be $false$ to all other transactions otherwise $T_i$ returns to $abort$. The detailed descriptions are in \apnref{ap-rcode}.

%It maintains the Current Version List (currVL), Next Version List (nextVL), All Return Value List (allRVL), Large Return Value List (largeRVL), Small Return Value List (smallRVL) from $ver_j$ of key $k$. currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. These terms helps to decide, whether  $T_i$ will create the version and commit while aborting the conflicting transactions or $T_i$ returns abort. 





First, it do the \emph{rv\_Validation()} at \Lineref{tcv2} as explained in \rvmt{()}. If \emph{rv\_Validation()} is successful and key $k$ exists in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$ at \Lineref{tcv5}. If $ver_j$ is $null$ at \Lineref{tcv111} then SF-KOSTM returns $abort$ for transaction $T_i$ because it does not find the version to replace otherwise after identifying the current version $ver_j$ it maintains the Current Version List (currVL), Next Version List (nextVL), All Return Value List (allRVL), Large Return Value List (largeRVL), Small Return Value List (smallRVL) from $ver_j$ of key $k$ at \Lineref{tcv6}. currVL and nextVL maintain the previous closest version and next immediate version of all the keys accessed in \tryc{()}. allRVL keeps the currVL.rvl whereas largeRVL and smallRVL stores all the $wts$ of currVL.rvl such that ($wts_{currVL.rvl}$ $>$ $wts_i$) and  ($wts_{currVL.rvl}$ $<$ $wts_i$) respectively. Acquire the locks on \emph{status} of all the transactions present in allRVL list including $T_i$ it self in predefined order to avoid the deadlock at \Lineref{tcv8}. First, it checks the \emph{status} of its own transaction $T_i$ at \Lineref{tcv10}. If \emph{status} of $T_i$ is \emph{false} then $T_i$ has to \emph{abort} the same reason as explained in \rvmt{()}. 

If the \emph{status} of $T_i$ is not \emph{false} then it compares the $its_i$ of its own transaction $T_i$ with the $its_p$ of other transactions $T_p$ present in the largeRVL at \Lineref{tcv13}. Along with this it checks the \emph{status} of $p$. If above conditions $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ succeed then it includes $T_p$ in the Abort Return Value List (abortRVL) at \Lineref{tcv14} to abort it later otherwise abort $T_i$ itself at \Lineref{tcv15}.  

\vspace{.2mm}
\begin{algorithm}
	%\label{alg:llsearch} 
	%	\scriptsize
	\caption{\emph{tryC\_Validation():} It is use for \tryc{()} validation.}
	\label{algo:trycVal} 
	%	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{62}\makeatother
		\Procedure{\emph{tryC\_Validation{()}}}{} \label{lin:tcv1}
		\If{(\emph{!rv\_Validation()})}
		Release the locks and \emph{retry}.\label{lin:tcv2}
		\EndIf\label{lin:tcv3}
		\If{(k $\in$ $M_k.\lsl$)}\label{lin:tcv4}
		\State Identify the version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp \blank{1cm} smaller (lts)} than $i$ and there exists no other version with timestamp $p$ by $T_p$ \blank{1cm} on key $k$ such that $\langle \emph{j $<$ p $<$ i}\rangle$.\label{lin:tcv5}
		\If{($ver_j$ == $null$)} /*Finite Versions*/
		\State return $\langle abort_i\rangle$ \label{lin:tcv111}
		\EndIf
		\State Maintain the list of $ver_j$, $ver_j.vNext$, $ver_j.rvl$, $(ver_j.rvl>i)$, and \blank{1cm} $(ver_j.rvl<i)$ as prevVL, nextVL, allRVL, largeRVL and smallRVL \blank{1cm} respectively for all key \emph{k} of $T_i$.\label{lin:tcv6}
		\State /*$p$ is the timestamp of transaction $T_p$*/
		\If{($p$ $\in$ allRVL)} /*Includes $i$ as well in allRVL*/\label{lin:tcv7}
		\State Lock \emph{status} of each $p$ in pre-defined order. \label{lin:tcv8}
		\EndIf\label{lin:tcv9}
		\If{(\emph{i.status == false})} return $\langle false \rangle$. \label{lin:tcv10}
		\EndIf\label{lin:tcv11}
		\ForAll{($p$ $\in$ largeRVL)}\label{lin:tcv12}
		\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv13}
		\State Maintain \emph{abort list} as abortRVL \& includes \emph{p} in it.\label{lin:tcv14}
		\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv15}
		\EndIf\label{lin:tcv16}
		
		\EndFor\label{lin:tcv17}
		\ForAll{($ver$ $\in$ nextVL)}\label{lin:tcv21}
		\State Calculate $tutl_i$ = min($tutl_i$, $ver.vNext$$.vrt-1$).\label{lin:tcv22}
		\EndFor\label{lin:tcv23}
		\ForAll{($ver$ $\in$ currVL)}\label{lin:tcv18}
		\State Calculate $tltl_i$ = max($tltl_i$, $ver.vrt+1$).\label{lin:tcv19}
		\EndFor\label{lin:tcv20}
		\State /*Store current value of global counter as commit time and increment it.*/
		\State $comTime$ = \emph{gcounter.add\&get(incrVal)};  \label{lin:tcv201}
		\State Calculate $tutl_i$ = min($tutl_i$, $comTime$); \label{lin:tcv202}
		\If{($tltl_i$ $>$ $tutl_i$)} /*abort $i$ itself*/
		\State return $\langle false \rangle$. \label{lin:tcv24}
		\EndIf\label{lin:tcv25}
		\ForAll{($p$ $\in$ smallRVL)}\label{lin:tcv26}
		\If{($tltl_p$ $>$ $tutl_i$)}\label{lin:tcv27}%/*Ensure limit don't cross for both $i$ and $k$*/
		\If{(($its_i$$<$$its_p$)$\&\&$(\emph{p.status==live}))} \label{lin:tcv28}
		\State Includes $p$ in abortRVL list.\label{lin:tcv29}
		\Else{} return $\langle false \rangle$. /*abort $i$ itself*/\label{lin:tcv30}
		\EndIf\label{lin:tcv31}
		\EndIf	\label{lin:tcv32}	
		\EndFor \label{lin:tcv33}
		\State $tltl_i$ = $tutl_i$. /*After this point $i$ can't abort*/\label{lin:tcv34}
		\ForAll{($p$ $\in$ smallRVL)}
		\State /*Only for \emph{live} transactions*/ \label{lin:tcv35}
		\State Calculate the $tutl_p$ = min($tutl_p$, $tltl_i-1$).\label{lin:tcv36}
		\EndFor \label{lin:tcv37}
		\ForAll{($p$ $\in$ abortRVL)} \label{lin:tcv38}
		\State Set the \emph{status} of $p$ to be $false$. \label{lin:tcv39}
		\EndFor \label{lin:tcv40}
		%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
		%		\If{($j.max_{rvl}$ > $i$)}\label{lin:trycv7}
		%		\State return $false$.\label{lin:trycv8}
		%		\EndIf \label{lin:trycv9}
		%		\EndFor\label{lin:trycv10}
		\EndIf\label{lin:tcv41}
		\State return $\langle true \rangle$.\label{lin:tcv42}
		\EndProcedure \label{lin:tcv43}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
\vspace{.2mm}

After that \tryc{()} maintains the $tltl_i$ and $tutl_i$ of transaction $T_i$ at \Lineref{tcv19} and \Lineref{tcv22}. The requirement of $tltl_i$ and $tutl_i$ is explained above in the \rvmt{()}. If limit of $tltl_i$ crossed with $tutl_i$ then $T_i$ have to abort at \Lineref{tcv24}. If $tltl_p$ greater than $tutl_i$ at \Lineref{tcv27} then it checks the $its_i$ and $its_p$. If $\langle (its_i < its_p) \&\& (p.status==live))\rangle$ then add the transaction $T_p$ in the abortRVL for all the smallRVL transactions at \Lineref{tcv29} otherwise, \emph{abort} $T_i$ itself at \Lineref{tcv30}.

At \Lineref{tcv34}, $tltl_i$ would be equal to $tutl_i$ and after this step transaction $T_i$ will never \emph{abort}. $T_i$ helps the other transaction $T_p$ to update the $tutl_p$ which exists in the smallRVL and still $live$ then it sets the $tutl_p$ to minimum of $\langle tutl_p \vee tltl_i-1\rangle$ to maintain the real-time order among the transaction at \Lineref{tcv36}. At \Lineref{tcv39}, \tryc{()} aborts all other conflicting transactions which are present in the abortRVL while modifying the \emph{status} field to be \emph{false} to achieve \emph{starvation-freedom}. 


\cmnt{
\emph{tryC\_Validation()} identifies whether the methods of invoking transaction $T_i$ are able to insert or delete a version corresponding to the keys while ensuring the \emph{starvation-freedom} and maintaining the \emph{real-time order} among the transactions. It follow the following steps for validation. Step 1: First, it do the \emph{rv\_Validation()} as explained in \rvmt{()} above. Step 2: If \emph{rv\_Validation()} is successful and key $k$ is exist in the $M_k.\lsl$ then it identifies the current version $ver_j$ with $ts=j$ such that $j$ is the \emph{largest timestamp smaller (lts)} than $i$. If $ver_j$ is \emph{not exist} then SF-KOSTM returns $abort$ for transaction $T_i$ because of bounded K-versions otherwise maintains the information of $ver_j$ and its next version ($ver_j.vNext$) which helps transaction $T_i$ to sets its $tltl_i$ and $tutl_i$. Step 3: If $wts_i$ of $T_i$ is less then other $live$ transactions $wts$ exist in $ver_j.rvl$ then $T_i$ sets the $status$ to be $false$ to all conflicting \emph{live} transactions otherwise $T_i$ returns $abort$. The detailed descriptions are in \apnref{ap-rcode}.
}


If all the steps of the \emph{tryC\_Validation()} is successful then the actual effect of the \tins{()} and \tdel{()} will be visible to the shared memory. At \Lineref{tc16}, \tryc{()} checks for \emph{poValidation()}. When two subsequent methods $\langle m_{ij}, m_{ik}\rangle$ of the same transaction $T_i$ identify the overlapping location of preds and currs in \emph{\lsl}. Then \emph{poValidation()} updates the current method $m_{ik}$ preds and currs with the help of previous method $m_{ij}$ preds and currs. 

If $m_{ij}$ is \tins{()} and key $k$ is not exist in the $M_k.\lsl{}$ then it creates the new node $n$ with key $k$ as $\langle \emph{key=k, lock=false, mark=false, vl=ver, nNext=}\phi \rangle$ at \Lineref{tc18}. Later, it creates a version ($ver$) for transaction $T_0$ and $T_i$ as $\langle$ \emph{ts=0, val=nil, rvl=i, vrt=0, vNext=i} $\rangle$ and $\langle \emph{ts=i, val=v, rvl=}\phi, \emph{vrt=i, vNext=}\phi \rangle$ at \Lineref{tc19}. The $T_0$ version created by transaction $T_i$ to helps other concurrent conflicting transactions (with lower timestamp than $T_i$) to lookup from $T_0$ version. Finally, it insert the node $n$ into $M_k.\lsl$ such that it is accessible via \rn{} as well as \bn{} at \Lineref{tc20}. If $m_{ij}$ is \tins{()} and key $k$ is exist in the $M_k.\lsl{}$ then it creates the new version $ver_i$ as $\langle \emph{ts=i, val=v, rvl=}\phi, \emph{vrt=i, vNext=}\phi \rangle$ corresponding to key $k$. If the limit of the version reach to $K$ then SF-KOSTM replaces the oldest version with $(K+1)^{th}$ version which is accessible via \rn{} as well as \bn{} at \Lineref{tc22}. 
\cmnt{
\vspace{.6mm}
\begin{algorithm}
	
	\scriptsize
	\caption{\emph{\tryc($T_i$)}: Validate the \upmt{s()} of $T_i$ and returns \emph{commit}.}
	%	\setlength{\dbltextfloatsep}{0pt}
	\setlength{\multicolsep}{-1pt}
	\label{algo:tryc}
	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{36}\makeatother
			\Procedure{$\tryc{(T_i)}$}{} \label{lin:tc1}
			%\State Get the local log list for corresponding transaction;
			\State /*Atomically check the \emph{status} of its own transaction \blank{.3cm} $T_i$ (or $i$)*/ \label{lin:tc2}
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:tc3}
			\EndIf \label{lin:tc4}
			\State /*Sort the $keys$ of $\llog_i$ in increasing order.*/ \label{lin:tc5}
			\State /*Method ($m$) will be either \tins or \emph{STM\_ \blank{.3cm} delete}*/\label{lin:tc6}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)} \label{lin:tc7}
			\If{\hspace{-.07cm}($m_{ij}$==\tins$||$$m_{ij}$==\tdel)\hspace{-.07cm}}\label{lin:tc8}
			\State Identify the \emph{preds[]} \& \emph{currs[]} for key \emph{k} in \blank{1cm} bucket $M_k$ of \emph{\lsl} using \bn\& \rn. \label{lin:tc9}
			\State Acquire the locks on \emph{preds[]} \& \emph{currs[]} in \blank{1cm} increasing order of keys to avoid deadlock. \label{lin:tc10}
			\If{($!tryC\_Validation()$)}
			\State return $\langle abort_i \rangle$.\label{lin:tc11}
			\EndIf\label{lin:tc12}
			\EndIf\label{lin:tc13}
			\EndFor\label{lin:tc14}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)}\label{lin:tc15}
			\State \emph{poValidation()}  modifies the \emph{preds[]} \& \emph{currs[]} of \blank{.6cm} current method which would have been updated \blank{.6cm} by previous method of the same transaction.\label{lin:tc16}
			\If{(($m_{ij}$==\tins)\&\&(k$\notin$$M_k$.\lsl))}\label{lin:tc17}
			\State Create new node $n$ with $k$ as: $\langle$\emph{key=k, \blank{1.1cm} lock=false, mark= false, vl=ver, nNext=$\phi$}$\rangle$. \label{lin:tc18}
			\State Create first version $ver$ for $T_0$ and next for \blank{1.1cm} $i$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, vNext=$\phi$}$\rangle$.\label{lin:tc19}
			\State Insert node $n$ into $M_k$.\emph{\lsl} such that \blank{1.1cm} it is accessible via \rn{} as well as \bn{}.\label{lin:tc20}
			\State /*\emph{lock} sets \emph{true}*/  
			\ElsIf{($m_{ij}$ == \tins{})}\label{lin:tc21}
			\State Add $ver$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, \blank{1.1cm} vNext=$\phi$}$\rangle$ into $M_k$.\emph{\lsl} \& accessible \blank{1.1cm} via \rn{}, \bn. /*\emph{mark=false}*/\label{lin:tc22}
			\EndIf\label{lin:tc23}
			\If{($m_{ij}$ == \tdel{})}\label{lin:tc24}
			\State Add \emph{ver}:$\langle$\emph{ts=i, val=nil, rvl=$\phi$, vrt=i,   \blank{1cm} vNext=$\phi$}$\rangle$ into  $M_k$.\emph{\lsl} \& accessible \blank{1cm} via \rn only. /*\emph{mark=true}*/\label{lin:tc25}
			\EndIf\label{lin:tc26}
			\State Update \emph{preds[]} \& \emph{currs[]} of $m_{ij}$ in $\llog_i$.\label{lin:tc27}
			
			\EndFor \label{lin:tc28}
			%\EndFor
			\State Release the locks; return $\langle commit_i \rangle$.\label{lin:tc29}
			\EndProcedure \label{lin:tc30}
		\end{algorithmic}
	\end{multicols}
\end{algorithm}

\vspace{.2mm}
}

\vspace{.6mm}
\begin{algorithm}
	
%	\scriptsize
	\caption{\emph{\tryc($T_i$)}: Validate the \upmt{s()} of $T_i$ and returns \emph{commit}.}
	%	\setlength{\dbltextfloatsep}{0pt}
	\setlength{\multicolsep}{-1pt}
	\label{algo:tryc}
%	\begin{multicols}{2}
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{111}\makeatother
			\Procedure{$\tryc{(T_i)}$}{} \label{lin:tc1}
			%\State Get the local log list for corresponding transaction;
			\State /*Atomically check the \emph{status} of its own transaction  $T_i$ (or $i$)*/ \label{lin:tc2}
			\If{(\emph{i.status == false})} return $\langle abort_i \rangle$. \label{lin:tc3}
			\EndIf \label{lin:tc4}
			\State /*Sort the $keys$ of $\llog_i$ in increasing order.*/ \label{lin:tc5}
			\State /*Method ($m$) will be either \tins or \emph{STM\_delete}*/\label{lin:tc6}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)} \label{lin:tc7}
			\If{\hspace{-.07cm}($m_{ij}$==\tins$||$$m_{ij}$==\tdel)\hspace{-.07cm}}\label{lin:tc8}
			\State Identify the \emph{preds[]} \& \emph{currs[]} for key \emph{k} in bucket $M_k$ of \emph{\lsl} \blank{1.5cm} using
			\bn\& \rn. \label{lin:tc9}
			\State Acquire the locks on \emph{preds[]} \& \emph{currs[]} in increasing order of keys to \blank{1.5cm} avoid deadlock. \label{lin:tc10}
			\If{($!tryC\_Validation()$)}
			\State return $\langle abort_i \rangle$.\label{lin:tc11}
			\EndIf\label{lin:tc12}
			\EndIf\label{lin:tc13}
			\EndFor\label{lin:tc14}
			\ForAll{($m_{ij}$ $\in$ $\llog_i$)}\label{lin:tc15}
			\State \emph{poValidation()}  modifies the \emph{preds[]} \& \emph{currs[]} of current method which \blank{1cm} would have been updated by previous method of the same transaction.\label{lin:tc16}
			\If{(($m_{ij}$==\tins)\&\&(k$\notin$$M_k$.\lsl))}\label{lin:tc17}
			\State Create new node $n$ with $k$ as: $\langle$\emph{key=k, lock=false, mark= false, vl=ver, \blank{1.5cm} nNext=$\phi$}$\rangle$. \label{lin:tc18}
			\State Create first version $ver$ for $T_0$ and next for $i$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, \blank{1.5cm} vNext=$\phi$}$\rangle$.\label{lin:tc19}
			\State Insert node $n$ into $M_k$.\emph{\lsl} such that it is accessible via \rn{} as \blank{1.5cm} well as \bn{}.\label{lin:tc20}
			\State /*\emph{lock} sets \emph{true}*/  
			\ElsIf{($m_{ij}$ == \tins{})}\label{lin:tc21}
			\State Add $ver$: $\langle$\emph{ts=i, val=v, rvl=$\phi$, vrt=i, vNext=$\phi$}$\rangle$ into $M_k$.\emph{\lsl} \& \blank{1.5cm} accessible via \rn{}, \bn. /*\emph{mark=false}*/\label{lin:tc22}
			\EndIf\label{lin:tc23}
			\If{($m_{ij}$ == \tdel{})}\label{lin:tc24}
			\State Add \emph{ver}:$\langle$\emph{ts=i, val=nil, rvl=$\phi$, vrt=i, vNext=$\phi$}$\rangle$ into  $M_k$.\emph{\lsl} \& \blank{1.5cm} accessible via \rn only. /*\emph{mark=true}*/\label{lin:tc25}
			\EndIf\label{lin:tc26}
			\State Update \emph{preds[]} \& \emph{currs[]} of $m_{ij}$ in $\llog_i$.\label{lin:tc27}
			
			\EndFor \label{lin:tc28}
			%\EndFor
			\State Release the locks; return $\langle commit_i \rangle$.\label{lin:tc29}
			\EndProcedure \label{lin:tc30}
		\end{algorithmic}
%	\end{multicols}
\end{algorithm}

\vspace{.2mm}

\noindent
If $m_{ij}$ is \tdel{()} and key $k$ is exist in the $M_k.\lsl{}$ then it creates the new version $ver_i$ as $\langle \emph{ts=i, val=nil, rvl=}\phi, \emph{vrt=i, vNext=}\phi \rangle$ which is accessible via \rn{} only at \Lineref{tc25}. At last it updates the preds and currs of each $m_{ij}$ into its $txLog_i$ to help the upcoming methods of the same transactions in \emph{poValidation()} at \Lineref{tc27}. Finally, it releases the locks on all the keys in predefined order and returns \emph{commit} at \Lineref{tc29}.

\cmnt{
\vspace{-.15cm}

\begin{theorem}
Any legal history $H$ generated by SF-SVOSTM satisfies co-opacity.
\end{theorem}
\vspace{-.3cm}
\begin{theorem}
Any valid history $H$ generated by SF-KOSTM satisfies  local-opacity.
\end{theorem}
\vspace{-.3cm}
\begin{theorem}
SF-SVOSTM and SF-KOSTM ensure starvation-freedom in presence of a fair scheduler that satisfies \asmref{bdtm}(bounded-termination) and in the absence of parasitic transactions that satisfies \asmref{self}.
\end{theorem}
\vspace{-.2cm}
Please find the proof of theorems in \apnref{gcofo}, \apnref{gcoflo}, and \apnref{ap-cc}.
}

==> ap-model.tex <==
\section{Remaining System Model}
\label{apn:ap-model}
In this section we define other useful notions and definitions used in main
paper such as sequential histories, real-time order and serial history, valid and
legal history, sub-histories, opacity, conflict-opacity, local opacity and 
strict-serializability as follows:

\noindent
\textbf{Sequential Histories:} Following \cite{KuznetsovPeri:Non-interference:TCS:2017, KuznetsovRavi:ConcurrencyTM:OPODIS:2011},  if all the methods of the history are complete and isolated from each other, i.e. all the methods of history are atomic and following the total order in $H$. So, with this assumption, the only relevant methods of a transaction $T_i$ are $l_i(k,v)$, 
$l_i(k,\abort)$, $i_i(k, v)$, $d_i(k, v)$, $\tryc_i(\commit)$ (or $c_i$ for short), 
$\tryc_i(\abort)$, and $\trya_i(\abort)$ (or $a_k$ for short). We form the complete history $\overline{H}$, by immediately inserting the abort to all the live transactions of $H$. But, if the first operation of \emph{STM\_tryC$_i$()} has returned successfully then $T_i$ returns commit.

\noindent
\textbf{Real-Time Order and Serial History:} Two complete method $m_{ij}$ and $m_{xy}$ are said to be in method real-time order (or MR), if the response of $m_{ij}$ happens before the invocation of $m_{xy}$. Formally, if ($rsp(m_{ij}) <_H inv(m_{xy})$)$\implies$($m_{ij} \prec_H^{\mr} m_{xy}$). Following \cite{Papad:1979:JACM}, if transaction $T_i$ terminates (either commits or aborts) before beginning of $T_j$ then $T_i$ and $T_j$  follows transaction real-time order (or TR). Formally, if ($Term(T_i) <_H \tbeg_j()$)$\implies$($T_i \prec_H^{\tr} T_j$).  If all the transactions of a history $H$ follow the real-time order, i.e. transactions are atomic then such history is known as \emph{serial} \cite{Papad:1979:JACM} or \emph{t-sequential} \cite{KuznetsovRavi:ConcurrencyTM:OPODIS:2011} history. % Since, transactions are atomic then implicitly methods will also be atomic so, any serial history will also be a sequential history.
Formally, $\langle (H \text{ is serial}) \implies (\forall T_{i} \in \txns{H}: (T_i \in Term{(H)}) \land (\forall T_{i}, T_{j} \in \txns{H}: (T_{i} \prec_H^{\tr} T_{j}) \lor (T_{j} \prec_H^{\tr} T_{i}))\rangle$. In the serial history all the methods within a transaction are also ordered, it is also sequential.
%\noindent
%\textbf{Valid and Legal History:} If all the \emph{rv} methods of $H$ returns the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}. Whereas, If all the \emph{rv} methods of $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.


%has been considered corresponding to each aborted transactions while keeping all the committed transaction including the aborted transaction till its successful method.

\noindent
\textbf{Valid and Legal History:}  If \emph{$rv\_method()$}  on key $k$ returns the value from any of the previously committed transactions then such \emph{$rv\_method()$} is known as \emph{valid method}. If all the \emph{$rv\_methods()$} of history $H$ return the value from any of the previously committed transactions then such $H$ is known as \emph{valid history}.

 Whereas, If \emph{$rv\_method()$}  on key $k$ returns the value from previous closest committed transaction then such \emph{$rv\_method()$} is known as \emph{legal method}. If all the \emph{$rv\_methods()$} of history $H$ returns the value from the previous closest committed transactions then such $H$ is known as \emph{legal history}.
 
 \cmnt{
 %\section{Valid and Legal Histories}
 %\label{apn:legal}
 %\vspace{-2mm}
 %In this section, we start with defining legal histories. 
 To simplify our analysis, we assume that there exists an initial transaction $T_0$ that invokes $\tdel$ \mth on all the keys of the \tab{} used by any transaction. 
 
 A \rvmt{} (\tdel{} and \tlook{}) $m_{ij}$ on key $k$ is valid if it returns the value updated by any of the previous committed transaction that updated key $k$. A history $H$ is said to valid if all the \rvmt{s} of H are valid. 
 
 We define \emph{\legality{}} of \rvmt{s} on sequential histories which we use to define correctness criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}. Consider a sequential history $H$ having a \rvmt{} $\rvm_{ij}(ht, k, v)$ (with $v \neq null$) as $j^{th}$ method belonging to transaction $T_i$. We define this \rvm \mth{} to be \emph{\legal} if: 
 \vspace{-1mm}
 \begin{enumerate}
 	%\setlength\itemsep{-1em}
 	%\vspace{-.2cm}
 	\item[LR1] \label{step:leg-same} If the $\rvm_{ij}$ is not first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $m_{ix}$ is the previous \mth of $T_i$ on $\langle ht, k \rangle$. Formally, $\rvm_{ij} \neq \fkmth{\langle ht, k \rangle}{T_i}{H}$ $\land (m_{ix}\\(ht, k, v') = \pkmth{\langle ht, k \rangle}{T_i}{H})$ (where $v'$ could be null). Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		%		\item if $m_{ix}(ht, k, v')$ is a \tins{} \mth i.e. $\tins_{ix}(ht, k, v')$ then $v = v'$. 
 		%		\item if $m_{ix}(ht, k, v')$ is a \tlook{} \mth i.e. $\tlook_{ix}(ht, k, v')$ then $v = v'$. 
 		%		\item if $m_{ix}(ht, k, v')$ is a \tdel{} \mth i.e. $\tdel_{ix}(ht, k, v'/NULL)$ then $v = NULL$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tins{} \mth then $v = v'$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tlook{} \mth then $v = v'$. 
 		\item If $m_{ix}(ht, k, v')$ is a \tdel{} \mth then $v = null$.
 	\end{enumerate}
 	
 	In this case, we denote $m_{ix}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $m_{ix}(ht, k, v') = \\\lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 	
 	\item[LR2] \label{step:leg-ins} If $\rvm_{ij}$ is the first \mth{} of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is not null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v \neq null)$. Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		\item There is a \tins{} \mth{} $\tins_{pq}(ht, k, v)$ in $\met{H}$ such that $T_p$ committed before $\rvm_{ij}$. Formally, $\langle \exists \tins_{pq}(ht, k, v) \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. 
 		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 	\end{enumerate}
 	
 	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $\tryc_{p}(ht, k, v)$= $\lupdt{\rvm_{ij}(ht, k, v)}{H}$.
 	
 	\item[LR3] \label{step:leg-del} If $\rvm_{ij}$ is the first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v = null)$. Then,
 	\begin{enumerate}
 		\setlength\itemsep{0em}
 		\item There is \tdel{} \mth{} $\tdel_{pq}(ht, k, v')$ in $\met{H}$ such that $T_p$ (which could be $T_0$ as well) committed before $\rvm_{ij}$. Formally, $\langle \exists \tdel_{pq}\\(ht, k,$ $ v') \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. Here $v'$ could be null. 
 		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
 	\end{enumerate}
 	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e., $\tryc_{p}(ht, k, v)$ $= \lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
 \end{enumerate}
 %\vspace{-.3cm}
 We assume that when a transaction $T_i$ operates on key $k$ of a \tab{} $ht$, the result of this \mth is stored in \emph{local logs} of $T_i$, $\llog_i$ for later \mth{s} to reuse. Thus, only the first \rvmt{} operating on $\langle ht, k \rangle$ of $T_i$ accesses the shared-memory. The other \rvmt{s} of $T_i$ operating on $\langle ht, k \rangle$ do not access the shared-memory and they see the effect of the previous \mth{} from the \emph{local logs}, $\llog_i$. This idea is utilized in LR1. With reference to LR2 and LR3, it is possible that $T_x$ could have aborted before $\rvm_{ij}$. For LR3, since we are assuming that transaction $T_0$ has invoked a \tdel{} \mth{} on all the keys used of the \tab{} objects, there exists at least one \tdel{} \mth{} for every \rvmt on $k$ of $ht$. We formally prove legality in \apnref{cmvostm} and then we finally show that history generated by \hmvotm{} is \opq{} \cite{GuerKap:Opacity:PPoPP:2008}.
 
 %This we also call \emph{conflict inheritance} as the conflict of the later \mth{} of $T_i$ operating on $\langle ht, k \rangle$ can be found using the conflicts of the first \mth{} of $T_i$.
 
 Coming to \tins{} \mth{s}, since a \tins{} \mth{} always returns $ok$ as they overwrite the node if already present therefore they always take effect on the $ht$. Thus, we denote all \tins{} \mth{s} as \legal{} and only give legality definition for \rvmt{}. We denote a sequential history $H$ as \emph{\legal} or \emph{linearized} if all its \rvm \mth{s} are \legal.%A sequential history \emph{linearized} \cite{HerlWing:1990:TPLS}

}



\noindent
\textbf{Sub-history:} Following \cite{Chaudhary+:KSFTM:Corr:2017}, A \textit{sub-history} ($SH$) of a history ($H$) is a collection of events represented as $\evts{SH}$. We denote a $SH$ as the tuple $\langle \evts{SH},$ $<_{SH}\rangle$, here $<_{SH}$ represents the
total order of among all the events of $SH$. Formally, $SH$ is defined as: (1) $<_{SH} \subseteq <_{H}$; (2) $\evts{SH} \subseteq \evts{H}$; (3) If an event of a transaction $T_k\in\txns{H}$ is in $SH$ then all the events of $T_k$ in $H$ should also be in $SH$. 

Let $P$ is a subset of $H$ which consists of a set transactions $\txns{H}$. Then the sub-history of $H$ is represented as $\shist{P}{H}$ which comprises of $\evts{}$ of $P$. 

\noindent
\textbf{Conflict-opacity (or Co-opacity):} It is a well known correctness criteria of STMs that is polynomial time verifiable. Co-opacity \cite{Peri+:OSTM:Netys:2018} is a subclass of opacity. A history $H$ is co-opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time as $H$ $\prec_S^{\tr} \subseteq \prec_H^{\tr}$. (4) $S$ preserves conflict-order of $H$, i.e. $\prec_S^{Conf} \subseteq \prec_H^{Conf}$.

\noindent
\textbf{Opacity and Strict Serializability:} A popular correctness criteria for STMs is opacity \cite{GuerKap:Opacity:PPoPP:2008}. A valid history $H$ is opaque, if there exist a serial history $S$ with following properties: (1) $S$ and $\overline{H}$ are equivalent, i.e. $\evts{S} = \evts{\overline{H}}$. (2) $S$ should be legal. (3) $S$ should respect the transactional real-time order as $H$, i.e. $\prec_S^{\tr} \subseteq \prec_H^{\tr}$.

 A valid history $H$ is strict serializable \cite{Papad:1979:JACM}, if sub-history  of $H$ as $\subhist(H)$ (consists of all the committed transactions of $H$) is opaque, i.e., $H.subhist(H.committed)$ is \emph{opaque}. So, if a history is \emph{strict serializable} then it will be \opq as well but  the vice-versa is not true. Unlike opacity, \emph{strict serializability} does not consider aborted transactions.

A commonly used correctness criteria in databases is \emph{serializability} \cite{Papad:1979:JACM} which considers committed transactions only. Guerraoui \& Kapalka \cite{GuerKap:Opacity:PPoPP:2008} show that STMs considers the correctness of \emph{aborted} transactions along with \emph{committed} transactions as well. So,  \emph{serializability} is not suitable for STMs. On the other hand, \emph{opacity} \cite{GuerKap:Opacity:PPoPP:2008} is a popular correctness criteria for STMs which considers \emph{aborted} as well as \emph{committed} transactions. Similar to \emph{opacity} but less restrictive, an another popular correctness criteria is \emph{local opacity} defined below.



\noindent
\textbf{Local Opacity (or LO):} It is an another popular correctness criteria for STMs which is less restrictive than opacity. Local-opacity \cite{KuznetsovPeri:Non-interference:TCS:2017} is a superclass of opacity. It considers a set of sub-histories for history $H$, denoted as $\shset{H}$ as follows: (1) We construct a $\subhist$ corresponding to each aborted transaction $T_i$ while including all the events $\evts{}$ of previously \emph{committed} transactions along with all successful $\evts{}$ of $T_i$ (i.e., $\evts{}$ which has not returned $\mathcal{A}$ yet) and put \emph{committed} $\mathcal{C}$ immediately after last successful operation of $T_i$; (2) We construct one more sub-history corresponding to last \emph{committed} transaction $T_l$ which considers all the previously \emph{committed} transactions only including  $T_l$.

If all the above defined sub-histories $\shset{H}$ for a history $H$ are opaque then $H$ is said to be \emph{\lopq} \cite{KuznetsovPeri:Non-interference:TCS:2017}. We can observe that a sub-history corresponding to an aborted transaction $T_i$ contains $\evts{}$ from only one aborted transaction which is $T_i$ itself and does not consider any other live/aborted transactions. Similarly, sub-history corresponding to last \emph{committed} transaction $T_l$ does not consider any $\evts{}$ of aborted and live transactions. Thus in \lopty, neither aborted nor live transaction cause any other transaction to abort. Researchers have been proved that \lopty 
\cite{KuznetsovPeri:Non-interference:TCS:2017} ensures greater concurrency than \opty \cite{GuerKap:Opacity:PPoPP:2008}. If a history is \opq then it will be \lopq as well but  the vice-versa is not true. On the other hand, if a history is \lopq then it will be \stsble as well, but the vice-versa need not be true. Please find  illustrations of local opacity in \apnref{gcoflo}.




\cmnt{
\todo{Copy conflict-notion from OSTM}



Opacity is a popular \cc{} for STMs. But, as observed in \secref{intro}, it can be proved that verifying the membership of \opty similar to view-serializability (VSR) in databases is NP-Complete \cite{Papad:1979:JACM}. To circumvent this issue, researchers in databases have identified an efficient sub-class of VSR, called conflict-serializability or \csr, based on the notion of conflicts. The membership of \csr can be verified in polynomial time using conflict graph characterization. Along the same lines, we develop the notion of conflicts for \otm and identify a sub-class of \opty, \coopty. The proposed \cc{} is extension of the notion of conflict-opacity developed for \emph{\rwtm} by Kuznetsov \& Peri \cite{KuzPer:NI:TCS:2017}.

We say two transactions $T_i, T_j$ of a sequential history $H$ for \otm{} are in \emph{conflict} if atleast one of the following conflicts holds:
\vspace{-.2cm}
\begin{itemize}
	\setlength\itemsep{0em}
	\item \textbf{tryC-tryC} conflict:(1) $T_i$ \& $T_j$ are committed and (2) $T_i$ \& $T_j$ update the same key $k$ of the \tab{}, $ht$, i.e., $(\langle ht,k \rangle \in \udset{T_i}) \land (\langle ht,k \rangle \in \udset{T_j})$, where $\udset{T_i}$ is update set of $T_i$. (3) $T_i$'s \tryc{} completed before $T_j$'s \tryc, i.e., $\tryc_i \prec_{H}^{\mr} \tryc_j$. 
	
	\item \textbf{tryC-rv} conflict:(1) $T_i$ is committed (2) $T_i$ updates the key $k$ of \tab{}, $ht$. $T_j$ invokes a \rvmt{} $rvm_{jy}$ on the key same $k$ of \tab{} $ht$ which is the first \mth{} on $\langle ht, k \rangle$. Thus, $(\langle ht,k \rangle \in \udset{T_i}) \land (\rvm_{jy}(ht, k, v) \in \rvset{T_j}) \land (\rvm_{jy}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_j}{H})$, where $\rvset{T_j}$ is return value set of $T_j$. (3) $T_i$'s \tryc{} completed before $T_j$'s \rvm, i.e., $\tryc_i \prec_{H}^{\mr} \rvm_{jy}$.% Same conflict is preserved by the subsequent \mth{s} of $T_j$, we call it \emph{conflict inheritance}. 
	
	\item \textbf{rv-tryC} conflict:(1) $T_j$ is committed (2) $T_i$ invokes a \rvmt on the key same $k$ of \tab{} $ht$ which is the first \mth{} on $\langle ht, k \rangle$. $T_j$ updates the key $k$ of the \tab{}, $ht$. Thus, $(\rvm_{ix}(ht, k, v) \in \rvset{T_i}) \land (\rvm_{ix}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H}) \land (\langle ht,k \rangle \in \udset{T_j})$ (3) $T_i$'s \rvm completed before $T_j$'s \tryc, i.e., $\rvm_{ix} \prec_{H}^{\mr} \tryc_j$. %Similarly, all subsequent \mth{s} of $T_i$ which happen before $\tryc_j$ preserve the same conflict we term it as \emph{conflict inheritance}. 
\end{itemize}

A \rvmt{} $\rvm_{ij}$ conflicts with a \tryc{} \mth{} only if $\rvm_{ij}$ is the first \mth{} of $T_i$ that operates on \tab{} with a given key. Thus the conflict notion is defined only by the \mth{s} that access the shared memory. $(\tryc_i{}, \tryc_j{})$, $(\tryc_i{}, \tlook_j)$, $(\tlook_i, \tryc_j{})$, $(\tryc_i{}, \tdel_j)$ and $(\tdel_i, \tryc_j{})$ can be the possible conflicting \mth{s}. For example, consider the history $H5: l_1(ht, k_1, NULL) l_2(ht, k_2$ $, NULL) i_2(ht, k_1, v_1) i_1(ht, k_4,$ $v_1) c_1 i_3(ht, k_3\\, v_3) c_3 d_2(ht, k_4, v_1) c_2 l_4(ht, k_4, NULL)$ $i_4(ht, k_2, v_4) c_4$ in \figref{netys}. $(l_1(ht, k_1, NULL), i_3(ht, k_1, v_1))$ and $(l_2(ht, k_2, NULL), i_4$ $(ht, k_2, v_4))$ are a conflict of type \emph{rv-tryC}. Conflict type of $(i_1(ht, k_4, v_1), \\d_2(ht, k_4, v_1))$ and $(i_1(ht, k_4, v_1),$ $l_4(ht, k_4, NULL))$ are \emph{tryC-tryC} and \emph{tryC-rv} respectively. 
%\vspace{-.3cm}
\begin{figure}[H]
	\centering
	%		\captionsetup{justification=centering}
	\scalebox{.5}{\input{figs/netys.pdf_t}}
	% \vspace{-16cm}
	\caption{Graph Characterization of history $H5$}
	\label{fig:netys}
\end{figure}

\vspace{1mm}
\noindent
\textbf{Conflict Opacity:} Using this conflict notion, we can now define \coopty. A sequential history $H$ is conflict-opaque (or co-opaque) if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e. , $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$ and (4) S preserves conflicts (i.e. $\prec^{CO}_{H}\subseteq\prec^{CO}_{S}$). 

\noindent Thus from the above definition, it can be seen that any history that is \coop is also \opq. 
\ignore{
	\vspace{-.4cm}
	\begin{definition}
		\label{def:co-opacity}
		\texttt{Co-opacity :} 	A sequential history $H$ is conflict-opaque (or co-opaque) if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e. , $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$ and (4) S preserves conflicts (i.e. $\prec$$^{CO}_{H}$ $\subseteq$ $\prec$$^{CO}_{S}$) \cite{KuzPer:NI:TCS:2017}. 
	\end{definition}
	\vspace{-.5cm}
}

\vspace{1mm}
\noindent
\textbf{Graph Characterization:} We now develop a graph characterization of \coopty. For a sequential history $H$, we define \emph{conflict-graph} of $H$, $\cg{H}$ as the pair $(V, E)$ where $V$ is the set of $\txns{H}$ and \emph{E} can be of following types: (a) \emph{conflict edges:} \{($T_i$, $T_j$) : ($T_i$, $T_j$) $\in$ \conf{H}\} where, \conf{H} is an ordered pair of transactions such that the transactions have one of the above pair of conflicts. (b) \emph{real-time edge(or rt edge):} \{($T_i$, $T_j$): Transaction $T_i$ precedes $T_j$ in real-time, i.e., $T_i \prec_{H}^{\tr} T_j $\}.

\ignore{
	\vspace{-.2cm}
	\begin{itemize}%[noitemsep,nolistsep]
		\item \emph{conflict edges:} \{($T_i$, $T_j$) : ($T_i$, $T_j$) $\in$ \conf{H}\} where, \conf{H} is an ordered pair of transactions such that the transactions have one of the above pair of conflicts. 
		
		\item \emph{real-time edge(or rt edge):} \{($T_i$, $T_j$) : $T_i \prec_{H}^{\tr} T_j $\}
	\end{itemize}
}

Now, we have the following theorem which explains how graph characterization is useful.

\ignore{
	\begin{lemma}
		\otm{} histories are sequential and legal.
		\vspace{-0.4cm}
	\end{lemma}
	
	In the accompanying report\cite{DBLP:journals/corr/abs-1709-00681} we show that at operational level \otm{} histories are linearizable and the conflicts \mth{} can be ordered in such a way that the generated sequential histories are legal.
}
%\vspace{-.3cm}
\begin{theorem}
	\label{thm:coop-graph}
	A legal \otm{} history $H$ is \coop{} iff CG(H) is acyclic.
	%\vspace{-0.4cm}
\end{theorem}
\noindent Using this framework, we next develop \otm using the notion of \bto. We show the correctness of the proposed algorithm by showing that all conflict graph of the histories generated by it are acyclic. %The legality and conflict notion established here are used to prove that histories generated by the \otm{} are correct or \coop{}\cite{KuzPer:NI:TCS:2017} in \secref{POC}.





\noindent
\textbf{Local-Opacity:} Following \cite{KuznetsovPeri:Non-interference:TCS:2017}, it is also a correctness criteria of a history $H$ which says if all the sub histories $SH$ corresponding to each aborted transactions and $SH$ corresponding to last committed transactions while considering only committed transactions are opaque then $H$ is locally opaque. Here, a sub history $SH$ consists of committed transaction till the successful methods of aborted transactions in it.

%Due to lack of space, please refer  \apnref{ap-corr} for the definition of valid history, legal history, opacity, co-opacity and local-opacity.

}

==> citations <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Sathya Peri",
%%%     date            = "17 Spet 2009",
%%%     filename        = "citations.bib",
%%%     url             = ""
%%%     www-home        = "http://www.cs.mun.ca/~sathya/",
%%%     address         = "Department of Computer Science,
%%%                        MUN,
%%%                        St John's, CA A1B 3X5,
%%%                        Canada",
%%%     email           = "sathya at mun.ca",
%%%     dates           = {1950--},
%%%     keywords        = "",
%%%     supported       = "yes",
%%%     supported-by    = "Sathya Peri",
%%%     abstract        = "Bibliography for Sathya Peri"
%%%  }
%%% ====================================================================


@String{PROC = {Proceedings of the}}
@String{AMS = {American Mathematical Society}}
@String{AW = {Addison-Wesley}}
@String{TCS = {Theoretical Computer Science}}
@String{JPDC = {Journal of Parallel and Distributed Computing (JPDC)}}
@String{WDAG = {Workshop on Distributed Algorithms (WDAG)}}
@String{WPDD = {ACM/ONR Workshop on Parallel and Distributed Debugging}}
@String{DC = {Distributed Computing (DC)}}
@String{TrCS = {ACM Transactions on Computer Systems}}
@String{SPDP = {IEEE Symposium on Parallel and Distributed Processing (SPDP)}}
@String{ICPP = {International Conference on Parallel Processing}}
@String{Com = {IEEE Computer}}
@String{KAP = {Kluwer Academic Publishers}}
@String{WAD = {International Workshop on Automated Debugging (AADEBUG)}}
@String{CSS = {International Conference on System Sciences}}
@String{Fre = {W. H. Freeman and Company, New York}}
@String{TPDS = {IEEE Transactions on Parallel and Distributed Systems (TPDS)}}
@String{FTCS = {IEEE Fault-Tolerant Computing Symposium (FTCS)}}
@String{JCC = {Journal of Computer Communications}}
@String{WSCT = {International Workshop on Structures in Concurrency Theory (STRICT)}}
@String{MH = {McGraw-Hill}}
@String{CACM = {Communications of the ACM (CACM)}}
@String{ICDCS = {IEEE International Conference on Distributed Computing Systems (ICDCS)}}
@String{PODC = {ACM Symposium on Principles of Distributed Computing (PODC)}}
@String{JS = {Journal of Supercomputing}}
@String{CAV = {International Conference on Computer-Aided Verification (CAV)}}
@String{LNCS = {Lecture Notes in Computer Science (LNCS)}}
@String{WPDS = {Workshop on Parallel and Distributed Simulation}}
@String{DISC = {Symposium on Distributed Computing (DISC)}}
@String{CSE = {Computer Science and Education}}
@String{TMH = {Tata McGraw-Hill Publishing Company Limited}}
@String{ES = {Elsevier Science Publishers B. V. (North-Holland)}}
@String{PDS = {The Parallel and Distributed Systems Laboratory}}
@String{DECE = {Department of Electrical and Computer Engineering}}
@String{DCS = {Department of Computer Science}}
@String{PPL = {Parallel Programming Laboratory}}
@String{UIUC = {University of Illinois at Urbana-Champaign}}
@String{UTA = {The University of Texas at Austin}}
@String{OSU = {The Ohio State University}}
@String{UTD = {The University of Texas at Dallas}}
@String{TC = {IEEE Transactions on Computers}}
@String{IPL = {Information Processing Letters (IPL)}}
@String{AMCSJ = {Applied Mathematics and Computer Science Journal}}
@String{WLCPC = {Workshop on Language and Compilers for Parallel Computing}}
@String{IBMARC = {IBM Almaden Research Center}}
@String{IBMZ = {IBM Research Laboratory, Zurich}}
@String{ICDE = {International Conference on Data Engineering (ICDE)}}
@String{CUP = {Cambridge University Press}}
@String{MVPP = {International Meeting on Vector and Parallel Processing}}
@String{TOPLAS = {ACM Transactions on Programming Languages and Systems (TOPLAS)}}
@String{SPDT = {Symposium on Parallel and Distributed Tools}}
@String{CJ = {The Computer Journal}}
@String{PH = {Prentice Hall}}
@String{MK = {Morgan Kaufmann}}
@String{SIGMOD = {ACM SIGMOD International Conference on Managament of Data}}
@String{SIGACT = {ACM Special Interest Group on Algorithms and Computation Theory (SIGACT)}}
@String{USPATENT = {United States Patent Number}}
@String{INFORMIX = {Informix Software Incorporated}}
@String{SV = {Springer-Verlag}}
@String{PDCS = {ISCA International Conference on Parallel and Distributed Computing Systems (PDCS)}}
@String{MIT = {The MIT Press}}
@String{JHUP = {The Johns Hopkins University Press}}
@String{DAM = {Discrete Applied Mathematics}}
@String{DM = {Discrete Mathematics}}
@String{DS = {Distributed Systems}}
@String{ICSKE = {IEEE International Conference on Software and Knowledge Engineering}}
@String{FSTTCS = {Conference on the Foundations of Software Technology and Theoretical
                  Computer Science (FSTTCS)}}
@String{TSE = {IEEE Transactions on Software Engineering}}
@String{JSS = {The Journal of Systems and Software}}
@String{WGCS = {International Workshop on Graph-Theoretic Concepts in Computer Science (WG)}}
@String{JWS = {John Wiley and Sons Limited}}
@String{JWSUS = {John Wiley and Sons, Incorporated}}
@String{ORDAL = {International Conference on Orders, Algorithms and Applications (ORDAL)}}
@String{AJM = {American Journal of Mathematics}}
@String{SRKU = {Sci. Reports Kanazawa Univ.}}
@String{SIAMJDM = {SIAM Journal on Discrete Mathematics}}
@String{KRUSE = {International KRUSE Symposium: Knowledge Use, Retrieval and Storage for Efficiency}}
@String{SIAMJADM = {SIAM Journal on Algebraic and Discrete Methods}}
@String{SIAMJC = {SIAM Journal on Computing}}
@String{MCT = {Mathematical Center Tracts}}
@String{STOC = {Annual ACM Symposium on Theory of Computing (STOC)}}
@String{OOPSLA = {Conference on Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}}
@String{JLMS = {Journal London Mathematics Society}}
@String{AM = {Annals of Mathematics}}
@String{TIT = {IEEE Transactions on Information Theory}}
@String{TR = {IEEE Transactions on Reliability}}
@String{WLP = {Workshop on Logics of Programs}}
@String{ISP = {International Symposium in Programming}}
@String{WSS = {Workshop on Self-Stabilizing Systems (WSS)}}
@String{ICALP = {International Colloquium on Automata, Languages and Systems (ICALP)}}
@String{JA = {Journal of Algorithms}}
@String{KDE = {IEEE Transactions on Knowledge and Data Engineering}}
@String{CS = {ACM Computing Surveys (CSUR)}}
@String{IPDPS = {International Parallel and Distributed Processing Symposium (IPDPS)}}
@String{PDC = {Parallel and Distributed Conference}}
@String{SP = {IEEE Symposium on Security and Privacy}}
@String{USS = {USENIX Security Symposium}}
@String{WNTS = {USENIX Windows NT Symposium}}
@String{UCS = {Computing Systems}}
@String{NCSC = {National Computer Security Conference}}
@String{RV = {Workshop on Runtime Verification (RV)}}
@String{ICPDCS = {IASTED International Conference on Parallel and Distributed Computing and Systems}}
@String{MCDS = {SCS MultiConference on Distributed Simulation}}
@String{SCS = {Society for Computer Simulation}}
@String{BCPC = {The Benjamin Cummings Publishing Company, Incorporated}}
@String{OPODIS = {International Conference on Principles of Distributed Systems (OPODIS)}}
@String{TWSIS = {Texas Workshop on Security of Information Systems (TWSIS)}}
@String{SCISS = {South Central Information Security Symposium (SCISS)}}
@String{CSS = {Computing Systems}}
@String{UCD = {University of California, Davis}}
@String{CSAC = {Annual Computer Security Applications Conference}}
@String{WETICE = {IEEE Workshop on Enabling Technologies: Infrastructure for Collaborative
                  Enterprises (WETICE)}}
@String{TOG = {ACM Transactions on Graphics}}
@String{SCCS = {School of Computer and Communication Sciences}}
@String{EPFL = {{\'E}cole Polytechnique F{\'e}d{\'e}rale de Laussane (EPFL)}}
@String{CORNELL = {Cornell University}}
@String{COMPSAC = {Annual Internation Computer Software and Applications Conference (COMPSAC)}}
@String{JPL = {Journal of Programming Languages}}
@String{PC = {Parallel Computing}}
@String{UWM = {University of Wisconsin, Madison}}
@String{UWTC = {USENIX Winter Technical Conference}}
@String{ICSSE = {Israeli Conference on Computer Systems and Software Engineering}}
@String{IPPS = {International Parallel and Processing Symposium (IPPS)}}
@String{HIS = {Journal of High Integrity Systems}}
@String{HPL = {Hewlett Packard Laboratories}}
@String{ACTA = {Acta Informatica}}
@String{FOCS = {Annual Symposium on Foundations of Computer Science (FOCS)}}
@String{CDS = {IEEE Proceedings---Computers and Digital Techniques}}
@String{JISE = {Journal of Information Science and Engineering}}
@String{ICPADS = {International Conference on Parallel and Distributed Systems (ICPADS)}}
@String{WPPS = {International Workshop on Peer-to-Peer Systems}}
@String{SAC = {IEEE Journal on Selected Areas in Communications}}
@String{TN = {IEEE/ACM Transactions on Networking}}
@String{SNA = {ACM-SIAM Symposium on Discrete Algorithms}}
@String{SIU = {Studia Informatica Universalis}}


@Unpublished{8LGM:1992,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk} (January 1992)}
}

@Article{AchBad:1992:IPL,
  author =   {A. Acharya and B. R. Badrinath},
  title =    {{Recording Distributed Snapshots Based on Causal
                   Order of Message Delivery}},
  journal =  IPL,
  volume =   {44},
  number =   {6},
  pages =    {317-321},
  year =     {1992},
  OPTurl =   {http://citeseer.nj.nec.com/acharya92recording.html}
}

@Misc{Adv:1990:SM,
  title =    {{Sendmail Vulnerability}},
  howpublished = {CERT Advisory CA-90:01 available from \textsf{cert.org} via anonymous ftp},
  month =    JAN,
  year =     {1990}
}

@Article{Adv:1992:Mail,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    JAN,
  year =     1992
}

@Article{Adv:1994:Pwd,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-7.UNIX.passwd.11-May-1994}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    MAY,
  year =     1994
}

@Article{AfeBre:1998:TCS,
  author =   {Y. Afek and A. Bremler},
  title =    {{Self-Stabilizing Unidirectional Network Algorithms by Power Supply}},
  journal =      TCS,
  year =     1998,
  volume =   1998,
  number =   3,
  month =    DEC
}

@InProceedings{AfeKut+:1991:WDAG,
  author =       {Y. Afek and S. Kutten and M. Yung},
  title =        {{Memory-Efficient Self-Stabilizing Protocols for General Networks}},
  booktitle =    PROC # " 4th " # WDAG,
  year =         {1991},
  pages =        {15-28},
  address =      {Bari, Italy},
  publisher =    SV,
}

@Manual{AgaGoe+:1996:IBM,
  author =   {A. Agarwal and A. Goel and A. Sood},
  title =    {{Software Design Description for DLFS on Solaris,
                  HP-UX, and AIX}},
  year =     {1996}
}

@InProceedings{AgrBor+:1989:MD,
  author =   {R. Agrawal and A. Borgida and H. V. Jagadish},
  title =    {{Efficient Management of Transitive Relationships in
                  Large Data and Knowledge Bases}},
  booktitle =    PROC # " " # SIGMOD,
  pages =    {253-262},
  year =     1989,
  address =  {Portland, Oregon}
}

@Book{AhoHop:1974:AW,
  author =   {A. V. Aho and J. E. Hopcroft and J. D. Ullman},
  OPTeditor =    {~},
  title =    {{The Design and Analysis of Computer Algorithms}},
  publisher =    AW,
  year =     1974,
  OPTnote =  {pages 384-386}
}

@InProceedings{AlaVen:1993:WAD,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Hierarchy in Testing Distributed Programs}},
  booktitle =    PROC # " " # WAD,
  pages =    {101-116},
  year =     {1993}
}

@Article{AlaVen:1994:IPL,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{An Optimal Algorithm for Recording Snapshots using Casual
                   Message Delivery}},
  journal =  IPL,
  year =     {1994},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  pages =    {311-316},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@InProceedings{AlaVen:1994:PDS,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  booktitle =    PROC # " " # PDS,
  pages =    {412-417},
  month =    DEC,
  year =     {1994}
}

@Article{AlaVen:2001:TSE,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  journal =  TSE,
  year =     2001,
  volume =   27,
  number =   8,
  pages =    {704-714},
  month =    AUG
}

@TechReport{AlaVid:1999:TR,
  author =   {K. Alagarsamy and K.Vidyasankar},
  title =    {{Elegant Solutions for Group Mutual Exclusion Problem}},
  institution =  {Department of Computer Science, Memorial University of Newfoundland,
                  St.John's, Newfoundland, Canada},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlmBaq+:2002:ICDCS,
  author =   {P. S. Almeida and C. Baquero and V. Fonte},
  title =    {{Version Stamps---Decentralized Version Vectors}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 22nd " # ICDCS,
  pages =    {544-551},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlvEln+:1999:FTCS,
  author =   {L. Alvisi and E. N. Elnozahy and S. Rao and
                  S. A. Hussain and A. D. Mel},
  title =    {{An Analysis of Communication-Induced Checkpointing}},
  booktitle =    PROC # " 29th " # FTCS,
  pages =    {242-249},
  year =     1999,
  address =  {Madison, Wisconsin},
  month =    JUN
}

@InProceedings{AlvMar:1995:ICDCS,
  author =   {L. Alvisi and K. Marzullo},
  title =    {{Message Logging: Pessimistic, Optimistic, and Causal}},
  booktitle =    PROC # " 15th " # ICDCS,
  pages =    {229-236},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@MastersThesis{Ang:2001:Thesis,
  author =   {R. Anguiano},
  title =    {{A Static Analysis Technique for the Detection of
                   TOCTTOU Vulnerabilities}},
  school =   {University of California, Davis},
  year =     {2001},
  OPTkey =   {},
  OPTtype =  {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{AroGou:1994:TC,
  author =   {A. Arora and M. G. Gouda},
  title =    {{Distributed Reset}},
  journal =      TC,
  year =     1994,
  volume =   43,
  number =   9,
  pages =    {1026-1038}
}

@Article{AroSin:1995:HIS,
  author =   {A. Arora and A. Singhai},
  title =    {{Fault-Tolerant Reconfiguration of Trees and Rings in Distributed Systems}},
  journal =      HIS,
  year =     1995,
  volume =   1,
  number =   4,
  pages =    {375-384}
}

@InProceedings{AtrMit+:2003:OPODIS,
  author =   {R. Atreya and N. Mittal and V. K. Garg},
  title =    {{Detecting Locally Stable Predicates without
                   Modifying Application Messages}},
  booktitle =    PROC # " 7th " # OPODIS,
  year =     2003,
  pages =        {20-33},
  address =  {La Martinique, France},
  month =    DEC
}

@Article{BabFro+:1996:JSS,
  author =   {{\"O}. Babao{\v{g}}lu and E. Fromentin and
                  M. Raynal},
  title =    {{A Unified Framework for the Specification and Run-time Detection
                   of Dynamic Properties in Distributed Computations}},
  journal =  JSS,
  volume =   {33},
  number =   {3},
  month =    JUN,
  pages =    {287-298},
  year =     {1996},
  url =      {http://citeseer.nj.nec.com/10396.html}
}

@incollection{BabMar:1993:DS,
  author =   {{\"{O}}. Babao{\v g}lu and K. Marzullo},
  title =    {{Consistent Global States of Distributed Systems: Fundamental Concepts and
                   Mechanisms}},
  booktitle =    DS,
  publisher =    AW,
  editor =   {S. Mullender},
  pages =    {55-96},
  year =     {1993},
  url =
                  {http://citeseer.nj.nec.com/babaoglu93consistent.html}
}

@Article{BabRay:1995:JPDC,
  author =   {{\"{O}}. Babao{\v g}lu and M. Raynal},
  title =    {{Specification and Verification of Dynamic Properties in Distributed Computations}},
  journal =  JPDC,
  year =     1995,
  volume =   28,
  number =   2,
  pages =    {173-185}
}

@Book{Bac:1987:Book,
  author =   {M. J Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987,
  isbn =     0132017997
}

@Book{Bac:1987:PH,
  author =   {M. J. Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987
}

@Manual{BalKan:1999:INFORMIX,
  author =   {I. Balabine and R. Kandasamy},
  title =    {{File System Interface to a Database}},
  note =     USPATENT # " 5937406 granted to " # INFORMIX,
  year =     {1999},
  month =    AUG
}

@InProceedings{BarBra+:1996:ICSSE,
  author =   {A. Barak and A. Braverman and A. Gilderman and O. La'adan},
  title =    {{Performance of PVM with MOSIX Preemptive Process Migration}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 7th " # ICSSE,
  pages =    {38-45},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Herzliya},
  month =    JUN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BeaCan+:2003:JISE,
  author =   {J. Beauquier and S. Cantarell and A. K. Datta and F. Petit},
  title =    {{Group Mutual Exclusion in Tree Networks}},
  journal =      JISE,
  year =     {2003},
  OPTkey =   {},
  volume =   {19},
  number =   {3},
  pages =    {415-432},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{BegDon+:PVM2.0,
  title =    {{H}ence: {A} users' guide - version 2.0. {PVM}
                  {D}esign and {V}isualization},
  author =   {A. Beguelin and J. Dongarra and G. A. Geist and
                  R. Manchek and K. Moore and P. Newton and
                  V. Sunderam}
}

@InProceedings{Bel:1990:MCDS,
  author =   {S. Bellenot},
  title =    {{Global Virtual Time Algorithms}},
  booktitle =    PROC # " " # MCDS,
  pages =    {122-127},
  year =     1990,
  volume =   22,
  number =   1,
  month =    JAN,
  organization = SCS
}

@TechReport{Bis:1995:TR:8,
  author =   {M. Bishop},
  title =    {{Race Conditions, Files, and Security Flaws: or, The
                   Tortoise and the Hare \emph{Redux}}},
  institution =  DCS # ", " # UCD,
  year =     {1995},
  OPTkey =   {},
  OPTtype =  {},
  number =   {95-8},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{BisDil:1996:CSS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File Accesses}},
  journal =  CSS,
  year =     2003,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Article{BisDil:1996:UCS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File
                  Accesses}},
  journal =  UCS,
  year =     1996,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Unpublished{BisHol:1978:PR:13,
  author =   {R. Bisbey and D. Hollingsworth},
  title =    {{Protection Analysis Project Final Report}},
  note =     {ISI/RR-78-13, DTIC AD A056816, USC/Information
                  Sciences Institute},
  OPTkey =   {},
  month =    MAY,
  year =     {1978},
  OPTannote =    {}
}

@Article{Bou:1987:TCS,
  author =   {L. Bouge},
  title =    {{Repeated Snapshots in Distributed Systems
                  with Synchronous Communication and their
                  Implementation in CSP}},
  journal =  TCS,
  year =     1987,
  volume =   49,
  pages =    {145-169}
}

@Article{Bre:1966:TIT,
  author =   {M. Breuer},
  title =    {{Coding Vertexes of a Graph}},
  journal =  TIT,
  year =     1966,
  volume =   12,
  pages =    {148-153}
}

@TechReport{BriLit+:1992:CONDOR,
  author =   {A. Bricker and M. Litzkow and M. Livny},
  title =    {{Condor Technical Summary, Version 4.1b}},
  institution =  "Computer Science Department, " # UWM,
  year =     {1992},
  OPTkey =   {},
  OPTtype =      {},
  number =   {CS-TR-92-1069},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BrzHel+:1993:ICDCS,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal},
  title =    {{Termination Detection in a Very General Distributed
                   Computing Model}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {374-381},
  year =     1993
}

@article{BrzHel+:1995:JPDC,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal and
                  M. Singhal},
  title =    {{Deadlock Models and a General Algorithm for
                   Distributed Deadlock Detection}},
  journal =  JPDC,
  volume =   {31},
  number =   {2},
  pages =    {112-125},
  year =     "1995"
}

@Misc{Bug:2002:RDR,
  title =    {{Recursive Directory Removal Race Condition}},
  howpublished = {http://mail.gnu.org/pipermail/bug-fileutils/2002-March/002433.html},
  month =    MAR,
  year =     2002
}

@Manual{CORBA:1997,
  author =   {Object Management Group},
  title =    {{The Common Object Request Broker: Architecture and Specification}}
}

@InProceedings{CanDat+:2001:ICDCS,
  author =   {S. Cantarell and A. K. Datta and F. Petit and V. Villain},
  title =    {{Token Based Group Mutual Exclusion for Asynchronous Rings}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {691-694},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Cap:1994:ORDAL,
  author =   {C. Capelle},
  title =    {{Representation of an Order as Union of Interval Orders}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {143-161},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =  {Lyon, France},
  month =    JUL,
  publisher =    SV
}

@InProceedings{Cas:1993:OOPSLA,
  author =   {Y. Caseau},
  title =    {{Efficient Handling of Multiple Inheritance Hierarchies}},
  booktitle =    PROC # " " # OOPSLA,
  pages =    {271-287},
  year =     1993
}

@Article{Cas:1995:CSS,
  author =   {J. Casas and R. Konuru and S. W. Otto and R. M. Prouty and J. Walpole},
  title =    {{MPVM---A Migration Transparent Version of PVM}},
  journal =      CSS,
  year =     {1995},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {171-216},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaDel+:1995:TOPLAS,
  author =   {B. Charron-Bost and C. Delporte-Gallet and
                  H. Fauconnier},
  title =    {{Local and Temporal Predicates in Distributed Systems}},
  journal =  TOPLAS,
  year =     1995,
  volume =   17,
  number =   1,
  pages =    {157-179}
}

@InProceedings{ChaGar:1995:WDAG,
  author =   {C. Chase and V. K. Garg},
  title =    {{On Techniques and their Limitations for the Global Predicate
                   Detection Problem}},
  booktitle =    PROC # " " # WDAG,
  year =     1995,
  address =  {France},
  month =    SEP,
  pages =    {303-317}
}

@Article{ChaGar:1998:DC,
  author =   {C. Chase and V. K. Garg},
  title =    {{Detection of Global Predicates: Techniques and their Limitations}},
  journal =  DC,
  year =     1998,
  volume =   11,
  number =   4,
  pages =    {191-201}
}

@Article{ChaLam:1985:TrCS,
  author =   {K. M. Chandy and L. Lamport},
  title =    {{Distributed Snapshots: Determining Global States of Distributed Systems}},
  journal =  TrCS,
  year =     1985,
  volume =   3,
  number =   1,
  pages =    {63-75},
  month =    FEB
}

@Article{ChaMis+:1983:TrCS,
  author =   {K. M. Chandy and J. Misra and L. M. Haas},
  title =    {{Distributed Deadlock Detection}},
  journal =      TrCS,
  year =     1983,
  volume =   1,
  number =   2,
  pages =    {144-156},
  month =    MAY
}

@Article{ChaMis:1984:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{The Drinking Philosophers Problem}},
  journal =      TOPLAS,
  year =     {1984},
  OPTkey =   {},
  volume =   {6},
  number =   {4},
  pages =    {632-646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:DC,
  author =   {K. M. Chandy and J. Misra},
  title =    {{How Processes Learn}},
  journal =  DC,
  year =     {1986},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {40-52},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Book{ChaMis:1988:Book,
  author =   {K. M. Chandy and J. Misra},
  title =    {{Parallel Program Design: A Foundation}},
  publisher =    AW,
  year =     1988
}

@Article{ChaTou:1996:JACM,
  author =   {T. D. Chandra and S. Toueg},
  title =    {{Unreliable Failure Detectors for Reliable Distributed Systems}},
  journal =  JACM,
  year =     {1996},
  volume =   {43},
  number =   {2},
  pages =    {225-267}
}

@Article{ChaVen:1990:JPDC,
  author =   {S. Chandrasekaran and S. Venkatesan},
  title =    {{A Message-Optimal Algorithm for Distributed
                  Termination Detection}},
  journal =  JPDC,
  year =     {1990},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {245-252},
  month =    MAR,
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Charron-Bost:size,
  author =   {B. Charron-Bost},
  title =    {{Concerning the Size of Logical Clocks in Distributed Systems}},
  journal =  IPL,
  year =     1991,
  month =    JUL,
  volume =   {39},
  pages =    {11-16},
}

@InProceedings{Che:1993:WAD,
  author =   {J. Cheng},
  title =    {{Slicing Concurrent Programs---A Graph-Theoretical Approach}},
  booktitle =    PROC # " " # WAD,
  pages =    {223-240},
  year =     1993
}

@Article{ChoMil+:1991:TOPLAS,
  author =   {J. Choi and B. P. Miller and R. Netzer},
  title =    {{Techniques for Debugging Parallel Programs with Flowback Analysis}},
  journal =  TOPLAS,
  year =     1991,
  volume =   13,
  number =   4,
  pages =    {491-530},
  month =    OCT
}

@InProceedings{ClaEme:1981:WLP,
  author =   {E. M. Clarke and E. A. Emerson},
  title =    {{Design and Synthesis of Synchronization Skeletons using
                   Branching Time Temporal Logic}},
  booktitle =    PROC # " " # WLP,
  address =  {Yorktown Heights, New York},
  month =    MAY,
  series =   LNCS,
  volume =   131,
  year =     1981
}

@InProceedings{CohLeh:1982:PODC,
  author =   {S. Cohen and D. Lehmann},
  title =    {{Dynamic Systems and their Distributed Termination}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # PODC,
  pages =    {29-33},
  year =     {1982},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Ottawa},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ColDol:1994:IPL,
  author =   {Z. Collin and S. Dolev},
  title =    {{Self-Stabilizing Depth-First Search}},
  journal =      IPL,
  year =     1994,
  volume =   49,
  number =   6,
  pages =    {297-301}
}

@InProceedings{CooMar:1991:WPDD,
  author =   {R. Cooper and K. Marzullo},
  title =    {{Consistent Detection of Global Predicates}},
  booktitle =    PROC # " " # WPDD,
  pages =    {163-173},
  year =     1991,
  address =  {Santa Cruz, California}
}

@Book{CorLei+:1991:MIT,
  author =   {T. H. Cormen and C. E. Leiserson and R. L. Rivest},
  title =    {{Introduction to Algorithms}},
  publisher =    MIT,
  address =  {Cambridge, Massachusetts},
  year =     {1991},
}

@InProceedings{CowBea+:2001:USS,
  author =   {C. Cowan and S. Beattie and C. Wright and
                  G. Korah-Hartman},
  title =    {{RaceGuard: Kernel Protection from Temporary File
                   Race Vulnerabilities}},
  booktitle =    PROC # " 10th " # USS,
  pages =    {165-172},
  year =     2001,
  month =    AUG
}

@Book{CoxGoo:1994:PH,
  author =   {J. Cox and B. Goodheart},
  title =    {{The Magic Garden Explained: The Internals of Unix
                   System V Release 4: An Open Systems Design}},
  publisher =    PH,
  year =     1994
}

@InProceedings{CypLeu:1995:SPDP,
  author =   {R. Cypher and E. Leu},
  title =    {{Efficient Race Detection for Message-Passing
                   Programs with Nonblocking Sends and Receives}},
  booktitle =    PROC # " " # SPDP,
  pages =    {534-541},
  year =     1995
}

@Manual{DB2SQL:1999:IBM,
  title =    {DB2 UDB SQL Reference},
  organization = {IBM},
  edition =  {V6.1},
  year =     1999
}

@Article{DarMay:2003:JPDC,
  author =   {D. Darling and J. Mayo},
  title =    {{Stable Predicate Detection in Dynamic Systems}},
  journal =      "Submitted to the " # JPDC,
  OPTpages =     {},
  year =     {2003},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{Dav:1999:IBM,
  title =    {{DataLinks: Managing External Data with DB2
                   Universal Database}},
  organization = {IBM Corporation},
  month =    FEB,
  year =     {1999},
  note =     {White paper prepared by J. R. Davis}
}

@Book{DavPri:1990:CUP,
  author =   {B. A. Davey and H. A. Priestley},
  title =    {{Introduction to Lattices and Order}},
  publisher =    CUP,
  address =  {Cambridge, UK},
  year =     {1990},
}

@TechReport{DemAro:2000:TR:05,
  author =   {M. Demirbas and A. Arora},
  title =    {{An Optimal Termination Detection Algorithm for
                   Rings}},
  institution =  OSU,
  year =     2000,
  number =   {OSU-CISRC-2/00-TR05},
  month =    FEB
}

@Article{Den:1987:TSE,
  author =   {D. Denning},
  title =    {{An Intrusion Detection Model}},
  journal =  TSE,
  volume =   {13},
  number =   {2},
  month =    FEB,
  year =     {1987},
  pages =    {222-232}
}

@Article{DhaIye+:1997:PC,
  author =   {D. M. Dhamdhere and S. R. Iyer and E. K. K. Reddy},
  title =    {{Distributed Termination Detection for Dynamic Systems}},
  journal =      PC,
  year =     {1997},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {2025-2045},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dij:1965:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Solution of a Problem in Concurrent Programming
                   Control}},
  journal =  CACM,
  pages =    569,
  year =     1965,
  volume =   8,
  number =   9,
  organization = {ACM}
}

@Article{Dij:1971:ACTA,
  author =   {E. W. Dijkstra},
  title =    {{Hierarchical Ordering of Sequential Processes}},
  journal =      ACTA,
  year =     1971,
  volume =   1,
  number =   2,
  pages =    {115-138},
  month =    OCT
}

@Article{Dij:1974:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Self-Stabilizing Systems in spite of Distributed Control}},
  journal =  CACM,
  year =     {1974},
  volume =   {17},
  number =   {11},
  pages =    {643-644}
}

@InCollection{Dij:1985:SV,
  author =   {E. W. Dijsktra},
  title =    {{The Distributed Snapshot of K. M. Chandy and L. Lamport}},
  booktitle =    {Control Flow and Data Flow: Concepts of Distributed
                  Programming},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    SV,
  year =     {1985},
  editor =   {M. Broy},
  volume =   {F14},
  OPTnumber =    {},
  series =   {NATO ASI},
  OPTtype =  {},
  OPTchapter =   {},
  address =  {New York, NY},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Dij:1986:DC,
  author =   {E. W. Dijkstra},
  title =    {{A Belated Proof of Self-Stabilization}},
  journal =  DC,
  year =     {1986},
  volume =   {1},
  pages =    {5-6}
}

@Article{DijFei+:1983:IPL,
  author =   {E. W. Dijkstra and W. H. J. Feijen and A. J. M. van
                  Gasteren},
  title =    {{Derivation of a Termination Detection Algorithm for
                   Distributed Computations}},
  journal =  IPL,
  volume =   {16},
  pages =    {217-219},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1983},
  OPTannote =    {}
}

@Article{DijSch:1980:IPL,
  author =   {E. W. Dijkstra and C. S. Scholten},
  title =    {{Termination Detection for Diffusing Computations}},
  journal =  IPL,
  year =     1980,
  volume =   11,
  number =   1,
  pages =    {1-4}
}

@Article{Dil:1950:AM,
  author =   {R. P. Dilworth},
  title =    {{A Decomposition Theorem for Partially Ordered Sets}},
  journal =  AM,
  year =     1950,
  volume =   51,
  pages =    {161-166}
}

@Article{DolIsr+:1993:DC,
  author =   {S. Dolev and A. Israeli and S. Moran},
  title =    {{Self-Stabilization of Dynamic Systems Assuming Only Read/Write Atomicity}},
  journal =      DC,
  year =     1993,
  volume =   7,
  number =   1,
  pages =    {3-16}
}

@InProceedings{DueGup+:1992:WLCPC,
  author =   {E. Duesterwald and R. Gupta and M. L. Soffa},
  title =    {{Distributed Slicing and Partial Re-execution for Distributed Programs}},
  booktitle =    PROC # " 5th " # WLCPC,
  pages =    {329-337},
  year =     1992
}

@Article{DusMil:1941:AJM,
  author =   {B. Dushnik and E. W. Miller},
  title =    {{Partially Ordered Sets}},
  journal =  AJM,
  year =     1941,
  volume =   63,
  pages =    {600-610}
}

@PhdThesis{Ell:1995:PhD,
  author =   {G. Ellis},
  title =    {{Managing Complex Objects}},
  school =   {University of Queensland},
  year =     1995
}

@Article{ElnAlv+:2002:CS,
  author =   {E. N. Elnozahy and L. Alvisi and Y.-M. Wang and
                  D. B. Johnson},
  title =    {{A Survey of Rollback-Recovery Protocols in
                   Message-Passing Systems}},
  journal =  CS,
  volume =   {34},
  number =   {3},
  year =     {2002},
  pages =    {373-408},
}

@Article{FelHab+:1994:SIAMJDM,
  author =   {S. Felsner and M. Habib and R. H. M{\"o}hring},
  title =    {{On the Interplay of Interval Dimension and Dimension}},
  journal =  SIAMJDM,
  volume =   7,
  pages =    {32-40},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/Idim-dim.ps.gz},
}

@Article{FelTro:1994:DM,
  author =   {S. Felsner and W. T. Trotter},
  title =    {{On the Fractional Dimension of Partially Ordered Sets}},
  journal =  DM,
  volume =   136,
  pages =    {101-117},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/fdim.ps.gz},
}

@Article{Fid:1991:Com,
  author =   {C. Fidge},
  title =    {{Logical Time in Distributed Computing Systems}},
  journal =  Com,
  year =     1991,
  volume =   24,
  number =   8,
  pages =    {28-33},
  month =    AUG
}

@InProceedings{FisLyn+:1979:FCS,
  author =   {M. J. Fischer and N. A. Lynch and  J. E. Burns and A. Borodin},
  title =    {{Resource Allocation with Immunity to Limited Process Failure
                   (preliminary report)}},
  booktitle =    PROC # " 20th " # FOCS,
  pages =    {234-254},
  year =     1979,
  month =    OCT
}

@Article{Fra:1980:TOPLAS,
  author =   {N. Francez},
  title =    {{Distributed Termination}},
  journal =  TOPLAS,
  year =     1980,
  volume =   2,
  number =   1,
  pages =    {42-55},
  month =    JAN
}

@InProceedings{FroRay+:1994:ICPP,
  author =   {E. Fromentin and M. Raynal and V. K. Garg and
                  A. I. Tomlinson},
  title =    {{On the Fly Testing of Regular Patterns in Distributed Computations}},
  booktitle =    PROC # " 23rd " # ICPP,
  pages =    {73-76},
  year =     1994,
  number =   2,
  address =  {Chicago, Illinois},
  month =    AUG
}

@InProceedings{FroRay:1994:SPDP,
  author =   {E. Fromentin and M. Raynal},
  title =    {{Inevitable Global States: A Concept to Detect
                   Unstable Properties of Distributed Computations in
                   an Observer Independent Way}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {242-248},
  year =     {1994},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}

@Misc{GDB,
  OPTkey =   {},
  OPTauthor =    {},
  title =    {{GDB: The GNU Project Debugger}},
  OPThowpublished = {},
  OPTmonth =     {},
  OPTyear =      {},
  note =     {Available at
                  \texttt{http://www.gnu.org/software/gdb/gdb.html}},
  OPTannote =    {}
}

@TechReport{Gae:2003:TR:38,
  author =   {F. C. G{\"a}rtner},
  title =    {{A Survey of Self-Stabilizing Spanning-Tree Construction Algorithms}},
  institution =  SCCS # ", " # EPFL,
  address =      {Lausanne, Switzerland},
  year =     2003,
  number =   {IC 2003/38}
}

@InProceedings{GaeKlo:2000:SRDS,
  author =   {F. C. G{\"a}rtner and S. Kloppenburg},
  title =    {{Consistent Detection of Global Predicates under a Weak Fault Assumption}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # ", " # SRDS,
  pages =    {94-103},
  year =     {2000},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {N{\"u}rnberg, Germany},
  month =    OCT,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{GaePle:2001:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in
                  Crash-Affected Systems using
                  Interrupt-Style Failure Detectors (Brief Announcement)}},
  booktitle =    PROC # " " # DISC,
  year =     2001,
  address =  {Lisbon, Portugal},
  month =    {October}
}
@TechReport{GaePle:2001:TR,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  institution =  IBMZ,
  year =     2001,
  number =   {RZ 3361 (\# 93407)},
  month =    AUG
}
@InProceedings{GaePle:2001:WSS,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  booktitle =    PROC # " 5th " # WSS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {98-113},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS # " 2194",
  address =  {Lisbon, Portugal},
  month =    {October},
  OPTorganization ={},
  publisher =    SV,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GaePle:2002:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{Failure Detection Sequencers: Necessary and Sufficient
                  Information about Failures to Solve Predicate Detection}},
  booktitle =    PROC # " 16th " #  DISC,
  pages =    {280-294},
  year =     2002,
  number =   2508,
  series =   LNCS,
  publisher =    SV
}
@InProceedings{GamNes+:1987:ICALP,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{Posets, Boolean Representations and Quick
                   Path Searching}},
  booktitle =    PROC # " 14th " # ICALP,
  year =     1987,
  pages =    {404-424},
  number =   267,
  series =   LNCS
}
@Article{GamNes+:1990:TCS,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{On Locally Presented Posets}},
  journal =  TCS,
  year =     {1990},
  OPTkey =   {},
  volume =   {70},
  number =   {2},
  pages =    {251-260},
  month =    JAN,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{Gar:1996:ICSKE,
  author =   {V. K. Garg},
  title =    {{Observation of Global Properties in Distributed Systems}},
  booktitle =    ICSKE,
  pages =    {418-425},
  year =     1996,
  address =  {Lake Tahoe, Nevada},
  month =    JUN
}
@Book{Gar:1996:KAP,
  author =   {V. K. Garg},
  OPTeditor =    {~},
  title =    {{Principle of Distributed Systems}},
  publisher =    KAP,
  year =     1996
}
@InProceedings{Gar:1997:WAD,
  author =   {V. K. Garg},
  title =    {{Observation and Control for Debugging
                   Distributed Computations}},
  booktitle =    PROC # " " # WAD,
  pages =    {1-12},
  year =     1997,
  address =  {Link{\"o}ping, Sweden},
  note =     {Keynote Presentation}
}
@Book{Gar:2002:Book,
  author =   {V. K. Garg},
  title =    {{Elements of Distributed Computing}},
  publisher =    JWSUS,
  address =  {New York, NY},
  year =     {2002},
}
@InProceedings{Gar:2002:FSTTCS,
  author =   {V. K. Garg},
  title =    {{Algorithmic Combinatorics based on Slicing Posets}},
  booktitle =    PROC # " 22nd " # FSTTCS,
  year =     2002,
  address =  {Kanpur, India},
  month =    {December}
}
@Article{GarBar:1985:ACM,
  author =   {H. Garcia-Molina and D. Barbar},
  title =    {{How to Assign Votes in a Distributed System}},
  journal =  JACM,
  year =     {1985},
  volume =   {32},
  number =   {4},
  pages =    {841-860},
  month =    OCT
}
@InProceedings{GarCha+:1995:CSS,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Detecting Conjunctive Channel Predicates in
                   a Distributed Programming Environment}},
  booktitle =    PROC # " " # CSS,
  pages =    {232-241},
  year =     1995,
  volume =   2,
  address =  {Maui, Hawaii},
  month =    JAN
}
@Article{GarCha+:1997:JPDC,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Efficient Detection of Channel Predicates in
                   Distributed Systems}},
  journal =  JPDC,
  year =     {1997},
  volume =   {45},
  number =   {2},
  pages =    {134-147},
  month =    SEP
}
@InProceedings{GarCha:1995:ICDCS,
  author =   {V. K. Garg and C. Chase},
  title =    {{Distributed Algorithms for Detecting
                   Conjunctive Predicates}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {423-430},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@Book{GarJoh:1991:Fre,
  author =   {M. R. Garey and D. S. Johnson},
  OPTeditor =    {Victor Klee},
  title =    {{Computer and Intractability: A Guide to the
                   Theory of \mbox{NP-Completeness}}},
  publisher =    Fre,
  year =     1991
}
@InProceedings{GarLun:1991:NCSC,
  author =   {T. D. Garvey and T. F. Lunt},
  title =    {{Model-Based Intrusion Detection}},
  booktitle =    PROC # " 14th " # NCSC,
  pages =    {372-385},
  year =     1991
}
@Article{GarMit+:2003:SIGACT,
  author =   {V. K. Garg and N. Mittal and A. Sen},
  title =    {{Applications of Lattice Theory to Distributed
                  Computing}},
  journal =  SIGACT # " News Distributed Computing Column",
  year =     2003,
  OPTpublisher = {ACM Press},
  editor =   {Sergio Rajsbaum},
  volume =   34,
  number =   3,
  pages =    {40-61},
  month =    SEP
}
@InProceedings{GarMit:1998:FSTTCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Implementable Failure Detectors in
                   Asynchronous Systems}},
  booktitle =    PROC # " " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {158-169},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =  {Chennai, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GarMit:1998:ICDCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Distributed Predicate Detection in a Faulty
                   Environment}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {416-423},
  year =     {1998},
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}
@InProceedings{GarMit:2001:ICDCS,
  author =   {V. K. Garg and N. Mittal},
  title =    {{On Slicing a Distributed Computation}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {322-329},
  year =     2001,
  address =  {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@InProceedings{GarSka:2001:PODC,
  author =   {V. K. Garg and C. Skawratananond},
  title =    {{String Realizers of Posets with Applications
                   to Distributed Computing}},
  booktitle =    PROC # " 20th " # PODC,
  year =     2001,
  address =  {Newport, Rhode Island},
  month =    AUG,
  pages =    {72-80}
}
@InProceedings{GarTom+:1995:SPDP,
  author =   {V. K. Garg and A. I. Tomlinson and E. Fromentin and
                  Michel Raynal},
  title =    {{E}xpressing and {D}etecting {G}eneral {C}ontrol
                  {F}low {P}roperties of {D}istributed {C}omputations},
  booktitle =    PROC # " 7th " # SPDP,
  pages =    {432-438},
  year =     1995,
  address =  {San Antonio, Texas},
  month =    OCT
}
@InProceedings{GarWal:1991:WPDD,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  month =    MAY,
  year =     {1991},
  OPTorganization ={ACM/ONR},
}
@InProceedings{GarWal:1992:FSTTCS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates in
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 12th " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {253-264},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS,
  address =  {New Delhi, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@Article{GarWal:1994:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Weak Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1994,
  volume =   5,
  number =   3,
  pages =    {299-307},
  month =    MAR
}
@Article{GarWal:1996:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Strong Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1996,
  volume =   7,
  number =   12,
  pages =    {1323-1333},
  month =    DEC
}
@Article{GhoGup+:1996:JCI,
  author =   {S. Ghosh and A. Gupta and S. V. Pemmaraju},
  title =    {{A Fault-containing Self-stabilizing Spanning Tree Algorithm}},
  journal =      JCI,
  year =     1996,
  volume =   2,
  number =   1,
  pages =    {322-328}
}
@Book{God:1996:SV,
  author =   {P. Godefroid},
  ALTeditor =    {},
  title =    {{P}artial-{O}rder {M}ethods for the {V}erification of
                  {C}oncurrent {S}ystems},
  publisher =    SV,
  year =     {1996},
  volume =   {1032},
  series =   {Lecture Notes in Computer Science}
}
@Book{GodCox:1993:PH,
  author =   {B. Goodheart and J. Cox},
  title =    {The Magic Garden Explained: The Internals of Unix
                  System V Release 4},
  publisher =    PH,
  year =     {1993}
}
@Misc{GoySit+:2003:SCISS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{A Partial Order Approach to Detect Race Condition Attacks}},
  howpublished = "Abstract published in " # SCISS ,
  month =    APR,
  year =     2003
}
@TechReport{GoySit+:2003:TR:03,
  author =       {B. Goyal and S. Sitaraman and S. Venkatesan},
  title =        {{A Unified Approach to Detect Binding Based Race Condition Attacks}},
  number =       {UTDCS-02-03},
  year =         2003,
  institution =  DCS # ", " # UTD # ", " # "\textsf{http://www.utdallas.edu/{\textasciitilde}venky/publications/race.pdf}"
}
@InProceedings{GoySri+:2003:TWSIS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{Methods To Tackle Vulnerabilities Caused by Lack of Mutual Exclusion}},
  booktitle =    PROC # " " # TWSIS,
  year =     2003,
  pages =        {17-21},
  address =      {College Station, Texas},
  month =    APR
}
@Book{GraReu:1993:MK,
  author =   {J. Gray and A. Reuter},
  title =    {Transaction Processing: Concepts and Techniques},
  publisher =    MK,
  year =     {1993}
}
@InProceedings{GraVol:1993:MVPP,
  author =   {S. Grabner and J. Volkert},
  title =    {{Debugging Parallel Programs Using Event Graph Manipulation}},
  booktitle =    PROC # " " # MVPP,
  pages =    {443-450},
  year =     1993,
  month =    OCT
}
@Book{Gratzer,
  author =       {G. Gratzer},
  title =        {{General Lattice Theory}},
  publisher =    {Academic Press},
  address =      {New York, NY},
  year =         1978
}
@InProceedings{HabHuc+:1995:KRUSE,
  author =   {M. Habib and M. Huchard and L. Nourine},
  title =    {{Embedding Partially Ordered Sets into Chain-Products}},
  booktitle =    PROC # " " # KRUSE,
  pages =    {147-161},
  year =     1995,
  address =      {University of California, Santa Cruz},
  month =    AUG
}
@InProceedings{HabNou:1994:ORDAL,
  author =   {M. Habib and L. Nourine},
  title =    {{Bit-Vector Encoding for Partially Ordered Sets}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {1-12},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =      {Lyon, France},
  month =    JUL,
  publisher = SV
}

@inproceedings{KuznetsovRavi:ConcurrencyTM:OPODIS:2011,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  booktitle = {OPODIS},
  year      = {2011},
  pages     = {112-127},
  ee        = {http://dx.doi.org/10.1007/978-3-642-25873-2_9}
}


@InProceedings{Had:2001:PODC,
  author =   {V. Hadzilacos},
  title =    {{A Note on Group Mutual Exclusion}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 20th " # PODC,
  OPTpages =     {},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    AUG,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Hadzilacos:1988:JACM,
 author = {Hadzilacos, Vassos},
 title = {A theory of reliability in database systems},
 journal = {J. ACM},
 issue_date = {Jan. 1988},
 volume = {35},
 number = {1},
 month = jan,
 year = {1988},
 issn = {0004-5411},
 pages = {121--145},
 numpages = {25}
} 


@InProceedings{HelJar+:1987:PODC,
  author =       {J.-M. H{\'e}lary and C. Jard and N. Plouzeau and M. Raynal},
  title =        {{Detection of Stable Properties in Distributed Applications}},
  booktitle =    PROC # " " # PODC,
  pages =        {125-136},
  year =         {1987}
}
@article{HelRay:1994:DC,

  author =       {J.-M. H{\'e}lary and M. Raynal},
  title =        {{Towards the Construction of Distributed Detection Programs, with
                   an Application to Distributed Termination}},
  journal =      DC,
  volume =       {7},
  number =       {3},
  pages =        {137-147},
  year =         "1994"
}
@Article{Hir:1951:SRKU,
  author =   {T. Hiraguchi},
  title =    {{On the Dimension of Partially Ordered Sets}},
  journal =      SRKU,
  year =     1951,
  volume =   1,
  pages =    {77-94}
}
@Article{Hir:1955:SRKU,
  author =   {T. Hiraguchi},
  title =    {{O}n the {D}imension of {O}rders},
  journal =      SRKU,
  year =     1955,
  volume =   4,
  pages =    {1-20}
}
@Article{HoRam:1982:TSE,
  author =   {G. S. Ho and C. V. Ramamoorthy},
  title =    {{Protocols for Deadlock Detection in Distributed Database Systems}},
  journal =      TSE,
  year =     {1982},
  OPTkey =   {},
  volume =   {8},
  number =   {6},
  pages =    {554-557},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hol:1997:TSE,
  author =   {G. Holzmann},
  title =    {{The Model Checker SPIN}},
  journal =      TSE,
  year =     1997,
  OPTkey =   {},
  volume =   23,
  number =   5,
  pages =    {279-295},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{HsiMit:2000:TC,
  author =   {H. Hsiao and N. Mittal},
  title =    {{Database Managed External File Update}},
  institution =  IBMARC,
  year =     2000,
  number =   {RJ10183},
  address =  {San Jose, California, 95120}
}
@Manual{HsiNar:1999:IBMARC,
  author =   {H. Hsiao and I. Narang},
  title =    {{Update In-Place Support with DataLinks}},
  organization = IBMARC,
  year =     {1999},
  note =     {Internal Document}
}
@InProceedings{HsiNar:2000:SIGMOD,
  author =   {H. Hsiao and I. Narang},
  title =    {{DLFM: A Transactional Resource Manager}},
  booktitle =    PROC # " 19th " # SIGMOD,
  pages =    {518-528},
  year =     2000,
  address =  {Dallas, Texas},
  month =    MAY
}
@InProceedings{Hua:1989:ICDCS,
  author =   {S.-T. Huang},
  title =    {{Detecting Termination of Distributed Computations by External Agents}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {79-84},
  year =     {1989},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hua:1989:IPL,
  author =   {S.-T. Huang},
  title =    {{Termination Detection by using Distributed Snapshots}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {32},
  OPTnumber =    {},
  pages =    {113-119},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{HuaChe:1992:IPL,
  author =   {S.-T. Huang and N.-S. Chen},
  title =    {{A Self-Stabilizing Algorithm for Constructing Breadth-First Trees}},
  journal =      IPL,
  year =     1992,
  volume =   41,
  number =   2,
  pages =    {109-117},
  month =    FEB
}
@InProceedings{HuaKin:1993:FTCS,
  author =   {Y. Huang and C. Kintala},
  title =    {{S}oftware {I}mplemented {F}ault {T}olerance:
                  {T}echnologies and {E}xperience},
  booktitle =    PROC # " " # FTCS,
  pages =    {138-144},
  year =     1993,
  month =    JUN
}
@InProceedings{HurMiz+:1996:SPDP,
  author =   {M. Hurfin and M. Mizuno and M. Raynal and
                  M. Singhal},
  title =    {{Efficient Distributed Detection of Conjunctions of Local Predicates in
                   Asynchronous Computations}},
  booktitle =    PROC # " 8th " # SPDP,
  pages =    {588-594},
  year =     1996,
  address =  {New Orleans},
  month =    OCT
}
@Article{HurPlo+:1993:JCC,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{A Debugging Tool for Distributed Estelle Programs}},
  journal =  JCC,
  year =     1993,
  volume =   16,
  number =   5,
  pages =    {328-333},
  month =    MAY
}
@InProceedings{HurPlo+:1993:WPDD,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{D}etecting {A}tomic {S}equences of {P}redicates in
                  {D}istributed {C}omputations},
  booktitle =    PROC # " " # WPDD,
  pages =    {32-42},
  year =     1993
}
@InProceedings{HurRay:1996:WGCS,
  author =   {M. Hurfin and M. Raynal},
  title =    {{D}etecting {D}iamond {N}ecklaces in {L}abeled {D}ags
                  ({A} {P}roblem from {D}istributed  {D}ebugging},
  booktitle =    PROC # " " # WGCS,
  pages =    {211-223},
  year =     1996,
  series =   LNCS,
  publisher =    SV
}
@Manual{ISO:1993,
  author =       {ISO},
  title =        {{S}pecification of the {A}synchronous {T}ransfer {M}ode
                  {R}ing {(ATMR)} {P}rotocol},
  month =        JAN,
  year =         1993,
}
@InProceedings{JarJer+:1994:ICDCS,
  author =       {C. Jard and T. J{\'e}ron and G.-V. Jourdan and J.-X. Rampon},
  title =        {{A} {G}eneral {A}pproach to {T}race-{C}hecking in
                  {D}istributed {C}omputing {S}ystems},
  booktitle =    PROC # " " # ICDCS,
  pages =        {396-403},
  year =         {1994},
  url =          {http://citeseer.nj.nec.com/jard94general.html}
}
@InProceedings{JegMed+:1995:WSCT,
  author =   {R. Jegou and R. Medina and L. Nourine},
  title =    {{L}inear {S}pace {A}lgorithm for {O}n-line
                  {D}etection of {G}lobal {P}redicates},
  booktitle =    PROC # " " # WSCT,
  pages =        {175-189},
  year =     1995,
  editor =   {J. Desel},
  publisher =    SV
}
@InProceedings{JohZwa:1988:PODC,
  author =   {D. B. Johnson and W. Zwaenepoel},
  title =    {{R}ecovery in {D}istributed {S}ystems {U}sing
                  {O}ptimistic {M}essage {L}ogging and
                  {C}heckpointing},
  booktitle =    PROC # " 6th " # PODC,
  pages =    {171-181},
  year =     1988,
  month =    AUG
}
@Article{JohZwa:1990:JA,
  author =       {D. B. Johnson and W. Zwaenepoel},
  title =        {{R}ecovery in {D}istributed {S}ystems using {O}ptimistic {M}essage {L}ogging
                 and {C}heckpointing},
  journal =      JA,
  volume =       {11},
  number =       {3},
  month =        SEP,
  year =         {1990},
  pages =        {462-491},
}
@Article{Jou:2000:DC,
  author =       {Y.-J. Joung},
  title =        {{A}synchronous {G}roup {M}utual {E}xclusion},
  journal =      DC,
  volume =       {13},
  number =       {4},
  pages =        {189-206},
  year =         {2000},
}
@Article{Jou:2002:DC,
  author =       {Y.-J. Joung},
  title =        {{T}he {C}ongenial {T}alking {P}hilosophers {P}roblem in {C}omputer
                  {N}etworks},
  journal =       DC,
  pages =        {155-175},
  year =         {2002},
}
@Article{Jou:2003:TPDS,
  author =       {Y.-J. Joung},
  title =        {{Q}uorum-{B}ased {A}lgorithms for {G}roup {M}utual {E}xclusion},
  journal =      TPDS,
  pages =        {463-475},
  year =         {2003},
  volume =       {14},
  number =       {5},
  month =        MAY
}
@Article{KaeMoh:1978:SIAM,
  author =   {R. Kaerkes and R. H. M{\"o}hring},
  title =    {{V}orlesungen u{\"b}er {O}rdnungen und {N}etzplantheorie},
  journal =      {Schriften zur Informatik und Angewandten Mathematik 45, RWTH Aachen},
  year =     1978
}
@InProceedings{KanNao+:1988:STOC,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  booktitle =    PROC # " 20th " # STOC,
  pages =    {334-343},
  year =     1988,
  address =      {Chicago},
  month =    MAY
}
@Article{KanNao+:1992:SIAMJDM,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  journal =      SIAMJDM,
  year =     1992,
  volume =   5,
  number =   4,
  pages =    {596-603},
  month =    NOV
}
@InProceedings{KanWil+:2003:ICDCS,
  author =   {B. B. H. Kang and R. Wilensky and J, Kubiatowicz},
  title =    {{The Hash History Approach for Reconciling Mutual Inconsistency}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {670-677},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Providence, Rhode Island},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KeaMoi:1999:PODC,
  author =   {P. Keane and M. Moir},
  title =    {{A} {S}imple {L}ocal-{S}pin {G}roup {M}utual {E}xclusion {A}lgorithm},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PODC,
  pages =    {23-32},
  year =     {1999},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{KhoHam+:2003:JPDC,
  author =   {A. A. Khokhar and S. E. Hambrusch and E. Kocalar},
  title =    {{Termination Detection in Data-Driven Parallel Computations/Applications}},
  journal =      JPDC,
  year =     2003,
  volume =   63,
  number =   3,
  pages =    {312-326},
  month =    MAR
}
@Article{KilCha:1997:CJ,
  author =   {R. Kilgore and C. Chase},
  title =    {{T}esting {D}istributed {P}rograms {C}ontaining
                  {R}acing {M}essages},
  journal =  CJ,
  year =     1997,
  volume =   40,
  number =   8,
  pages =    {489-498},
  month =    NOV
}
@InProceedings{KilCha:1997:CSS,
  author =   {R. Kilgore and C. Chase},
  title =    {{R}e-execution of {D}istributed {P}rograms to
                  {D}etect {B}ugs {H}idden by {R}acing {M}essages},
  booktitle =    PROC # " " # CSS,
  pages =        {423-432},
  year =     1997,
  address =  {Hawaii},
  month =    JAN
}
@PhdThesis{KoChe:1996:Thesis,
  author =       {C. Ko and W. Cheuk},
  title =        {{Execution Monitoring Of Security Critical Programs in a Distributed
                   System: A Specification Based Approach}},
  year =         1996,
  school =       UCD
},
  month =        {August},
  year =         1997
}
@InProceedings{KoRed:2002:SP,
  author =   {C. Ko and T. Redmond},
  title =    {{Noninterference and Intrusion Detection}},
  year =     2002,
  booktitle =    PROC # " " # SP,
  pages =        {177-187},
  address =      {Berkeley, California},
  month =    MAY
}
@InProceedings{KocKho+:1999:PDC,
  author =   {E. Kocalar and A. A. Khokhar and S. E. Hambrusch},
  title =    {{T}ermination {D}etection: {M}odels and {A}lgorithms for {SPMD}
                  {C}omputing {P}aradigms},
  booktitle =    PROC # " " # PDC,
  year =     1999
}
@Book{Koh:1978:MH,
  author =   {Z. Kohavi},
  OPTeditor =    {~},
  title =    {{S}witching and {F}inite {A}utomata {T}heory},
  publisher =    MH,
  year =     1978,
  edition =  {2nd}
}
@Misc{KohGei:1995,
  OPTkey =   {},
  author =   {J. A. Kohl and G. A. Geist},
  title =    {{T}he {PVM 3.4} {T}racing {F}acility and {XPVM 1.1}},
  howpublished = {Computer Science and Mathematics Divison, Oak Ridge National Laboratory, TN, USA},
  OPTmonth =     {},
  year =     {1995},
  note =     {},
  OPTannote =    {}
}
@Article{KorFer:1992:AMCSJ,
  author =   {B. Korel and R. Ferguson},
  title =    {{Dynamic Slicing of Distributed Programs}},
  journal =  AMCSJ,
  year =     1992,
  volume =   2,
  number =   2,
  pages =    {199-215}
}
@Article{KorLas:1988:IPL,
  author =   {B. Korel and J. Laski},
  title =    {{Dynamic Program Slicing}},
  journal =  IPL,
  year =     1988,
  volume =   29,
  number =   3,
  pages =    {155-163}
}
@InProceedings{KorRil:1997:WAD,
  author =   {B. Korel and J. Rilling},
  title =    {{Application of Dynamic Slicing in Program Debugging}},
  booktitle =    PROC # " 3rd " # WAD,
  pages =    {43-57},
  year =     1997,
  editor =   {Mariam Kamkar},
  address =  {Link{\" o}ping, Sweden},
  month =    MAY
}
@Article{Ksh:1998:TCS,
  author =   {A. D. Kshemkalyani},
  title =    {{A Framework for Viewing Atomic Events in Distributed Computations}},
  journal =      TCS,
  year =     {1998},
  OPTkey =   {},
  volume =   {196},
  number =   {1-2},
  pages =    {45-70},
  month =    APR,
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KshSin:1990:SPDP,
  author =       {A. D. Kshemkalyani and M. Singhal},
  title =        {{Correct Two-phase and One-phase Deadlock Detection
                   Algorithms for Distributed Systems}},
  booktitle =    PROC # " " # SPDP,
  pages =        {126-129},
  month =        DEC,
  year =         {1990}
}
@Article{KunBla+:1997:CJ,
  author =   {T. Kunz and J. P. Black and D. J. Taylor and T. Basten},
  title =    {{POET}: {T}arget-{S}ystem {I}ndependent {V}isualizations of {C}omplex
                  {D}istributed-{A}pplications {E}xecutions},
  journal =      CJ,
  year =     {1997},
  OPTkey =   {},
  volume =   {40},
  number =   {8},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lai:1986:JPDC,
  author =   {T. H. Lai},
  title =    {{Termination Detection for Dynamic Distributed Systems with
                  Non-First-In-First-Out Communication}},
  journal =      JPDC,
  year =     {1986},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {577-599},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{LaiTse+:1992:IPPS,
  author =       {T.-H. Lai and Y.-C. Tseng and X. Dong},
  title =        {{A More Efficient Message-Optimal Algorithm for
                  Distributed Termination Detection}},
  booktitle =    PROC # " 6th " # IPPS,
  year =         {1992},
  pages =        {646--649},
  publisher = {IEEE Computer Society},
}
@Article{LaiWu:1995:TPDS,
  author =   {T.-H. Lai and L.-F. Wu},
  title =    {{An $(N -1)$-Resilient Algorithm for Distributed Termination Detection}},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   1,
  pages =    {63-78}
}
@Article{LaiYan:1987:IPL,
  author =   {T.-H. Lai and T. H. Yang},
  title =    {{On Distributed Snapshots}},
  journal =      IPL,
  year =     {1987},
  OPTkey =   {},
  volume =   {25},
  number =   {3},
  pages =    {153-158},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1974:CACM,
  author =   {L. Lamport},
  title =    {{A New Solution of Dijkstra's Concurrent Programming Problem}},
  journal =      CACM,
  year =     {1974},
  OPTkey =   {},
  volume =   {18},
  number =   {8},
  pages =    {453-455},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1978:CACM,
  author =   {L. Lamport},
  title =    {{T}ime, {C}locks, and the {O}rdering of {E}vents in
                  a {D}istributed {S}ystem},
  journal =  CACM,
  year =     1978,
  volume =   21,
  number =   7,
  pages =    {558-565},
  month =    JUL
}
@Article{LanBul+:1994:CS,
  author =   {C. E. Landwehr and A. R. Bull and J. P. McDermott and W. S. Choi},
  title =    {{A} {T}axonomy of {C}omputer {P}rogram {S}ecurity {F}laws},
  journal =      CS,
  year =     1994,
  volume =   26,
  number =   3,
  pages =    {211-254},
  issn =         {0360-0300}
}
@Article{Law:1976:MCT,
  author =   {E. L. Lawler},
  title =    {{G}raphical {A}lgorithms and their {C}omplexity},
  journal =      MCT,
  year =     1976,
  volume =   81,
  pages =    {3-32}
}
@Article{LebMel:1987:TC,
  author =   {T. J. LeBlanc and J. M. Mellor-Crummey},
  title =    {{D}ebugging {P}rograms with {I}nstant {R}eplay},
  journal =  TC,
  year =     1987,
  volume =   {C-36},
  number =   4,
  pages =    {471-482},
  month =    APR
}
@Article{MadWes:1991:DM,
  author =   {T. Madej and D. B. West},
  title =    {{T}he {I}nterval {I}nclusion {N}umber of a {P}artially {O}rdered {S}et},
  journal =      DM,
  year =     1991,
  volume =   88,
  pages =    {259-277},
  note =     ES
}
@Article{Mae:1985:TrCS,
  author =       {M. Maekawa},
  title =        {{A}lgorithm for {M}utual {E}xclusion in {D}ecentralized {S}ystem},
  journal =      TrCS,
  pages =        {145-159},
  year =         {1985},
  volume =       {3},
  number =       {2},
  month =        MAY,
  OPTorganization = {ACM}
}
@Book{Mae:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  OPTeditor =    {},
  title =    {{Operating Systems Advanced Concepts}},
  publisher =    BCPC,
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Menlo Park, California},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{MaeOld+:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  title =    {{O}perating {S}ystems {A}dvanced {C}oncepts},
  publisher =    BCPC,
  year =     1987,
  address =      {Menlo Park, California}
}
@Article{MagWel+:1981:TCS,
  author =   {A. Maggiolo-Schettini and H. Welde and J. Winkowski},
  title =    {{M}odeling a {S}olution for a {C}ontrol {P}roblem in
                  {D}istributed {S}ystems by {R}estrictions},
  journal =  TCS,
  year =     1981,
  volume =   13,
  number =   1,
  pages =    {61-83},
  month =    JAN
}
@Unpublished{MahDut:2004:JPDC,
  author =   {N. R. Mahapatra and S. Dutt},
  title =    {{An Efficient Delay-Optimal Distributed Termination Detection Algorithm}},
  note =     "To Appear in " # JPDC,
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2004},
  OPTannote =    {}
}
@Misc{Man:Rdist,
   title =      {{Man pages: Rdist - Remote File Distribution Program}},
   organization = {Sun Microsystems}
}
@article{ManIma:1992:JPDC,
  author =       {Y. Manabe and M. Imase},
  title =        {{G}lobal {C}onditions in {D}ebugging {D}istributed {P}rograms},
  journal =      JPDC,
  volume =       {15},
  number =       {1},
  pages =        {62-69},
  year =         {1992}
}
@InProceedings{MarNei:1991:WDAG,
  author =       {K. Marzullo and G. Neiger},
  title =        {{D}etection of {G}lobal {S}tate {P}redicates},
  booktitle =    PROC # " " # WDAG,
  pages =        {254-272},
  year =         {1991}
}
@Article{MarSab:1994:DC,
  author = {K. Marzullo and L. Sabel},
  title = {{E}fficient {D}etection of a {C}lass of {S}table {P}roperties},
  journal = DC,
  volume = {8},
  number = {2},
  pages = {81-91},
  year = {1994},
  url = "citeseer.nj.nec.com/marzullo94efficient.html"
}
@Article{Mat:1987:DC,
  author =   {F. Mattern},
  title =    {{Algorithms for Distributed Termination Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {161-175},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Mat:1989:IPL,
  author =   {F. Mattern},
  title =    {{Global Quiescence Detection based on Credit Distribution
                   and Recovery}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {195-200},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Mat:1989:WDAG,
  author =   {F. Mattern},
  title =    {{Virtual Time and Global States of Distributed Systems}},
  booktitle =    "Parallel and Distributed Algorithms: " # PROC # " "
                  # WDAG,
  pages =    {215-226},
  year =     1989,
  publisher =    ES
}
@Article{Mat:1993:JPDC,
  author =       {F. Mattern},
  title =        {{E}fficient {A}lgorithms for {D}istributed {S}napshots and {G}lobal
                  {V}irtual {T}ime {A}pproximation},
  journal =      JPDC,
  volume =       {18},
  number =       {4},
  pages =        {423-434},
  year =         {1993},
  url =          {http://citeseer.nj.nec.com/mattern93efficient.html}
}
@Article{MatCap:1999:JSS,
  author =   {J. Matocha and T. Camp},
  title =    {{A Taxonomy of Distributed Termination Detection Algorithms}},
  journal =      JSS,
  year =     1999,
  volume =   43,
  number =   3,
  pages =    {207-221},
  month =    NOV
}
@Techreport{MatMeh+:1991:TR:32,
  author =       {F. Mattern and H. Mehl and A. Schoone and G. Tel},
  title =        {{Global Virtual Time Approximation with Distributed
                  Termination Detection Algorithms}},
  institution =  {University of Utrecht, The Netherlands},
  number =       {RUU-CS-91-32},
  year =         {1991},
  url =          {http://citeseer.nj.nec.com/mattern91global.html}
}
@Manual{MatMel+:1997:ISO,
  author =   {N. Mattos and J. Melton and J. Richey},
  title =    {Database Language SQL - Part 9: Management of
                  External Data (SQL/MED)},
  organization = {ISO working draft},
  month =    JUN,
  year =     1997
}
@InProceedings{McMLi:1993:COMPSAC,
  author =   {P. Li and B. McMillin},
  title =    {{Fault-Tolerant Distributed Deadlock Detection/Resolution}},
  booktitle =    PROC # " 17th " # COMPSAC,
  pages =    {224-230},
  year =     1993,
  month =    NOV
}
@InProceedings{MilCho:1988:ICDCS,
  author =   {B. P. Miller and J. Choi},
  title =    {{B}reakpoints and {H}alting in {D}istributed
                  {P}rograms},
  booktitle =    PROC # " 8th " # ICDCS,
  pages =    {316-323},
  year =     1988
}
@InProceedings{Mis:1983:PODC,
  author =   {J. Misra},
  title =    {{Detecting Termination of Distributed Computations using Markers}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  pages =    {290-294},
  year =     {1983},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@PhdThesis{Mit:2002:Thesis,
  author =       {N. Mittal},
  title =        {{T}echniques for {A}nalyzing {D}istributed {C}omputations},
  school =       UTA,
  year =         2002,
  month =        MAY,
  note =         {Available at \texttt{http://www.utdallas.edu/{\symbol{126}}neerajm}}
}
@InProceedings{MitGar:1998:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  booktitle =    PROC # " 18th " # ICDCS,
  pages =    {582-589},
  year =     {1998},
  address =      {Amsterdam, The Netherlands},
  month =    MAY
}
@TechReport{MitGar:1998:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     1998,
  number =   {TR-PDS-1998-005},
  address =      {Austin, TX 78712}
}
@InProceedings{MitGar:2000:PODC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  booktitle =    PROC # " 19th " # PODC,
  pages =    {239-248},
  year =     2000,
  address =  {Portland, Oregon},
  month =    JUL
}
@TechReport{MitGar:2000:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2000,
  number =   {TR-PDS-2000-002},
  address =  {Austin, TX 78712},
  month =    MAY
}
@InProceedings{MitGar:2001:DISC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  booktitle =    PROC # " " # DISC,
  pages =    {78-92},
  year =     2001,
  address =      {Lisbon, Portugal},
  month =    OCT
}
@InProceedings{MitGar:2001:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{On Detecting Global Predicates in Distributed Computations}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {3-10},
  year =     2001,
  address =      {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at
                  \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@TechReport{MitGar:2001:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2001,
  number =   {TR-PDS-2001-002},
  OPTaddress =   {Austin, TX 78712},
  month =    APR,
  note =         {Available at \texttt{http://www.cs.utexas.edu/users/neerajm}}
}
@TechReport{MitGar:2001:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{A Rigorous Proof of $O(n^2)$ Bound on the Number of Moves
                  for Stabilization of Dijkstra's 3-State Algorithm}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2001-005},
  address =      {Austin, TX 78712},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitGar:2003:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Software Fault Tolerance of Distributed Programs using Computation Slicing}},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {105-113},
  year =     2003,
  address =  {Providence, Rhode Island},
  month =    MAY
}
@TechReport{MitGar:2003:TR:15,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Techniques and Applications of Computation Slicing}},
  institution =  DCS # ", " # UTD,
  year =     2003,
  number =   {UTDCS-15-03},
  OPTaddress =   {Richardson, TX 75083},
  month =    APR
}
@Article{MitGar:2004:DC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Finding Missing Synchronization in a Distributed Computation using
                  Controlled Re-execution}},
  journal =      DC,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  month =    MAR,
  note =     {Online First},
  OPTannote =    {}
}
@InProceedings{MitHsi:2000:ICDE,
  author =   {N. Mittal and H. Hsiao},
  title =    {{D}atabase {M}anaged {E}xternal {F}ile {U}pdate},
  booktitle =    PROC # " 17th " # ICDE,
  pages =    {557-564},
  year =     2001,
  address =  {Heidelberg, Germany},
  month =    APR
}
@InProceedings{MitSen+:2004:IPDPS,
  author =   {N. Mittal and A. Sen and V. K. Garg and R. Atreya},
  title =    {{Finding Satisfying Global States: All for One and One for All}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # IPDPS,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    APR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitVen+:2004:DISC,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  booktitle =    PROC # " " # DISC,
  pages =        {290-304},
  year =     2004,
  address =      {Amsterdam, The Netherlands},
  month =    OCT
}
@TechReport{MitVen+:2004:TR,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  institution =  UTD,
  number =       {UTDCS-08-04},
  month =        FEB,
  year =     2004,
  note =     {Available at
                  \texttt{http://www.utdallas.edu/{\textasciitilde}neerajm/}}
}
@InProceedings{MurGar:1997:ICDCS,
  author =   {V. V. Murty and V. K. Garg},
  title =    {{C}haracterization of {M}essage {O}rdering
                  {S}pecifications and {P}rotocols},
  booktitle =    PROC # " 17th " # ICDCS,
  year =     1997,
  month =    MAY
}
@Article{Nas:1961:JLMS,
  author =   {C. Nash-Williams},
  title =    {{E}dge-{D}isjoint {S}panning {T}rees of {F}inite {G}raphs},
  journal =      JLMS,
  year =     1961,
  volume =   36,
  pages =    {445-450}
}
@InProceedings{NetBre+:1996:SPDT,
  author =   {R. Netzer and T. Brennan and S. Damodaran-Kamal},
  title =    {{D}ebugging {R}ace {C}onditions in
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " " # SPDT,
  pages =    {31-40},
  year =     1996,
  month =    MAY
}
@Article{NetMil:1995:JS,
  author =   {R. H. B. Netzer and B. P. Miller},
  title =    {{O}ptimal {T}racing and {R}eplay for {D}ebugging
                  {M}essage-{P}assing {P}rograms},
  journal =  JS,
  year =     1995,
  volume =   8,
  number =   4,
  pages =    {371-388}
}
@Article{NetXu:1995:TPDS,
  author =   {R. H. B. Netzer and J. Xu},
  title =    {{N}ecessary and {S}ufficient {C}onditions for {C}onsistent
                  {G}lobal {S}napshots},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   2,
  pages =    {165-169},
  month =    FEB
}
@Unpublished{POTAwebsite,
  author =   {A. Sen and V. K. Garg},
  title =    {{P}artial {O}rder {T}race {A}nalyzer {(POTA)}},
  note =     {http://maple.ece.utexas.edu/{\textasciitilde}sen/POTA.html},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}
@Article{PapWas+:1999:SIGMOD,
  author =   {M. Papiani and J. Wason and A. Dunlop and D. Nicole},
  title =    {{A} {D}istributed {S}cientific {A}rchive {U}sing the
                  {W}eb, {XML} and {SQL}/{MED}},
  journal =  {SIGMOD Record},
  volume =   {28},
  number =   {3},
  pages =    {56-62},
  month =    SEP,
  year =     {1999}
}
@Article{ParPop+:1983:TSE,
  author =   {D. S. Parker and G. J. Popek and G. Rudisin and A. Stoughton
                  and B. J. Walker and E. Walton and J. M. Chow and D. A. Edwards
                  and S. Kiser and C. S. Kline},
  title =    {{Detection of Mutual Inconsistency in Distributed Systems}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {240-247},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PerMit:2004:PDCS,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  booktitle =    PROC # " " # PDCS,
  pages =        {209-215},
  year =     2004,
  address =      {San Francisco, California},
  month =    SEP
}
@TechReport{PerMit:2004:TR,
  author =   {S. Peri and N. Mittal},
  title =    {{An Efficient Snapshot Protocol for a Dynamic System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{PerMit:2004:TR:15,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-15-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PlaBec+:1995:UWTC,
  author =   {J. S. Plank and M. Beck and G. Kingsley},
  title =    {{Libckpt: Transparent Checkpointing under UNIX}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # UWTC,
  pages =    {213-223},
  year =     {1995},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New Orleans, Louisiana},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Misc{Pom:2000:TUT,
  OPTkey =   {},
  author =   {W. Torres-Pomales},
  title =    {{S}oftware {F}ault {T}olerance: {A} {T}utorial},
  OPThowpublished = {},
  OPTmonth =     {},
  year =     {2000},
  note =     {NASA Langley Research Center},
  OPTannote =    {}
}
@InProceedings{PraSin:1994:SPDP,
  author =   {R. Prakash and M. Singhal},
  title =    {{Maximal Global Snapshot with Concurrent Initiators}},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {344-351},
  year =     1994,
  address =      {Dallas, Texas},
  month =    OCT
}
@InProceedings{QueSif:1982:ISP,
  author =       {J. P. Queille and J. Sifakis},
  title =        {{S}pecification and {V}erification of {C}oncurrent {S}ystems in {CESAR}},
  address =      {New York},
  booktitle =    PROC # " 5th " # ISP,
  pages =        {337-351},
  publisher =    SV,
  series =       LNCS,
  volume =       137,
  year =         1982
}
@Article{Ran:1983:IPL,
  author =   {S. P. Rana},
  title =    {{A Distributed Solution of the Distributed Termination
                   Problem}},
  journal =      IPL,
  year =     {1983},
  OPTkey =   {},
  volume =   {17},
  number =   {1},
  pages =    {43-46},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{RaoAlv+:2000:KDE,
  author =       {S. Rao and L. Alvisi and H. Vin},
  title =        {{T}he {C}ost of {R}ecovery in {M}essage {L}ogging {P}rotocols},
  journal =      KDE,
  volume =       {12},
  number =       {2},
  year =         {2000},
  pages =        {160-173},
}
@Book{Ray:1988:JWS,
  author =       {M. Raynal},
  title =        {{D}istributed {A}lgorithms and {P}rotocols},
  publisher =    JWS,
  year =         {1988}
}
@Article{Ray:1989:TrCS,
  author =   {K. Raymond},
  title =    {{A} {T}ree based {A}lgorithm for {D}istributed {M}utual {E}xclusion},
  journal =      TrCS,
  year =     1989,
  volume =   7,
  number =   1,
  pages =    {61-77}
}
@Article{RicAgr:1981:CACM,
  author =       {G. Ricart and A. K. Agrawala},
  title =        {{An Optimal Algorithm for Mutual Exclusion in Computer Networks}},
  journal =      CACM,
  volume =       {24},
  number =       {1},
  year =         {1981},
  pages =        {9-17},
  publisher =    {ACM Press},
  month =        JAN,
}
@Article{Riv:1974:AMS,
  author =   {I. Rival},
  title =    {{M}aximal {S}ublattices of {F}inite {D}istributive {L}attices {II}},
  journal =      PROC # " " # AMS,
  year =     1974,
  volume =   44,
  number =   2,
  pages =    {263-268}
}
@Book{STA,
  author =       {R. Stanley},
  title =        {{E}numerative {C}ombinatorics {V}olume 1},
  publisher =    {Wadsworth and Brookes/Cole},
  address =      {Monterey, California},
  year =         1986
}
@Unpublished{SafDij:1987:998,
  author =   {E. W. Dijkstra},
  title =    {{Shmuel Safra's Version of Termination Detection}},
  note =     {EWD Manuscript 998. Available at \texttt{http://www.cs.utexas.edu/users/EWD}},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1987},
  OPTannote =    {}
}
@TechReport{Sai:2002:TR:51,
  author =   {Y. Saito},
  title =    {{Unilateral Version Vector Pruning using Loosely Synchronized Clocks}},
  institution =  HPL,
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {HPL-2002-51},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{SchGet:1987:TOG,
  author =       {R.W. Scheifler and J. Gettys},
  title =        {{The X Window System}},
  journal =      TOG,
  month =        APR,
  year =         1987,
  volume =       5,
  number =       2,
  pages =        {79-109}
}
@Article{SchMat:1994:DC,
  author =   {R. Schwartz and F. Mattern},
  title =    {{D}etecting {C}ausal {R}elationships in {D}istributed  {C}omputations:
                  {I}n {S}earch of the {H}oly {G}rail},
  journal =      DC,
  year =     1994,
  volume =   7,
  number =   3,
  pages =    {149-174}
}
@InProceedings{SchWyl:1991:SOSP,
  author =   {F. Schmuck and J. Wyllie},
  title =    {{Experience with Transactions in QuickSilver}},
  booktitle =    PROC # " 13th " # SOSP,
  pages =    {239-253},
  year =     1991,
  month =    OCT
}
@InProceedings{SenGar:2002:IPDPS,
  author =   {A. Sen and V. K. Garg},
  title =    {{D}etecting {T}emporal {L}ogic {P}redicates in the {H}appened-{B}efore {M}odel},
  booktitle =    PROC # " " # IPDPS,
  year =     2002,
  address =      {Florida},
  month =    APR
}
@TechReport{SenGar:2002:TR:001,
  author =   {A. Sen and V. K. Garg},
  title =    {{A}utomatic {G}eneration of {C}omputation {S}lices for
                  {D}etecting {T}emporal {L}ogic {P}redicates},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2003-001},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{SenGar:2003:OPODIS,
  author =       {A. Sen and V. K. Garg},
  title =        {{Detecting Temporal Logic Predicates in Distributed
                   Programs using Computation Slicing}},
  booktitle =    PROC # " " # OPODIS,
  OPTpages =     {},
  month =        DEC,
  year =         {2003}
}
@InProceedings{SenGar:2003:RV,
  author =       {A. Sen and V. K. Garg},
  title =        {{P}artial {O}rder {T}race {A}nalyzer ({POTA}) for
                  {D}istributed {P}rograms},
  booktitle =    PROC # " Third " # RV,
  OPTseries =    {Electronic Notes in Theoretical Computer Science},
  volume =       {89},
  issue =        {2},
  publisher =    {Elsevier},
  year =         {2003}
}


@InProceedings{ShaFra:1986:ICALP,
  author =   {N. Shavit and N. Francez},
  title =    {{A New Approach to Detection of Locally Indicative Stability}},
  booktitle =    PROC # " " # ICALP,
  pages =    {344-358},
  year =     1986,
  address =      {Rennes, France}
}


@TechReport{ShaTou:1984:TR:624,
  author =   {A. Shah and S. Toueg},
  title =    {{Distributed Snapshots in spite of Failures}},
  institution =  DCS # ", " # CORNELL,
  year =     1984,
  number =   {TR84-624},
  address =      {Ithaca, NY},
  month =    JUL,
  note =     {(Revised February 1985)}
}


@InProceedings{SheDea:2002:WETICE,
  author =       {J. S. Sherif and T. G. Dearmond},
  title =        {{Intrusion Detection: Systems and Models}},
  booktitle =    PROC # " " # WETICE,
  pages =        {115-136},
  month =        JUN,
  year =         {2002},
  address =      {Pittsburgh, Pennsylvania}
}


@Book{SinShi:1994:Book,
  author =       {M. Singhal and N. G. Shivaratri},
  title =        {{Advanced Concepts in Operating Systems}},
  publisher =    MH # " and " # MIT,
  year =         {1994},
  ISBN =         {0-07-057572-X}
}

@InProceedings{SkaMit+:1999:PDCS,
  author =   {C. Skawratananond and N. Mittal and V. K. Garg},
  title =    {{A} {L}ightweight {A}lgorithm for {C}ausal {M}essage
                  {O}rdering in {M}obile {C}omputing {S}ystems},
  booktitle =    PROC # " 12th " # PDCS,
  pages =    {245-250},
  year =     {1999},
  address =      {Florida}
}


@Unpublished{SolDes,
  author =   {Solar Designer},
  title =    {{Root Programs and Links}},
  note =     {Available at \texttt{http://www.openwall.com/linux/}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@Unpublished{SolDes:OP,
  author =   {Openwall Project},
  title =    {{Linux Kernel Patch}},
  note =     {\textsf{http://www.openwall.com/linux}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@InProceedings{SpeKea:1986:ICDCS,
  author =   {M. Spezialetti and P. Kearns},
  title =    {{Efficient Distributed Snapshots}},
  booktitle =    PROC # " 6th " # ICDCS,
  pages =    {382-388},
  year =     1986
}


@Article{SpiBra:1987:DAM,
  author =   {J. Spinrad and A. Brandstadt and L. Stewart},
  title =    {{Bipartite Permutation Graphs}},
  journal =      DAM,
  year =     1987,
  volume =   18,
  pages =    {279-292}
}



@InProceedings{SriSiv:2002:ICPDCS,
  author =   {N. Sridhar and P. A. G. Sivilotti},
  title =    {{L}azy {S}napshots},
  booktitle =    PROC # " 14th " # ICPDCS,
  pages =    {96-101},
  year =     {2002},
  OPTeditor =    {S.G. Akl and T.Gonzalez},
  address =      {Cambridge, MA},
  month =    NOV,
  OPTorganization = {IASTED},
  OPTpublisher =    {ACTA Press},
  OPTurl =          {http://citeseer.nj.nec.com/sridhar02lazy.html}
}



@InProceedings{SroSch+:1998:WNTS,
  author =   {J. Srouji and P. Schuster and M. Bach and Y. Kuzmin},
  title =    {{A Transparent Checkpoint Facility on NT}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 2nd " # WNTS,
  OPTpages =     {},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Seattle, Washington},
  month =    {August},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Sta:2001:PH,
  author =   {W. Stallings},
  title =    {{O}perating {S}ystems: {I}nternals and {D}esign {P}rinciples},
  publisher =    PH,
  year =     2001
}




@InCollection{StoLiu:1998:CAV,
  author =   {S. D. Stoller and Y. A. Liu},
  title =    {{E}fficient {S}ymbolic {D}etection of {G}lobal
                  {P}roperties in {D}istributed {S}ystems},
  booktitle =    PROC # " 10th " # CAV,
  pages =    {357-368},
  publisher =    {Springer-Verlag},
  year =     1998,
  editor =   {Alan J. Hu and Moshe Y. Vardi},
  volume =   1427,
  series =   LNCS
}



@InProceedings{StoSch:1995:WDAG,
  author =   {S. D. Stoller and F. Schneider},
  title =    {{F}aster {P}ossibility {D}etection by {C}ombining
                  {T}wo {A}pproaches},
  booktitle =    PROC # " " # WDAG,
  pages =        {318-332},
  year =     1995,
  volume =       {972},
  series =       LNCS,
  address =  {France},
  month =    SEP
}


@InProceedings{StoUnn+:2000:CAV,
  author =   {S. D. Stoller and L. Unnikrishnan and Y. A. Liu},
  title =    {{Efficient Detection of Global Properties in
                  Distributed Systems Using Partial-Order Methods}},
  booktitle =    PROC # " 12th " # CAV,
  pages =    {264-279},
  year =     2000,
  volume =   1855,
  series =   LNCS,
  month =    JUL,
  publisher =    {Springer-Verlag}
}



@InProceedings{Stu:2002:DISC,
  author =   {G. Stupp},
  title =    {{Stateless Termination Detection}},
  booktitle =    PROC # " 16th " # DISC,
  pages =    {163-172},
  year =     2002,
  address =      {Toulouse, France}
}


@InProceedings{Tai:1997:ICDCS,
  author =   {K. Tai},
  title =    {{R}ace {A}nalysis of {T}races of {A}synchronous
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " 17th " # ICDCS,
  pages =    {261-268},
  year =     1997
}



@PhdThesis{Tar:2000:Thesis,
  author =   {A. Tarafdar},
  title =    {{S}oftware {F}ault {T}olerance in {D}istributed {S}ystems
                  {U}sing {C}ontrolled {R}e-execution},
  school =   {The University of Texas at Austin},
  year =     2000,
  month =    AUG
}


@InProceedings{TarGar:1998:ICDCS,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{A}ddressing {F}alse {C}ausality while {D}etecting
                  {P}redicates in {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # ICDCS,
  pages =    {94-101},
  year =     1998,
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}

@InProceedings{TarGar:1998:SPDP,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{P}redicate {C}ontrol for {A}ctive {D}ebugging of
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # SPDP,
  pages =        {763-769},
  year =     1998,
  address =  {Orlando}
}

@InProceedings{TarGar:1999:DISC,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{S}oftware {F}ault {T}olerance of {C}oncurrent
                  {P}rograms {U}sing {C}ontrolled {R}e-execution},
  booktitle =    PROC # " 13th " # DISC,
  pages =    {210-224},
  year =     1999,
  address =  {Bratislava, Slovak Republic},
  month =    SEP
}


@Book{Tel:2000:CUP,
  author =   {G. Tel},
  title =    {{Introduction to Distributed Algorithms}},
  publisher =    CUP # "~(US Server)",
  year =     2000,
  edition =      {Second},
  month =    SEP
}

@Article{TelMat:1993:TOPLAS,
  author =   {G. Tel and F. Mattern},
  title =    {{The Derivation of Distributed Termination Detection Algorithms from Garbage Collection Schemes}},
  journal =      TOPLAS,
  year =     1993,
  volume =   15,
  number =   1,
  pages =    {1-35},
  month =    JAN
}



@Article{Tip:1995:JPL,
  author =   {F. Tip},
  title =    {{A Survey of Program Slicing Techniques}},
  journal =      JPL,
  year =     1995,
  volume =   3,
  number =   3,
  pages =    {121-189}
}

@InProceedings{TomGar:1993:WPDS,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{An Algorithm for Minimally Latent Global Virtual Time}},
  booktitle =    PROC # " 7th " # WPDS,
  pages =        {35-42},
  year =     1993,
  address =  {San Diego, California},
  month =    MAY
}


@InProceedings{TomGar:1994:CSE,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{Maintaining Global Assertions in Distributed Systems}},
  booktitle =    CSE,
  pages =    {257-272},
  year =     1994,
  publisher =    TMH
}


@Article{TomGar:1994:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@InProceedings{TomGar:1995:FSTTCS,
  author =       {A. I. Tomlinson and V. K. Garg},
  title =        {{Observation of Software for Distributed Systems with RCL}},
  booktitle =    PROC # " 15th " # FSTTCS,
  pages =        {195-209},
  year =         {1995},
  url =          {http://citeseer.nj.nec.com/tomlinson95observation.html}
}

@Article{TomGar:1997:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {2},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@Book{Tro:1992:JHUP,
  author =   {W. T. Trotter},
  title =    {{C}ombinatorics and {P}artially {O}rdered {S}ets: {D}imension {T}heory},
  publisher =    JHUP,
  year =     1992,
  address =      {Baltimore, MD}
}

@article{Tse:1995:JPDC,
  author =       {Y.-C. Tseng},
  title =        {{Detecting Termination by Weight-Throwing in a Faulty Distributed System}},
  journal =      JPDC,
  volume =       {25},
  number =       {1},
  pages =        {7-15},
  year =         "1995",
  OPTnote =      "previous label was Tse:1992:JPDC"
}

@Article{TseTan:2001:TPDS,
  author =       {Y.-C. Tseng and C.-C. Tan},
  title =        {{On Termination Detection Protocols in a Mobile Distributed
                   Computing Environment}},
  journal =      TPDS,
  year =         2001,
  volume =       12,
  number =       6,
  pages =        {558-566}
}


@InProceedings{TsyYee:2003:USS,
  author =   {E. Tsyrklevich and B. Yee},
  title =    {{Dynamic Detection and Prevention of Race Conditions in File Accesses}},
  booktitle =    PROC # " 12th " # USS,
  pages =    {243-255},
  year =     2003,
  month =    AUG
}

@Article{Tur:1984:DAM,
  author =   {G. Turan},
  title =    {{Succinct Representations of Graphs}},
  journal =      DAM,
  year =     1984,
  volume =   8,
  pages =    {289-294}
}

@Book{Vah:1996:PH,
  author =   {U. Vahalia},
  title =    {Unix Internals: The New Frontiers},
  publisher =    PH,
  year =     1996,
  month =    JAN
}

@Article{ValTar+:1982:SIAMJC,
  author =   {J. Valdes and R. E. Tarjan and E. L. Lawler},
  title =    {{T}he {R}ecognition of {S}eries-{P}arallel {D}igraphs},
  journal =      SIAMJC,
  year =     1982,
  volume =   11,
  pages =    {298-314}
}

@Article{Ven:1989:TR,
  author =   {S. Venkatesan},
  title =    {{Reliable Protocols for Distributed Termination Detection}},
  journal =      TR,
  year =     1989,
  volume =   38,
  number =   1,
  pages =    {103-110},
  month =    APR
}




@Article{Ven:1995:TOPLAS,
  author =   {G. Venkatesh},
  title =    {{Experimental Results from Dynamic Slicing of C Programs}},
  journal =      TOPLAS,
  year =     1995,
  volume =   17,
  number =   2,
  pages =    {197-216}
}







@Article{SuzKas:1985:TrCS,
  author =   {I. Suzuki and T. Kasami},
  title =    {{A Distributed Mutual Exclusion Algorithm}},
  journal =      TrCS,
  year =     1985,
  volume =   3,
  number =   4,
  pages =    {344-349}
}



@Article{VenDat:1995:TSE,
  author =   {S. Venkatesan and B. Dathan},
  title =    {{T}esting and {D}ebugging {D}istributed {P}rograms {U}sing
                  {G}lobal {P}redicates},
  journal =      TSE,
  year =     1995,
  volume =   21,
  number =   2,
  pages =    {163-177},
  month =    FEB
}


@InProceedings{VieBlo+:2000:CSAC,
  author =   {J. Viega, J. Bloch, T. Kohno and G. McGraw},
  title =    {{ITS4: A Static Vulnerability Scanner for C and C++ Code}},
  booktitle =    PROC # " " # CSAC,
  year =     2000,
  month =    DEC
}


@InProceedings{WalGar:1991:WPDD,
  author =       {B. Waldecker and V. K. Garg },
  title =        {{U}nstable {P}redicate {D}etection in {D}istributed
                  {P}rogram {D}ebugging},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  pages =        {276-278},
  month =    MAY,
  year =     1991
}

@Article{Wan:1997:TC,
  author =   {Y.-M. Wang},
  title =    {{C}onsistent {G}lobal {C}heckpoints that {C}ontain a
                  {G}iven {S}et of {L}ocal {C}heckpoints},
  journal =      TC,
  year =     1997,
  volume =   46,
  number =   4,
  pages =    {456-468},
  month =    APR
}


@InProceedings{WanDam+:1997:ICDCS,
  author =       {Y. M. Wang and O. P. Damani and V. K. Garg},
  title =        {{D}istributed {R}ecovery with {K}-{O}ptimistic Logging},
  pages =        {60-67},
  booktitle =    PROC # " 17th " # ICDCS,
  address =      {Baltimore, Maryland},
  month =        JUN,
  publisher =    {IEEE},
  address =  {Washington - Brussels - Tokyo},
  year =         1997,
}



@Article{WanHua+:1997:TC,
  author =   {Y.-M. Wang and Y. Huang and W. K. Fuchs and
                  C. Kintala and G. Suri},
  title =    {{P}rogressive {R}etry for {S}oftware {F}ailure
                  {R}ecovery in {M}essage-{P}assing {A}pplications},
  journal =  TC,
  year =     1997,
  volume =   46,
  number =   10,
  pages =    {1137-1141},
  month =    OCT
}



@InProceedings{WanMay:2004:IPDPS,
  author =   {X. Wang and J. Mayo},
  title =    {{A General Model for Detecting Termination in Dynamic Systems}},
  booktitle =    PROC # " 18th " # IPDPS,
  year =     2004,
  address =      {Santa Fe, New Mexico},
  month =    APR
}


@Article{Wei:1982:CACM,
  author =   {M. Weiser},
  title =    {{P}rogrammers {U}se {S}lices when {D}ebugging},
  journal =  CACM,
  year =     1982,
  volume =   25,
  number =   7,
  pages =    {446-452}
}

@Article{WuJou:2000:CDS,
  author =   {K.-P. Wu and Y.-J. Joung},
  title =    {{Asynchronous Group Mutual Exclusion in Ring Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  journal =      CDS,
  pages =    {1-8},
  year =     {2000},
  OPTeditor =    {},
  volume =   {147},
  number =   {1}
}



@Article{Yan:1982:SIAMHADM,
  author =   {M. Yannakakis},
  title =    {{T}he {C}omplexity of the {P}artial {O}rder {D}imension {P}roblem},
  journal =      SIAMJADM,
  year =     1982,
  volume =   3,
  pages =    {351-358}
}




@InProceedings{ZibGil:1997:OOPSLA,
  author =   {Y. Zibin and Y. Gil},
  title =    {{E}fficient {S}ubtyping {T}ests with {PQ}-{E}ncoding},
  booktitle =    PROC # " 16th Annual " # OOPSLA,
  pages =    {96-107},
  year =     1997,
  address =      {Tampa Bay, Florida},
  month =    OCT
}

@Manual{iFS:1999,
  author =   {Oracle},
  title =    {iFS: Oracle Internet File System},
  note =     {\\ {\sf
                  http://www.oracle.com/database/options/ifs.html}},
  year =     1999
}

@InProceedings{WuLai+:1992:ICPADS,
  author =   {L.-F. Wu and T.-H. Lai and Y.-C. Tseng},
  title =    {{Consensus and Termination Detection in the Presence of Faulty Processes}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPADS,
  pages =    {267-274},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Hsinchu, Taiwan},
  month =    DEC,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{DwoLyn+:1988:JACM,
  author =       {C. Dwork and N. Lynch and L. Stockmeyer},
  title =        {{Consensus in the presence of partial synchrony}},
  OPTcrossref =  "",
  OPTkey =       "",
  journal =      JACM,
  year =         "1988",
  volume =       "35",
  number =       "2",
  pages =        {288-323},
  month =        APR,
  OPTnote =      "",
  annote =       "The authors study practically motivated models of
                  synchrony that lie between fully asynchronous and
                  fully synchronous systems in which consensus shall
                  be achieved. The models of partial synchrony studied
                  include: (1) upper bounds on processor speeds and
                  message latency exist but are unknown, and (2) upper
                  bounds exists and are known, but only hold after
                  some unknown time (eventually). In both cases
                  consensus with different resiliency can be achieved."
}


@InProceedings{DelFau+:2004:PODC,
  author =   {C. Delporte-Gallet and H. Fauconnier and R. Guerraoui and
                  V. Hadzilacos and P. Kouznetsov and S. Toueg},
  title =    {{The Weakest Failure Detector to Solve Certain Fundamental Problems
                   in Distributed Computing}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {St. Johns, Newfoundland, Canada},
  month =    JUL,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{MitGae+:2004:TR:37,
  author =   {N. Mittal and F. G{\"a}rtner and S. Venkatesan and L. D. Penso},
  title =    {{ Detecting Termination in a Crash-Prone Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-37-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{HurMiz+:1998:TSE,
  author =       {M. Hurfin and M. Mizuno and M. Singhal and M. Raynal},
  title =        {Efficient Distributed Detection of Conjunctions of Local Predicates},
  journal =      TSE,
  volume =       {24},
  number =       {8},
  year =         {1998},
  issn =         {0098-5589},
  pages =        {664--677},
  doi =          {http://dx.doi.org/10.1109/32.707701},
  publisher =    {IEEE Press},
}

@Book{Lyn:1996:MK,
  author =   {N. Lynch},
  OPTeditor =    {},
  title =    {{Distributed Algorithms}},
  publisher =    MK,
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Awe:1987:STOC,
  author =       {B. Awerbuch},
  title =        {{Optimal Distributed Algorithms for Minimum Weight Spanning Tree, Counting,
                   Leader Election, and Related Problems}},
  booktitle =    PROC # " 19th " # STOC,
  year =         {1987},
  pages =        {230-240},
  address =      {New York, New York, United States},
  publisher =    {ACM Press},
}

@Article{SchSan:1994:DC,
  author =   {A. Schiper and A. Sandoz},
  title =    {{Strong Stable Properties in Distributed Systems}},
  journal =      DC,
  year =     {1994},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {93-103},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{SinKal+:1993:TR:93-11,
  author =   {A. Sinha and L. Kal{\'e} and B. Ramkumar},
  title =    {{A Dynamic and Adaptive Quiescence Detection Algorithm}},
  institution =  PPL # ", " #  DCS # ", "  # UIUC,
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {93-11},
  OPTaddress =   {Urbana-Champaign, IL 61801},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{An Example of Stepwise Refinement of Distributed Programs: Quiescence Detection}},
  journal =      TOPLAS,
  year =     {1986},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {326-343},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{KshSin:1994:TSE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{Efficient Detection and Resolution of Generalized Distributed Deadlocks}},
  journal =      TSE,
  year =     {1994},
  OPTkey =   {},
  volume =   {20},
  number =   {1},
  pages =    {43-54},
  month =    JAN,
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BraTou:1987:DC,
  author =   {G. Bracha and S. Toueg},
  title =    {{Distributed Deadlock Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {127-138},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Kna:1987:CS,
  author =   {E. Knapp},
  title =    {{Deadlock Detection in Distributed Databases}},
  journal =      CS,
  year =     {1987},
  OPTkey =   {},
  volume =   {19},
  number =   {4},
  pages =    {303-328},
  month =    DEC,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LynMal+:2002:WPPS,
  author =   {N. Lynch and D. Malkhi and D. Ratajczak},
  title =    {{Atomic Data Access in Content Addressable Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # WPPS,
  pages =    {295-305},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LiMis+:2004:DISC,
  author =   {X. Li and J. Misra and C. G. Plaxton},
  title =    {{Active and Concurrent Topology Maintenance}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # DISC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{ZhaHua+:2003:SAC,
  author =   {B. Y. Zhao and L. Huang and J. Stribling and S. C. Rhea and A. D. Joseph and J. Kubiatowicz},
  title =    {{Tapestry: A Resilient Global-Scale Overlay for Service Deployment}},
  journal =      SAC,
  year =     {2003},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {41-53},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoMor+:2003:TN,
  author =   {I. Stoica and R. Morris and D. Liben-Nowell and D. R. Karger and M. F. Kaashoek
                  and F. Dabek and H. Balakrishnan},
  title =    {{Chord: A Scalable Peer-to-Peer Lookup Service for Internet Applications}},
  journal =      TN,
  year =     {2003},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {17-32},
  month =    FEB,
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AspSha:2003:SDA,
  author =   {J. Aspnes and G. Shah},
  title =    {{Skip Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 14th Annual " # SDA,
  pages =    {384-393},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BanMay:2004:SIU,
  author =   {S. Bansod and J. Mayo},
  title =    {{A Distributed Algorithm for Unstable Global Predicate Evaluation with Approximately Synchronized Clocks}},
  journal =      SIU,
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {2},
  pages =    {151-168},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{AgaGar:2004:TR,
  author =   {A. Agarwal and V. K. Garg},
  title =    {{Chain Clock: Efficient Causality Tracking for Shared Memory Systems}},
  note =     "Submitted to the " # ICDCS,
  OPTkey =   {},
  month =    JUN,
  year =     {2005},
  OPTannote =    {}
}



@Article{Lee:2004:TSE,
  author =   {S. Lee},
  title =    {{Fast, Centralized Detection and Resolution of Distributed Deadlocks in the
                   Generalized Model}},
  journal =      TSE,
  year =     {2004},
  OPTkey =   {},
  volume =   {30},
  number =   {9},
  pages =    {561-573},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BouTro:1998:TPDS,
  author =   {A. Boukerche and C. Tropper},
  title =    {{A Distributed Graph Algorithm for the Detection of Local Cycles and Knots}},
  journal =      TPDS,
  year =     {1998},
  OPTkey =   {},
  volume =   {9},
  number =   {8},
  pages =    {748-757},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{CheDen+:1996:ICDCS,
  author =   {S. Chen and Y. Deng and P. C. Attie and W. Sun},
  title =    {{Optimal Deadlock Detection in Distributed Systems based on
                   Locally Constructed Wait-For Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {613-619},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAY,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hol:1972:CS,
  author =   {R. C. Holt},
  title =    {{Some Deadlock Properties of Computer Systems}},
  journal =      CS,
  year =     {1972},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  pages =    {179-195},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1999:KDE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{A One-Phase Algorithm to Detect Distributed Deadlocks in
                   Replicated Databases}},
  journal =      KDE,
  year =     {1999},
  OPTkey =   {},
  volume =   {11},
  number =   {6},
  pages =    {880-895},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{ManSin:2002:ICPP,
  author =   {D. Manivannan and M. Singhal},
  title =    {{A Distributed Algorithm for Knot Detection in a Distributed Graph}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPP,
  OPTpages =     {},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ManSin:2003:TPDS,
  author =   {D. Manivannan and M. Singhal},
  title =    {{An Efficient Distributed Algorithm for Detecting Knots and
                   Cycles in a Distributed Graph}},
  journal =      TPDS,
  year =     {2003},
  OPTkey =   {},
  volume =   {14},
  OPTnumber =    {10},
  pages =    {961-972},
  month =    OCT,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Sin:1989:Com,
  author =   {M. Singhal},
  title =    {{Deadlock Detection in Distributed Systems}},
  journal =      Com,
  year =     {1989},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {37-48},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1994:JPDC,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{On Characterization and Correctness of Distributed Deadlock Detection}},
  journal =      JPDC,
  year =     {1994},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {44-59},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{JagVas:1983:TSE,
  author =   {J. R. Jagannathan and R. Vasudevan},
  title =    {{Comments on ``Protocols for Deadlock Detection in
                  Distributed Database Systems''}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {371},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Awe:1985:JACM,
  author =   {B. Awerbuch},
  title =    {{Complexity of Network Synchronization}},
  journal =      JACM,
  year =     {1985},
  OPTkey =   {},
  volume =   {32},
  number =   {4},
  pages =    {804-823},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@inproceedings{XiaPlax:2002:POMC,
 author = {Xiaozhou Li and C. Greg Plaxton},
 title = {On name resolution in peer-to-peer networks},
 booktitle = {POMC '02: Proceedings of the second ACM international workshop on Principles of mobile computing},
 year = {2002},
 isbn = {1-58113-511-4},
 pages = {82--89},
 location = {Toulouse, France},
 doi = {http://doi.acm.org/10.1145/584490.584507},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@URL{dist,
  author =       {},
  title =        "www.distributed.net/rc5",
  howpublished = {},
  year =         "2002",
  month =        "Dec",
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
  file = F
}

@CONFERENCE{SatNeer:2005:FSTTCS,
  author =       {Sathya Peri and Neeraj Mittal},
  title =        {Monitoring Stable Properties in Dynamic Peer-to-Peer Distributed Systems},
  booktitle =    PROC # " 25th " # FSTTCS,
  year =         {2005},
  pages  =       {420-431},
  address =      {Hyderabad, India},
  month =        {December},
  note =         {},
  key =          {},
  crossref =     {},
  annote =       {},
}

@TECHREPORT{BalHelPier:2004:TR,
  AUTHOR =       {R. Baldoni and J. Helary and S. Tucci Piergiovanni},
  TITLE =        {Maintaining group connectivity in dynamic asynchronous distributed systems},
  INSTITUTION =  {``Dipartimento di Informatica e Sistemistica, A.Ruberti, Universit?? di Roma la Sapienza"},
  YEAR =         {2004},
  doi=           {"http://www.dis.uniroma1.it/~midlab"},
}

@article{PageJacChen:1993:TPDS,
 author = {I. Page and T. Jacob and E. Chern},
 title = {Fast Algorithms for Distributed Resource Allocation},
 journal = {IEEE Trans. Parallel Distrib. Syst.},
 volume = {4},
 number = {2},
 year = {1993},
 issn = {1045-9219},
 pages = {188--197},
 doi = {http://dx.doi.org/10.1109/71.207594},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
}

@article{ChoiSing:1995:TOPLAS,
 author = {Manhoi Choy and Ambuj K. Singh},
 title = {Efficient fault-tolerant algorithms for distributed resource allocation},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {17},
 number = {3},
 year = {1995},
 issn = {0164-0925},
 pages = {535--559},
 doi = {http://doi.acm.org/10.1145/203095.203101},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@TECHREPORT{SatNeer:2006:TR,
  AUTHOR =       {Sathya Peri and Neeraj Mittal},
  TITLE =        {Lower bounds on Departures for Dynamic Asynchronous Peer-to-Peer systems},
  INSTITUTION =  {University of Texas at Dallas},
  YEAR =         {2006},
}

@INPROCEEDINGS{WeidPagPerv:1991:SPDP,
  AUTHOR =       {Weidman.E.B and Page.I.P and Pervin.W.J},
  TITLE =        {{Explicit dynamic exclusion algorithm}},
  BOOKTITLE =    {Proceedings of the Third IEEE Symposium on Parallel and Distributed Processing},
  YEAR =         {1991},
  pages =        {142-149},
  month =        {DEC},
  organization = {IEEE},
}

@INPROCEEDINGS{LynMalRata:2002:IPTPS,
  AUTHOR =       {N. Lynch and D. Malkhi and D. Ratajczak},
  TITLE =        {{Atomic Data Access in Content Addressable Networks}},
  BOOKTITLE =    {Proceedings for the 1st International Workshop on Peer-to-Peer Systems (IPTPS '02)},
  YEAR =         {2002},
  month =        {Mar},
  publisher =    {Springer-Verlag},
}
%% Citations included by Sat in the area of STMs

@article{HerlMoss:1993:SigArch,
 author = {Maurice Herlihy and J. Eliot B.Moss },
 title = {{Transactional memory: {A}rchitectural {S}upport for {L}ock-{F}ree {D}ata {S}tructures}},
 journal = {SIGARCH Comput. Archit. News},
 volume = {21},
 number = {2},
 year = {1993},
 issn = {0163-5964},
 pages = {289--300},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ShavTou:1995:PODC,
 author = {Shavit, Nir and Touitou, Dan},
 title = {{{S}oftware {T}ransactional {M}emory}},
 booktitle = {PODC},
 year = {1995},
 isbn = {0-89791-710-3},
 pages = {204--213},
 location = {Ottowa, Ontario, Canada},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{Harretal:2005:PPoPP,
 author = {Tim Harris and Simon Marlow and Simon Peyton-Jones and Maurice Herlihy},
 title = {{Composable memory transactions}},
 booktitle = {PPoPP},
 year = {2005},
 isbn = {1-59593-080-9},
 pages = {48--60},
 location = {Chicago, IL, USA},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Yangetal:2007:PPoPP,
 author = {Ni, Yang and Menon, Vijay S. and Adl-Tabatabai, Ali-Reza and Hosking, Antony L. and Hudson, Richard L. and Moss, J. Eliot B. and Saha, Bratin and Shpeisman, Tatiana},
 title = {{Open nesting in software transactional memory}},
 booktitle = {PPoPP},
 year = {2007},
 isbn = {978-1-59593-602-8},
 pages = {68--78},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1229428.1229442},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{AgarLeiSukh:2006:MSPC,
 author = {Agrawal, Kunal and Leiserson, Charles E. and Sukha, Jim},
 title = {{Memory models for open-nested transactions}},
 booktitle = {MSPC '06: Proceedings of the 2006 workshop on Memory system performance and correctness},
 year = {2006},
 isbn = {1-59593-578-9},
 pages = {70--81},
 location = {San Jose, California},
 doi = {http://doi.acm.org/10.1145/1178597.1178610},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{MossAnt:2006:SCP,
 author = {Moss, J. Eliot B. and Hosking, Antony L.},
 title = {{Nested transactional memory: model and architecture sketches}},
 journal = {Sci. Comput. Program.},
 volume = {63},
 number = {2},
 year = {2006},
 issn = {0167-6423},
 pages = {186--201},
 doi = {http://dx.doi.org/10.1016/j.scico.2006.05.010},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@inproceedings{AgarFinSukh:2008:PPoPP,
 author = {Agrawal, Kunal and Fineman, Jeremy T. and Sukha, Jim},
 title = {{Nested parallelism in transactional memory}},
 booktitle = {PPoPP '08: Proceedings of the 13th ACM SIGPLAN Symposium on Principles and practice of parallel programming},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {163--174},
 location = {Salt Lake City, UT, USA},
 doi = {http://doi.acm.org/10.1145/1345206.1345232},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Moretal:2006:ASPLOS,
 author = {Moravan, Michelle J. and Bobba, Jayaram and Moore, Kevin E. and Yen, Luke and Hill, Mark D. and Liblit, Ben and Swift, Michael M. and Wood, David A.},
 title = {{Supporting nested transactional memory in logTM}},
 booktitle = {ASPLOS-XII: Proceedings of the 12th international conference on Architectural support for programming languages and operating systems},
 year = {2006},
 isbn = {1-59593-451-0},
 pages = {359--370},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1168857.1168902},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@Article{Moss:2006:MPI,
	author = {J.E.B.Moss},
	journal = {In Workshop on Memory Performance Issues},
	year = {2006},
	title = {{Open Nested Transactions: Semantics and Support}}
}

@inproceedings{GuerKap:Opacity:PPoPP:2008,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {{On the {C}orrectness of {T}ransactional {M}emory}},
 booktitle = {PPoPP},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {},
 location = {},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{ImbsRay:LockSTM:OPODIS:2008,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A Lock-Based STM Protocol That Satisfies Opacity and Progressiveness}},
 booktitle = {OPODIS '08: Proceedings of the 12th International Conference on Principles of Distributed Systems},
 year = {2008},
 isbn = {978-3-540-92220-9},
 pages = {226--245},
 location = {Luxor, Egypt},
 doi = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 }

@article{Herlihy+:Linearizability:TPLS:1990,
 author = {Herlihy, Maurice P. and Wing, Jeannette M.},
 title = {{Linearizability: a correctness condition for concurrent objects}},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {12},
 number = {3},
 year = {1990},
 issn = {0164-0925},
 pages = {463--492},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{Papad:1979:JACM,
 author = {Papadimitriou, Christos H.},
 title = {{The serializability of concurrent database updates}},
 journal = {J. ACM},
 volume = {26},
 number = {4},
 year = {1979},
 issn = {0004-5411},
 pages = {},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@BOOK{tm-book,
	AUTHOR		= {Guerraoui, Rachid and  Kapalka, Michal},
	TITLE		= {{Principles of Transactional Memory, Synthesis Lectures on Distributed Computing Theory}},
	PUBLISHER	= {Morgan and Claypool},
	YEAR		= {2010},
}

@article{Vidya:1987:AINF,
 author = {Vidyasankar, K.},
 title = {{Generalized theory of serializability}},
 journal = {Acta Inf.},
 volume = {24},
 number = {1},
 year = {1987},
 issn = {0001-5903},
 pages = {105--109},
 doi = {http://dx.doi.org/10.1007/BF00290709},
 publisher = {Springer-Verlag New York, Inc.},
 address = {Secaucus, NJ, USA},
 }

@article{RenAbba:1994:IPL,
 author = {Resende, R. F. and El Abbadi, A.},
 title = {{On the serializability theorem for nested transactions}},
 journal = {Inf. Process. Lett.},
 volume = {50},
 number = {4},
 year = {1994},
 issn = {0020-0190},
 pages = {177--183},
 doi = {http://dx.doi.org/10.1016/0020-0190(94)00033-6},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@book{WeiVoss:TIS:2002:Morg,
  author    = {Gerhard Weikum and
               Gottfried Vossen},
  title     = {{Transactional Information Systems: Theory, Algorithms, and
               the Practice of Concurrency Control and Recovery}},
  publisher = {Morgan Kaufmann},
  year      = {2002},
  isbn      = {1-55860-508-8},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Imbs+:2009:PODC,
 author = {Imbs, Damien and de Mendivil, Jos\'{e} Ramon and Raynal, Michel},
 title = {{Brief announcement: virtual world consistency: a new condition for STM systems}},
 booktitle = {PODC '09: Proceedings of the 28th ACM symposium on Principles of distributed computing},
 year = {2009},
 isbn = {978-1-60558-396-9},
 pages = {280--281},
 location = {Calgary, AB, Canada},
 doi = {http://doi.acm.org/10.1145/1582716.1582764},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ImbsRay:2009:SIROCCO,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A versatile {STM} protocol with invisible read operations that satisfies the virtual world consistency condition}},
 booktitle = {Proceedings of the 16th international conference on Structural Information and Communication Complexity},
 series = {SIROCCO'09},
 year = {2010},
 isbn = {3-642-11475-X, 978-3-642-11475-5},
 location = {Piran, Slovenia},
 pages = {266--280},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-11476-2_21},
 doi = {10.1007/978-3-642-11476-2_21},
 acmid = {2174448},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {atomic object, causal past, commit/abort, concurrency control, consistency condition, consistent global state, lock, read-from relation, regular read/write object, serializability, shared memory, software transactional memory, transaction, vector clock},
} 

@inproceedings{CIR11,
  author    = {Tyler Crain and
               Damien Imbs and
               Michel Raynal},
  title     = {{Read Invisibility, Virtual World Consistency and Probabilistic
               Permissiveness are Compatible}},
  booktitle = {ICA3PP (1)},
  year      = {2011},
  pages     = {244-257}
}

@inproceedings{israeli-disjoint,
 author = {Israeli, Amos and Rappoport, Lihu},
 title = {{Disjoint-access-parallel implementations of strong shared memory primitives}},
 booktitle = {Proceedings of the thirteenth annual ACM symposium on Principles of distributed computing},
 series = {PODC '94},
 year = {1994},
 isbn = {0-89791-654-9},
 location = {Los Angeles, California, United States},
 pages = {151--160},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/197917.198079},
 doi = {http://doi.acm.org/10.1145/197917.198079},
 acmid = {198079},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{AHM09,
 author = {Attiya, Hagit and Hillel, Eshcar and Milani, Alessia},
 title = {{Inherent limitations on disjoint-access parallel implementations of transactional memory}},
 booktitle = {Proceedings of the twenty-first annual symposium on Parallelism in algorithms and architectures},
 series = {SPAA '09},
 year = {2009},
 isbn = {978-1-60558-606-9},
 location = {Calgary, AB, Canada},
 pages = {69--78},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1583991.1584015},
 doi = {http://doi.acm.org/10.1145/1583991.1584015},
 acmid = {1584015},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {disjoint-access parallelism, impossibility result, lower bound, partial snapshots, transactional memory},
} 

@InProceedings{Doherty+:2009:REFINE,
	booktitle = {REFINE},
	year = {2009},
	author = {Simon Doherty and Lindsay Groves and Victor Luchangco and Mark Moir},
	title = {{Towards Formally Specifying and Verifying Transactional Memory}}
}

@TechReport{SatVid:2010:TR,
	author = {Sathya Peri and K.Vidyasankar},
	institution = {Memorial University of Newfoundland},
	title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
	year = {July, 2011}
}

@inproceedings{SatVid:2011:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
 booktitle = {12th International Conference on Distributed Computing and Networking},
 pages = {95--106},
 year = {2011},
 location = {Bangalore, Canada},
 }

@inproceedings{SatVid:2012:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{An efficient scheduler for closed nested transactions that satisfies all-read-consistency and non-interference}},
 booktitle = {13th International Conference on Distributed Computing and Networking},
 year = {2012},
 location = {Bangalore, Canada},
 }



@inproceedings{Guer+:disc1:2008, author = {Rachid Guerraoui and Thomas A. Henzinger and Vasu Singh}, title = {Permissiveness in Transactional Memories}, booktitle = {DISC}, pages = {305--319}, year = {2008}, crossref = {DBLP:conf/wdag/2008}, url = {https://doi.org/10.1007/978-3-540-87779-0\_21}, doi = {10.1007/978-3-540-87779-0\_21}, timestamp = {Tue, 13 Jun 2017 10:37:55 +0200}, biburl = {https://dblp.org/rec/bib/conf/wdag/GuerraouiHS08}, bibsource = {dblp computer science bibliography, https://dblp.org} }

@inproceedings{Crain+:RI_VWC:ICA3PP:2011, author = {Tyler Crain and Damien Imbs and Michel Raynal}, title = {Read Invisibility, Virtual World Consistency and Probabilistic Permissiveness are Compatible}, booktitle = {ICA3PP}, pages = {244--257}, year = {2011}, crossref = {DBLP:conf/ica3pp/2011-1}, url = {https://doi.org/10.1007/978-3-642-24650-0\_21}, doi = {10.1007/978-3-642-24650-0\_21}, timestamp = {Sun, 11 Mar 2018 01:37:22 +0100}, biburl = {https://dblp.org/rec/bib/conf/ica3pp/CrainIR11}, bibsource = {dblp computer science bibliography, https://dblp.org} }

@InProceedings{Baretto+:PPoPP:2010,
   address     = { },
   affiliation = {EPFL},
   author      = {Baretto, Joao and Dragojevic, Aleksandar and Ferreira,
                 Paulo and Guerraoui, Rachid and Kapalka, Michal},
   booktitle   = {Proceedings of the 15th {ACM} {SIGPLAN} symposium on
                 {P}rinciples and {P}ractice of {P}arallel {C}omputing},
   details     = {http://infoscience.epfl.ch/record/144050},
   documenturl = {http://infoscience.epfl.ch/getfile.py?recid=144050&mode=best},
   doi         = {10.1145/1693453.1693466},
   keywords    = {Nested parallel programs; Fork-join; Work-stealing; Transactional memory},
   location    = {Bangalore, India},
   pages       = {91--100},
   publisher   = {ACM},
   review      = {REVIEWED},
   series      = { },
   status      = {PUBLISHED},
   title       = {{Leveraging {P}arallel {N}esting in {T}ransactional {M}emory}},
   unit        = {LPD},
   url         = { },
   year        = 2010
}

@InProceedings{RanVid:Tran:2011,
	author = {Ranjeet Kumar and Krishnamurthy Vidyasankar},
	booktitle = {TRANSACT 2011},
	title = {{HParSTM: A Hierarchy-based STM Protocol for Supporting Nested Parallelism}},
	month = {June},
	year = {2011}
}

@Article{RaviSat:IJCCT:2012,
	title = {{A Correctness Criterion for Eager Approach Validation for Transactional Memory System}},
	year = {2012},
	pages = {43-49},
	author = {Ravi Kumar and Sathya Peri},
	volume = {3},
	journal = {International Journal of Computer and Communication Technology (IJCCT)},
	number = {2}
}

@article{KuzSat:Corr:2012,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{On Non-Interference of Transactions}},
  journal   = {CoRR},
  volume    = {abs/1211.6315},
  year      = {2012},
  ee        = {http://arxiv.org/abs/1211.6315},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Bernstein+:MCC:TDS:1983,
 author = {Bernstein, Philip A. and Goodman, Nathan},
 title = {{{M}ultiversion {C}oncurrency {C}ontrol: {T}heory and {A}lgorithms}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {Dec. 1983},
 volume = {8},
 number = {4},
 month = dec,
 year = {1983},
 issn = {0362-5915},
 pages = {465--483},
 numpages = {19},
 url = {http://doi.acm.org/10.1145/319996.319998},
 doi = {10.1145/319996.319998},
 acmid = {319998},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transaction processing},
}
 
@Article{CachRito:2006:CP,
	title = {{{V}ersioned {B}oxes as the basis for {M}emory {T}ransactions}},
	year = {2006},
	number = {2},
	author = {J. Cachopo and A. Rito-Silva},
	pages = {172--185},
	journal = {Science of Computer Programming},
	volume = {63}
}

@inproceedings{AydAbd:2008:Serial:transact,
  author	= {Aydonat, Utku and Abdelrahman, Tarek},
  title		= {{Serializability of {T}ransactions in {S}oftware {T}ransactional {M}emory}},
  booktitle	= {TRANSACT~'08: 3rd Workshop on Transactional Computing},
  pdf		= {http://www.unine.ch/transact08/papers/Aydonat-Serializability.pdf},
  year		= {2008},
  month		= {feb},
}

@article{PapadKanel:1984:MultVer:TDS,
 author = {Papadimitriou, Christos H. and Kanellakis, Paris C.},
 title = {{On Concurrency Control by Multiple Versions}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {March 1984},
 volume = {9},
 number = {1},
 month = mar,
 year = {1984},
 issn = {0362-5915},
 pages = {89--99},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/348.318588},
 doi = {10.1145/348.318588},
 acmid = {318588},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Perel+:2011:SMV:DISC,
  author    = {Dmitri Perelman and
               Anton Byshevsky and
               Oleg Litmanovich and
               Idit Keidar},
  title     = {{SMV}: {S}elective {M}ulti-{V}ersioning {STM}},
  booktitle = {DISC},
  year      = {2011},
  pages     = {125-140},
  ee        = {http://dx.doi.org/10.1007/978-3-642-24100-0_9},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{herlihy+:2003:stm-dynamic:podc,
  author	= {Herlihy, Maurice and Luchangco, Victor and Moir, Mark and {William N. Scherer}, III},
  title		= {{Software Transactional Memory for Dynamic-Sized Data Structures}},
  booktitle	= {PODC~'03: Proc. 22nd ACM Symposium on Principles of Distributed Computing},
  pages		= {92--101},
  month		= {Jul},
  urlpage	= {http://doi.acm.org/10.1145/872035.872048},
  year		= {2003},
}

@inproceedings{dice:2006:tl2:disc,
  author	= {Dice, Dave and Shalev, Ori and Shavit, Nir},
  title		= {{Transactional Locking II}},
  booktitle	= {DISC~'06: Proc. 20th International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 4167},
  pages		= {194--208},
  year		= {2006},
  month		= {sep},
}

@inproceedings{perel+:2010:MultVer:PODC,
  author    = {Dmitri Perelman and Rui Fan and Idit Keidar},
  title     = {{{O}n {M}aintaining {M}ultiple {V}ersions in {STM}}},
  booktitle = {PODC},
  year      = {2010},
  pages     = {16-25},
  ee        = {http://doi.acm.org/10.1145/1835698.1835704},
}

@incollection{riegel+:2006:LSA:DISC,
  author	= {Riegel, Torvald and Felber, Pascal and Fetzer, Christof},
  editor	= {},
  title		= {{A {L}azy {S}napshot {A}lgorithm with {E}ager {V}alidation}},
  booktitle	= {Proceedings of the 20th International Symposium on Distributed Computing, {DISC} 2006},
  publisher	= {Springer},
  month		= {Sep},
  year		= {},
  volume	= {4167},
  isbn		= {3-540-44624-9},
  pages		= {284--298},
  series	= {Lecture Notes in Computer Science},
  urlpage	= {http://dx.doi.org/10.1007/11864219_20}
}

@inproceedings{riegel+:sistm:transact:2006,
  author	= {Riegel, Torvald and Fetzer, Christof and Felber, Pascal},
  booktitle	= {Proceedings of the First ACM SIGPLAN Workshop on Languages, Compilers, and Hardware Support for Transactional Computing},
  month		= {Jun},
  title		= {{Snapshot Isolation for Software Transactional Memory }},
  year		= {2006}
}

@article{attiyaHill:sinmvperm:tcs:2012,
  author    = {Hagit Attiya and
               Eshcar Hillel},
  title     = {{A {S}ingle-{V}ersion {STM} that is {M}ulti-{V}ersioned {P}ermissive}},
  journal   = {Theory Comput. Syst.},
  volume    = {51},
  number    = {4},
  year      = {2012},
  pages     = {425-446},
  ee        = {http://dx.doi.org/10.1007/s00224-012-9406-3},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{prisat:mvto:corr:2013,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{A TimeStamp based Multi-version STM Protocol that satisfies
               Opacity}},
  journal   = {CoRR},
  volume    = {abs/1305.6624},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1305.6624},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Fern+:LSMVSTM:PPoPP:2011,
 author = {Fernandes, S{\'e}rgio Miguel and Cachopo, Joao},
 title = {{Lock-free and {S}calable {M}ulti-version {S}oftware {T}ransactional {M}emory}},
 booktitle = {},
 series = {PPoPP '11},
 year = {2011},
 isbn = {978-1-4503-0119-0},
 location = {San Antonio, TX, USA},
 pages = {},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1941553.1941579},
 doi = {10.1145/1941553.1941579},
 acmid = {1941579},
 publisher = {},
 address = {New York, NY, USA},
 keywords = {garbage collection, lock-free synchronization, multi-version concurrency control, transactional memory},
} 

@Article{LuScott:UMV:Transact:2012,
	journal = {Transact},
	title = {{Unmanaged Multiversion STM}},
	year = {2012},
	author = {Li Lu and Michael L. Scott}
}

@inproceedings{SinhaMalik:RuntimeSee:IPDPS:2010,
  author    = {Arnab Sinha and
               Sharad Malik},
  title     = {{Runtime checking of serializability in software transactional
               memory}},
  booktitle = {IPDPS},
  year      = {2010},
  pages     = {1-12},
  ee        = {http://dx.doi.org/10.1109/IPDPS.2010.5470389},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{HadzPapad:AAMVCC:PODS:1985,
 author = {Hadzilacos, Thanasis and Papadimitriou, Christos H.},
 title = {{Algorithmic aspects of multiversion concurrency control}},
 booktitle = {Proceedings of the fourth ACM SIGACT-SIGMOD symposium on Principles of database systems},
 series = {PODS '85},
 year = {1985},
 isbn = {0-89791-153-9},
 location = {Portland, Oregon, USA},
 pages = {96--104},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/325405.325417},
 doi = {10.1145/325405.325417},
 acmid = {325417},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{KuznetsovPeri:Non-interference:TCS:2017,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{Non-interference and local correctness in transactional memory}},
  journal   = {Theor. Comput. Sci. 2017},
  volume    = {},
  pages     = {},
  year      = {},
  url       = {},
  doi       = {},
  timestamp = {Tue, 04 Jul 2017 17:27:30 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/tcs/KuznetsovP17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Kumar+:MVTO:ICDCN:2014,
  author    = {Priyanka Kumar and
               Sathya Peri and
               K. Vidyasankar},
  title     = {{A TimeStamp Based Multi-version STM Algorithm}},
  booktitle = {ICDCN},
  year      = {2014},
  pages     = {},
  ee        = {http://dx.doi.org/10.1007/978-3-642-45249-9_14},
  crossref  = {DBLP:conf/icdcn/2014},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@book{Har+:TMBook:2010,
  author    = {Tim Harris and
               James R. Larus and
               Ravi Rajwar},
  title     = {{Transactional Memory, 2nd edition}},
  booktitle = {Transactional Memory (2.ed.)},
  publisher = {Morgan {\&} Claypool Publishers},
  series    = {Synthesis Lectures on Computer Architecture},
  year      = {2010},
  ee        = {http://dx.doi.org/10.2200/S00272ED1V01Y201006CAC011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{OluHamm:MicroBook:Queue:2005,
 author = {Olukotun, Kunle and Hammond, Lance},
 title = {{The Future of Microprocessors}},
 journal = {Queue},
 issue_date = {September 2005},
 volume = {3},
 number = {7},
 month = sep,
 year = {2005},
 issn = {1542-7730},
 pages = {26--29},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1095408.1095418},
 doi = {10.1145/1095408.1095418},
 acmid = {1095418},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@book{HerlihyShavit:AMP:Book:2012,
	author = {Herlihy, Maurice and Shavit, Nir},
	title = {The Art of Multiprocessor Programming, Revised Reprint},
	year = {2012},
	isbn = {9780123973375, 9780123977953},
	edition = {1st},
	publisher = {Morgan Kaufmann Publishers Inc.},
	address = {San Francisco, CA, USA},
} 

@inproceedings{HerlihyShavit:Progress:Opodis:2011,
	author = {Herlihy, Maurice and Shavit, Nir},
	title = {On the Nature of Progress},
	booktitle = {},
	series = {OPODIS 2011},
	year = {},
	isbn = {978-3-642-25872-5},
	location = {Toulouse, France},
	pages = {},
	numpages = {16},
	url = {},
	doi = {},
	acmid = {2183558},
	publisher = {},
	address = {},
} 

@inproceedings{Harris:NBList:DISC:2001,
	author    = {Timothy L. Harris},
	title     = {A Pragmatic Implementation of Non-blocking Linked-Lists},
	booktitle = {DISC},
	pages     = {},
	year      = {2001},
	
	timestamp = {Fri, 26 May 2017 14:09:14 +0200},
	biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/wdag/Harris01},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Herlihy:WaitFree:1991,
  title={{Wait-free synchronization}},
  author={Herlihy, Maurice},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={13},
  number={1},
  pages={124--149},
  year={1991},
  publisher={ACM}
}

@INPROCEEDINGS{Attiya+:DUOp:ICDCS:2013,
author={Attiya, H. and Hans, S. and Kuznetsov, P. and Ravi, S.},
booktitle={Distributed Computing Systems (ICDCS), 2013 IEEE 33rd International Conference on},
title={{Safety of Deferred Update in Transactional Memory}},
year={2013},
month={July},
pages={601-610},
keywords={concurrency control;transaction processing;committed transactions;deferred update safety;deferred-update semantics;opacityc riterion;prefix serializations;sequential execution;sequential order;speculative transactions;transactional memory;unique-write assumption;History;Law;Real-time systems;Safety;Semantics;Silicon;Limit-closure;Safety;Transactional Memory},
doi={10.1109/ICDCS.2013.57},
ISSN={1063-6927},}

@article{PriSat:MVC:Corr:2015,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{Multi-Version Conflict Notion}},
  journal   = {CoRR},
  volume    = {abs/1307.8256},
  year      = {2013},
  url       = {http://arxiv.org/abs/1307.8256},
  timestamp = {Thu, 15 Aug 2013 15:30:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KumarP13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Attiya+:TMS:DISC:2014,
  author    = {Hagit Attiya and
               Alexey Gotsman and
               Sandeep Hans and
               Noam Rinetzky},
  title     = {{Safety of Live Transactions in Transactional Memory: {TMS} is Necessary
               and Sufficient}},
  booktitle = {Distributed Computing - 28th International Symposium, {DISC} 2014,
               Austin, TX, USA, October 12-15, 2014. Proceedings},
  pages     = {376--390},
  year      = {2014},
  crossref  = {DBLP:conf/wdag/2014},
  url       = {http://dx.doi.org/10.1007/978-3-662-45174-8_26},
  doi       = {10.1007/978-3-662-45174-8_26},
  timestamp = {Tue, 30 Sep 2014 10:44:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/AttiyaGHR14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Herlihy:WFS:TPLS:1991,
 author = {Herlihy, Maurice},
 title = {{Wait-free Synchronization}},
 journal = {ACM Trans. Program. Lang. Syst.},
 issue_date = {Jan. 1991},
 volume = {13},
 number = {1},
 month = jan,
 year = {1991},
 issn = {0164-0925},
 pages = {124--149},
 numpages = {26},
 url = {http://doi.acm.org/10.1145/114005.102808},
 doi = {10.1145/114005.102808},
 acmid = {102808},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {linearization, wait-free synchronization},
} 



@inproceedings{LuScott:GMV:DISC:2013,
  author    = {Li Lu and
               Michael L. Scott},
  title     = {{Generic Multiversion {STM}}},
  booktitle = {DISC},
  pages     = {134--148},
  year      = {2013},
  crossref  = {DBLP:conf/wdag/2013},
  url       = {http://dx.doi.org/10.1007/978-3-642-41527-2_10},
  doi       = {10.1007/978-3-642-41527-2_10},
  timestamp = {Mon, 28 Oct 2013 18:03:50 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/LuS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{CachAnt:VBoxes:SCOOL:2005,
  author	= {Cachopo, Joao and Rito-Silva, Antonio},
  title		= {{Versioned Boxes as the Basis for Memory Transactions}},
  booktitle	= {OOPSLA 2005 Workshop on Synchronization and Concurrency in Object-Oriented Languages (SCOOL)},
  urlpage	= {http://hdl.handle.net/1802/2101},
  year		= {2005},
  month		= {oct},
}

@article{Thomas:TWR:TDS:1979,
 author = {Thomas, Robert H.},
 title = {{A Majority Consensus Approach to Concurrency Control for Multiple Copy Databases}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {June 1979},
 volume = {4},
 number = {2},
 month = jun,
 year = {1979},
 issn = {0362-5915},
 pages = {180--209},
 numpages = {30},
 url = {http://doi.acm.org/10.1145/320071.320076},
 doi = {10.1145/320071.320076},
 acmid = {320076},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {clock synchronization, computer networks, concurrency control, distributed computation, distributed control, distributed databases, multiprocess systems, update synchronization},
} 

@inproceedings{Gramoli+:OptListSet:DISC-BA:2015,
  TITLE = {{Brief Announcement: A Concurrency-Optimal List-Based Set}},
  AUTHOR = {Gramoli, Vincent and Kuznetsov, Petr and Ravi, Srivatsan and Shang, Di},
  URL = {https://hal.archives-ouvertes.fr/hal-01207872},
  BOOKTITLE = {{DISC 2015}},
  ADDRESS = {Tokyo, Japan},
  ORGANIZATION = {{Toshimitsu Masuzawa and Koichi Wada}},
  EDITOR = {Yoram Moses and Matthieu Roy},
  PUBLISHER = {{Springer-Verlag Berlin Heidelberg}},
  SERIES = {29th International Symposium on Distributed Computing},
  VOLUME = {LNCS 9363},
  YEAR = {2015},
  MONTH = Oct,
  PDF = {https://hal.archives-ouvertes.fr/hal-01207872/file/37-BA.pdf},
  HAL_ID = {hal-01207872},
  HAL_VERSION = {v1},
}

@article{Gramoli+:OptListSet:CoRR:2015,
  author    = {Vincent Gramoli and
               Petr Kuznetsov and
               Srivatsan Ravi and
               Di Shang},
  title     = {{A Concurrency-Optimal List-Based Set}},
  journal   = {CoRR},
  volume    = {abs/1502.01633},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.01633},
  timestamp = {Mon, 02 Mar 2015 14:17:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GramoliKRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Heller+:LazyList:PPL:2007,
  author    = {Steve Heller and
               Maurice Herlihy and
               Victor Luchangco and
               Mark Moir and
               William N. Scherer III and
               Nir Shavit},
  title     = {{A Lazy Concurrent List-Based Set Algorithm}},
  journal   = {Parallel Processing Letters},
  volume    = {17},
  number    = {4},
  pages     = {411-424},
  year      = {2007},
  url       = {},
  doi       = {},
  timestamp = {Mon, 23 Jun 2008 13:43:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ppl/HellerHLMSS07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Ziv+:Composing:POPL:2015,
  title={{Composing Concurrency Control}},
  author={Ziv, Ofri and Aiken, Alex and Golan-Gueta, Guy and Ramalingam, G and Sagiv, Mooly},
  booktitle={Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
  pages={240--249},
  year={2015},
  organization={ACM}
}

@article{marathe2004qualitative,
  title={{A qualitative survey of modern software transactional memory systems}},
  author={Marathe, Virendra J and Scott, Michael L},
  journal={University of Rochester Computer Science Dept., Tech. Rep},
  year={2004}
}

@inproceedings{Vafeiadis:2006:PCH:1122971.1122992,
 author = {Vafeiadis, Viktor and Herlihy, Maurice and Hoare, Tony and Shapiro, Marc},
 title = {{Proving Correctness of Highly-concurrent Linearisable Objects}},
 booktitle = {PPoPP},
 series = {},
 year = {2006},
 isbn = {1-59593-189-9},
 location = {},
 pages = {129--136},
 numpages = {8},
 url = {},
 doi = {},
 acmid = {1122992},
 publisher = {},
 address = {},
 keywords = {concurrent programming, formal verification, linearisability, rely-guarantee reasoning, shared-memory concurrency},
}


@techreport{marathe:stm-survey:urcs-tr:2004,
  author	= {Marathe, Virendra J. and Scott, Michael L.},
  title		= {{A Qualitative Survey of Modern Software Transactional Memory Systems}},
  number	= {TR 839},
  institution	= {University of Rochester Computer Science Dept.},
  month		= {Jun},
  year		= {2004},
  pdf		= {http://www.cs.rochester.edu/u/scott/papers/2004_TR839.pdf}
}

@phdthesis{Fraser:PracticalLF:2004,
  title={{Practical lock-freedom}},
  author={Fraser, Keir},
  year={2004},
  school={University of Cambridge}
}

@inproceedings{Herlihy+:STM-DynamicSize:PODC:2003,
  title={{Software transactional memory for dynamic-sized data structures}},
  author={Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer III, William N},
  booktitle={Proceedings of the twenty-second annual symposium on Principles of distributed computing},
  pages={92--101},
  year={2003},
  organization={ACM}
}
@inproceedings{Marathe+:STM-Tradeoff:LCRS:2004,
  title={{Design tradeoffs in modern software transactional memory systems}},
  author={Marathe, Virendra J and Scherer, William N and Scott, Michael L},
  booktitle={Proceedings of the 7th workshop on Workshop on languages, compilers, and run-time support for scalable systems},
  pages={1--7},
  year={2004},
  organization={ACM}
}

@article{Barghouti:1991:CCA:116873.116875,
 author = {Barghouti, Naser S. and Kaiser, Gail E.},
 title = {{Concurrency Control in Advanced Database Applications}},
 journal = {ACM Comput. Surv.},
 issue_date = {Sept. 1991},
 volume = {23},
 number = {3},
 month = sep,
 year = {1991},
 issn = {0360-0300},
 pages = {269--317},
 numpages = {49},
 url = {http://doi.acm.org/10.1145/116873.116875},
 doi = {10.1145/116873.116875},
 acmid = {116875},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {advanced database applications, concurrency control, cooperative transactions, design environments, extended transaction models, long transactions, object-oriented databases, relaxing serializability},
}

@article{Beeri+:Nested:JACM:1989,
 author = {Beeri, Catriel and Bernstein, Philip A. and Goodman, Nathan},
 title = {{A Model for Concurrency in Nested Transactions Systems}},
 journal = {J. ACM},
 issue_date = {April 1989},
 volume = {36},
 number = {2},
 month = apr,
 year = {1989},
 issn = {0004-5411},
 pages = {230--269},
 numpages = {40},
 url = {http://doi.acm.org/10.1145/62044.62046},
 doi = {10.1145/62044.62046},
 acmid = {62046},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{HerlihyKosk:Boosting:PPoPP:2008,
	author    = {Maurice Herlihy and
	Eric Koskinen},
	title     = {Transactional boosting: a methodology for highly-concurrent transactional
	objects},
	booktitle = {{PPOPP}},
	pages     = {},
	year      = {2008},
	crossref  = {DBLP:conf/ppopp/2008},
	url       = {http://doi.acm.org/10.1145/1345206.1345237},
	doi       = {10.1145/1345206.1345237},
	timestamp = {Tue, 22 May 2012 15:24:56 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/ppopp/HerlihyK08},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Hassan+:OptBoost:PPoPP:2014,
	author    = {Ahmed Hassan and
	Roberto Palmieri and
	Binoy Ravindran},
	title     = {{Optimistic transactional boosting}},
	booktitle = {PPoPP},
	pages     = {},
	year      = {2014},
	crossref  = {DBLP:conf/ppopp/2014},
	url       = {},
	doi       = {},
	timestamp = {Sun, 03 Jul 2016 16:10:52 +0200},
	biburl    = {http://dblp.dagstuhl.de/rec/bib/conf/ppopp/HassanPR14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Hassan:OptTransLazy:Opodis:2014,
	title={{On developing optimistic transactional lazy set}},
	author={Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
	booktitle={OPODIS},
	pages={437--452},
	year={2014},
	organization={Springer}
}

@inproceedings{Spiegelman+:TransDS:PLDI:2016,
	title={{Transactional data structure libraries}},
	author={Spiegelman, Alexander and Golan-Gueta, Guy and Keidar, Idit},
	booktitle={PLDI},
	pages={682--696},
	year={2016},
	organization={ACM}
}

@article{Anand+:CaPRa:Corr:2015,
  author    = {Anshu S. Anand and
               R. K. Shyamasundar and
               Sathya Peri},
  title     = {{Opacity Proof for CaPR+ Algorithm}},
  journal   = {CoRR},
  volume    = {abs/1510.06967},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.06967},
  timestamp = {Sun, 01 Nov 2015 17:30:45 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AnandSP15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Lev-Ari+:OnCorrectness:DISC:2014,
	author    = {Kfir Lev{-}Ari and
	Gregory V. Chockler and
	Idit Keidar},
	title     = {{On Correctness of Data Structures under Reads-Write Concurrency}},
	booktitle = {DISC},
	pages     = {273--287},
	year      = {2014},
	crossref  = {DBLP:conf/wdag/2014},
	url       = {},
	doi       = {},
	timestamp = {Fri, 19 May 2017 01:25:17 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/Lev-AriCK14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Lev-Ari+:ConsApproachLinz:DISC:2015,
	author = {Lev-Ari, Kfir and Chockler, Gregory V and Keidar, Idit},
	booktitle = {DISC},
	doi = {},
	editor = {Moses, Yoram},
	isbn = {978-3-662-48652-8},
	pages = {356--370},
	publisher = {Springer},
	series = {},
	title = {{A Constructive Approach for Proving Data Structures' Linearizability}},
	url = {},
	volume = {},
	year = {2015}
}

@article{zhang2016high,
  title={{High-Performance Composable Transactional Data Structures}},
  author={Zhang, Deli},
  year={2016}
}

@techreport{zhang2010composability,
  author={Zhang, Rui and Budimli{\'c}, Zoran and Scherer III, William N},
  title={{Composability for application-specific transactional optimizations}},
  institution={Department of Computer Science, Rice University},
  year={2010}
}

@article{DBLP:journals/corr/abs-0910-0366,
  author    = {Daniel Cederman and
               Philippas Tsigas},
  title     = {{Supporting Lock-Free Composition of Concurrent Data Objects}},
  journal   = {CoRR},
  volume    = {abs/0910.0366},
  year      = {2009},
  url       = {},
  timestamp = {Wed, 07 Jun 2017 14:40:49 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/corr/abs-0910-0366},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Hassan2015,
author = {Hassan, Ahmed and Wang, Chao and Broadwater, Robert P},
mendeley-groups = {PhD Thesis},
title = {{Designing , Modeling , and Optimizing Transactional Data Structures}},
year = {2015}
}

@article{harris2007abstract,
	title={{Abstract nested transactions}},
	author={Harris, Tim and others},
	year={2007},
	publisher={Citeseer}
}


@inproceedings{Peri+:OSTM:Netys:2018,
	author = {Sathya Peri and
	Ajay Singh and
	Archit Somani},
	title = {{Efficient means of Achieving Composability using Transactional Memory}},
	booktitle = {},
	series = {NETYS '18},
	year = {2018},
	isbn = {978-1-4503-4210-0},
	keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@article{Felber+:ElasticTrans:2017:jpdc,
 author = {Felber, Pascal and Gramoli, Vincent and Guerraoui, Rachid},
 title = {{Elastic Transactions}},
 journal = {J. Parallel Distrib. Comput.},
 issue_date = {February 2017},
 volume = {100},
 number = {C},
 month = feb,
 year = {2017},
 issn = {0743-7315},
 pages = {},
 numpages = {25},
 url = {https://doi.org/10.1016/j.jpdc.2016.10.010},
 doi = {10.1016/j.jpdc.2016.10.010},
 acmid = {3066828},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Concurrent data structures, Transactional memory},
} 


@inproceedings{ZhangDech:LockFreeTW:SPAA:2016,
 author = {Zhang, Deli and Dechev, Damian},
 title = {{Lock-free Transactions Without Rollbacks for Linked Data Structures}},
 booktitle = {},
 series = {SPAA '16},
 year = {2016},
 isbn = {978-1-4503-4210-0},
 location = {Pacific Grove, California, USA},
 pages = {},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2935764.2935780},
 doi = {10.1145/2935764.2935780},
 acmid = {2935780},
 publisher = {},
 address = {New York, NY, USA},
 keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@inproceedings{Dalessandro+:NoRec:PPoPP:2010,
  added-at = {2010-01-19T00:00:00.000+0100},
  author = {Dalessandro, Luke and Spear, Michael F. and Scott, Michael L.},
  biburl = {https://www.bibsonomy.org/bibtex/2bb4ff560750c574e33fceb87457d3cce/dblp},
  booktitle = {PPOPP},
  crossref = {conf/ppopp/2010},
  editor = {Govindarajan, R. and Padua, David A. and Hall, Mary W.},
  ee = {http://doi.acm.org/10.1145/1693453.1693464},
  interhash = {65ad98c6f111ce3b454219b4fd45ebb8},
  intrahash = {bb4ff560750c574e33fceb87457d3cce},
  isbn = {978-1-60558-877-3},
  keywords = {dblp},
  pages = {},
  publisher = {ACM},
  timestamp = {2012-05-23T11:41:17.000+0200},
  title = {{NOrec: Streamlining STM by Abolishing Ownership Records}},
  url = {http://dblp.uni-trier.de/db/conf/ppopp/ppopp2010.html#DalessandroSS10},
  year = 2010
}



@online{ethereum,
	author    = {Ethereum},
	url       = {http://github.com/ethereum}
}

@misc{Nakamoto:Bitcoin:2009,
	added-at = {2014-04-17T08:33:06.000+0200},
	author = {Nakamoto, Satoshi},
	biburl = {https://www.bibsonomy.org/bibtex/23db66df0fc9fa2b5033f096a901f1c36/ngnn},
	interhash = {423c2cdff70ba0cd0bca55ebb164d770},
	intrahash = {3db66df0fc9fa2b5033f096a901f1c36},
	keywords = {imported},
	timestamp = {2014-04-17T08:33:06.000+0200},
	title = {Bitcoin: A peer-to-peer electronic cash system},
	url = {http://www.bitcoin.org/bitcoin.pdf},
	year = 2009
}

@inproceedings{Dickerson+:ACSC:PODC:2017,
	author = {Dickerson, Thomas and Gazzillo, Paul and Herlihy, Maurice and Koskinen, Eric},
	title = {Adding Concurrency to Smart Contracts},
	booktitle = {},
	series = {PODC '17},
	year = {},
	isbn = {978-1-4503-4992-5},
	location = {Washington, DC, USA},
	pages = {},
	numpages = {10},
	url = {},
	doi = {},
	acmid = {3087835},
	publisher = {},
	address = {},
	keywords = {blockchain, concurrency, ethereum, fork-join, miners, smart contracts, validators},
} 


@inproceedings{SergeyandHobor:ACP:2017,
	title={A Concurrent Perspective on Smart Contracts},
	author={Ilya Sergey and Aquinas Hobor},
	booktitle={Financial Cryptography Workshops},
	year={2017}
}

@InProceedings{ZangandZang:ECSC:WBD:2018,
	author="Zhang, An
	and Zhang, Kunlong",
	editor="Cai, Yi
	and Ishikawa, Yoshiharu
	and Xu, Jianliang",
	title="Enabling Concurrency on Smart Contracts Using Multiversion Ordering",
	booktitle="Web and Big Data",
	year="2018",
	publisher="",
	address="Cham",
	pages="425--439",
	abstract="Blockchain-based platforms, such as Ethereum, allow transactions in blocks to call user-defined scripts named smart contracts. In the blockchain network, after being generated by a miner, a block will be validated many times by the peers who accept it. Hence by enabling concurrency on smart contracts, especially validation, we can improve the efficiency and the throughput of those platforms.",
	isbn="978-3-319-96893-3"
}


@article{Nick:PublicN:journals:1997, 
	author = {Nick Szabo}, 
	title = {Formalizing and Securing Relationships on Public Networks}, 
	journal = {First Monday}, 
	volume = {2}, number = {9}, year = {1997} } 

@inproceedings{Luu+:DIC:CCS:2015, 
	author = {Luu, Loi and Teutsch, Jason and Kulkarni, Raghav and Saxena, Prateek}, title = {Demystifying Incentives in the Consensus Computer}, booktitle = {Proceedings of the 22Nd ACM SIGSAC Conference on Computer and Communications Security}, series = {CCS '15}, year = {2015}, isbn = {978-1-4503-3832-5}, location = {Denver, Colorado, USA}, pages = {706--719}, numpages = {14}, url = {}, doi = {}, acmid = {2813659}, publisher = {ACM}, address = {New York, NY, USA}, keywords = {bitcoin, consensus computer, cryptocurrency, ethereum, incentive compatibility, verifiable computation}, }

@online{Solidity,
	author    = {Solidity documentation},
	url       = {http://solidity.readthedocs.io/en/latest/index.html}
}


@inproceedings{Luu+:MSC:CCS:2016,
	author = {Luu, Loi and Chu, Duc-Hiep and Olickel, Hrishi and Saxena, Prateek and Hobor, Aquinas},
	title = {Making Smart Contracts Smarter},
	booktitle = {CCS '16},
	series = {},
	year = {},
	isbn = {978-1-4503-4139-4},
	location = {Vienna, Austria},
	pages = {},
	numpages = {16},
	url = {},
	doi = {},
	acmid = {2978309},
	publisher = {},
	address = {},
	keywords = {blockchain, cryptocurrencies, ethereum, smart contract, symbolic execution},
} 

@inproceedings{Delmolino+:SSTCSC:FC:2016,
	author    = {Kevin Delmolino and
	Mitchell Arnett and
	Ahmed E. Kosba and
	Andrew Miller and
	Elaine Shi},
	title     = {Step by Step Towards Creating a Safe Smart Contract: Lessons and Insights
	from a Cryptocurrency Lab},
	booktitle = {Financial Cryptography and Data Security - {FC} 2016 International
	Workshops, BITCOIN, VOTING, and WAHC, Christ Church, Barbados, February
	26, 2016.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/fc/2016w},
	url       = {},
	doi       = {},
	timestamp = {Wed, 30 May 2018 16:11:58 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/fc/DelmolinoAKMS16},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{HerlihyandWing:1990:LCC:ACM,
	author = {Herlihy, Maurice P. and Wing, Jeannette M.},
	title = {Linearizability: A Correctness Condition for Concurrent Objects},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {July 1990},
	volume = {12},
	number = {3},
	month = jul,
	year = {1990},
	issn = {0164-0925},
	pages = {463--492},
	numpages = {30},
	url = {},
	doi = {},
	acmid = {78972},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{DBLP:journals/corr/abs-1809-01326,
  author    = {Parwat Singh Anjana and
               Sweta Kumari and
               Sathya Peri and
               Sachin Rathor and
               Archit Somani},
  title     = {An Efficient Framework for Concurrent Execution of Smart Contracts},
  journal   = {CoRR},
  volume    = {abs/1809.01326},
  year      = {2018},
  url       = {http://arxiv.org/abs/1809.01326},
  archivePrefix = {arXiv},
  eprint    = {1809.01326},
  timestamp = {Fri, 05 Oct 2018 11:34:52 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1809-01326},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{Bushkov+:Live-TM:PODC:2012,
	author    = {Victor Bushkov and Rachid Guerraoui and Michal Kapalka},
	title     = {On the liveness of transactional memory},
	booktitle = {PODC'12.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/podc/2012},
	url       = {http://doi.acm.org/10.1145/2332432.2332435},
	doi       = {10.1145/2332432.2332435},
	timestamp = {Sun, 15 Jul 2012 18:49:17 +0200},
	biburl    = {http://dblp.org/rec/bib/conf/podc/BushkovGK12},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Gramoli+:TM2C:Eurosys:2012,
	author = {Gramoli, Vincent and Guerraoui, Rachid and Trigonakis, Vasileios},
	title = {{TM2C: A Software Transactional Memory for Many-cores}},
	booktitle = {},
	series = {EuroSys 2012},
	year = {2012},
	isbn = {978-1-4503-1223-3},
	location = {Bern, Switzerland},
	pages = {},
	numpages = {14},
	url = {},
	doi = {},
	acmid = {2168872},
	publisher = {},
	address = {},
	keywords = {concurrent programming, contention management, many-cores, transactional memory},
} 


@article{WaliSten:Starve:CC:2009,
	author    = {M. M. Waliullah and
	Per Stenstr{\"{o}}m},
	title     = {{Schemes for Avoiding Starvation in Transactional Memory Systems}},
	journal   = {Concurrency and Computation: Practice and Experience},
	volume    = {},
	number    = {},
	pages     = {},
	year      = {2009},
	url       = {},
	doi       = {},
	timestamp = {Sat, 20 May 2017 00:25:18 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/concurrency/WaliullahS09},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@unknown{Spear+:CCM:PPoPP:2009,
author = {Spear, Michael F. and Dalessandro, Luke and Marathe, Virendra J. and Scott, Michael L.},
 title = {A Comprehensive Strategy for Contention Management in Software Transactional Memory},
 booktitle = {Proceedings of the 14th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '09},
 year = {2009},
 isbn = {978-1-60558-397-6},
 location = {Raleigh, NC, USA},
 pages = {141--150},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1504176.1504199},
 doi = {10.1145/1504176.1504199},
 acmid = {1504199},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {condition synchronization, contention management, inevitability, priority, software transactional memory},
} 


@inproceedings{Juyal+:SSS:2018,
	author    = {Chirag Juyal and
	Sandeep S. Kulkarni and
	Sweta Kumari and
	Sathya Peri and
	Archit Somani},
	title     = {An Innovative Approach to Achieve Compositionality Efficiently Using
	Multi-version Object Based Transactional Systems},
	booktitle = {{SSS'18}.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/sss/2018},
	url       = {https://doi.org/10.1007/978-3-030-03232-6\_19},
	doi       = {10.1007/978-3-030-03232-6\_19},
	timestamp = {Thu, 06 Dec 2018 00:00:00 +0100},
	biburl    = {https://dblp.org/rec/bib/conf/sss/JuyalKKPS18},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Chaudhary+:KSFTM:Corr:2017a,
	author    = {Ved Prakash Chaudhary and Chirag Juyal and Sandeep S. Kulkarni and Sweta Kumari and Sathya Peri},
	title     = {Achieving Starvation Freedom in Multi-Version Transactional Memory Systems},
	journal   = {CoRR},
	volume    = {abs/1709.01033},
	year      = {2017},
	url       = {http://arxiv.org/abs/1709.01033},
	archivePrefix = {arXiv},
	eprint    = {1709.01033},
	timestamp = {Thu, 06 Dec 2018 17:39:41 +0100},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1709-01033},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Chaudhary+:KSFTM:Corr:2017,
	author    = {Ved Prakash Chaudhary and Chirag Juyal and Sandeep S. Kulkarni and Sweta Kumari and Sathya Peri},
	title     = {Achieving Starvation Freedom in Multi-Version Transactional Memory Systems},
	journal   = {NETYS 2019},
	volume    = {},
	year      = {},
	url       = {},
	archivePrefix = {},
	eprint    = {},
	timestamp = {},
	biburl    = {},
	bibsource = {}
}

@inproceedings{Bobba:2007:PPH:1250662.1250674,
	author = {Bobba, Jayaram and Moore, Kevin E. and Volos, Haris and Yen, Luke and Hill, Mark D. and Swift, Michael M. and Wood, David A.},
	title = {Performance Pathologies in Hardware Transactional Memory},
	booktitle = {Proceedings of the 34th Annual International Symposium on Computer Architecture},
	series = {ISCA '07},
	year = {2007},
	isbn = {978-1-59593-706-3},
	location = {San Diego, California, USA},
	pages = {81--91},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1250662.1250674},
	doi = {10.1145/1250662.1250674},
	acmid = {1250674},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {contention management, hardware, pathology, performance, transactional memory},
} 

@MASTERSTHESIS{Erb2012, author = {Benjamin Erb}, title = {Concurrent Programming for Scalable Web Architectures}, school = {Institute of Distributed Systems, Ulm University}, year = {2012}, type = {Diploma Thesis}, keywords = {web, scalability, architecture, concurrency}, month = {April}, number = {VS-D01-2012}, url = {http://www.benjamin-erb.de/thesis} } 

@inproceedings{Riegel+:LSA:DISC:2006,
	author    = {Torvald Riegel and
	Pascal Felber and
	Christof Fetzer},
	title     = {A Lazy Snapshot Algorithm with Eager Validation},
	booktitle = {DISC 2006.},
	pages     = {},
	year      = {},
	crossref  = {DBLP:conf/wdag/2006},
	url       = {},
	doi       = {},
	timestamp = {Fri, 02 Jun 2017 13:01:06 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/RiegelFF06},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Juyal+:CORR:SF-MVOSTM:2019,
	author    = {Chirag Juyal and
	Sandeep S. Kulkarni and
	Sweta Kumari and
	Sathya Peri and
	Archit Somani},
	title     = {Obtaining Progress Guarantee and GreaterConcurrency in Multi-Version
	Object Semantics},
	journal   = {CoRR},
	volume    = {abs/1904.03700},
	year      = {2019},
	url       = {http://arxiv.org/abs/1904.03700},
	archivePrefix = {arXiv},
	eprint    = {1904.03700},
	timestamp = {Thu, 25 Apr 2019 13:55:01 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1904-03700},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

==> dsDesign.tex <==
\subsection{Data Structure and Design of SF-OSTM and SF-MVOSTM}
\label{subsec:dsde}



==> figs/dsDesign.tex <==
\subsection{Data Structure and Design of SF-OSTM and SF-MVOSTM}
\label{subsec:dsde}



==> figs/figures.tex <==
\section{Designated Figures}
\label{sec:figs}

\begin{figure}
	\centerline{\scalebox{0.5}{\input{figs/adv.pdf_t}}}
	\caption{Advantage of OSTMs over RWTSMs}
	\label{fig:adv}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/sostm.pdf_t}}}
	\caption{Advantage of SF-OSTM over OSTMs}
	\label{fig:sostm}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/advmvostm.pdf_t}}}
	\caption{Benefits of MVOSTM over Single version SF-OSTM}
	\label{fig:advmvostm}
\end{figure} 

\begin{figure}
	\centerline{\scalebox{0.45}{\input{figs/design.pdf_t}}}
	\caption{Data Structure and Design of SF-MVOSTM}
	\label{fig:advmvostm}
\end{figure} 


\begin{figure}
	\centering
	\begin{minipage}[b]{0.49\textwidth}
		\centering
		\captionsetup{justification=centering}
		\scalebox{.45}{\input{figs/stmore.pdf_t}}
		% \vspace{-16cm}
		\caption{Searching $k_9$ over \emph{lazy-list}}
		\label{fig:nostm2}
	\end{minipage}   
	\hfill
	\begin{minipage}[b]{0.49\textwidth}
		\scalebox{.45}{\input{figs/stless.pdf_t}}
		\centering
		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{Searching $k_9$ over $\lsl{}$}
		\label{fig:nostm}
	\end{minipage}
\end{figure}

==> figs/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

%\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}

%\newtheorem{definition}{Definition}

\newcounter{history}
\newcommand{\hist}[1]{\refstepcounter{history} {#1}}

%\newcommand{\proof}[1][]{\noindent{\bf\boldmath
 %                         P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------Theorem Notations Defined by Petr --------------------------------------------------------------------------------------------------------
%% Defined by Petr

%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{observation}[theorem]{Observation}


%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\insref}[1]{line~\ref{ins:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

\newcommand{\linref}[1]{Line~\ref{lin:#1}}
%\newcommand{\algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}
\newcommand{\algoref}[1]{{Algo~\ref{algo:#1}}}
\newcommand{\subsecref}[1]{SubSection{\ref{subsec:#1}}}

\newcommand{\histref}[1]{\ref{hist:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{eq(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}
\newcommand{\Confref}[1]{Conflict~\ref{conf:#1}}




\newcommand{\theqed}{$\Box$}


\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}


%------------------------------------------------------------------------------------------------------------------
% Definitions for Object STM paper
%------------------------------------------------------------------------------------------------------------------
%

\newcommand{\tobj} {t-object\xspace}
\newcommand{\txns}[1] {txns(#1)}
\newcommand {\comm}[1] {committed(#1)}
\newcommand {\aborted}[1] {aborted(#1)}
\newcommand {\incomp}[1] {incomp(#1)}
\newcommand {\live}[1] {live(#1)}
\newcommand {\term}[1] {term(#1)}
\newcommand {\key}[1] {key(#1)}
\newcommand {\confevt}[1] {conf-event(#1)}
\newcommand {\confmth}[1] {conf-method(#1)}
\newcommand {\conf}[1] {conflict(#1)}
\newcommand {\termn}[1] {terminate(#1)}

\newcommand {\tcomp} {t-complete\xspace}
\newcommand {\tinc} {t-incomplete\xspace}

\newcommand{\ssch} {sub-history}
\newcommand{\sschs} {sub-histories}

\newcommand{\nseq} {non-sequential}
\newcommand{\tseq} {t-sequential\xspace}
%\newcommand{\seq} {sequential}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}

\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\vwrite} {valWrite}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastup} {lastUpdt}
\newcommand{\lupdt}[2] {#2.lastUpdt(#1)}
\newcommand{\lseen}[2] {#2.lastSeen(#1)}

\newcommand{\mr} {MR}
\newcommand{\tr} {TR}

%\newcommand{\valid} {valid}
\newcommand{\validity} {validity\xspace}
\newcommand{\legal} {legal\xspace}
\newcommand{\legality} {legality\xspace}

\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}
%\newcommand{\rvmt} {rv\_method\xspace}
%\newcommand{\upmt} {upd\_method\xspace}
\newcommand{\rvp} {\emph{\rvmt execution} phase}
\newcommand{\cp} {\emph{\upmt execution} phase}

\newcommand{\termop} {terminal operation\xspace}
\newcommand{\cc} {correctness-criterion\xspace}
\newcommand{\ccs} {correctness-criteria\xspace}
\newcommand{\gen}[1] {gen(#1)}

\newcommand{\inv} {$inv$}
\newcommand{\rsp} {$rsp$}
\newcommand{\rmw} {rmw}
\newcommand{\first}[1] {first(#1)}
\newcommand{\last}[1] {last(#1)}

\newcommand{\evts}[1] {evts(#1)}
\newcommand{\met}[1] {methods(#1)}

\newcommand{\sgt} {SGT\xspace}
\newcommand{\memop} {memory operation\xspace}
\newcommand{\pref}[2] {#2.prefix(#1)}

\newcommand{\init} {\emph{init}\xspace}
\newcommand{\tbeg} {\emph{t\_begin}\xspace}
\newcommand{\tread} {\emph{t\_read}\xspace}
\newcommand{\twrite} {\emph{t\_write}\xspace}
\newcommand{\tins} {\emph{STM\_insert}\xspace}
\newcommand{\tdel} {\emph{STM\_delete}\xspace}
\newcommand{\tlook} {\emph{STM\_lookup}\xspace}
\newcommand{\tryc} {\emph{tryC}\xspace}%{\emph{tryC}}
\newcommand{\trya} {\emph{tryA}\xspace}%{\emph{tryA}}


\newcommand{\failed} {failed\xspace}
\newcommand{\unaborted} {unaborted\xspace}

%\newcommand{\ins} {\emph{list\_insert}}
%\newcommand{\del} {\emph{list\_del}}
%\newcommand{\look} {\emph{list\_lookup}}

\newcommand{\inss} {\emph{list\_insert}}
\newcommand{\dell} {\emph{list\_del}}
\newcommand{\lookk} {\emph{list\_lookup}}

\newcommand{\ins} {\emph{lsl\_ins}\xspace}
\newcommand{\del} {\emph{lsl\_del}\xspace}
\newcommand{\look} {\emph{lsl\_Search}\xspace}

\newcommand{\rv} {\emph{rv}}
\newcommand{\up} {\emph{up}}

\newcommand{\rset}[1] {rset(#1)}
\newcommand{\wset}[1] {wset(#1)}
\newcommand{\rvar} {readVar}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co\text{-}opacity\xspace}

\newcommand{\vwc} {VWC\xspace}
\newcommand{\lo} {LO\xspace}
\newcommand{\lopty} {LO\xspace}
\newcommand{\lopq} {locally-opaque\xspace}

\newcommand{\tab} {hash-table\xspace}
\newcommand{\set}{table\xspace}
\newcommand{\llist} {list\xspace}
\newcommand{\otm} {\textit{OSTM}\xspace}%{ObjSTM}
\newcommand{\sotm} {\textit{SV-OSTM}\xspace}%{ObjSTM}

\newcommand{\rwtm} {\textit{RWSTM}\xspace}
%\newcommand{\lotm} {Table-OSTM}
\newcommand{\lotm} {OSTMs\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\bst} {BST\xspace}
\newcommand{\lsl} {rblazy\text{-}list\xspace}
\newcommand{\lazy} {lazy-list\xspace}

\newcommand{\csr} {CSR\xspace}

\newcommand{\perm} {permissive\xspace}
\newcommand{\pness} {permissiveness\xspace}
\newcommand{\permfn}[1] {perm(#1)}

\newcommand{\sspec} {sequential-specification\xspace}
\newcommand{\samp} {sample-stm\xspace}

\newcommand{\cg}[1] {CG(#1)}

\newcommand{\uset} {updtSet\xspace}
\newcommand{\lset} {lookupSet\xspace}
\newcommand{\rvm} {\emph{rvm}\xspace}
%\newcommand{\ht} {\emph{hash table}}

\newcommand{\firste} {firstEvt\xspace}
\newcommand{\laste} {lastEvt\xspace}
\newcommand{\fevt}[1] {#1.firstEvt}
\newcommand{\levt}[1] {#1.lastEvt}

\newcommand{\fkmth}[3] {#3.firstKeyMth(#1, #2)}
\newcommand{\pkmth}[3] {#3.prevKeyMth(#1, #2)}

\newcommand{\bstu} {\emph{bst-update}}
\newcommand{\lllist} {locallog\_list}

\newcommand{\udset}[1] {updtSet(#1)}
\newcommand{\rvset}[1] {rvSet(#1)}
%\newcommand{\bst}{BST}

\newcommand{\refr}[1]{refNode(#1)}
\newcommand{\lin}[1]{#1.LP\xspace}

%\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\newcommand\tabspace[1][1cm]{\hspace*{#1}}

%%%%%%% DS macros
%\newcommand{\glslhead}{getLslHead($obj\_id \downarrow, key \downarrow$)}


%\newcommand{\txlfind} {\textup{translog.find\_in\_loclog}$(obj\_id \downarrow, key \downarrow)$}
\newcommand{\txgid} {txlog.getTid()}
%\newcommand{\txgllist} {txlog.getLlList($t_{i} \downarrow$)}
\newcommand{\txsetst}[1] {L\_txlog.setStatus($L\_txstatus \downarrow$, $ OK \downarrow$)}
\newcommand{\txbegin}[1] {begin(#1)}

%\newcommand{\lsls}[1] {list\_lookup($obj\_id \downarrow,  key \downarrow, knext \uparrow, value \uparrow$, #1)}

\newcommand{\rvvalidate} {rvValidate($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

%\newcommand{\lslins}[1] {lslIns($preds[] \downarrow$, $currs[] \downarrow$, #1)}
\newcommand{\lsldel} {lslDel($preds[] \downarrow$, $currs[] \downarrow$)}


%\newcommand{\rlsol} {releaseOrderedLocks($ordered\_ll\_list \downarrow$)}

\newcommand{\ctov} {commitTOValidation($ll\_entry_i \downarrow$)}
\newcommand{\rvtov} {rvTOValidation($ key \downarrow$, $curr \downarrow$)}
\newcommand{\toval} {toValidation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}
\newcommand{\validation} {validation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}


\newcommand{\ifvalidation} {$$\textup{interferenceValidation}$(preds[] \downarrow, currs[] \downarrow)$$}
%\newcommand{\handlea}{tryAbort($obj\_id \downarrow$)}

%\newcommand{\llsort}{ll.sort ($ll\_list \downarrow$)}

%%---------------------macro w/o parameter

\newcommand{\npctov} {\emph{commitTOValidation()}}
\newcommand{\nptov} {\emph{toValidation()}}
\newcommand{\npintv} {\emph{intraTransValidation()}}
\newcommand{\nptc} {\emph{STM tryC()}}
\newcommand{\npins} {\emph{STM insert()}}
\newcommand{\npdel} {\emph{STM delete()}}
\newcommand{\npluk} {\emph{STM lookup()}}
\newcommand{\nplsls} {\emph{list\_lookup()}}
\newcommand{\nplsldel} {\emph{lslDel()}}
\newcommand{\nplslins} {\emph{list\_Ins()}}
\newcommand{\npbegin} {\emph{STM begin}}
\newcommand{\nppoval} {\emph{lostUpdateValidation()}}
\newcommand{\tcins} {\emph{tryC_{ins}}}
\newcommand{\npcld}{\emph{commonLu\&Del()}}


\newcommand{\rn} {\textcolor{red}{RL}\xspace}
\newcommand{\bn} {\textcolor{blue}{BL}\xspace}

\newcommand{\rc} {\textcolor{red}{currs[0]}}
\newcommand{\bc} {\textcolor{blue}{currs[1]}}
\newcommand{\bp} {\textcolor{blue}{preds[0]}}
\newcommand{\rp} {\textcolor{red}{preds[1]}}


\newcommand{\eevts}[1] {#1.evts}
\newcommand{\hst}[1] {#1.hist\xspace}
\newcommand{\exec}[1] {#1.exec\xspace}
%\newcommand{\state}[1] {#1.state\xspace}
\newcommand{\alls}[1] {#1.allStates\xspace}
\newcommand{\pres}[1] {#1.pre\text{-}state\xspace}
\newcommand{\posts}[1] {#1.post\text{-}state\xspace}

\newcommand{\shist}[2] {#2.subhist(#1)}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subh}  {sub\text{-}history\xspace}

\newcommand{\preds} {G\_preds[]}
\newcommand{\currs} {G\_currs[]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mvotm} {\textit{MVOSTM}\xspace}
\newcommand{\mvotms} {\textit{MV-OSTM}\xspace}
\newcommand{\hmvotm} {\textit{HT-MVOSTM}\xspace}
\newcommand{\lmvotm} {\textit{list-MVOSTM}\xspace}
\newcommand{\hotm} {\textit{HT-OSTM}\xspace}
\newcommand{\kotm} {\textit{KOSTM}\xspace}
\newcommand{\hkotm} {\textit{HT-KOSTM}\xspace}
\newcommand{\lkotm} {\textit{list-KOSTM}\xspace}
\newcommand{\mvotmgc} {\textit{MVOSTM-GC}\xspace}
\newcommand{\hmvotmgc} {\textit{HT-MVOSTM-GC}\xspace}
\newcommand{\lmvotmgc} {\textit{list-MVOSTM-GC}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% Local %%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\llog} {txLog\xspace}

\newcommand{\txlfind} {$L\_txlog.find(L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow)$}
\newcommand{\txll} {$L\_txlog$}
\newcommand{\txllf} {$L\_txlog()$}
\newcommand{\llsopn}[1] {$L\_rec.setOpn(L\_obj\_id \downarrow$, $L\_key \downarrow$, #1)}
\newcommand{\llsval}[1] {$L\_rec.setVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}
\newcommand{\llsopst}[1] {$L\_rec.setOpStatus(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}

\newcommand{\llgopn}[1] {$L\_rec.getOpn(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsopn}[1] {$L\_getOpn((obj\_id \downarrow$, $key \downarrow$, #1)}

\newcommand{\llgval}[1] {$L\_rec.getVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsval}[1] {loclog.getVal($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llspc} {$L\_rec.setPred\&Curr(L\_obj\_id \downarrow$, $ L\_key \downarrow$, $G\_pred \downarrow$, $G\_curr \downarrow$)}

\newcommand{\llgaptc}[1] {$L\_rec.getAptCurr$(#1)}
\newcommand{\llgkeyobj} {$L\_rec.getKey\&Objid(L\_rec_{i} \downarrow$)}

\newcommand{\llgopst} {$L\_rec.getOpStatus(L\_obj\_id \downarrow$, $L\_key \downarrow$)}
%\newcommand{\llsopst}[1] {loclog.getOpStatus($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llgallpc}{$L\_rec.getAllPreds\&Currs(L\_rec_{i} \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}

\newcommand{\poval}{lostUpdateValidation($L\_rec_{i}\downarrow$, $preds[]\uparrow$, $currs[]\uparrow$ )}

\newcommand{\llsort}{$L\_txlog.sort$($L\_list \downarrow$)}

\newcommand{\txgllist} {$L\_txlog.getList(L\_t\_id \downarrow$)}

\newcommand{\cld}{$commonLu\&Del$($L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$)}
%%%%%%%%%%%%%%%%%%%% Global %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cnt} {G\_cnt}
\newcommand{\livetx} {live\_trans}
\newcommand{\gi} {$get\&inc(G\_cnt \downarrow)$}
\newcommand{\glslhead}{getListHead($L\_obj\_id \downarrow, L\_key \downarrow$)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%From MVTO%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}

\newcommand{\mv} {mv}
\newcommand{\rvf} {rvf}
\newcommand{\rt} {rt}
\newcommand{\rvmt} {rv\_method\xspace}
\newcommand{\upmt} {upd\_method\xspace}

%\newcommand{\op} {operation}
\newcommand{\checkv} {check\_versions}
\newcommand{\remid} {removeId}
\newcommand{\instup} {ins\_tuple}
\newcommand{\gc} {gc}
\newcommand{\liveset} {liveSet}
\newcommand{\livel} {liveList}
\newcommand{\locko} {lockOrder}
\newcommand{\mvto} {MV-OSTM}
\newcommand{\valid} {valid}
\newcommand{\seq}[2] {linearize(#2, #1)}
\newcommand{\stl}[3] {#3.stl(#1, #2)}
%\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\aco} {accessOrder}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% methods%%%%%%%%%%%%%%%%%%

\newcommand{\lsls}[1] {list\_lookup($L\_obj\_id \downarrow,  L\_key \downarrow, G\_pred \uparrow, G\_curr \uparrow$)}
\newcommand{\find} {find\_lts}
\newcommand{\handlea}{return ABORT}
\newcommand{\lslins}[1] {list\_Ins($G\_pred \downarrow$, $G\_curr \downarrow$, $node \uparrow$)}
\newcommand{\rlsol} {releaseOrderedLocks($L\_list \downarrow$)}

\newcommand{\mvperm} {mv-permissive\xspace}
\newcommand{\mvpness} {mv-permissiveness\xspace}

\newcommand {\cmnts}[1] {\State{\textcolor{gray}{/* #1 */} }}
\renewcommand{\thefootnote}{\arabic{footnote}}	

%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
\algrenewcommand{\algorithmiccomment}[1]{/* #1 */}

\newcommand{\stfdm} {starvation\text{-}freedom\xspace}
\newcommand{\stf} {starvation\text{-}free\xspace}
\newcommand{\wtfdm} {wait\text{-}freedom\xspace}
\newcommand{\wtf} {wait\text{-}free\xspace}
\newtheorem{assumption}{Assumption}

==> figs/pm.tex <==
\section{Proposed Mechanism}
\label{sec:pm}

\input{stardef}

\input{dsDesign}

\input{working}

==> figures.tex <==
\section{Designated Figures}
\label{sec:figs}


%\vspace{1cm}

\begin{figure*}
	\centerline{\scalebox{0.45}{\input{figs/sostm.pdf_t}}}
	\caption{Advantage of SF-OSTM over OSTMs}
	\label{fig:sostm}
\end{figure*} 

%\vspace{1cm}


%\vspace{5cm}



%\vspace{3cm}%


%\clearpage
\cmnt{
\begin{figure}[H]
	\centerline{\scalebox{0.6}{\input{figs/sfmv-correct.pdf_t}}}
	\caption{$wts$ violating the real-time order}
	\label{fig:wtsf}
\end{figure} 
}

%\clearpage
%\vspace{1.5cm}


==> resultsold.tex <==
%\vspace{-0.3cm}
\section{Experimental Evaluation}
%\section{Conclusion}
\label{sec:exp}

This section represents the experimental analysis of variants of the proposed starvation free object-based STMs (SF-OSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM)\footnote{Code is available here: https://github.com/PDCRL/SF-MVOSTM.} for two data structure hash table (HT-SF-OSTM, HT-SF-MVOSTM, HT-SF-MVOSTM-GC and HT-SF-KOSTM)  and linked-list (list-SF-OSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM) implemented in C++. We analyzed that HT-SF-KOSTM and  list-SF-KOSTM perform best among all the proposed variants of STMs. So, we compared our HT-SF-KOSTM with hash table based state-of-the-art STMs ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, RWSTM \cite [Chap. 4]{ WeiVoss:TIS:2002:Morg}, HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, HT-OSTM \cite{Peri+:OSTM:Netys:2018}, HT-KOSTM \cite{Juyal+:SSS:2018} and our list-SF-KOSTM with list based state-of-the-art STMs NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, list-OSTM \cite{Peri+:OSTM:Netys:2018}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, list-KSFTM \cite{Chaudhary+:KSFTM:Corr:2017}, list-KOSTM \cite{Juyal+:SSS:2018}.  
%For a fair experimental evaluation we have implemented all our proposed variations of starvation free object based STMs in C++, and we have compared the performance against all the existing state-of-the-art algorithms depending on whether their data-structure is hash-table or list. Our Hash-Table implementation of SF-OSTM, SF-MVOSTM, SF-MVOSTM-GC, and SF-KOSTM is compared with ESTM[1], RWSTM[2], MVTO[3], OSTM[4], KOSTM[5] and our list implementation is compared with NoRec[6], Translist[7], Boosting[8], OSTM[9], MVTO[3], OSTM[4], KOSTM[5].

\noindent
\textbf{Experimental Setup:} The system configuration for experiments is 2 socket Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 14 cores per socket and 2 hyper-threads per core, for a total of 56 threads. A private 32KB L1 cache and 256 KB L2 cache is with each core. It has 32 GB RAM with Ubuntu 16.04.2 LTS running Operating System. Default scheduling algorithms of Linux are used in our experiments, where all threads have the same base priority. This allows \asmref{bdtm}(bounded-termination) to hold and we ensure the absence of parasitic transactions for our setup that satisfies \asmref{self}. %(bounded-termination) to hold. We completely ensure that no parasitic transactions[10] exists in our setup.

\noindent	
\textbf{Methodology:} Irrespective of underlying data structures (hash table and linked-list) the methodology for our experiments remain same. We have considered three different types of workloads namely, W1 (Lookup Intensive (Li)- 8\% Insert, 2\% Delete, and 90\% Lookup), W2 (Mid Intensive (Mi) - 25\% Insert, 25\% Delete, and 50\% Lookup), and W3 (Update Intensive (Ui) - 45\% Insert, 45\% Delete, and 10\% Lookup) respectively. To analyze the absolute benefit of starvation-freedom we used a customized application called as the Counter application which provides us flexibility to create a high contention environment where the probability of transactions undergoing starvation on an average is very high. Our high contention environment includes only 30 keys, number of threads ranging from 50 to 250, each thread spawns upon a transaction, where each transaction performs 10 operations (Insert, Delete and Lookup) depending upon the workload chosen. To study starvation-freedom of various algorithms, we have used \emph{max-time} which is the maximum time required by a transaction to finally commit from its first incarnation, which also involves time taken by all its aborted incarnations. We perform each of our experiments 10 times and considered the average of these runs in order to avoid the effect of outliers. 


%\vspace{1.5cm}
\begin{figure}
	\includegraphics[width=12cm, height=5cm]{figs/htli-comp.pdf}
	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on hash table}
	\label{fig:htcomp}
\end{figure}


%\vspace{1.5cm}
\begin{figure}
	\includegraphics[width=12cm, height=5cm]{figs/List-comp.pdf}
	\caption{ Performance analysis of SF-KOSTM and State-of-the-art STMs on list}
	\label{fig:listcomp}
\end{figure}
%\vspace{1.5cm}

%\vspace{1.5cm}


\noindent
\textbf{Results Analysis:} All our results reflect the same ideology as proposed showcasing the benefits of starvation-free multi-version object based STMs. We started our experiments with hash table data structure of bucket size 5 as shown in \figref{htus}. First, we compared all our proposed HT-SF-OSTM and variations of HT-SF-MVOSTM which are HT-SF-MVOSTM, HT-SF-MVOSTM-GC (due to lack of space please find the implementation details in the \apnref{ap-result}), and HT-SF-KOSTM to find the best out of the all. \figref{htus} depicts that the finite version HT-SF-KOSTM performs best among all the proposed algorithms on all the three types of workloads (W1, W2, and W3) with value of $K$ and C as 5 and 0.1 respectively. Where $K$ is the number of versions in the version list and C is the variable used to define the $wts$. So, we chose the HT-SF-KOSTM to compare against rest state-of-the-arts STMs with hash table data structure. \figref{htcomp} shows that HT-SF-KOSTM takes minimum \emph{max-time} for a transaction to commit, and achieved an average speedup of 3.9x, 32.18x, 22.67x, 10.8x and 17.1x over HT-KOSTM, HT-OSTM, ESTM, RWSTM and HT-MVTO respectively.

We further considered another data structure the linked-list and compared among all our proposed variants list-SF-OSTM, list-SF-MVOSTM, list-SF-MVOSTM-GC and list-SF-KOSTM. \figref{listus} represents that list-SF-KOSTM performs best for all the workloads. So, in a next genuine step, we compared list-SF-KOSTM with rest state-of-the-arts STMs  and observed that list-SF-KOSTM beats all other algorithm by taking the minimum $max-time$ on an average for a transaction to commit under high contention, high starving environment as shown in \figref{listcomp}. list-SF-KOSTM achieved an average  speedup of 2.4x, 10.6x, 7.37x, 36.7x, 9.05x, 14.47x, and 1.43x over list-KOSTM, list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO and list-KSFTM respectively.



In all our experiments, we have taken value of K as 5 and value of C as 0.1 which we found are the optimal values by experimenting and tuning these hyper-parameters across different workloads for hash table and linked-list as shown in \figref{htck} (a), (b) and \figref{listck} (a), (b) respectively. Additionally, we perform experiments to analyze the stability of our algorithm. By \textit{stability} we refer to the number of transactions committed should be approximately same in increasing time intervals where each thread performs relatively large number of transactions. \figref{htck} (c) and \figref{listck} (c) displays that number of committed transactions are almost consistent in HT-SF-KOSTM and list-SF-KOSTM for all the workloads while varying time interval and considered 5 seconds as warm-up period. This shows indeed that algorithm proposed here is stable.  Please refer the \apnref{ap-result} for further experiments which involve performance of HT-SF-KOSTM and list-SF-KOSTM under low contention and number of aborts with varying number of threads.
